CacheGen: KV Cache Compression and Streaming for Fast Large Language Model Serving

As large language models (LLMs) take on complex tasks, their inputs are supplemented with longer contexts that incorporate domain knowledge. Yet using long contexts is challenging, as nothing can be generated until the whole context is processed by the LLM. While the context-processing delay can be reduced by reusing the KV cache of a context across different inputs, fetching the KV cache, which contains large tensors, over the network can cause high extra network delays. CacheGen is a fast context-loading module for LLM systems. First, CacheGen uses a custom tensor encoder, leveraging KV cache's distributional properties to encode a KV cache into more compact bitstream representations with negligible decoding overhead, to save bandwidth usage. Second, CacheGen adapts the compression level of different parts of a KV cache to cope with changes in available bandwidth, in order to maintain low context-loading delay and high generation quality. % When available bandwidth drops, CacheGen may raise the compression level for a part of the context or recompute its KV cache on the fly. We test CacheGen on popular LLMs and datasets. Compared to the recent systems that reuse the KV cache, CacheGen reduces the KV cache size by 3.5-4.3x and the total delay in fetching and processing contexts by 3.2-3.7x with negligible impact on the LLM response quality. Our code is at: https://github.com/UChi-JCL/CacheGen.

==> F/fig-example.tex <==

\begin{figure}[t]
\centering
    \includegraphics[width=.55\textwidth]{figs/improv.pdf}
    \vspace{-0.2cm}
    \tightcaption{\name's gains over the best baseline across different workloads (\ie Bandwidth throughput, GPU utilization).
    \yh{Putting this for now, let's polish later}
    }
    \yh{Better visualization. linear scale. Only need the number for a long input? rent a cloud instance for longer input? }

    \label{fig:resource}
\end{figure}



==> F/offline/fig-offline.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.8\columnwidth]{F/offline/storage.pdf}
    \tightcaption{}
    \label{fig:offline}
\end{figure}



==> backups/1-introduction-0130.tex <==
\begin{itemize}
\item Generative models have become extremely popular recently (list popular generative models-based applications, and specifically the popularity of Transformer-based models)
\item \jc{need a para here to highlight the importance of the metric of "time to first token" (TTFT). what it is and why it's crucial for user experience. and then the next para should start with "while TTFT is crucial, it's in conflict with another important trend of xxx"}
\item Those Transformer-based generative models need to take in a lot of history input from the users into consideration
\begin{itemize}
\item Use a concrete example: in one ChatGPT session, a user asks a question ``Consider the example generated in the previous question, how to ...''. Without considering the previous question and response generated in the session, it will be very hard for the model to output meaningful answer 
\item List innovative ways to use GPT, like AutoGPT to show emerging applications require long history input

\jc{need a couple of NON-GPT and non-NLP examples. otherwise, the paper seems quite narrow for HotNets}
\end{itemize}
\item \jc{more history tokens $\rightarrow$ longer TTFT} The self-attention operation's compute complexity is $O(n^2)$ where $n$ is the number of history tokens; 
\item To alleviate the cost of self-attention, \jc{many} previous works propose caching the attention vectors \jc{in various forms} calculated for history tokens. \jc{this should be a para on itself, and it should define what ``history state'' means}
\item \jc{these prior efforts assume the cached data is already stored in GPU memory and thus can be immediately used, but in reality, the cached data may be stored in different locations than the inference model for multiple reasons. mobile users may connect to different edge servers over time. a model may use a cached history state from several hours/weeks ago. different users cached history state may be reused. etc} 
\item \jc{therefore, before implementing a new system that manages and distributes history states, we should first answer some basic questions (this is our first contribution): what are the basic design choices for caching transformer states? how much data should be cached? how much delay budget to load cached states to maintain a low TTFT?} the question of when and how to cache history tokens, and what's the challenges when the cached data is stored in distributed locations remains unanswered. 
\item \jc{inspired by these measurements, we examine a several potential optimizations to allow low TTFT even in distributed setting.}
% In this paper, we profiled the benefits of caching history tokens on a wide range of generative tasks, and present the challenges of storing and fetching cached history from distributed servers.
    % \item Generative models have become extremely popular recently (list popular generative models-based applications, and specifically the popularity of Transformer-based models)
    % \item However, those Transformer-based generative models usually suffer from high inference delay (list some example numbers)
    % \item We first perform a systematic measurement study to identify the computation bottleneck of Transformer-based generative models. We show that the self-attention operation's delay will grow quadratically with the number of input tokens.  
    % \item Although the generative models suffer from high inference delay, many generative-models-based applications share one unique property: the users continuously interact with the models 
    % \item The interactive property for generative models allows caching historically seen context.
    % \item In this paper, we prototyped an inference system for Transformer-based generative models, and show the benefits of caching history data in terms of reduction in inference delay with a wide range of generative tasks, including text, code, music and video generation. 
\end{itemize}

==> backups/1-introduction-0927.tex <==
\label{sec:intro}

\subsection{Motivation}
Nowadays, there have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the images. Due to the heavy burden of designing and training such DNNs, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}. However, the generic ML APIs might not be able to solve the tasks that the software intends to perform. 

When the service providers design the ML APIs, their goal is mainly to improve traditional class-wise accuracy metrics (\ie high average recall and precision)~\cite{wang2020multi} over all classes for large-scale datasets. However, when developers employ the ML APIs in their software, they care about whether ML APIs' outputs match their expectations (\ie as if the ML APIs' outputs are exactly the ground-truth labels). This gap in service providers' and software developers' purposes can lead to many software mis-behaviors, thus model adaptation is needed to provide a customized model that reduces software mis-behaviors as much as possible.





% Therefore, there is a need to adapt the ML APIs to directly optimize for producing correct software behaviors \cc{``ML APIs are xxx, while software are xxxx. Therefore, there is a need to adapt xxx''} 

To understand how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors, we take the software application Smart can in Figure~\ref{fig:app_example} as an example. This application defines three lists to classify trash into categories. It calls Google's multi-label classification API to get the labels that describe the content in the image. The application then compares the output labels, ranked with descending order of confidence scores, with the three lists and returns the corresponding judgment if the outputs intersect with one of the lists. 
% goes through the output labels, and executes a branch if an output label is included in its corresponding pre-defined list. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with a highly reliable ML API. For example, consider an input image (trash\_image) with ground-truth labels specified in the figure. The multi-label classification API returns an ordered list of labels, ranked in descending order of confidence scores. If we measure the outputs according to traditional recall and precision, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software.  
According to the ground-truth labels, the correct branch to be executed is the one that returns ``This belongs to Compost'', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``This belongs to Recycle. ''

% where its ground-truth labels include \emph{['Alcoholic beverage', \textcolor{red}{``Glass''}, 'Cocktail', 'Liqueur', 'Stemware'] }, and the API outputs are \emph{['Stemware', \textcolor{cyan}{``Food''}, 'Cocktail', 'Alcoholic beverage', 'Liqueur', 'Wine', \textcolor{red}{``Glass''}]}\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}
% Reader have to work hard to understand what is going on here }. This output yields a per-example recall of 100\% and precision of 71.5\%, while this prediction will be considered completely wrong from the view of the software. To be more specific, the correct branch to be executed, according to the ground-truth labels, should be \textcolor{red}{Recycle}. However, the labels generated by the ML API will lead to executing the branch which returns Compost. 
% \cc{This is not reason, but a detailed version of ``software considers it wrong''. Maybe use another way to describe this fact. Also, ``human-labeled ground-truth label'' and ``expected'' seem come out of blue. Suddenly human appears, and there is an expectation. You may just say the correct branch is xxx, according the ground-truth label} 

% This example demonstrates a common pattern of the mismatch between the generic tasks that the ML APIs are designed for and the specific tasks the software intends to perform. 
This is not the only case where the ML APIs' outputs lead to wrong software behaviors. When the software developers use the ML APIs in specific scenarios (\eg performing garbage classification), errors made by the ML APIs have different levels of severity: errors that lead to wrong software behaviors are more damaging than others. For example, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that are not included in the pre-defined lists associated with wrong program branches. 
Thus, an ideal solution for using ML APIs in the software is to customize the DNNs behind the ML APIs to reduce the errors that lead to wrong software behaviors. 
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

Automatically adapting the ML APIs has many challenges. 

\begin{itemize}

\item First, automatic model adaptation is hard. We need to infer the software-specific task from the software. The software developers did not explicitly specify the specific tasks they are performing and are not able to specify the specific tasks in the format that can be directly used to optimize the DNNs behind the ML APIs. 

% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\item Secondly, model adaptation needs to be very efficient. As the software developers typically lack the computation resources to perform model training, model adaptation has to happen on the cloud service providers' side. Thus, it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   
\end{itemize}
Existing works have performed model customization in different scenarios. 
They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
   \centering
\begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['plastic', 'wood', 'glass', 'paper', 'cardboard', 'metal', 'aluminum', 'tin', 'carton']
Compost = ['food', 'produce', 'snack']
Donate = ['clothing', 'jacket', 'shirt', 'pants', 'footwear', 'shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
  if obj.name in Compost:
    return 'It is compostable.'
  if obj.name in Donate:
    return 'It is donatable.'
\end{lstlisting}
\includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \caption{Heapsortcypher, a smart can application \cite{xxx} using Google Cloud API.}
    \label{fig:app_example}
    
\end{figure}
\subsection{Contributions} 
\begin{itemize}
%  \item We present \tool, which is an end-to-end system which automatically extracts software context from the applications that incorporate ML APIs, and adapt the ML models to improve the software accuracy. 
\item Studied a wide range of software applications that incorporate image classification APIs, and identified that one of the common software-specific tasks is mapping fine-grained ML API output classes to program branches. 
\item Automatically extracts the software-specific task from the code the software developers write, and transforms it into a mathematical expression that can adapt the ML APIs to the software. 
% Defined a template to automatically transform the code that the software developers write into mathematical expression that can adapt the ML APIs to the software. 
% \item defined the template and the transformation to math expression 
\item Leveraged two ways of model adaptation with the defined software context that (1) changes the training data distribution to reflect the subset of classes that the users care about; (2) modifies training loss function to directly optimize for the software-specific task. 
% \item Compared the ways of model adaptation in terms of accuracy improvement and training cost on \todo{X} real applications using ML APIs.

% defined two types of software context that can improve the accuracy of the software: (1) Data distribution context; (2) Subset of classes context. 

% \item Developed a tool to automatically extract the defined context from the Python code written by software developers 


\end{itemize}

==> backups/1-introduction-1004.tex <==
\label{sec:intro}

% \subsection{Motivation}

% \kt{It is not common to put subsections inside introduction (I'm not sure if it is common in SE community though)}
Nowadays, there have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the input. Due to the heavy burden of designing and training such DNNs
% \kt{need citations here}
, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}.  However, the generic ML APIs with good accuracy might lead to misbehaviors when applied to the software.
% \kt{The argument ``the software misbehavior is because that APIs are agnostic to software'' is an important argument and it directly leads to your key contribution. You bring this point too quick without much support, making this argument sounds trivial. I would suggest we postpone the mentioning of this point and just say a general ML API with good performance can lead to a lot of software behavior.}
% \yh{example: use the figure 1 example }
% \yh{existing works cost reduction by leveraging e.g., model compression 

% correct software misbehaviors by improving the ml models  =>  }

To illustrate how ML APIs with good accuracy may lead to software misbehaviors,
% how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors,
% \kt{Maybe discribe the software behavior following the processing order of the software, like input -> API -> labels -> list -> output}
we take the software application \emph{Heapsortcypher} in Figure~\ref{fig:app_example} as an example. The application takes an image as input, and calls Google's multi-label classification API to get the labels that describe the content in the image. This application then goes through a post-processing step which classifies the ML APIs' outputs into categories of garbage. The application pre-defines three lists, \emph{Recycle, Compost, and Donate}. It then checks the output labels (\eg [Glass, Candy, Snack, Confectionery, Lollipop]), ranked with descending order of confidence scores, and searches for the first label (\eg Glass) that matches any of the labels in the three pre-defined lists. Then it executes the branch that corresponds to the found pre-defined list (\eg the one that outputs returns ``It is recyclable. '').
% the corresponding judgment if the outputs intersect with one of the lists. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with an ML API that is able to correctly identify most of the classes.
% \kt{80\% recall does not sound like highly reliable. Also, ``highly reliable'' is vague. Maybe just say ``even when the ML API correctly identifies most of the classes''.} 
 Figure~\ref{fig:app_example2} shows a concrete example of how \emph{Heapsortcypher} works.  
% \cc{Maybe directly say that ``the bottom of Figure 1 shows a concrete example'', instead repeating what we have introduced earlier} 
 Given the outputs of the ML API, if we use traditional recall and precision as the metrics~\cite{wang2020multi}, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software. 
According to the ground-truth labels, the correct branch to be executed is the one that returns ``It is compostable. '', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``It is recyclable. '' \kt{From a system guy's perspective, I guess it is better  to highlight the cost of such software misbehavior. I'm not sure if this is needed in SE conference though.}
% \cc{P4 \& 5 have duplicate description}
%\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}
% Reader have to work hard to understand what is going on here }. This output yields a per-example recall of 100\% and precision of 71.5\%, while this prediction will be considered completely wrong from the view of the software. To be more specific, the correct branch to be executed, according to the ground-truth labels, should be \textcolor{red}{Recycle}. However, the labels generated by the ML API will lead to executing the branch which returns Compost. 
% \cc{This is not reason, but a detailed version of ``software considers it wrong''. Maybe use another way to describe this fact. Also, ``human-labeled ground-truth label'' and ``expected'' seem come out of blue. Suddenly human appears, and there is an expectation. You may just say the correct branch is xxx, according the ground-truth label} 

% This example demonstrates a common pattern of the mismatch between the generic tasks that the ML APIs are designed for and the specific tasks the software intends to perform. 
\kt{It is a cool empirical finding. The current way of giving this point is a bit too direct, and unintentionally trigger the reader to downplay the importance of this finding. Maybe back this finding up with more empirical evidence.} \yh{systematically find on Github}
This example represents a common usage pattern of ML APIs in software: developers specify a subset of labels that they care about in the specific application, such as the classes in different garbage categories, and how they plan to use the labels, such as which sets of labels trigger the same program branches. Under such usage patterns, ML API mis-predictions can have different levels of severity: errors that lead to wrong software behaviors are more damaging than others.\kt{You are somewhat downplaying an important new point (errors have different severity) by ``hiding'' it inside the para that seems to introducing the common usage pattern of ML API. Make this point clear by giving it a new paragraph.}  
% \cc{need connection. This example represents a common usage pattern of ML API:xxxx. Under such usage pattern, ML API mis-prediction have different level of damages to the software. xxx (not all API errors would lead to failure)}
For example, when the developer write the code as shown in Figure~\ref{fig:app_example}, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that do not affect the behavior of the software. 


\kt{Maybe contrast this design point with the one-size-fit-for-all design point.}Thus, an ideal solution for using ML APIs in the software is to customize the DNNs such that they are aware of the errors that lead to software misbehaviors. On this front, we want to 
% \cc{``we want''. It's still the motivation section, not contribution} 
re-train the DNNs behind the ML APIs with a re-constructed loss function that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).  
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% \kt{As I learned from Junchen, in general, when introducing related works, it is better to suggest what we are going to do, but do not say it directly.}
Existing work proposes solutions to improve ML models on specific tasks without the knowledge of the software. 
% \kt{Adapting ML models sounds a bit abrupt. Maybe say ``existing work improves the performance of ML API by adapting the ML model.}
% \kt{Also, for me it feels early for us to mention ``optimizing without the knowledge of the software'' as the definition and importance of software knowledge is unclear here.}
% One line of work customizes the DNNs based on run-time data statistics and still optimizes for the same tasks (\eg image classification)~\cite{kim2021pool, cao2021thia, anderson2019physical}. Another line of work trains specialized models performing the tasks specified through a subset of SQL queries, such as aggregation and limit ~\cite{kang2018blazeit, kang2017noscope}.

\kt{Saying that we are targeting a different problem sounds like we are not picking the correct related work for our problem. Maybe try to say previous work are solving the same problem with the wrong assumption.}
However, we are tackling a different problem than these prior work. Firstly, as software developers typically write Python code to use the ML APIs, instead of declarative\kt{declarative is a ``noise'' here. It's better for us to focus on the popularity of the language here.} languages such as SQL.\kt{Previous work use SQL is not immediately clear to the reader.}
Second of all, the operations that can be expressed in SQL queries that the prior work optimizes for are limited (\eg aggregation, limit)\kt{People tend to not directly care about the limit of operations. Maybe link to what people care, like SQL limits what the \textbf{software can do}, and give a real (at least seemingly real) example to convince people a true need of software cannot be expressed by SQL.}, while there are a wider range of operations that can be expressed by Python. For example, aggregation or limit queries cannot specify subsets of labels can have the same effects on the final program behaviors. Thirdly, in order to use the these systems that optimize for SQL queries, users need to translate their code into SQL queries, which incurs an extra development burden for the users.\kt{For me, this point is essentially the same as the first point. The effect of choosing a programming language that people don't use is forcing the user to ``tranlate'' their code to another language.} Lastly, these approaches cannot guide the ML APIs to produce outputs that lead to correct software behaviors\kt{Personally I feel like this is the most fundamental reason. Putting it at the last is kind of downplaying this point.}\kt{I guess maybe you are referring that these works cannot fix the misbehavior of the software as they are just compressing the model, not improving the model. ``Software behavior'' and ``ground-truth labels'' are noise.} (\ie as if the ground-truth labels are returned), as they only optimize for inference delay. 

% When the service providers design the ML APIs, their goal is mainly to improve traditional class-wise accuracy metrics (\ie high average recall and precision)~\cite{wang2020multi} over all classes for large-scale datasets. However, when developers employ the ML APIs in their software, they care about whether ML APIs' outputs match their expectations (\ie as if the ML APIs' outputs are exactly the ground-truth labels). This gap in service providers' and software developers' purposes can lead to many software mis-behaviors, thus model adaptation is needed to provide a customized model that reduces software mis-behaviors as much as possible.


\kt{Maybe contrast this design point with the one-size-fit-for-all design point.}Thus, an ideal solution for using ML APIs in the software is to customize the DNNs such that they are aware of the errors that lead to software misbehaviors. On this front, we want to 
% \cc{``we want''. It's still the motivation section, not contribution} 
re-train the DNNs behind the ML APIs with a re-constructed loss function that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).  
% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

Automatically adapting the DNNs behind ML APIs to fit the software's need has many challenges. 

\begin{itemize}

\item First, automatic model adaptation is hard. We need to automatically extract information embedded in the code structure that indicates how the software plans to use the labels. We also need to transform the information extracted from the software into loss functions that can directly be applied to optimize the DNNs. 


% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\item Secondly, model adaptation needs to be very efficient. Given how the interface of the ML APIs is designed, the software developers who call the ML APIs are not able to adapt the DNNs behind the ML APIs. Thus, model adaptation has to happen on the cloud service providers' side, and it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   
\end{itemize}
% Existing works have performed model customization in different scenarios. 
% They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
\begin{subfigure}{0.45\textwidth}    
         \centering
         \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['plastic', 'wood', 'glass', 'paper', 'cardboard', 'metal', 'aluminum', 'tin', 'carton']
Compost = ['food', 'produce', 'snack']
Donate = ['clothing', 'jacket', 'shirt', 'pants', 'footwear', 'shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
    if obj.name in Compost:
    return 'It is compostable.'
  if obj.name in Donate:
    return 'It is donatable.'
    \end{lstlisting}
\subcaption{The software implementation}
\label{fig:app_example}
% \includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \end{subfigure}
 \hfill
    \begin{subfigure}{0.45\textwidth}  
        \includegraphics[width=\linewidth]{figs/app_example2.pdf}
        \subcaption[]{A concrete example. }
        \label{fig:app_example2}
    \end{subfigure}
    \caption{Heapsortcypher, a garbage classification application \cite{heapsort} using Google Cloud API.}
\end{figure}

\subsection{Contributions} 
 We present \tool, which helps the cloud service providers, who offer the ML APIs, to automatically adapt the ML APIs to the applications the developers write. 

To understand common tasks software developers intend to perform, we conduct an empirical study on the applications using Google's \code{label\_detection} in a recently published benchmark suite studying ML software~\cite{wan2021machine}, a multi-label image classification API. We focus on 19 applications whose control flow decisions are affected by ML APIs' outputs, for example, the software will print out a warning if the outputs contain ``Gun'' or ``Fire'', and do nothing otherwise. We found that a common pattern of the code structures for these applications is triggering the same program actions for sets of labels, such as returning the same message for labels specified in the same pre-defined list. For example, labels specified in the \emph{Compost} list, including ``Food'', ``Produce'', and ``Snack'', triggers the same program behavior (\ie returning the message ``This is recyclable''). However, different applications have different specific ways of triggering program behaviors based on pre-defined lists. We generalized three levels of abstraction from the code structures of the applications in the benchmark suite: (1) labels that will trigger the same program behaviors; (2) whether the final program output is exclusively 
 
\begin{itemize}

\item Perform program analysis to extract the information needed to perform model adaptation, including the subset of labels that the software cares about, and the sets of labels that are considered equivalent by the software. We also re-constructed loss functions using the extracted information to directly reflect the damaging errors that are not acceptable by the software. 
% Defined a template to automatically transform the code that the software developers write into mathematical expression that can adapt the ML APIs to the software. 
% \item defined the template and the transformation to math expression 
\item Re-train the DNNs behind the ML APIs with the re-constructed loss function, and systematically measure the improvement in the rate of software mis-behaviors on \todo{X} open-source applications invoking ML APIs. 
% \item Compared the ways of model adaptation in terms of accuracy improvement and training cost on \todo{X} real applications using ML APIs.

% defined two types of software context that can improve the accuracy of the software: (1) Data distribution context; (2) Subset of classes context. 

% \item Developed a tool to automatically extract the defined context from the Python code written by software developers 


\end{itemize}

==> backups/1-introduction-1106.tex <==
\label{sec:intro}

\subsection{Motivation}
\kt{I would suggest listing the first sentence of each para as bullet points here. It is important to iterate on the structure and the logic (instead of the language details) first.}

% \kt{It is not common to put subsections inside introduction (I'm not sure if it is common in SE community though)}
% \begin{itemize}
%     \item increasing number of software applications use off-the-shelf ML APIs to understand what is present in the input. However, the generic ML APIs with good accuracy might make small mistakes leading to software misbehaviors
%     \item Illustrate how small mistakes could lead to software misbehaviors with the application example 
%     \item This 
% \end{itemize}
There have been an increasing number of software applications with the need of deploying deep neural networks (DNNs) to understand what is present in the input. Due to the heavy burden of designing and training such DNNs
% \kt{need citations here}
, many software developers use off-the-shelf machine learning (ML) APIs provided by many cloud service providers (\eg Google, Microsoft, Amazon) to reduce their development effort~\cite{wan2021machine}.  However, the accuracy of generic ML APIs misaligns with software correctness\shan{This sentence needs rewording. Not clearly what it tries to deliver.}. 
% \kt{The argument ``the software misbehavior is because that APIs are agnostic to software'' is an important argument and it directly leads to your key contribution. You bring this point too quick without much support, making this argument sounds trivial. I would suggest we postpone the mentioning of this point and just say a general ML API with good performance can lead to a lot of software behavior.}
% \yh{example: use the figure 1 example }
% \yh{existing works cost reduction by leveraging e.g., model compression 

% correct software misbehaviors by improving the ml models  =>  }

To illustrate how ML APIs with good accuracy may lead to software misbehaviors\shan{This opening sentence is a bit odd: it seems to fit our OOPSLA submission better, don't you think so? Furthermore, even with your tool and ML APIs with increased accuracy, the software may still misbehave, right?},
% how and why optimizing class-wise accuracy does not necessarily lead to the correct software behaviors,
% \kt{Maybe discribe the software behavior following the processing order of the software, like input -> API -> labels -> list -> output}
we take the software application \emph{Heapsortcypher} in Figure~\ref{fig:app_example} as an example. It takes a trash image as input, and invokes \code{label\_detection}, Google's multi-label classification API, to get the labels that describe the content in the image. It then goes through a post-processing step which classifies the ML APIs' outputs into categories of garbage. Heapsortcypher pre-defines three lists, \emph{Recycle, Compost, and Donate}. It checks the output labels (\eg [Glass, Candy, Snack, Confectionery, Lollipop]), ranked with descending order of confidence scores, and searches for the first label (\eg Glass) that matches any of the labels in the three pre-defined lists. Finally it executes the branch that corresponds to the found pre-defined list (\eg the one that outputs returns ``It is recyclable. '').
% the corresponding judgment if the outputs intersect with one of the lists. 

% and 
% then performs a post-processing step which executes one of \emph{Recycle, Compost, } and \emph{Donate} branches if the output labels contain any of the keywords specified in the pre-defined list \code{Recycle, Compost, Donate} \cc{``the pre-defined list'', you need to explain what is recycle, as it means a branch in the last reference} .


This simple post-processing step incurs potential software mis-behaviors even with an ML API that only mis-classifies one class, as shown in Figure~\ref{fig:input_example_top_wrong}.
% \kt{80\% recall does not sound like highly reliable. Also, ``highly reliable'' is vague. Maybe just say ``even when the ML API correctly identifies most of the classes''.} 
% Figure~\ref{fig:app_example2} shows a concrete example of how \emph{Heapsortcypher} works.  
% \cc{Maybe directly say that ``the bottom of Figure 1 shows a concrete example'', instead repeating what we have introduced earlier} 
% Given the outputs of the ML API, if we use traditional recall and precision as the metrics~\cite{wang2020multi}, this output yields a recall of 100\% and a precision of 80\%. Nevertheless, this output is completely wrong from the view of the software. 
% According to the ground-truth labels, the correct branch to be executed is the one that returns ``It is compostable. '', since the only intersection between the ground-truth labels and the three lists is the one associated with the \emph{Compost} branch. However, the API's outputs lead to the program executing the branch which returns ``It is recyclable. '' 
Given a candy image, the ML API wrongly returns the label ``Glass''. This mistake is minor in terms of the multi-label classification task~\cite{wang2020multi}: it  finds all the objects in the input image while recognizing an extra wrong object ``Glass'', providing a recall of 100\% and a precision of 80\%\shan{I don't understand how you get these numbers: 100\% and 80\%.}. However, it leads to a completely wrong software behavior. While this image belongs to \emph{compostable} branch, the software wrongly executes the \emph{recyclable} branch as \code{Recycle} list contains the first API output label ``Glass''.

\shan{After I finished reading the above two paragraphs, I finally saw what you are trying to tell the readers. I guess you are trying to say that not all mistakes of an ML API are equally important for a software application. Is that what you are trying to say? You need to clearly present what messages you want to deliver BEFORE you present examples. You cannot ask readers to summarize/infer what you mean AFTER they read the example.}


% \cc{I changed the description. Please proof read}

% \kt{From a system guy's perspective, I guess it is better  to highlight the cost of such software misbehavior. I'm not sure if this is needed in SE conference though.}
% \cc{P4 \& 5 have duplicate description}
%\cc{Maybe create a figure with a concrete image example and show the list (use color to show overlaps). 
% \yh{}

% \kt{It is a cool empirical finding. The current way of giving this point is a bit too direct, and unintentionally trigger the reader to downplay the importance of this finding. Maybe back this finding up with more empirical evidence.}
\kt{I would expect you saying this type of error is a common error. People do not directly care about the common usage pattern of ML API.}
% This example represents a common error pattern of applying ML APIs in software: developers specify a subset of labels that they care about, such as \code{Recycle}, \code{Compost}, and \emph{Donate} lists, and how they use the labels, such as these three lists correspond to three software branches. 
% We perform an empirical study to study the common patterns of the applications in the benchmark suite~\cite{wan2021machine}, focusing on the applications whose program behaviors are affected by the ML APIs' outputs\footnote{We study these applications as they reflect non-trivial ways of using ML APIs. If the applications directly return the APIs' outputs, they do not provide extra information for us to perform adaptation. }. We find that it is common for applications to pre-define one or more lists of labels, and execute different branches by comparing the output labels with the lists. \kt{People may wonder what happened to the remaining 40\% applications.} 
% \kt{It would be better to separate these two important points {\footnotesize (This pattern is common \& mispredictions have different levels of severity)} into two paragraphs.}
This example represents a common phenomenon in ML software. The reason is that the ML APIs are optimized for generic accuracy over a large number of classes, but the ML software has a different focus and priority: it cares about whether the ML API can produce outputs leading to correct control flow decisions\shan{I think it is a bit too early to mention control flow here. Please think and rephrase.}. 

The way the ML software is typically written can cause accurate ML APIs' outputs to lead to wrong control flow decisions\shan{?????What? Am I in the wrong paper? This sentence seems to fit our OOPSLA submission but does NOT fit here AT ALL. Your example so far is about wrong API result; it is NOT about accurate API result that leads to software failure. I am very confused.}. Specifically,  developers usually specify a subset of labels that they care about, such as \code{Recycle}, \code{Compost}, and \emph{Donate} lists, and how they use the labels, such as these three lists correspond to three software branches. Under such code patterns, ML API mis-predictions have different levels of severity: errors that lead to wrong software behaviors are more damaging than others\shan{No, it is not about which one is more damaging. Some mis-prediction simply has NO damage at all. Right?}. For example, in Heapsortcypher, the confusion within the lists, such as misclassifying a ``Food'' image to ``Produce'', is less damaging \shan{Again, when you say ``less damaging'', you are implying there exists some damage. But, that is not true here. mis-classifying food to produce has no damage to the software at all!} than across the list, such as misclassifying a ``Food'' image to ``Glass'', as only the latter would lead to a wrong control flow decision.



% Under such code patterns, ML API mis-predictions have different levels of severity: errors that lead to wrong software behaviors are more damaging than others. For example, in Heapsortcypher, the confusion within the lists, such as misclassifying a ``Food'' image to ``Produce'', is less damaging than across the list, such as misclassifying a ``Food'' image to ``Glass'', as only the latter would lead to a wrong execution path.
% \cc{Please explain the effect of mis-classification inside list and outside list} \yh{Done}
% \kt{You are somewhat downplaying an important new point (errors have different severity) by ``hiding'' it inside the para that seems to introducing the common usage pattern of ML API. Make this point clear by giving it a new paragraph.}  
% For example, when the developer write the code as shown in Figure~\ref{fig:app_example}, false positives that lead to the program executing the wrong program branches, such as the ``Glass'' prediction that leads to the Recycle branch, are more devastating than false positives that do not affect the behavior of the software. 


% \kt{Maybe contrast this design point with the one-size-fit-for-all design point.}
% \kt{``customize the DNNs'' is a surprise. Maybe give more rationales to justify why customizing DNN instead of something like redesigning the API interface.}
% \cc{Be aware of software behavior? aim to improve software correctness?} \yh{Done} \kt{This issue is not solved yet. I guess Chengcheng questions these two things because they are vague. Maybe try to answer what kind of concrete software behavior are you aim to improving/what is software correctness/what kind of software correctness are you trying to improve.}

Thus, instead of providing a generic ML API that could be applied to all software, an ideal solution is to customize the DNNs behind ML API for each software, while keeping the same interface\shan{How do you define interface? If you really keep the same interface, how do you collect the software control flow information for the API provider?}. In this way, the ML API is aware of how the ML APIs' outputs affect the software behavior and is optimized to provide outputs that ensure\shan{no way you can ensure} software behaves as if the ground-truth of the input is returned by the ML APIs. Meanwhile, the developers would not be bothered to modify their software to fit the adaptation. 
% On this front, we want to re-train these DNNs behind the ML APIs with a re-constructed loss function\kt{Justify this design choice.} that reflects the subset of labels the software cares about and the most damaging errors. For example, given the code structure in Figure~\ref{fig:app_example}, the re-constructed loss function will incur penalty only if the DNN makes mistakes that lead to wrong program branch (\eg ``Glass'' appearing in the outputs), and ignores any other types of errors that do not affect the software behavior(\eg the DNNs being confused between ``Snack'' and ``Food'', both belonging to the pre-defined list associated with \emph{Compost} branch).   \cc{This is solution. So I comment it out. I'll put them in Section 1.2}

% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% \kt{As I learned from Junchen, in general, when introducing related works, it is better to suggest what we are going to do, but do not say it directly.}
% \kt{This paragraph is tooooo long. Maybe illustrate these two line of works in two paragraphs?}
% \cc{``To the best of our knowledge, we are the first to study xxx problem.'' Can we claim something like this? If not, maybe starts with ``Existing work cannot tackle our problem. They improve xxxx without the knowledge of software.'' } \yh{I mentioned we are tackling a different problem, is this ok? }
% \kt{Adapting ML models sounds a bit abrupt. Maybe say ``existing work improves the performance of ML API by adapting the ML model.}
% \kt{Also, for me it feels early for us to mention ``optimizing without the knowledge of the software'' as the definition and importance of software knowledge is unclear here.}

% Existing work proposes solutions to improve the performance or accuracy of ML models without the knowledge of the software. However, we are tackling a different problem than these prior work. 
% One line of work optimizes the ML APIs' query accuracy or cost by adaptively choosing a sequential strategy to invoke available APIs within a resource budget ~\cite{chen2020frugalml, chen2022frugalmct}. 
% These work requires modifications on the developers' side, such as changing the code to apply the most accurate API. 

% Another line of work trains specialized models performing the tasks specified through a subset of SQL queries, such as aggregation and limit, such that the inference delay is reduced ~\cite{kang2018blazeit, kang2017noscope}. 
% The problem we are targeting at is different from this line of work for the following reasons. Firstly, these approaches cannot guide the ML APIs to produce outputs that lead to correct software behaviors, as they only optimize for inference delay instead of improving the model. Secondly, a great number of existing applications on GitHub calling ML APIs are written in Python~\cite{wan2021machine} instead of SQL. Thirdly, the operations that can be expressed in SQL queries that the prior work optimizes for are limited. For example, the SQL queries that are optimized by these work can only count average number of objects among all the video frames, or selecting limited number of frames that meet several constraints. Nevertheless, there are a wider range of operations that can be expressed by Python. For example, aggregation or limit queries cannot specify subsets of labels can have the same effects on the final program behaviors. 
% Lastly, in order to use the these systems that optimize for SQL queries, users need to translate their code into SQL queries, which incurs an extra development burden for the users.


Existing work proposes solutions to improve the performance or accuracy of ML models in software applications.
However, we found that existing solutions are not desirable as they add extra burden on the developers.
Specifically, one line of works focus on improving accuracy of ML task itself by modifying the software call to the ML APIs~\cite{chen2020frugalml, chen2022frugalmct}. 
Given a resource budget, they adaptively invokes several ML APIs from different cloud providers and ensemble their results. 
However, this approach require changing the software implementation in order to call different ML APIs, thus creating extra burden to the developers\shan{I find this argument very weak: the change required sounds very minimal and can be easily wrapped inside a library call. More importantly, I feel there are much more fundamental differences between your work and this previous work and yet you didn't mention.}.
Another line of work aims to reduce latency by compressing DNNs to perform a specialized task defined by a subset of SQL syntax~\cite{kang2018blazeit, kang2017noscope}. 
However, this approach cannot correct the software misbehavior triggered by wrong DNN output (as the DNN compression reduces the DNN latency while keeping the DNN ouput the same). 
Besides, this approach adds extra developer effort to reimplement their software logic (which is typically written in Python~\cite{wan2021machine}) using SQL syntax.
% In addition, they focus on SQL, while we study real-world applications written in general purpose language like Python~\cite{wan2021machine}, which supports much more operations.

Our goal is to \textit{automatically} adapting the DNNs behind the ML API \textit{without extra developer effort}.
\shan{Just like my comments in the abstract, I feel you still didn't make it very clear about your assumption. What is your assumption about what you have access to and what you can change? This assumption is VERY different from our OOPSLA submission, right? That is why you need to clearly explain your problem statement and assumption here.}

% \kt{Saying that we are targeting a different problem sounds like we are not picking the correct related work for our problem. Maybe try to say previous work are solving the same problem with the wrong assumption.}


% as software developers typically write Python code to use the ML APIs, instead of declarative\kt{declarative is a ``noise'' here. It's better for us to focus on the popularity of the language here.} languages such as SQL.\kt{Previous work use SQL is not immediately clear to the reader.}
% \kt{People tend to not directly care about the limit of operations. Maybe link to what people care, like SQL limits what the \textbf{software can do}, and give a real (at least seemingly real) example to convince people a true need of software cannot be expressed by SQL.}, 
% \kt{For me, this point is essentially the same as the first point. The effect of choosing a programming language that people don't use is forcing the user to ``tranlate'' their code to another language.}  \kt{Personally I feel like this is the most fundamental reason. Putting it at the last is kind of downplaying this point.}\kt{I guess maybe you are referring that these works cannot fix the misbehavior of the software as they are just compressing the model, not improving the model. ``Software behavior'' and ``ground-truth labels'' are noise.} 


% \cc{Please say it is ideal solution. Maybe sth. like ``An ideal solution is to automatically adapt the network behind ML API to the task software performs''} 
% \cc{This paragraph is very strange, and does not provide any additional information. We usually say sth. like ``this example shows a common feature of xxxx'' or ``this is not the only example. A number of xxxx''} \cc{What gap? and how to define the gap? You need to introduce it first. Actually, I prefer you define the second half of this sentence as the gap}


% \emph{Automatically} adapting the ML APIs is important since the developers that call the ML APIs typically lack the knowledge of ML model training, or they do not have the compute resource to afford model training. 
% \cc{I move this sentence to this paragraph. Please change this sentence starting from sth. like ``Automation is important as ....''}

% As a result, we need an approach that automatically adapts the ML models behind ML APIs such that they are aware of the damaging errors that will lead to software misbehaviors\cc{This sentence belongs to P5. It also looks like a repletion of P5-sentence1}.

Automatically adapting the ML models faces several challenges. 



\emph{Firstly}, automatic model adaptation is hard. Aiming to help non-expert developers, an automatic approach that minimizes developer effort is desired. To achieve such automatic adaptation, we need to understand how software uses ML API output label and the severity of different types of mis-predictions. We also need to translate these information to a DNN-understandable format for adaptation, such as a loss function, which is inherently hard due to rich code syntax. 
% \cc{Yuhan, please proof read}

% Automation is necessary because the application developers using the ML APIs typically lack expertise in ML, thus may not be able to efficiently perform model adaptation. We need to automatically extract information\kt{vague} embedded in the code structure that indicates how the software plans to use ML APIs' output labels. We also need to transform the information extracted from the software into loss functions that can directly be applied to optimize the DNNs.  
% \cc{why automation? please explain} \yh{added. }


% from the software about the specific task. 
% why infer? Users didn't explicitly specify the tasks, and they are non-experts, so they are not able to specify the tasks in the form that can be directly used to optimize for DNNs' accuracy 
% It is unrealistic to provide extra input for model adaptation (\eg manuals for performing model re-training) at the software developers' end. The main reason is that the software developers who call the ML APIs are typically non-experts in ML, thus it is hard for them to provide an effective model adaptation strategy. 


\emph{Secondly}, model adaptation needs to be very efficient. 
 Since we need to re-train the ML model for each software application, model adaptation should be fast. Moreover, software applications may change time to time during the development procedure, thus adapting the ML models quickly can greatly save the time and operation cost of re-training. 
 \shan{I guess we also assume that we cannot obtain new training data from application developers.}
 % \kt{Another reason is that your approach needs to train different DNNs for different softwares, so the training need to be cheap.}
% Given how the interface of the ML APIs is designed, the software developers who call the ML APIs are not able to adapt the DNNs behind the ML APIs. Thus, model adaptation has to happen on the cloud service providers' side, and it is important to provide a quick way of adapting models which reduces errors leading to wrong software behaviors with minimum training cost. \cc{It does not matter whether developer or service provider pay the training cost. Actually, service providers could charge more on developer if training takes more time. You may say (1) software may change time by time during development (2) a fast adaptation could save time and operation cost} 


% such that the number of damaging errors leading to incorrect software behaviors can be reduced most effectively (\ie incurring minimal training cost).  

% \item We performed empirical study on the applications that use ML APIs performing image classification tasks to affect the control flow of the software. We found that a common pattern 


% \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    % \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    % \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    % \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    

    % \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    % \item Automatically adapting the ML APIs to the software is challenging. 
    % \begin{itemize}
    %     \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

    %     % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
    %     % \item Need to transform cognition task into math expression 
    %     % create the template 
    %     \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
    %     \item Need to adapt the ML APIs efficiently 
       
    % \end{itemize}
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    

   

% Existing works have performed model customization in different scenarios. 
% They either directly input (\eg the classes that need to be classified)~\cite{kim2021pool, cao2021thia} or specify the specific tasks through a fixed program interface (\eg SQL)~\cite{kang2018blazeit}, and adjust the models, by training specialized models or reorganize different pre-trained model components, based on the specific tasks. Another line of work observes run-time data distribution and customizes the model to fit the specific content in the data. 

\begin{figure}
\begin{subfigure}{0.45\textwidth}    
         \centering
         \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['Plastic', 'Wood', 'Glass', 'Paper', 'Cardboard', 'Metal', 'Aluminum', 'Tin', 'Carton']
Compost = ['Food', 'Produce', 'Snack']
Donate = ['Clothing', 'Jacket', 'Shirt', 'Pants', 'Footwear', 'Shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'It is recyclable.'
  elif obj.name in Compost:
    return 'It is compostable.'
  elif obj.name in Donate:
    return 'It is donatable.'
return 'It is others.'
\end{lstlisting}
%          \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Recycle = ['Plastic', 'Wood', 'Glass', 'Paper', 'Cardboard', 'Metal', 'Aluminum', 'Tin', 'Carton']
% Compost = ['Food', 'Produce', 'Snack']
% Donate = ['Clothing', 'Jacket', 'Shirt', 'Pants', 'Footwear', 'Shoe']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% Predictions = []
% for obj in response.label_annotations:
%   Predictions.append(obj.name)
% if any([label in Recycle for label in Predictions]):
%   return 'It is recyclable.'
% elif any([label in Compost for label in Predictions]):
%   return 'It is compostable.'
% elif any([label in Donate for label in Predictions]):
%   return 'It is donatable.'
%     \end{lstlisting}
\subcaption{The software implementation}
\label{fig:app_example}
% \includegraphics[width=.99\linewidth]{figs/app_example2.pdf}
    \end{subfigure}
 \hfill
    \begin{subfigure}{0.45\textwidth}  
        \includegraphics[width=\linewidth]{figs/app_example2.pdf}
        \subcaption[]{Including an extra wrong\shan{???What do you mean by missing???} recognition ``Glass'' leads to software mis-behavior. The arrows starting from the Ground-truth labels are the correct software control flow decision (\ie as if the ground-truth labels are output by the ML API). In this example, the correct control flow is executing the branch associated with the Compost list, because the ground-truth labels only have an intersection with the Compost list. \shan{This caption is very difficult for readers to understand.}}
        \label{fig:input_example_top_wrong}
    \end{subfigure}
    %     \begin{subfigure}{0.45\textwidth}  
    %     \includegraphics[width=\linewidth]{figs/input_example_top_label_correct.pdf}
    %     \subcaption[]{Mis-classifying the label ``Wood'' does not lead to software mis-behavior. }
    %     \label{fig:input_example_top_correct}
    % \end{subfigure}
    % \caption{Heapsortcypher, a garbage classification application \cite{heapsort} using Google Cloud API. 
    % \kt{The key in this figure is the contrast between highly accurate API output and wrong software misbehavior. Maybe not calling the ideal API output as ``ground-truth''? It is better for your point to come across without letting the reader to parse what does ``ground-truth'' means, and realize that this image comes from your dataset and it is an image annotated with ground-truth label.}\cc{It's fine. We just take it literally: the correct answer.}
    % }
\label{fig:app_example_entire}
\end{figure}


\subsection{Contributions} 
%\kt{I would expect contributions to be some short and condensed bullet points.}\cc{Let's first make a long version and then decide how to compress it.}


% We present \tool, which helps the cloud service providers to automatically re-train the ML models behind the ML APIs to the applications the developers write, so as to reduce the software mis-behaviors incurred by the ML APIs' outputs.
% \cc{I changed the description. Please proof read} \yh{we are not helping developers, our solution happens on the cloud service providers' side. }

% We find that the code structures reflect the severity of different API mis-predictions.
% For example, in Figure~\ref{fig:app_example}, labels in the \emph{Recycle} list and labels in the \emph{Compost} list trigger different program behaviors. Therefore, given an input image only containing labels in the \emph{Recycle} list, it is a severe error if the ML API outputs labels in the \emph{Compost} list. \cc{This paragraph should belong to empirical study} 

To understand how real world applications use ML APIs\shan{This opening sentence is toooo generic. I could have used it in all recent papers from our group. If I am a reviewer, I would wonder ``haven't people already conducted tons of study to understand how applications use ML APIs? Why do you need to study again?????''. What EXACTLY was not understood before and hence you want to understand?}, we conduct an empirical study on a recently published ML software benchmark suite~\cite{wan2021machine}. We found five code structure patterns of how ML software post-process ML APIs' outputs, and derived three types of abstractions to characterize how the control flows are affected by ML APIs' outputs (details are in Section~\ref{sec:empirical})\shan{Again, why isn't this already covered by previous work?}.  
% We focus on 19 applications which invokes Google \code{label\_detection} API to make control flow decisions. These applications use the ML APIs' outputs to determine which program branch to be executed, like Heapsortcypher in Figure~\ref{fig:app_example}. They typically define several lists of labels and program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 

% To characterize the application's post-processing step of ML API outputs, we defined three types of abstraction: (1) the sets of labels that have equivalent effects on the control flow;  (2) whether the final output of the software is exclusively associated with only one program branch; and (3) whether errors made in some sets of labels can be disguised by correct predictions in other sets of labels.


% \cc{Do we want to mention mutually exclusive?}. 
% Specifying the values of the abstractions can uniquely identify how the applications are going to post-process the ML APIs' outputs. 

Guided by the empirical study, we propose \tool, an automated framework that adapts ML models behind the ML API to the software implementation while keeping the same API interface, so as to reduce software misbehaviors. Tackling automation challenge, it first perform static analysis on the Python source code to extract the abstractions from the software. \tool then re-constructed the loss function to reflect the different severity of mis-predictions on software correctness. Tackling efficiency challenge, \tool adopts fine-tuning approach to adapt the ML model behind ML API with minimum training costs.
\shan{I like this paragraph, but clearer than earlier paragraphs.}
% \cc{Can you map these solutions to challenges?} \yh{i put the second challenge in the evaluation part}
% \cc{The second half of sentence are evaluation} 



% We systematically measure the improvement in the rate of software mis-behaviors on 19 open-source applications that call multi-label image classification API.
We systematically evaluate \tool on 19 open-source applications that use multi-label image classification API to make control flow decision.
Our evaluation shows that the re-constructed loss function provides up to \todo{X\%} improvements in reduction of software mis-behaviors, whereas alternative approach only improves rate of software mis-behaviors by \todo{Y\%}. Our evaluation also shows that performing model adaptation with the re-constructed loss function can finish within \todo{Z} minutes.  \yh{Will update the numbers after I finish the evaluation section. }
% (1) labels that will trigger the same program behaviors; (2) whether the final software output is exclusively associated with only one program branch, for example, in the application example shown in Figure~\ref{fig:app_example}, the final output of the software is the message specified in one of the program branches; (3) whether different sets of labels triggering same program behaviors have different priority levels. 


==> backups/1-introduction-v2.tex <==
\begin{itemize}
\item Generative models have become extremely popular recently (list popular generative models-based applications, and specifically the popularity of Transformer-based models)
\item Transformer models will be queried by users over a longer period of time, thus long context will be accumulated

\item When users use the generative-model-based applications, one of the most important metric for users' experience is the ``time-to-first-token'', which we refer to as \emph{TTFT}. TTFT limits the 
\end{itemize}

==> backups/1-introduction.tex <==
\label{sec:intro}

\subsection{Motivation}

\begin{itemize}
    \item Nowadays, more and more software applications require the underlying software to understand what is present in the images with Deep Neural Networks (DNNs). As training such DNNs can be expensive, the software developers use off-the-shelf ML APIs to reduce their development effort~\cite{wan2021machine}. 
    % \item Machine Learning (ML) offers effective ML APIs to a wide range of cognition tasks. Many cloud providers offer ML APIs, supported by underlying Deep Neural Networks (DNNs), that perform well on generic tasks (\eg image classification). These ML APIs are utilized in a wide range of software applications for different specific tasks. However, the ML APIs are not adapted to achieve the application specific tasks, leading to many software misbehaviors.
    \item List an application such that why/how high class-wise accuracy does not lead to correct software behavior or vice versa and cite~\cite{wan2022automated} to illustrate that there are many such applications. 
    \ref{fig:app_example} is an example software that incorporates Google \code{label\_detection} API, which outputs all the existing labels in the input image. If we consider traditional class-wise F1 score of the application, the ML API can achieve 
    % \yh{List the number of applications on GitHub that employs ML APIs}
    \item Here we define the software achieving correct behaviors if the outputs of the ML APIs lead to the same software behavior as if the ground-truth is returned.  
    \item Explain why the accuracy of the software would be low: the service providers train the ML models aiming to maximize class-wise accuracy, while the software developers need to ensure correct software behavior given the ML API outputs.  
    % \begin{itemize}
    %     \item the service providers pre-train the ML models that support the ML APIs with large-scale datasets (\eg Open Images dataset), aiming at providing good class-wise accuracy. \cc{Do you want to emphasis that they have different optimization goals?}
    %     \item When software developers use the ML APIs in their software, they expect the ML APIs to output classes that lead to the correct software behavior (\ie same software behavior as what the ground-truth leads to) \cc{What's the different between point2 \& 3?} 
    %     \item The pre-trained ML models may make mistakes that lead to the wrong software behavior
    % \end{itemize}
    
     
    % \item Accordingly, there is a mismatch between how the developers measure the end-to-end accuracy of the software and the original accuracy of the ML APIs. Even though the ML APIs are supposed to have very high accuracy on the overall generic accuracy of the ML APIs, the overall accuracy of the software using the ML APIs may be lower than the accuracy of the original ML APIs. \yh{list example numbers. }
    \item An ideal case of utilizing the ML APIs is to adapt the ML APIs so that they are aware of the errors that are unacceptable by the software (\ie leading to wrong software control flow). 
    % \cc{Automation is mentioned in next bullect. In this bullet, you'd better talk about customization only.} 
    \item Automatically adapting the ML APIs to the software is important: (1) The developers who use the ML APIs are usually not experts in ML, thus may not know how to adapt the models (2) The developers do not have an affordable way to support model adaptation. 
    % \yh{mention why automation is important}
    % \yh{Emphasize that the problem is important}
    
    
    
    % \item However, when the developers use the ML APIs in their software, they are either unaware of the mismatch between ML APIs' accuracy and software's accuracy, or they do not have an affordable way to adapt the ML APIs to fit the software application they are writing.  \yh{Define affordable: 1. developers do not need to provide training data 2. they do not need to specify what are the context that can be digested by the DNNs to improve accuracy. }
    \item Automatically adapting the ML APIs to the software is challenging. 
    \begin{itemize}
        \item No existing benchmark has shown that there is a discrepancy between the outputs resulting in high class-wise accuracies and the ones leading to the correct software behaviors

        % (prior works either (1) only study ML APIs themselves (2) realize the low accuracy of ML APIs in the software~\cite{wan2021machine} (3) do not understand why the ML APIs do not work when applying to the software (SW only cares about branch prediction are correct) )
        % \item Need to transform cognition task into math expression 
        % create the template 
        \item Need to extract software specific cognitive task automatically and transform the extracted software context into mathematical expression that enables ML API adaptation
        \item Need to efficiently adapt the ML APIs 
       
    \end{itemize}
    
    \yh{why related works cannot handle }
    
    
    
    
    
    % \yh{To adapt the ML solutions to the software, software developers face many issues... (or accuracy decrease) or say adaptation is very important}
    % \yh{why do adaptation ? if not, will cause accuracy decrease. }
    
    % \yh{Developers did not realize this issue or they do not have an affordable way to adapt}
    
    % \yh{List an example}
    
    
    % \yh{Automatically adapt to the software is challenging. }
    
    
    % \item However, when the software developers incorporate the ML APIs in their software applications, they usually only care about specific context.  
    % \item To understand the specific context that the software developers usually focus on, consider the Smart Can application in Figure~\ref{fig:app_example}. Smart Can uses the Google \code{label\_detection} API to perform image classification on a user input photo. ... 
    % \item For the Smart Can application, the software developers only care about if the ML API is able to correctly recognize classes in the specified lists (\eg Plastic, Food etc.). 
    % \item Additionally, the end-to-end accuracy of the software does not equal to the accuracy of the ML API. 
    % \item These two fronts bring the opportunity to adapt the ML models to improve the accuracy of the software that incorporate the ML APIs. 
    % \item However, there are several open challenges in adapting the ML models to the software. 
    
%     1. How to define the context of the software?  \yh{What should be the context? what is the context that can be digested by the NN? }
% \begin{itemize}
%     \item The subset of classes specified in the software
% \end{itemize}
    
%     2. How to extract the context automatically? \yh{merge into the first one}
    
%     3. How to utilize the context? Re-train the underlying ML models
%     \begin{itemize}
%         \item Modify the training data distribution 
%         \item Modify the training loss
%         \item Modify the model architecture to directly predict the output of the software 
%     \end{itemize}
    
%     4. Affordable re-training (training time, training data)
    
   
\end{itemize}


\begin{figure}
   \centering
\begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Recycle = ['plastic', 'wood', 'glass', 'paper', 'cardboard', 'metal', 'aluminum', 'tin', 'carton']
Compost = ['food', 'produce', 'snack']
Donate = ['clothing', 'jacket', 'shirt', 'pants', 'footwear', 'shoe']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Recycle:
    return 'Recycle'
  if obj.name in Compost:
    return 'Compost'
  if obj.name in Donate:
    return 'Donate'
\end{lstlisting}
    \caption{heapsortcypher, a smart can application \cite{xxx} using Google Cloud API. \cc{TODO}}
    \label{fig:app_example}
\end{figure}

\subsection{Contributions} 
\begin{itemize}
%  \item We present \tool, which is an end-to-end system which automatically extracts software context from the applications that incorporate ML APIs, and adapt the ML models to improve the software accuracy. 
\item Studied a wide range of software applications that incorporate ML APIs, and identified that one of the common software context is mapping fine-grained ML API output classes to program branches. 
\item Defined a template to automatically transform the code that the software developers write into mathematical expression that can adapt the ML APIs to the software. 
% \item defined the template and the transformation to math expression 
\item Leveraged two ways of model adaptation with the defined software context that (1) changes the training data distribution to reflect the subset of classes that the users care about; (2) modifies training loss function to directly reflect the control flow of the software. 

% \item Compared the ways of model adaptation in terms of accuracy improvement and training cost on \todo{X} real applications using ML APIs.

% defined two types of software context that can improve the accuracy of the software: (1) Data distribution context; (2) Subset of classes context. 

% \item Developed a tool to automatically extract the defined context from the Python code written by software developers 


\end{itemize}

==> backups/2-1-background-v2.tex <==






\begin{figure}
     \includegraphics[width=.99\linewidth]{figs/motivation.pdf}
    \tightcaption{An illustration of } 
    \label{fig:moti}
\end{figure}

\begin{itemize}
    \item Generative tasks have become extremely popular these days
    \begin{itemize}
        \item Code generation: AI-based code autocompletion suggestion given function name or part of code based on previous code in one file 
        \item Music generation: AI-based music generation based on text prompt 
        \item Image generation: AI-based image generation based on input text prompt, part of an image, or a combination of image and text prompts
        \item Text generation: AI-based conversational bot based on input texts 
        \item Retrieval-augmented generation: 
    \end{itemize}
    \item Transformer-based models have been deployed in these wide range of generative tasks~\cite{openai2023gpt4, agostinelli2023musiclm}
    \item Define context
    \begin{itemize}
        \item In \qa, context is defined as all the previous interactions between the LLM and users. For example, when the user queries the LM with the question ``What if the assumption in the above question changes to ...'', without considering the previous, and potentially very long, context, the answer will be very bad
        \item In \rag, context is defined as all the documents relevant to one input question
    \end{itemize}
    \item Define TTFT: the inference delay starting from the time when the inference request is submitted to the time at which the first token appears on the users' interface
    \begin{itemize}
        \item Why this is important? During TTFT, users are purely waiting for the response. 
        \item For example, for ChatGPT, if the first token takes too much time to appear, the user may switch to another window because he feels the job has been queued for a very long time
        \item For example, for Copilot, if the first token appears very quickly, the user can decide if the autocompletion is completely off or may be acceptable. This will greatly enhance the efficiency of the code-writing process 
    \end{itemize}
    \item Given  how important it is for the first token to appear as soon as possible for enhancing users' experience in using generative model based apps, it’s very crucial to try to reduce TTFT 
    \item \todo{Add some evidence to show why we focus on initial phase delay by citing papers which reduces incremental phase delay}
    \item The Transformer model needs two steps to generate the first token for an answer: (1) compute the Attention key and value for the context; (2) generate the first token conditioned on context’s Attention key and value. The first step composts a vast majority of TTFT.
    \item Previous works~\cite{li2022decoupled,izacard2020leveraging,mialon2023augmented,komeili2021internet,shuster2021retrieval,milbauer2023lait} propose to pre-compute and re-use Attention key and value of the context, in order to avoid re-computing (Use fig~\ref{fig:moti}). 
\end{itemize}

\jc{please start with a couple of paras on key background:
\begin{itemize}
    \item some examples of generative tasks (not just text)
    \item how transformer is widely used in a range of generative apps, not just text, but music, images, videos, code, and so forth
    \item define the basic terms: session, token, history, state, etc
    \item why TTFT is crucial (cite papers and user studies, etc), and why we focus on TTFT rather than the delay for incrementally generate each token.
\end{itemize}}

% \mypara{Transformer-based generative model inference workflow} \jc{highlight that the arch is shared by all transformer-based models (it's true, right?)}
% \begin{itemize}
%     \item Use Figure~\ref{fig:workflow} to explain the delay components of Transformer-based generative model's inference
%     \item Use Figure~\ref{fig:delay_components} to show the fraction of each delay components
%     \item Attention operation is the computation bottlneck: Explain why history can increase dramatically (\eg letting GPT to summarize papers, or writing code with Copilot with thousands lines of code), why attention is the bottleneck,  and why it's growing quadratically with the number of tokens
% \end{itemize}

% \jc{need more evidence why history increase dramatically (like i mentioned on phone, this is not natural to me) and how it cause the TTFT to grow quadratically. } 
% % \yh{Better include a CDF of history length statistics from a dataset }

% \mypara{}
% % \mypara{How to alleviate the attention operation's delay?} \jc{maybe change it something like "prior efforts to reduce delay"}
% \begin{itemize}
%     \item Since the generative models typically interact with the generative model in one session (\ie conversation about one topic, where later interactions will refer to previous ones) continuously, previous interactions between the user and the generative model can be cached. 
%     % \item Give a concrete example using ChatGPT to illustrate the definition of session and history \jc{this doesn't belong here}
%     \item Explain what to cache 
%     \item Explain why caching is even possible: history only depends on past, not the future, thus the history cached data will not change, refer to Section~\ref{sec:appendix} for formal definition
%     % \item Show inference delay speedups by enabling caching with Figure~\ref{fig:caching}
% \end{itemize}


% % \begin{figure*}
% %      \includegraphics[width=.99\linewidth]{figs/fig9.pdf}
% %     \tightcaption{Initial phase's delay with or without caching enabled. \todo{Mock figures}}
% %     \label{fig:caching}
% % \end{figure*}

% \begin{figure*}
%      \includegraphics[width=.99\linewidth]{figs/workflow.pdf}
%     \tightcaption{Inference workflow of Transformer-based generative models. }
%     \label{fig:workflow}
% \end{figure*}




==> backups/2-1-background.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\section{Background \& Motivation}

\mypara{Transformer architecture} 
The Transformer model~\cite{vaswani2023attention}  has revolutionized the field of natural language processing (NLP). 


The key of Transformer architecture is multiple stacked Transformer layers, as shown in Figure~\ref{fig:}(a). 
% Each of the Transformer layers consists of a self-attention module and a fully-connected module, where the self-attention module is the major characteristic that differentiates Transformers from other ML architecture.
The key of each Transformer layer is the self-attention module, as shown in Figure~\ref{fig:}(b). 
Each Transformer layer comprises a distinctive self-attention module, as illustrated in Figure~\ref{fig:}(b). 
This self-attention mechanism plays a pivotal role in distinguishing Transformers from other ML architectures. 
Upon an input \emph{sequence} of text, this module generates three distinct embeddings for each input token, namely: query, key, and value.


% For a clearer grasp of the implications of query, key, and value embeddings, consider the analogy of a Google search. 
% When users search for a product on Google, the search engine correlates the user's \emph{query} (the text in the search bar) with a set of \emph{keys} (product titles and descriptions) linked to items in the database. 
% Subsequently, it presents users with the most relevant \emph{values} (the actual products).

Then the self-attention module performs dot product of the current token's query with the keys of all previous tokens, followed by a Softmax function. 
This computation quantifies the significance or ``attention'' the current token should allocate to preceding tokens.  
Consequently, the module performs a dot product on the value embeddings with the product of query and key. 

Although being extremely powerful in a wide range of tasks, the self-attention module has high computation overhead, with a $O(T^2)$ computation complexity, where T being the length of the input. 

\mypara{Transformer's inference procedure}In language applications akin to ChatGPT, users typically submit an \emph{input prompt} to engage with the language model (LM). 
The LM subsequently responds to the user's prompt by considering the user's earlier interactions (history) with the LM and referencing a knowledge database. 
Throughout this paper, we will refer to the LM's utilized context for responding as the \emph{context}.

The generation of answers is auto-regressive, with words produced iteratively. 
 In the initial iteration, tokens from the input prompt, combined with tokens from the context, are processed through the tokenizer and embedding layer to formulate query, key, and value embeddings. 
 These input embeddings subsequently traverse the series of Transformer layers to yield a probability distribution governing word generation. 
 Subsequently, the output of the first generation is appended to the input embeddings, creating the input for the subsequent generation iteration. 
 This iterative process continues until either the end-of-sequence token is generated or a predetermined limit is attained.
% In the first iteration, all the tokens for the input prompt, together with the tokens for the context are fed into the tokenizer and embedding layer to generate the query, key, and value embeddings.
% Then, the input embeddings go through the stack of Transformer layers to output a distribution of probabilities that will determine the generated word. 
% Afterwards, the output of the first generation will be concatenated with the input embeddings, to form as the input to the next generation iteration. 
% This procedures go on and on until the end-of-sequence token is output or the limit is reached.
% \begin{figure*}
%      \includegraphics[width=.99\linewidth]{figs/workflow.pdf}
%     \tightcaption{Inference workflow of Transformer-based generative models. }
%     \label{fig:workflow}
% \end{figure*}


\begin{figure}
     \includegraphics[width=.99\linewidth]{figs/motivation.pdf}
    \tightcaption{An illustration of inference with key-value cache. \yh{TODO}} 
    \label{fig:moti}
\end{figure}

\mypara{}

\mypara{Why caching key/value embeddings?} Given that each generation iteration necessitates the key and value embeddings for all prior tokens, previous works~\cite{li2022decoupled,anagnostidis2023dynamic,izacard2020leveraging,mialon2023augmented,komeili2021internet,shuster2021retrieval,milbauer2023lait,dai2019transformer,wolf-etal-2020-transformers,pope2023efficiently,ott2019fairseq} 
have introduced the concept of caching these embeddings, which we refer to the \emph{\kv}. 

% This avoids the need for re-calculating  key and value embeddings for preceding tokens. 
% Among the previous works, for those Transformer models designed for conversational applications, after initializing the \kv for the context, the delay later generation iterations, which require the key and value embeddings for all preceding tokens, can be reduced. 
% On the other hand, for those Transformer models designed for retrieval-augmented generation, the generation requires fetching retrieval embeddings most relevant to the prompt submitted by users. 
% Thus,
% the \kv can reduce the delay for preprocessing the documents in the retrieval databases. 

% We argue that in the future, the key and value embeddings for the context will be pre-computed, so as to not only reducing the generation delay for later itarations, but also the delay for the first iteration.
% Figure~\ref{fig:moti} serves as an illustrative depiction of the inference procedure with and without cached key/value embeddings for ChatGPT-like conversational applications. 
Among these prior works, in the context of Transformer models designed for conversational applications, initializing the \kv for the context at the first iteration results in a reduction in the delay during subsequent generation iterations, which demand key and value embeddings for all prior tokens. Conversely, for Transformer models designed to enhance retrieval-augmented generation, the process of generation entails retrieving embeddings most pertinent to the user's submitted prompt. Consequently, the \kv proves instrumental in curtailing the preprocessing delay linked to documents stored within retrieval databases.

We contend that, looking forward, pre-computing the key and value embeddings for the context will emerge as a pivotal strategy. This innovation stands to not only expedite the generation process in subsequent iterations but also mitigate delays associated with the initial iteration. To illustrate these concepts, Figure~\ref{fig:moti} offers a visual representation of the inference procedure, contrasting scenarios with and without cached key/value embeddings, particularly in the context of ChatGPT-like conversational applications.


==> backups/2-2-empirical-1025.tex <==
\label{sec:empirical}

To understand how developers use ML API in real-world applications, we conduct an empirical study on ML software that invokes  ML APIs to make control flow decisions. \cc{I weakly remember that you plan to study Amazon APIs. Please revise it if I'm wrong}

% We observe that there are different ways for developers to specify how they plan to use the ML APIs' outputs to affect the control flow of ML software. 
% In order to understand the common patterns of the control flows of the ML software, we conduct an empirical study on ML software using Google's \code{label\_detection} API, which performs multi-label image classification.  
% From the case study, we summarize three types of abstractions for the code structures of the ML software. 



% \yh{ML API on OI or pretrained on OI}
\subsection{Methodology}

\subsubsection{Application selection}



% Google (benchmark, search), AWS (search)
We study 40 open-source ML software applications  whose control flows are affected by the output of a multi-label image classification API. These applications comes from two sources: (1) 19 applications come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}; and (2) 21 applications comes from GitHub by random checking around 60 applications.
Among these applications, 29 of them use Google \code{label\_detection} API and 11 use Amazon \code{detect\_labels} API.

\yh{select applications using multi-label classification and object-detection APIs, because that's representative of the ML software }

% \cc{Maybe also add some statistics}


We do not study the applications that directly print out the ML APIs' outputs or store these outputs without post-processing. The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

\subsubsection{Test data selection}
TO-DO
\cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}




% We study the open-source applications from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}. We focus on applications whose control flows are affected by the ML APIs' outputs. We focus on 19 applications which invoke Google \code{label\_detection} API to make control flow decisions. These applications use the ML APIs' outputs to determine which program branch to be executed. For example, in the application example in Figure~\ref{fig:app_example}, the API output labels in Figure~\ref{fig:app_example2} will lead the software executing \code{return 'Recycle'} on line 8 because ``Glass'' is included in the \code{Recycle} list. We refer to the branch being executed, such as \code{return  `Recycle'}, when the if condition is satisfied, as \emph{if/then branch}. 
% To characterize the application's post-processing step of ML API outputs, we defined three types of abstraction: (1) the sets of labels that have equivalent effects on the control flow;  (2) whether the final output of the software is exclusively associated with only one program branch; and (3) whether errors made in some sets of labels can be disguised by correct predictions in other sets of labels.
% We do not study the applications that directly print out the ML APIs' outputs or store all the outputs in the databases, because these applications do not have mismatch between ML APIs' outputs and software's output thus do not have room for improvement. 




% \subsection{Common patterns of code structure of software utilizing ML APIs}
\subsection{Result summary}
Across all applications we studied, 48\% of them defines several whitelists and compares ML API output labels with them. 

Take Heapsortcypher (Figure~\ref{fig:app_example_entire}) as an example. It executes Line 8 when given a candy image, as the API output ``Glass'' is included in the \code{Recycle} list and thus fulfills the statement in Line 7. We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}.
We refer to a list of labels (or classification category) leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example.

% \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

While these applications typically uses whitelists to post-process ML API results, they vary in the way of using whitelists to make control flow decisions. Even with same whitelists and API inputs, the applications would behave differently according to its code structure. Next, we will introduce the common patterns observed in the studied applications.


% We find that these software typically pre-defines one or several lists of labels as branch conditions, and then maps the original output labels to the pre-defined lists which intersect with the labels. Then the software executes one or more \ifts that correspond to those mapped pre-defined lists. 
% In other words, all the labels specified in one list will lead to the same control flow decision. 

% We refer to the lists of labels leading to the same control flow decisions as \emph{whitelists} in the rest of the paper. For example, in the application example shown in Figure~\ref{fig:app_example}, the software defines three \emph{whitelists}, Recycle, Compost, and Donate. 



% They typically define several lists of labels and which one or more program branches the application should execute by comparing the API output labels and these lists. 
% They typically define several lists of labels and which one or more program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 


\begin{figure}
    \centering
     \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}

\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_non_mut}
\end{figure}


\subsection{Abstractions}
\label{sec:abstractions}
As summarized in Figure~\ref{fig:hierarchy} we define four types of abstractions to characterize the code structure. We will use several minimal templates to illustrate the four types of abstractions. 


\textbf{1) Number of whitelists.} The software specifies one \wl or multiple \wls. Particularly, as shown in Figure~\ref{fig:template1}, each whitelist is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wl. In the rest of the paper, we will refer to executing a branch as mapping API outputs to its corresponding whitelist.

\textbf{2) Type of mapping.} For the software specifying multiple \wls, there are two types of mapping from ML API outputs to whitelists: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels are mapped to several \wls; (ii) the software checks whitelists in a specific order, and only executes the lower-ranked \ifts when API outputs do not intersect with any higher-ranked whitelist, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% \cc{I changed it from multiple to several, so that it means 0 to N}

% For the software specifying multiple \wls, when the software checks if the output labels intersect with the \wls, there are two possible ways of checking: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels may be mapped to multiple \wls; (ii) the software checks the branch conditions in a specific order, and only executes the lower-ranked \ifts if the higher-ranked branch conditions are false, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% (i) the software executes at most one if/then branch when the API's outputs intersect with the \wl associated with the branch condition; (ii) the software executes all the if/then branches when the API's outputs intersect with the \wls associated with the branch condition. 
% For the software that specifies several \wls, some software will compare the ML APIs' outputs with the \wls, and break at a program branch once the outputs intersect with the \wl associated with the branch. In other words, the final output of the software is the message corresponding to with only one program branch. Other software compares the ML APIs' outputs with the \wls, and outputs all the messages 

\textbf{3)Type of output.} For the software which maps original output labels of the ML API to several \wls, it either construct the final output in a format of (i) set or (ii) list. In the latter, the final output is affected by the order of examination.
% For the software which maps original output labels of the ML API to several \wls, there are two possible ways for software to construct the final output:  (1) the software checks the output labels one by one, and add a \wl to a list if the output labels intersect with the \wl. Finally, the software outputs the list containing all the matched \wls. In this case, the order at which the \wls intersect with the output labels does matter; (2) the software checks the output labels one by one, and add a \wl to a set if the output labels intersect with the \wl. Finally, the software outputs the set containing all the matched \wls. In this case, the order at which the \wls intersect with the output labels does not matter.

\textbf{4) Order of examination.}  For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.
% For the software which executes at most one \ift, the order at which the software performs the checking on the branch conditions may either prioritize the specified \wls or the output labels. 
% As a result, for the software that prioritizes the order of the output labels, mis-classifications happened on the lower-ranked output labels do not matter, as long as the higher-ranked output labels can lead to the correct control flow decisions. Similarly, for the software that prioritizes \wls, mis-classifications happened on the lower-ranked \wl do not matter, as long as the . 

\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Common code patterns of ML software. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}



\subsection{Common Code Patterns}
\label{sec:examples}
\yh{TODO: add connection to the abstractions} \cc{Also add how many applications belongs to each category}
Based on these four types of abstractions, Figure~\ref{fig:hierarchy} summarized all the possible code patterns in a structure of decision tree. Each decision nodes represent an abstraction. Each leaf node represents a code pattern constructed with the sequences of different decisions made at each decision node. While Figure~\ref{fig:hierarchy} illustrates six possibilities, our studied applications only contain four of them (green box in solid lines).

% Based on these four types of abstractions, we can characterize the common code structures as shown in Figure~\ref{fig:hierarchy}. Each decision node in the decision tree represents an abstraction as described in Section~\ref{sec:abstractions}. Each leaf node in the decision tree represents a type of code structure constructed with the sequences of different decisions made at each decision node. The leaf nodes are all the possible code structures constructed with the abstractions. However, we only found a subset of all the possible code structures in the benchmark suite. The existing types of code structures are shown in the leaf nodes with edges marked with solid lines, whereas the non-exisiting code structures are the leaf nodes with edges marked with dashed lines in Figure~\ref{fig:hierarchy}. We list four patterns of ML software. 
% software examples to illustrate the common patterns of how ML APIs' outputs affect ML software's control flow decisions. 

\subsubsection{Software pattern 1: T-or-F} This type of software only specifies one \wl which includes multiple labels, such that labels in the \wl have an equivalent effect on the software's control flow decisions. Around 35\% applications in our benchmark suite belongs to this category.

Figure~\ref{fig:app_example_level1} shows a carnivore identification application. It goes through all the predicted labels of an input photo, and executes the \ift \code{ return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, mis-classifications within the pre-defined \wl Animal (\ie mis-classifying a dog image as ``Wolf'') do not lead to software misbehavior. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. On the contrary, if an image contains a carnivore, while the API output do not include any label in the \wl (Figure~\ref{fig:input_example_tf_wrong}). 


To quantify the difference in the metrics of the ML API and the correctness of this software, the traditional F1 score of the ML API on the test dataset is 58\%, while only 43\% of the data correctly identified classes in the \code{Dog} \wl, leading to software behaviors as human expected. 


% percentage of data such that the software behaves as human expected is 43\%. 

% \cc{I found it awkward to say groud-truth label contains xxxx. Can we just say the image contains a carnivore?} 

% For example, in Figure~\ref{fig:app_example_level1}, the software goes through all the predicted labels of an input image, and executes the \ift \code{return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, we can see that mis-classifications within the pre-defined \wl Animal do not matter, such as mis-classifying an input image with ground-truth label `Dog' to `Wolf'. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. 

% For example, in Figure~\ref{fig:input_example_tf_wrong}, the ML API's output labels lead to incorrect control flow decision because the ground-truth of the input image include a label in the pre-defined \wl (\ie ``Carnivore''), while the output labels do not include any label in the \wl. 

\subsubsection{Software pattern 2: M-to-N-set} In our benchmark, 25\% software defines multiple \wls, and the \wls themselves are parallel to each other. In other words, all the \wls have equivalent priority and all the \wls that have an intersection with the output labels will be reflected in the final output of the software. In Figure~\ref{fig:app_example_non_mut}, the food classifier application invokes ML API to determine the existence of protein, fruit, and grain in a food image\cc{Yuhan, please make sure you introduce what this app is doing before talking about its code structure}. It iterates through the predicted labels of an input image, and executes all the \ifts whose corresponding branch conditions are satisfied. In this example, we can see that mis-classifications within any of the \wls could still lead to correct software behavior.

As shown in Figure~\ref{fig:input_example_mton_correct}, for an input image that includes pasta with meat,  mis-classifying ``Pasta'' to ``Noodle'' does not matter, because the ML API's outputs lead the software to correctly set \code{protein} and \code{grain} variables to \code{True}.
% \cc{Please directly say misclassify which label as which label. The same description already exists in the previous paragraph}. 
However, if an input image has ground-truth labels covering all of the \wls, the correct software behavior is setting \code{protein}, \code{fruit} and \code{grain} to \code{True}. Missing ``Bread'' in the output leads to wrong software behavior: only setting \code{protein} and \code{fruit} variables to \code{True}. 
% \cc{Same here, please describe the example. By looking at this paragraph, it could be applied to any example}.  
% \cc{yuhan, please make the format consistent. Some whitelist names are in code format, some are not}

We also quantitatively measure the difference in the metrics for the ML API and this ML Software's correctness after invoking the ML API. We see that the ML API's F1 score on the food classifier application is 73.88\%. However, only 54.72\% of the input images in which the ML API's output labels lead the software executing all the corresponding \ifts as human expected. 

\subsubsection{Software pattern 3: Priority-list} Around 10\% software defines multiple \wls, and checks the \wls one by one until finding the first one that intersects with output labels. For example, Aander-ETL (Figure~\ref{fig:priority_input_example}) specifies three \wls (\code{Monument, Construction, Person}) to classify tourist photos. It first checks if the output labels have an intersection with the \code{Monument} \wl, and executes the corresponding \ift if having an intersection. If the output labels do not intersect with \code{Monument}, the software compares the output labels with \code{Construction} and \code{Person} in a similar way. Under such software pattern, we can see that mis-classifications for labels inside any of the lower-ranked \wl will not lead to wrong control flow decisions if ML API correctly recognizes the existence of labels in the hig her-ranked \wls. 

In Figure~\ref{fig:input_example_priority_correct}, the software behaves correctly even when the API recognizes an extra incorrect label ``Mansion'' in the \wl \code{ Construction}, as API correctly recognize ``Ancient history'', which belongs to the highest-ranked \wl \code{ Monument}. However, in Figure~\ref{fig:input_example_priority_wrong},  only missing the label ``Landmark'' in the \wl \code{  Monument} can lead to completely incorrect software behavior: the software wrongly executes the \ift corresponding to the second-highest ranked \wl \code{ Construction} since it is the first \wl that intersects with the API's output labels.

We observe that the ML API's overall F1 score for the Anander-ETL software is 61\%, while only 54\% of API's output labels lead to the software executing the \ift corresponding to the highest-ranked \wl included in the input images. 

% for an input image with ground-truth labels that intersect with all the three \wls, the ML API's output labels lead to incorrect control flow decision because missing the label ``Landmark'' in the highest-ranked \wl makes the software executing the \ift corresponding to the second-highest ranked \wl. 


\subsubsection{Software pattern 4: Top-label} For APIs that produce multiple output labels, some software maps the output labels to control flow decisions in a specific order. Around 30\% applications fall in this category.
For example, Heapsortcypher (Figure~\ref{fig:app_example}) iterates through the API output labels that are ranked in descending order of their confidence scores and finds the first output label that intersects with any of the specified \wls. Then the software executes the corresponding \ift associated with the found \wl. Therefore, mis-classification for lower-ranked output labels will not lead to software misbehavior if the higher-ranked output intersects with \wls. 

As shown in Figure~\ref{fig:input_example_top_correct}, API correctly recognizes ``Produce'' for an image of apple on table, which intersects with \wl Compost. Therefore, even it wrongly outputs a lower-ranked label``Wood'' which belongs to another \wl, the software still makes a correct control flow decision. 






\begin{figure}
\begin{subfigure}{0.45\textwidth}    
    \centering
\begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Dog = ['Dog','Mammal','Carnivore','Wolf']
image = types.Image(content=dog_image)
response = client.label_detection(image=image)
for obj in response.label_annotations:
  if obj.name in Dog:
    return 'It is a animal.'
return 'It belongs to others.'
\end{lstlisting}
    \caption{Code pattern: T-or-F. }
    \label{fig:app_example_level1}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
    \caption{Failing recognize the carnivore leads to software failure. }
    \label{fig:input_example_tf_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
    \caption{Mis-classifying a dog as wolf does not trigger software failure. }
    \label{fig:input_example_tf_correct}
\end{subfigure}
\caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
\label{fig:tf_example}
\end{figure}



\begin{figure}
\begin{subfigure}{0.45\textwidth}    

    \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
proteinfoods = ['Hamburger', 'Meat', 'Patty']
fruitfoods = ['Apple', 'Fruit', 'Orange']
grainfoods = ['Noodle', 'Pasta', 'Al dente']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
protein, fruit, grain = False, False, False
for obj in response.label_annotations:
  if obj.name in proteinfoods:
    protein = True
  if obj.name in fruitfoods:
    fruit = True
  if obj.name in grainfoods:
    grain = True
RENDER_TEMPLATE(protein, fruit, grain)
\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_non_mut}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
    \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
    \label{fig:input_example_mton_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
    \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
    \label{fig:input_example_mton_correct}
\end{subfigure}
\caption{Food classifier~\cite{food}, an application that classifies food images.}
\end{figure}


\begin{figure}
    \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
proteinfoods = ['Hamburger', 'Meat', 'Patty']
fruitfoods = ['Apple', 'Fruit', 'Orange']
grainfoods = ['Noodle', 'Pasta', 'Al dente']
image = types.Image(content=trash_image)
response = client.label_detection(image=image)
food_list = []
for obj in response.label_annotations:
  if obj.name in proteinfoods:
    food_list.append('protein')
  if obj.name in fruitfoods:
    food_list.append('fruit')
  if obj.name in grainfoods:
    food_list.append('grain')
return food_list
\end{lstlisting}
    \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
    \label{fig:app_example_non_mut}
\end{figure}



\begin{figure}
\begin{subfigure}{0.45\textwidth}
        \centering
             \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
Monument = ['Landmark', 'Sculpture', 'Monument']
Construction = ['Building', 'Estate', 'Mansion']
Person = ['Human','Person',  'Lady']
image = types.Image(content=landmark_image)
response = client.label_detection(image=image)
Predictions = []
for obj in response.label_annotations:
  Predictions.append(obj.name)
if any([label in Monument for label in Predictions]):
  return 'It belongs to monument.'
elif any([label in Construction for label in Predictions]):
  return 'It is construction.'
elif any([label in Person for label in Predictions]):
  return 'It is person.'
\end{lstlisting}
    \caption{Software implementation. }
    \label{fig:app_example_priority}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
    \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
    \label{fig:input_example_priority_wrong}
\end{subfigure}
\begin{subfigure}{0.45\textwidth}
     \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
    \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
\label{fig:input_example_priority_correct}
\end{subfigure}
\caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
\label{fig:priority_input_example}
\end{figure}

\cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> backups/2-2-empirical-1110.tex <==
\label{sec:empirical}

To understand how developers use ML API in real-world applications\shan{As I commented in Introduction, this opening sentence has to be more precise. It is tooooo generic now.}, we conduct an empirical study on ML software that invokes  ML APIs to make control flow decisions. 

\shan{The overall feeling of this section is lack of motivation. As a reader, I keep asking myself: why do I care how many applications use whitelists? Why do I care how many types of abstraction you use to characterize code structure? Or, why do I care about the whatever code structure? It is not clear to me, as a reader, why any of these have ANYTHING to do with software correctness, with how to customize ML APIs for software. This is related to my comments of your over-general opening sentences. Please keep in mind that readers do NOT necessarily want to ``understand how developers use ML API''. In other words, there are many more readers who want to understand how to customize an ML API to improve software correctness than readers who want to know how many whitelists a software defines. As a reader and an (impatient) reviewer, I skip paragraphs and sections that do not motivate me.}

% \yh{ML API on OI or pretrained on OI}
\subsection{Methodology}

\subsubsection{Application selection}



% Google (benchmark, search), AWS (search)
We study 40 open-source ML software applications  whose control flows are affected by the output of \emph{a multi-label image classification API}. 

We do not study the applications that directly print out the ML APIs' outputs or store these outputs without post-processing. The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

The 40 applications come from two sources: (1) 19 applications, which post-process the ML APIs' outputs to make control flow decisions, come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}\shan{Why do you pick these 19?}; and (2) 21 applications come from GitHub by random checking around 60 applications\shan{What exactly are you looking for when you randomly check? Why don't you use all these 60?}.
Among these applications, 29 use Google \code{label\_detection} API, and 11 use Amazon \code{detect\_labels} API.

% \cc{Maybe also add some statistics}



\subsubsection{Test data selection}
TO-DO
\cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}







% \subsection{Common patterns of code structure of software utilizing ML APIs}
\subsection{Result summary}
The 40 applications whose control flow decisions are affected by the ML APIs' outputs pre-define several \wls, and compare ML APIs' outputs with them to decide which if-branch edge to execute, which we refer to as making application decision. 


\shan{Without knowing your application selection criteria, I cannot interpret what this ``48\%'' implies. What does the remaining 52\% applications do? If all applications in your bencharmk suite use ML API output to affect control flow, how can there be no whitelist? Can you offer more explanation here about what exactly this 48\% mean?} \yh{Sorry 48\% was an out-dated number. All the 40 apps whose control flow are affected by the ML APIs' outputs do specify whitelists. }

Take Heapsortcypher (Figure~\ref{fig:app_example}) as an example. It executes Line 8 when given a garbage image, as the API output ``Glass'' is included in the \code{Recycle} list and thus fulfills the statement in Line 7. 
% We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}\shan{what if there is if-elsif-then?}.
We refer to a list of classes (or classification category) defined in the code\shan{what labels? you mean outputs of an ML API?} leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example\shan{This definition has a lot of flaws.
One quick question: based on your definition, aren't all labels minus those in Recycle, Compost, and Donate also a white list? Are they?
}.

% \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

While these applications typically use \wls to post-process ML API results, they vary in the way of using whitelists to make application decisions. Even with the same whitelists and API outputs, the applications would behave differently according to their code structure. Next, we will introduce the common patterns observed in the studied applications.


% We find that these software typically pre-defines one or several lists of labels as branch conditions, and then maps the original output labels to the pre-defined lists which intersect with the labels. Then the software executes one or more \ifts that correspond to those mapped pre-defined lists. 
% In other words, all the labels specified in one list will lead to the same control flow decision. 

% We refer to the lists of labels leading to the same control flow decisions as \emph{whitelists} in the rest of the paper. For example, in the application example shown in Figure~\ref{fig:app_example}, the software defines three \emph{whitelists}, Recycle, Compost, and Donate. 



% They typically define several lists of labels and which one or more program branches the application should execute by comparing the API output labels and these lists. 
% They typically define several lists of labels and which one or more program branches the application should execute when the ML APIs' output labels intersect with their associated pre-defined list. 


% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X]
% if X == C1: 
%     return "B1"
% elif X == C2: 
%     return "B2"
% elif X == C3: 
%     return "B3"
% elif X == C4: 
%     return "B4"
% \end{lstlisting}
%     \caption{Minimal example showing an application without any post-processing on the ML API's output labels.  }
%     \label{fig:template_0}
% \end{figure}

% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X]
% A = [C1, C2]
% if X in A: 
%     return "X"
% else:
%     return "Y"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_1}
% \end{figure}


% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% A = [c1, c2]
% B = [c3, c4]
% count = 1
% for W in [A, B]:
%     for x in [x1, x2, ...]:



% for x in [x1, x2, ...]:
%     for W in [A, B]:


% for W in [A, B]:
%     if x1 in W or x2 in W:
%         return "branch " + str(count)
%     if X2 in W:
%         return "branch " + str(count)
%     count += 1
% return "branch 3"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_2}
% \end{figure}

% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% A = [C1, C2]
% B = [C3, C4]
% for X in [X1, X2]:
%     if X in A:
%         return "branch 1"
%     if X in B:
%         return "branch 2"
% return "branch 3"
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_3}
% \end{figure}




% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% ML_API_outputs = [X1, X2]
% W1 = [C1, C2]
% W2 = [C3]
% output = set()
% for X in ML_API_outputs:
%     if X in W1:
%         output.add("B1")
%     elif X in W2:
%         output.add("B2")
% return output 
% \end{lstlisting}
%     \caption{Minimal example showing an application that defines a single \wl.}
%     \label{fig:template_4}
% \end{figure}


\subsection{Abstractions}
\label{sec:abstractions}
As summarized in Figure~\ref{fig:hierarchy} we define four types of abstractions to characterize the code structure. 

% We denote the whole set of classes that the DNN behind the ML API is able to classify as $C=\{C_1, C_2, C_3, C_4, C_5, C_6\}$, and the labels that the input images contain as $G$. To start with, Figure~\ref{fig:template_0} shows a minimal example application without any post-processing of the ML APIs' output labels (\eg directly prints out the output labels). The application simply returns the direct output of the ML API. In other words, any one of the ML API's output classes will lead to the software executing its corresponding \ift. In the following section, we will use several minimal templates to illustrate four types of abstractions. 


% Applications may specify a \wl candidate, such that when the API's output labels intersect with the \wl, then the corresponding \ift will be executed, \code{return "B1"} in Figure~\ref{fig:template_1}. In the rest of the paper, we will refer to executing a \ift as mapping the API outputs to its corresponding \wl. In this case, mis-classifications inside the \wl do not matter, as long as the ML API output labels intersect with the \wl for images containing labels in \wl. 

% Applications may specify multiple \wls candidates, and check these whitelists one by one to find the first one that intersects with API result as shown in Figure~\ref{fig:template_2}. In this case, mis-classifications for lower-ranked \wls do not matter, as long as the output labels in higher-ranked whitelists lead to the correct control flow decision. 


\textbf{1) How many \wl candidates does the software define? } The software may specify one or several \wls candidates. Each \wl candidate is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wls candidates. In the rest of the paper, we will refer to executing the \ift as selecting its associated \wl.

\textbf{2) How are the \wls selected? } For the software specifying several \wls, there are three ways such that the \wls are selected: (1) the software checks the \wls in a specific order, and selects at most one \wl when the API outputs intersect with the \wl; (2) the software selects a set of \wls which intersect with API outputs; (3) the software selects an ordered list of \wls which intersect with API outputs. In this case, the order in which the API outputs appear and intersect with the \wls matters. 
 
% (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels are mapped to several \wls; (ii) the software checks whitelists in a specific order, and only executes the lower-ranked \ifts when API outputs do not intersect with any higher-ranked whitelist, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% \cc{I changed it from multiple to several, so that it means 0 to N}

% For the software specifying multiple \wls, when the software checks if the output labels intersect with the \wls, there are two possible ways of checking: (i) the software executes all the \ifts when the API's outputs intersect with the \wls associated with the branch condition. In other words, the original output labels may be mapped to multiple \wls; (ii) the software checks the branch conditions in a specific order, and only executes the lower-ranked \ifts if the higher-ranked branch conditions are false, leading to at most one \ift to be executed. In other words, the original output labels are mapped to at most one \wl. 
% (i) the software executes at most one if/then branch when the API's outputs intersect with the \wl associated with the branch condition; (ii) the software executes all the if/then branches when the API's outputs intersect with the \wls associated with the branch condition. 
% For the software that specifies several \wls, some software will compare the ML APIs' outputs with the \wls, and break at a program branch once the outputs intersect with the \wl associated with the branch. In other words, the final output of the software is the message corresponding to with only one program branch. Other software compares the ML APIs' outputs with the \wls, and outputs all the messages 


\textbf{3) How is the order determined?}  For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.




\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Abstractions that characterize the code structure. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}




\begin{figure*}
     \includegraphics[width=\linewidth]{figs/code.pdf}
    \caption{Examples of software such that the ML APIs' outputs affect the control flow decisions. }
\label{fig:code}
\end{figure*}



\subsection{Common Code Patterns}
\label{sec:examples}
\yh{Currently re-writing this section}
Based on these four types of abstractions, Figure~\ref{fig:hierarchy} summarized all the possible code patterns in a structure of a decision tree. Each decision nodes represent an abstraction. Each leaf node represents a code pattern constructed with the sequences of different decisions made at each decision node. While Figure~\ref{fig:hierarchy} illustrates six possibilities, our studied applications only contain four of them (green box in solid lines).

% Based on these four types of abstractions, we can characterize the common code structures as shown in Figure~\ref{fig:hierarchy}. Each decision node in the decision tree represents an abstraction as described in Section~\ref{sec:abstractions}. Each leaf node in the decision tree represents a type of code structure constructed with the sequences of different decisions made at each decision node. The leaf nodes are all the possible code structures constructed with the abstractions. However, we only found a subset of all the possible code structures in the benchmark suite. The existing types of code structures are shown in the leaf nodes with edges marked with solid lines, whereas the non-exisiting code structures are the leaf nodes with edges marked with dashed lines in Figure~\ref{fig:hierarchy}. We list four patterns of ML software. 
% software examples to illustrate the common patterns of how ML APIs' outputs affect ML software's control flow decisions. 

\subsubsection{Software pattern 1: T-or-F} This type of software only specifies one \wl which includes multiple labels, such that labels in the \wl have an equivalent effect on the software's control flow decisions. Around 35\% of applications in our benchmark suite belong to this category.

As shown in Figure~\ref{fig:code}(a), the application defines a \wl \code{A = [c1, c2]}, and goes through the outputs of the ML API. It  executes the if-branch edge \code{return "branch 1"} when it finds an output class belonging to \code{A}. We refer to executing the if-branch edge as selecting the \wl \code{ A} in the rest of the paper.  If none of the output classes belongs to \code{A}, the application executes the code \code{return "branch 2"}. We refer to executing the code when the ML API's outputs do not match any of the \wls as selecting \code{others}. 

In this application pattern, mis-classifications within the pre-defined \wl do not matter, as long as samples with ground-truth 
% shows a carnivore identification application. It goes through all the predicted labels of an input photo, and executes the \ift \code{ return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, mis-classifications within the pre-defined \wl Animal (\ie mis-classifying a dog image as ``Wolf'') do not lead to software misbehavior. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. On the contrary, if an image contains a carnivore, while the API output do not include any label in the \wl (Figure~\ref{fig:input_example_tf_wrong}). 


% To quantify the difference in the metrics of the ML API and the correctness of this software, the traditional F1 score of the ML API on the test dataset is 58\%, while only 43\% of the data correctly identified classes in the \code{Dog} \wl, leading to software behaviors as human expected. 


% percentage of data such that the software behaves as human expected is 43\%. 

% \cc{I found it awkward to say groud-truth label contains xxxx. Can we just say the image contains a carnivore?} 

% For example, in Figure~\ref{fig:app_example_level1}, the software goes through all the predicted labels of an input image, and executes the \ift \code{return `It is an animal. '} if the predicted labels intersect with the pre-defined \wl Animal. In this example, we can see that mis-classifications within the pre-defined \wl Animal do not matter, such as mis-classifying an input image with ground-truth label `Dog' to `Wolf'. Instead, the ML API only needs to guarantee that the input images that should lead the software executing the \ift corresponding to \wl Animal (\ie having ground-truth labels that intersect with the \wl Animal), are classified into at least one of labels specified in \wl  Animal. 

% For example, in Figure~\ref{fig:input_example_tf_wrong}, the ML API's output labels lead to incorrect control flow decision because the ground-truth of the input image include a label in the pre-defined \wl (\ie ``Carnivore''), while the output labels do not include any label in the \wl. 

\subsubsection{Software pattern 2: M-to-N-set} In our benchmark, 25\% software defines multiple \wls, and the \wls themselves are parallel to each other. In other words, all the \wls have equivalent priority and all the \wls that have an intersection with the output labels will be reflected in the final output of the software. In Figure~\ref{fig:app_example_non_mut}, the food classifier application invokes ML API to determine the existence of protein, fruit, and grain in a food image\cc{Yuhan, please make sure you introduce what this app is doing before talking about its code structure}. It iterates through the predicted labels of an input image, and executes all the \ifts whose corresponding branch conditions are satisfied. In this example, we can see that mis-classifications within any of the \wls could still lead to correct software behavior.

As shown in Figure~\ref{fig:input_example_mton_correct}, for an input image that includes pasta with meat,  mis-classifying ``Pasta'' to ``Noodle'' does not matter, because the ML API's outputs lead the software to correctly set \code{protein} and \code{grain} variables to \code{True}.
% \cc{Please directly say misclassify which label as which label. The same description already exists in the previous paragraph}. 
However, if an input image has ground-truth labels covering all of the \wls, the correct software behavior is setting \code{protein}, \code{fruit} and \code{grain} to \code{True}. Missing ``Bread'' in the output leads to wrong software behavior: only setting \code{protein} and \code{fruit} variables to \code{True}. 
\shan{This example's discussion is confusing. The phenomenon of mis-classifying pasta to noodle does not matter is not unique to this pattern; it applies to the first T-of-F pattern as well. I also don't understand why you emphasize 
``if an input ... has ground-truth labels covering all ...''. Even if the ground truth labels do not cover all but
instead only cover fruit and grain, wouldn't missing bread still a problem? None of your discussion here sounds 
unique to this pattern to me.}
% \cc{Same here, please describe the example. By looking at this paragraph, it could be applied to any example}.  
% \cc{yuhan, please make the format consistent. Some whitelist names are in code format, some are not}

% We also quantitatively measure the difference in the metrics for the ML API and this ML Software's correctness after invoking the ML API. We see that the ML API's F1 score on the food classifier application is 73.88\%. However, only 54.72\% of the input images in which the ML API's output labels lead the software executing all the corresponding \ifts as human expected. 

\subsubsection{Software pattern 3: Priority-list} Around 10\% software defines multiple \wls, and checks the \wls one by one until finding the first one that intersects with output labels. 



% For example, Aander-ETL (Figure~\ref{fig:priority_input_example}) specifies three \wls (\code{Monument, Construction, Person}) to classify tourist photos. It first checks if the output labels have an intersection with the \code{Monument} \wl, and executes the corresponding \ift if having an intersection. If the output labels do not intersect with \code{Monument}, the software compares the output labels with \code{Construction} and \code{Person} in a similar way. Under such software pattern, we can see that mis-classifications for labels inside any of the lower-ranked \wl will not lead to wrong control flow decisions if ML API correctly recognizes the existence of labels in the higher-ranked \wls. 

% In Figure~\ref{fig:input_example_priority_correct}, the software behaves correctly even when the API recognizes an extra incorrect label ``Mansion'' in the \wl \code{ Construction}, as API correctly recognize ``Ancient history'', which belongs to the highest-ranked \wl \code{ Monument}. However, in Figure~\ref{fig:input_example_priority_wrong},  only missing the label ``Landmark'' in the \wl \code{  Monument} can lead to completely incorrect software behavior: the software wrongly executes the \ift corresponding to the second-highest ranked \wl \code{ Construction} since it is the first \wl that intersects with the API's output labels.

% We observe that the ML API's overall F1 score for the Anander-ETL software is 61\%, while only 54\% of API's output labels lead to the software executing the \ift corresponding to the highest-ranked \wl included in the input images. 

% for an input image with ground-truth labels that intersect with all the three \wls, the ML API's output labels lead to incorrect control flow decision because missing the label ``Landmark'' in the highest-ranked \wl makes the software executing the \ift corresponding to the second-highest ranked \wl. 


\subsubsection{Software pattern 4: Top-label} For APIs that produce multiple output labels, some software maps the output labels to control flow decisions in a specific order\shan{???In pattern 3, software maps ... ``in a specific order'' as well.}. Around 30\% applications fall in this category.
For example, Heapsortcypher (Figure~\ref{fig:app_example}) iterates through the API output labels that are ranked in descending order of their confidence scores and finds the first output label that intersects with any of the specified \wls. Then the software executes the corresponding \ift associated with the found \wl. Therefore, mis-classification for lower-ranked output labels will not lead to software misbehavior if the higher-ranked output intersects with \wls. 

As shown in Figure~\ref{fig:input_example_top_correct}, API correctly recognizes ``Produce'' for an image of apple on table, which intersects with \wl Compost. Therefore, even it wrongly outputs a lower-ranked label``Wood'' which belongs to another \wl, the software still makes a correct control flow decision. 

\shan{What is the F1 score drop for this category?}






% \begin{figure}
% \begin{subfigure}{0.45\textwidth}    
%     \centering
% \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Dog = ['Dog','Mammal','Carnivore','Wolf']
% image = types.Image(content=dog_image)
% response = client.label_detection(image=image)
% for obj in response.label_annotations:
%   if obj.name in Dog:
%     return 'It is a animal.'
% return 'It belongs to others.'
% \end{lstlisting}
%     \caption{Code pattern: T-or-F. }
%     \label{fig:app_example_level1}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
%     \caption{Failing recognize the carnivore leads to software failure. }
%     \label{fig:input_example_tf_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
%     \caption{Mis-classifying a dog as wolf does not trigger software failure. }
%     \label{fig:input_example_tf_correct}
% \end{subfigure}
% \caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
% \label{fig:tf_example}
% \end{figure}



% \begin{figure}
% \begin{subfigure}{0.45\textwidth}    

%     \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% proteinfoods = ['Hamburger', 'Meat', 'Patty']
% fruitfoods = ['Apple', 'Fruit', 'Orange']
% grainfoods = ['Noodle', 'Pasta', 'Al dente']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% protein, fruit, grain = False, False, False
% for obj in response.label_annotations:
%   if obj.name in proteinfoods:
%     protein = True
%   if obj.name in fruitfoods:
%     fruit = True
%   if obj.name in grainfoods:
%     grain = True
% RENDER_TEMPLATE(protein, fruit, grain)
% \end{lstlisting}
%     \caption{Software implementation. }
%     \label{fig:app_example_non_mut}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
%     \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
%     \label{fig:input_example_mton_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
%     \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
%     \label{fig:input_example_mton_correct}
% \end{subfigure}
% \caption{Food classifier~\cite{food}, an application that classifies food images.}
% \end{figure}


% \begin{figure}
%     \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% proteinfoods = ['Hamburger', 'Meat', 'Patty']
% fruitfoods = ['Apple', 'Fruit', 'Orange']
% grainfoods = ['Noodle', 'Pasta', 'Al dente']
% image = types.Image(content=trash_image)
% response = client.label_detection(image=image)
% food_list = []
% for obj in response.label_annotations:
%   if obj.name in proteinfoods:
%     food_list.append('protein')
%   if obj.name in fruitfoods:
%     food_list.append('fruit')
%   if obj.name in grainfoods:
%     food_list.append('grain')
% return food_list
% \end{lstlisting}
%     \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
%     \label{fig:app_example_non_mut}
% \end{figure}



% \begin{figure}
% \begin{subfigure}{0.45\textwidth}
%         \centering
%              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% Monument = ['Landmark', 'Sculpture', 'Monument']
% Construction = ['Building', 'Estate', 'Mansion']
% Person = ['Human','Person',  'Lady']
% image = types.Image(content=landmark_image)
% response = client.label_detection(image=image)
% Predictions = []
% for obj in response.label_annotations:
%   Predictions.append(obj.name)
% if any([label in Monument for label in Predictions]):
%   return 'It belongs to monument.'
% elif any([label in Construction for label in Predictions]):
%   return 'It is construction.'
% elif any([label in Person for label in Predictions]):
%   return 'It is person.'
% \end{lstlisting}
%     \caption{Software implementation. }
%     \label{fig:app_example_priority}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
%     \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
%     \label{fig:input_example_priority_wrong}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
%      \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
%     \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
% \label{fig:input_example_priority_correct}
% \end{subfigure}
% \caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
% \label{fig:priority_input_example}
% \end{figure}

% \cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> backups/2-2-empirical-1117.tex <==
\label{sec:empirical}

This section introduces how ML API influences the behavior of MLaaS applications and then motivates:  
(1) the need to customize the ML API backend for each application, and 
(2) common patterns in which ML API output affects an application's decision process.
\subsection{Definitions}

% In addition, ML APIs are only loosely integrated into these applications, e.g., not interacting with other software components. We believe they do not represent the future direction of ML software.

% The 40 applications come from two sources: (1) 19 applications, which post-process the ML APIs' outputs to make control flow decisions, come from a recently published, open-sourced benchmark suite for ML software~\cite{wan2021machine}\shan{Why do you pick these 19?}; and (2) 21 applications come from GitHub by random checking around 60 applications\shan{What exactly are you looking for when you randomly check? Why don't you use all these 60?}.
% Among these applications, 29 use Google \code{label\_detection} API, and 11 use Amazon \code{detect\_labels} API.

% \cc{Maybe also add some statistics}



% \subsubsection{Test data selection}
% TO-DO
% \cc{It is weird to have a subsection that only has one subsubsection. How about we also introduce the open image data and ground-truth label?}


\begin{figure}
     \includegraphics[width=.95\linewidth]{figs/motivate_2examples.pdf}
    \caption{Code snippets from two example applications. Branch conditions influenced by API output and the structures over the conditional branches are highlighted.}
\label{fig:2examples}
\end{figure}

\mypara{Preliminaries} We begin with basic definitions.
% We first define the terminologies used in our paper.



% \begin{itemize}
%     \item \emph{Application decision}: the control flow decision of  which ML-API-related branch edge to execute
%     \item \emph{Conditional branches}: the lists of classes the application pre-defines in their source code, such that classes in these lists will lead to the same application decision. \yh{needs polish}
%     \item Selecting a whitelist $A$: the process of executing the branch edge corresponding to whitelist A
%     \item Selecting \code{others}: the process of executing the branch edge for not selecting any \wls
%     \item \emph{Ground-truth decision}: the application decision led by the human-labeled ground-truth of the input
% \end{itemize}


\begin{packeditemize}
    \item {\em ML API output:} the output of the MLaaS in response to the invocation of a single input, \eg a list of classes describing the content of an input image or the scores indicating the sentiment of the input text.
    % \item \emph{Conditional branches}: the branch conditioned on the API outputs 
    \item \emph{Branch conditions:} once the application receives the API output, it uses the branch conditions to decide which branch or branches to execute based on the API outputs.
    % \item \emph{Target-edge:} the branch edge that is executed when the API outputs fulfill a branch condition.%predicate of containing certain values. It typically is the edge following \code{then} statement.
    % \item \emph{A-edge}: for applications that compare API outputs with arrays of classes (\eg \code{A, B, C}), we refer to the Target-edge that is executed when the branch condition using array \code{A} is fulfilled as \emph{A-edge}.
    % \item \emph{Otherwise-edge}: the edge that is executed when none of the Target-edge is executed. 
    % \item \emph{Fall-through edge}: The non-target edge of a branch.
    % \item \emph{Path}: A feasible combination of edges of all conditional branches.
    % \item \emph{Target-path}: A path that contains at least one target edge.
    
    % % \item \emph{Whitelist}: A whitelist is a set of all ML API outputs that lead software to execute its corresponding whitelist-path.
    % \item \emph{Otherwise-path}: A path without any target edge. \cc{Please feel free to remove any concepts that are needed}
    \item \emph{Application decision}: given particular ML API output, the branch or branches whose branch conditions are satisfied.\footnote{Here, it is implicitly assumed that the application decision is affected only by the ML API output on the current input, not previous API output. While this may not be universally true, it holds for all the real-world applications that we have studied.}
    % the decision of which \emph{Target-edge} or \emph{Otherwise-edge} to execute. 
    % \item Selecting a whitelist $A$: the process of executing the branch edge corresponding to whitelist A
    \item \emph{Ground-truth decision}: the application decision if the API output is  human-labeled ground-truth of the input. 
    % \item \emph{Critical errors}: the errors that lead the application to execute edges different from the ground-truth decisions.
\end{packeditemize}


\mypara{Software decision process}
Given these definitions, an application's {\em software decision process} is the logic that maps an ML API output to an application decision. 
The code snippet in Figure~\ref{fig:input_example} shows an example software decision process, which maps the output of a classification ML API on an image to the image's recycling categorization specific to this application.

\mypara{Critical and non-critical errors}
Importantly, each software decision process decides when different ML API outputs lead to the same ground-truth decision (defined above), \ie {\em non-critical} error of ML API output {\em vs.} when different ML API outputs lead to decisions different from the ground-truth decision, \ie {\em critical} error of ML API output.

As we will see, the key is that {\em not} all errors are critical and that the critical errors {\em vary} across applications (using the same ML API) due to their different application decision processes.
%Thus, each application's decision process, if used carefully, could be leveraged to improve ML API output to reduce wrong application decisions. 
In the remainder of the section, we first present a systematic taxonomy of application decision processes and then apply the taxonomy to analyze a range of real-world applications using commercial MLaaS ML APIs.
%However, to unleash such potential in practice, we first need a deep understanding on the software contexts of various applications using real MLaaS {\em in the wild}.
In this empirical analysis, we focus on two central questions:
\begin{packeditemize}
\item Among applications using the same ML API, how much they differ in their application decision processes, and 
\item Despite the application heterogeneity, whether common patterns emerge which might allow extraction of information regarding an application's decision process.
\end{packeditemize}



\begin{figure}
     \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
    \caption{Key dimensions that differentiate the code structures. The decision nodes (in blue) are key dimensions. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
\label{fig:hierarchy}
\end{figure}



%\subsection{\hspace{-0.2cm} How ML API affects conditional branches}
\subsection{How is an application decision process affected by ML API?}
%\subsection{Taxonomy on how ML APIs affect application decision process}

\jc{text in this section can be tightened..}

%For each of these applications in our study, its software context is determined along two dimensions
% An application decision process can be characterized in two dimensions:
Two application decision processes may differ along one (or both) of the following dimensions:
{\em (i)} how each branch condition uses ML API output, and
{\em (ii)} how the conditional branches are structured.


\yh{be more precise about the titles, ask questions, define it and measure it }

\mypara{Two types of API output-based branch conditions}
% We identify two types of conditional branches
Figure~\ref{fig:2examples} shows an illustrative example for each.
%\item{\em Class lists:} 
The first type is used when the API output is a label or a list of labels, and several pre-defined {\em class lists} are then used to check if the API output labels belong to which list.
The code snippet of \code{Heapsortcypher}~\cite{heapsort} in Figure~\ref{fig:2examples}(a), for example, calls MLaaS with an image and receives class labels as ML API output.
It then checks if the API output belongs to three lists of classes, \code{Recycle}, \code{Compost}, \code{Donate} as the branch conditions to decide which branch to execute.
For an input with ground-truth class \code{``Shirt''}, the ground-truth decision is to execute the \code{Donate} branch.
If the ML API output is \code{``Paper''}, it will be a critical error, because the application decision (the \code{Recycle} branch) deviates from the ground-truth decision, whereas, if the ML API output is \code{``Jacket''}, it is not a critical error since the application's decision remains the same as the ground-truth decision.
%For example, the branch conditions in the \code{Heapsortcypher} application check if each API output class belongs to one of the three pre-defined lists. 
% \shan{This example is already discussed in the Introduction.}

%\item{\em Value ranges:}



The second type of branch condition is used when the API output is a score, and several pre-defined {\em value ranges} are then used to check if the API output scores fall in which range. 
The code snippet of \code{FoodDelivery}~\cite{food-delivery} in Figure~\ref{fig:2examples}(b), for example, calls MLaaS with a text sentence and receives a sentiment score as the ML API output. 
It uses three branch conditions, each checking if the API output score lies in a certain range. 
Given an input sentence whose ground-truth label is ``positive'', the ground-truth decision will print \code{It's a positive sentence}, and a critical error in this case will be when the API outputs a score lower than 0.6 on this sentence. 

% \shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
%As shown in the \code{FoodDelivery} application in Figure~\ref{fig:input_example}(b), it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text. 
%The branch condition checks whether the score is over 0.6 (\ie the text is positive) or below 0.3 (\ie the text is negative), or otherwise (neutral). 
%\end{packeditemize}



%While these concepts may sound high-level, let us make them more concrete using two real-world applications, \code{Heapsortcypher} (Figure~\ref{fig:input_example}(a)) and \code{Food-delivery} (Figure~\ref{fig:input_example}(b)).
%
%\begin{packeditemize}
%\item 
%
%%\shan{This example is already discussed in the Introduction.}
%
%\item 
%%\shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
%\end{packeditemize}


\begin{figure*}
     \includegraphics[width=\linewidth]{figs/code.pdf}
    \caption{Examples of software such that the ML APIs' outputs affect the control flow decisions. }
\label{fig:code}
\end{figure*}


\mypara{Common structures over conditional branches}
Given the conditional branches, the way these branches are structured can also greatly affects the application decision process.
The structures over conditional branches differ along three key dimensions.
(1) the {\em number of conditional branches}; 
(2) the {\em number of executed branches} (for applications with several conditional branches, the application can either execute the first satisfied branch or all branches that satisfy the branch conditions); and finally
(3) the {\em order of examination}---when there are multiple elements in an ML API output {\em and} multiple conditional branches, an application can choose to examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
%\begin{packeditemize}
%\item {\em Number of conditional branches:} The applications may define one or several branch conditions. 
%\item {\em Number of executed branches:} For applications with several conditional branches, the application can either execute the first satisfied branch or all branches that satisify the branch conditions. 
%\item {\em Order of examination:}  
%When there are multiple elements in an ML API output {\em and} multiple conditional branches, an application can choose to examine each element one by one against the conditional branches (\ie examining the $1^{\textrm{st}}$ element in API output against all branch conditions before moving to the $2^{\textrm{nd}}$ element, and so forth) or examine all elements against each conditional branch (\ie examining all elements against the $1^{\textrm{st}}$ branch condition, then all elements against the $2^{\textrm{nd}}$ condition, and so forth). 
%%Applications that execute at most one branch  may either iterate through branch conditions first or the API outputs first in a two-level for loop. 
%\end{packeditemize}

With these dimensions, we identify four structures over conditional branches (Figure~\ref{fig:hierarchy}). 
Figure~\ref{fig:code} depicts a simple illustrative example of each structure.
\jc{we need to replace these names with macros. they will definitely be changed.}
\jc{yuhan, can you explain these categories using the three dimensions just introduced? what's the point of introducing the dimensions without actually using them?}
\begin{packeditemize}
\item {\em T-or-F:} Figure~\ref{fig:code}(a) is an example code structure where the first key dimension is only one branch condition. The application checks if the API outputs intersect with the list \code{A}. If so, it executes the branch \code{return "branch 1"}, otherwise, the branch \code{return "branch 2"} is executed. 
\item {\em M-to-N-set:}  Figure~\ref{fig:code}(b) is an example where it falls into the category of (1) defining more than one branch condition at the first key dimension; (2) executing a set of branches at the second key dimension.  The application defines two branch conditions in the for loop. If any of the branch conditions are fulfilled, the branch will be executed (\ie adding the message corresponding to the branch to the final output set). 
\item {\em Priority-list:} This type of applications define several class lists, and check the class lists in order until finding the first one that intersects with the API outputs. Figure~\ref{fig:code}(c) is an example of this code structure, and it falls into the category of (1) defining more than one branch condition at the first key dimension; (2) executing at most one branch; (3) first enumerate the branch conditions first at the third key dimension. 
\item {\em Top-label:} This type of applications iterate over the API outputs until finding one that intersects with any of the defined class lists, as shown in Figure~\ref{fig:code}(d). 
\end{packeditemize}





% \mypara{Software context}
% Given these definitions, we define the software context of an application as the {\em critical errors} on the ML API output that will lead to different application decisions than the ground-truth decisions\shan{???I don't quite get it}.
% While these applications may sound high-level, let us make them more concrete using two real-world applications, \code{Heapsortcypher} (Figure~\ref{fig:input_example}(a)) and \code{Food-delivery} (Figure~\ref{fig:input_example}(b)).

% \begin{packeditemize}
% \item 
% The code snippet of \code{Heapsortcypher} in Figure~\ref{fig:input_example}(a) calls MLaaS with an image and receives class labels as ML API output.
% It then checks if the API output belongs to three lists of classes, \code{Recycle}, \code{Compost}, \code{Donate} as the branch conditions to decide which branch to execute.
% % , so that 
% % % s. Each of the branch conditions 
% % checks if the API output belongs to the list of classes associated with the branch. 
% For an input with ground-truth class \code{``Shirt''}, the ground-truth decision is to execute the \code{Donate} branch.
% % \emph{Target-edge} associated with the \code{Donate} list. 
% If the ML API output is \code{``Paper''}, it will be a critical error, because the application decision will be the \code{Recycle} branch, deviating from the ground-truth decision.
% % is executing the \emph{Target-edge} associated with the \code{Recycle} list. This application decision deviates from the ground-truth decision, thus forming a critical error. 
% Nevertheless, if the ML API output is 
% % mis-classifies the Shirt image to 
% \code{``Jacket''}, it is not a critical error since the application's decision remains the same as the ground-truth decision.
% % is still executing the \emph{Target-edge} associated with the \code{Donate} edge.
% \shan{This example is already discussed in the Introduction.}

% \item The code snippet of \code{FoodDelivery} in Figure~\ref{fig:input_example}(b) calls MLaaS with a sentence and receives a sentiment score as the ML API output. 
% It uses three branch conditions, each checking
% % . Each branch condition checks 
% if the API output score lies in a range. Given an input sentence whose ground-truth label is ``positive'', the ground-truth decision will execute the branch that prints \code{It's a positive sentence}, and a critical error in this case will be when the API outputs a score lower than 0.6 on this sentence. 
% \shan{I am not totally sure about this arrangement. We already motivated somewhat in Introduction. How about we put any extra examples to a bit later when we discuss our empirical study result? It will also help move the pace faster into the empirical study.}
% \end{packeditemize}

% Importantly, these examples show that {\em not} all errors are critical errors, and thus such per-application software context, if used carefully, could improve ML API output to reduce wrong application decisions. 
% However, to unleash such potential in practice, we first need a deep understanding on the software contexts of various applications using real MLaaS {\em in the wild}.


% \mypara{An empirical study over real MLaaS applications}
% To this end, in the remainder of this section, we run an empirical study over 77 open-source applications which collectively use 6 ML APIs.
% These applications are selected from a recently published benchmark suite~\cite{wan2021machine}.
% We keep all applications except those that directly print out or store the ML API outputs without post-processing (for these applications, by definition any errors of API output will be critical).

% Our empirical analysis focuses two central questions:
% (1) among applications using the same ML API, how much they differ in their software context (critical errors), and 
% (2) despite the application heterogeneity, whether common patterns emerge which might allow automatic extraction of software context.  



% \subsection{\hspace{-0.2cm} Use of API output in conditional branches}


% For each of these applications in our study, its software context is determined along two dimensions
% {\em (i)} the branch conditions that use API output, and
% {\em (ii)} the structure over the branch conditions.Two applications' software contexts can differ along either or both dimensions. 

% \mypara{Use of API output in branch conditions}
% Depending on the API output, we identify two types of conditional branches. 
% \begin{packeditemize}
% \item{\em Class lists:} The first type is used when the API output is a label or a list of labels, and it checks if the API output labels belong to several pre-defined lists of classes.
% For example, the branch conditions in the \code{Heapsortcypher} application check if each API output class belongs to one of the three pre-defined lists. 
% \item{\em Value ranges:}
% The second type of branch condition is used when the API output is a score, and it  then checks if the API output scores fall in several pre-defined value ranges. 
% As shown in the \code{FoodDelivery} application in Figure~\ref{fig:input_example}(b), it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text. 
% The branch condition checks whether the score is over 0.6 (\ie the text is positive) or below 0.3 (\ie the text is negative), or otherwise (neutral). 
% \end{packeditemize}


% \mypara{Structures of conditional branches}
% Given the API output and conditional branches, the way these conditional branches are structured can also greatly affect the application decision.
% The structures of conditional branches differ along three key dimensions, shown in Figure~\ref{fig:hierarchy}:
% \begin{packeditemize}
% \item Number of branch conditions: The applications may define one or several branch conditions. 
% \item Number of executed branches: For applications that define several branch conditions, the application can either execute at most one branch or execute a set of branches that fulfill the branch conditions. 
% \item Order of examination:  Applications that execute at most one branch  may either iterate through branch conditions first or the API outputs first in a two-level for loop. 
% \end{packeditemize}

% Along these dimensions, we carefully categorize the conditional branch structure of each application in our study.
% Four common structures emerge.
% \begin{packeditemize}
% \item T-or-F: As shown in Figure~\ref{fig:code}(a), the application defines one branch condition to check if the API outputs intersect with the list \code{A}. If so, it executes the branch \code{return "branch 1"}, otherwise, the branch \code{return "branch 2"} is executed. 
% \item M-to-N-set: As shown in Figure~\ref{fig:code}(b), the application defines two branch conditions in the for loop. If any of the branch conditions are fulfilled, the branch will be executed (\ie adding the message corresponding to the branch to the final output set). 
% \item Priority-list: This type of applications define several class lists, and check the class lists in order until finding the first one that intersects with the API outputs. Figure~\ref{fig:code}(c) is an example of this code structure.  
% \item Top-label: This type of applications iterate over the API outputs until finding one that intersects with any of the defined class lists, as shown in Figure~\ref{fig:code}(d). 
% \end{packeditemize}

















\subsection{\hspace{-0.25cm}Empirical study of application heterogeneity}


{\em As a consequence of the application decision processes, not all errors are critical.
And because each application has unique conditional branches and its structure over these branches, their critical errors are greatly different. 
}

\mypara{An empirical study over real MLaaS applications}
To this end, in the remainder of this section, we run an empirical study over 77 open-source applications which collectively use 6 ML APIs.
These applications are selected from a recently published benchmark suite~\cite{wan2021machine}.
We keep all applications except those that directly print out or store the ML API outputs without post-processing (for these applications, by definition, any errors of API output will be equally critical, so there is little room for improvement by customizing the model based on critical errors.)

\mypara{How code structures affect critical errors of API output}
If a misclassification occurs within a class list associated to the same conditional branch, then it is not a critical error. 
But it would be a critical error, if an image is misclassified with a label in the class list of a different conditional branch than the ground-truth label.

Even with the same branch conditions, the critical errors can differ depending on the structure of the conditional branches.

Take the code structures in Figure~\ref{fig:code} as an example. Figure~\ref{fig:code}(b)(c)(d) defines two same class lists. Given an input  with ground-truth class \code{c1} and API outputs \code{[c3, c1]}. The ground-truth decision is execute the branch corresponding to \code{A}. For M-to-N-set, this API output leads the execution of branches corresponding to class lists \code{A} and \code{B}, thus forming a critical error. However, for Priority-list, this API output correctly leads the application to execute the branch corresponding to \code{A}. On the other hand, Top-label iterates over the outputs and breaks at the branch corresponding to \code{B}, which is also a critical error for the application. 


% \jc{Yuhan, please fill in}

\mypara{Empirical observations on application heterogeneity}
Figure~\ref{tab:stats} enumerates the conditional branches used in the applications under our study and assigns each application to one of the aforementioned structures. 
We make three empirical observations.
\begin{packeditemize}
\item In each application, {\em the number of pre-defined class lists and value ranges are relatively small}, indicating a potential for MLaaS to increase accuracy on specific classes by customizing (retraining) the ML models behind ML API. 
Collectively, set of classes in the class lists is relatively small compared to the number of classes in a typical classification training dataset (\eg 9605 classes in OpenImages~\cite{openimages} or 1000 classes in ImageNet~\cite{5206848}). 
\item More importantly, there are {\em very few overlaps among the branch conditions of different applications}, making a case for {\em per-application} customization of ML API backend model.
Specifically, among all (826 \footnote{We separately count the pairs for the 40 Vision tasks and 5 NLP entity recognition task, and 36 NLP text classification tasks as they do not share label sets}) pairs of applications with class-list-based branch conditions, only 71 of them overlap by more than one classes between their class lists. 
Similarly, among the 381 classes that appear in at least one application's branch conditions, only 16 of them appear in more than three applications.
\item Similarly, the structure over the conditional branches also varies greatly across applications, though four common patterns are enough to cover them. Out of the applications we study, 32\% of applications are T-or-F, 23\% of them fall into the pattern of M-to-N-set, 8\% of them are M-to-N-set, and the rest of them are Top-label.
% \jc{a few words on this}
\end{packeditemize}



% \mypara{An empirical study over real MLaaS applications}
% % Given the rich syntax that can be expressed by Python, critical errors for applications in the wild can be very different.
% % To understand common types of software context that affect the application decisions, we first perform 
% To this end, in the remainder of this section, we run an empirical study over 78 open-source applications  whose application decisions 
% % control flow decisions 
% which collectively use \fillme ML APIs.
% These applications are from a recently published benchmark suite~\cite{wan2021machine}~\footnote{
% We ignore applications that directly print out the ML API outputs or store these outputs without post-processing, and thus by definition any errors of API output will be critical.
% % The tasks that these applications perform are the same as the task of ML API. Therefore, there is no need to adapt APIs to software. 
% }. 
% These applications cover a wide range of use cases, from \fillme to \fillme. 



% % Google (benchmark, search), AWS (search)

% % \begin{definition}[Application decision]\label{def:app_decision}
        
% % \end{definition}

% % These applications compare the ML API's output classes with the applications' pre-defined lists of classes, and decide which if-branch edge to execute. We refer to this process as making \textit{application decisions} and the pre-defined lists of class as \wls. 



% % \shan{Without knowing your application selection criteria, I cannot interpret what this ``48\%'' implies. What does the remaining 52\% applications do? If all applications in your bencharmk suite use ML API output to affect control flow, how can there be no whitelist? Can you offer more explanation here about what exactly this 48\% mean?} \yh{Sorry 48\% was an out-dated number. All the 40 apps whose control flow are affected by the ML APIs' outputs do specify whitelists. }

% % The application goes through a list of conditional branches based on API outputs, whether a branch is executed is determined by if the API outputs matches with the branch condition or not 

% % \yh{use sentiment analysis, the way to map conditional branch to app decisions is different }


% % The application defines three \wls, \code{Recycle, Compost, Donate}. 
% % The human labeled ground-truth of the input image is ``Shirt'', so the ground-truth decision is executing the if-branch edge \code{return donate(trash\_image)}, which we refer to as selecting the \code{Donate} whitelist. 
% % Furthermore, if the ML API's outputs lead the application to make the decision of executing the code \code{return "It is others." }, such as outputting class ``Dog'', we refer to this decision as selecting \code{others}. 

% % We refer to this executed branch as \emph{if/then branch}. Correspondingly, we refer to another branch that  not executes Line 8 as \emph{if/else branch}\shan{what if there is if-elsif-then?}.
% % We refer to a list of classes (or classification categories) defined in the code\shan{what labels? you mean outputs of an ML API?} leading to the same control flow decision as a \emph{whitelist}. \code{Recycle}, \code{Compost}, and \code{Donate} are the three whitelists, taking Heapsortcypher as an example
% \shan{This definition has a lot of flaws.
% One quick question: based on your definition, aren't all labels minus those in Recycle, Compost, and Donate also a white list? Are they?
% }

% % \cc{yuhan, please put terminologies (those used in Section 3) here. Make sure that you are only using the Heapsortcypher as an example}

% % While these applications typically use \wls to post-process ML API results, they vary in the way of using whitelists to make application decisions. Even with the same whitelists and API outputs, the applications would behave differently according to their code structure. Next, we will introduce the common patterns observed in the studied applications.

% % We find that the common software context consists of two components: (1) Types of branch conditions (\eg checking if the API output belongs to a list of classes), details described in Section~\ref{sec:content}; (2) The organization of conditional branches, details in Section~\ref{sec:org}. 




% \begin{figure}
%     \centering
%      \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% sentiment_text = types.Document(content = a_piece_of_text)
% annotations = client.analyze_sentiment(document=sentiment_text)
% sentiment_score = annotations.document_sentiment.score
% if sentiment_score < 0.3:
%     print("It's a negative sentence!")
% elif sentiment_score > 0.6:
%     print("It's a positive sentence!")
% else:
%     print("It's a neutral sentence!")
% \end{lstlisting}
%     \caption{The code snippet in the app \code{FoodDelivery}~\cite{food-delivery} calls Google's analyze\_sentiment API to determine the sentiment of a given text.}
%     \label{fig:sentiment}
% \end{figure}


% \subsection{Types of the branch conditions}
% \label{sec:content}
% % \yh{2.1 => what does the context entail, 2.2 and 2.3, differs from ...., but follows a set of common structure, not arbitrary }

% Our study reveals two types of conditional branches, comparing the API outputs with lists of classes, or setting ranges to branch the API outputs. 

% \subsubsection{Lists of classes} 


% % \begin{figure}
% %      \includegraphics[width=.8\linewidth]{figs/stats.pdf}
% %     \caption{ The number of classes included in the lists used to make application decisions. }
% % \label{fig:stats}
% % \end{figure}


% The Applications calling APIs that output categorical results (\eg image classification) 
% pre-define lists of classes, and compare the API outputs with the lists, to make the application decision. For example, the branch conditions in the \code{Heapsortcypher} application check if the API output class belongs to one of the three pre-defined lists. We observe that the lists the applications define typically cover only a very small subset of whole label set. In Figure~\ref{fig:stats}, we summarized the number of classes included in the lists used to make application decisions in our study. Out of the 9605 \yh{double check this number} classes that are covered in Google's classification API, the lists of classes used by the applications to make decisions include less than 20 classes.

% Since the ML API  is typically optimized on a much wider range of classes, the focus on the small subsets classes defined by the applications indicates great room for improvement on the ML API. 


% \subsubsection{Setting ranges}

% Some  applications  call APIs that output floating point values. As shown in the \code{Cloud-computing} application in Figure~\ref{fig:sentiment}, it calls Google's \code{analyze\_sentiment} API to output a score indicating the emotional opinion of the input text, where a score closer to 1 indicates the text is more positive, and a score closer to -1 is more negative. In this case, the  branch condition is checking if the predicted score falls into a specific range. 



% \subsection{How the branch conditions are organized}
% \label{sec:org}

% % \yh{Can those branch conditions directly determine how the application decisions, how the branches are structured => affects the critical errors}
% % \yh{Bad news: there's no one structure, good news: a handful of structures }
% A thoughtful reader may wonder: Does identifying the content of the branch conditions enough to determine the application decisions?


% % Can the branch conditions themselves enough to  determine the application decisions? 

% The answer is no. Our study reveals that even when the content of the branch conditions are the same (\ie defining the same lists of classes as branch conditions), the application decision may still be different based on how the  branch conditions are organized 

% Fortunately, we can classify different organization of branch conditions into a handful of categories. To illustrate the different ways the organization of conditional branches affects the application decision, we begin with defining three key abstractions.


% \subsubsection{Key Abstractions}
% \label{sec:abstractions}
% As summarized in Figure~\ref{fig:hierarchy} we define three types of abstractions to characterize the code structure. 


% \textbf{1) Number of branch conditions } The applications may define one or several branch conditions. If the applications only define one branch condition, whether to execute the branch or not only depends on if API outputs fulfill the only branch condition or not. On the other hand, for applications that define several branch conditions, the application decisions are also affected by other aspects. 
% % The software may specify one or several \wls candidates. Each \wl candidate is related to a particular software branch: the software will execute the corresponding \ift when the ML APIs' outputs intersect with the labels in the \wls candidates. In the rest of the paper, we will refer to executing the \ift as selecting its associated \wl.

% \textbf{2) Number of executed target-paths} Applications that define more than one branch condition can either (1) execute at most one branch; (2) execute the set of branches that fulfill 
%  their branch conditions. 



% \textbf{3) Order of examination}  Applications that execute at most one branch define a two-level nested loop to determine the branch to execute. The applications may iterate through branch conditions in the outer loop or the API outputs in the outer loop. 
% % For the software specifying multiple \wls, the order of examining intersections between \wls and ML API outputs determines software behavior. If we reconstruct the examination into a two-level nested loop that iterates through \wls and API outputs, there naturally arises two types of loop structure: prioritize the specified \wls or the API output labels.


% \begin{figure}
%      \includegraphics[width=\linewidth]{figs/hierarchy.pdf}
%     \caption{Abstractions that characterize the code structure. The decision nodes (in blue) are abstractions defined in Section~\ref{sec:abstractions}. The leaf nodes (in green) are the type of code structures constructed with the sequence of decisions made at each decision node. }
% \label{fig:hierarchy}
% \end{figure}



% \subsubsection{Common branch condition structures}
% \label{sec:examples}

% Based on these three types of abstractions, we can classify the common code structures into four categories shown in Figure~\ref{fig:hierarchy}. Each decision node represents an abstraction. Each leaf node represents a structure of branch conditions constructed with the sequences of different decisions made at each decision node. 

% In the following section, we explain the common branch condition structures with simple code snippets. 

% \subsubsection{Branch condition structure 1: T-or-F} The applications with this pattern only specifies one branch condition on the API outputs. Around 32\% of applications in our benchmark suite belong to this category.

% As shown in Figure~\ref{fig:code}(a), the application defines one branch condition to check if the API output belongs to the pre-defined list \code{A}. 

% \textbf{Input example} In this application pattern, given inputs with ground-truth decision of executing the \code{A} branch, the critical error is failing to include any of classes in \code{A} in API outputs.


% \subsubsection{Branch condition structure 2: M-to-N-set} 
% \label{sec:m_to_n}
% In our benchmark, 23\% applications define several branch conditions, and execute the set of branches whose branch conditions are fulfilled based on API outputs. 

% As shown in Figure~\ref{fig:code}(b), the application iterates over the API outputs with a for loop. Inside the for loop, two branch conditions are defined to check if the API output belongs to the lists \code{A} or \code{B}. If the API output belongs to the list \code{A}, the branch \code{final\_output.add("branch 1")} is executed. If the API output belongs to the list \code{B}, the branch \code{final\_output.add("branch 2")} is executed. 

% \textbf{Input example} In this case, given an input  whose ground-truth is \code{c1}, the ground-truth decision is only executing the branch \code{final\_output.add("branch 1")}. When the API outputs \code{[c3, c1]}, both \code{final\_output.add("branch 1")} and \code{final\_output.add("branch 2")} are executed. This output forms a critical error in M-to-N-set. 



% % defines two \wls, \code{A} and \code{B}, and iterates through the ML API's outputs, and adds the string \code{"branch 1"} to the final output set if the outputs intersect with the whitelist \code{A}, and adds the string \code{"branch 2"} to the final output set if the outputs intersect with the whitelist \code{B}. 

% % In this pattern, mis-classifications inside \ do not matter, as long as the ML API's output classes include at least one class in the \wls that should be selected in the ground-truth decision, and not include any class in the \wls that are not in ground-truth decision. 

% % \yh{
% % Given the ground-truth is [Bread, Cheese]

% % Critical errors: failed to include any class in Grainfoods and Proteinfoods, and including any one class in fruitfoods

% % }


% \subsubsection{Branch condition structure 3: Priority-list}
% \label{sec:priority}Around 8\% software defines multiple branch conditions, and check the branch conditions one-by-one until the API outputs fulfill the condition. If none of the conditions are fulfilled, the branch \code{return ``branch 3''} is executed. 

% For example, in Figure~\ref{fig:code}(c), the application defines two lists of classes,  \code{A} and \code{B}, and iterates over the two lists. If any of the API outputs belongs to \code{A}, the application makes the decision of executing the branch \code{return "branch 1"}. If not, the application checks if the API outputs intersect with \code{B}. If the API outputs do not intersect with either \code{A} or \code{B}, the branch \code{return "branch 3"} is then executed. 

% \textbf{Input example} With the same example discussed in Section~\ref{sec:m_to_n}, given an input with ground-truth \code{c1}, the ground-truth decision is executing the branch \code{return "branch 1"}. However, when the API outputs \code{[c3, c1]}, only the branch  \code{return "branch 1"} is executed because the API outputs intersect with \code{A}. This API output, thus do not lead to a critical error for Priority-list. 


% % For example, in Figure~\ref{fig:code}(c), the application defines two \wls, \code{A} and \code{B}, and \code{A} has higher priority than \code{B}. The application uses a nested loop that first iterates through the \wls, and then the output classes. The three possible decisions this application may make are: (1) selecting whitelist \code{A} if the ML API's outputs intersect with \code{A}; (2) selecting whitelist \code{B} if the ML API's outputs do not intersect with \code{A} and intersects with \code{B}; (3) selecting \code{others} if the ML API's outputs do not intersect with either \code{A} or \code{B}.

% % In this pattern, mis-classifications within the for labels inside any of the lower-ranked \wl will not lead to wrong application decisions if ML API correctly recognizes the existence of classes in the higher-ranked \wls. 

% % \yh{
% % Given the ground truth is [Building]

% % critical errors: including any class in monument 

% % }



% \subsubsection{Branch condition structure 4: Top-label}
% \label{sec:top_label}
% Applications that belong to this pattern make decisions by checking the ML API's output classes one by one until finding the first class that fulfills a branch condition. \shan{???In pattern 3, software maps ... ``in a specific order'' as well.}. Around 37\% of applications fall into this category.

% For example, as shown in Figure~\ref{fig:code}(d), the  application defines two lists of classes, and iterates over API outputs. If the first output, \code{x1}, belongs to any of the lists, the corresponding branch will be executed. If not, the application checks if the second output, \code{x2}, matches any one of the two lists or not. If none of the API outputs matches the two lists, the branch will be executed. 

% \textbf{Input example} With the same example discussed in Section~\ref{sec:priority}, different from Priority-list, the API outputs \code{[c3, c1]} lead the execution of the branch \code{return "branch 2"}.  This API output, thus incurs a critical error for Top-label. 

% %  the application defines two \wls, \code{A} and \code{B}. The application defines a nested for loop that first iterates through the output classes (\ie [\code{x1}, \code{x2}]), and then the \wls. If \code{x1} intersects with any of the \wls, the application selects the corresponding one. If \code{x1} does not match with any of the \wls, then the application checks if \code{x2} belongs to any of the \wls. Otherwise, it selects \code{others}. 

% % In this pattern, mis-classifications for classes ranked lower in the ML API's outputs do not matter, as long as the classes that rank higher leads to correct application decisions. 

% % \yh{Pie chart showing some statistics  }

% \subsubsection{Summary}

% In short, in these different structures of branch conditions, even when the branch conditions are the same (\eg checking if the API outputs interest with lists of classes), the same API outputs can lead to different application decisions. As a result, the patterns of critical errors can be very different for these different structures. 

% Although we use examples whose branch conditions are lists of classes, applications whose branch conditions are based on the range of the output scores also fall in the branch condition structures described in Section~\ref{sec:priority} or Section~\ref{sec:top_label}. 
% % \shan{What is the F1 score drop for this category?}

% \subsection{Summary of findings}

% To summarize, the real applications covered in our study reveal that there is a rich set of \emph{software context}. This motivates the need for customizing the ML API to incorporate the different \emph{software context}. 

% Luckily, although there is a rich set of \emph{software context}, the context is \emph{not} arbitrary. We can express the context in a format that combines the content and the structure of the branch condition, which can be extracted from the applications' source code.  
% % \yh{\textbf{Why we need to customize}}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}    
% %     \centering
% % \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % Dog = ['Dog','Mammal','Carnivore','Wolf']
% % image = types.Image(content=dog_image)
% % response = client.label_detection(image=image)
% % for obj in response.label_annotations:
% %   if obj.name in Dog:
% %     return 'It is a animal.'
% % return 'It belongs to others.'
% % \end{lstlisting}
% %     \caption{Code pattern: T-or-F. }
% %     \label{fig:app_example_level1}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_tf_wrong.pdf}
% %     \caption{Failing recognize the carnivore leads to software failure. }
% %     \label{fig:input_example_tf_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/app_input_example_level1.pdf}
% %     \caption{Mis-classifying a dog as wolf does not trigger software failure. }
% %     \label{fig:input_example_tf_correct}
% % \end{subfigure}
% % \caption{Dogecoin~\cite{food}, an application that classifies carnivore images.  }
% % \label{fig:tf_example}
% % \end{figure}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}    

% %     \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % proteinfoods = ['Hamburger', 'Meat', 'Patty']
% % fruitfoods = ['Apple', 'Fruit', 'Orange']
% % grainfoods = ['Noodle', 'Pasta', 'Al dente']
% % image = types.Image(content=trash_image)
% % response = client.label_detection(image=image)
% % protein, fruit, grain = False, False, False
% % for obj in response.label_annotations:
% %   if obj.name in proteinfoods:
% %     protein = True
% %   if obj.name in fruitfoods:
% %     fruit = True
% %   if obj.name in grainfoods:
% %     grain = True
% % RENDER_TEMPLATE(protein, fruit, grain)
% % \end{lstlisting}
% %     \caption{Software implementation. }
% %     \label{fig:app_example_non_mut}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_mton_wrong.pdf}
% %     \caption{Failing to recognize ``Cheese'' leads to software mis-behavior. }
% %     \label{fig:input_example_mton_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_mton_correct.pdf}
% %     \caption{Mis-classifying ``Pasta'' to ``Noodle'' still leads to correct software behavior. }
% %     \label{fig:input_example_mton_correct}
% % \end{subfigure}
% % \caption{Food classifier~\cite{food}, an application that classifies food images.}
% % \end{figure}


% % \begin{figure}
% %     \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % proteinfoods = ['Hamburger', 'Meat', 'Patty']
% % fruitfoods = ['Apple', 'Fruit', 'Orange']
% % grainfoods = ['Noodle', 'Pasta', 'Al dente']
% % image = types.Image(content=trash_image)
% % response = client.label_detection(image=image)
% % food_list = []
% % for obj in response.label_annotations:
% %   if obj.name in proteinfoods:
% %     food_list.append('protein')
% %   if obj.name in fruitfoods:
% %     food_list.append('fruit')
% %   if obj.name in grainfoods:
% %     food_list.append('grain')
% % return food_list
% % \end{lstlisting}
% %     \caption{An example software that maps original output labels of the ML APIs to a list of \wls.  }
% %     \label{fig:app_example_non_mut}
% % \end{figure}



% % \begin{figure}
% % \begin{subfigure}{0.45\textwidth}
% %         \centering
% %              \begin{lstlisting}[language=Python, style=mystyle, firstnumber=1]{micros}
% % Monument = ['Landmark', 'Sculpture', 'Monument']
% % Construction = ['Building', 'Estate', 'Mansion']
% % Person = ['Human','Person',  'Lady']
% % image = types.Image(content=landmark_image)
% % response = client.label_detection(image=image)
% % Predictions = []
% % for obj in response.label_annotations:
% %   Predictions.append(obj.name)
% % if any([label in Monument for label in Predictions]):
% %   return 'It belongs to monument.'
% % elif any([label in Construction for label in Predictions]):
% %   return 'It is construction.'
% % elif any([label in Person for label in Predictions]):
% %   return 'It is person.'
% % \end{lstlisting}
% %     \caption{Software implementation. }
% %     \label{fig:app_example_priority}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_priority_wrong.pdf}
% %     \caption{Missing a label ``Landmark'' leads to software mis-behavior. }
% %     \label{fig:input_example_priority_wrong}
% % \end{subfigure}
% % \begin{subfigure}{0.45\textwidth}
% %      \includegraphics[width=\linewidth]{figs/input_example_priority_correct.pdf}
% %     \caption{Recognizing an extra wrong label ``Mansion'' still leads to correct software behavior. }
% % \label{fig:input_example_priority_correct}
% % \end{subfigure}
% % \caption{Aander-ETL~\cite{etl}, an application that classifies landmark images.  }
% % \label{fig:priority_input_example}
% % \end{figure}

% % \cc{Do we want to introduce the accuracy difference between API and software? And the room for improvement?}

==> backups/2-2-empirical.tex <==
\begin{figure}
     \includegraphics[width=.99\linewidth]{figs/fig1.pdf}
    \tightcaption{Inference delay for initial phase and incremental phase for different generative tasks.  }
    \label{fig:initial_incremental}
\end{figure}
\mypara{Delay for initial phase and incremental phase}
Figure~\ref{fig:initial_incremental} shows the difference in inference delay of the initial phase and incremental phase, with \fillme input tokens. 

\mypara{Computation modules breakdown}
Figure~\ref{fig:delay_components} shows the inference delay for different delay components for different generative tasks. 


\begin{figure}
     \includegraphics[width=.99\linewidth]{figs/fig2.pdf}
    \tightcaption{Inference delay for different delay components for different generative tasks.  }
    \label{fig:delay_components}
\end{figure}

\begin{figure}
     \includegraphics[width=.8\linewidth]{figs/fig7.pdf}
    \tightcaption{Inference delay when varying number of input tokens for vanilla Attention and FlashAttention.  }
    \label{fig:flash}
\end{figure}


\mypara{Different impact factors}
Figures~\ref{fig:input_tokens},\ref{fig:batch},\ref{fig:model} show how the delay varies by different impact factors.
\begin{figure*}
     \includegraphics[width=.99\linewidth]{figs/fig4.pdf}
    \tightcaption{Inference delay for different generative tasks as we vary number of input tokens.  }
    \label{fig:input_tokens}
\end{figure*}

\begin{figure*}
     \includegraphics[width=.99\linewidth]{figs/fig5.pdf}
    \tightcaption{Inference delay for different generative tasks as we vary batch size.  }
    \label{fig:batch}
\end{figure*}

\begin{figure*}
     \includegraphics[width=.8\linewidth]{figs/fig6.pdf}
    \tightcaption{Inference delay for different generative tasks as we vary the model size.  }
    \label{fig:model}
\end{figure*}



\mypara{Summary} As we can see, for short input prompts, FFN and Attention together are usually the bottleneck (> 50\%) of the inference delay for both initial phase and incremental phase. 
But the Attention operation will dominate the inference delay for initial phase. 
This conclusion holds for different tasks.
The conclusion also holds even we use some memory efficient attention operations like FlashAttention~\cite{dao2022flashattention} shown in Figure~\ref{fig:flash}.

==> backups/3-caching.tex <==


% \begin{figure}
%      \includegraphics[width=.8\linewidth]{figs/budget.pdf}
%     \tightcaption{The size of cached data and transmission delay budget as the number of history data grows for text-generation. \todo{Mock figures} }
%     \label{fig:budget}
% \end{figure}

% \begin{figure}
%      \includegraphics[width=.8\linewidth]{figs/budget.pdf}
%     \tightcaption{The size of cached data and transmission delay budget as the number of history data grows for retrieval-augmented-generation. \todo{Mock figures} }
%     \label{fig:budget3}
% \end{figure}


% \begin{figure}
%      \includegraphics[width=.8\linewidth]{figs/budget2.pdf}
%     \tightcaption{The size of cached data and transmission delay budget as the number of history data grows. \todo{Mock figures} }
%     \label{fig:budget2}
% \end{figure}
\begin{itemize}
    \item Explain scenarios where the cached history may not be at the same server where the DNN inference happens (\eg Do inference on edge servers, while storing cached data at central datacenters)
    \item Define several possible transmission delay budgets
    \begin{itemize}
        \item  $T_{\text{Inference w/o caching}} > \alpha (T_{\text{Inference w/ caching}} + T_{\text{Transmitting cached data}})$ (where $\alpha$ is a tunable parameter) Figure~\ref{fig:budget}, \ref{fig:budget3} shows how delay budgets v.s. size of cached data grows when the number of history tokens grows
        \item a fixed threshold $T$ specified by different users or different applications
        Figure~\ref{fig:budget2} shows how delay budgets v.s. size of cached data grows when the number of history tokens grows
    \end{itemize}
    % \item Given the interactive property of generative tasks, there will be a transmission delay budget. 
    % We define the transmission delay budget as the deadline before which the cached data has to arrive in order to keep $T_{\text{Inference w/o caching}} > T_{\text{Inference w/ caching}} + T_{\text{Transmitting cached data}}$
    % We define the transmission delay budget as the deadline before which the cached data has to arrive in order to maintain the application-side latency SLO. 
    % \item Use figure~\ref{fig:budget} to illustrate how size of cached data grows v.s. the transmission budget varies as the history data grows. 
    \item Present challenges to meet the delay budgets when storing cached history remotely:
    \begin{enumerate}
        % \item Which jobs' cached history should be stored in the server where DNN inference happens, and which jobs' cached history should be stored remotely? 
        \item Which portion of cached data should be fetched from remote servers so as the speedup from caching can be maximized?
        \begin{itemize}
            \item A simple solution: Maintain a queue of jobs, and determine whether to fetch cached data from remote server in FIFO order. For one job, if its transmission delay is within the delay budget and the fetched data can fit CPU memory, fetch the cached data, and store the fetched data in CPU memory, otherwise, don't fetch, and do the inference afresh.
            % Every time before one inference job fetching cached data from the remote server, determine whether the transmission delay will be within the delay budget; if so, fetch the cached data, otherwise, don't fetch, and do the inference afresh.
            \item Why this solution can fall short?: CPU memory can be filled up with cached data from jobs who will not benefit from caching the most 
            \item Why further optimization is possible? Should get accurate enough estimation of $\frac{\Delta Delay}{\Delta \text{Size of fetched cached data}}$ for each job and fetch cached data at the size where the delay reduction starts become marginal
            \jc{i think a key insight (which is currently missing) is the fact that once the history state is loaded to GPU, the delay can be precisely predicted.}
        \end{itemize}
        \item How to compress the cached data?
        \begin{itemize}
            \item Use the STOA quantization techniques to compress the floating point attention vectors into int8
            \item Why this can fall short?: even with the quantization technique, transmitting the compressed data can still violate the delay budget. \eg assuming we want to transmit 1K of history tokens for LLaMA-13B, then the size of the cached data can be 1.3 GB after compression (even with entropy coding, it will still be \fillme MB), assuming the delay budget is 220 ms, and the network bandwidth is 500Mbps, the transmission delay can violate the delay budget 100 $\times$
            \item Why further optimization is possible? These compression methods still require sending the whole attention, but given that there will be a small portion of outlier features, it may be possible to use learned methods (\eg AE) to compress the cached data \yh{TBD}
        \end{itemize}
        % \item How to tolerate packet losses when fetching cached data from remote servers? 
    \end{enumerate}
      
    
\end{itemize}

==> backups/3-method-1123.tex <==
\label{sec:method}

\subsection{System architecture}

\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted Software decision process}

Figure~\ref{fig:system} shows the overall system architecture of \tool.
In the offline stage, the developers run a parser plugin locally, which extracted the software decision process from the application source code. The extracted software decision process is displayed in JSON format, consisting of: (1) the content of class lists used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of software decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.

% In the online stage, 




% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the DNN behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the DNNs behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the DNN behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



\subsection{How to customize the ML model in the ML API backend}

We first start with introducing the re-training scheme in \tool. 


\yh{Outline of this section: 
1. first list the goal in math (or text): minimize the incorrect app decisions
2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted software decision process (key dimensions) }
As shown in our empirical study in Section~\ref{sec:empirical}, we find the software decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

In this section, we will describe how we incorporate the software decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the software decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


To begin with, we first introduce the loss function traditionally used in multi-label image classification.


The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
\begin{equation}
    L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
\end{equation}
where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input sample $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


\subsubsection{Clustering training data}


To achieve the first step, one approach is to assign different weights to samples with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the DNN is able to classify. 
 The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-samples,  is $A$. 
 % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-samples. If we want to balance the distribution between $W$-samples and \code{others}-samples, we can use a loss function that assigns higher weights to \code{W}-samples:

\begin{equation}
    L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
\end{equation}
where $y_1$ indicates whether this sample is a \code{$W$}-sample or not. In other words, $y_1 = 1$ when the sample is a \code{$W$}-sample ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 
% \cc{This example seems to be T-or-F. Could we use consistency description as Section 3.4.2? }


% In this way, samples whose ground-truth decisions are selecting the \wl and those whose ground-truth decisions are selecting \code{others} are taking the same effect during training, instead of biasing towards either selecting the \wl or selecting \code{others}. 
In this way, \code{$W$}-samples and \code{others}-samples are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

\subsubsection{Branch condition structure 1: T-or-F} 

For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-samples; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-samples.



% \begin{equation}
% \left\{
% \begin{split}
%     L_{W_1} &= y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \\
%     P_1 &= xxx 
% \end{split}
% \right.
% \cc{Another format}
% \end{equation}

% \kt{$L_{W_i} = y_i (p_i\succ \theta) + (1-y_i) (\theta \succ p_i)$, where $y_1$ indicates whether ground truth contains classes inside $WL_1$ (in other word, ???=1, ???=0), $p_1$ is the maximum probability among white list 1 (\ie $WL_1$) and $\theta$ is the threshold used inside the ML API}.
% \cc{Some equations have numbers, some do not. Please make them consistent}

% \begin{itemize}
%     \item $y_1$ \cc{yuhan, this part is not finished yet}
% \end{itemize}

\begin{equation}
    L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
\label{eq:loss}
\end{equation}
where
$y_1$ indicates whether this sample is a \code{$W_1$}-sample or not. 
In other words, $y_1 = 1$ if the sample is a \code{$W_1$}-sample, and $y_1=0$ if the sample is a \code{others}-sample. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-samples. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-samples. Similarly for \code{other}-samples. 


% For example, in the example\cc{yuhan, please read these five words again to see what's the problem...} software shown in Figure~\ref{fig:tf_example}, given a prediction threshold of 0.5, when the probability scores of the labels in the specified \wl are $\langle0.2, 0.3, 0.4, 0.9\rangle$ for Dog, Mammal, Carnivore, and Wolf respectively in Figure~\ref{fig:input_example_tf_correct}, the penalty incurred by the loss function is 0.40. On the other hand, in Figure~\ref{fig:input_example_tf_wrong}, where the ground-truth labels include one of the labels in the \wl, thus the ML API should output at least one label in the \wl in order to produce the correct control flow decision. When the probability scores for  Dog, Mammal, Carnivore, and Wolf are $\langle0.2, 0.3, 0.35, 0.3\rangle$\cc{I use parenthesis to make them look like lists instead of random number. yuhan, could also change other places?} respectively, leading to none of the labels in the \wl being output, the penalty incurred by the loss function is 0.537. 


\subsubsection{Branch condition structure 2: M-to-N-set} 

 In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

We derive the following loss function for M-to-N-set:
\begin{equation}
    L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
\end{equation}
where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

 Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.
 % \cc{be low or be zero? should we also mention the probability differences?}. 


% \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



\subsubsection{Branch condition structure 3: Priority-list}

Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

We derive the loss function as:
\begin{equation}
\begin{split}
    L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
    (1-y_i) \cdot \textrm{S}(P - \theta) \,,
\end{split}
\end{equation}
where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
$k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 

% \begin{equation*}
%     \footnotesize
%     \begin{split}
%     L(O, G) &=  \begin{cases}
%    P \Big( T, \max\limits_{c \in W} p_c \Big ), & G \cap W = \emptyset \\
%      P \Big( \max\limits_{c \in WL_k } p_c, T \Big ) + P\Big( \max\limits_{c \in WL_k} p_c, \max\limits_{c \in W \setminus WL_k} p_c \Big ), & G \cap W \neq \emptyset \\
% \end{cases}\\
% k &= \min \{i|WL_i \cap G \neq \emptyset\}
%     \end{split}
% \end{equation*}
% \kt{$L_{W_k}$, where $k=???$}


% Given this loss function, we can ensure that: (1) for images with ground-truth labels intersecting with at least one \wl, as long as the \wls that intersect with the output labels are not the one that ranked highest among those intersecting with the ground-truth labels, the penalty incurred by the loss function will be large; (2) for images with ground-truth labels that do not have an intersection with any of the \wls, as long as the output labels intersect with the labels in any of the \wls, the penalty incurred by the loss function will be large. 


% For example, in the example software \cc{I prefer directly writing down software name (if we already introduce it) or describe what type of software, e.g. trash classification application. It's hard for people to recall what happens only with the figure number} shown in Figure~\ref{fig:priority_input_example}, the prediction threshold is 0.5. In the input example in Figure~\ref{fig:input_example_priority_correct}, the probability scores of the labels in the Monument \wl are 0.2, 0.3 and 0.1 respectively, and the probability scores of the labels in the Construction \wl are 0.8, 0.2, 0.05, and the probability scores of the labels in the Person \wl are 0.45, 0.4, 0.2. The penalty incurred by the loss function is $Sigmoid(0.5-0.8)$ + $Sigmoid(0.45-0.8)$ = 0.8388. 

% On the other hand, in the input example in Figure~\ref{fig:input_example_priority_wrong}, the probability scores of the labels in the Monument \wl are 0.3, 0.2 and 0.15 respectively, and the probability scores of the labels in the Construction \wl are 0.7, 0.2, 0.1, and the probability scores of the labels in the Person \wl are 0.45, 0.8, 0.2. The penalty incurred by the loss function is $Sigmoid(0.5-0.3)$ + $Sigmoid(0.8-0.3)$ = 1.17. The penalty, in this case, is greater than the penalty in Figure~\ref{fig:input_example_priority_correct}, because labels in the highest-ranked \wl intersecting with the ground-truth labels do not appear in the output. 

\subsubsection{Branch condition structure 4: Top-label}

Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

We derive the loss function as:
\begin{equation}
    L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
\end{equation}
where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 
% \begin{equation*}
%     \footnotesize
%     L(O, G) =  \begin{cases}
%    P \Big( T, \max_{c \in W} p_c \Big ), & G \cap W = \emptyset \\
%      P \Big( \max_{c \in G \cap W } p_c, T \Big ) + P\Big( T, \max_{c \in W \setminus G } p_c \Big ), & G \cap W \neq \emptyset \\
% \end{cases}
% \end{equation*}

% \kt{$L_W$, where $W={\bigcap_{W_i \cup G\neq \phi} W_i}$ is ....}

Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the software decision process}
% How we use sym-ex to get info, and which info 
\yh{Change all the whitelists}
To extract software context, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. For each combination of branch decisions, \tool adopts symbolic execution engine DSE~\cite{irlbeck2015deconstructing} and CVC5 constraint solver~\cite{cvc5} to find all the API outputs that lead to these decisions, which is the corresponding \wl.
If the software specifies only 1 branch condition, \tool reports pattern T-or-F. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{How is the whitelist selected?} \tool analyzes all the statements inside the edges of an ML-API-related if-branch. If the software terminates all the examinations inside one of the branch edges (e.g., a break statement inside the loop and a return statement inside a function body), \tool regards that it as ``select 1 whitelist'' and further examines the order. 
If there is no such termination, \tool determines it is a M-to-N-set structure. 
% If there is no such termination, \tool determines whether it is pattern M-to-N-set or M-to-N-list according to the data structure of function returned value.

\emph{How is the order determined?} \tool finds all the loop structures and the equivalent statements outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators. 
If the software does not contain any loop iterating ML API's output or \wls, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates the ML API's output and the outer (inner) loop iterates the \wls, \tool regards it as pattern Priority-list (Top-label).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to change the MLaaS run-time backend}


% \subsection{Network Architecture}
% How we change the architecture of pre-trained model (freezing some part of the model)


% \subsection{Dataset Construction}



==> backups/3-method-1126.tex <==
\label{sec:method}

\subsection{Key components and workflow}

\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. 
    % \jc{the overall flow looks ok, but there are so many minor issues in this figure. just to name a few: 
    % (1) where is "cloud service" coming from? 
    % (2) (a) and (b) shouldn't be distinguished (see comment in 3.1).
    % (3) i thought we decided to drop the arrow of giving the parser to developer?
    % (4) why "software context" is still used?
    % (5) user is not running python code! they run real apps
    % (6) why calling it "prediction" instead of API output?
    % (7) what's "model inference code"? if it's simply selecting the right model to run, we shouldn't introduce a new term.
    % (8) the three customized models should be put side by side (either all vertically or horizontally),
    % (9) why calling them "adapted" ML model? if the term we always use is "customized", then stick to that.}
    % \jc{in general, EVERY word must be picked very carefully, which you clearly didn't do :)}
    \yh{fixed comments, I'm calling it ML-model outputs instead of API outputs because the outputs comes before the ``output interface'', thus it's not API outputs yet}
    \jc{sorry i disagree. again, don't introduce new terms unless really necessary, which i don't think is the case. why dont you change the figure, to move the output and input the left of the model output interface, which should also be changed to "ML API"?}
    \jc{and don't let arrows overlap with arrows or lines (e.g., Model pool, Select)}
    }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted Software decision process}
Guided by the empirical study in \S~\ref{sec:empirical}, we propose \tool, an optimization framework that extracts the software decision process of the applications querying the MLaaS, and customizes the ML-model in the MLaaS backend. 
% summarizes the overall workflow of \tool.


As shown in Figure~\ref{fig:system}, when the application is being developed, 
% \jc{the term offline is new. the contrast between offline and online is overcomplicating. can we say something like when the application is being developed?}
besides the existing development procedure, the developers also run an MLaaS-provided parser plugin on their own machines, 
% \jc{the ``parser'' comes from nowhere. who provides it? even a simple ``MLaaS-provided parser'' is better}
% \jc{``locally'' has many meanings. pick a more precise term}, 
which extracts a summary of the software decision process
% \jc{maybe we need a different term; ``key features'' invites unnecessary confusion when used in an ML-related paper. how about a ``summary of the application's decision process''?}
% \jc{``extracts xxx from app into a file'' sounds wrong. shouldn't it be ``extract xxx from an app and uploads it as a file to xxx''?} 
from the application source code (details in \S~\ref{sec:extract}), and uploads it as a file to the MLaaS backend. In the MLaaS backend, \tool constructs a loss function based on the uploaded file, re-trains the ML-model with the constructed loss function, and adds the re-trained ML-model into the model pool (details in \S~\ref{sec:loss}). 
Finally, 
% \jc{the last phrase can be deleted}
an application queries the MLaaS with inputs via the existing interface,  
the MLaaS backend selects and runs inference with the customized ML-model(details in \S~\ref{sec:runtime}). 
% \jc{the separation among the three stages (``developer'', ``retraining'' and ``run-time'') is unnecessarily complicating the flow, and it introduces unnecessary terms, like ``run-time''. }

\jc{when introducing the flow, shouldn't we also highlight what we DO change and what we do NOT change?}

% The software decision process extracted from the Python source code, is composed of the key features characterizing it.\cc{This sentence does not provide additional information. Also, we could mention python in the implementation section} 

\jc{please don't explain a concept together with an application. you should always explain the concept first, and THEN use an example to explain it in a specific context.}
The summary of the software decision process consists of three aspects: (1) what are the target classes?  (2) what is the type of decision out of \emph{True-False}, \emph{Multi-Choice}, or \emph{Multi-Select}? (3) if the application makes a \emph{Multi-Choice} decision, how does the application reach a decision? 
These three aspects can uniquely identify which errors are critical or non-critical to the applications. Identifying the critical errors, as discussed in \S~\ref{sec:empirical}, which vary greatly across applications, provides us with great opportunities to customize the ML-models per application. 

Take the garbage classification application in Figure~\ref{fig:code}(a) as an example to illustrate. The summary of the software decision process for this application contains: (1) the three target classes \code{Recycle}, \code{Compost}, \code{Donate}; (2) a \emph{Multi-Choice} decision; (3) it follows the \emph{API-output order} to reach the \emph{Multi-Choice} decision.  

\jc{this last sentence is important but quite misleading. first of all, these features don't uniquely describe a decision process (e.g., they dont say what decisions will be made for each branch). instead, they specify what errors are critical and what errors are not critical.
second, you didn't say WHY they SHOULD be used by \tool to customize the ML model.}


\begin{comment}
\jc{this definition is extremely important and should be elevated. i suggest explain it in a separate paragraph. so you will have two paragraphs: one explain the overall workflow, and the second explains what's extracted from the source code and used to customize ML-model. it's important to keep the 1st para short.} 
\jc{it should be explained more formally, probably with a simple example, and the terms (e.g., multi-select vs. multi-choice) should be tightly connected to when they are first defined. remember, many reviewers may have skipped (or missed) their definitions in section 2.} 
\jc{moreover, i wouldn't mention JSON at the beginning. the exact format (not the content in the file) seems secondary to me}
\jc{what about score ranges? we need a way to explain all cases under consideration} 
% used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of software decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.
\jc{i wouldn't distinguish training data resampling and loss function as two separate steps. last time we met as a group, we decided to say changing loss function is all that's needed, though the real implementation does resampling to speedup training. i like this idea, so the distinction should be secondary.} 

\jc{regarding the terminology, the parser doesn't extract the entire application decision process, it merely extracts the key features of the application decision process, which include xxx}



\jc{now this is too low-level when explaining the workflow. here, you can just say ``each time an application calls the ML API, the ML API backend will select the ML-model model customized for the application, ...''}
% the applications submit inference request to the ML API with input and the credential, like 

\jc{two meta comments: 1. Yuhan, you should read the terms used in the new Section 2 and use them consistently in section 3.
2. when writing 3.1, please make sure that every important term appears with a forward pointer to a later subsection that explains it in detail as well as a pointer to Figure 4}
\end{comment}

% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the ML-model behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the ML-models behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the ML-model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



% \subsection{How to customize the ML model in the MLaaS backend}
\subsection{Customizing ML model for an application decision process}
\label{sec:loss}
As introduced in \S~\ref{sec:empirical},  applications in the wild differ greatly in their software decision processes. 
% For example, they may  define different number of target classes or include only a small subset of labels of the whole label set in their target classes and so on. 
This heterogeneity can lead to differences in critical errors\jc{remind people what critical errors are?} across applications. 
It is possible for an ML API error to be non-critical for one application, while critical for another. Thus, customizing the DNN in the MLaaS backend is important in order to incorporate the differences in software decision processes across applications.
\jc{the whole first paragraph is redundant to 3.1. this para should highlight why we start by explaining the step of DNN retraining}

The customization goal is to minimize the critical errors for each application.
% caused by ML API errors. 
Formally, the software decision process can be viewed as $\z = \Decision(\API(\x))$, where $\x$ is the input to the API, $\API(\x)$ is the ML API output, and $\Decision$ is the post-processing the application performs to make decisions based on API outputs. 
Let $\x_i\in \X$ denote the $i^{th}$ input, where $1 \leq i \leq M$, to the ML API, and $\hat{y_i}$ denote its ground-truth label. 
% $API(x_i)$ is a list of probabilities for label-based API (\eg image or text classification), 
% [$p_1, p_2, \dots, p_n$], for every label in the whole label set, and a score $O_i$ for score-based API (\eg sentiment analysis API). 
Formally, our customization goal is:
% Let $\mathds{1}_{x}$ denote the indicator function, where $\mathds{1}_{x} = 1$ when $x$ is \emph{True} and 0 otherwise. Therefore, the customization goal is:

\begin{equation}
    \min |\{x_i \in X | Decision(API(x_i)) \neq Decision(y_i)\}|
    \label{eq:goal}
\end{equation}

With this customization goal, together with the observation that applications typically heavily cluster on a small subset of labels in mind, we naturally come up with a \emph{strawman} of customization: re-train the ML-model with a re-sampled training dataset, which clusters on the labels appearing in the target classes of the application. 
While the original model is optimized to minimize average label-wise errors across a wide range of labels\footnote{Traditionally, the loss function minimizes the average error between the predicted probability and ground-truth labels for every class, which we refer to as average label-wise errors. } (\eg 9605 labels in Open Images~\cite{ASL}), this strawman approach can reduce the label-wise errors of labels belonging to the target classes. However, it is unaware that applications may make different decisions, including \emph{True-False}, \emph{Multi-select}, and \emph{Multi-choice}, and how these decisions affect the severity of ML API errors. 

Fortunately, the loss function used in ML-model training provides a \emph{differentiable} way to capture the incorrectness of the ML-model's predictions with respect to the ground-truth. In addition, we formulate the software decision process in a structured format. This allows \tool to translate it into a loss function with the goal of both clustering on labels in target classes and directly minimizing the critical errors (Equation~\ref{eq:goal}). 
% \yh{Why they fails and we do not fail }
% \yh{add general recipe }
Compared to the strawman which may spare energy penalizing non-critical errors, such as penalizing mis-classifications within the target classes, 
our solution only focuses on penalizing the critical ones, such as mis-classifications across target classes. 





As illustrated in \S~\ref{sec:empirical}, the critical errors in the applications can differ greatly for different target classes, types of decisions, and order of examination. As a result, we construct different loss functions, with the unified goal of minimizing critical errors, for each type of applications. 

A general recipe for our loss function is formulated as:

\begin{equation}
    L_i = H_{o}(\hat{y_i}) \cdot S(\theta-G(y_i)) + \sum_{j=1}^{m} H_j(\hat{y_i}) \cdot S(F(y_i)-G_j(y_i))  
\end{equation}

\mypara{True-False} This type of application defines only one target class, checking if the API outputs match with
% \cc{I suspect ``intersect'' is a better praise, as we the API output includes a list of items}
it. We denote the labels included in the target class as $W_1$. Therefore, the corresponding loss function is:
\begin{equation}
    L = y_i\cdot \frac{M}{N_1}  \cdot \textrm{S}(\theta - P_1) + (1-y_i) \cdot \frac{M}{M-N_1} \textrm{S}(P_1 - \theta) \,,
\label{eq:loss}
\end{equation}
where $y_i = 1$ when the ground-truth of the input intersects with the target class $W_1$, and $y_i=0$ otherwise. $\theta$ is the prediction threshold, where output labels whose predicted probability are greater than it will be included in the output label list. $P_1$ is the maximum probability of labels in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will keep the notation in the rest of the paper. $N_1$ is the total number of inputs in the training dataset whose ground-truth decision is the target class (\ie $N_1 = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_j}\cap W_1 \neq \emptyset}$), denoted as target-inputs. The inputs whose ground-truth decision is selecting the non-target class are denoted as non-target-inputs. 


% With this loss function, \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 

Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for target-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for target-inputs. Similarly for non-target-inputs. 

Furthermore, to achieve the effect of clustering on labels in $W_1$, the loss function applies a weight of $\frac{M}{N_1}$ on target-inputs, and a weight of $\frac{M}{M-N_1}$. Therefore, the number of target-inputs and non-target-inputs are effectively balanced, instead of biasing towards either the target class or non-target class. 

\mypara{Multi-Select} This type of application defines several target classes, $\{W_1, W_2, \dots, W_m\}$, and multiple selections are allowed about which class(es) the ML API output belongs to. We construct the following loss function:

\begin{equation}
    L = \frac{M}{N_i}\sum_{j=1}^{m} y_i \cdot \textrm{S}(\theta - P_j) + (1-y_i) \cdot \textrm{S}(P_j - \theta) \,,
\label{eq:multi-select}
\end{equation}
where $y_i$ indicates whether this input belongs to the $j^{th}$ target class $W_j$, $y_i = 1$ when $\hat{y_i} \cap W_j \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_j$ is the maximum probability of classes belonging to $W_j$ (\ie $P_j = max_{c \in W_j} p_c$). Let $\mathbb{W} = \bigcup\limits_{j=1}^{m} W_j$ denote the union of all the target classes defined in the application, and $\mathcal{W}_i = \bigcup_{W_j \cap  \hat{y_i} \neq \emptyset} W_j $ denote the union of all the ground-truth target classes for the $i^{th}$ input (same notation used in the rest of the section). 
When $\hat{y_i} \cap \mathbb{W} \neq \emptyset$, $N_i$ is the total number of inputs in the training data belonging to $\mathcal{W}_i$ (\ie $N_i = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_j}\cap \mathcal{W}_i \neq \emptyset}$); otherwise, $N_i$ denotes the total number of non-target-inputs (\ie $N_i = \sum\limits_{j=1}^{M}\mathds{1}_{\hat{y_i} \cap \mathbb{W} = \emptyset}$), the same notation will be used throughout this section. Similarly to Equation~\ref{eq:loss}, the weight $\frac{M}{N_i}$ is used to achieve the effect of balancing each of the target classes and non-target class.

With this loss function, only if the application decisions led by the ML API outputs exactly match with the ground-truth decisions, the penalty will be low.

\mypara{Multi-Choice API-output order} This type of application defines several target classes, and starts with checking if the first API output label matches with any of the classes. If so, the rest of the labels are skipped. Otherwise, later labels will be checked. We construct the following loss function:
 \begin{equation}
    L = \frac{M}{N_i} \Bigl( y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \Bigr) \,,
\label{eq:api_output}
\end{equation}
where $y_i  = 1$ indicates ground-truth labels intersect with $\mathbb{W}$, and $y_i=0$ otherwise. $P^{+}$ is the maximum probability out of classes in $\mathcal{W}_i$ (\ie $P^+ = \max_{c \in \mathcal{W}_i } p_c$), and $P^-$ is the maximum probability out of classes in the incorrect target classes (\ie $P^- = \max_{c \in (\mathbb{W} \setminus \mathcal{W}_i) } p_c$). 

Therefore, the loss function ensures only if the first output label encountered belonging to any of the target classes, matches with the ground-truth class, the penalty will be low. 

\mypara{Multi-Choice application-choice order} This type of application starts with checking if the first target class matches with any output label before moving to the next class. We construct the following loss function for this type:

\begin{equation}
\begin{split}
    L = \frac{M}{N_i} \Bigl( y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
    (1-y_i) \cdot \textrm{S}(P - \theta) \Bigr) \,,
\end{split}
\label{eq:app_choice}
\end{equation}

Similarly to Equation~\ref{eq:api_output},  $y_i  = 1$ indicates ground-truth labels intersect with $\mathbb{W}$, and $y_i=0$ otherwise. $k$ is the index of the highest-priority target class that intersects with the ground-truth labels (\ie $k = \min \{j|W_j \cap \hat{y_i} \neq \emptyset\}$). $P_k$ is the maximum probability for labels belonging to $W_k$, and $P_{k^{-}}$ is the maximum probability out of the labels belonging to higher priority classes than the ground-truth class (\ie$W_{k^{-}} = \bigcup_{\{j|\hat{y_i} \cap W_j \neq \emptyset  \textrm{ and }  j < k \}} W_j$ and $P_{k^{-}} = \max_{c\in W_{k^{-}} }p_c$). $P$ is the maximum probability of the classes belonging to $\mathbb{W}$. 


This loss function ensure that only if the first target class that matches with any of the output labels is the ground-truth class, the penalty incurred by the loss function will be low. 


\mypara{Value-ranges} For APIs outputting scores, such as the sentiment analysis API, application check whether the score lies in defined value ranges. The loss function we construct is:

\begin{equation}
    L = \frac{M}{N_i} \cdot \Bigl( S(l_i - O_i) + S(O_i - h_i) \Bigr) \,,
\end{equation}
where $l_i$ is the lower bound of the ground-truth  value range, and $h_i$ is the upper bound of the ground-truth value range. $N_i$ is defined similarly to previous sections. 

Therefore, the penalty incurred by the loss function will be low only when the API output score lies in the ground-truth value ranges.
% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\jc{
an example outline of this subsection (each bullet is a para)
\begin{itemize}
\item why we start with this? the key step is customizing ML-model for each application.
\item what's the goal
\item what's a strawman (resampling training data)? and why is it not good (doesn't distinct multi-choice vs multi-option and order of examination)? (this para must be short). if room, also bring up some prior work that also does this
\item our idea: rewriting loss function. give a general recipe of how this is done
\item why is it better? (this should directly contrast with the strawman)
\item more case-by-case explanation.
\end{itemize}
}

\jc{regarding how to explain the goal, you can expand the following: formally an application can be viewed as $z=Decision(Model(x))$. for a given decision process $Decision$, the goal is to minimize $Decision(Model(x_i))\neq Decision(\hat{y_i})$ over a set of $x_i$, where $\hat{y_i}$ is the ground truth label of $x_i$.}



% \mypara{Notations} 
% Denote the total number of classes that the ML-model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows. 
% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the ML-model behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}

% \mypara{Customization goal} For T-or-F, we want to minimize the critical errors which are caused by the API outputs that lead to the  execution of the \emph{False} branch, when the statement should be \emph{True} according to the ground-truth, and vice versa. With the above notations, our goal can be written as:

% \begin{equation}
% \begin{aligned}
% \min \sum\limits_{i=1}^{M}( y_i \cdot \mathds{1}_{\theta - P} + (1-y_i) \cdot \mathds{1}_{P-\theta} )
% \end{aligned}
% \end{equation}

% Where $\mathds{1}_{x} = 1$ when $x > 0$, and 0 otherwise. $y_i = 1$ if the $i^{th}$ input belongs to the class list defined in the branch condition, which we denote as $W$. $\theta$ is the prediction threshold, where classes whose predicted probability is higher than the threshold will be included in the output label list. $P$ is the maximum probability of classes in $W$, in other words, $P = max_{c \in W} p_c$.
% there are two types of critical errors: (1) for inputs whose statement in the branch condition is \emph{True} according to the ground-truth, which we refer to as \emph{target-inputs}, the API outputs lead the application selecting the \emph{False} branch; (2) for inputs whose statement is \emph{False}, the API outputs lead the application selecting the \emph{True} branch. To minimize incorrect application decisions, we want: 




% \yh{Outline of this section: 
% 1. first list the goal in math (or text): minimize the incorrect app decisions
% 2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted software decision process (key dimensions) }
% As shown in our empirical study in Section~\ref{sec:empirical}, we find the software decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

% In this section, we will describe how we incorporate the software decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the software decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


% To begin with, we first introduce the loss function traditionally used in multi-label image classification.


% The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
% \begin{equation}
%     L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
% \end{equation}
% where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input input $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


% \subsubsection{Clustering training data}


% To achieve the first step, one approach is to assign different weights to inputs with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
% We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the ML-model is able to classify. 
%  The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-inputs,  is $A$. 
%  % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
% The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-inputs. If we want to balance the distribution between $W$-inputs and \code{others}-inputs, we can use a loss function that assigns higher weights to \code{W}-inputs:

% \begin{equation}
%     L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
% \end{equation}
% where $y_1$ indicates whether this input is a \code{$W$}-input or not. In other words, $y_1 = 1$ when the input is a \code{$W$}-input ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 

% In this way, \code{$W$}-inputs and \code{others}-inputs are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% % We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

% \subsubsection{Branch condition structure 1: T-or-F} 

% For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-inputs; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-inputs.




% \begin{equation}
%     L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
% \label{eq:loss}
% \end{equation}
% where
% $y_1$ indicates whether this input is a \code{$W_1$}-input or not. 
% In other words, $y_1 = 1$ if the input is a \code{$W_1$}-input, and $y_1=0$ if the input is a \code{others}-input. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



% Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 



% \subsubsection{Branch condition structure 2: M-to-N-set} 

%  In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

% We derive the following loss function for M-to-N-set:
% \begin{equation}
%     L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
% \end{equation}
% where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

%  Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.


% % \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



% \subsubsection{Branch condition structure 3: Priority-list}

% Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

% We derive the loss function as:
% \begin{equation}
% \begin{split}
%     L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
%     (1-y_i) \cdot \textrm{S}(P - \theta) \,,
% \end{split}
% \end{equation}
% where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
% $k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

% Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 


% \subsubsection{Branch condition structure 4: Top-label}

% Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
% In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

% We derive the loss function as:
% \begin{equation}
%     L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
% \end{equation}
% where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 


% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the software decision process}
\label{sec:extract}
% How we use sym-ex to get info, and which info 
\yh{Change all the whitelists}
To extract software decision process, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. For each combination of branch decisions, \tool adopts symbolic execution engine DSE~\cite{irlbeck2015deconstructing} and CVC5 constraint solver~\cite{cvc5} to find all the API outputs that lead to these decisions, which is the corresponding \wl.
If the software specifies only 1 branch condition, \tool reports pattern True-False. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{Whether multi-select or multi-choice?} \tool analyzes all the statements inside the edges of an ML-API-related if-branch. If the software terminates all the examinations inside one of the branch edges (e.g., a break statement inside the loop and a return statement inside a function body), \tool regards that it as a multi-choice and further examines the order. 
If there is no such termination, \tool determines it is multi-select structure. 


\emph{How is the order determined?} \tool finds all the loop structures and the equivalent statements outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators. 
If the software does not contain any loop iterating ML API's output or application choices, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates the ML API's output and the outer (inner) loop iterates the application choices, \tool regards it as pattern Application-choice order (API-output order).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to change the MLaaS run-time backend}
\label{sec:runtime}



==> backups/3-method-1129.tex <==
\label{sec:method}

Guided by the empirical study in \S\ref{sec:empirical}, this section presents \tool, an optimization framework that customizes ML models of the MLaaS backend for the decision processes of different applications.

\subsection{Key components and workflow}
\label{sec:overall}
\begin{figure}
     \includegraphics[width=\linewidth]{figs/system_overview.pdf}
    \caption{System architecture of \tool. 
    % \jc{the overall flow looks ok, but there are so many minor issues in this figure. just to name a few: 
    % (1) where is "cloud service" coming from? 
    % (2) (a) and (b) shouldn't be distinguished (see comment in 3.1).
    % (3) i thought we decided to drop the arrow of giving the parser to developer?
    % (4) why "software context" is still used?
    % (5) user is not running python code! they run real apps
    % (6) why calling it "prediction" instead of API output?
    % (7) what's "model inference code"? if it's simply selecting the right model to run, we shouldn't introduce a new term.
    % (8) the three customized models should be put side by side (either all vertically or horizontally),
    % (9) why calling them "adapted" ML model? if the term we always use is "customized", then stick to that.}
    % \jc{in general, EVERY word must be picked very carefully, which you clearly didn't do :)}
    % \yh{fixed comments, I'm calling it ML model outputs instead of API outputs because the outputs comes before the ``output interface'', thus it's not API outputs yet}
    % \jc{sorry i disagree. again, don't introduce new terms unless really necessary, which i don't think is the case. why dont you change the figure, to move the output and input the left of the model output interface, which should also be changed to "ML API"?}
    % \jc{and don't let arrows overlap with arrows or lines (e.g., Model pool, Select)}
    }
\label{fig:system}
\end{figure}
% \mypara{Main components}

% \mypara{Extracted application's decision process}
% the application's decision process of the applications querying the MLaaS, and customizes the ML model in the MLaaS backend.
% summarizes the overall workflow of \tool.


\mypara{Workflow}
Figure~\ref{fig:system} depicts \tool's high-level workflow. 
When the developers publish an application \App, they first run a parser script provided by \tool on \App's source code to extract its {\em decision-process summary} (explained shortly), and then upload the summary to \tool's MLaaS backend (details in \S\ref{sec:extract}). 
In the backend, \tool uses the received decision-process summary to construct a new loss function, such that when the ML model is re-trained using the new loss function, it will produce inference results that yield fewer application decision failures for the application \App (details in \S\ref{sec:loss}).
\tool then adds the new ML model to a pool of customized ML models. 
% \jc{the last phrase can be deleted}
When a user of application \App queries the MLaaS backend with an input via the existing ML API, the backend will select the ML model customized for \App and return the inference result of the selected ML model (details in \S\ref{sec:runtime}).


\begin{comment}
When the application is being developed, 
% \jc{the term offline is new. the contrast between offline and online is overcomplicating. can we say something like when the application is being developed?}
besides the existing development procedure, the developers also run an MLaaS-provided parser plugin on their own machines, 
% \jc{the ``parser'' comes from nowhere. who provides it? even a simple ``MLaaS-provided parser'' is better}
% \jc{``locally'' has many meanings. pick a more precise term}, 
which extracts a summary of the application's decision process
% \jc{maybe we need a different term; ``key features'' invites unnecessary confusion when used in an ML-related paper. how about a ``summary of the application's decision process''?}
% \jc{``extracts xxx from app into a file'' sounds wrong. shouldn't it be ``extract xxx from an app and uploads it as a file to xxx''?} 
from the application source code (details in \S\ref{sec:extract}), and uploads it as a file to the MLaaS backend. 
\end{comment}




% \jc{the separation among the three stages (``developer'', ``re-training'' and ``run-time'') is unnecessarily complicating the flow, and it introduces unnecessary terms, like ``run-time''. }

% \jc{when introducing the flow, shouldn't we also highlight what we DO change and what we do NOT change?}

% The application's decision process extracted from the Python source code, is composed of the key features characterizing it.\cc{This sentence does not provide additional information. Also, we could mention python in the implementation section} 

% \jc{please don't explain a concept together with an application. you should always explain the concept first, and THEN use an example to explain it in a specific context.}

\smallskip
\noindent
The {\bf \summary} extracted from an application includes three pieces of information: 
\begin{packeditemize}
\item the values included in each target class; \yh{double check}
\item the type of decision (\ie \emph{True-False}, \emph{Multi-Choice}, or \emph{Multi-Select});
\item the matching order over the target classes, if the application makes a \emph{Multi-Choice} decision.
\end{packeditemize}
These three pieces of information can uniquely identify which errors are critical and which are non-critical to the application, which provides vital information to customize the ML model for the application, as elaborated in \S\ref{sec:loss}. 
% vary greatly across applications, 
% provides us with great opportunities to customize the ML models per application. 

To give a concrete example, the \summary of the garbage classification application in Figure~\ref{fig:code}(a) contains
(1) the three target classes (each being a list of labels): \code{Recycle}, \code{Compost}, and \code{Donate}; (2) the \emph{Multi-Choice} type of decision; and 
(3) it follows the \emph{API-output order} to reach the \emph{Multi-Choice} decision.  


\mypara{What is changed, what is not}
It is important to notice that \tool does {\em not} change the ML API or the source code or the executable of the application.
% \jc{check the term with shan/chengcheng}
That said, \tool does change two things. 
First, the application developers need to run \tool's parser script to extract the decision-process summary.
Second, \tool modifies the MLaaS backend to re-train an ML model per application (instead of serving the same model to all applications) and selects the right ML model to serve each query.
% When the application queries the MLaaS, 
% a model selector module is added in the backend to choose the ML model customized to the application, based on the application ID incorporated in the identification credential.

% \jc{this last sentence is important but quite misleading. first of all, these features don't uniquely describe a decision process (e.g., they dont say what decisions will be made for each branch). instead, they specify what errors are critical and what errors are not critical.
% second, you didn't say WHY they SHOULD be used by \tool to customize the ML model.}


\begin{comment}
\jc{this definition is extremely important and should be elevated. i suggest explain it in a separate paragraph. so you will have two paragraphs: one explain the overall workflow, and the second explains what's extracted from the source code and used to customize ML model. it's important to keep the 1st para short.} 
\jc{it should be explained more formally, probably with a simple example, and the terms (e.g., multi-select vs. multi-choice) should be tightly connected to when they are first defined. remember, many reviewers may have skipped (or missed) their definitions in section 2.} 
\jc{moreover, i wouldn't mention JSON at the beginning. the exact format (not the content in the file) seems secondary to me}
\jc{what about score ranges? we need a way to explain all cases under consideration} 
% used in branch conditions; (2) whether the application is making multi-select or multi-choice decisions; (3) the order of examination for applications making multi-choice decisions. Then, the developers will upload the JSON of application's decision process to the MLaaS backend. On the MLaaS backend side, \tool will re-train the ML model by re-sampling the training data with a more focus on the classes appeared in the applications, and constucting loss functions which directly penalize the critical errors.
\jc{i wouldn't distinguish training data resampling and loss function as two separate steps. last time we met as a group, we decided to say changing loss function is all that's needed, though the real implementation does resampling to speedup training. i like this idea, so the distinction should be secondary.} 

\jc{regarding the terminology, the parser doesn't extract the entire application decision process, it merely extracts the key features of the application decision process, which include xxx}



\jc{now this is too low-level when explaining the workflow. here, you can just say ``each time an application calls the ML API, the ML API backend will select the ML model model customized for the application, ...''}
% the applications submit inference request to the ML API with input and the credential, like 

\jc{two meta comments: 1. Yuhan, you should read the terms used in the new Section 2 and use them consistently in section 3.
2. when writing 3.1, please make sure that every important term appears with a forward pointer to a later subsection that explains it in detail as well as a pointer to Figure 4}
\end{comment}

% which consists of a parser plugin, an ML model re-training scheme run in the offline stage, and in the online stage, \tool selects the customized ML model based on applications' credentials, and run inference with the customized model.  


% 3.2: given the extracted json, how should we re-train teh model 
% 3.3. how to extract
% 3.4: how to change the run-time interface

% \tool is an automated framework that adapts the ML model behind the ML APIs, such that the number of software mis-behaviors can be greatly reduced when applied to an ML software. 

% \tool first performs static analysis to extract the code structure of the applications invoking MLaaS to understand how the software uses the ML API outputs to make application decisions. Then \tool constructs loss functions that penalize the critical errors of the applications. Finally, \tool re-trains the ML models behind the ML APIs with the constructed loss function, without modifying the output interface of the ML APIs. 

% In this section, we will introduce how \tool performs static analysis and constructs the loss functions for the applications. 


% \subsection{Understanding Software Context}

% \subsection{Notations}
% \yh{not 3.2 }
% Denote the total number of classes that the ML model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows:

% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the DNN behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}



% \subsection{How to customize the ML model in the MLaaS backend}
\subsection{Customizing ML model for an application decision process}
\label{sec:loss}
% As introduced in \S\ref{sec:empirical},  applications in the wild differ greatly in their application's decision processes. 
% % For example, they may  define different number of target classes or include only a small subset of labels of the whole label set in their target classes and so on. 
% This heterogeneity can lead to differences in critical errors\jc{remind people what critical errors are?} across applications. 
% It is possible for an ML API error to be non-critical for one application, while critical for another. Thus, customizing the DNN in the MLaaS backend is important in order to incorporate the differences in application's decision processes across applications.
% \jc{the whole first paragraph is redundant to 3.1. this para should highlight why we start by explaining the step of DNN re-training}

% Model re-training has been widely adopted in ML to update the generic pre-trained ML models to work for related but different tasks~\cite{mullapudi2019online,ekya}. In model re-training, the model is initialized from a pre-trained model, and  its model parameters are updated based on the goal of the new task.
The idea of model re-training has been widely adopted in ML to update the generic pre-trained ML models to work for related but different tasks~\cite{mullapudi2019online,ekya}. The key challenge is how to formulate the customized optimization goal and design re-training strategy to efficiently achieve high  accuracy on different tasks.
\shan{Reading this sentence, as a picky reviewer, I would start worrying about the novelty of this work over model re-training work. The next sentence ``In our problem setting'' reads quite similar to the previous sentences. Is it possible to rephrase so that the difference is more obvious?}  \cc{Done. I feel the last sentence actually do not provide new information. So I deleted it.}
% In our problem setting, we want to initialize from a pre-trained model for the original ML task (\eg image or text classification), and re-train it with our customization goal.  
  

Our {\bf customization goal} is to minimize the critical errors for each application.
% caused by ML API errors. 
If we view the application's decision process  as $\z = \Decision(\API(\x))$, where $\x$ is the input to the API, $\API(\x)$ is the ML API output, and $\Decision$ is the post-processing the application performs to make decisions based on API outputs. 
Let $\x_i\in \X$ denote the $i^{th}$ input to the ML API, and $\hat{y_i}$ denote its ground-truth label. 
% $API(x_i)$ is a list of probabilities for label-based API (\eg image or text classification), 
% [$p_1, p_2, \dots, p_n$], for every label in the whole label set, and a score $O_i$ for score-based API (\eg sentiment analysis API). 
Formally, our customization goal is written as:
% Let $\mathds{1}_{x}$ denote the indicator function, where $\mathds{1}_{x} = 1$ when $x$ is \emph{True} and 0 otherwise. Therefore, the customization goal is:

\begin{equation}
    \min |\{x_i \in X | Decision(API(x_i)) \neq Decision(\hat{y_i})\}|
    \label{eq:goal}
\end{equation}


A common practice in ML is to utilize the loss function to express the optimization goal~\cite{celoss}. For example, the Binary Cross Entropy loss is used in image or text classification tasks, and Mean Squared Error loss is used in regression tasks. 

% Take classification task as an example, the Binary Cross Entropy loss is defined as:

% \begin{equation}
%     L_{BCE}(y_i) = \sum_{j=1}^{n} -\hat{y_{i, j}} \cdot log(y_{i,j}) - (1-\hat{y_{i,j}}) \cdot log(1-y_{i,j})
%     \label{eq:bce}
% \end{equation}
% where $y_i$ is the output of the ML model on the $i^{th}$ input, which is a list of probabilities. The higher the probability at the $j^{th}$ index is, the more confident the model is about the existence of the $j^{th}$ label in the input.  $\hat{y_i}$ is the ground truth for the $i^{th}$ input. $\hat{y_{i,j}} = 1$ if the $j^{th}$ label is in the ground truth of the $i^{th}$ input. Intuitively, this loss function incurs a high penalty when the $j^{th}$ label is present in the ground truth, but the model outputs a low probability for it, and vice versa. 

The question we want to answer is,  \emph{how to design a loss function that can achieve our customization goal?}

\mypara{Strawman}With the observation that applications typically heavily cluster on a small subset of labels appearing in the target classes(\S\ref{sec:empirical}), we naively come up with a \emph{strawman} of loss function design: assigning higher penalties to errors made by the ML model on inputs whose ground-truth decisions are selecting the target classes. 

% \begin{equation}
% L(y_i) = w_i \cdot T_i \cdot L_{BCE}(y_i) + (1-T_i) \cdot L_{BCE}(y_i)
% \end{equation}
% where $w_i$ is a large weight (\eg $w_i = 20$), and $T_i = 1$ if the ground-truth labels of the $i^{th}$ sample overlap with the applications' target classes, and 0 otherwise. 


% Intuitively, this \emph{strawman} loss function is compatible with our goal since it prioritizes the reduction of the loss on the samples belonging to the target classes than the non-target ones. 

Take the classification task  as an example to illustrate this idea. 
The ML model predicts a list of probabilities for an input, in which the $j^{th}$ element describes how confident the model is about whether the $j^{th}$  label exists in the input. 
The ground truth is a list, where the $j^{th}$ element is 1 if the $j^{th}$ label exists in the input, and 0 otherwise. 
The pre-trained model is trained to reduce the \emph{average} errors between the probabilities and the ground truth across a wide range of labels (\eg 9605 labels in Open Images~\cite{ASL}).
On the other hand, 
this strawman approach can prioritize the reduction of errors on the inputs whose ground-truth decisions are selecting the target classes. 
However, the strawman penalizes mis-classifications within one target class, such as mis-classifying a paper image into plastic in the garbage classification application example in Figure~\ref{fig:code}(a), and this type of errors are non-critical to the application.
% because the strawman is unaware that different applications may make different decisions given the same output (\eg \emph{True-False}, \emph{Multi-select}, and \emph{Multi-choice}) and how these decisions affect the severity of ML model errors
\shan{This last sentence is not clear.}. 

\mypara{New loss function}We propose a new loss function directly constructed from the \summary.
% \yh{Why they fails and we do not fail }
% \yh{add general recipe }
Compared to the strawman which may spare energy penalizing non-critical errors\shan{?? what exactly are non-critical errors spared by strawman?} \yh{I put in the last para: \ie mis-classifications within one target class}, 
our proposed solution only focuses on penalizing the critical ones. 
Specifically, two types of critical errors are being penalized\shan{I don't understand the (1) and (2) presented below}: 
(1)\shan{Hmm, what does this mean?}\emph{all} the labels in a target class have low probabilities in the prediction, but ground-truth decision selects it. 
(2) \emph{at least one of} the labels in a target class has a high probability, but ground-truth decision does not select it.

\tool's  loss function uses the Sigmoid function (\ie $Sigmoid(y) = \frac{1}{1+e^{k\cdot y}}$) to penalize the critical errors. The intuition behind using the Sigmoid function is that it provides a differentiable way to incur a high penalty when $y >0$\shan{what is y?}, and a low penalty otherwise, which appropriately fits our needs. 

% , such as mis-classifications across target classes. 
% For example, the strawman penalizes mis-classifications within the target classes, which are non-critical, while 



Formally, the loss function can be written as:

\begin{align*}
L_{i} &= 
\overbrace{ \sum_{j \in \{ \textrm{selected target classes}\}} ~\textrm{Sigmoid}(\F(y_i)-M_j(y_i))
}^{\substack{\text{\sf \footnotesize {Penalize low probability for the selected target class
	}} 
}} \\ &+ 
\overbrace{\sum_{j \in \{ \textrm{unselected target classes}\}} \textrm{Sigmoid}(M_j(y_i)-\Q(y_i) )
}^{\substack{\text{\sf \footnotesize {Penalize high probability for the unselected target class
	}} 
}} \label{eq:loss}
\end{align*}
where $M_j(y)$ is the \emph{maximum} probability in $y$ at indices that belong to the $j^{th}$ target class.  $\Q(y), \F(y)$ are two scores that differ by different types of applications. Generally, $ \F(y) > M_j(y)$ or $ M_j(y) > \Q(y)$ suggest that $y$ leads to an incorrect decision, otherwise, a correct decision is made\shan{hmmm, too complicated for me to understand} \yh{Working on how to make this clearer now}. 
% where $H_o(y) = 1$ if $y$ leads to the selection of the non-target class, and $H_o(y) = 0$ otherwise. $H_j(y) = 1$ if $y$ leads to the selection of the $j^{th}$ target class, and  $H_j(y) = 0$ otherwise. $Q_j(y) = 0$ for applications making \emph{Multi-Choice} decisions in API-output order, and $Q_j(y) = 1-H_j(y)$ otherwise. 
% $\theta$ is the prediction threshold of ML model, where any labels whose predicted probability is higher than it will be included in the output. $G_j(y)$ is the maximum probability in $y$ at indices that belong to the $j^{th}$ target class. $G(y) = max_{j \in \{1, \dots, m\}} (G_j(y))$ is the maximum probability in $y$ at indices belonging to all the target classes. $\F(y) = max$($\theta$, maximum probability in  $y$ at the indices that belong to any ground-truth unselected target class(es)). 

% In order to achieve the goal of re-sampling the training data,  our loss function assigns a weight $\frac{M}{N_i}$, where $M$ is the total number of data in the original training dataset, and $N_i$ is the number of training samples whose ground-truth labels overlap with the ground-truth target class(es) of the $i^{th}$ input. This weight, intuitively,  alleviates the effect of class skews in the original dataset by assigning higher weight to less dominant target classes, and lower weight for more dominant ones. 
% \yh{care more about the target classes} 


% M is the total number of data in the original training dataset. $N_i$ is the total number of data whose ground-truth selected target class(es) overlap with the ground-truth target class(es) of the $i^{th}$ input.  

As we have seen in \S\ref{sec:empirical}, the critical errors can vary greatly across different types of application's decision processes. Thus, in order to accurately capture the critical errors, we design different loss functions for each type of decision process. 

% Next, we describe the loss function for each type of decision process case-by-case. 


\mypara{True-False} In \emph{True-False} decision, only one target class is defined, and the application checks if the API output matches with it. 
Denote the prediction threshold of the ML model as $\theta$, where all the labels whose probabilities are higher than it will be included in the output. 
In this case, $\F(y) = \theta$, and $\Q(y) = \theta$. \shan{I understand the next few sentences, but I don't understand why F(y) is $\theta$, and 
Q(y) is $\theta$. I went back to read the $L_i$ formula, but still don't understand.}
For an input whose ground-truth decision selects the target class, a high penalty will be incurred if none of the labels in the target class appear in the output. 
% Thus, when the maximum probability for labels belonging to the 
On the other hand, for an input whose ground-truth decision selects the non-target class, a high penalty will be incurred  when there is at least one label in the target class included in the output. 

\mypara{Multi-Select} As for \emph{Multi-Select} decision, multiple selections are allowed about which target class(es) the ML API output matches with. 
In this case, the ground-truth target class(es) are those which overlap with the ground-truth labels of the input. 
$\F(y) = \theta$ and $\Q(y) = \theta$ for this type. 
The loss function will incur a high penalty when there are ground-truth target class(es) whose maximum probability is lower than $\theta$, 
or when there are target class(es) unselected by ground-truth whose maximum probability is higher than the $\theta$. 
\shan{Is Multi-Select's loss function essentially the same as True-False? Or, maybe you can tell me what exactly is the difference between them?}


% Denote the output of the ML model on the $i^{th}$ input as [$y_{i, 1}, \dots, y_{i,n}$]


\mypara{Multi-Choice application choice order} This type of application reaches only one selection by checking if the highest-priority target class matches with the output labels, if not, it moves on to the next target class, and so on. In this case, the ground-truth target class is the highest priority class out of those overlapping with its ground-truth labels. $\F(y) = max(\theta$, \textrm{maximum probability in $y$ at indices of unselected target class(es)}), and $\Q(y) = \theta$. Take the example in Figure~\ref{fig:loss} to illustrate. The application defines three target classes. Given an input image whose ground-truth label is \code{``Mansion''}, the ground-truth target class is the second one. In this example, $\F(y_i) = max(\theta, M_1(y_i)) = 0.8$ because the first target class has higher priority than the ground-truth target class. $\Q(y_i) = 0.5$ in this example. Thus, the penalty incurred by the loss function is Sigmoid(0.8-0.5) + Sigmoid(0.8-0.7) + Sigmoid(0.4-0.5). 
 
We can see that the loss function will incur a high penalty if any target class(es) with higher priority than the ground-truth target class are included in the output. 


\begin{figure}
     \includegraphics[width=\linewidth]{figs/loss.pdf}
    \caption{Illustration of \tool's loss function.
    }
\label{fig:loss}
\end{figure}


\mypara{Multi-Choice API output order} In this case, similar to the application choice order, only one selection is allowed. However, the application reaches a decision by checking if the first output label matches with any of the target classes, if not, it moves on to the next output label. 
In this case, the ground-truth target classes are those  overlapping with ground-truth labels. 
$\F(y) = max(\theta, $ maximum probability in $y$ at indices of unselected target classes by ground-truth decision), and $\Q(y) = $ the maximum probability in $y$ at indices of the ground-truth target classes.  
Thus, for the ground-truth target class, only if the maximum probability of it  is smaller than the maximum probability of unselected target class(es) or the prediction threshold, a high penalty will be incurred by the loss function. 


\mypara{Value ranges} As for APIs that output a score $y_i$ to describe the input, applications typically define $m$ value ranges as target classes to make decisions, where the lower bound of the $j^{th}$ value range is denoted as $l_j$ and the upper bound of the $j^{th}$ value range is denoted as $u_j$. The loss function commonly used to optimize for this type of regression task is the Mean Squared Error loss defined as follows:

\begin{equation}
    L_{MSE}(y_i) = (y_i - g_i)^2
\end{equation}
where $g_i$ is the ground truth. 

We construct the following loss function:

\begin{align*}
L(y_i) &= 
\overbrace{ ~\textrm{Sigmoid}(l_j-y_i)
}^{\substack{\text{\sf \footnotesize {Penalize the output if lower than ground-truth lower bound
	}} 
}} \\ &+ 
\overbrace{\textrm{Sigmoid}(y_i-u_j )
}^{\substack{\text{\sf \footnotesize {Penalize the output if higher than ground-truth upper bound
	}} 
}} \label{eq:}
\end{align*}
where $u_j$ and $l_j$ are the upper and lower bound of the value range the ground-truth score selects. 

Similar to the idea of the loss function we construct for classification tasks, compared to the Mean Squared Error loss which penalizes the score $y_i$ if it is not equal to the ground truth,  \tool's proposed loss function only penalizes the score if it falls out of the range that ground truth lies in. 
% MSE loss, borrow the idea 
 

% \jc{
% an example outline of this subsection (each bullet is a para)
% \begin{itemize}
% \item why we start with this? the key step is customizing ML model for each application.
% \item what's the goal
% \item what's a strawman (resampling training data)? and why is it not good (doesn't distinct multi-choice vs multi-option and order of examination)? (this para must be short). if room, also bring up some prior work that also does this
% \item our idea: rewriting loss function. give a general recipe of how this is done
% \item why is it better? (this should directly contrast with the strawman)
% \item more case-by-case explanation.
% \end{itemize}
% }

% \jc{regarding how to explain the goal, you can expand the following: formally an application can be viewed as $z=Decision(Model(x))$. for a given decision process $Decision$, the goal is to minimize $Decision(Model(x_i))\neq Decision(\hat{y_i})$ over a set of $x_i$, where $\hat{y_i}$ is the ground truth label of $x_i$.}



% \mypara{Notations} 
% Denote the total number of classes that the ML model behind the ML API can classify as $n$, and the whole set of classes is $C=\{C_1, C_2, ..., C_n\}$.  We define the symbols in our problem setting as follows. 
% \begin{itemize}
%     \item $I$: the input image
%     \item $G=\{G_1, ..., G_a\}$: ground truth label set of $I$, where $G_i \in C$ for $1 \leq i \leq a$
%     \item $T$: the prediction threshold of the ML model behind the ML API
%     \item $O=\{O_1, O_2, ..., O_b\}$: the predicted classes over the prediction threshold $T$, where $P_i \in C$ for $1 \leq i \leq b$
%     \item $P=\{p_1, p_2, ..., p_b\}$: the corresponding probability for the predicted classes
    
    
% \end{itemize}

% \mypara{Customization goal} For T-or-F, we want to minimize the critical errors which are caused by the API outputs that lead to the  execution of the \emph{False} branch, when the statement should be \emph{True} according to the ground-truth, and vice versa. With the above notations, our goal can be written as:

% \begin{equation}
% \begin{aligned}
% \min \sum\limits_{i=1}^{M}( y_i \cdot \mathds{1}_{\theta - P} + (1-y_i) \cdot \mathds{1}_{P-\theta} )
% \end{aligned}
% \end{equation}

% Where $\mathds{1}_{x} = 1$ when $x > 0$, and 0 otherwise. $y_i = 1$ if the $i^{th}$ input belongs to the class list defined in the branch condition, which we denote as $W$. $\theta$ is the prediction threshold, where classes whose predicted probability is higher than the threshold will be included in the output label list. $P$ is the maximum probability of classes in $W$, in other words, $P = max_{c \in W} p_c$.
% there are two types of critical errors: (1) for inputs whose statement in the branch condition is \emph{True} according to the ground-truth, which we refer to as \emph{target-inputs}, the API outputs lead the application selecting the \emph{False} branch; (2) for inputs whose statement is \emph{False}, the API outputs lead the application selecting the \emph{True} branch. To minimize incorrect application decisions, we want: 




% \yh{Outline of this section: 
% 1. first list the goal in math (or text): minimize the incorrect app decisions
% 2. a naive re-training scheme is to use a training data that  focuses on classes appeared in the apps 3. why this design is not good: it can only solve xxx, but not xxx 4. describe our loss function }
% \yh{goal: minimize the incorrect app decisions; what we have: extracted application's decision process (key dimensions) }
% As shown in our empirical study in Section~\ref{sec:empirical}, we find the application's decision process can be characterized by two aspects: (1) the class list(s) or value ranges that are used in branch conditions (2) the structures of the branch conditions.

% In this section, we will describe how we incorporate the application's decision process in the loss function. Our optimization is composed of two steps: (1) clustering the training data to focus on classes appearing in the branch conditions; (2) constructing the loss functions to be aware of the application's decision process. Our objective is to incur a high penalty on critical errors, and no penalty if the errors make no impact on the application. 


% To begin with, we first introduce the loss function traditionally used in multi-label image classification.


% The binary cross-entropy loss function used in multi-label classification task~\cite{ASL} is denoted as:
% \begin{equation}
%     L_{bce}  = -\frac{1}{n}\sum_{i=1}^n{(y_i\log(p_i) + (1 - y_i)\log(1 - p_i))} \,,
% \end{equation}
% where $y_i = 1$ if class $i$ is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. $p_i$ is the predicted probability for class $i$. 
% \begin{itemize}
%     \item  $y_i = 1$ if the $i^{th}$ class is included in the ground-truth classes for input $I$, and $y_i=0$ otherwise. 
%     \item $p_i$ is the predicted probability for the $i^{th}$ class.
% \end{itemize}
% where $y_i$ indicates whether the $i^{th}$ class exists in the input input $I$ or not. In other words, $y_i = 1$ if the $i^{th}$ class exists in the input $I$, and $y_i = 0$ otherwise. \cc{It is still one sentence, so please do not start a new paragraph}


% \subsubsection{Clustering training data}


% To achieve the first step, one approach is to assign different weights to inputs with ground-truth decisions of executing the \code{Others} branch and non-\code{Others} branches.  
% We take a simple example to illustrate this approach. An application  defines one branch condition to check if the API outputs intersect with a class list $W_1$. $W_1$ is a non-empty subset of the whole label set $C$ that the ML model is able to classify. 
%  The original fraction of images in the training data whose ground-truth  decisions are executing the \code{$W_1$}-branch (\ie $G \cap W \neq \emptyset$), which we refer to as \code{$W_1$}-inputs,  is $A$. 
%  % \cc{This sentence is very hard to read. Can we use phrase like ``which we refer to as $W$-images''?} 
% The fraction of images whose ground-truth decisions are executing the \code{other}-branch is $1-A$,  which we refer to as \code{others}-inputs. If we want to balance the distribution between $W$-inputs and \code{others}-inputs, we can use a loss function that assigns higher weights to \code{W}-inputs:

% \begin{equation}
%     L_D = y_1 \cdot \frac{1}{A} \cdot L_{bce} + (1-y_1)\cdot A \cdot L_{bce} \,,
% \end{equation}
% where $y_1$ indicates whether this input is a \code{$W$}-input or not. In other words, $y_1 = 1$ when the input is a \code{$W$}-input ($G \cap W \neq \emptyset$), and $y_1 = 0$ otherwise ($G \cap W = \emptyset$). 

% In this way, \code{$W$}-inputs and \code{others}-inputs are taking the same effect during training, instead of biasing towards either \code{W} or \code{others}. 

% % We construct loss functions for each type of software represented by the software examples shown in section~\ref{sec:empirical}. \cc{Maybe say some high-level ideas, more intuition}

% \subsubsection{Branch condition structure 1: T-or-F} 

% For the software that defines only one branch condition, checking if the output labels $O$ intersect with a class list $W_1$. We penalize the critical errors: (1) all the classes in $W_1$ are not included in top predictions for \code{$W_1$}-inputs; or (2) at least one class in $W_1$ are included in top predictions for \code{others}-inputs.




% \begin{equation}
%     L_{W_1} =y_1 \cdot \textrm{S}(\theta - P_1) + (1-y_1) \cdot \textrm{S}(P_1 - \theta) \,,
% \label{eq:loss}
% \end{equation}
% where
% $y_1$ indicates whether this input is a \code{$W_1$}-input or not. 
% In other words, $y_1 = 1$ if the input is a \code{$W_1$}-input, and $y_1=0$ if the input is a \code{others}-input. $\theta$ is the prediction threshold, where classes whose predicted probability will be included in the output label list. $P_1$ is the maximum probability of classes in $W_1$ (\ie $P_1 = max_{c \in W_1} p_c  $). $S(x)$ is the Sigmoid function $\frac{1}{1+e^{-k x}}$, which we will denote as $S$ in the rest of the paper. 



% Ideally, we want the loss function to be a step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{no penalty} when $P_1$ is greater than $\theta$ for  \code{$W_1$}-inputs. However, to make the loss function differentiable, we use the Sigmoid function to approximate the step function, which incurs \emph{a high penalty} when $\theta$ is greater than $P_1$, and \emph{a low penalty} otherwise, for \code{$W_1$}-inputs. Similarly for \code{other}-inputs. 



% \subsubsection{Branch condition structure 2: M-to-N-set} 

%  In M-to-N-set, several branch conditions are defined, each checking if a class list intersects with the API output $O$. All the fulfilled branches will be executed. We denote all the $m$ class lists the application uses in branch conditions as {$W_1$, ..., $W_m$}. In this pattern, the ground-truth  decisions is executing \emph{all} the branches whose class lists  intersect with the ground-truth labels. 

% We derive the following loss function for M-to-N-set:
% \begin{equation}
%     L = \sum_{i=1,\cdots,m} y_i \cdot \textrm{S}(\theta - P_i) + (1-y_i) \cdot \textrm{S}(P_i - \theta) \,,
% \end{equation}
% where $y_i$ indicates whether  $W_i$ is among the branches the ground-truth decision executes, in other words, $y_i = 1$ if $G \cap W_i \neq \emptyset$, and $y_i = 0$ otherwise. Similar to Equation~\ref{eq:loss}, $P_i$ is the maximum probability of classes belonging to $W_i$ (\ie $P_i = max_{c \in W_i} p_c$). 

%  Only if the application decisions led by $O$ exactly match with the ground-truth decisions, the penalty will be low.


% % \kt{$\sum_{i=1,\cdots,N} L_{W_i}$}



% \subsubsection{Branch condition structure 3: Priority-list}

% Priority-list defines several branch conditions, and each of them is associated with a class list $W_i$. The application checks the branch conditions from highest to lowest priority until finding the first one whose class list intersects with API output labels $O$. Let $W_i$ (where $1 \leq i \leq m$) denote the class lists used in branch conditions, where class lists with smaller $i$ indicate higher priority. Let $W$ denote the union of the classes in all the whitelists, in other words, $W = \cup^{m}_{i=1}W_i$. The ground-truth decision  is executing the highest priority branch whose associated class list intersects with the ground-truth classes $G$. 

% We derive the loss function as:
% \begin{equation}
% \begin{split}
%     L = y_i \cdot \textrm{S} (\max(\theta, P_{k^{-}})  - P_k ) + 
%     (1-y_i) \cdot \textrm{S}(P - \theta) \,,
% \end{split}
% \end{equation}
% where $y_i = 1$ when the ground-truth decision is executing one of the branches in $\{ W_1, \cdots, W_m\}$ (\ie $G \cap W \neq \emptyset$), and  $y_i = 0$ when the ground-truth decision is executing the \code{others} branch. 
% $k$ is the index of the highest-priority branch whose class list intersects with the ground-truth classes (\ie $k = \min \{i|WL_i \cap G \neq \emptyset\}$). $P_k$ is the maximum predicted probability for classes belonging to $W_k$, and $P_{k^{-}}$ is the maximum predicted probability out of the classes belonging to higher priority branches than the ground-truth branch (\ie $k^{-} = \min \{i | W_i \cap (G \setminus W ) \neq \emptyset \textrm{ and } i < k \}$). $P$ is the maximum probability of the classes belonging to $W$. 

% Given this loss function, only if the highest-priority branch whose class list intersects with the predicted classes $O$ is the ground-truth decision, the penalty will be low. 


% \subsubsection{Branch condition structure 4: Top-label}

% Top-label defines several branch conditions, and associates with each of them with a class list $W_i$, similar to Priority-list. However, unlike Priority-list, it checks the \emph{API output labels} one by one until one of them intersects with any of the class lists. Similar to the previous section, $W$ is the union of classes in all the defined class lists. We denote the classes belonging to class lists intersecting with ground-truth classes as $W^+ = \bigcup_{W_i \cap G \neq \emptyset} W_i$, and the classes belonging to \wls that do not intersect with ground-truth classes as $W^- = W \setminus W^+$.
 
% In this pattern, the ground-truth decision is to execute the branch condition  whose class list  intersects with the ground-truth classes. 

% We derive the loss function as:
% \begin{equation}
%     L = y_i \cdot S(\max(P^{-}, \theta) - P^{+}) + (1-y_i) \cdot S(P^- - \theta) \,,
% \end{equation}
% where $y_i  = 1$ indicates that the ground-truth decision is executing one of the branches in \{$W_1$, $W_2$, ...$W_m$\}, and $y_i = 0$ indicates the ground-truth decision is selecting \code{others}, similarly to the previous section. $P^{+}$ is the maximum probability out of classes in $W^+$ (\ie $P^+ = \max_{c \in W^+ } p_c$), and $P^-$ is the maximum probability out of classes in $W^-$ (\ie $P^- = \max_{c \in W^- } p_c$). 


% Given this loss function, we can ensure that only when the first class encountered in the predicted labels, that belongs to $W$, is one of the classes in the ground-truth decision, the penalty would be low. 




\subsection{How to extract the application's decision process}
\label{sec:extract}
% How we use sym-ex to get info, and which info 
% \yh{Change all the whitelists}
To extract application's decision process, we conduct an offline static analysis to detect code patterns introduced in Section~\ref{sec:empirical}. 
Particularly, we focus on the control-flow structures that are directly affected by ML API results. 

Given a code location of ML API invocation, \tool analyzes all the if-branches that have dependency on the ML API's output. 
\shan{hmmm, I feel your paper discussion so far has never talked about ``combination of branch decisions''. I don't have a clear picture about how it would fit our taxonomy ...}\cc{Updated}
Particularly, we focus on the branch conditions that software compares ML API output with certain values to make selection decisions, which are typically reflected by whether executing the target branch edge.
For each possible software decisions, \tool adopts standard symbolic execution to find all the API outputs that lead to these decisions, which is the corresponding target class.
If the software specifies only one target class\shan{what exactly does this mean ...}\cc{Done}, \tool reports pattern True-False. Otherwise, \tool analyzes the code structure to determine the pattern. % according to Figure~\ref{fig:hierarchy}:

\emph{Whether multi-select or multi-choice?} \tool analyzes all the statements inside the edges of an \shan{What is the definition of ML-API-related if-branch? I know we probably already used this phrase before. However, here, we are talking about static analysis, so we need to be particularly precise.}\cc{Done} if-branch that compares ML API output with target class. If the software exits the examination process after making a selection \shan{no no no. This is not a precise PL language. I don't know what you mean by ``terminates all examination inside one ...''. If you are doing control flow analysis here, you need to use control flow language to describe your algorithm.}\cc{How about this?} (\eg a break statement inside the loop and a return statement inside a function body), \tool regards that it as a multi-choice and further examines the order. 
If there is no such exit\shan{``termination'' usually refers to the termination of a program.}\cc{Done}, \tool determines it is multi-select structure. 


\emph{How is the order determined?} \tool finds all the loop structures\shan{??? what are ``equivalent statements''???}\cc{Removed. I put that phrase just in case there are other statements that lead to loop-like control flow} outside the ML-API-related if-branches. It analysis their nested levels and the data dependency relationship of their iterators -- due to Python syntax, the loop structure typically directly specify the list/set to be iterated (\eg~\code{for iterator in list}).
If the software does not contain any loop iterating ML API's output or application choices, \tool stops examination and reports an absence of code pattern. 
If an inner (outer) loop iterates\shan{how do you even know what variables a loop ``iterates'' through??? For example, in LLVM, index variables are identified for certain simple loops, but not all. I cannot believe you can identify what variables a loop ``iterates'' through for any type of loops. There must be unwritten assumptions here.}\cc{There's a widely-used Python syntax \code{for iter in list}. } the ML API's output and the outer (inner) loop iterates the application choices, \tool regards it as pattern Application-choice order (API-output order).  Note that, if the software contains multiple nested loops iterating the same variable, \tool focuses on the innermost one.


\subsection{How to integrate \tool in the MLaaS backend}
\label{sec:runtime}
TO-DO
To apply the \tool in xx,  we still keep the ML API, when users 

\tool modifies the MLaaS backend to serve the customized ML model per application. 
The MLaaS backend, as described in \S\ref{sec:overall}, adds the ML model to a model pool.
As depicted in Figure~\ref{fig:system}, when a user of an application queries the ML API, same as existing ML API querying, he/she first sets up a per-application authentication credential~\cite{google-cloud}, which is used for billing purposes. Then, when the user feeds the input to the ML API, the backend of MLaaS probes the model pool of customized ML models, selects the right model customized to the 

==> backups/3-method.tex <==
\begin{itemize}
    \item We argue that, the key challenge for desiging an efficient  inference serving system for Transformer-based generative models lies in how to reduce the size of pre-computed Attention keys and values. 
    \item Existing compression schemas are not enough to make the pre-computing pay-off the cost of re-compute
    \begin{itemize}
        \item first show a figure that compares baselines compression ratio, and show that it still cannot fit the latency budget 
        \item  In order to meet the fetching latency budget make the inference delay with pre-computing context pay-off the inference delay with re-computing context, we need to apply better compression method. We then show the preliminary results of potential compression strategies that will be able to fit the latency budget
    \end{itemize}
    \item Lastly, we present some potential system challenges in designing such a system for storing and fetching context
    \begin{itemize}
        \item How to predict whether the fetching latency budget can be met? This is challenging because the real fetching delay can depend a lot on the dynamic system resource usage
    \end{itemize}
\end{itemize}


==> backups/6-discussion.tex <==
\label{sec:discussion}

TO-DO



==> backups/abstract-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\begin{abstract}

As large language models (LLMs) take on more complex tasks, their inputs incorporate increasingly {\em long contexts}.
For instance, to answer a domain-specific question, supplementary texts that contain domain knowledge are added to the LLM input as the context of the question, with longer contexts often yielding better response quality.
However, long contexts pose a challenge, when they must be fetched and processed on-demand before the generation can start.
%and personal-assistant applications might need the conversation history between a user and the LLM as the context to answer the user's next prompt. 
%In both cases, longer contexts yield better generation quality, however, it also poses a challenge to load and process long contexts efficiently. 
Directly feeding a long context to the LLM results in significant computational delays, but retrieving the intermediate key-value (KV) features of the context require high network bandwidth.
Though some emerging methods can shorten contexts or reduce KV tensor size in GPU memory, it remains a challenge to minimize or control the loading delays of long contexts without impacting generation quality or modifying the LLM.

%If we feed a long context directly to the LLM, it will take too long for the LLM to process them before generation starts, whereas if we cache the intermediate key-value features of the contexts, it will take much storage space and significant delay to load the key-value cache to GPU when they are fetched remotely.

This paper presents \name, a fast context-loading system for LLMs.
Unlike recent methods that reduce the dimensions of context or KV features in GPU memory, \name accelerates the loading of long contexts by compressing their KV caches into compact bitstreams, reducing the network bandwidth needed for transmission. 
The compression leverages a tailored arithmetic coder and layer-specific quantization, taking advantage of KV features' distributional characteristics, such as locality across nearby tokens.
%further compresses key-value caches to bitstreams that require by leveraging key-value features' distributional properties, such as locality across nearby tokens, custom entropy coding, and layer-specific quantization.
%Furthermore, \name reduces the computation delay of long contexts by pipelining the loading of key-value features at each layer and computation of layer-wise inference to generate new tokens.
Moreover, \name allows the application to specify a context-loading deadline and automatically chooses the compression level (\eg quantization) and loading strategy (\eg loading context directly vs. the KV cache) to meet the deadline with minimum quality degradation on generation.
Our evaluation shows that compared to prior methods to handle long context (\eg gisting and quantization), \name reduces bandwidth usage by \fillme\% and the loading delay by \fillme\% while achieving the same generation quality in terms of perplexity or accuracy.
Importantly, as \name requires no change on the input tokens or the pre-trained LLM, it could be combined with parallel efforts in ML to speed up LLM inference or condense long contexts to fewer tokens. 


%To our best knowledge, \name is the first to optimize the communication and dynamic loading of long contexts for LLM inference, and it is complementary to recent efforts that speed up LLM inference or fit long contexts in GPU memory. 
%Our evaluation shows that compared to existing techniques to compress context (\eg gisting and quantization), \name reduces the size of key-value caches by \fillme\% and the delay of generating the first token by \fillme\% while achieving the same generation quality in terms of perplexity and accuracy.

\begin{comment}
It entails three techniques to greatly speed up both loading and processing of long context for LLMs with only marginal quality degradation.
%\name chooses between (1) directly loading the memory text to LLM to be processed from scratch, which sends much less data but needs substantial computation, or (2) loading the cached key-value features of the memory, which sends more data but saves much computation.
%two strategies: 
%(1) when the memory text is short, we feed the memory text to LLM and let it process the memory from scratch; and 
%(2) when the memory text is long, we cache the key-value features of the memory text and apply a novel compression algorithm to significantly reduce the feature size and speed up the loading of key-value features under limited bandwidth.
%To speed up memory-augmented LLM inference, \name contains three components. 
First, \name compresses the key-value features of long contexts by leveraging distributional properties of the transformer-generated key-value features.
Second, \name fetches and loads the cached key-value features into GPU in a layer-wise fashion, to pipeline the fetching of key-value features and computation of self-attention.
Third, \name automatically switches between loading key-value features and directly feeding the context text to the LLM, depending on the length of the context and the speed of LLM inference.
%which requires more computation but minimizes data transmission, leading to a smaller loading delay, especially when the context is short enough.
%it judiciously combines  between loading cached key-value features, which sends more data but reduces computation, and directly feeding the context text to the LLM, which minimizes data transmission but requires more computation.
To our best knowledge, \name is the first to optimize the compression and communication of long context for LLM inference and is complementary to parallel recent efforts that speedup LLM inference or enable LLMs to process long context. 
Our evaluation shows that compared to existing techniques to compress context (\eg sampling and quantization), \name reduces the size of context by \fillme\% and the delay of generate the first token by \fillme\%.
\end{comment}

%A context in LLM input might be the conversational history between a user and the LLM, or some supplementary text retrieved from a background knowledge base to help answer a query. 
%As users have more interactions with LLMs
%As the contexts increase in size, however, it becomes more challenging to load them remotely into the GPUs that run the LLM.

\end{abstract}



\begin{comment}
\begin{abstract}
% \fillme
As large language models (LLMs) take on increasingly complex tasks, we see an emerging trend that these LLMs take inputs that have longer {\em contexts}.
When a user enters a prompt, the input to LLM will also include a context that encompasses broader information that LLM uses to generate a response. 
%The context in an LLM input encompasses broader information that LLM uses to generation response. 
A context might be the entire conversational history of interactions between a user and the LLM, or it might be some supplementary text retrieved from a background knowledge base and provided to the LLM as part of a query.
%(1) with long sequences of queries and (2) with reference to additional documents. 
%As a result, LLM inference is augmented with a {\em memory} (\eg conversational history or additional documents).
As the contexts increase in size, however, it becomes more challenging to load them remotely into the GPUs that run the LLM.
%However, the best strategy to load such growing context into GPU for fast text generation remains unclear, especially given that the context can be long, dynamic, and fetched remotely from a different location through the network.
To address this, we introduce \name, an efficient context-loading system for LLMs. 
While \name precomputes the context's intermediate LLM output (key-value features) and caches them, much like conventional LLM systems, it also incorporates three components to significantly accelerate the inference.
%\name chooses between (1) directly loading the memory text to LLM to be processed from scratch, which sends much less data but needs substantial computation, or (2) loading the cached key-value features of the memory, which sends more data but saves much computation.
%two strategies: 
%(1) when the memory text is short, we feed the memory text to LLM and let it process the memory from scratch; and 
%(2) when the memory text is long, we cache the key-value features of the memory text and apply a novel compression algorithm to significantly reduce the feature size and speed up the loading of key-value features under limited bandwidth.
%To speed up memory-augmented LLM inference, \name contains three components. 
First, a novel compression algorithm is employed to shrink the size of key-value features of context by leveraging distributional properties of the key-value features.
Second, \name fetches and loads the cached key-value features into GPU layer by layer in a way that pipelines the fetching of key-value features and computation of attention on loaded layers.
Third, \name automatically switches from loading cached key-value features to directly feeding the context text to the LLM, which requires more computation but minimizes data transmission, leading to a smaller loading delay, especially when the context is short enough.
%it judiciously combines  between loading cached key-value features, which sends more data but reduces computation, and directly feeding the context text to the LLM, which minimizes data transmission but requires more computation.
To our best knowledge, \name is the first to optimize the compression and communication of long context for LLM inference and is complementary to other efforts that enable LLMs to handle longer context. 
Our evaluation shows that \fillme

%\jc{the intro and abstract may need to be updated with in-context learning}

%this memory must be first encoded, in the form of key and value features, and loaded in GPU RAM before the LLM can generate the response, causing substantial additional delay.
%% each user interacts with LLMs over a long period of time and from multiple locations, and that more {\em contextual data}, such as dialog history or relevant knowledge, must be dynamically fed to LLMs for high-quality text generation. 
%% Consequently, as a growing amount of contextual data cannot be always kept in GPU memory, they must be dynamically retrieved.
%Though the key-value features are cacheable, a key question remains --- {\em when the cached key-value features are not cached locally in GPU memory, how to minimize the delay of retrieving them without affecting the quality of LLM inference?} 
%To tackle this challenge, we present \name, a retrieval system of key-value features of memory-augmented LLMs.
%\name consists of a compression scheme tailored for key-value features and a controller that dynamically chooses the compression level depending on the amount of contextual data and how much delay is tolerable.
%\name, to our best knowledge, is the first to optimize the compression and communication of key/value features and is complementary to existing efforts that select or cache key/value features. 
%Our evaluation shows that \fillme
\end{abstract}

\end{comment}

==> backups/abstract-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\begin{abstract}

As large language models (LLMs) take on more complex tasks, their inputs incorporate increasingly {\em long contexts}.
For instance, to answer a domain-specific question, supplementary texts that contain domain knowledge are added to the LLM input as the context of the question, with longer contexts often yielding better response quality.
However, long contexts pose a challenge, when they must be fetched and processed on-demand before the generation can start.
%and personal-assistant applications might need the conversation history between a user and the LLM as the context to answer the user's next prompt. 
%In both cases, longer contexts yield better generation quality, however, it also poses a challenge to load and process long contexts efficiently. 
Directly feeding a long context to the LLM results in significant computational delays, but retrieving the intermediate key-value (KV) features of the context require high network bandwidth.

%If we feed a long context directly to the LLM, it will take too long for the LLM to process them before generation starts, whereas if we cache the intermediate key-value features of the contexts, it will take much storage space and significant delay to load the key-value cache to GPU when they are fetched remotely.

This paper presents \name, a fast context-loading system for LLMs.
Unlike the recent methods that shrink the tensor size of KV features, \name aims at reducing the network bandwidth needed for transmitting KV features of long contexts by compressing them into compact bitstreams using a new context encoder.
%the loading of long contexts by compressing their KV features into compact bitstreams using a custom context encoder, thus reducing the network bandwidth needed for transmission. 
\name's context encoder combines layer-specific quantization with a tailored arithmetic coder that takes advantage of KV features' distributional characteristics, such as locality across nearby tokens.
%further compresses key-value caches to bitstreams that require by leveraging key-value features' distributional properties, such as locality across nearby tokens, custom entropy coding, and layer-specific quantization.
%Furthermore, \name reduces the computation delay of long contexts by pipelining the loading of key-value features at each layer and computation of layer-wise inference to generate new tokens.
Moreover, \name allows applications to specify a time budget for loading context and automatically chooses the compression level (\eg quantization) and loading strategy (\eg loading the KV cache or the text) that minimizes the quality degradation without violating the specified time budget.
\name is a simple plug-and-play module, requiring no new training or change on the pre-trained LLM. 
Yet, it demonstrates a great room for improving the loading of long contexts in a distributed setting. 
Compared to prior methods to handle long context (\eg gisting and quantization), \name reduces bandwidth usage by \fillme\% and the loading delay by \fillme\% while achieving the same generation quality in perplexity or accuracy.

%\name can be combined with other emerging efforts that speed up LLM inference or shorten long context. 
%Our evaluation demonstrates that a great room for improving the loading process and minimizing the degradation of generation quality while containing the loading delay.
%Compared to prior methods to handle long context (\eg gisting and quantization), \name reduces bandwidth usage by \fillme\% and the loading delay by \fillme\% while achieving the same generation quality in terms of perplexity or accuracy.

%Importantly, as \name requires no change on the input tokens or the pre-trained LLM, it could be combined with parallel efforts in ML to speed up LLM inference or condense long contexts to fewer tokens. 
%
%Though some emerging methods can shorten contexts or reduce KV tensor size in GPU memory, it remains a challenge to minimize or control the loading delays of long contexts without impacting generation quality or modifying the LLM.


%To our best knowledge, \name is the first to optimize the communication and dynamic loading of long contexts for LLM inference, and it is complementary to recent efforts that speed up LLM inference or fit long contexts in GPU memory. 
%Our evaluation shows that compared to existing techniques to compress context (\eg gisting and quantization), \name reduces the size of key-value caches by \fillme\% and the delay of generating the first token by \fillme\% while achieving the same generation quality in terms of perplexity and accuracy.

\begin{comment}
It entails three techniques to greatly speed up both loading and processing of long context for LLMs with only marginal quality degradation.
%\name chooses between (1) directly loading the memory text to LLM to be processed from scratch, which sends much less data but needs substantial computation, or (2) loading the cached key-value features of the memory, which sends more data but saves much computation.
%two strategies: 
%(1) when the memory text is short, we feed the memory text to LLM and let it process the memory from scratch; and 
%(2) when the memory text is long, we cache the key-value features of the memory text and apply a novel compression algorithm to significantly reduce the feature size and speed up the loading of key-value features under limited bandwidth.
%To speed up memory-augmented LLM inference, \name contains three components. 
First, \name compresses the key-value features of long contexts by leveraging distributional properties of the transformer-generated key-value features.
Second, \name fetches and loads the cached key-value features into GPU in a layer-wise fashion, to pipeline the fetching of key-value features and computation of self-attention.
Third, \name automatically switches between loading key-value features and directly feeding the context text to the LLM, depending on the length of the context and the speed of LLM inference.
%which requires more computation but minimizes data transmission, leading to a smaller loading delay, especially when the context is short enough.
%it judiciously combines  between loading cached key-value features, which sends more data but reduces computation, and directly feeding the context text to the LLM, which minimizes data transmission but requires more computation.
To our best knowledge, \name is the first to optimize the compression and communication of long context for LLM inference and is complementary to parallel recent efforts that speedup LLM inference or enable LLMs to process long context. 
Our evaluation shows that compared to existing techniques to compress context (\eg sampling and quantization), \name reduces the size of context by \fillme\% and the delay of generate the first token by \fillme\%.
\end{comment}

%A context in LLM input might be the conversational history between a user and the LLM, or some supplementary text retrieved from a background knowledge base to help answer a query. 
%As users have more interactions with LLMs
%As the contexts increase in size, however, it becomes more challenging to load them remotely into the GPUs that run the LLM.

\end{abstract}



\begin{comment}
\begin{abstract}
% \fillme
As large language models (LLMs) take on increasingly complex tasks, we see an emerging trend that these LLMs take inputs that have longer {\em contexts}.
When a user enters a prompt, the input to LLM will also include a context that encompasses broader information that LLM uses to generate a response. 
%The context in an LLM input encompasses broader information that LLM uses to generation response. 
A context might be the entire conversational history of interactions between a user and the LLM, or it might be some supplementary text retrieved from a background knowledge base and provided to the LLM as part of a query.
%(1) with long sequences of queries and (2) with reference to additional documents. 
%As a result, LLM inference is augmented with a {\em memory} (\eg conversational history or additional documents).
As the contexts increase in size, however, it becomes more challenging to load them remotely into the GPUs that run the LLM.
%However, the best strategy to load such growing context into GPU for fast text generation remains unclear, especially given that the context can be long, dynamic, and fetched remotely from a different location through the network.
To address this, we introduce \name, an efficient context-loading system for LLMs. 
While \name precomputes the context's intermediate LLM output (key-value features) and caches them, much like conventional LLM systems, it also incorporates three components to significantly accelerate the inference.
%\name chooses between (1) directly loading the memory text to LLM to be processed from scratch, which sends much less data but needs substantial computation, or (2) loading the cached key-value features of the memory, which sends more data but saves much computation.
%two strategies: 
%(1) when the memory text is short, we feed the memory text to LLM and let it process the memory from scratch; and 
%(2) when the memory text is long, we cache the key-value features of the memory text and apply a novel compression algorithm to significantly reduce the feature size and speed up the loading of key-value features under limited bandwidth.
%To speed up memory-augmented LLM inference, \name contains three components. 
First, a novel compression algorithm is employed to shrink the size of key-value features of context by leveraging distributional properties of the key-value features.
Second, \name fetches and loads the cached key-value features into GPU layer by layer in a way that pipelines the fetching of key-value features and computation of attention on loaded layers.
Third, \name automatically switches from loading cached key-value features to directly feeding the context text to the LLM, which requires more computation but minimizes data transmission, leading to a smaller loading delay, especially when the context is short enough.
%it judiciously combines  between loading cached key-value features, which sends more data but reduces computation, and directly feeding the context text to the LLM, which minimizes data transmission but requires more computation.
To our best knowledge, \name is the first to optimize the compression and communication of long context for LLM inference and is complementary to other efforts that enable LLMs to handle longer context. 
Our evaluation shows that \fillme

%\jc{the intro and abstract may need to be updated with in-context learning}

%this memory must be first encoded, in the form of key and value features, and loaded in GPU RAM before the LLM can generate the response, causing substantial additional delay.
%% each user interacts with LLMs over a long period of time and from multiple locations, and that more {\em contextual data}, such as dialog history or relevant knowledge, must be dynamically fed to LLMs for high-quality text generation. 
%% Consequently, as a growing amount of contextual data cannot be always kept in GPU memory, they must be dynamically retrieved.
%Though the key-value features are cacheable, a key question remains --- {\em when the cached key-value features are not cached locally in GPU memory, how to minimize the delay of retrieving them without affecting the quality of LLM inference?} 
%To tackle this challenge, we present \name, a retrieval system of key-value features of memory-augmented LLMs.
%\name consists of a compression scheme tailored for key-value features and a controller that dynamically chooses the compression level depending on the amount of contextual data and how much delay is tolerable.
%\name, to our best knowledge, is the first to optimize the compression and communication of key/value features and is complementary to existing efforts that select or cache key/value features. 
%Our evaluation shows that \fillme
\end{abstract}

\end{comment}

==> backups/abstract-v4.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\begin{abstract}

% \shan{I have reworded the abstact, particularly the first paragraph.}

As large language models (LLMs) take on more complex tasks, their inputs incorporate {\em longer contexts} to respond to questions that require domain knowledge or user-specific conversational histories.
%For instance, to answer a domain-specific question, supplementary texts that contain domain knowledge are added to the LLM input as the context of the question, with longer contexts often yielding better response quality.
Yet, using long contexts poses a challenge for responsive LLM systems, as nothing can be generated
until all the contexts are {\em fetched} to and {\em processed} by the LLM.
Existing systems optimize only the computation delay in context processing (\eg by caching intermediate key-value features of the text context) but often cause longer network delays in context fetching (\eg key-value features consume orders of magnitude larger bandwidth than the text context).
%For instance, caching intermediate key-value (KV) features of long contexts saves computation at the
%cost of potentially higher  
%, but fetching these KV features requires high network bandwidth, thus greatly increasing the overall delay of loading long contexts.
%A common approach to reducing the computation delay of long contexts is to cache the intermediate key-value (KV) features of the contexts, but fetching these KV features requires a high network bandwidth, thus significantly increasing the overall delay of loading long contexts.
%and personal-assistant applications might need the conversation history between a user and the LLM as the context to answer the user's next prompt. 
%In both cases, longer contexts yield better generation quality, however, it also poses a challenge to load and process long contexts efficiently. 
%Directly feeding a long context to the LLM causes a significant computational delay, but fetching the intermediate key-value (KV) features of the context requires a high network bandwidth.

%If we feed a long context directly to the LLM, it will take too long for the LLM to process them before generation starts, whereas if we cache the intermediate key-value features of the contexts, it will take much storage space and significant delay to load the key-value cache to GPU when they are fetched remotely.

This paper presents \name to minimize the delays in fetching \emph{and} processing contexts for LLMs.
\name reduces the bandwidth needed for transmitting long contexts' key-value (KV) features through a novel encoder that compresses KV features into more compact bitstream representations.
The encoder combines adaptive quantization with a tailored arithmetic coder, taking advantage of the KV features' distributional properties, such as locality across tokens.
Furthermore, \name minimizes the {\em total} delay in fetching and processing a context by using
% rather than separately, 
% while maintaining a high LLM performance on various tasks.
% a high generation quality.
%of the network delay and computation delay 
a controller that determines when to load the context as compressed KV features or raw text and picks the appropriate compression level if loaded as KV features.
%based on the context length.
We test \name on three models of various sizes and three datasets of different context lengths.
Compared to recent methods that handle long contexts, \name reduces bandwidth usage by 3.7-4.3$\times$ and the total delay in fetching and processing contexts by 2.7-3$\times$ while maintaining similar LLM performance on various tasks as loading the text contexts.
% similar quality of generated response.
% Compared to the state-of-the-art methods for handling long context (\eg quantization and token selection), \name reduces 
% \shan{is it similar as text-context baseline or similar as quantization-based prior work?}
% while achieving the same generation quality in perplexity or accuracy.


\begin{comment}
Unlike the recent methods that shrink the tensor size of KV features, \name aims at reducing the network bandwidth needed for transmitting KV features of long contexts by compressing them into compact bitstreams using a new context encoder.
%the loading of long contexts by compressing their KV features into compact bitstreams using a custom context encoder, thus reducing the network bandwidth needed for transmission. 
\name's context encoder combines layer-specific quantization with a tailored arithmetic coder that takes advantage of KV features' distributional characteristics, such as locality across nearby tokens.
%further compresses key-value caches to bitstreams that require by leveraging key-value features' distributional properties, such as locality across nearby tokens, custom entropy coding, and layer-specific quantization.
%Furthermore, \name reduces the computation delay of long contexts by pipelining the loading of key-value features at each layer and computation of layer-wise inference to generate new tokens.
Moreover, \name allows applications to specify a time budget for loading context and automatically chooses the compression level (\eg quantization) and loading strategy (\eg loading the KV cache or the text) that minimizes the quality degradation without violating the specified time budget.
\name is a simple plug-and-play module, requiring no new training or change on the pre-trained LLM. 
Yet, it demonstrates a great room for improving the loading of long contexts in a distributed setting. 
Compared to prior methods to handle long context (\eg gisting and quantization), \name reduces bandwidth usage by \fillme\% and the loading delay by \fillme\% while achieving the same generation quality in perplexity or accuracy.
\end{comment}

%\name can be combined with other emerging efforts that speed up LLM inference or shorten long context. 
%Our evaluation demonstrates that a great room for improving the loading process and minimizing the degradation of generation quality while containing the loading delay.
%Compared to prior methods to handle long context (\eg gisting and quantization), \name reduces bandwidth usage by \fillme\% and the loading delay by \fillme\% while achieving the same generation quality in terms of perplexity or accuracy.

%Importantly, as \name requires no change on the input tokens or the pre-trained LLM, it could be combined with parallel efforts in ML to speed up LLM inference or condense long contexts to fewer tokens. 
%
%Though some emerging methods can shorten contexts or reduce KV tensor size in GPU memory, it remains a challenge to minimize or control the loading delays of long contexts without impacting generation quality or modifying the LLM.


%To our best knowledge, \name is the first to optimize the communication and dynamic loading of long contexts for LLM inference, and it is complementary to recent efforts that speed up LLM inference or fit long contexts in GPU memory. 
%Our evaluation shows that compared to existing techniques to compress context (\eg gisting and quantization), \name reduces the size of key-value caches by \fillme\% and the delay of generating the first token by \fillme\% while achieving the same generation quality in terms of perplexity and accuracy.

\begin{comment}
It entails three techniques to greatly speed up both loading and processing of long context for LLMs with only marginal quality degradation.
%\name chooses between (1) directly loading the memory text to LLM to be processed from scratch, which sends much less data but needs substantial computation, or (2) loading the cached key-value features of the memory, which sends more data but saves much computation.
%two strategies: 
%(1) when the memory text is short, we feed the memory text to LLM and let it process the memory from scratch; and 
%(2) when the memory text is long, we cache the key-value features of the memory text and apply a novel compression algorithm to significantly reduce the feature size and speed up the loading of key-value features under limited bandwidth.
%To speed up memory-augmented LLM inference, \name contains three components. 
First, \name compresses the key-value features of long contexts by leveraging distributional properties of the transformer-generated key-value features.
Second, \name fetches and loads the cached key-value features into GPU in a layer-wise fashion, to pipeline the fetching of key-value features and computation of self-attention.
Third, \name automatically switches between loading key-value features and directly feeding the context text to the LLM, depending on the length of the context and the speed of LLM inference.
%which requires more computation but minimizes data transmission, leading to a smaller loading delay, especially when the context is short enough.
%it judiciously combines  between loading cached key-value features, which sends more data but reduces computation, and directly feeding the context text to the LLM, which minimizes data transmission but requires more computation.
To our best knowledge, \name is the first to optimize the compression and communication of long context for LLM inference and is complementary to parallel recent efforts that speedup LLM inference or enable LLMs to process long context. 
Our evaluation shows that compared to existing techniques to compress context (\eg sampling and quantization), \name reduces the size of context by \fillme\% and the delay of generate the first token by \fillme\%.
\end{comment}

%A context in LLM input might be the conversational history between a user and the LLM, or some supplementary text retrieved from a background knowledge base to help answer a query. 
%As users have more interactions with LLMs
%As the contexts increase in size, however, it becomes more challenging to load them remotely into the GPUs that run the LLM.

\end{abstract}



\begin{comment}
\begin{abstract}
% \fillme
As large language models (LLMs) take on increasingly complex tasks, we see an emerging trend that these LLMs take inputs that have longer {\em contexts}.
When a user enters a prompt, the input to LLM will also include a context that encompasses broader information that LLM uses to generate a response. 
%The context in an LLM input encompasses broader information that LLM uses to generation response. 
A context might be the entire conversational history of interactions between a user and the LLM, or it might be some supplementary text retrieved from a background knowledge base and provided to the LLM as part of a query.
%(1) with long sequences of queries and (2) with reference to additional documents. 
%As a result, LLM inference is augmented with a {\em memory} (\eg conversational history or additional documents).
As the contexts increase in size, however, it becomes more challenging to load them remotely into the GPUs that run the LLM.
%However, the best strategy to load such growing context into GPU for fast text generation remains unclear, especially given that the context can be long, dynamic, and fetched remotely from a different location through the network.
To address this, we introduce \name, an efficient context-loading system for LLMs. 
While \name precomputes the context's intermediate LLM output (key-value features) and caches them, much like conventional LLM systems, it also incorporates three components to significantly accelerate the inference.
%\name chooses between (1) directly loading the memory text to LLM to be processed from scratch, which sends much less data but needs substantial computation, or (2) loading the cached key-value features of the memory, which sends more data but saves much computation.
%two strategies: 
%(1) when the memory text is short, we feed the memory text to LLM and let it process the memory from scratch; and 
%(2) when the memory text is long, we cache the key-value features of the memory text and apply a novel compression algorithm to significantly reduce the feature size and speed up the loading of key-value features under limited bandwidth.
%To speed up memory-augmented LLM inference, \name contains three components. 
First, a novel compression algorithm is employed to shrink the size of key-value features of context by leveraging distributional properties of the key-value features.
Second, \name fetches and loads the cached key-value features into GPU layer by layer in a way that pipelines the fetching of key-value features and computation of attention on loaded layers.
Third, \name automatically switches from loading cached key-value features to directly feeding the context text to the LLM, which requires more computation but minimizes data transmission, leading to a smaller loading delay, especially when the context is short enough.
%it judiciously combines  between loading cached key-value features, which sends more data but reduces computation, and directly feeding the context text to the LLM, which minimizes data transmission but requires more computation.
To our best knowledge, \name is the first to optimize the compression and communication of long context for LLM inference and is complementary to other efforts that enable LLMs to handle longer context. 
Our evaluation shows that \fillme

%\jc{the intro and abstract may need to be updated with in-context learning}

%this memory must be first encoded, in the form of key and value features, and loaded in GPU RAM before the LLM can generate the response, causing substantial additional delay.
%% each user interacts with LLMs over a long period of time and from multiple locations, and that more {\em contextual data}, such as dialog history or relevant knowledge, must be dynamically fed to LLMs for high-quality text generation. 
%% Consequently, as a growing amount of contextual data cannot be always kept in GPU memory, they must be dynamically retrieved.
%Though the key-value features are cacheable, a key question remains --- {\em when the cached key-value features are not cached locally in GPU memory, how to minimize the delay of retrieving them without affecting the quality of LLM inference?} 
%To tackle this challenge, we present \name, a retrieval system of key-value features of memory-augmented LLMs.
%\name consists of a compression scheme tailored for key-value features and a controller that dynamically chooses the compression level depending on the amount of contextual data and how much delay is tolerable.
%\name, to our best knowledge, is the first to optimize the compression and communication of key/value features and is complementary to existing efforts that select or cache key/value features. 
%Our evaluation shows that \fillme
\end{abstract}

\end{comment}

==> backups/abstract-v5.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{abstract}

% \shan{I have reworded the abstact, particularly the first paragraph.}

As large language models (LLMs) take on more complex tasks, their inputs incorporate {\em longer contexts} to respond to questions that require domain knowledge or user-specific conversational histories.
%For instance, to answer a domain-specific question, supplementary texts that contain domain knowledge are added to the LLM input as the context of the question, with longer contexts often yielding better response quality.
Yet, using long contexts poses a challenge for responsive LLM systems, as nothing can be generated
until all the contexts are {\em fetched} to and {\em processed} by the LLM.
Existing systems reduce only the context processing delay by re-using the intermediate key-value (KV) cache of contexts.
However, they often cause longer network delays to fetch contexts since the KV cache requires much more bandwidth to fetch than the contexts themselves.

This paper presents \name to minimize the total delay in fetching \emph{and} processing contexts for LLMs.
\name uses two ideas.
First, it greatly reduces the bandwidth needed for transmitting KV cache by a novel encoder that compresses KV cache into more compact bitstream representations.
% \name reduces the bandwidth needed for transmitting long contexts' KV cache through a novel encoder that compresses KV cache into more compact bitstream representations.
Our encoder of KV cache combines adaptive quantization with a tailored arithmetic coder, taking advantage of the distributional properties of KV cache, such as locality across tokens.
Second, to cope with the temporal variance of network throughput, \name splits contexts into {\em token chunks} and stores the KV cache of each chunk at multiple compression levels with various quality-size tradeoffs. 
\name then uses a custom adaptation logic to determine, for each token chunk, in which compression level it should be fetched or whether the throughput is too low and it is faster to compute the KV cache on the fly.
% and uses an adaptation logic to dynamically determine, for each KV chunk, which the compression level should it be 
% Furthermore, \name minimizes the {\em total} delay in fetching and processing a context by using
% % rather than separately, 
% % while maintaining a high LLM performance on various tasks.
% % a high generation quality.
% %of the network delay and computation delay 
% a controller that determines when to load the context as compressed KV features or raw text and picks the appropriate compression level if loaded as KV features.
%based on the context length.
We test \name on three models of various sizes and three datasets of different context lengths.
Compared to recent methods that handle long contexts, \name reduces bandwidth usage by 3.7-4.3$\times$ and the {\em total} delay in fetching and processing contexts by 2.7-3$\times$ while maintaining almost the same LLM response quality on various tasks as loading the text contexts.
% \shan{What does this last sentence mean? Does ``performance'' here mean accuracy or throughput/latency or something else?}
% similar quality of generated response.
% Compared to the state-of-the-art methods for handling long context (\eg quantization and token selection), \name reduces 
% \shan{is it similar as text-context baseline or similar as quantization-based prior work?}
% while achieving the same generation quality in perplexity or accuracy.
\end{abstract}

==> backups/abstract-v6.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{abstract}

% \shan{I have reworded the abstact, particularly the first paragraph.}

As large language models (LLMs) take on more complex tasks, their inputs incorporate {\em longer contexts} to respond to questions that require domain knowledge or user-specific conversational histories.
%For instance, to answer a domain-specific question, supplementary texts that contain domain knowledge are added to the LLM input as the context of the question, with longer contexts often yielding better response quality.
Yet, using long contexts poses a challenge for responsive LLM systems, as nothing can be generated
until all the contexts are {\em fetched} to and {\em processed} by the LLM.
Existing systems reduce only the context processing delay by re-using the intermediate key-value (KV) cache of contexts.
However, they often cause longer network delays to fetch contexts since the KV cache requires much more bandwidth to fetch than the contexts themselves.

\name is a fast context-loading module for LLM systems by {\em (1)} greatly reducing the bandwidth needed to transmit KV cache, and {\em (2)} adapting the KV-compression level based on network throughput to minimize the total delay in fetching and processing contexts while ensuring high generation quality.
\name compresses a KV cache into more compact bitstream representations, by embracing the distributional properties of KV cache, such as locality across tokens.
Moreover, \name splits a context into token chunks and compresses the KV of different chunks separately in multiple compression levels.
Based on the throughput variation, \name adapts the compression level when fetching each token chunk or chooses to compute the KV cache on the fly if the network throughput is too low. 
We test \name on three models of various sizes and three datasets of different context lengths.
Compared to recent methods that handle long contexts, \name reduces bandwidth usage by 3.7-4.3$\times$ and the {\em total} delay in fetching and processing contexts by 2.7-3$\times$ while maintaining almost the same LLM response quality on various tasks as loading the text contexts.


\end{abstract}


%This paper presents \name to minimize the total delay in fetching \emph{and} processing contexts for LLMs.
%\name uses two ideas.
%First, it greatly reduces the bandwidth needed for transmitting KV cache by a novel encoder that compresses KV cache into more compact bitstream representations.
%% \name reduces the bandwidth needed for transmitting long contexts' KV cache through a novel encoder that compresses KV cache into more compact bitstream representations.
%Our encoder of KV cache combines adaptive quantization with a tailored arithmetic coder, taking advantage of the distributional properties of KV cache, such as locality across tokens.
%Second, to cope with the temporal variance of network throughput, \name splits contexts into {\em token chunks} and stores the KV cache of each chunk at multiple compression levels with various quality-size tradeoffs. 
%\name then uses a custom adaptation logic to determine, for each token chunk, in which compression level it should be fetched or whether the throughput is too low and it is faster to compute the KV cache on the fly.
%We test \name on three models of various sizes and three datasets of different context lengths.
%Compared to recent methods that handle long contexts, \name reduces bandwidth usage by 3.7-4.3$\times$ and the {\em total} delay in fetching and processing contexts by 2.7-3$\times$ while maintaining almost the same LLM response quality on various tasks as loading the text contexts.


% and uses an adaptation logic to dynamically determine, for each KV chunk, which the compression level should it be 
% Furthermore, \name minimizes the {\em total} delay in fetching and processing a context by using
% % rather than separately, 
% % while maintaining a high LLM performance on various tasks.
% % a high generation quality.
% %of the network delay and computation delay 
% a controller that determines when to load the context as compressed KV features or raw text and picks the appropriate compression level if loaded as KV features.
%based on the context length.
% \shan{What does this last sentence mean? Does ``performance'' here mean accuracy or throughput/latency or something else?}
% similar quality of generated response.
% Compared to the state-of-the-art methods for handling long context (\eg quantization and token selection), \name reduces 
% \shan{is it similar as text-context baseline or similar as quantization-based prior work?}
% while achieving the same generation quality in perplexity or accuracy.

==> backups/eval-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}[t]
\centering

    \begin{tabular}{@{}c@{}}
        \includegraphics[width=0.92\textwidth]{figs/overall_up.pdf}
        \vspace{-0.4cm}
        \\[\abovecaptionskip]
        (a) KV cache size reduction by dataset.
    \end{tabular}

    % \begin{subfigure}
    %      \centering
    %      \includegraphics[width=0.99\textwidth]{figs/overall_up.pdf}
    %      \caption{Size reduction}
    %      % \label{fig:three sin x}
    %  \end{subfigure}

    \begin{tabular}{@{}c@{}}
        \includegraphics[width=0.92\textwidth]{figs/overall_bot.pdf} 
        \vspace{-0.5cm}
        \\[\abovecaptionskip]
        (b) TTFT reduction vs. LLM performance by dataset.
    \end{tabular}


     % \begin{subfigure}{1\textwidth}
     %     \centering
     %     \includegraphics[width=0.99\textwidth]{figs/overall_bot.pdf}
     %     \caption{TTFT reduction}
     %     % \label{fig:three sin x}
     % \end{subfigure}
    
    \tightcaption{End-to-end test result (KV cache size and TTFT reduction) of the three pipelines.
    % Overall results on three different pipelines shown in Table~\ref{tab:eval}.
    }
    \label{fig:overall}
\end{figure*}


\tightsection{Evaluation}


Our evaluation answers the following key questions:
\begin{itemize}
    \item Given a context, how much can \name's KV encoder reduce the bandwidth needed to transfer its KV cache? 
    \item Given a network bandwidth, how much can \name reduce TTFT (including both network and compute delays)? 
    \item How sensitive is \name's performance gain across different models, context lengths, and network bandwidths? 
    \item Does \name have a better tradeoff between LLM performance and TTFT than baselines that reduce TTFT by pruning the contexts or using smaller models?
    
    % \jc{the items blow dont seem high priority?}
    % \item How much runtime memory usage does \name reduce? 
    % \item What's the overhead of \name?
    % \item How much does each of the components of \name contribute to the total improvement? 
%    \item How generalizable is \name's compressor? 
\end{itemize}




\begin{figure*}[t]
\centering
    \includegraphics[width=.92\textwidth]{figs/sensitivity_all.pdf}
    \vspace{-0.2cm}
    \tightcaption{Sensitivity of \name's gains over the baseline across different token lengths, network bandwidths, and models.}
    \label{fig:sensitivity}
\end{figure*}

\tightsubsection{Setup}


\mypara{Models and testing datasets} 
We evaluate \name on three pipelines, summarized in Table~\ref{tab:eval}, that span models with different sizes and datasets for different tasks.
% Table~??????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????????\ref{tab:eval} summarizes the setup.
% Specifically, we test \name in three pipelines.
\begin{packeditemize}

\item {\em Pipeline A} tests the Llama-13b model and Llama-7b model~\cite{llama}, both scaled with Neural Tangent Kernel (NTK), on the Wikitext~\cite{wikitext} dataset. 
The task is to predict the probability of the next token in a sequence based on the context consisting of relevant documents that belong to a specific Wiki page.
% based on the criterion of belonging to a specific Wikipedia page.
The Wikitext dataset covers a wide range of topics, with the context length ranging from 1.8K-24K tokens.
% The documents in the dataset 
% % are filtered such that they are reviewed by humans are considered well-written, and 
% cover a wide range of topics.
% Most contexts are around 1.8K-24K tokens. 

\item {\em Pipeline B} tests the LongChat-7b-16k model~\cite{longchat2023} on the LongChat~\cite{longchat2023} dataset, recently released to test LLMs on queries like ``What was the first topic we discussed? '' based on all the previous conversations as the context. 
Most contexts are around 9K-9.6K tokens. 
We chose LongChat-7b-16k since it is one of the best models on this dataset.

\item {\em Pipeline C} tests the T5-large model~\cite{raffel2023exploring} on Natural Question dataset~\cite{47761}, a question-answering dataset developed by Google. 
Following previous work (\eg~\cite{atlas}), it tests the model to answer user queries from a Q \& A dataset with the context from  Wikipedia documents relevant to the queries.
Most contexts are around 8K-12K tokens. 
\end{packeditemize}
It is worth noting that these pipelines represent the two typical apps with long contexts (\S\ref{subsec:apps}): chat apps (Pipeline B) and retrieval-based apps (Pipeline A and C).


\begin{comment}
We evaluate \name on a set of popular models following previous works~\cite{??, ??, ??}. 
For conversational applications, we evaluate LongChat-7b-16k models with the LongChat dataset~\cite{longchat2023}. 
For retrieval-based applications, we evaluate the T5-large model~\cite{t5} on the Natural Questions dataset~\cite{nq}  following previous works~\cite{atlas};
 we also evaluate NTK\_scaled\_LLaMA-7B, on the second variant with the Wikitext~\cite{wikitext} dataset.
We use perplexity~\cite{} as the metric to evaluate those range of models. 

\mypara{Applications} We evaluate \name on two types of applications: 
\begin{itemize}
\item Conversational applications: the context is previous conversational history between the user and LLM. Following previous work~\cite{longchat2023}, the LLM tries to answer the user query ``What was the first topic we discussed? '' based on all the previous conversation. 
\item  Retrieval-based applications: the context is all the relevant documents to the user query. 
We evaluate two variants of this retrieval-based applications: (1) Following previous work~\cite{atlas}, the LLM tries to answer user queries from a Q \& A dataset with support from  Wikipedia documents relevant to the queries; (2) Following previous work~\cite{wikitext}, the LLM predicts the probability of the next token in a sequence based on the content of all relevant documents.
\end{itemize}


\mypara{Metrics} We mainly evaluate \name on two types of metrics: 
\begin{itemize}
    \item Delay metric: We use the Time-to-first-token (TTFT) as the delay metric, as described in \S\ref{sec:??}. This is the delay from knowing the prompt till generating the first token. 
    \item Size of key-value caches: We compare the size of the key-value caches for each scheme (which we explain shortly)
    \item Quality metric: For the LongChat task, we use \fillme as the metric. 
    For the retrieval-based applications, we use  F1 score as the metric to evaluate the question answering task. 
    We use the perplexity score to evaluate the second variant.
    The perplexity is defined as the exponentiated average negative log-likelihood of the next token. 
    The larger the perplexity is, the less likely the model is to generate the right next token.
    The F1 score captures how well the generated answer matches the ground truth answer of the question answering task.
    %  \yh{use two sentences to explain perplexity, F1 score}. 
\end{itemize}
\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



%\begin{table}[]
%\begin{tabular}{cccc}
%\hline
%  & Dataset          & Model(s)                                                                               & Quality metric \\ \hline\hline
%A & LongChat         & longchat-7B-16k                                                                        & Accuracy       \\ \hline
%B & NaturalQuestions & T5-large                                                                               & F1 score       \\ \hline
%C & Wikitext         & \begin{tabular}[c]{@{}c@{}}LLaMA-13B\\ LLaMA-7B\end{tabular} & Perplexity     \\ \hline
%\end{tabular}
%\caption{}
%\label{tab:my-table}
%\end{table}

% \mypara{Generation quality metric}
\mypara{LLM task performance}
We measure generation quality using the standard metric of each dataset.
\begin{packeditemize}

\item {\em Perplexity} is used to evaluate the model's performance on the Wikitext dataset. 
The perplexity is defined as the exponentiated average negative log-likelihood of the next token~\cite{ppl1, ppl2}.
A low perplexity means the model likely generates the right next token.
While perplexity does not equate to text-generation quality, it is widely used as a decent proxy~\cite{adiwardana2020humanlike}.
This metric has been commonly used by prior works to test the impact of pruning or quantizing LLMs on generation performance~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% widely used in previous works in evaluating whether shrinking the model size or quantizing models degrade the generation quality~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% \jc{this metric may not sound intuitive to system reviewers. add some citations and explain why we should care about it?}

\item {\em Accuracy} is used to evaluate the model's output on the LongChat dataset. 
The task predicts the first topic in the conversational history between the user and the LLM. 
The accuracy is defined as the percentage of generated answers that exactly includes the ground-truth topic. % It is defined as the percentage of the generated answer that matches the ground-truth first topic of the conversation.
% \jc{Yuhan, please add some details and explain why it is a good metric}

\item {\em F1 score} is used to evaluate the model's response in the Natural Questions dataset.
It measures the probability that the generated answer matches the ground truth answer of the question-answering task.
\end{packeditemize}





\mypara{Baselines} 
We compare \name with baselines that do not change the contexts or model (\S\ref{subsec:eval:micro} evaluates more baselines). 
\begin{itemize}
% \item \code{torch.save}: 
\item {\em ``Original KV''} uses \texttt{torch.save} to serialize the KV features in GPU memory to a file.
This serves as a reference for the most straightforward implementation. 
\item {\em ``Default quantization \& AC''} combines the uniform quantization of KV features~\cite{flexgen} with the default arithmetic coding (AC) that uses a global probability distribution for all elements.
Like \name, this baseline also uses quantization and AC but with a simpler design on each component. 
\item {\em ``Text context''} fetches the text of the context and feeds it to LLM to compute self-attention. 
It represents the design of minimizing data transmission but at the expense of high computation overhead, especially under long contexts.


    % \item \recomp: This scheme sends the texts of the context and compute the \kv based on the texts before generating the first token. 
    % % \item Model quantization baseline: This scheme quantizes the model weights into less number of bits in order to reduce the memory usage at inference time~\cite{??, ??, ??}. For this scheme, we report the quality metrics after applying the model quantization. 
    % % For the size metrics, we report the size of the key-value caches saved by \code{torch.save}.
    % % \item Original models with shorter contexts: This scheme rewrites the contexts with gisting~\cite{??}, and generates the first token with the compressed contexts. \yh{Say a few sentences about the pretrained gisting models only allow us to test on specific models and datasets}
    % \item \kv quantization + \code{torch.save}: This scheme quantizes the key-value cache, and saves the compressed \kv via \code{torch.save}. 
    % \item \kv quantization + naive AC: This scheme quantizes the key-value cache, and saves the compressed \kv via naive AC (\ie no optimization on the grouping of \kv to improve compression ratio). 
    % % \item Smaller model architectures: This scheme approximates the line of work that uses smaller model architectures to reduce the memory footprint of LLMs~\cite{??, ??}. We compare \name's \kv with smaller models' \kv in terms of our metrics. 
    % \item \name (Ours): The orignal models with compressed \kv with \name's compressor and controller. 
\end{itemize}




\mypara{Hardware settings} We use an NVIDIA A40 GPU server to benchmark our results. 
The server is equipped with 384GB of memory and two Intel(R) Xeon(R) Gold 6130 CPUs with Hyper-threading and Turbo Boost enabled by default.
% The server is equipped with 64 Intel(R) Xeon(R) Gold 6130 CPU cores. 
% \yh{describe our CPU and GPU machines }




% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock2.pdf}
%     \tightcaption{Results on Size of KV cache } 
%     \label{fig:mock2}
% \end{figure*}



% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock1.pdf}
%     \tightcaption{Results on TTFT } 
%     \label{fig:mock1}
% \end{figure*}

\tightsubsection{Overall improvement}
\label{subsec:overall_eval}
\mypara{KV cache size reduction} 
Figure~\ref{fig:overall}a shows the size and task performance trade-offs
of \name's KV encoder and the baselines.
% applying the quantization baselines, with default AC or \code{torch.save}, and \name's context encoder to encode the \kv.
Across the three datasets, \name's KV encoder reduces the KV cache size by $3.7-4.3\times$ compared to the best baseline when achieving similar task performance. 
% \name reduces the size of \kv by 4.3$\times$, 3.9$\times $, 3.7$\times$, and 4$\times$ compared to the strongest baseline (8-bit quantization with naive AC) across the three pipelines respectively. 
In particular, the degradation in task performance is very marginal---the increase of perplexity is within 0.5 (which is negligible~\cite{llmint8,smoothquant}), the drop in F1 score is less than 1\%, and the drop in accuracy is below 4\%. 

While our results only show task performance in numbers, \S\ref{sec:appendix} will present concrete examples that compare the generated texts of \name vs. without KV compression.


% The degradation of generation quality is small, with the perplexity score increasing within 0.5~\footnote{Since perplexity is an exponentially growing metric, an increase of perplexity score within 0.5 is really negligible~\cite{llmint8,smoothquant}.} or an F1 score degradation within 1 point (from 59.2 to 58.7) and accuracy degradation within 4-percentage-points (from 100\% to 96\%), compared to the baseline.
% Compared to the baseline that saves \kv tensors with \code{torch.save}, \name reduces the size of \kv by 3.8-4.5$\times $. 

% Note that baseline with default AC reduces the size of \kv more than \code{torch.save} because it further compresses


\mypara{TTFT reduction} 
Figure~\ref{fig:overall}b shows \name's reduction in TTFT when the bandwidth to transfer the context is set to 2~Gbps (\S\ref{subsec:eval:sensitivity} will vary bandwidth).
It shows that \name reduces TTFT by 2.7-3$\times$ compared to the most competitive baseline. 
\name's gains result from reduced KV cache as well as the ability to choose to load text context when the context is short enough (\eg 20\% of contexts in Pipeline A).
% The ``original KV tensor'' baseline (saved by \texttt{torch.save}) has a bigger size but is sometimes faster than the use of default AC, because of the additional decompression overhead of the \texttt{torchac} library.
% As a side note, quatization baseline with \code{torch.save}, which is the default and optimized deserialization tool in Pytorch~\cite{pytorch}, is a little faster than default AC because AC incurs an additional decompression overhead than \code{torch.save}.  


These reductions in KV cache sizes and TTFT confirm \name's effectiveness on different models and datasets. 
% The next section will show more sensitivity tests. 


% This consistent improvement across these models and pipelines also indicate that \name is generally applicable to different model architectures and sizes. 

% Compared to the \recomp baseline, \name is able to reduce the TTFT because it 
% avoids the computation of the self-attention operation on the long context.

% \yh{Comments a bit on why \name can achieve smaller sizes compared to baselines}



\tightsubsection{Sensitivity analysis}
\label{subsec:eval:sensitivity}



% To study how different network bandwidths or input token lengths affect the performance of \name, we conduct a sensitivity analysis to study the impact of these two factors on the gains of \name compared to the baselines.


\mypara{Impact of context length}
Figure~\ref{fig:sensitivity}a varies the input token length from 0.1K to 10K and shows the TTFT reduction of \name compared to the baselines under a fixed network bandwidth of 2~Gbps.
% As shown in the figure, compared to the \recomp baseline, \name can reduce the TTFT by 2-4$\times$.
The result mirrors the illustration of Figure~\ref{fig:intro}.
Specifically, when the context is long, the gain of \name is mostly from reducing the KV cache sizes.
And when the context is short (below 1K), \name automatically reverts to loading the text context, if it is faster than loading any KV cache.
% We can see that \name's speedup generally increases with longer context lengths.
% This is because when the input token length is small, the time of self-attention is small, making the saving from removing the self-attention delay less significant.


\mypara{Impact of network bandwidth}
Figure~\ref{fig:sensitivity}b varies the network bandwidth (0.2 - 10Gbps) and shows \name's TTFT reduction compared to the baselines.
% As shown in the figure, compared to the \recomp baseline, \name can reduce the TTFT by 2-4.5$\times$.
We can see that \name consistently outperforms the baselines on different bandwidths. 
Under a high network bandwidth, \name's reduction of KV cache size results in lower TTFT as less data is transferred.
Under a low bandwidth, \name again reverts to loading the text context as the delay of sending KV cache always outweighs the saving in computation dalays.
% Particularly, when the network bandwidth is low, 
% sending \kv over the network will not be able to compromise the saving in TTFT by removing the time of self-attention. 
% However, when the network bandwidth is large, the time of sending \kv will become less significant, making the saving from removing the self-attention delay more significant.
% We can see that the gains of \name increase as the network bandwidth increases.

% \mypara{Reduction in runtime memory} 
% A accompanied benefit of caching key and value features, compared to the on-the-fly computation baseline, is that it saves GPU runtime memory usage. 
% This is because by caching the key and value features, the memory heavy self-attention operation based on the long input is avoided. As shown in Figure~\ref{fig:}, \name's GPU memory usage is \fillme smaller than the on-the-fly computation baseline.  
% \yh{Comments a bit on what side benefits it can bring: batching is possible for generating the first token with \name}.

% \mypara{Overhead of \name} The overhead of \name is mainly in two aspects. 
% First, before the inference runtime, \name's compressor needs to run AC on the uncompressed \kv , and store them in the storage server. 
% This includes the overhead of moving the uncompressed \kv from GPU to CPU(which causes \fillme seconds overhead), and then applying torchac's encoder on it, leading to an overhead of 0.8 seconds. 
% Secondly, at inference runtime, \name needs to send the compressed \kv over the network bandwidth link, and then apply torchac's decoder on it before feeding to the LLM for inference. 
% The decoder incurs 0.83 seconds of overhead. 
\mypara{Impact of different models}
Figure~\ref{fig:sensitivity}c tests \name with different LLMs but on the {\em same} dataset (Wikitext). 
It shows that across different models, \name consistently reduces TTFT, while achieving negligible degradation to generation quality compared with the default quantization with AC baseline. 
This shows \name's gain is not sensitive to the corresponding dataset with the model. 
% \fillme \jc{Yuhan :)}
%on each type of the model evaluated in \S\ref{subsec:overall_eval}, all on the Wikitext dataset, in order to study whether \name's improvement is sensitive to the xx.

\begin{figure}[t]
\centering
    \includegraphics[width=0.7\columnwidth]{figs/CDF.pdf}
    \tightcaption{The distribution of compressed KV size of each token in the Wikitext dataset.}
    \label{fig:cdf_context}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=0.99\columnwidth]{figs/overhead.pdf}
    \tightcaption{The breakdowns of the average online TTFT (left) to load and process a context in Wikitext, offline delays (middle) to compress a context in Wikitext, and the storage overhead (right) to store the KV cache a context Wikitext.}
    \label{fig:overhead}
\end{figure}

\begin{figure*}[t]
\centering
    \includegraphics[width=1.9\columnwidth]{figs/figure_14.pdf}
    \tightcaption{Comparing \name and more intrusive methods, including smaller models, token dropping (left), context selection (middle), and gisting (right).
    % Zoomed in to lower perplexity scores for better illustration. \kt{more spacing between figures}
    }
    \label{fig:intrusive}
\end{figure*}

\mypara{Size reduction by context}
Figure~\ref{fig:cdf_context} shows the distribution of KV cache sizes under \name and the baselines. 
It shows that across all the contexts in the Wikitext dataset, \name reduces the size of KV Cache by 3.6 to 4$\times$ compared to the original KV, and 4.2 to 4.6 comparing with default quantization \& AC. 
This shows \name's gain over that baselines is not sensitive to specific contexts. 
% \fillme \jc{Yuhan :)}

\tightsubsection{Microbenchmarks} 
\label{subsec:eval:micro}

% \mypara{What's the delay breakdown of \name's context-encoder and the baseline? } 
\mypara{Breakdown of online delays}
While having better compression efficiency on KV features, \name does incur (marginally) more overhead than the baselines.
To examine the overheads in delays, Figure~\ref{fig:overhead}a breaks down the TTFTs of \name and the baselines on a context of 8.5K tokens into data transfer, decompression (or \texttt{torch.load}), CPU-GPU data movement, and computation by LLM in GPU. 
We can see that while \name has slightly more non-transmission delays, particularly decompression, it is overwhelmingly compensated by its reduction in transmission. 
This figure confirms our illustration in Figure~\ref{fig:motivate_baselines}.


%The readers may wonder, comparing to the a relatively simple baseline, which applies the same levels of quantization and directly saves the \kv with \code{torch.save}, how much overhead does \name's context-decoder introduce?
%To be more specific, comparing with saving \kv with \code{torch.save} and deserializing with \code{torch.load}, whose deserialization presumably has lower delay, \name's context-decoder has the higher overhead of decompressing the \kv with AC. 
%Also, since \name's context-decoder requires a further operation 
%Figure~\ref{fig:delay_breakdown} shows the delay breakdown of \name's context-decoder and the quantization and \code{torch.save} baseline.
%
%As shown in the figure, the delay of \name's context-decoder is 0.83 seconds, and the delay to send the \kv from CPU to GPU is 0.12 seconds (with layer-wise loading pipelining as discussed in \S\ref{sec:design}).



\mypara{Offline delays and storage overheads}
\label{subsec:eval:storage}
Unlike prior methods that compress each context only once, \name compresses multiple versions (\S\ref{subsec:controller}), and Figure~\ref{fig:overhead}b and \ref{fig:overhead}c evaluate the overheads in delays and storage. 
We can see that despite needing to encode and store multiple bitstream representations, the total, \name still requires less storage than the baselines since each version requires much less space than the baselines.
\name compresses each context almost as fast as the baselines because the additional compression delays are much smaller than computing KV features. 



% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.5\columnwidth]{figs/intrusive2.pdf}
%     \tightcaption{}
%     \label{fig:intrusive2}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.6\columnwidth]{figs/gisting.pdf}
%     \tightcaption{}
%     \label{fig:intrusive3}
% \end{figure}


\mypara{\name vs. more intrusive methods}
So far, all methods we have evaluated, including \name, do not modify the LLM or context.
As a complement, Figure~\ref{fig:intrusive} tests \name against recent methods that {\em change} the context or LLM. 
\begin{packeditemize}
\item {\em Smaller models:} 
Replacing the LLM with {\em smaller models} may speed up the computation.
Figure~\ref{fig:intrusive}a replaces the Llama-7B model with a smaller Llama-3B and applies different quantization levels. 
\item {\em Token selection:}
Figure~\ref{fig:intrusive}b uses \scis as an example of {\em removing tokens} with low self-attention scores from the LLM input~\cite{liu2023scissorhands}. 
Since the self-attention scores are only available during the actual generation, it cannot reduce TTFT, but we make an effort to create an idealized version of \scis (Scissorhands*) by running the self-attention offline to determine which tokens to drop and provide this information to Scissorhands* online.
\item {\em Context selection:}
Another trick used by some retrieval-based apps is to select fewer documents as the context. 
We test this idea on Pipeline C because the dataset already has this optimization.
By default, it picks the top 20 documents as context, and Figure~\ref{fig:intrusive}b tries top-10 and top-4. 
\item {\em Gisting}
Finally, we test Gisting as an example of a more advanced method that shortens contexts into gist tokens and changes the LLM to accept the gist tokens~\cite{gisting}.
\edit{In Figure~\ref{fig:intrusive}c, we test the pre-trained gisting model, which is based on Llama-7B. 
The gisting model retrains the LLM's attention model in order to run inference on a compressed version of the input prompts. 
Since the gisting model can compress arbitrary long contexts into \textit{one token}, we vary the compression ratio of the gisting model to obtain a trade-off in size and accuracy.
This is done by adapting the fraction of input tokens that are compressed into one token.
% changes the LLM attention scheme and fine-tunes Llama-7B\jc{the phrase right before here is awkward, can we just say "retrain the LLM's attention model"?} to run inference on a compressed version of the input prompts. 
% \jc{is it necessary to have the next sentence?}
% The pre-trained gisting model can compress arbitrary long contexts into 1 token.
% We vary the compression ratio of the gisting model by changing the number of tokens compressed in the LLM input.
% The more tokens gisting compress into one token, the less quality it can achieve.\jc{exactly every how many tokens did you compress to 1 gist token? is that not important?}
We apply \name on the original Llama-7B model on the PIQA~\cite{bisk2019piqa} dataset, which is one of the most popular question-answering datasets. 
We did not apply \name on other datasets in our evaluation because the public pre-trained gisting model can only take up to 512 tokens, and truncating the dataset into smaller chunks will not be able to preserve the information in the context. 
}
% Figure~\ref{fig:intrusive}c tests the pre-trained gisting model re-trained on Llama-7B and compare it with \name which uses the original Llama-7B on PIQA~\cite{bisk2019piqa}, one of the most popular Q/A datasets.\footnote{We did not use the Natural Questions dataset (Pipeline C) because the public pre-trained gisting model cannot work with the long contexts in the open-domain version of Natural Questions.}
\end{packeditemize}
We can see that \name outperforms these baselines, reducing TTFT or KV cache size while achieving similar or better LLM's performance on the respective tasks.
In particular, \name is faster than smaller models (which are slowed down by transformer operations), and can reduce KV cache better than context selection or gisting because it compresses the KV features to more compact bitstream representations.
We want to stress that even though \name is compared head-to-head with these methods, it makes no assumption about the context and the model, so one can combine \name with these methods to potentially further improve the performance.

%\mypara{How does \name compare with context reduction baselines? }
% The evaluation till now assumes the context is already been preprocessed and ready to use. 
% However, there are other works~\cite{??, ??} trying to shrink the length of the context so as to reduce the memory footprint of LLMs. 
%  \yh{say that previous evals assumes the context is given. Now we wanna compare with techniques that reduce context length via prompt rewriting or token selection. }

% \begin{figure}
% \centering
% \includegraphics[width=0.33\textwidth]{figs/scissorhands.pdf}
% \caption{Comparison of \name and \scis*. }
% \label{fig:scissorhands}
% \end{figure}


% \scis removes tokens from the LLM input with low self-attention scores. 
% This method has to execute the  \emph{self-attention} operation in order to determine the tokens to be removed. 
% Thus, \scis would not be able to reduce the TTFT. 
% However, we evaluate the idealized version of \scis to see how much it can reduce the size of \kv. 
% By an idealized version, we simply run the self-attention operation and obtain the scores, and remove those tokens whose attention scores are small.  
% Figure~\ref{fig:scissorhands} shows the quality and size trade-off for \name and \scis. 
% \name even achieves better trade-offs than the idealized \scis. 

% Similarly, we apply another context reduction 
% \yh{todo: add gisting's results}



%\mypara{How does \name compare with smaller model architectures? } 
% To alleviate the high computation delay or the memory footprint of LLMs,
% applications may choose to use smaller model architectures~\cite{??, ??}.
% In order to show if using a smaller model can achieve better trade-offs than \name, we evaluate 
% \name's \kv with smaller models' \kv.
% As shown in Figure~\ref{fig:smaller}, the trade-off curve of the smaller model (Llama-3B) is obtained by varying the quantization levels. 
% We can see that \name achieves better trade-offs than smaller models.


\mypara{Component-wise analysis}
% As shown in Section \ref{sec:??}, \name's context encoder incorporates three key insights. 
To study the impact of individual components in \name's KV encoder,  Figure~\ref{fig:insights} progressively adds each idea into the baseline of uniform quantization and default AC, starting with the use of delta tensors, and  then our AC that uses probability distribution for each channel-layer combination, and finally layer-wise quantization.
This result underscores the substantial contribution from each idea to the overall reduction of KV cache size. %, with the combined effect being particularly impactful.

% Each curve represents a trade-off obtained by adding our AC, delta compression, and layer-wise quantization atop the quantization baseline employing naive AC.

% Our AC technique alone achieves a remarkable reduction in size, approximately two times more efficient than naive AC. 
% The other two insights further enhance the size reduction. Specifically, they reduce the size in comparison to the baseline quantization and our AC by approximately \fillme and \fillme, respectively.


\begin{figure}
\centering
        \includegraphics[width=0.4\textwidth]{figs/insight.pdf} 
        \tightcaption{Contributions of individual ideas behind KV encoder: change-based encoding, layer-wise quantization, and AC based on channel-layer grouping.
        % \jc{can we make the figure NOT seem to show that naive vs. our AC is so much more dominantly useful than other techniques?} 
        }
        \label{fig:insights}
    \end{figure}


\begin{figure}[t]
\centering
    \includegraphics[width=0.7\columnwidth]{figs/prediction_error.pdf}
    \tightcaption{The prediction errors of \name's controller. Measured with Llama-7B on the Wikitext dataset.}
    \label{fig:cdf_error}
\end{figure}

\mypara{Controller prediction error}
Finally, we zoom in on \name's controller and test whether the controller can predict the TTFT of a compression level with low errors based on history measurements.
Figure~\ref{fig:cdf_error} shows the distribution of \name's prediction error, defined by the difference between the predicted TTFT and the real TTFT, on the contexts in the Wikitext dataset.
Since the TTFT does not depend on the content of the context, the prediction error mostly reflects the statistical noise of loading and processing contexts of the same length.
Empirically, as prediction errors are dominantly smaller than the actual TTFT, \name can almost always pick the right compression level to meet a given TTFT target. 




%\mypara{What's the storage overhead of \name? } 
% \jc{need to add the storage overhead here}






% \mypara{Does the position of the context affect the gains of \name? } In some scenarios, the context is 
% not always at the beginning of the input~\cite{??, ??}.
% For example, some applications may define some templates for the user to fill in, 
% and the context may lie in any position of the input.
% In order to understand how the position of the context affects the gains of \name,
%  we conduct an experiment to evaluate \name on the wikitext dataset with the context being at the end of the input.
% Similar to the case where the context appears in front of the query, 
% we can see that our gain, compared to the \recomp baseline and the quantization baseline, 
% \name still achieves similar reduction in TTFT, as shown in Figure~\ref{fig:}.




%\mypara{How does each insight in \name's encoder contribute to the overall reduction in size? } 
% As shown in \S\ref{sec:??}, we use three insights in \name's context encoder. 
% In order to understand how much does each component in the context-encoder contribute to the overall reduction in size of \kv. 
% In Figure~\ref{fig:insights}, we incrementally add \name's three insights step-by-step. 
% From right to left, the trade-off curves are obtained by adding our AC, compressing deltas and layer-wise quantization, on top of the quantization baseline with naive AC respectively. 
% As we can see, our AC can reduce the size by about 2$times$ compared to naive AC.
% The other two insights reduces the size from baseline quantization and our AC by \fillme and \fillme respectively. 


% \begin{figure}[t]
% \centering
%      \includegraphics[width=.8\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. \jc{some cosmetic changes:
%     (1) change x-axis title to real size (in bits). 
%     (2) change y-axis title to "generation quality (perplexity)", 
%     (3) add a "better" arrow pointing to the bottom left corner, 
%     (4) legend: Original KV feature compression vs. Delta-based compression, 
%     (5) cut the x-axis to remove the blank on the left side}
%     \yh{remove this}} 
%     \label{fig:delta_insight}
% \end{figure}

%Next, we zoom-in on individual components and evaluate the effect of their design choices.

% \mypara{Delta-based compression}
% To validate the advantage of delta-based compression, we pick the contexts in the \fillme dataset and contrast the performance of compressing their original KV features and the delta tensors explained above.
% %compress them with different quantization levels .
% In Figure~\ref{fig:delta_insight}, we vary the quantization levels (explained shortly) and show the spectrum of the tradeoffs between the compressed sizes and the generation quality (measured in perplexity) of the \fillme model on the decompressed context. 
% We can see that compared to compressing the original KV features, \name's delta-based compression has a much more favorable tradeoff.
% \jc{we should say something about other models? otherwise, people may feel it applies only to this model.}

% \begin{figure}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/ac.pdf}
%     \tightcaption{How different groupings of segments in key-value features affect the entropy. \yh{remove this}} 
%     \label{fig:ac}
% \end{figure}

% \mypara{Different grouping in AC}
% To illustrate the effectiveness of grouping feature values by their channels and layers, Figure~\ref{fig:ac} uses the same dataset and model from Figure~\ref{fig:delta_insight} and comparing the AC-encoded sizes when the probability distributions are conditioned on different combinations of channel, layer, and token index.

% \mypara{Benefit of \name's controller}
% \yh{discuss this}


==> backups/eval-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\input{fig-e2e}

\tightsection{Evaluation}


Our evaluation answers the following key questions:
\begin{itemize}
    \item Given a context, how much can \name's KV encoder reduce the bandwidth needed to transfer its KV cache? 
    \item Given a network bandwidth, how much can \name reduce TTFT (including both network and compute delays)? 
    \item How sensitive is \name's performance gain across different models, context lengths, and network bandwidths? 
    \item Does \name have a better tradeoff between LLM performance and TTFT than baselines that reduce TTFT by pruning the contexts or using smaller models?
    
    % \jc{the items blow dont seem high priority?}
    % \item How much runtime memory usage does \name reduce? 
    % \item What's the overhead of \name?
    % \item How much does each of the components of \name contribute to the total improvement? 
%    \item How generalizable is \name's compressor? 
\end{itemize}




% \begin{figure*}[t]
% \centering
%     \includegraphics[width=.92\textwidth]{figs/sensitivity_all.pdf}
%     \vspace{-0.2cm}
%     \tightcaption{Sensitivity of \name's gains over the baseline across different token lengths, network bandwidths, and models.}
%     \label{fig:sensitivity}
% \end{figure*}

\tightsubsection{Setup}


\mypara{Models and testing datasets} 
We evaluate \name on three pipelines, summarized in Table~\ref{tab:eval}, that span models with different sizes and datasets for different tasks.
% Table~\ref{tab:eval} summarizes the setup.
% Specifically, we test \name in three pipelines.
\begin{packeditemize}

\item {\em Pipeline A} tests the Llama-13b model and Llama-7b model~\cite{llama}, both scaled with Neural Tangent Kernel (NTK), on the Wikitext~\cite{wikitext} dataset. 
The task is to predict the probability of the next token in a sequence based on the context consisting of relevant documents that belong to a specific Wiki page.
% based on the criterion of belonging to a specific Wikipedia page.
The Wikitext dataset covers a wide range of topics, with the context length ranging from 1.8K-24K tokens.
% The documents in the dataset 
% % are filtered such that they are reviewed by humans are considered well-written, and 
% cover a wide range of topics.
% Most contexts are around 1.8K-24K tokens. 

\item {\em Pipeline B} tests the LongChat-7b-16k model~\cite{longchat2023} on the LongChat~\cite{longchat2023} dataset, recently released to test LLMs on queries like ``What was the first topic we discussed? '' based on all the previous conversations as the context. 
Most contexts are around 9K-9.6K tokens. 
We chose LongChat-7b-16k since it is one of the best models on this dataset.

\item {\em Pipeline C} tests the T5-large model~\cite{raffel2023exploring} on Natural Question dataset~\cite{47761}, a question-answering dataset developed by Google. 
Following previous work (\eg~\cite{atlas}), it tests the model to answer user queries from a Q \& A dataset with the context from  Wikipedia documents relevant to the queries.
Most contexts are around 8K-12K tokens. 
\end{packeditemize}
It is worth noting that these pipelines represent the two typical apps with long contexts (\S\ref{subsec:apps}): chat apps (Pipeline B) and retrieval-based apps (Pipeline A and C).


\begin{comment}
We evaluate \name on a set of popular models following previous works~\cite{??, ??, ??}. 
For conversational applications, we evaluate LongChat-7b-16k models with the LongChat dataset~\cite{longchat2023}. 
For retrieval-based applications, we evaluate the T5-large model~\cite{t5} on the Natural Questions dataset~\cite{nq}  following previous works~\cite{atlas};
 we also evaluate NTK\_scaled\_LLaMA-7B, on the second variant with the Wikitext~\cite{wikitext} dataset.
We use perplexity~\cite{} as the metric to evaluate those range of models. 

\mypara{Applications} We evaluate \name on two types of applications: 
\begin{itemize}
\item Conversational applications: the context is previous conversational history between the user and LLM. Following previous work~\cite{longchat2023}, the LLM tries to answer the user query ``What was the first topic we discussed? '' based on all the previous conversation. 
\item  Retrieval-based applications: the context is all the relevant documents to the user query. 
We evaluate two variants of this retrieval-based applications: (1) Following previous work~\cite{atlas}, the LLM tries to answer user queries from a Q \& A dataset with support from  Wikipedia documents relevant to the queries; (2) Following previous work~\cite{wikitext}, the LLM predicts the probability of the next token in a sequence based on the content of all relevant documents.
\end{itemize}


\mypara{Metrics} We mainly evaluate \name on two types of metrics: 
\begin{itemize}
    \item Delay metric: We use the Time-to-first-token (TTFT) as the delay metric, as described in \S\ref{sec:??}. This is the delay from knowing the prompt till generating the first token. 
    \item Size of key-value caches: We compare the size of the key-value caches for each scheme (which we explain shortly)
    \item Quality metric: For the LongChat task, we use \fillme as the metric. 
    For the retrieval-based applications, we use  F1 score as the metric to evaluate the question answering task. 
    We use the perplexity score to evaluate the second variant.
    The perplexity is defined as the exponentiated average negative log-likelihood of the next token. 
    The larger the perplexity is, the less likely the model is to generate the right next token.
    The F1 score captures how well the generated answer matches the ground truth answer of the question answering task.
    %  \yh{use two sentences to explain perplexity, F1 score}. 
\end{itemize}
\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



%\begin{table}[]
%\begin{tabular}{cccc}
%\hline
%  & Dataset          & Model(s)                                                                               & Quality metric \\ \hline\hline
%A & LongChat         & longchat-7B-16k                                                                        & Accuracy       \\ \hline
%B & NaturalQuestions & T5-large                                                                               & F1 score       \\ \hline
%C & Wikitext         & \begin{tabular}[c]{@{}c@{}}LLaMA-13B\\ LLaMA-7B\end{tabular} & Perplexity     \\ \hline
%\end{tabular}
%\caption{}
%\label{tab:my-table}
%\end{table}

% \mypara{Generation quality metric}
\mypara{LLM task performance}
We measure generation quality using the standard metric of each dataset.
\begin{packeditemize}

\item {\em Perplexity} is used to evaluate the model's performance on the Wikitext dataset. 
The perplexity is defined as the exponentiated average negative log-likelihood of the next token~\cite{ppl1, ppl2}.
A low perplexity means the model likely generates the right next token.
While perplexity does not equate to text-generation quality, it is widely used as a decent proxy~\cite{adiwardana2020humanlike}.
This metric has been commonly used by prior works to test the impact of pruning or quantizing LLMs on generation performance~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% widely used in previous works in evaluating whether shrinking the model size or quantizing models degrade the generation quality~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% \jc{this metric may not sound intuitive to system reviewers. add some citations and explain why we should care about it?}

\item {\em Accuracy} is used to evaluate the model's output on the LongChat dataset. 
The task predicts the first topic in the conversational history between the user and the LLM. 
The accuracy is defined as the percentage of generated answers that exactly includes the ground-truth topic. % It is defined as the percentage of the generated answer that matches the ground-truth first topic of the conversation.
% \jc{Yuhan, please add some details and explain why it is a good metric}

\item {\em F1 score} is used to evaluate the model's response in the Natural Questions dataset.
It measures the probability that the generated answer matches the ground truth answer of the question-answering task.
\end{packeditemize}





\mypara{Baselines} 
We compare \name with baselines that do not change the contexts or model (\S\ref{subsec:eval:micro} evaluates more baselines). 
\begin{itemize}
% \item \code{torch.save}: 
\item {\em ``Original KV''} uses \texttt{torch.save} to serialize the KV features in GPU memory to a file.
This serves as a reference for the most straightforward implementation. 
% \item {\em ``Default quantization \& AC''} combines the uniform quantization of KV features~\cite{flexgen} with the default arithmetic coding (AC) that uses a global probability distribution for all elements.
% Like \name, this baseline also uses quantization and AC but with a simpler design on each component. 
\item {\em ``Default quantization''} uses the uniform quantization of KV features~\cite{flexgen}. 
\item {\em ``Text context''} fetches the text of the context and feeds it to LLM to compute self-attention. 
It represents the design of minimizing data transmission but at the expense of high computation overhead, especially under long contexts.


    % \item \recomp: This scheme sends the texts of the context and compute the \kv based on the texts before generating the first token. 
    % % \item Model quantization baseline: This scheme quantizes the model weights into less number of bits in order to reduce the memory usage at inference time~\cite{??, ??, ??}. For this scheme, we report the quality metrics after applying the model quantization. 
    % % For the size metrics, we report the size of the key-value caches saved by \code{torch.save}.
    % % \item Original models with shorter contexts: This scheme rewrites the contexts with gisting~\cite{??}, and generates the first token with the compressed contexts. \yh{Say a few sentences about the pretrained gisting models only allow us to test on specific models and datasets}
    % \item \kv quantization + \code{torch.save}: This scheme quantizes the key-value cache, and saves the compressed \kv via \code{torch.save}. 
    % \item \kv quantization + naive AC: This scheme quantizes the key-value cache, and saves the compressed \kv via naive AC (\ie no optimization on the grouping of \kv to improve compression ratio). 
    % % \item Smaller model architectures: This scheme approximates the line of work that uses smaller model architectures to reduce the memory footprint of LLMs~\cite{??, ??}. We compare \name's \kv with smaller models' \kv in terms of our metrics. 
    % \item \name (Ours): The orignal models with compressed \kv with \name's compressor and controller. 
\end{itemize}




\mypara{Hardware settings} We use an NVIDIA A40 GPU server to benchmark our results. 
The server is equipped with 384GB of memory and two Intel(R) Xeon(R) Gold 6130 CPUs with Hyper-threading and Turbo Boost enabled by default.
% The server is equipped with 64 Intel(R) Xeon(R) Gold 6130 CPU cores. 
% \yh{describe our CPU and GPU machines }




% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock2.pdf}
%     \tightcaption{Results on Size of KV cache } 
%     \label{fig:mock2}
% \end{figure*}



% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock1.pdf}
%     \tightcaption{Results on TTFT } 
%     \label{fig:mock1}
% \end{figure*}

\tightsubsection{Overall improvement}
\label{subsec:overall_eval}
\mypara{KV cache size reduction} 
Figure~\ref{fig:overall}a shows the size and task performance trade-offs
of \name's KV encoder and the baselines.
% applying the quantization baselines, with default AC or \code{torch.save}, and \name's context encoder to encode the \kv.
Across the three datasets, \name's KV encoder reduces the KV cache size by $3.7-4.3\times$ compared to the best baseline when achieving similar task performance. 
% \name reduces the size of \kv by 4.3$\times$, 3.9$\times $, 3.7$\times$, and 4$\times$ compared to the strongest baseline (8-bit quantization with naive AC) across the three pipelines respectively. 
In particular, the degradation in task performance is very marginal---the increase of perplexity is within 0.5 (which is negligible~\cite{llmint8,smoothquant}), the drop in F1 score is less than 1\%, and the drop in accuracy is below 4\%. 

While our results only show task performance in numbers, \S\ref{sec:appendix} will present concrete examples that compare the generated texts of \name vs. without KV compression.


% The degradation of generation quality is small, with the perplexity score increasing within 0.5~\footnote{Since perplexity is an exponentially growing metric, an increase of perplexity score within 0.5 is really negligible~\cite{llmint8,smoothquant}.} or an F1 score degradation within 1 point (from 59.2 to 58.7) and accuracy degradation within 4-percentage-points (from 100\% to 96\%), compared to the baseline.
% Compared to the baseline that saves \kv tensors with \code{torch.save}, \name reduces the size of \kv by 3.8-4.5$\times $. 

% Note that baseline with default AC reduces the size of \kv more than \code{torch.save} because it further compresses


\mypara{TTFT reduction} 
Figure~\ref{fig:overall}b shows \name's reduction in TTFT when the bandwidth to transfer the context is set to 2~Gbps (\S\ref{subsec:eval:sensitivity} will vary bandwidth).
It shows that \name reduces TTFT by 2.7-3$\times$ compared to the most competitive baseline. 
\name's gains result from reduced KV cache as well as the ability to choose to load text context when the context is short enough (\eg 20\% of contexts in Pipeline A).
% The ``original KV tensor'' baseline (saved by \texttt{torch.save}) has a bigger size but is sometimes faster than the use of default AC, because of the additional decompression overhead of the \texttt{torchac} library.
% As a side note, quatization baseline with \code{torch.save}, which is the default and optimized deserialization tool in Pytorch~\cite{pytorch}, is a little faster than default AC because AC incurs an additional decompression overhead than \code{torch.save}.  


These reductions in KV cache sizes and TTFT confirm \name's effectiveness on different models and datasets. 
% The next section will show more sensitivity tests. 


% This consistent improvement across these models and pipelines also indicate that \name is generally applicable to different model architectures and sizes. 

% Compared to the \recomp baseline, \name is able to reduce the TTFT because it 
% avoids the computation of the self-attention operation on the long context.

% \yh{Comments a bit on why \name can achieve smaller sizes compared to baselines}

\yhedit{\subsection{Controller evaluation}

Figure~\ref{fig:adapt} and \ref{fig:adapt2} shows how \name's controller adapts to changes of workloads when transmitting KV cache. 

In figure~\ref{fig:adapt} illustrates a timeline of transmitting the KV cache for one piece of context. 
To start with, \name's controller decides to transmit the compressed KV cache for the first \fillme layers. 
At 2 seconds,
the throughput suddenly drops from \fillme to \fillme. 
After the throughput change is being reflected to the transmission server, \name's controller decides to transmit the text context and do the computation to generate the KV for subsequent \fillme layers.
After 4 seconds, the throughput increases again from \fillme to \fillme, and \name's controller decides to switch back to transmit the KV cache for later layers. 
Nevertheless, for the baseline that applies default quantization on the KV cache, it always sends the quantized version of KV cache without any adaptation, which leads to \fillme from 2 seconds to 4 seconds. 

In figure~\ref{fig:adapt2}, we show how \name's controller adapts to different workloads change across time when transmitting different contexts. 
We can see that due to the adaptation made by \name's controller, everytime when the workloads change in the middle of transmitting the context, the adaptation \name made further improves the gain of \name over the baseline. 

}

\begin{figure}[t]
\centering
    \includegraphics[width=.5\textwidth]{figs/adaptation.pdf}
    \vspace{-0.2cm}
    \tightcaption{\todo{Mock fig for now. replace with real!}Adaptation made by \name's controller during the transmission of the KV cache for one context. 
    % When the inference request comes in, \name's controller first decides to transmit cached KV features. After 2 seconds, The bandwidth throughput drops. \name's controller decides to transmit the text context, and compute KV features on the GPU. After 4 seconds, the bandwidth throughput increases again and \name's controller decides to transmit the cached KV again.
    }
    \label{fig:adapt}
\end{figure}


% \begin{figure}[t]
% \centering
%     \includegraphics[width=.5\textwidth]{figs/adaptation2.pdf}
%     \vspace{-0.2cm}
%     \tightcaption{\todo{Mock fig for now. replace with real!}}
%     \label{fig:adapt2}
% \end{figure}

\subsection{Sensitivity analysis}
\label{subsec:eval:sensitivity}

\yhedit{\mypara{Impact of resource allocation}
Figure~\ref{fig:resource} shows the improvement ratio of \name over the baselines when resource allocation (\ie throughput and GPU utilization) for two different context lengths.
For both context lengths, \name has \fillme$\times$ reduction in TTFT across a wide range of throughputs, \fillme - \fillme if the job uses 100\% of the GPU, and \fillme - \fillme when the job uses 20\% of the GPU. 
\name has more gains when the context length is long, as the TTFT of the text context baseline is growing super-linear to the context length. 

% \yh{Say more sentences that when we have improvement }
\input{fig-example} 
}


\begin{figure}[t]
\centering
    \includegraphics[width=.5\textwidth]{figs/fig11.pdf}
    \vspace{-0.2cm}
    \tightcaption{\name's gain varying input token lengths and different LLMs. }
    \label{fig:sensitivity}
\end{figure}

% To study how different network bandwidths or input token lengths affect the performance of \name, we conduct a sensitivity analysis to study the impact of these two factors on the gains of \name compared to the baselines.


\mypara{Impact of context length}
Figure~\ref{fig:sensitivity}a varies the input token length from 0.1K to 10K and shows the TTFT reduction of \name compared to the baselines under a fixed network bandwidth of 2~Gbps.
% As shown in the figure, compared to the \recomp baseline, \name can reduce the TTFT by 2-4$\times$.
The result mirrors the illustration of Figure~\ref{fig:intro}.
Specifically, when the context is long, the gain of \name is mostly from reducing the KV cache sizes.
And when the context is short (below 1K), \name automatically reverts to loading the text context, if it is faster than loading any KV cache.
% We can see that \name's speedup generally increases with longer context lengths.
% This is because when the input token length is small, the time of self-attention is small, making the saving from removing the self-attention delay less significant.


% \mypara{Impact of network bandwidth}
% Figure~\ref{fig:sensitivity}b varies the network bandwidth (0.2 - 10Gbps) and shows \name's TTFT reduction compared to the baselines.
% % As shown in the figure, compared to the \recomp baseline, \name can reduce the TTFT by 2-4.5$\times$.
% We can see that \name consistently outperforms the baselines on different bandwidths. 
% Under a high network bandwidth, \name's reduction of KV cache size results in lower TTFT as less data is transferred.
% Under a low bandwidth, \name again reverts to loading the text context as the delay of sending KV cache always outweighs the saving in computation dalays.
% Particularly, when the network bandwidth is low, 
% sending \kv over the network will not be able to compromise the saving in TTFT by removing the time of self-attention. 
% However, when the network bandwidth is large, the time of sending \kv will become less significant, making the saving from removing the self-attention delay more significant.
% We can see that the gains of \name increase as the network bandwidth increases.

% \mypara{Reduction in runtime memory} 
% A accompanied benefit of caching key and value features, compared to the on-the-fly computation baseline, is that it saves GPU runtime memory usage. 
% This is because by caching the key and value features, the memory heavy self-attention operation based on the long input is avoided. As shown in Figure~\ref{fig:}, \name's GPU memory usage is \fillme smaller than the on-the-fly computation baseline.  
% \yh{Comments a bit on what side benefits it can bring: batching is possible for generating the first token with \name}.

% \mypara{Overhead of \name} The overhead of \name is mainly in two aspects. 
% First, before the inference runtime, \name's compressor needs to run AC on the uncompressed \kv , and store them in the storage server. 
% This includes the overhead of moving the uncompressed \kv from GPU to CPU(which causes \fillme seconds overhead), and then applying torchac's encoder on it, leading to an overhead of 0.8 seconds. 
% Secondly, at inference runtime, \name needs to send the compressed \kv over the network bandwidth link, and then apply torchac's decoder on it before feeding to the LLM for inference. 
% The decoder incurs 0.83 seconds of overhead. 
\mypara{Impact of different models}


Figure~\ref{fig:sensitivity}c tests \name with different LLMs but on the {\em same} dataset (Wikitext). 
It shows that across different models, \name consistently reduces TTFT, while achieving negligible degradation to generation quality compared with the default quantization with AC baseline. 
This shows \name's gain is not sensitive to the corresponding dataset with the model. 
% \fillme \jc{Yuhan :)}
%on each type of the model evaluated in \S\ref{subsec:overall_eval}, all on the Wikitext dataset, in order to study whether \name's improvement is sensitive to the xx.

\begin{figure}[t]
\centering
    \includegraphics[width=0.7\columnwidth]{figs/CDF.pdf}
    \tightcaption{\yhedit{The distribution of compressed ratio of \name compared with the default quantization baseline at the same  quality, plotted with different contexts in the Wikitext dataset.}}
    \label{fig:cdf_context}
\end{figure}

\begin{figure}[t]
\centering
    \includegraphics[width=0.99\columnwidth]{figs/overhead.pdf}
    \tightcaption{The breakdowns of the average online TTFT (left) to load and process a context in Wikitext, offline delays (middle) to compress a context in Wikitext, and the storage overhead (right) to store the KV cache a context Wikitext.}
    \label{fig:overhead}
\end{figure}

\begin{figure*}[t]
\centering
    \includegraphics[width=1.9\columnwidth]{figs/figure_14.pdf}
    \tightcaption{Comparing \name and more intrusive methods, including smaller models, token dropping (left), context selection (middle), and gisting (right).
    % Zoomed in to lower perplexity scores for better illustration. \kt{more spacing between figures}
    }
    \label{fig:intrusive}
\end{figure*}

\mypara{Size reduction by context}
Figure~\ref{fig:cdf_context} shows the distribution of KV cache sizes under \name and the baselines. 
It shows that across all the contexts in the Wikitext dataset, \name reduces the size of KV Cache by 3.6 to 4$\times$ compared to the original KV, and 4.2 to 4.6 comparing with default quantization \& AC. 
This shows \name's gain over that baselines is not sensitive to specific contexts. 

\begin{figure}[t]
\centering
    \includegraphics[width=0.9\columnwidth]{figs/output (1).png}
    \tightcaption{Responses produced by CacheGen improves QoE of Real Users over other pipelines\hc{Yuhan plz replace graph}}
    \label{fig:qoe}
\end{figure}


\begin{figure}[t]
\centering
    \includegraphics[width=0.9\columnwidth]{figs/concurrent.pdf}
    \tightcaption{TTFT of \name and the baselines when there are multiple concurrent requests. }
    \label{fig:concurrent}
\end{figure}



\yhedit{\mypara{Impact of number of concurrent requests} Figure~\ref{fig:concurrent} shows how the TTFT varies when there are $X$ concurrent requests sharing one link and one GPU. 
As we can see in the breakdown of \name, although the transmission delay grows linearly when there are multiple requests sharing one link, the decompression time grows only marginally since the decompression for one request does not saturate the GPU computation. 
The computation delay of processing the prompt also grows marginally as batching $X$ jobs has little increase in delay. 
}

% \fillme \jc{Yuhan :)}

\tightsubsection{Microbenchmarks} 
\label{subsec:eval:micro}

\mypara{Quality of Experience}
We performed an IRB-approved user study to validate the effectiveness of \name. We selected three conversation history from dataset xxx\hc{Yuhan please fill in} used in \S\ref{tab:eval}. For each user, we first present the conversation history with ChatGPT. Then we show the same response but produced by different pipelines by adding different TTFT and let users rate the quality of response. By 270 ratings collected from Amazon MTurk~\cite{mturk}, we show that \name consistently outperforms other pipelines in QoE with shorter TTFT in Fig. \ref{fig:qoe}.

% \mypara{What's the delay breakdown of \name's context-encoder and the baseline? } 
\mypara{Breakdown of online delays}
While having better compression efficiency on KV features, \name does incur (marginally) more overhead than the baselines.
To examine the overheads in delays, Figure~\ref{fig:overhead}a breaks down the TTFTs of \name and the baselines on a context of 8.5K tokens into data transfer, decompression (or \texttt{torch.load}), CPU-GPU data movement, and computation by LLM in GPU. 
We can see that while \name has slightly more non-transmission delays, particularly decompression, it is overwhelmingly compensated by its reduction in transmission. 
This figure confirms our illustration in Figure~\ref{fig:motivate_baselines}.


%The readers may wonder, comparing to the a relatively simple baseline, which applies the same levels of quantization and directly saves the \kv with \code{torch.save}, how much overhead does \name's context-decoder introduce?
%To be more specific, comparing with saving \kv with \code{torch.save} and deserializing with \code{torch.load}, whose deserialization presumably has lower delay, \name's context-decoder has the higher overhead of decompressing the \kv with AC. 
%Also, since \name's context-decoder requires a further operation 
%Figure~\ref{fig:delay_breakdown} shows the delay breakdown of \name's context-decoder and the quantization and \code{torch.save} baseline.
%
%As shown in the figure, the delay of \name's context-decoder is 0.83 seconds, and the delay to send the \kv from CPU to GPU is 0.12 seconds (with layer-wise loading pipelining as discussed in \S\ref{sec:design}).



\mypara{Offline delays and storage overheads}
\label{subsec:eval:storage}
Unlike prior methods that compress each context only once, \name compresses multiple versions (\S\ref{subsec:controller}), and Figure~\ref{fig:overhead}b and \ref{fig:overhead}c evaluate the overheads in delays and storage. 
We can see that despite needing to encode and store multiple bitstream representations, the total, \name still requires less storage than the baselines since each version requires much less space than the baselines.
\name compresses each context almost as fast as the baselines because the additional compression delays are much smaller than computing KV features. 



% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.5\columnwidth]{figs/intrusive2.pdf}
%     \tightcaption{}
%     \label{fig:intrusive2}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.6\columnwidth]{figs/gisting.pdf}
%     \tightcaption{}
%     \label{fig:intrusive3}
% \end{figure}


\mypara{\name vs. more intrusive methods}
So far, all methods we have evaluated, including \name, do not modify the LLM or context.
As a complement, Figure~\ref{fig:intrusive} tests \name against recent methods that {\em change} the context or LLM. 
\begin{packeditemize}
\item {\em Smaller models:} 
Replacing the LLM with {\em smaller models} may speed up the computation.
Figure~\ref{fig:intrusive}a replaces the Llama-7B model with a smaller Llama-3B and applies different quantization levels. 
\item {\em Token selection:}
Figure~\ref{fig:intrusive}b uses \scis as an example of {\em removing tokens} with low self-attention scores from the LLM input~\cite{liu2023scissorhands}. 
Since the self-attention scores are only available during the actual generation, it cannot reduce TTFT, but we make an effort to create an idealized version of \scis (Scissorhands*) by running the self-attention offline to determine which tokens to drop and provide this information to Scissorhands* online.
\item {\em Context selection:}
Another trick used by some retrieval-based apps is to select fewer documents as the context. 
We test this idea on Pipeline C because the dataset already has this optimization.
By default, it picks the top 20 documents as context, and Figure~\ref{fig:intrusive}b tries top-10 and top-4. 
\item {\em Gisting}
Finally, we test Gisting as an example of a more advanced method that shortens contexts into gist tokens and changes the LLM to accept the gist tokens~\cite{gisting}.
\edit{In Figure~\ref{fig:intrusive}c, we test the pre-trained gisting model, which is based on Llama-7B. 
The gisting model retrains the LLM's attention model in order to run inference on a compressed version of the input prompts. 
Since the gisting model can compress arbitrary long contexts into \textit{one token}, we vary the compression ratio of the gisting model to obtain a trade-off in size and accuracy.
This is done by adapting the fraction of input tokens that are compressed into one token.
% changes the LLM attention scheme and fine-tunes Llama-7B\jc{the phrase right before here is awkward, can we just say "retrain the LLM's attention model"?} to run inference on a compressed version of the input prompts. 
% \jc{is it necessary to have the next sentence?}
% The pre-trained gisting model can compress arbitrary long contexts into 1 token.
% We vary the compression ratio of the gisting model by changing the number of tokens compressed in the LLM input.
% The more tokens gisting compress into one token, the less quality it can achieve.\jc{exactly every how many tokens did you compress to 1 gist token? is that not important?}
We apply \name on the original Llama-7B model on the PIQA~\cite{bisk2019piqa} dataset, which is one of the most popular question-answering datasets. 
We did not apply \name on other datasets in our evaluation because the public pre-trained gisting model can only take up to 512 tokens, and truncating the dataset into smaller chunks will not be able to preserve the information in the context. 
}
% Figure~\ref{fig:intrusive}c tests the pre-trained gisting model re-trained on Llama-7B and compare it with \name which uses the original Llama-7B on PIQA~\cite{bisk2019piqa}, one of the most popular Q/A datasets.\footnote{We did not use the Natural Questions dataset (Pipeline C) because the public pre-trained gisting model cannot work with the long contexts in the open-domain version of Natural Questions.}
\end{packeditemize}
We can see that \name outperforms these baselines, reducing TTFT or KV cache size while achieving similar or better LLM's performance on the respective tasks.
In particular, \name is faster than smaller models (which are slowed down by transformer operations), and can reduce KV cache better than context selection or gisting because it compresses the KV features to more compact bitstream representations.
We want to stress that even though \name is compared head-to-head with these methods, it makes no assumption about the context and the model, so one can combine \name with these methods to potentially further improve the performance.

%\mypara{How does \name compare with context reduction baselines? }
% The evaluation till now assumes the context is already been preprocessed and ready to use. 
% However, there are other works~\cite{??, ??} trying to shrink the length of the context so as to reduce the memory footprint of LLMs. 
%  \yh{say that previous evals assumes the context is given. Now we wanna compare with techniques that reduce context length via prompt rewriting or token selection. }

% \begin{figure}
% \centering
% \includegraphics[width=0.33\textwidth]{figs/scissorhands.pdf}
% \caption{Comparison of \name and \scis*. }
% \label{fig:scissorhands}
% \end{figure}


% \scis removes tokens from the LLM input with low self-attention scores. 
% This method has to execute the  \emph{self-attention} operation in order to determine the tokens to be removed. 
% Thus, \scis would not be able to reduce the TTFT. 
% However, we evaluate the idealized version of \scis to see how much it can reduce the size of \kv. 
% By an idealized version, we simply run the self-attention operation and obtain the scores, and remove those tokens whose attention scores are small.  
% Figure~\ref{fig:scissorhands} shows the quality and size trade-off for \name and \scis. 
% \name even achieves better trade-offs than the idealized \scis. 

% Similarly, we apply another context reduction 
% \yh{todo: add gisting's results}



%\mypara{How does \name compare with smaller model architectures? } 
% To alleviate the high computation delay or the memory footprint of LLMs,
% applications may choose to use smaller model architectures~\cite{??, ??}.
% In order to show if using a smaller model can achieve better trade-offs than \name, we evaluate 
% \name's \kv with smaller models' \kv.
% As shown in Figure~\ref{fig:smaller}, the trade-off curve of the smaller model (Llama-3B) is obtained by varying the quantization levels. 
% We can see that \name achieves better trade-offs than smaller models.

% \begin{figure}
% \centering
%         \includegraphics[width=0.4\textwidth]{figs/quantize_model.pdf} 
%         \tightcaption{}
%         \label{fig:quant}
%     \end{figure}



% \todo{Add a section which shows \name is applicable on quantized models, like figure~\ref{fig:quant}. }

% \todo{Add a section to show \name is similarly effective in compressing the size of kv cache for larger models (Llama 65B model)~\ref{fig:larger}}

\mypara{Component-wise analysis}
% As shown in Section \ref{sec:??}, \name's context encoder incorporates three key insights. 
To study the impact of individual components in \name's KV encoder,  Figure~\ref{fig:insights} progressively adds each idea into the baseline of uniform quantization and default AC, starting with the use of delta tensors, and  then our AC that uses probability distribution for each channel-layer combination, and finally layer-wise quantization.
This result underscores the substantial contribution from each idea to the overall reduction of KV cache size. %, with the combined effect being particularly impactful.

% Each curve represents a trade-off obtained by adding our AC, delta compression, and layer-wise quantization atop the quantization baseline employing naive AC.

% Our AC technique alone achieves a remarkable reduction in size, approximately two times more efficient than naive AC. 
% The other two insights further enhance the size reduction. Specifically, they reduce the size in comparison to the baseline quantization and our AC by approximately \fillme and \fillme, respectively.


\begin{figure}
\centering
        \includegraphics[width=0.4\textwidth]{figs/insights.pdf} 
        \tightcaption{\todo{Placeholder figure} Contributions of individual ideas behind KV encoder: change-based encoding, layer-wise quantization, and AC based on channel-layer grouping. 
        % \jc{can we make the figure NOT seem to show that naive vs. our AC is so much more dominantly useful than other techniques?} 
        }
        \label{fig:insights}
    \end{figure}


\begin{figure}[t]
\centering
    \includegraphics[width=0.7\columnwidth]{figs/prediction_error.pdf}
    \tightcaption{The prediction errors of \name's controller. Measured with Llama-7B on the Wikitext dataset.}
    \label{fig:cdf_error}
\end{figure}

\mypara{Controller prediction error}
Finally, we zoom in on \name's controller and test whether the controller can predict the TTFT of a compression level with low errors based on history measurements.
Figure~\ref{fig:cdf_error} shows the distribution of \name's prediction error, defined by the difference between the predicted TTFT and the real TTFT, on the contexts in the Wikitext dataset.
Since the TTFT does not depend on the content of the context, the prediction error mostly reflects the statistical noise of loading and processing contexts of the same length.
Empirically, as prediction errors are dominantly smaller than the actual TTFT, \name can almost always pick the right compression level to meet a given TTFT target. 




%\mypara{What's the storage overhead of \name? } 
% \jc{need to add the storage overhead here}






% \mypara{Does the position of the context affect the gains of \name? } In some scenarios, the context is 
% not always at the beginning of the input~\cite{??, ??}.
% For example, some applications may define some templates for the user to fill in, 
% and the context may lie in any position of the input.
% In order to understand how the position of the context affects the gains of \name,
%  we conduct an experiment to evaluate \name on the wikitext dataset with the context being at the end of the input.
% Similar to the case where the context appears in front of the query, 
% we can see that our gain, compared to the \recomp baseline and the quantization baseline, 
% \name still achieves similar reduction in TTFT, as shown in Figure~\ref{fig:}.




%\mypara{How does each insight in \name's encoder contribute to the overall reduction in size? } 
% As shown in \S\ref{sec:??}, we use three insights in \name's context encoder. 
% In order to understand how much does each component in the context-encoder contribute to the overall reduction in size of \kv. 
% In Figure~\ref{fig:insights}, we incrementally add \name's three insights step-by-step. 
% From right to left, the trade-off curves are obtained by adding our AC, compressing deltas and layer-wise quantization, on top of the quantization baseline with naive AC respectively. 
% As we can see, our AC can reduce the size by about 2$times$ compared to naive AC.
% The other two insights reduces the size from baseline quantization and our AC by \fillme and \fillme respectively. 


% \begin{figure}[t]
% \centering
%      \includegraphics[width=.8\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. \jc{some cosmetic changes:
%     (1) change x-axis title to real size (in bits). 
%     (2) change y-axis title to "generation quality (perplexity)", 
%     (3) add a "better" arrow pointing to the bottom left corner, 
%     (4) legend: Original KV feature compression vs. Delta-based compression, 
%     (5) cut the x-axis to remove the blank on the left side}
%     \yh{remove this}} 
%     \label{fig:delta_insight}
% \end{figure}

%Next, we zoom-in on individual components and evaluate the effect of their design choices.

% \mypara{Delta-based compression}
% To validate the advantage of delta-based compression, we pick the contexts in the \fillme dataset and contrast the performance of compressing their original KV features and the delta tensors explained above.
% %compress them with different quantization levels .
% In Figure~\ref{fig:delta_insight}, we vary the quantization levels (explained shortly) and show the spectrum of the tradeoffs between the compressed sizes and the generation quality (measured in perplexity) of the \fillme model on the decompressed context. 
% We can see that compared to compressing the original KV features, \name's delta-based compression has a much more favorable tradeoff.
% \jc{we should say something about other models? otherwise, people may feel it applies only to this model.}

% \begin{figure}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/ac.pdf}
%     \tightcaption{How different groupings of segments in key-value features affect the entropy. \yh{remove this}} 
%     \label{fig:ac}
% \end{figure}

% \mypara{Different grouping in AC}
% To illustrate the effectiveness of grouping feature values by their channels and layers, Figure~\ref{fig:ac} uses the same dataset and model from Figure~\ref{fig:delta_insight} and comparing the AC-encoded sizes when the probability distributions are conditioned on different combinations of channel, layer, and token index.

% \mypara{Benefit of \name's controller}
% \yh{discuss this}


==> backups/evaluation-v1.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}[t]
\centering
    % \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
    %     \label{fig:multi_choice}
    % }
    % \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-13B model on wikitext dataset)]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/ppl_size_13b.pdf} 
    %     \label{fig:multi_choice}
    % }
    % \subfloat[][Retrieval-based applications (T5-large model on Natural Questions dataset): F1 score and size of KV cache tradeoff]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/ret_size.pdf} 
    %     \label{fig:ppl_size}
    % }
    % \subfloat[][Conversational applications (LongChat-7B model on longchat dataset): Accuracy and TTFT tradeoff]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/conv_size.pdf} 
    %     \label{fig:multi_choice}
    % }


    % \subfloat[][Perplexity and TTFT tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/ppl_ttft.pdf} 
    %     \label{fig:multi_choice}
    % }
    % \subfloat[][Perplexity and TTFT tradeoff (NTK\_scaled\_LLaMA-13B model on wikitext dataset)]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/ppl_ttft_13b.pdf} 
    %     \label{fig:multi_choice}
    % }
    % \subfloat[][Retrieval-based applications (T5-large model on Natural Questions dataset): F1 score and TTFT tradeoff]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/ret_ttft.pdf} 
    %     \label{fig:ppl_size}
    % }
    % \subfloat[][Conversational applications: Accuracy and TTFT tradeoffs (LongChat-7B model on longchat dataset) ]
    % {
    %     \includegraphics[width=0.24\textwidth]{figs/conv_ttft.pdf} 
    %     \label{fig:multi_choice}
    % }
    % \tightcaption{Overall results on three different applications and four models.
    % \jc{(1) can you have ONE legend on top of all figures?
    % (2) increase the line thickness and point size
    % (3) shouldn't our method also have a tradeoff curve with multiple points on it?
    % (4) add a "better" arrow pointing to the top left or the bottom left corner}
    % \yh{Gonna update this figure later. Once i add the tradeoff curve for \name. }
    % }
    \includegraphics[width=0.99\textwidth]{figs/eval.pdf}
    \tightcaption{Overall results on three different pipelines shown in Table~\ref{tab:eval}. \jc{can you split this figure into two rows, one for size reduction, and one for TTFT?}
    }
    \label{fig:overall}
\end{figure*}


\section{Evaluation}


Our evaluation answers the following key questions:
\begin{itemize}
    \item Given a context, how much can \name's KV encoder reduce the KV cache size? 
    \item Given a network bandwidth, how much can \name reduce TTFT (including both network and compute delays)? 
    \item How sensitive is \name's performance gain across different models, context lengths, and network bandwidths? 
    \item Does \name have a better tradeoff between LLM performance and TTFT than baselines that reduce TTFT by pruning the contexts or using smaller models?
    
    % \jc{the items blow dont seem high priority?}
    % \item How much runtime memory usage does \name reduce? 
    % \item What's the overhead of \name?
    % \item How much does each of the components of \name contribute to the total improvement? 
%    \item How generalizable is \name's compressor? 
\end{itemize}

\subsection{Setup}


\mypara{Models and testing datasets} 
We evaluate \name in three pipelines, summarized in Table~\ref{tab:eval}, that span various models with different sizes and datasets for different tasks.
% Table~\ref{tab:eval} summarizes the setup.
% Specifically, we test \name in three pipelines.
\begin{packeditemize}

\item {\em Pipeline A} tests the Llama-13b model and Llama-7b model~\cite{??}, both scaled with Neural Tangent Kernel (NTK), on the Wikitext~\cite{wikitext} dataset. 
The task is to predict the probability of the next token in a sequence based on the context consisting of relevant documents that belong to a specific Wiki page.
% based on the criterion of belonging to a specific Wikipedia page.
The documents in the dataset 
% are filtered such that they are reviewed by humans are considered well-written, and 
cover a wide range of topics.
Most contexts are around 1.8K-24K tokens. 

\item {\em Pipeline B} tests the longchat-7b-16k model~\cite{??} on the LongChat~\cite{longchat2023} dataset, recently released to test LLMs on queries like ``What was the first topic we discussed? '' based on all the previous conversations as the context. 
Most contexts are around 9K-9.6K tokens. 
We chose langchat-7b-16k since it is one of the best models on this dataset.

\item {\em Pipeline C} tests the T5-large model~\cite{??} on Natural Question dataset~\cite{??}, a question-answering dataset developed by Google. 
Following previous work (\eg~\cite{atlas}), it tests the model to answer user queries from a Q \& A dataset with the context from  Wikipedia documents relevant to the queries.
Most contexts are around 8K-12K tokens. 
\end{packeditemize}
It is worth noting that these pipelines represent the two typical apps with long contexts (\S\ref{subsec:apps}): chat apps (Pipeline B) and retrieval-based apps (Pipeline A and C).


\begin{comment}
We evaluate \name on a set of popular models following previous works~\cite{??, ??, ??}. 
For conversational applications, we evaluate LongChat-7b-16k models with the LongChat dataset~\cite{longchat2023}. 
For retrieval-based applications, we evaluate the T5-large model~\cite{t5} on the Natural Questions dataset~\cite{nq}  following previous works~\cite{atlas};
 we also evaluate NTK\_scaled\_LLaMA-7B, on the second variant with the Wikitext~\cite{wikitext} dataset.
We use perplexity~\cite{} as the metric to evaluate those range of models. 

\mypara{Applications} We evaluate \name on two types of applications: 
\begin{itemize}
\item Conversational applications: the context is previous conversational history between the user and LLM. Following previous work~\cite{longchat2023}, the LLM tries to answer the user query ``What was the first topic we discussed? '' based on all the previous conversation. 
\item  Retrieval-based applications: the context is all the relevant documents to the user query. 
We evaluate two variants of this retrieval-based applications: (1) Following previous work~\cite{atlas}, the LLM tries to answer user queries from a Q \& A dataset with support from  Wikipedia documents relevant to the queries; (2) Following previous work~\cite{wikitext}, the LLM predicts the probability of the next token in a sequence based on the content of all relevant documents.
\end{itemize}


\mypara{Metrics} We mainly evaluate \name on two types of metrics: 
\begin{itemize}
    \item Delay metric: We use the Time-to-first-token (TTFT) as the delay metric, as described in \S\ref{sec:??}. This is the delay from knowing the prompt till generating the first token. 
    \item Size of key-value caches: We compare the size of the key-value caches for each scheme (which we explain shortly)
    \item Quality metric: For the LongChat task, we use \fillme as the metric. 
    For the retrieval-based applications, we use  F1 score as the metric to evaluate the question answering task. 
    We use the perplexity score to evaluate the second variant.
    The perplexity is defined as the exponentiated average negative log-likelihood of the next token. 
    The larger the perplexity is, the less likely the model is to generate the right next token.
    The F1 score captures how well the generated answer matches the ground truth answer of the question answering task.
    %  \yh{use two sentences to explain perplexity, F1 score}. 
\end{itemize}
\end{comment}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}



%\begin{table}[]
%\begin{tabular}{cccc}
%\hline
%  & Dataset          & Model(s)                                                                               & Quality metric \\ \hline\hline
%A & LongChat         & longchat-7B-16k                                                                        & Accuracy       \\ \hline
%B & NaturalQuestions & T5-large                                                                               & F1 score       \\ \hline
%C & Wikitext         & \begin{tabular}[c]{@{}c@{}}LLaMA-13B\\ LLaMA-7B\end{tabular} & Perplexity     \\ \hline
%\end{tabular}
%\caption{}
%\label{tab:my-table}
%\end{table}

% \mypara{Generation quality metric}
\mypara{LLM task performance}
We measure generation quality using the standard metric of each dataset.
\begin{packeditemize}

\item {\em Perplexity} is used to evaluate the model's performance on the Wikitext dataset. 
The perplexity is defined as the exponentiated average negative log-likelihood of the next token~\cite{ppl1, ppl2}.
A low perplexity means the model is likely to generate the right next token.
While perplexity does not equate to generation quality, it is widely used as a decent proxy~\cite{https://arxiv.org/abs/2001.09977}.
This metric has been commonly used by prior works to test the impact of pruning or quantizing LLMs on generation performance~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% widely used in previous works in evaluating whether shrinking the model size or quantizing models degrade the generation quality~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% \jc{this metric may not sound intuitive to system reviewers. add some citations and explain why we should care about it?}

\item {\em Accuracy} is used to evaluate the model's output on the LongChat dataset. 
The task predicts the first topic in the conversational history between the user and the LLM. 
The accuracy is defined as the percentage of generated answers that exactly includes the ground-truth topic. % It is defined as the percentage of the generated answer that matches the ground-truth first topic of the conversation.
% \jc{Yuhan, please add some details and explain why it is a good metric}

\item {\em F1 score} is used to evaluate the model's response in the Natural Questions dataset.
It measures the probability that the generated answer matches the ground truth answer of the question-answering task.
\end{packeditemize}





\mypara{Baselines} 
We first compare \name with baselines that do not change the given contexts. 
\begin{itemize}
% \item \code{torch.save}: 
\item {\em Original KV tensor} uses \texttt{torch.save} library to serialize the KV features in GPU memory to a file.
This serves as a reference for the most straightforward implementation. 
\item {\em KV quantization + default AC} combines the uniform quantization of KV features~\cite{flexgen} with the default arithmetic coding (AC) that uses a global probability distribution for all elements.
Like \name, this baseline also uses quantization and AC but with a simpler design on each component. 
\item {\em \recomp} fetches the raw text of the context and feeds it directly to LLM to compute self-attention. 
It represents the design of minimizing data transmission but at the expense of high computation overhead, especially under long contexts.


    % \item \recomp: This scheme sends the texts of the context and compute the \kv based on the texts before generating the first token. 
    % % \item Model quantization baseline: This scheme quantizes the model weights into less number of bits in order to reduce the memory usage at inference time~\cite{??, ??, ??}. For this scheme, we report the quality metrics after applying the model quantization. 
    % % For the size metrics, we report the size of the key-value caches saved by \code{torch.save}.
    % % \item Original models with shorter contexts: This scheme rewrites the contexts with gisting~\cite{??}, and generates the first token with the compressed contexts. \yh{Say a few sentences about the pretrained gisting models only allow us to test on specific models and datasets}
    % \item \kv quantization + \code{torch.save}: This scheme quantizes the key-value cache, and saves the compressed \kv via \code{torch.save}. 
    % \item \kv quantization + naive AC: This scheme quantizes the key-value cache, and saves the compressed \kv via naive AC (\ie no optimization on the grouping of \kv to improve compression ratio). 
    % % \item Smaller model architectures: This scheme approximates the line of work that uses smaller model architectures to reduce the memory footprint of LLMs~\cite{??, ??}. We compare \name's \kv with smaller models' \kv in terms of our metrics. 
    % \item \name (Ours): The orignal models with compressed \kv with \name's compressor and controller. 
\end{itemize}




\mypara{Hardware settings} \yh{describe our CPU and GPU machines }




% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock2.pdf}
%     \tightcaption{Results on Size of KV cache } 
%     \label{fig:mock2}
% \end{figure*}



% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock1.pdf}
%     \tightcaption{Results on TTFT } 
%     \label{fig:mock1}
% \end{figure*}

\subsection{Overall improvement}
\label{subsec:overall_eval}
\mypara{Size reduction of KV cache} 
Figure~\ref{fig:overall}(a, b, c, d) shows the size and task performance trade-offs
of \name's KV encoder and the baselines.
% applying the quantization baselines, with default AC or \code{torch.save}, and \name's context encoder to encode the \kv.
Across the three datasets, \name's KV encoder reduces the KV cache size by $3.7-4.3\times$ compared to the best baseline when achieving similar task performance. 
% \name reduces the size of \kv by 4.3$\times$, 3.9$\times $, 3.7$\times$, and 4$\times$ compared to the strongest baseline (8-bit quantization with naive AC) across the three pipelines respectively. 
In particular, the degradation in task performance is very marginal---the increase of perplexity is within 0.5 (which is negligible~\cite{llmint8,smoothquant}), the drop in F1 score within 1\%, and the drop in accuracy is below 4\%. 

While our results only show task performance in numbers, \S\ref{appendix} will present concrete examples that compare the generated texts of \name vs. without KV compression.


% The degradation of generation quality is small, with the perplexity score increasing within 0.5~\footnote{Since perplexity is an exponentially growing metric, an increase of perplexity score within 0.5 is really negligible~\cite{llmint8,smoothquant}.} or an F1 score degradation within 1 point (from 59.2 to 58.7) and accuracy degradation within 4-percentage-points (from 100\% to 96\%), compared to the baseline.
% Compared to the baseline that saves \kv tensors with \code{torch.save}, \name reduces the size of \kv by 3.8-4.5$\times $. 

% Note that baseline with default AC reduces the size of \kv more than \code{torch.save} because it further compresses


\mypara{Reduction in TTFT} 
We then show \name's reduction in TTFT when the bandwidth to transfer the context is set to 2~Gbps (we will test under varying bandwidth in \S\ref{subsec:eval:sensitivity}).
We can see in Figure~\ref{fig:overall} that \name reduces TTFT by 2.7-3$\times$ compared to the most competitive baseline. 
Note that \name's gains result from reduced KV cache and the ability to choose loading text context when the context is short enough (\eg \fillme\% of contexts in Pipeline A).
The ``original KV tensor'' baseline (saved by \texttt{torch.save}) has a bigger size but is sometimes faster than the use of default AC, because of the additional decompression overhead of the \texttt{torchac} library.
% As a side note, quatization baseline with \code{torch.save}, which is the default and optimized deserialization tool in Pytorch~\cite{pytorch}, is a little faster than default AC because AC incurs an additional decompression overhead than \code{torch.save}.  



\name's overall reduction in KV cache sizes and in TTFT confirms its effectiveness across a range of model sizes and datasets. 
The next section will show more sensitivity tests. 


% This consistent improvement across these models and pipelines also indicate that \name is generally applicable to different model architectures and sizes. 

% Compared to the \recomp baseline, \name is able to reduce the TTFT because it 
% avoids the computation of the self-attention operation on the long context.

% \yh{Comments a bit on why \name can achieve smaller sizes compared to baselines}



\subsection{Sensitivity analysis}
\label{subsec:eval:sensitivity}



% To study how different network bandwidths or input token lengths affect the performance of \name, we conduct a sensitivity analysis to study the impact of these two factors on the gains of \name compared to the baselines.


\begin{figure}
\centering
        \includegraphics[width=0.3\textwidth]{figs/len_sens.pdf} 
        \caption{How does different input token length affect the gains of \name. 
        \jc{why the figure seems to show that the increase of the recomputation baseline is slowing down?}
        \jc{
        (1) Change axis to "\# of tokens in context (K)"
        (2) use consistent coloring with other figures.
        }}
        \label{fig:token_length}
\end{figure}

\mypara{Impact of context length}
Figure~\ref{fig:token_length} varies the input token length from 0.1K to 10K and shows the TTFT reduction of \name compared to the baselines under a fixed network bandwidth of 2Gbps.
% As shown in the figure, compared to the \recomp baseline, \name can reduce the TTFT by 2-4$\times$.
It mirrors the illustration of Figure~\ref{fig:intro}.
Specifically, when the context is long, the gain of \name is mostly from reducing the KV cache sizes, but when the context is short (below 1K), \name automatically reverts to loading the text context, which is faster than loading the KV cache.
% We can see that \name's speedup generally increases with longer context lengths.
% This is because when the input token length is small, the time of self-attention is small, making the saving from removing the self-attention delay less significant.

\begin{figure}
\centering
        \includegraphics[width=0.3\textwidth]{figs/bw_sens.pdf} 
        \caption{How does different network bandwidth affect the gains of \name. \jc{please use consistent coloring with the last fig}}
        \label{fig:bandwidth}
\end{figure}

\mypara{Impact of network bandwidth}
Figure~\ref{fig:bandwidth} varies the network bandwidth from 0.2Gbps to 10Gbps and shows \name's TTFT reduction compared to the baselines.
% As shown in the figure, compared to the \recomp baseline, \name can reduce the TTFT by 2-4.5$\times$.
We can see that \name consistently outperforms the baselines on different bandwidths. 
Under high network bandwidth, \name's reduction of KV cache size results in faster TTFT as less data needs to be transferred.
Under low bandwidth, \name again reverts to loading the text context as the cost of sending KV cache always outweighs the saving in computation dalay.
% Particularly, when the network bandwidth is low, 
% sending \kv over the network will not be able to compromise the saving in TTFT by removing the time of self-attention. 
% However, when the network bandwidth is large, the time of sending \kv will become less significant, making the saving from removing the self-attention delay more significant.
% We can see that the gains of \name increase as the network bandwidth increases.

% \mypara{Reduction in runtime memory} 
% A accompanied benefit of caching key and value features, compared to the on-the-fly computation baseline, is that it saves GPU runtime memory usage. 
% This is because by caching the key and value features, the memory heavy self-attention operation based on the long input is avoided. As shown in Figure~\ref{fig:}, \name's GPU memory usage is \fillme smaller than the on-the-fly computation baseline.  
% \yh{Comments a bit on what side benefits it can bring: batching is possible for generating the first token with \name}.

% \mypara{Overhead of \name} The overhead of \name is mainly in two aspects. 
% First, before the inference runtime, \name's compressor needs to run AC on the uncompressed \kv , and store them in the storage server. 
% This includes the overhead of moving the uncompressed \kv from GPU to CPU(which causes \fillme seconds overhead), and then applying torchac's encoder on it, leading to an overhead of 0.8 seconds. 
% Secondly, at inference runtime, \name needs to send the compressed \kv over the network bandwidth link, and then apply torchac's decoder on it before feeding to the LLM for inference. 
% The decoder incurs 0.83 seconds of overhead. 
\mypara{Impact of different models}
In Figure~\ref{fig:model_sens}, we apply \name on each type of the model evaluated in \S\ref{subsec:overall_eval}, all on the Wikitext dataset, in order to study whether \name's improvement is sensitive to the xx.

\subsection{Microbenchmarks} 
\label{subsec:eval:micro}

\begin{figure}
\centering
        \includegraphics[width=0.4\textwidth]{figs/delay_breakdown.pdf} 
        \tightcaption{Delay breakdown for \name and quantization + torch.save baseline. 
        % \jc{can we also add the recomputation baseline?}
        % \yh{and reverse x and y axis}
        }
        \label{fig:delay_breakdown}
    \end{figure}

% \mypara{What's the delay breakdown of \name's context-encoder and the baseline? } 
\mypara{Online delay breakdown}

\mypara{Storage overhead}


The readers may wonder, comparing to the a relatively simple baseline, which applies the same levels of quantization and directly saves the \kv with \code{torch.save}, how much overhead does \name's context-decoder introduce?
To be more specific, comparing with saving \kv with \code{torch.save} and deserializing with \code{torch.load}, whose deserialization presumably has lower delay, \name's context-decoder has the higher overhead of decompressing the \kv with AC. 
Also, since \name's context-decoder requires a further operation 
Figure~\ref{fig:delay_breakdown} shows the delay breakdown of \name's context-decoder and the quantization and \code{torch.save} baseline.

As shown in the figure, the delay of \name's context-decoder is 0.83 seconds, and the delay to send the \kv from CPU to GPU is 0.12 seconds (with layer-wise loading pipelining as discussed in \S\ref{sec:design}).


\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/delay_budget.pdf} 
    \tightcaption{Left: per-context average storage cost. Right: per-context average  encoding delay.  Both profiled with Llama-7B on the Wikitext dataset.  \jc{can you make this fig and the previous one in the same style?}} 
    \label{fig:delay_budget_overall}
\end{figure}

\mypara{What's the storage overhead of \name? } In order to meet different delay budgets, \name stores multiple versions of compressed \kv, so that \name's controller will be able to select the right one given a delay budget. 
Although this design will incur storage overhead than only storing one version of compressed \kv, the storage overhead will be small because those multiple versions \name stores are all compressed.
Here we evaluate the storage overhead of \name to store multiple versions of compressed \kv.
As shown in Figure~\ref{fig:delay_budget_overall}, \yh{fill in explanation here}.
% \jc{need to add the storage overhead here}

\mypara{\name vs. more intrusive baselines}

\mypara{How does \name compare with context reduction baselines? }The evaluation till now assumes the context is already been preprocessed and ready to use. 
However, there are other works~\cite{??, ??} trying to shrink the length of the context so as to reduce the memory footprint of LLMs. 
 \yh{say that previous evals assumes the context is given. Now we wanna compare with techniques that reduce context length via prompt rewriting or token selection. }

% \begin{figure}
% \centering
% \includegraphics[width=0.33\textwidth]{figs/scissorhands.pdf}
% \caption{Comparison of \name and \scis*. }
% \label{fig:scissorhands}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figs/scissorhands.pdf}
    \caption{Left: comparing \name with context reduction baseline Scissorhands* and a smaller model. }
    \label{fig:scissorhands}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figs/gisting.pdf}
    \caption{Comparing \name and Prompt gisting~\cite{gisting} on the PIQA dataset. }
    \label{fig:gisting}
\end{figure}

\scis removes tokens from the LLM input with low self-attention scores. 
This method has to execute the  \emph{self-attention} operation in order to determine the tokens to be removed. 
Thus, \scis would not be able to reduce the TTFT. 
However, we evaluate the idealized version of \scis to see how much it can reduce the size of \kv. 
By an idealized version, we simply run the self-attention operation and obtain the scores, and remove those tokens whose attention scores are small.  
Figure~\ref{fig:scissorhands} shows the quality and size trade-off for \name and \scis. 
\name even achieves better trade-offs than the idealized \scis. 

Similarly, we apply another context reduction 
\yh{todo: add gisting's results}



\mypara{How does \name compare with smaller model architectures? } To alleviate the high computation delay or the memory footprint of LLMs,
applications may choose to use smaller model architectures~\cite{??, ??}.
In order to show if using a smaller model can achieve better trade-offs than \name, we evaluate 
\name's \kv with smaller models' \kv.
As shown in Figure~\ref{fig:smaller}, the trade-off curve of the smaller model (Llama-3B) is obtained by varying the quantization levels. 
We can see that \name achieves better trade-offs than smaller models.


% \mypara{Does the position of the context affect the gains of \name? } In some scenarios, the context is 
% not always at the beginning of the input~\cite{??, ??}.
% For example, some applications may define some templates for the user to fill in, 
% and the context may lie in any position of the input.
% In order to understand how the position of the context affects the gains of \name,
%  we conduct an experiment to evaluate \name on the wikitext dataset with the context being at the end of the input.
% Similar to the case where the context appears in front of the query, 
% we can see that our gain, compared to the \recomp baseline and the quantization baseline, 
% \name still achieves similar reduction in TTFT, as shown in Figure~\ref{fig:}.



\subsection{Component-wise analysis}

\begin{figure}
\centering
        \includegraphics[width=0.3\textwidth]{figs/insight.pdf} 
        \caption{How does each insight contribute to the overall improvement. \jc{can we make the figure NOT seem to show that naive vs. our AC is so much more dominantly useful than other techniques?} 
        }
        \label{fig:insights}
    \end{figure}

\mypara{How does each insight in \name's encoder contribute to the overall reduction in size? } 
As shown in Section \ref{sec:??}, \name's context encoder incorporates three key insights. 
To study the individual impact of each component within the context encoder on the overall reduction in key-value (\kv) size, we conducted a ablation study.

In Figure~\ref{fig:insights}, we progressively introduce \name's three insights into the encoder, moving from right to left.
Each curve represents a trade-off obtained by adding our AC, delta compression, and layer-wise quantization atop the quantization baseline employing naive AC.

Our AC technique alone achieves a remarkable reduction in size, approximately two times more efficient than naive AC. 
The other two insights further enhance the size reduction. Specifically, they reduce the size in comparison to the baseline quantization and our AC by approximately \fillme and \fillme, respectively.

This analysis underscores the significant contributions of each of \name's insights to the overall reduction in \kv size, with the combined effect being particularly impactful.
% As shown in \S\ref{sec:??}, we use three insights in \name's context encoder. 
% In order to understand how much does each component in the context-encoder contribute to the overall reduction in size of \kv. 
% In Figure~\ref{fig:insights}, we incrementally add \name's three insights step-by-step. 
% From right to left, the trade-off curves are obtained by adding our AC, compressing deltas and layer-wise quantization, on top of the quantization baseline with naive AC respectively. 
% As we can see, our AC can reduce the size by about 2$times$ compared to naive AC.
% The other two insights reduces the size from baseline quantization and our AC by \fillme and \fillme respectively. 


% \begin{figure}[t]
% \centering
%      \includegraphics[width=.8\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. \jc{some cosmetic changes:
%     (1) change x-axis title to real size (in bits). 
%     (2) change y-axis title to "generation quality (perplexity)", 
%     (3) add a "better" arrow pointing to the bottom left corner, 
%     (4) legend: Original KV feature compression vs. Delta-based compression, 
%     (5) cut the x-axis to remove the blank on the left side}
%     \yh{remove this}} 
%     \label{fig:delta_insight}
% \end{figure}

Next, we zoom-in on individual components and evaluate the effect of their design choices.

% \mypara{Delta-based compression}
% To validate the advantage of delta-based compression, we pick the contexts in the \fillme dataset and contrast the performance of compressing their original KV features and the delta tensors explained above.
% %compress them with different quantization levels .
% In Figure~\ref{fig:delta_insight}, we vary the quantization levels (explained shortly) and show the spectrum of the tradeoffs between the compressed sizes and the generation quality (measured in perplexity) of the \fillme model on the decompressed context. 
% We can see that compared to compressing the original KV features, \name's delta-based compression has a much more favorable tradeoff.
% \jc{we should say something about other models? otherwise, people may feel it applies only to this model.}

% \begin{figure}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/ac.pdf}
%     \tightcaption{How different groupings of segments in key-value features affect the entropy. \yh{remove this}} 
%     \label{fig:ac}
% \end{figure}

% \mypara{Different grouping in AC}
% To illustrate the effectiveness of grouping feature values by their channels and layers, Figure~\ref{fig:ac} uses the same dataset and model from Figure~\ref{fig:delta_insight} and comparing the AC-encoded sizes when the probability distributions are conditioned on different combinations of channel, layer, and token index.

% \mypara{Benefit of \name's controller}
% \yh{discuss this}


==> backups/implementation-v1.tex <==
\section{Implementation}
\yh{Quantization, AC what library}
\yh{Pipelining}
\yh{Can insert KV cache for inference: need to say Transformers can take in key values as input}


1. each module's  library  
2. performance optimization 
3. LLM applications integration 

==> backups/intro-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

%Generative AI, in the form of large language models (LLMs), has transformed many internet applications.
With its impressive capabilities gradually recognized by the public, generative AI, in the form of large language models (LLMs), is used in a range of complex tasks, including personal assistant and recommendation, AI healthcare and marketing, to mention a few. 
The availability of the latest LLMs, APIs or frameworks (such as OpenAI GPT-4, LLaMA, and Langchain) to developers further contributes to the growth in LLMs' popularity in the coming years.
\jc{cite some industry reports on the rapid growth of GPT queries or LLM in general}


As LLMs are increasingly deployed for complex tasks, we see a notable trend: the augmentation of LLM inference with extended {\em memory} text.
%a new breed of applications arises that {\em augment LLMs with memory}. 
Traditional language models typically handle ``one-off'' queries or prompts. 
However, when using memory-augmented LLMs, users can issue a sequence of queries, with the response to each query becomes part of the ``memory'' of subsequent queries. 
In the meantime, to produce high-quality responses, LLMs may require large supplementary input. 
For instance, answering a legal inquiry may need access to a database of prior cases.
These supplementary inputs, whether they are conversation histories or additional documents, essentially serve as the LLM's ``memory''.
%Many recent efforts of memory augmented LLMs have been focused on how LLMs can be trained to process long memory (\eg~\cite{??,??,??}). 


However, integrating memory to LLM inference also presents challenges, especially when the memory text is long, dynamic, and fetched remotely. 

\begin{packeditemize}
\item {\em Length:} Techniques such as prompt engineering and in-context learning, which imbue LLMs with new knowledge via a series of prompts, have become popular. 
As a result, conversational histories can easily contain thousands of tokens (words).
Moreover, recent retrieval-based LLMs (\eg~\cite{??,??}), capable of handling memory texts with more than 100K tokens, have demonstrated the ability to produce superior answers when provided with more supplementary documents.

\item {\em Dynamism:} 
Memory text is not static either; it is {\em dynamically} determined. 
Which documents are relevant to a query depends on the current query (prompt). 
Similarly, as a dialogue progresses, its conversational history expands, and sometimes only a subset of it might be pertinent for each query. 
\footnote{This subset could be any part of the dialog history, not necessarily the most recent history, for example, ``write a reminder to X based on the email I sent her a week ago.''}

\item {\em Remote fetching:} 
Last but not least, the memory text often needs to be retrieved from external servers.
As a user travels between locations, her queries might be processed by different GPUs.
Consequently, a user's ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
Similarly, supplementary documents assising LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.

\end{packeditemize}

\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/intro_perf.pdf}
    \tightcaption{} 
    \label{fig:intro}
\end{figure*}


%These memory-augmented LLMs raise new challenges for the underlying LLM serving systems, which serve large DNNs but with a relatively small prompt input, rather than dynamic history. 
Currently, memory-augmented LLMs can be served in two ways, but as depicted in Figure~\ref{fig:intro}(a), neither is ideal for different reasons. 

\begin{packedenumerate}
\item A traditional method is that the LLM takes the memory in the form of tokens or words. 
The LLM needs to process the tokens to {\em keys-values} features first before generating the response.
The advantage of this method is the relative small size of tokenized memory text, so it can be fetched quickly. 
However, the delay to process the memory can increase quadratically with the length of the memory. 

\item Alternatively, one can pre-compute and cache the keys and values, or even self-attention matrices, the of memory text, storing them as intermediate outcomes.
%leverage that the masked attention mechanism in transformers to cache the keys and values (or self-attention matrices) the of memory text as intermediate results. 
This strategy minimizes the processing delay for memory text. 
However, the size of the key and value features are much larger than tokens, so it can take longer to retrieve the key and value features. 
\jc{need some concrete numbers here}

\end{packedenumerate}

As a result, how to fetch memory text efficiently to unlock the full potential of memory-augmented LLMs remains a challenge and will likely be more so in the future. 


%To make it more concrete, we perform a measurement the size of key-value features of two different LLMs under two datasets, each including over \fillme tokens.

This work designs and implements \name, a new memory-retrieval system for LLMs.
\name incorporates three ideas to significantly accelerate the loading of memory text for LLMs.


First, \name shrinks the size of cached key-value features using a new compression algorithm.
The compression algorithm leverages several domain-specific insights, such as \fillme. \jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}

Second, even retrieving the key-value features, the LLM still needs to calculate the attention matrices (self-attention and cross attention) of each layer. 
To expedite the inference process, \name loads key-value features layer by layer in a way that pipelines the transferring of features and computation.

Third, depending on the text input and the hardware specifics, it is sometimes faster to directly processing the memory tokens (text) from scratch when the memory is short, rather than loading the compressed key-value features which involves additional decompression overhead. 
To minimize loading delay of various memory length, \name predicts the delays of both methods and chooses the one with the lowest predicted delay.



To our best knowledge, \name is the first to optimize the communication aspects of memory-augmented LLM inference, and it complements other efforts aimed at augmenting LLMs with longer memory. 

Our evaluation shows that \fillme

\jc{finally, a paragraph on evaluation highlights. we create a benchmark with \fillme. key takeaways are:
\begin{packeditemize}
\item \name can compress the memory \fillme more efficiently than \fillme at the same perplexity
\item \name reduces memory loading delay by \fillme
\item with the same memory-loading delay budget, \name can achieve \fillme better quality (perplexity, accuracy)
\end{packeditemize}
}


%
%The idea of \name is to compress the key-value features of memory first before retrieving them from remote servers, instead of retrieving them in the form of tensors. \hc{Maybe also mention the potential to make llm inference much faster here?}
%
%Though this idea may seem simple, compressing key-value features is by no means trivial. 
%For instance, quantization is commonly used to reduce footprint of tensors in GPU RAM, but it reduces memory size at the cost of greatly increased perplexity (illustrated in Figure~\ref{fig:intro}(b)). 
%Similarly, arithmetic coding, though lossless, does not yield much compression when applied directly on key-value features. 
%Instead, \name embraces several common patterns of key-value features.
%\jc{list the insights here.}
%Moreover, given a delay target, \name can automatically select the right compression configuration to retrieve maximum amount of memory without violating the delay target. 
%\jc{a few words on this}

 







==> backups/intro-v4.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

%Generative AI, in the form of large language models (LLMs), has transformed many internet applications.
With its impressive generative capabilities gradually recognized by the public, large language models (LLMs) are used in a range of complex tasks, including personal assistant and recommendation, AI healthcare and marketing, to mention a few. 
The availability of the latest LLMs, APIs or frameworks (such as OpenAI GPT-4, LLaMA, and Langchain) to developers further contributes to the growth in LLMs' popularity in the coming years.
\jc{cite some industry reports on the rapid growth of GPT queries or LLM in general}


With LLMs being used in more complex tasks, we see a notable trend---the augmentation of LLM's input with extended {\em context}.
%a new breed of applications arises that {\em augment LLMs with memory}. 
While traditionally language models take single standalone prompts  as input, it has changed as LLMs are used in real-world applications. 
For instance, as users constantly interact with LLMs, they accumulate long conversation histories (prompts and responses), and the next prompt may use information from prior interactions.
To provide coherent responses, LLM applications often include many previous prompts and responses as part of the input to the LLM, because the LLM itself keeps no internal state between two inferences.
%users today form longer interactions with LLMs (\eg in-context learning), may refer to any prior interactions in the next prompt, and demand coherent responses.
%Since the LLM keeps no internal state between two inferences, this means that the input of LLM needs to include many or even the entire conversational history of interactions between a user and an LLM, which we refer to as the ``context'' part of the input.
Similarly, in retrieval-based learning, answering a query may require the LLM to first process some supplementary documents extracted from a knowledge base.
%However, when using memory-augmented LLMs, users can issue a sequence of queries, with the response to each query becomes part of the ``memory'' of subsequent queries. 
%In the meantime, to produce high-quality responses, LLMs may require large supplementary input. 
For instance, answering a legal inquiry may need access to a database of prior cases.
These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%Many recent efforts of memory augmented LLMs have been focused on how LLMs can be trained to process long memory (\eg~\cite{??,??,??}). 


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/intro_perf.pdf}
    \tightcaption{} 
    \label{fig:intro}
\end{figure*}

However, integrating context to LLM inference also presents challenges, especially when the context is long and must be fetched remotely. 

\begin{packeditemize}
\item {\em Long context:} 
Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow an LLM  to learn new knowledge by feeding LLM with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).
Moreover, retrieval-based LLMs (\eg~\cite{??,??}), capable of handling memory texts with more than 100K works, have demonstrated the ability to produce superior answers when provided with more supplementary documents.

\begin{comment}
\item {\em Dynamism:} 
The context of an LLM input is present before a prompt is received, but it is not static; rather it can change constantly. 
%Memory text is not static either; it is {\em dynamically}. 
As interactions between a user and an LLM progresses, its conversational history expands, and sometimes only a subset of it might be pertinent for each query.\footnote{This subset could be any part of the dialog history, not necessarily the most recent history, for example, ``write a reminder to X based on the email I sent her a week ago.''}
Similarly, depending on the next query, the supplementary documents extracted as the context will differ.
\end{comment}

\item {\em Remote fetching:} 
Last but not least, the context of an input often needs to be retrieved from an external server.
For instance, as a user travels between locations, her queries might be processed by different GPUs, so her conversation history cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.

\end{packeditemize}



%These memory-augmented LLMs raise new challenges for the underlying LLM serving systems, which serve large DNNs but with a relatively small prompt input, rather than dynamic history. 
Currently, long context can be handled in two ways, but as depicted in Figure~\ref{fig:intro}(a), neither is ideal for different reasons. 

\begin{packedenumerate}
\item Traditionally, LLM takes the context of a prompt in the form of raw text.
The LLM needs to process the words to {\em keys-value} features as intermediate results first before generating the response.
The advantage of this method is the relative small size of context text, so it can be fetched quickly. 
However, the delay to process context can increase quadratically with the length of the context. 

\item Alternatively, one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
This is because the context is often from a knowledge base known in advance or from prior interactions of a user whose key-value features are already computed.
%one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
%leverage that the masked attention mechanism in transformers to cache the keys and values (or self-attention matrices) the of memory text as intermediate results. 
This strategy minimizes the processing delay for context. 
However, the size of the key and value features are much larger than text, so it can take longer to retrieve the key and value features. 
\jc{need some concrete numbers here}

\end{packedenumerate}

As a result, how to fetch context efficiently to unlock the full potential of LLMs remains a challenge and will likely be more so in the future. 


%To make it more concrete, we perform a measurement the size of key-value features of two different LLMs under two datasets, each including over \fillme tokens.

This work designs and implements \name, an efficient context-loading system for LLMs, which entails three ideas. % to significantly accelerate the loading of memory text for LLMs.


First, \name shrinks the size of cached key-value features using a new compression algorithm.
The compression algorithm leverages several domain-specific insights, such as \fillme. \jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}

Second, even retrieving the key-value features, the LLM still needs to calculate the attention matrices (self-attention and cross attention) of each layer. 
To expedite the inference process, \name loads key-value features layer by layer in a way that pipelines the transferring of features and computation.

Third, depending on the text input and the hardware specifics, it is sometimes faster to directly processing the context text from scratch when the context is short, rather than loading the compressed key-value features which involves additional decompression overhead. 
To minimize loading delay of various context length, \name predicts the delays of both methods and chooses the one with the lowest predicted delay.



To our best knowledge, \name is the first to optimize the communication aspects of LLM with long context, and it complements other efforts aimed at augmenting LLMs with longer context. 

Our evaluation shows that \fillme

\jc{finally, a paragraph on evaluation highlights. we create a benchmark with \fillme. key takeaways are:
\begin{packeditemize}
\item \name can compress the memory \fillme more efficiently than \fillme at the same perplexity
\item \name reduces memory loading delay by \fillme
\item with the same memory-loading delay budget, \name can achieve \fillme better quality (perplexity, accuracy)
\end{packeditemize}
}


%
%The idea of \name is to compress the key-value features of memory first before retrieving them from remote servers, instead of retrieving them in the form of tensors. \hc{Maybe also mention the potential to make llm inference much faster here?}
%
%Though this idea may seem simple, compressing key-value features is by no means trivial. 
%For instance, quantization is commonly used to reduce footprint of tensors in GPU RAM, but it reduces memory size at the cost of greatly increased perplexity (illustrated in Figure~\ref{fig:intro}(b)). 
%Similarly, arithmetic coding, though lossless, does not yield much compression when applied directly on key-value features. 
%Instead, \name embraces several common patterns of key-value features.
%\jc{list the insights here.}
%Moreover, given a delay target, \name can automatically select the right compression configuration to retrieve maximum amount of memory without violating the delay target. 
%\jc{a few words on this}

 







==> backups/intro-v5.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

%Generative AI, in the form of large language models (LLMs), has transformed many internet applications.
With its impressive generative capabilities gradually recognized by the public, large language models (LLMs) are used in a wide range of tasks, including personal assistant and recommendation, AI healthcare and marketing, to mention a few. 
The availability of the latest LLMs, APIs or frameworks (such as OpenAI GPT-4, LLaMA, and Langchain) to developers further contributes to the growth in LLMs' popularity in the coming years.
\jc{cite some industry reports on the rapid growth of GPT queries or LLM in general}


As LLMs take on increasingly complex tasks, we see a notable trend---the augmentation of LLM's input with {\em long contexts}.
%a new breed of applications arises that {\em augment LLMs with memory}. 
Traditionally, language models take standalone prompts as input and use only the information embedded in the model to generate responses. 
Today, however, users often query LLMs with questions that require domain knowledge not seen by the LLM before, so applications often supplement these quries with documents retrieved from a knowledge base that encompasses useful domain information.
For instance, to answer a legal inquiry, the LLM input may include documents retrieved from a database of prior cases.
The literature on retrieval-based learning (\eg~\cite{??,??}) also shows that LLMs produce superior answers when provided with longer context. 
%Recently, retrieval-based learning (\eg~\cite{??,??}) enables LLMs to process contexts with over hundreds of thousands of tokens (or words) and shows they produce superior answers when provided with longer context. 


More interactions between users and LLMs also increase context length. 
As users constantly interact with LLMs, they accumulate longer conversation histories, and the LLM needs to information from prior prompts and responses to enhance generation quality and coherence (\eg ``write a reminder to X based on the email to her which was generated a week ago'').
% the next prompt may use information from any prior interactions.
Long context in conversation histories are also common in long-context learning and few-shot learning, where LLMs learn new knowledge or to behavior in certain way by first processing a series of prompts, whose length can easily be over thousands of words.
%, and these prompts and responses become the ``context'' of the LLM's next input. 
For instance, \jc{TODO: add an example here}
Because the LLM itself keeps no internal states, LLM applications must store the conversation history and include a part or the whole of it to the LLM as the context of a prompt.

%Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow LLMs  to learn new knowledge by feeding them with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).


\begin{comment}
in retrieval-based learning, to answer a user query, applications often supplement the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 

These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%it has changed as LLMs are used in real-world applications. 
However, as users constantly interact with LLMs, they accumulate long conversation histories (prompts and responses), and the next prompt may use information from prior interactions.
Because the LLM itself keeps no internal state between two inferences, to provide coherent responses, LLM applications often include many previous prompts and responses as part of the input to the LLM.
%users today form longer interactions with LLMs (\eg in-context learning), may refer to any prior interactions in the next prompt, and demand coherent responses.
%Since the LLM keeps no internal state between two inferences, this means that the input of LLM needs to include many or even the entire conversational history of interactions between a user and an LLM, which we refer to as the ``context'' part of the input.
Similarly, in retrieval-based learning, to answer a user query, an application often supplements the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 
For instance, answering a legal inquiry may need access to a database of prior cases.
These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
\end{comment}

%the LLM to first process some supplementary documents extracted from a knowledge base.
%%However, when using memory-augmented LLMs, users can issue a sequence of queries, with the response to each query becomes part of the ``memory'' of subsequent queries. 
%%In the meantime, to produce high-quality responses, LLMs may require large supplementary input. 
%For instance, answering a legal inquiry may need access to a database of prior cases.
%These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%Many recent efforts of memory augmented LLMs have been focused on how LLMs can be trained to process long memory (\eg~\cite{??,??,??}). 


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/intro_perf.pdf}
    \tightcaption{} 
    \label{fig:intro}
\end{figure*}

Keeping long contexts in GPU memory is not always feasible, as they sometimes are {\em dynamically loaded and processed}, between receiving a query and starting to generate the response. 
For instance, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
Similarly, as the prompts from a user may spread in both time (across a long time) and space (from different locations), they might be processed by different machines, so the conversation history will be loaded on-demand over the network.
%Even if the same GPU serves all prompts of a user, it may be shared with many other users and cannot keep each user's context indefinitely in GPU.

%If we naively feed the long context directly to the LLM, the latency of processing a context in transformer models will grow quadratically with the context length. 
%While we can reduce the context length by sampling only the most relevant part, but doing so often degrade generation quality~\cite{??,??}.
%%it would take too much time to process them before the actual generation starts. 


It might be tempting to tackle long context by caching intermediate outcome, namely key-value (KV) features, of contexts (\eg~\cite{??,??,??}).
Compared to directly processing the context whose delay grows quadratically with the context length, a KV cache speeds up the inference. 
However, KV features need significantly more space to store and more network bandwidth to fetch remotely.
\jc{TODO: need some concrete numbers here.}
If we quantize the KV features or filter most relevant tokens, the size can be reduced but at a great expense of generation quality.
%An alternative approach is to filter the context and only feed LLM with the most relevant text (\eg~\cite{??,??,??}), but it always degrade generation quality.

In general, many previous efforts have focused on speeding up inference (\eg caching KV features or shrinking model sizes) and enabling long-context inference without exceeding the GPU memory limit. 
However, they do not directly optimize the size of KV cache of long contexts and the delay to load and process long context when it is not in GPU memory. 

%In short, existing solutions are remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(2) reduce the context length by sampling only the most relevant part.
%
%
%
%Instead, many LLM systems cache the intermediate processed outcome---{\em key-value features}---of contexts.


%To avoid high inference delay, current LLM systems employ two methods.
%First, they cache the intermediate processed outcome, \ie key-value features, of contexts.
%Compared to directly loading context, this significantly speeds up the inference but it needs much more space to store and much more bandwidth to fetch.
%Alternatively, some works sample contexts and only include the most relevant text in LLM input, but they have to degrade generation quality to reduce the context length.
%As a result, it remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(1) cache the key-value features of contexts, and 
%(2) sample contexts and only include the most relevant text in LLM input.
%Compared to loading context as text, the former needs significantly more space to store and more bandwidth to fetch, whereas the latter has to degrade generation quality to reduce the context length.

%how to fetch context efficiently to unlock the full potential of LLMs remains a challenge and will likely be more so in the future. 




% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
%Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
%Last but not least, 


\begin{comment}

However, integrating context to LLM inference also presents challenges, especially when the context is long and must be fetched remotely. 

\begin{packeditemize}
\item {\em Long context:} 
Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow an LLM  to learn new knowledge by feeding LLM with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).
Moreover, retrieval-based LLMs (\eg~\cite{??,??}), capable of handling memory texts with more than 100K works, have demonstrated the ability to produce superior answers when provided with more supplementary documents.

\item {\em Dynamism:} 
The context of an LLM input is present before a prompt is received, but it is not static; rather it can change constantly. 
%Memory text is not static either; it is {\em dynamically}. 
As interactions between a user and an LLM progresses, its conversational history expands, and sometimes only a subset of it might be pertinent for each query.\footnote{This subset could be any part of the dialog history, not necessarily the most recent history, for example, ``write a reminder to X based on the email I sent her a week ago.''}
Similarly, depending on the next query, the supplementary documents extracted as the context will differ.


\item {\em Remote fetching:} 
Last but not least, the context of an input often needs to be retrieved from an external server.
For instance, as a user travels between locations, her queries might be processed by different GPUs, so her conversation history cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.

\end{packeditemize}


%These memory-augmented LLMs raise new challenges for the underlying LLM serving systems, which serve large DNNs but with a relatively small prompt input, rather than dynamic history. 
Currently, long context can be handled in two ways, but as depicted in Figure~\ref{fig:intro}(a), neither is ideal for different reasons. 

\begin{packedenumerate}
\item Traditionally, LLM takes the context of a prompt in the form of raw text.
The LLM needs to process the words to {\em keys-value} features as intermediate results first before generating the response.
The advantage of this method is the relative small size of context text, so it can be fetched quickly. 
However, the delay to process context can increase quadratically with the length of the context. 

\item Alternatively, one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
This is because the context is often from a knowledge base known in advance or from prior interactions of a user whose key-value features are already computed.
%one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
%leverage that the masked attention mechanism in transformers to cache the keys and values (or self-attention matrices) the of memory text as intermediate results. 
This strategy minimizes the processing delay for context. 
However, the size of the key and value features are much larger than text, so it can take longer to retrieve the key and value features. 
\jc{need some concrete numbers here}

\end{packedenumerate}

\end{comment}



%To make it more concrete, we perform a measurement the size of key-value features of two different LLMs under two datasets, each including over \fillme tokens.

To bridge this gap, this work presents \name, an efficient context-loading system for LLMs, which entails three techniques to reduce the size and processing delay of context with only marginal quality degradation. % to significantly accelerate the loading of memory text for LLMs.


First, \name shrinks the size of cached key-value features using a new compression algorithm.
The compression algorithm leverages several domain-specific insights, such as \fillme. \jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}

Second, even retrieving the key-value features, the LLM still needs to calculate the attention matrices (self-attention and cross attention) of each LLM layer. 
To expedite this process, \name fetch cached key-value features in a layer-by-layer fashion, so that the transferring of features and computation of attention matrices can be pipelined.

Third, since loading compressed key-value features involves additional cost, including decompression and loading more data to GPU memory, directly loading the context tokens might sometimes be faster when the context is short. 
Therefore, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens based on estimated delay of each method. 

%to minimize loading and processing delay under various context length, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens, which might be much faster with short context, depending on the hardware of the GPU machine. 

%depending on the text input and the inference speed, it is sometimes faster to directly load and process the tokens of context, rather than loading the compressed key-value features which involves additional decompression overhead. 




%To our best knowledge, \name is the first to optimize the communication aspects of LLM with long context, and it complements other efforts aimed at augmenting LLMs with longer context. 
Our evaluation shows that \fillme

\jc{finally, a paragraph on evaluation highlights. we create a benchmark with \fillme. key takeaways are:
\begin{packeditemize}
\item \name can compress the memory \fillme more efficiently than \fillme at the same perplexity
\item \name reduces memory loading delay by \fillme
\item with the same memory-loading delay budget, \name can achieve \fillme better quality (perplexity, accuracy)
\end{packeditemize}
}


%
%The idea of \name is to compress the key-value features of memory first before retrieving them from remote servers, instead of retrieving them in the form of tensors. \hc{Maybe also mention the potential to make llm inference much faster here?}
%
%Though this idea may seem simple, compressing key-value features is by no means trivial. 
%For instance, quantization is commonly used to reduce footprint of tensors in GPU RAM, but it reduces memory size at the cost of greatly increased perplexity (illustrated in Figure~\ref{fig:intro}(b)). 
%Similarly, arithmetic coding, though lossless, does not yield much compression when applied directly on key-value features. 
%Instead, \name embraces several common patterns of key-value features.
%\jc{list the insights here.}
%Moreover, given a delay target, \name can automatically select the right compression configuration to retrieve maximum amount of memory without violating the delay target. 
%\jc{a few words on this}

 







==> backups/intro-v6.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

%Generative AI, in the form of large language models (LLMs), has transformed many internet applications.
With its impressive generative capabilities gradually recognized by the public, large language models (LLMs) are used in a wide range of tasks, including personal assistant and recommendation, AI healthcare and marketing, to mention a few. 
The widespread use of LLM APIs (\eg GPT-4~\cite{??}) and application frameworks (\eg Langchain~\cite{??}), combined with the open-source of industry-quality LLMs (\eg LLaMA~\cite{??}), further boosts LLMs' popularity in the coming years.
%The availability of the LLMs, APIs or frameworks (such as OpenAI GPT-4, LLaMA, and Langchain) to developers further contributes to the growth in LLMs' popularity in the coming years.
\jc{cite some industry reports on the rapid growth of GPT queries or LLM in general}


As LLMs take on increasingly complex tasks, we see a notable trend which has profound implications on the underlying LLM serving systems---the augmentation of LLM's input with {\em long contexts}.
%a new breed of applications arises that {\em augment LLMs with memory}. 
Traditionally, language models take standalone prompts as input and use only the information embedded in the model to generate responses. 
Today, however, users often query LLMs with questions that require domain knowledge not seen by the LLM before, so applications often supplement these queries with documents retrieved from a knowledge base that encompasses useful domain information.
For instance, to answer a legal inquiry, the LLM input may include documents retrieved from a database of prior cases.
Retrieval-based LLMs (\eg~\cite{??,??}) also show superior generation quality when provided with longer context. 
%Recently, retrieval-based learning (\eg~\cite{??,??}) enables LLMs to process contexts with over hundreds of thousands of tokens (or words) and shows they produce superior answers when provided with longer context. 


More interactions between users and LLMs also increase context length. 
As users accumulate longer conversation histories with LLM services, and LLMs need information from prior prompts and responses to ensure generation quality and coherence (\eg ``write a reminder to X based on the email to her which was generated a week ago'').
% the next prompt may use information from any prior interactions.
Long context in conversation histories are also common in long-context learning and few-shot learning, where LLMs learn new knowledge or to behavior in certain way by first processing a series of prompts, whose length can easily be over thousands of words.
%, and these prompts and responses become the ``context'' of the LLM's next input. 
For instance, \jc{TODO: add an example here}
Because the LLM itself keeps no internal states, LLM applications must store the conversation history and include a part or the whole of it to the LLM as the context of a prompt.

%Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow LLMs  to learn new knowledge by feeding them with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).


\begin{comment}
in retrieval-based learning, to answer a user query, applications often supplement the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 

These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%it has changed as LLMs are used in real-world applications. 
However, as users constantly interact with LLMs, they accumulate long conversation histories (prompts and responses), and the next prompt may use information from prior interactions.
Because the LLM itself keeps no internal state between two inferences, to provide coherent responses, LLM applications often include many previous prompts and responses as part of the input to the LLM.
%users today form longer interactions with LLMs (\eg in-context learning), may refer to any prior interactions in the next prompt, and demand coherent responses.
%Since the LLM keeps no internal state between two inferences, this means that the input of LLM needs to include many or even the entire conversational history of interactions between a user and an LLM, which we refer to as the ``context'' part of the input.
Similarly, in retrieval-based learning, to answer a user query, an application often supplements the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 
For instance, answering a legal inquiry may need access to a database of prior cases.
These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
\end{comment}

%the LLM to first process some supplementary documents extracted from a knowledge base.
%%However, when using memory-augmented LLMs, users can issue a sequence of queries, with the response to each query becomes part of the ``memory'' of subsequent queries. 
%%In the meantime, to produce high-quality responses, LLMs may require large supplementary input. 
%For instance, answering a legal inquiry may need access to a database of prior cases.
%These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%Many recent efforts of memory augmented LLMs have been focused on how LLMs can be trained to process long memory (\eg~\cite{??,??,??}). 


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/intro_perf.pdf}
    \tightcaption{} 
    \label{fig:intro}
\end{figure*}



To process long context, a common approach is by caching intermediate outcome, namely key-value (KV) features, of contexts (\eg~\cite{??,??,??}).
Compared to directly processing the context whose delay grows quadratically with the context length, a KV cache speeds up the inference. 
However, KV features of long context can be large in size. \jc{some concrete numbers here}

While the size of KV features is not a serious issue when KV features are kept in GPU memory or on the same machine, unfortunately, long contexts sometimes have to be {\em dynamically loaded and processed}.
%it is not always feasible to keep KV features in GPU memory, as the contexts are sometimes {\em dynamically loaded and processed}.
%Unfortunately, keeping the KV features in the GPU memory is not always feasible, as the contexts are sometimes {\em dynamically loaded and processed}.
%between receiving a query and starting to generate the response. 
For instance, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
Similarly, as the prompts from a user may spread in both time (across a long time) and space (from different locations), they might be processed by different machines, so the conversation history will be loaded on-demand over the network.
As a result, if we cache KV features, it may need too much space to store and too much bandwidth to fetch dynamically. 
\jc{TODO: need some concrete numbers here.}
If we quantize the KV features or filter most relevant tokens, the size can be reduced but at a great expense of generation quality.

%However, KV features need significantly more space to store and more network bandwidth to fetch remotely.
%\jc{TODO: need some concrete numbers here.}
%If we quantize the KV features or filter most relevant tokens, the size can be reduced but at a great expense of generation quality.
%An alternative approach is to filter the context and only feed LLM with the most relevant text (\eg~\cite{??,??,??}), but it always degrade generation quality.

%Even if the same GPU serves all prompts of a user, it may be shared with many other users and cannot keep each user's context indefinitely in GPU.

%If we naively feed the long context directly to the LLM, the latency of processing a context in transformer models will grow quadratically with the context length. 
%While we can reduce the context length by sampling only the most relevant part, but doing so often degrade generation quality~\cite{??,??}.
%%it would take too much time to process them before the actual generation starts. 




In general, many previous efforts have focused on speeding up inference (\eg caching KV features or shrinking model sizes) and enabling long-context inference without exceeding the GPU memory limit. 
However, they do not directly optimize the size of KV cache of long contexts and the delay to load and process long context when it is not in GPU memory. 

%In short, existing solutions are remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(2) reduce the context length by sampling only the most relevant part.
%
%
%
%Instead, many LLM systems cache the intermediate processed outcome---{\em key-value features}---of contexts.


%To avoid high inference delay, current LLM systems employ two methods.
%First, they cache the intermediate processed outcome, \ie key-value features, of contexts.
%Compared to directly loading context, this significantly speeds up the inference but it needs much more space to store and much more bandwidth to fetch.
%Alternatively, some works sample contexts and only include the most relevant text in LLM input, but they have to degrade generation quality to reduce the context length.
%As a result, it remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(1) cache the key-value features of contexts, and 
%(2) sample contexts and only include the most relevant text in LLM input.
%Compared to loading context as text, the former needs significantly more space to store and more bandwidth to fetch, whereas the latter has to degrade generation quality to reduce the context length.

%how to fetch context efficiently to unlock the full potential of LLMs remains a challenge and will likely be more so in the future. 




% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
%Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
%Last but not least, 


\begin{comment}

However, integrating context to LLM inference also presents challenges, especially when the context is long and must be fetched remotely. 

\begin{packeditemize}
\item {\em Long context:} 
Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow an LLM  to learn new knowledge by feeding LLM with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).
Moreover, retrieval-based LLMs (\eg~\cite{??,??}), capable of handling memory texts with more than 100K works, have demonstrated the ability to produce superior answers when provided with more supplementary documents.

\item {\em Dynamism:} 
The context of an LLM input is present before a prompt is received, but it is not static; rather it can change constantly. 
%Memory text is not static either; it is {\em dynamically}. 
As interactions between a user and an LLM progresses, its conversational history expands, and sometimes only a subset of it might be pertinent for each query.\footnote{This subset could be any part of the dialog history, not necessarily the most recent history, for example, ``write a reminder to X based on the email I sent her a week ago.''}
Similarly, depending on the next query, the supplementary documents extracted as the context will differ.


\item {\em Remote fetching:} 
Last but not least, the context of an input often needs to be retrieved from an external server.
For instance, as a user travels between locations, her queries might be processed by different GPUs, so her conversation history cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.

\end{packeditemize}


%These memory-augmented LLMs raise new challenges for the underlying LLM serving systems, which serve large DNNs but with a relatively small prompt input, rather than dynamic history. 
Currently, long context can be handled in two ways, but as depicted in Figure~\ref{fig:intro}(a), neither is ideal for different reasons. 

\begin{packedenumerate}
\item Traditionally, LLM takes the context of a prompt in the form of raw text.
The LLM needs to process the words to {\em keys-value} features as intermediate results first before generating the response.
The advantage of this method is the relative small size of context text, so it can be fetched quickly. 
However, the delay to process context can increase quadratically with the length of the context. 

\item Alternatively, one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
This is because the context is often from a knowledge base known in advance or from prior interactions of a user whose key-value features are already computed.
%one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
%leverage that the masked attention mechanism in transformers to cache the keys and values (or self-attention matrices) the of memory text as intermediate results. 
This strategy minimizes the processing delay for context. 
However, the size of the key and value features are much larger than text, so it can take longer to retrieve the key and value features. 
\jc{need some concrete numbers here}

\end{packedenumerate}

\end{comment}



%To make it more concrete, we perform a measurement the size of key-value features of two different LLMs under two datasets, each including over \fillme tokens.

To bridge this gap, this work presents \name, an efficient context-loading system for LLMs, which entails three techniques to reduce the size and processing delay of context with only marginal quality degradation. % to significantly accelerate the loading of memory text for LLMs.


First, \name shrinks the size of cached key-value features using a new compression algorithm.
The compression algorithm leverages several domain-specific insights, such as \fillme. \jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}

Second, even retrieving the key-value features, the LLM still needs to calculate the attention matrices (self-attention and cross attention) of each LLM layer. 
To expedite this process, \name fetch cached key-value features in a layer-by-layer fashion, so that the transferring of features and computation of attention matrices can be pipelined.

Third, since loading compressed key-value features involves additional cost, including decompression and loading more data to GPU memory, directly loading the context tokens might sometimes be faster when the context is short. 
Therefore, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens based on estimated delay of each method. 

%to minimize loading and processing delay under various context length, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens, which might be much faster with short context, depending on the hardware of the GPU machine. 

%depending on the text input and the inference speed, it is sometimes faster to directly load and process the tokens of context, rather than loading the compressed key-value features which involves additional decompression overhead. 




%To our best knowledge, \name is the first to optimize the communication aspects of LLM with long context, and it complements other efforts aimed at augmenting LLMs with longer context. 
Our evaluation shows that \fillme

\jc{finally, a paragraph on evaluation highlights. we create a benchmark with \fillme. key takeaways are:
\begin{packeditemize}
\item \name can compress the memory \fillme more efficiently than \fillme at the same perplexity
\item \name reduces memory loading delay by \fillme
\item with the same memory-loading delay budget, \name can achieve \fillme better quality (perplexity, accuracy)
\end{packeditemize}
}


%
%The idea of \name is to compress the key-value features of memory first before retrieving them from remote servers, instead of retrieving them in the form of tensors. \hc{Maybe also mention the potential to make llm inference much faster here?}
%
%Though this idea may seem simple, compressing key-value features is by no means trivial. 
%For instance, quantization is commonly used to reduce footprint of tensors in GPU RAM, but it reduces memory size at the cost of greatly increased perplexity (illustrated in Figure~\ref{fig:intro}(b)). 
%Similarly, arithmetic coding, though lossless, does not yield much compression when applied directly on key-value features. 
%Instead, \name embraces several common patterns of key-value features.
%\jc{list the insights here.}
%Moreover, given a delay target, \name can automatically select the right compression configuration to retrieve maximum amount of memory without violating the delay target. 
%\jc{a few words on this}

 







==> backups/intro-v7.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

%Generative AI, in the form of large language models (LLMs), has transformed many internet applications.
With its impressive generative capabilities gradually recognized by the public, large language models (LLMs) are used in many tasks, including personal assistant and recommendation, AI healthcare and marketing, to mention a few. 
The widespread use of LLM APIs (\eg GPT-4~\cite{??}) and application frameworks (\eg Langchain~\cite{??}), combined with the open-source of industry-quality LLMs (\eg LLaMA~\cite{??}), further boosts LLMs' popularity in the coming years.
%The availability of the LLMs, APIs or frameworks (such as OpenAI GPT-4, LLaMA, and Langchain) to developers further contributes to the growth in LLMs' popularity in the coming years.
\jc{cite some industry reports on the rapid growth of GPT queries or LLM in general}

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_long_input.pdf}
    \tightcaption{The input length accepted by LLMs has increased significantly in the last year.} 
    \label{fig:motivate_long_input}
\end{figure}

With LLMs used in more applications, we see a notable trend---the augmentation of LLM's input with {\em long contexts}.
%a new breed of applications arises that {\em augment LLMs with memory}. 
Traditionally, language models take standalone prompts as their input and rely on information embedded in the models to generate responses. 
Today, however, more users query LLMs with prompts that require domain or new knowledge not possessed by the LLM.
Thus, applications often supplement these prompts with ``context'' texts retrieved from a knowledge base that includes relevant domain information.
For instance, to answer a legal question, the LLM input may include documents retrieved from a database of relevant cases.
Similarly, more interactions between users and LLMs create longer conversation histories, which are fed to the LLM as user-specific ``context'' to ensure quality and coherent responses (\eg ``write a reminder to X based on the email to her which was generated a week ago'').
The recent literature of LLMs often use long contexts that contain thousands to tens of thousands of tokens (or words), with longer contexts often leading to superior generation quality (\eg~\cite{??,??}). 
%Retrieval-based LLMs (\eg~\cite{??,??}) also show superior generation quality when provided with longer context. 
%Recently, retrieval-based learning (\eg~\cite{??,??}) enables LLMs to process contexts with over hundreds of thousands of tokens (or words) and shows they produce superior answers when provided with longer context. 

\begin{comment}
More interactions between users and LLMs also increase context length. 
As users accumulate longer conversation histories with LLM services, and LLMs need information from prior prompts and responses to ensure generation quality and coherence (\eg ``write a reminder to X based on the email to her which was generated a week ago'').
% the next prompt may use information from any prior interactions.
Long context in conversation histories are also common in long-context learning and few-shot learning, where LLMs learn new knowledge or to behavior in certain way by first processing a series of prompts, whose length can easily be over thousands of words.
%, and these prompts and responses become the ``context'' of the LLM's next input. 
For instance, \jc{TODO: add an example here}
Because the LLM itself keeps no internal states, LLM applications must store the conversation history and include a part or the whole of it to the LLM as the context of a prompt.
\end{comment}

%Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow LLMs  to learn new knowledge by feeding them with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).


\begin{comment}
in retrieval-based learning, to answer a user query, applications often supplement the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 

These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%it has changed as LLMs are used in real-world applications. 
However, as users constantly interact with LLMs, they accumulate long conversation histories (prompts and responses), and the next prompt may use information from prior interactions.
Because the LLM itself keeps no internal state between two inferences, to provide coherent responses, LLM applications often include many previous prompts and responses as part of the input to the LLM.
%users today form longer interactions with LLMs (\eg in-context learning), may refer to any prior interactions in the next prompt, and demand coherent responses.
%Since the LLM keeps no internal state between two inferences, this means that the input of LLM needs to include many or even the entire conversational history of interactions between a user and an LLM, which we refer to as the ``context'' part of the input.
Similarly, in retrieval-based learning, to answer a user query, an application often supplements the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 
For instance, answering a legal inquiry may need access to a database of prior cases.
These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
\end{comment}

%the LLM to first process some supplementary documents extracted from a knowledge base.
%%However, when using memory-augmented LLMs, users can issue a sequence of queries, with the response to each query becomes part of the ``memory'' of subsequent queries. 
%%In the meantime, to produce high-quality responses, LLMs may require large supplementary input. 
%For instance, answering a legal inquiry may need access to a database of prior cases.
%These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%Many recent efforts of memory augmented LLMs have been focused on how LLMs can be trained to process long memory (\eg~\cite{??,??,??}). 


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/intro_perf.pdf}
    \tightcaption{} 
    \label{fig:intro}
\end{figure*}

Since the context must be processed by the LLM before it starts to generate any response, long contexts pose a challenge when these contexts are stored {\em separately} from the GPUs running the LLM. 
% to the underlying LLM serving system 
% when {\em the storage and computation of these contexts are separate}.
For instance, a knowledge base might reside in a separate server and the supplementary documents assisting LLM inference are only to be selected and fetched to the LLM when a query is received~\cite{??,??}.
Similarly, as the prompts from a user may spread in both time (\eg two queries can be days apart) and space (from different locations), they might be processed by different machines, so the conversation history (\ie context) must be loaded on-demand to the GPUs serving the current request~\cite{??,??}.

In the LLM literature, contexts are handled in two ways but neither is ideal for fast loading of long contexts.
First, storing each context as text has a small size, but due to the self-attention mechanism, the delay for an LLM to process a long context increases quadratically with the context length~\cite{??}.
Alternatively, long-context learning sometimes caches the LLM's intermediate outcome of a context, namely, the key-value (KV) features (\eg~\cite{??,??,??}).
However, these KV features, which are multi-dimensional tensors of float numbers, can be much larger in size than the context itself \jc{some concrete numbers here}.
Thus, they require much more network bandwidth to send to the GPUs running the LLM.  
While some emerging methods can shorten context or reduce KV tensor size in GPU memory~\cite{scissorhand,gisting,flexgen,autoencoder-incontext}, it remains a challenge to minimize or control the loading delays of long contexts without impacting generation quality or modifying the LLM.


%Some emerging research on long-context modeling also tries to the footprint of KV cache in memory or rewriting 
%In short, how to {\em quickly load and process} long contexts remains a challenge.

\begin{comment}
In general, many previous efforts have focused on speeding up inference (\eg caching KV features or shrinking model sizes) and enabling long-context inference without exceeding the GPU memory limit. 
However, they do not directly optimize the size of KV cache of long contexts and the delay to load and process long context when it is not in GPU memory. 

The increase of context length has a profound implication on the underlying LLM serving system when {\em the storage and computation of these contexts are separate}. 

Rather than feeding the context directly to the LLM, a common approach to handle a long context is to cache the intermediate outcome of LLM on the context, namely, the key-value (KV) cache (\eg~\cite{??,??,??}).
Compared to directly processing the context whose delay grows quadratically with the context length, a KV cache speeds up the inference. 
However, KV features of long context can be large in size. \jc{some concrete numbers here}

While the size of KV features is not a serious issue when KV features are kept in GPU memory or on the same machine, unfortunately, long contexts sometimes have to be {\em dynamically loaded and processed}.
%it is not always feasible to keep KV features in GPU memory, as the contexts are sometimes {\em dynamically loaded and processed}.
%Unfortunately, keeping the KV features in the GPU memory is not always feasible, as the contexts are sometimes {\em dynamically loaded and processed}.
%between receiving a query and starting to generate the response. 
For instance, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
Similarly, as the prompts from a user may spread in both time (across a long time) and space (from different locations), they might be processed by different machines, so the conversation history will be loaded on-demand over the network.
As a result, if we cache KV features, it may need too much space to store and too much bandwidth to fetch dynamically. 
\jc{TODO: need some concrete numbers here.}
If we quantize the KV features or filter most relevant tokens, the size can be reduced but at a great expense of generation quality.


In general, many previous efforts have focused on speeding up inference (\eg caching KV features or shrinking model sizes) and enabling long-context inference without exceeding the GPU memory limit. 
However, they do not directly optimize the size of KV cache of long contexts and the delay to load and process long context when it is not in GPU memory. 

\end{comment}


%However, KV features need significantly more space to store and more network bandwidth to fetch remotely.
%\jc{TODO: need some concrete numbers here.}
%If we quantize the KV features or filter most relevant tokens, the size can be reduced but at a great expense of generation quality.
%An alternative approach is to filter the context and only feed LLM with the most relevant text (\eg~\cite{??,??,??}), but it always degrade generation quality.

%Even if the same GPU serves all prompts of a user, it may be shared with many other users and cannot keep each user's context indefinitely in GPU.

%If we naively feed the long context directly to the LLM, the latency of processing a context in transformer models will grow quadratically with the context length. 
%While we can reduce the context length by sampling only the most relevant part, but doing so often degrade generation quality~\cite{??,??}.
%%it would take too much time to process them before the actual generation starts. 





%In short, existing solutions are remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(2) reduce the context length by sampling only the most relevant part.
%
%
%
%Instead, many LLM systems cache the intermediate processed outcome---{\em key-value features}---of contexts.


%To avoid high inference delay, current LLM systems employ two methods.
%First, they cache the intermediate processed outcome, \ie key-value features, of contexts.
%Compared to directly loading context, this significantly speeds up the inference but it needs much more space to store and much more bandwidth to fetch.
%Alternatively, some works sample contexts and only include the most relevant text in LLM input, but they have to degrade generation quality to reduce the context length.
%As a result, it remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(1) cache the key-value features of contexts, and 
%(2) sample contexts and only include the most relevant text in LLM input.
%Compared to loading context as text, the former needs significantly more space to store and more bandwidth to fetch, whereas the latter has to degrade generation quality to reduce the context length.

%how to fetch context efficiently to unlock the full potential of LLMs remains a challenge and will likely be more so in the future. 




% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
%Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
%Last but not least, 


\begin{comment}

However, integrating context to LLM inference also presents challenges, especially when the context is long and must be fetched remotely. 

\begin{packeditemize}
\item {\em Long context:} 
Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow an LLM  to learn new knowledge by feeding LLM with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).
Moreover, retrieval-based LLMs (\eg~\cite{??,??}), capable of handling memory texts with more than 100K works, have demonstrated the ability to produce superior answers when provided with more supplementary documents.

\item {\em Dynamism:} 
The context of an LLM input is present before a prompt is received, but it is not static; rather it can change constantly. 
%Memory text is not static either; it is {\em dynamically}. 
As interactions between a user and an LLM progresses, its conversational history expands, and sometimes only a subset of it might be pertinent for each query.\footnote{This subset could be any part of the dialog history, not necessarily the most recent history, for example, ``write a reminder to X based on the email I sent her a week ago.''}
Similarly, depending on the next query, the supplementary documents extracted as the context will differ.


\item {\em Remote fetching:} 
Last but not least, the context of an input often needs to be retrieved from an external server.
For instance, as a user travels between locations, her queries might be processed by different GPUs, so her conversation history cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.

\end{packeditemize}


%These memory-augmented LLMs raise new challenges for the underlying LLM serving systems, which serve large DNNs but with a relatively small prompt input, rather than dynamic history. 
Currently, long context can be handled in two ways, but as depicted in Figure~\ref{fig:intro}(a), neither is ideal for different reasons. 

\begin{packedenumerate}
\item Traditionally, LLM takes the context of a prompt in the form of raw text.
The LLM needs to process the words to {\em keys-value} features as intermediate results first before generating the response.
The advantage of this method is the relative small size of context text, so it can be fetched quickly. 
However, the delay to process context can increase quadratically with the length of the context. 

\item Alternatively, one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
This is because the context is often from a knowledge base known in advance or from prior interactions of a user whose key-value features are already computed.
%one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
%leverage that the masked attention mechanism in transformers to cache the keys and values (or self-attention matrices) the of memory text as intermediate results. 
This strategy minimizes the processing delay for context. 
However, the size of the key and value features are much larger than text, so it can take longer to retrieve the key and value features. 
\jc{need some concrete numbers here}

\end{packedenumerate}

\end{comment}



%To make it more concrete, we perform a measurement the size of key-value features of two different LLMs under two datasets, each including over \fillme tokens.

This paper presents \name, a fast LLM inference system designed for loading long contexts.
\name has three design goals: 
(1) minimizing the network bandwidth usage to fetch KV cache of long contexts; 
(2) being able to meet a time budget on the total delay of loading and processing long contexts with minimum impact on generation quality; and 
(3) no need to train a new NN or modify the pre-trained LLM.
To meet these goals, \name entails two key techniques.
%Unlike the recent efforts that reduce the dimensionality of context or key-value features. (\eg~\cite{??,??,??}), \name aims at reducing the communication overhead to meet the application-specified response deadline with minimum impact on generation quality and no modification to the pre-trained LLM.

First, \name reduces the network bandwidth demand of long contexts by compressing their KV caches into compact bitstreams.
Compared to recent efforts that shrink the KV tensor sizes, our compression is more efficient because our compressed bitstreams do not have to be in the form of a tensor.
Our compression leverages a tailored arithmetic coder which takes advantage of KV features' distributional characteristics.
For instance, \jc{pick an interesting one to highlight here}
It also leverages the fact that different layers of the KV features affect the final generation quality differently, so it applies different quantization levels to different layers.
\name further speeds up the loading of long contexts by pipelining the decompression and GPU memory loading of KV caches in a layer-wise fashion.

Second, \name allows LLM applications to set a budget on the time to the generation of the first token (TTFT), which includes the time to load the context into GPU and the additional computation time to process the prompt.
To this end, rather than compressing the context once, \name compresses each context in multiple versions, covering a range of tradeoffs between TTFT and generation quality.
Notably, these versions also include loading the context as raw text, rather than KV features, 
because when the context is relatively short (less than 100s tokens), the overhead of decompressing the KV cache and loading it to GPU exceeds the delay saved by caching KV features.
When given a TTFT budget and an input (context and prompt), \name estimates the distribution of TTFT of different versions of the context using history TTFTs and estimated bandwidth.

%For a given query (including the prompt and the context), 
%While it is hard to guarantee a delay due to inherent system noise, \name predicts the 
%
%To meet the budget, \name predicts a minimum compression level of the KV cache such that the delay to load the KV cache and compute the cross-attention between prompt and context will not exceed the deadline. 
%To this end, \name will also automatically switch to loading the context as raw text as oppose to its KV cache.
%This is because when the context is short enough, the overhead of decompressing the KV cache and loading it to GPU exceeds the delay saving of caching KV features.

%Unlike the recent efforts that aim at reducing the dimensionality or memory footprint of the key-value tensors, \name compresses key-value caches to bitstreams by leveraging key-value features' distributional properties, such as locality across nearby tokens, custom entropy coding, and layer-specific quantization.
%\jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}

%Second, even retrieving the key-value features, the LLM still needs to calculate the attention matrices (self-attention and cross attention) of each LLM layer. 
%To expedite this process, \name fetch cached key-value features in a layer-by-layer fashion, so that the transferring of features and computation of attention matrices can be pipelined.

%Finally, since loading compressed key-value features involves additional cost, including decompression and loading more data to GPU memory, directly loading the context tokens might sometimes be faster when the context is short. 
%Therefore, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens based on estimated delay of each method. 



\begin{comment}
\name entails three techniques to reduce the size and processing delay of context with only marginal quality degradation. % to significantly accelerate the loading of memory text for LLMs.


First, \name shrinks the size of cached key-value features using a new compression algorithm.
The compression algorithm leverages several domain-specific insights, such as \fillme. \jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}



Third, since loading compressed key-value features involves additional cost, including decompression and loading more data to GPU memory, directly loading the context tokens might sometimes be faster when the context is short. 
Therefore, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens based on estimated delay of each method. 

%to minimize loading and processing delay under various context length, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens, which might be much faster with short context, depending on the hardware of the GPU machine. 
\end{comment}

%depending on the text input and the inference speed, it is sometimes faster to directly load and process the tokens of context, rather than loading the compressed key-value features which involves additional decompression overhead. 




%To our best knowledge, \name is the first to optimize the communication aspects of LLM with long context, and it complements other efforts aimed at augmenting LLMs with longer context. 
Our evaluation shows that \fillme

\jc{finally, a paragraph on evaluation highlights. we create a benchmark with \fillme. key takeaways are:
\begin{packeditemize}
\item \name can compress the KV caches of long contexts \fillme more efficiently than \fillme at the same perplexity
\item \name reduces time to generation by \fillme
\item with the same generation delay, \name can achieve \fillme better quality (perplexity, accuracy)
\end{packeditemize}
}


%
%The idea of \name is to compress the key-value features of memory first before retrieving them from remote servers, instead of retrieving them in the form of tensors. \hc{Maybe also mention the potential to make llm inference much faster here?}
%
%Though this idea may seem simple, compressing key-value features is by no means trivial. 
%For instance, quantization is commonly used to reduce footprint of tensors in GPU RAM, but it reduces memory size at the cost of greatly increased perplexity (illustrated in Figure~\ref{fig:intro}(b)). 
%Similarly, arithmetic coding, though lossless, does not yield much compression when applied directly on key-value features. 
%Instead, \name embraces several common patterns of key-value features.
%\jc{list the insights here.}
%Moreover, given a delay target, \name can automatically select the right compression configuration to retrieve maximum amount of memory without violating the delay target. 
%\jc{a few words on this}

 







==> backups/intro-v8.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Introduction}

%Generative AI, in the form of large language models (LLMs), has transformed many internet applications.
With its impressive generative capabilities gradually recognized by the public, large language models (LLMs) are widely used~\cite{??,??} in personal assistant and recommendation, AI healthcare and marketing, to mention a few. 
The widespread use of LLM APIs (\eg GPT-4~\cite{??}) and application frameworks (\eg Langchain~\cite{??}), combined with the open-source of industry-quality LLMs (\eg LLaMA~\cite{??}), further boosts LLMs' popularity in the coming years.
%The availability of the LLMs, APIs or frameworks (such as OpenAI GPT-4, LLaMA, and Langchain) to developers further contributes to the growth in LLMs' popularity in the coming years.
%\jc{cite some industry reports on the rapid growth of GPT queries or LLM in general}

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_long_input.pdf}
    \tightcaption{The input length accepted by LLMs has increased significantly in the last year.} 
    \label{fig:motivate_long_input}
\end{figure}

%- trend: long input
%- reason: ability to learn
%- examples
%
%- most of input is context, which can be pre-processed
%- but must be loaded dynamically




A key to LLMs' success is their ability to reason about and learn new knowledge from long inputs.
Long-context learning has also become a key research topic, which demonstrates that longer inputs often improve the quality of the generated response.
Consequently, the input length accepted by LLMs has increased dramatically in the last year, from 2K tokens in ChatGPT to \fillme~K in \fillme, as shown in Figure~\ref{fig:motivate_long_input}.

%With LLMs used in more applications, 
As LLMs are capable of processing longer inputs, we see a notable trend in LLM applications---the augmentation of LLM's input with {\em long contexts}.
%a new breed of applications arises that {\em augment LLMs with memory}. 
Traditionally, language models take standalone prompts as their input and generate response based only on information embedded in the models. 
Today, more users query LLMs with prompts that require domain knowledge not possessed by the LLM, and applications often add ``context'' texts retrieved from a knowledge base that includes relevant domain information.
For instance, to answer a legal question, the LLM input may include documents retrieved from a database of relevant cases.
Similarly, as each user interacts with LLM applications, longer conversation histories need to be fed to the LLM as user-specific ``context'' to ensure quality and coherent responses (\eg ``write a reminder to X based on the email to her which was generated a week ago'').
%The recent literature of LLMs often use long contexts that contain thousands to tens of thousands of tokens (or words), with longer contexts often leading to superior generation quality (\eg~\cite{??,??}). 
%Retrieval-based LLMs (\eg~\cite{??,??}) also show superior generation quality when provided with longer context. 
%Recently, retrieval-based learning (\eg~\cite{??,??}) enables LLMs to process contexts with over hundreds of thousands of tokens (or words) and shows they produce superior answers when provided with longer context. 

\begin{comment}
More interactions between users and LLMs also increase context length. 
As users accumulate longer conversation histories with LLM services, and LLMs need information from prior prompts and responses to ensure generation quality and coherence (\eg ``write a reminder to X based on the email to her which was generated a week ago'').
% the next prompt may use information from any prior interactions.
Long context in conversation histories are also common in long-context learning and few-shot learning, where LLMs learn new knowledge or to behavior in certain way by first processing a series of prompts, whose length can easily be over thousands of words.
%, and these prompts and responses become the ``context'' of the LLM's next input. 
For instance, \jc{TODO: add an example here}
Because the LLM itself keeps no internal states, LLM applications must store the conversation history and include a part or the whole of it to the LLM as the context of a prompt.
\end{comment}

%Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow LLMs  to learn new knowledge by feeding them with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).


\begin{comment}
in retrieval-based learning, to answer a user query, applications often supplement the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 

These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%it has changed as LLMs are used in real-world applications. 
However, as users constantly interact with LLMs, they accumulate long conversation histories (prompts and responses), and the next prompt may use information from prior interactions.
Because the LLM itself keeps no internal state between two inferences, to provide coherent responses, LLM applications often include many previous prompts and responses as part of the input to the LLM.
%users today form longer interactions with LLMs (\eg in-context learning), may refer to any prior interactions in the next prompt, and demand coherent responses.
%Since the LLM keeps no internal state between two inferences, this means that the input of LLM needs to include many or even the entire conversational history of interactions between a user and an LLM, which we refer to as the ``context'' part of the input.
Similarly, in retrieval-based learning, to answer a user query, an application often supplements the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 
For instance, answering a legal inquiry may need access to a database of prior cases.
These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
\end{comment}

%the LLM to first process some supplementary documents extracted from a knowledge base.
%%However, when using memory-augmented LLMs, users can issue a sequence of queries, with the response to each query becomes part of the ``memory'' of subsequent queries. 
%%In the meantime, to produce high-quality responses, LLMs may require large supplementary input. 
%For instance, answering a legal inquiry may need access to a database of prior cases.
%These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%Many recent efforts of memory augmented LLMs have been focused on how LLMs can be trained to process long memory (\eg~\cite{??,??,??}). 

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/intro_perf_short.pdf}
    \tightcaption{Context processing delay of this work vs. existing context-retrieval methods.} 
    \label{fig:intro}
\end{figure}

%\begin{figure*}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/intro_perf.pdf}
%    \tightcaption{} 
%    \label{fig:intro}
%\end{figure*}

Since the context must be processed by the LLM before it starts to generate any response, long contexts pose a challenge when these contexts are stored {\em separately} from the GPUs running the LLM. 
% to the underlying LLM serving system 
% when {\em the storage and computation of these contexts are separate}.
For instance, a knowledge base might reside in a separate server and the supplementary documents assisting LLM inference are only to be selected and fetched to the LLM when a query is received~\cite{??,??}.
Similarly, as the prompts from a user may spread in both time (\eg two queries can be days apart) and space (from different locations), they might be processed by different machines, so the conversation history (\ie context) must be loaded on-demand to the GPUs serving the current request~\cite{??,??}.

In the LLM literature, contexts are handled in two ways but neither is ideal for fast loading of long contexts.
First, storing each context as text has a small size, but due to the self-attention mechanism, the delay for an LLM to process a long context increases quadratically with the context length~\cite{??}.
Alternatively, long-context learning sometimes caches the LLM's intermediate outcome of a context, namely, the key-value (KV) features (\eg~\cite{??,??,??}).
However, these KV features, which are multi-dimensional tensors of float numbers, can be much larger in size than the context itself \jc{some concrete numbers here}.
Thus, they require much more network bandwidth to send to the GPUs running the LLM.  
While some emerging methods can shorten context or reduce KV tensor size in GPU memory~\cite{scissorhand,gisting,flexgen,autoencoder-incontext}, it remains a challenge to minimize or control the loading delays of long contexts without impacting generation quality or modifying the LLM.


%Some emerging research on long-context modeling also tries to the footprint of KV cache in memory or rewriting 
%In short, how to {\em quickly load and process} long contexts remains a challenge.

\begin{comment}
In general, many previous efforts have focused on speeding up inference (\eg caching KV features or shrinking model sizes) and enabling long-context inference without exceeding the GPU memory limit. 
However, they do not directly optimize the size of KV cache of long contexts and the delay to load and process long context when it is not in GPU memory. 

The increase of context length has a profound implication on the underlying LLM serving system when {\em the storage and computation of these contexts are separate}. 

Rather than feeding the context directly to the LLM, a common approach to handle a long context is to cache the intermediate outcome of LLM on the context, namely, the key-value (KV) cache (\eg~\cite{??,??,??}).
Compared to directly processing the context whose delay grows quadratically with the context length, a KV cache speeds up the inference. 
However, KV features of long context can be large in size. \jc{some concrete numbers here}

While the size of KV features is not a serious issue when KV features are kept in GPU memory or on the same machine, unfortunately, long contexts sometimes have to be {\em dynamically loaded and processed}.
%it is not always feasible to keep KV features in GPU memory, as the contexts are sometimes {\em dynamically loaded and processed}.
%Unfortunately, keeping the KV features in the GPU memory is not always feasible, as the contexts are sometimes {\em dynamically loaded and processed}.
%between receiving a query and starting to generate the response. 
For instance, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
Similarly, as the prompts from a user may spread in both time (across a long time) and space (from different locations), they might be processed by different machines, so the conversation history will be loaded on-demand over the network.
As a result, if we cache KV features, it may need too much space to store and too much bandwidth to fetch dynamically. 
\jc{TODO: need some concrete numbers here.}
If we quantize the KV features or filter most relevant tokens, the size can be reduced but at a great expense of generation quality.


In general, many previous efforts have focused on speeding up inference (\eg caching KV features or shrinking model sizes) and enabling long-context inference without exceeding the GPU memory limit. 
However, they do not directly optimize the size of KV cache of long contexts and the delay to load and process long context when it is not in GPU memory. 

\end{comment}


%However, KV features need significantly more space to store and more network bandwidth to fetch remotely.
%\jc{TODO: need some concrete numbers here.}
%If we quantize the KV features or filter most relevant tokens, the size can be reduced but at a great expense of generation quality.
%An alternative approach is to filter the context and only feed LLM with the most relevant text (\eg~\cite{??,??,??}), but it always degrade generation quality.

%Even if the same GPU serves all prompts of a user, it may be shared with many other users and cannot keep each user's context indefinitely in GPU.

%If we naively feed the long context directly to the LLM, the latency of processing a context in transformer models will grow quadratically with the context length. 
%While we can reduce the context length by sampling only the most relevant part, but doing so often degrade generation quality~\cite{??,??}.
%%it would take too much time to process them before the actual generation starts. 





%In short, existing solutions are remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(2) reduce the context length by sampling only the most relevant part.
%
%
%
%Instead, many LLM systems cache the intermediate processed outcome---{\em key-value features}---of contexts.


%To avoid high inference delay, current LLM systems employ two methods.
%First, they cache the intermediate processed outcome, \ie key-value features, of contexts.
%Compared to directly loading context, this significantly speeds up the inference but it needs much more space to store and much more bandwidth to fetch.
%Alternatively, some works sample contexts and only include the most relevant text in LLM input, but they have to degrade generation quality to reduce the context length.
%As a result, it remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(1) cache the key-value features of contexts, and 
%(2) sample contexts and only include the most relevant text in LLM input.
%Compared to loading context as text, the former needs significantly more space to store and more bandwidth to fetch, whereas the latter has to degrade generation quality to reduce the context length.

%how to fetch context efficiently to unlock the full potential of LLMs remains a challenge and will likely be more so in the future. 




% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
%Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
%Last but not least, 


\begin{comment}

However, integrating context to LLM inference also presents challenges, especially when the context is long and must be fetched remotely. 

\begin{packeditemize}
\item {\em Long context:} 
Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow an LLM  to learn new knowledge by feeding LLM with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).
Moreover, retrieval-based LLMs (\eg~\cite{??,??}), capable of handling memory texts with more than 100K works, have demonstrated the ability to produce superior answers when provided with more supplementary documents.

\item {\em Dynamism:} 
The context of an LLM input is present before a prompt is received, but it is not static; rather it can change constantly. 
%Memory text is not static either; it is {\em dynamically}. 
As interactions between a user and an LLM progresses, its conversational history expands, and sometimes only a subset of it might be pertinent for each query.\footnote{This subset could be any part of the dialog history, not necessarily the most recent history, for example, ``write a reminder to X based on the email I sent her a week ago.''}
Similarly, depending on the next query, the supplementary documents extracted as the context will differ.


\item {\em Remote fetching:} 
Last but not least, the context of an input often needs to be retrieved from an external server.
For instance, as a user travels between locations, her queries might be processed by different GPUs, so her conversation history cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.

\end{packeditemize}


%These memory-augmented LLMs raise new challenges for the underlying LLM serving systems, which serve large DNNs but with a relatively small prompt input, rather than dynamic history. 
Currently, long context can be handled in two ways, but as depicted in Figure~\ref{fig:intro}(a), neither is ideal for different reasons. 

\begin{packedenumerate}
\item Traditionally, LLM takes the context of a prompt in the form of raw text.
The LLM needs to process the words to {\em keys-value} features as intermediate results first before generating the response.
The advantage of this method is the relative small size of context text, so it can be fetched quickly. 
However, the delay to process context can increase quadratically with the length of the context. 

\item Alternatively, one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
This is because the context is often from a knowledge base known in advance or from prior interactions of a user whose key-value features are already computed.
%one can cache the pre-computed keys and values, or even self-attention matrices, of the context, storing them as intermediate outcomes.
%leverage that the masked attention mechanism in transformers to cache the keys and values (or self-attention matrices) the of memory text as intermediate results. 
This strategy minimizes the processing delay for context. 
However, the size of the key and value features are much larger than text, so it can take longer to retrieve the key and value features. 
\jc{need some concrete numbers here}

\end{packedenumerate}

\end{comment}



%To make it more concrete, we perform a measurement the size of key-value features of two different LLMs under two datasets, each including over \fillme tokens.

This paper presents \name, a fast LLM inference system designed for loading long contexts.
\name has three design goals: 
(1) minimizing the network bandwidth needed for transmitting fetch the KV cache of long contexts; 
(2) being able to minimize the impact on the quality of generation without exceeding a targeted loading delay specified by the application; and
%meet a given time budget on the total delay of loading and processing long contexts with minimum impact on generation quality; and 
(3) no need to train a new NN or modify the pre-trained LLM.
To meet these goals, \name entails two key techniques.
%Unlike the recent efforts that reduce the dimensionality of context or key-value features. (\eg~\cite{??,??,??}), \name aims at reducing the communication overhead to meet the application-specified response deadline with minimum impact on generation quality and no modification to the pre-trained LLM.

First, \name reduces the network bandwidth demand of long contexts by compressing their KV caches into compact bitstreams using a new context encoder.
Compared to recent efforts that shrink the KV tensor sizes, our context encoding is more efficient as the encoded bitstreams do not have to be in the form of a tensor.
\name's context encoder leverages a tailored arithmetic coder which takes advantage of KV features' distributional characteristics.
For instance, \jc{pick an interesting one to highlight here}
It also leverages the fact that different layers of the KV features affect the final generation quality differently, so it applies different quantization levels to different layers.
\name further speeds up the loading of long contexts by pipelining the decompression and GPU memory loading of KV caches in a layer-wise fashion.

Second, \name allows LLM applications to set a budget on the time to the generation of the first token (TTFT), which includes the time to load the context into GPU and the additional computation time to process the prompt.
To this end, rather than compressing the context once, \name compresses each context in multiple versions, covering a range of tradeoffs between TTFT and generation quality.
Notably, these versions also include loading the context as raw text, rather than KV features, 
because when the context is relatively short (less than 100s tokens), the overhead of decompressing the KV cache and loading it to GPU exceeds the delay saved by caching KV features.
When given a TTFT budget and an input (context and prompt), \name estimates the distribution of TTFT of different versions of the context using history TTFTs and estimated bandwidth.

%No individual component of \name is exactly new . 
To put \name's design into perspective, each of its component has been used in other domains. 
Adapting compression level to navigate size-quality tradeoffs is commonly done in video streaming.
Quantization and arithmetic coding has been used to in DNN training clusters to compress gradient tensors~\cite{??,??}. 
Caching KV features is a common trick in LLM services to speedup inference~\cite{??,??}. 
Nonetheless, the exact designs of these components in \name embrace domain-specific insights about KV features, and \name integrates them in a way that explicitly minimizes the loading delay of LLMs with long contexts for the first time.

%For a given query (including the prompt and the context), 
%While it is hard to guarantee a delay due to inherent system noise, \name predicts the 
%
%To meet the budget, \name predicts a minimum compression level of the KV cache such that the delay to load the KV cache and compute the cross-attention between prompt and context will not exceed the deadline. 
%To this end, \name will also automatically switch to loading the context as raw text as oppose to its KV cache.
%This is because when the context is short enough, the overhead of decompressing the KV cache and loading it to GPU exceeds the delay saving of caching KV features.

%Unlike the recent efforts that aim at reducing the dimensionality or memory footprint of the key-value tensors, \name compresses key-value caches to bitstreams by leveraging key-value features' distributional properties, such as locality across nearby tokens, custom entropy coding, and layer-specific quantization.
%\jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}

%Second, even retrieving the key-value features, the LLM still needs to calculate the attention matrices (self-attention and cross attention) of each LLM layer. 
%To expedite this process, \name fetch cached key-value features in a layer-by-layer fashion, so that the transferring of features and computation of attention matrices can be pipelined.

%Finally, since loading compressed key-value features involves additional cost, including decompression and loading more data to GPU memory, directly loading the context tokens might sometimes be faster when the context is short. 
%Therefore, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens based on estimated delay of each method. 



\begin{comment}
\name entails three techniques to reduce the size and processing delay of context with only marginal quality degradation. % to significantly accelerate the loading of memory text for LLMs.


First, \name shrinks the size of cached key-value features using a new compression algorithm.
The compression algorithm leverages several domain-specific insights, such as \fillme. \jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}



Third, since loading compressed key-value features involves additional cost, including decompression and loading more data to GPU memory, directly loading the context tokens might sometimes be faster when the context is short. 
Therefore, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens based on estimated delay of each method. 

%to minimize loading and processing delay under various context length, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens, which might be much faster with short context, depending on the hardware of the GPU machine. 
\end{comment}

%depending on the text input and the inference speed, it is sometimes faster to directly load and process the tokens of context, rather than loading the compressed key-value features which involves additional decompression overhead. 




%To our best knowledge, \name is the first to optimize the communication aspects of LLM with long context, and it complements other efforts aimed at augmenting LLMs with longer context. 
Our evaluation shows that \fillme

\jc{finally, a paragraph on evaluation highlights. we create a benchmark with \fillme. key takeaways are:
\begin{packeditemize}
\item \name can compress the KV caches of long contexts \fillme more efficiently than \fillme at the same perplexity
\item \name reduces time to generation by \fillme
\item with the same generation delay, \name can achieve \fillme better quality (perplexity, accuracy)
\end{packeditemize}
}


%
%The idea of \name is to compress the key-value features of memory first before retrieving them from remote servers, instead of retrieving them in the form of tensors. \hc{Maybe also mention the potential to make llm inference much faster here?}
%
%Though this idea may seem simple, compressing key-value features is by no means trivial. 
%For instance, quantization is commonly used to reduce footprint of tensors in GPU RAM, but it reduces memory size at the cost of greatly increased perplexity (illustrated in Figure~\ref{fig:intro}(b)). 
%Similarly, arithmetic coding, though lossless, does not yield much compression when applied directly on key-value features. 
%Instead, \name embraces several common patterns of key-value features.
%\jc{list the insights here.}
%Moreover, given a delay target, \name can automatically select the right compression configuration to retrieve maximum amount of memory without violating the delay target. 
%\jc{a few words on this}

 







==> backups/intro-v9.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\tightsection{Introduction}

With their impressive generative capabilities,
%recognized by the public, 
large language models (LLMs) are widely used~\cite{llm-app-1,llm-app-2,llm-app-3,llm-app-4} in personal assistance and recommendation, AI healthcare, and marketing, to mention a few. 
The widespread use of public LLM APIs (\eg GPT-4~\cite{gpt4-api}) and application frameworks (\eg Langchain~\cite{langchain}), combined with the open-source of industry-quality LLMs (\eg Llama~\cite{llama}), further boosts LLMs' popularity. 

%with longer inputs often producing higher response quality\shan{any citation for this claim?}.

%in the coming years.
%The availability of the LLMs, APIs or frameworks (such as OpenAI GPT-4, LLaMA, and Langchain) to developers further contributes to the growth in LLMs' popularity in the coming years.
%\jc{cite some industry reports on the rapid growth of GPT queries or LLM in general}

\begin{figure}
\centering
     \includegraphics[width=.85\linewidth]{figs/llm_token.pdf}
    \tightcaption{The input length accepted by LLMs has increased significantly in the last year.
    y-axis is plotted in log-scale.
%    \jc{yuhan, please make this figure once you get a chance}
} 
    \label{fig:motivate_long_input}
\end{figure}


%A key to LLMs' success is their ability to reason about and learn new knowledge from long inputs. This strength of LLMs, referred to as long-context learning, has also become a key research topic, with longer inputs often improving the quality of the generated response. Consequently, the input length accepted by LLMs has increased dramatically in the last year, 

%With LLMs used in more applications, 
%Capitalizing on LLMs' ability to process long inputs, 
With LLMs increasingly used in complex tasks, many applications augment their user inputs (\ie prompts)
to LLMs with {\em long contexts} containing at least thousands of tokens.
For example, some context supplements user prompts with
domain-knowledge texts so that LLMs can generate responses using domain knowledge
beyond information embedded in LLMs themselves.
%we see a notable trend in LLM applications---the augmentation of LLM's input with {\em long contexts}.
%a new breed of applications arises that {\em augment LLMs with memory}. 
%Traditionally, language models rely on information embedded in themselves to generate responses. 
%take short prompts as input and generate response based only on information embedded in the models. 
%Today, many user prompts require domain knowledge not possessed by LLMs,
% and it is common to supplement user prompts with 
%domain-knowledge texts (i.e., context) to help LLMs generate better responses.
%, with longer contexts often yielding better response quality.
%As a result, applications often add ``context'' texts retrieved from a knowledge base that includes relevant domain information.
%For instance, to answer a legal question, the LLM input may include documents retrieved from a database of relevant cases.
As another example, some context supplements user prompts with the conversation histories
accumulated during the interaction between a user and the LLM.
%Another type of long contexts is related to conversational history.
%When users interact with the LLM, conversation histories are accumulated. Supplementing a user-input
%text with such conversation histories (i.e., context) can help LLM generate responses with 
%higher quality and better coherence. 

This trend of long contexts is well reflected by the recent race to train LLMs that accept ever longer inputs, 
%The increasing use of long contexts also has led to a dramatic increase of input length accepted by LLMs, 
from 2K tokens in ChatGPT to 100K in Claude~\cite{long-context} (Figure~\ref{fig:motivate_long_input}).
While short LLM inputs can still be useful~\cite{arxiv-1,arxiv-2}, many studies have shown that longer inputs often help improve response quality and coherence~\cite{beltagy2020longformer,long-llama, wu2022memorizing, dai*2019transformerxl,roy2021efficient,bertsch2023unlimiformer, fid, retro}. 


% \shan{what exactly does this example mean?} 
% \eg ``write a reminder to X based on the email to her which was generated a week ago'').
%The recent literature of LLMs often use long contexts that contain thousands to tens of thousands of tokens (or words), with longer contexts often leading to superior generation quality (\eg~\cite{??,??}). 
%Retrieval-based LLMs (\eg~\cite{??,??}) also show superior generation quality when provided with longer context. 
%Recently, retrieval-based learning (\eg~\cite{??,??}) enables LLMs to process contexts with over hundreds of thousands of tokens (or words) and shows they produce superior answers when provided with longer context. 

\begin{comment}
More interactions between users and LLMs also increase context length. 
As users accumulate longer conversation histories with LLM services, and LLMs need information from prior prompts and responses to ensure generation quality and coherence (\eg ``write a reminder to X based on the email to her which was generated a week ago'').
% the next prompt may use information from any prior interactions.
Long context in conversation histories are also common in long-context learning and few-shot learning, where LLMs learn new knowledge or to behavior in certain way by first processing a series of prompts, whose length can easily be over thousands of words.
%, and these prompts and responses become the ``context'' of the LLM's next input. 
For instance, \jc{TODO: add an example here}
Because the LLM itself keeps no internal states, LLM applications must store the conversation history and include a part or the whole of it to the LLM as the context of a prompt.
\end{comment}

%Popular techniques such as long-context learning~\cite{??} and few-shot learning~\cite{??} allow LLMs  to learn new knowledge by feeding them with many ``warm-up'' prompts and use them as the ``context'' of the LLM's next input, whose length can easily be over thousands of words. 
%Popular techniques such as long-context learning and retrieval-based learning allows LLMs to learn new knowledge by feeding LLM with many ``warm-up'' prompts or supplement documents. 
%As a result, conversational histories can easily contain thousands of tokens (words).


\begin{comment}
in retrieval-based learning, to answer a user query, applications often supplement the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 

These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%it has changed as LLMs are used in real-world applications. 
However, as users constantly interact with LLMs, they accumulate long conversation histories (prompts and responses), and the next prompt may use information from prior interactions.
Because the LLM itself keeps no internal state between two inferences, to provide coherent responses, LLM applications often include many previous prompts and responses as part of the input to the LLM.
%users today form longer interactions with LLMs (\eg in-context learning), may refer to any prior interactions in the next prompt, and demand coherent responses.
%Since the LLM keeps no internal state between two inferences, this means that the input of LLM needs to include many or even the entire conversational history of interactions between a user and an LLM, which we refer to as the ``context'' part of the input.
Similarly, in retrieval-based learning, to answer a user query, an application often supplements the query with long relevant documents retrieved from a knowledge base that encompasses useful information. 
For instance, answering a legal inquiry may need access to a database of prior cases.
These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
\end{comment}

%the LLM to first process some supplementary documents extracted from a knowledge base.
%%However, when using memory-augmented LLMs, users can issue a sequence of queries, with the response to each query becomes part of the ``memory'' of subsequent queries. 
%%In the meantime, to produce high-quality responses, LLMs may require large supplementary input. 
%For instance, answering a legal inquiry may need access to a database of prior cases.
%These supplementary text, whether they are conversation histories or additional documents, essentially serve as the ``context'' of an LLM input.
%Many recent efforts of memory augmented LLMs have been focused on how LLMs can be trained to process long memory (\eg~\cite{??,??,??}). 


%\begin{figure*}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/intro_perf.pdf}
%    \tightcaption{} 
%    \label{fig:intro}
%\end{figure*}

Although improving response-generation quality, using long context poses challenges to response-generation {\em latency}, as no response can be generated until all the contexts are loaded and processed. 

To tackle this latency challenge, previous work reduces the computational delays of context processing by caching the 
intermediate processing results: key-value (KV) features. 
This way, instead of repeating the self-attention computation on text context, whose complexity is super-linear to the text length\cite{vaswani2023attention, dao2022flashattention, beltagy2020longformer, zaheer2021big, roy2021efficient}, LLM systems can directly use the KV features and 
skip the redundant computation.

Unfortunately, previous work reduces the computational delay at the cost of increased communication delay, as KV features are multi-dimensional tensors of floating-point numbers and can be orders of magnitude larger than their corresponding text contexts. 
The cost of loading KV features is particularly concerning, as in practice, they often need to be fetched remotely from another machine(s). 
For instance, a database of background documents might reside in a separate server and the supplementary documents assisting LLM inference are only to be selected and fetched to the LLM when a relevant query is received~\cite{langchain-retrival,arxiv-information-retrieval,generative-agents,autogpt,beltagy2020longformer}.
Similarly, as the prompts from a user may spread in space (\eg from different locations) and time (\eg two queries can be days apart), they can be processed by different machines, so the conversation history (\ie context) must be loaded on-the-fly to the GPUs serving the current request~\cite{langchain-retrival,arxiv-information-retrieval}.
Some emergent work shortens context, like dropping tensors, after KV features are loaded into GPU memory~\cite{scissorhand,gisting,autoencoder-incontext}. However, the dropped tensor information inevitably hurts LLM's response quality, and the resulting KV features, in the shape of large tensors, still require high bandwidth to transmit.
%, and they fall short of optimizing the total delay in fetching and processing contexts. 
%\jc{Shan, is this more convincing to you now?}

% \shan{hmm, again, I am not convinced by the next sentence.}
% While some emerging methods propose to rewrite contexts or shrink KV size to pack longer contexts in GPU memory~\cite{scissorhand,gisting,flexgen,autoencoder-incontext}, they do not directly reduce the bandwidth usage of fetching the KV cache or balance the network delay and computation delay. 


Therefore, solely optimizing computational delay is not enough for long-context response generation and may even \emph{degrade} the end-to-end performance, as loading the KV features increases the network delay. %, as shown in Figure \ref{fig:intro}. 
Instead, LLM systems must optimize not only the computational delay but also the communication (network) delay in handling long contexts.
% We define {\em time to first token} ({\em TTFT}) as the total delay of fetching and processing a context, since it reflects the delay between knowing the context and generating the first token for the user.
%Existing solutions that only optimize computation delay are not sufficient.


%Thus, they require much more network bandwidth to transmit, greatly increasing the overall  context-loading delays.
% to send to the GPUs running the LLM.  

%


%Using long contexts can be challenging as they increase {\em both} the computation delay to process the context, as well as the network delay to fetch them.
%Current LLM systems assume the context is stored locally and thus focuses only on reducing computation delay, 
%%and have thus mainly been focused only on reducing the computation delay of processing long contexts.
%
%Therefore, LLM systems must also reduce the network delay to fetch long contexts and balance the network delay and the computation delay, in order to minimize the whole loading delay of long contexts.





\begin{comment}


Using long contexts can be challenging as they increase {\em both} the computation delay to process the context, as well as the network delay to fetch them when the contexts are stored separately from the GPUs running the LLM. 
%Since the context must be processed by the LLM before it starts to generate any response, long contexts pose a challenge when these contexts are stored {\em separately} from the GPUs running the LLM. 
% to the underlying LLM serving system 
% when {\em the storage and computation of these contexts are separate}.
For instance, a knowledge base might reside in a separate server and the supplementary documents assisting LLM inference are only to be selected and fetched to the LLM when a query is received~\cite{??,??}.
Similarly, as the prompts from a user may spread in both time (\eg two queries can be days apart) and space (from different locations), they might be processed by different machines, so the conversation history (\ie context) must be loaded on-demand to the GPUs serving the current request~\cite{??,??}.
Therefore, the whole loading delay of long context incorporates the network delay to fetch the long context to GPUs serving the request and then the computation delay to process the long context and the prompt before starting to generate the response.



Current LLM systems for long-context learning have mainly been focused only on reducing the computation delay of processing long contexts, rather than the entire loading delay, as they target settings where the context is available locally. 
As the computation delay of context grows superlinearly with the context length, most LLM systems avoid the long computation delay by caching the LLM's intermediate key-value (KV) features of a context, namely, the KV cache (\eg~\cite{??,??,??}).
However, these KV features, which are multi-dimensional tensors of float numbers, can be much larger in size than the context itself \jc{some concrete numbers here}.
Thus, they require much more network bandwidth to send to the GPUs running the LLM.  
While some emerging methods can shorten context or reduce KV tensor size in GPU memory~\cite{scissorhand,gisting,flexgen,autoencoder-incontext}, they do not directly reduce the bandwidth usage of fetching the KV cache or balance the network delay and computation delay. 




In the LLM literature, contexts are handled in two ways but neither is ideal for fast loading of long contexts.
First, storing each context as text has a small size, but due to the self-attention mechanism, the delay for an LLM to process a long context increases quadratically with the context length~\cite{??}.
Alternatively, long-context learning sometimes caches the LLM's intermediate outcome of a context, namely, the key-value (KV) features (\eg~\cite{??,??,??}).
However, these KV features, which are multi-dimensional tensors of float numbers, can be much larger in size than the context itself \jc{some concrete numbers here}.
Thus, they require much more network bandwidth to send to the GPUs running the LLM.  
While some emerging methods can shorten context or reduce KV tensor size in GPU memory~\cite{scissorhand,gisting,flexgen,autoencoder-incontext}, it remains a challenge to minimize or control the loading delays of long contexts without impacting generation quality or modifying the LLM.
\end{comment}

%Some emerging research on long-context modeling also tries to the footprint of KV cache in memory or rewriting 
%In short, how to {\em quickly load and process} long contexts remains a challenge.


%However, KV features need significantly more space to store and more network bandwidth to fetch remotely.
%\jc{TODO: need some concrete numbers here.}
%If we quantize the KV features or filter most relevant tokens, the size can be reduced but at a great expense of generation quality.
%An alternative approach is to filter the context and only feed LLM with the most relevant text (\eg~\cite{??,??,??}), but it always degrade generation quality.

%Even if the same GPU serves all prompts of a user, it may be shared with many other users and cannot keep each user's context indefinitely in GPU.

%If we naively feed the long context directly to the LLM, the latency of processing a context in transformer models will grow quadratically with the context length. 
%While we can reduce the context length by sampling only the most relevant part, but doing so often degrade generation quality~\cite{??,??}.
%%it would take too much time to process them before the actual generation starts. 





%In short, existing solutions are remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(2) reduce the context length by sampling only the most relevant part.
%
%
%
%Instead, many LLM systems cache the intermediate processed outcome---{\em key-value features}---of contexts.


%To avoid high inference delay, current LLM systems employ two methods.
%First, they cache the intermediate processed outcome, \ie key-value features, of contexts.
%Compared to directly loading context, this significantly speeds up the inference but it needs much more space to store and much more bandwidth to fetch.
%Alternatively, some works sample contexts and only include the most relevant text in LLM input, but they have to degrade generation quality to reduce the context length.
%As a result, it remains a challenge how to handle long context in LLMs when the long context is loaded on-demand. 

%(1) cache the key-value features of contexts, and 
%(2) sample contexts and only include the most relevant text in LLM input.
%Compared to loading context as text, the former needs significantly more space to store and more bandwidth to fetch, whereas the latter has to degrade generation quality to reduce the context length.

%how to fetch context efficiently to unlock the full potential of LLMs remains a challenge and will likely be more so in the future. 




% ``memory'' cannot always be maintained on a single machine; instead, it is dynamically loaded across different machines via network connections. 
%Similarly, supplementary documents assisting LLM inference might reside in a separate database only to be fetched to the LLM when a query is received.
%Last but not least, 




%To make it more concrete, we perform a measurement the size of key-value features of two different LLMs under two datasets, each including over \fillme tokens.

This paper presents \name, a fast context-loading module for LLM systems, designed for
(1) reducing the bandwidth needed to transmit a context's KV features and 
(2) minimizing the \emph{total} delay in fetching \emph{and} processing contexts, rather than each separately.
% To achieve them, \name entails two components. 

%minimize the delays in fetching and processing long contexts for LLMs.


%This paper presents \name, a fast LLM inference system designed to explicitly reduce the bandwidth needed to transmit the KV cache of long contexts as well as balance the network delay and computation delay.

\name reduces the bandwidth needed for transmitting long contexts' KV features by compressing,
instead of dropping or rewriting, these feature tensors into more compact bitstreams using a new KV encoder. The design of our KV encoder leverages unique properties of KV features across tokens
and layers to achieve high size reduction and little information loss.
It uses a tailored arithmetic coder that takes advantage of KV features' distributional properties, such as locality across tokens; it varies compression strategies across layers of KV features, leveraging the fact that LLM's generation performance has different sensitivities towards the compression losses at different layers of KV features. 
% Unlike other methods that rewrite or shorten contexts, our KV encoding compresses a context's KV features into more compact bitstreams, in order to minimize bandwidth usage.

%It also leverages the fact that different layers of the KV features affect the final generation quality differently, so it applies different quantization levels to different layers.


%For instance, \jc{pick an interesting one to highlight here}
%\name further speeds up the loading of long contexts by pipelining the decompression and GPU memory loading of KV caches in a layer-wise fashion.

With its KV encoder, \name has the flexibility of transmitting a context in different forms, including
KV features in multiple bitstream representations each with a different compression
rate\footnote{The compression is done before a user query arrives.} and
the original raw text, which incurs more LLM processing cost but no decompression cost or information
loss. Right before transmitting a context, \name uses a controller to decide which form to use, flexibly navigating the tradeoffs among LLM generation quality, the transmission
bandwidth, and the decompression cost. It picks the context form that
optimizes the combined cost of transmission and decompression, or the form that
fits in a given time budget with the least information loss.

%\naombined cost of me cthe compresses KV features of a context in multiple bitstream representations, unlike previous methods that shrink KV tensors only once in GPU memory.
% which differs from prior schemes.
%Given a context, 
% To minimize the totally delay in fetching and processing a given context, \name uses a controller to determine when to load the context as compressed KV features or raw text and picks the appropriate compression level if loaded as KV features.
%Note that loading the text context, rather than its KV feature, can sometimes be advantageous if the delay of decompressing KV features exceeds the delay saving of caching KV features.
% It uses a controller to automatically determine the appropriate compression strategy that minimizes impact on the generation quality while not exceeding a delay budget set by the application.
% \name can also choose to fetch the text of a context, rather than its KV features, when the overhead of decompressing and loading it to GPU exceeds the delay saved by caching KV features, particularly of short contexts.

\begin{comment}
    
Second, \name uses a controller to automatically determine the appropriate compression strategy that 
% strikes a desirable tradeoff between generation quality and the delay to fetch and process
balance the network delay (fetching the context) and the computation delay while maintaining high generation quality.
%based on the context length and (optionally) a time budget specified by the application.
%whether to load the context as KV features or raw text, and if loaded as KV features, selecting .
To navigate the tradeoffs between generation quality and delays more flexibly, \name compresses a context at multiple compression levels, which differs from prior schemes.
Notably, when the context is short enough, \name can choose to fetch the context as raw text rather than as KV features.
This is because the overhead of decompressing and loading it to GPU exceeds the delay saved by caching KV features on short contexts.
\end{comment}

Figure~\ref{fig:intro} illustrates \name's benefits.
% reduction in the total delay of fetching and processing a context.
%, which we refer to as the {\em time to first token} ({\em TTFT}) since it reflects the delay between knowing the context and generating the first token for the user.
By compressing KV features to more compact bitstreams, \name significantly cuts the bandwidth usage for KV-feature transfers for long contexts, thus outperforming the baselines that fetch the KV features directly as well as the baseline that loads the text context without the KV cache.
% Leveraging KV cache, \name avoids the high computation delay experienced by the baseline that directly feeds the context to the LLM. 
% Moreover, by compressing KV features to compact bitstreams, \name significantly cuts the bandwidth usage for KV cache transfers, thus outperforming the baselines that fetch the KV cache.
For shorter contexts, \name automatically opts to load the text context directly, rather than its KV features.
%, because it sends less data while maintaining a low computation delay.


\begin{comment}

This paper presents \name, a fast LLM inference system designed for loading long contexts.
\name has three design goals: 
(1) minimizing the network bandwidth needed for transmitting fetch the KV cache of long contexts; 
(2) being able to minimize the impact on the quality of generation without exceeding a targeted loading delay specified by the application; and
%meet a given time budget on the total delay of loading and processing long contexts with minimum impact on generation quality; and 
(3) no need to train a new NN or modify the pre-trained LLM.
To meet these goals, \name entails two key techniques.
%Unlike the recent efforts that reduce the dimensionality of context or key-value features. (\eg~\cite{??,??,??}), \name aims at reducing the communication overhead to meet the application-specified response deadline with minimum impact on generation quality and no modification to the pre-trained LLM.



First, \name reduces the network bandwidth demand of long contexts by compressing their KV caches into compact bitstreams using a new context encoder.
Compared to recent efforts that shrink the KV tensor sizes, our context encoding is more efficient as the encoded bitstreams do not have to be in the form of a tensor.
\name's context encoder leverages a tailored arithmetic coder which takes advantage of KV features' distributional characteristics.
For instance, \jc{pick an interesting one to highlight here}
It also leverages the fact that different layers of the KV features affect the final generation quality differently, so it applies different quantization levels to different layers.
\name further speeds up the loading of long contexts by pipelining the decompression and GPU memory loading of KV caches in a layer-wise fashion.


Second, \name allows LLM applications to set a budget on the time to the generation of the first token (TTFT), which includes the time to load the context into GPU and the additional computation time to process the prompt.
To this end, rather than compressing the context once, \name compresses each context in multiple versions, covering a range of tradeoffs between TTFT and generation quality.
Notably, these versions also include loading the context as raw text, rather than KV features, 
because when the context is relatively short (less than 100s tokens), the overhead of decompressing the KV cache and loading it to GPU exceeds the delay saved by caching KV features.
When given a TTFT budget and an input (context and prompt), \name estimates the distribution of TTFT of different versions of the context using history TTFTs and estimated bandwidth.


\end{comment}

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/intro_perf_short.pdf}
    \tightcaption{\name with the two common practices: loading text contexts directly or loading the cached KV features.
    % \shan{The Y-axis caption is wrong, right? ``Loading'' sounds like network/communication
    % delay only. }
%    Context processing delay of this work vs. existing context-retrieval methods.
    } 
    \label{fig:intro}
\end{figure}

%No individual component of \name is exactly new . 

To put \name's design into perspective, each of its components (adaptive compression and KV cache) may have been studied before. 
%Adapting compression level to navigate size-quality tradeoffs is commonly done in video streaming.
%Quantization and arithmetic coding has been used to in DNN training clusters to compress gradient tensors~\cite{??,??}. 
%Caching KV features is a common trick in LLM services to speedup inference~\cite{??,??}. 
Nonetheless, the exact designs of these components in \name embrace domain-specific insights about KV features and are integrated into an end-to-end system that explicitly minimizes LLMs' network and computation delays regarding context for the first time.

%For a given query (including the prompt and the context), 
%While it is hard to guarantee a delay due to inherent system noise, \name predicts the 
%
%To meet the budget, \name predicts a minimum compression level of the KV cache such that the delay to load the KV cache and compute the cross-attention between prompt and context will not exceed the deadline. 
%To this end, \name will also automatically switch to loading the context as raw text as oppose to its KV cache.
%This is because when the context is short enough, the overhead of decompressing the KV cache and loading it to GPU exceeds the delay saving of caching KV features.

%Unlike the recent efforts that aim at reducing the dimensionality or memory footprint of the key-value tensors, \name compresses key-value caches to bitstreams by leveraging key-value features' distributional properties, such as locality across nearby tokens, custom entropy coding, and layer-specific quantization.
%\jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}

%Second, even retrieving the key-value features, the LLM still needs to calculate the attention matrices (self-attention and cross attention) of each LLM layer. 
%To expedite this process, \name fetch cached key-value features in a layer-by-layer fashion, so that the transferring of features and computation of attention matrices can be pipelined.

%Finally, since loading compressed key-value features involves additional cost, including decompression and loading more data to GPU memory, directly loading the context tokens might sometimes be faster when the context is short. 
%Therefore, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens based on estimated delay of each method. 



\begin{comment}
\name entails three techniques to reduce the size and processing delay of context with only marginal quality degradation. % to significantly accelerate the loading of memory text for LLMs.


First, \name shrinks the size of cached key-value features using a new compression algorithm.
The compression algorithm leverages several domain-specific insights, such as \fillme. \jc{pick an interesting one to highlight here, which should also explain why it has less quality loss as depicted in Figure~\ref{fig:intro}(b).}



Third, since loading compressed key-value features involves additional cost, including decompression and loading more data to GPU memory, directly loading the context tokens might sometimes be faster when the context is short. 
Therefore, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens based on estimated delay of each method. 

%to minimize loading and processing delay under various context length, \name judiciously chooses between loading compressed key-value features and directly loading the context tokens, which might be much faster with short context, depending on the hardware of the GPU machine. 
\end{comment}

%depending on the text input and the inference speed, it is sometimes faster to directly load and process the tokens of context, rather than loading the compressed key-value features which involves additional decompression overhead. 




%To our best knowledge, \name is the first to optimize the communication aspects of LLM with long context, and it complements other efforts aimed at augmenting LLMs with longer context. 
We evaluate \name on three models of different capacities and three datasets of different tasks that use contexts of different lengths.
Compared to a baseline quantization and arithmetic coding scheme that does not consider the distributional properties of KV, \name can save the bandwidth usage for transferring KV features by 3.7-4.3$\times$ and the delays in transferring and processing KV features by 2.7-3$\times$, while maintaining higher LLM performance on various tasks, measured by task-specific metrics such as perplexity and accuracy. Compared to the baseline of
loading text contexts, \name cuts the  latency of processing KV features by 2.8-4.5$\times$ with less than
1\% drop in F1 score or a perplexity score increase of 0.5.
Moreover, at similar task performance, \name also has lower total fetching, processing delays and
higher LLM performance than more sophisticated baselines that modify contexts or retrain models to shorten the contexts. 

% \jc{finally, a paragraph on evaluation highlights. we create a benchmark with \fillme. key takeaways are:
% \begin{packeditemize}
% \item \name can compress the KV caches of long contexts \fillme more efficiently than \fillme at the same perplexity
% \item \name reduces time to generation by \fillme
% \item with the same generation delay, \name can achieve \fillme better quality (perplexity, accuracy)
% \end{packeditemize}
% }


%
%The idea of \name is to compress the key-value features of memory first before retrieving them from remote servers, instead of retrieving them in the form of tensors. \hc{Maybe also mention the potential to make llm inference much faster here?}
%
%Though this idea may seem simple, compressing key-value features is by no means trivial. 
%For instance, quantization is commonly used to reduce footprint of tensors in GPU RAM, but it reduces memory size at the cost of greatly increased perplexity (illustrated in Figure~\ref{fig:intro}(b)). 
%Similarly, arithmetic coding, though lossless, does not yield much compression when applied directly on key-value features. 
%Instead, \name embraces several common patterns of key-value features.
%\jc{list the insights here.}
%Moreover, given a delay target, \name can automatically select the right compression configuration to retrieve maximum amount of memory without violating the delay target. 
%\jc{a few words on this}

 







==> backups/method-v1.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US



\section{\name Design}

\yh{yuhan working on this }


\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
    \tightcaption{Overall workflow of \name. } 
    \label{fig:system}
\end{figure}


\subsection{Overview}

We present \name, a fast context-loading system for LLMs. 
\name has three design objectives:
(1) reduce the network bandwidth usage to load the KV cache of a long context without affecting generation quality; 
(2) no change to the pre-trained LLM or need to train a new model;
(3) the ability to navigate the tradeoffs between TTFT and generation quality.

%In this section, we will describe \name's design in detail. 
To achieve them, \name includes two main components: a context encoder/decoder and a context-loading controller.
Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.
Following the set up of recent works in long-context learning, \name is first provided with the KV features of each context. 
\name then uses the context encoder to compress the KV features of the context into multiple bitstream representations using different compression levels.
When a prompt and its context is received in runtime, the context-loading controller first picks the compression level of the context, fetches it through network, decompresses it and feed it to the LLM. 
%One way to select The compression level is selected 
%determines the compression level of the context such that the resulting TTFT will meet a time budget specified by the application that calls the LLM.


\begin{comment}
before the inference runtime, the context encoding algorithm will compress the key-value cache into bitstreams, with multiple compression configurations.
% \jc{let's dont introduce a separate storage server. it should be just stored where the context is originally stored, right?}
At inference runtime, the context-loading controller will select the right version of compressed key-value cache from the storage server, based on the delay budget specified by the application. 
Then \name will send the compressed key-value cache over the network, decompress them, and feed into LLM inference. 
\end{comment}

% \jc{Yuhan, regarding the terminology, how about we call it "context encoder" and "context-loading controller". the term compressor sounds too much like air compressor :)}


%\subsection{Compressor}
\subsection{Context encoding}

% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
The compression of a KV cache consists of three steps: 
(1) calculate the deltas across consecutive tokens; 
(2) pick the quantization level for each layer; and 
(3) run entropy coding.
Conceptually, these steps may look similar to video coding with each token's KV features being a frame. 
However, the exact design of each step is driven by new observations on KV features produced by LLMs.



\mypara{Cross-token locality} 
Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
We refer to this as cross-token locality. 


\begin{insight}
{\bf{(Cross-token locality)}} Tokens in close proximity have more similar KV features in their values compared to tokens that are further apart.
\end{insight}


\begin{figure}
\centering
     \includegraphics[width=.6\linewidth]{figs/delta_vis.pdf}
    \tightcaption{Visualization of the numerical values of the key features for one layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023}.  } 
    \label{fig:delta_vis}
\end{figure}

\begin{figure}
\centering
     \includegraphics[width=.9\linewidth]{figs/delta_insight.pdf}
    \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. } 
    \label{fig:delta_insight}
\end{figure}

To illustrate, Figure~\ref{fig:delta_vis} provides a visualization of the numerical values inherent to the key features across a single layer. 
The color similarity between two elements directly corresponds to their numerical value similarity. 
As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
This observation shows our first insight: There is cross-token locality in the key-value features.

This observation is intuitive when we consider the meaning of the key-value features.
As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
A crucial aspect of the self-attention mechanism is that the key and value features for a given token position are calculated based on the key-value features of \textit{all} preceding tokens.
This mechanism inherently leads to numerical similarity in the key and value features of \textit{nearby} token positions.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 
\begin{figure}
\centering
     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
    \tightcaption{Proposed scheme to utilize cross-token locality. } 
    \label{fig:delta}
\end{figure}

To utilize this cross-token locality, we propose that instead of compressing the raw key-value features directly, we partition the tokens within a context into multiple chunks. 
For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
Figure~\ref{fig:delta} is an illustration of our proposed approach. 
Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 
Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the raw key-value features versus compressing the deltas with different levels of quantization. 
As we can see, compressing the deltas achieves a better tradeoff than compressing the raw key-value features. 

% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
\mypara{Picking level of quantization}
When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
The quantization level is defined as the size of the integer. 
For instance, in the case of an 8-bit quantization level, we rescale the original floating-point tensor to fit within the range of $[-2^7, 2^7]$. 
This rescaling is achieved by dividing $2^7$ by the absolute maximum value present in the floating-point tensor.

A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 

\begin{insight}
{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the deeper layers than to those in the shallower layers.
\end{insight}

To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 

To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
This can be both time and resource-consuming.
Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).

In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  

% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\mypara{Arithmetic coding} In order to further reduce the network bandwidth usage for transferring the \kv, we  apply \textit{arithmetic coding}~\cite{ac} (AC) on top of the two previous schemes. 
AC is a widely-used technique used to compress the input into bitstreams.
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.



A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\begin{insight}
{\bf{(Impact of channel, layer, and token position)}}
In a KV cache, each value is distinguished by its channel, layer, and token position. However, the information gains from its channel and layer are significantly higher than from its token position.
\end{insight}


Thus, in our encoder, we use a  per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

\begin{figure}
\centering
     \includegraphics[width=.9\linewidth]{figs/ac.pdf}
    \tightcaption{How different groupings of segments in key-value features affect the entropy. } 
    \label{fig:ac}
\end{figure}
% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.




\subsection{Controller}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.

Specifically, we formulate the goal of the controller as minimizing generation quality degradation, compared to no compression, while meeting the time budget. 

In order to achieve this, \name maintains different versions of compressed \kv.
The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 
As seen in Figure~\ref{fig:??}, beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 
Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
It then selects the \kv version that fits within the time budget while maximizing its size. 

%\subsection{Putting all together}
%\yh{todo}
\jc{no need for a separate putting it together subsec}

\subsection{Implementation}
\begin{itemize}
\item basic library info: how many lines of code (a github link?)? ac? quantization? 
\item integrate with existing apps: how to obtain kv features of a context offline
\item interface with LLM: e.g., how to get kv features, how to feed kv features
\item any optimization to improve compression/decompression speed
\end{itemize}

% \yh{Use a figure to show that it's better to compute the context's self-attention on the fly with the texts, when  the number of input tokens is small. }

% Also, \yh{say a few sentences that different compression configurations form a tradeoff in quality and size. }
% \name maintains a database of key-value caches. 
% For each cached context, \name stores several versions of key-value caches, with different compression configurations.
% \name's controller also profiles the delay and quality tradeoffs for each of the compression configurations.
% The profiling of different compression configurations allows \name to navigate through the quality and size tradeoff. 
% Once the application specifies a delay budget, \name 
% selects the compression configuration that reaches the delay budget with the maximum generation quality, which is typically the most conservative compression configuration below the budget. 

% \name profiles the delay for different compression configurations for each 

% As an illustrative example, we plotted the 

==> backups/method-v10.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

We now present the design of \name, a concrete KV cache streamer for fast context-loading in LLM inference systems.
%, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
%\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

\begin{comment}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\end{comment}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

% \tightsubsection{Context KV encoding}
\tightsubsection{KV cache encoding}
\label{subsec:encoding}
% \yh{Jumps too much from previous }
% \yh{Emphasize the similarity with video coding. 
% Before starting change-based encodingxxx, start by saying why blindly applying video techniques is not ok.

% move the  insights in one zone.

% Mention this is empirical observation. 

% What we have is a representative dataset? 
% }

% \shan{Again, where is this discussed? I guess it should be in Section 2.1, but currently Figure 1
% is not well explained in that sub-section.}
% Recall from \S\ref{sec:delay} 
% that a KV cache of a context contains two tensors (K and V) of the same shape: 
% $[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ are the number of tokens, layers, and channels, respectively.

At high level, for any context, \name compresses the K and V tensor of its KV cache in three steps: 
\begin{packedenumerate}
\item calculate the {\em delta tensors} (defined shortly) between the KV cache of nearby tokens; 
\item apply different quantization to each layer of the delta tensors; and 
\item run the arithmetic coder on the quantized delta tensors.
\end{packedenumerate}
% \yc{Is delta tensor defined anywhere? It's not clear what's a delta tensor.}


These steps of compressing KV cache to a bitstream are conceptually similar to video coding, which transforms from pixels to an encoded bitstream.
It also first computes the delta between two nearby frames and then quantize them before encoding the result with arithmetic coding~\cite{cabac}.
%Here, the delta between two nearby frames (\textit{e.g.}, motion vectors and residuals) are quantized and then encoded with arithmetic coding~\cite{cabac}.
%In KV cache compression, each token's KV cache is similar to a frame in video coding.
%can be seen as a frame. 
% where each token's KV cache can be seen as a frame. 
Yet, blindly apply existing video codecs may not work well since they are optimized for pixel values in natural video content. 
Instead, the exact design of \name is inspired by domain-specific insights on KV cache produced by LLMs.

Specifically, \name leverages the following empirical observations on KV cache.
% the insights we empirically find in the KV cache include: 
\begin{packedenumerate}
    \item \emph{At the same layer and channel, tokens in closer proximity have more similar KV cache values compared to tokens that are further apart.}
    \item \emph{In a KV cache, each element is distinguished by its channel, layer, and token index. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.}
\item \emph{The output from the LLM is more sensitive to losses in the KV cache values of the shallower layers than to those in the deeper layers.}
\end{packedenumerate}


Next, we will explain each step of \name's KV cache encoder and its rationale. %and insight along with the rationale behind it.


%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}  Our first insight is about the similarity between KV cache values of nearby tokens.
This {\em token-wise} locality 
%Why do KV features have such \emph{token-wise} locality? It does
%not necessarily mean nearby tokens themselves are similar
%or more correlated (and they are not). Rather, it 
stems from
the transformer (the self-attention) mechanism that computes the KV
cache. In essence, the K/V tensors \shan{What is the right terminology
here? If we have defined KV cache to be a 3-D tensor, saying `KV cache' of an individual token is wrong. We have used this `KV cache' phrase many times. Please settle down on the right terminology and use it consistently.} of a given token
% \shan{token or token index? Are they the same thing? If they
% are the same, please use one consistently.}
are calculated based on the KV cache of previous tokens\footnote{More strictly, the KV cache are generated in a layer-by-layer manner. The KV of token $t$ at layer $i$ is computed based on the attention matrix 
 from all the previous tokens' attention matrix at the previous layer~\cite{vaswani2023attention, attention2}.}.
%Particularly, we observe that:

%that if two tokens' positions are near to each other in the context, their KV feature values at the same channel and same layer are similar.

% \begin{insight}
% %{\bf{(Token-wise locality)}} 
% At the same layer and channel, tokens in closer proximity have more similar KV cache values compared to tokens that are further apart.
% \end{insight}



% \jc{i know it's technically correct, but like you said many time, the conventional understanding is that KV is computed layer by layer, not token by token. it seems this claim is essential to the locality observation, can you add some text to explain it and also find any citations to back it up?}
% This dependency inherently leads to numerical similarity in their KV features across \emph{nearby} tokens in a context.


\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.7\linewidth]{figs/delta_insight.pdf}
    \tightcaption{\yh{Replace with real}} 
    \label{fig:delta_insight}
\end{figure}


This token-wise locality suggests an opportunity for better compression without affecting :
\yc{Yuhan, I feel like ``without affecting generation quality'' is a bit vague here. I can understand why we can have more efficient compression by reading the text below, but it's not clear why it does not affect the generation quality.} 
the values in the original KV tensors\shan{terminology: what is
the difference between KV cache and KV tensors?}
% given one channel and layer,\jc{i don't think we really need to stress that it's a given channel or layer, do we?} 
tend to span a wider range with a higher variance than 
%However, if we compute 
the \emph{delta} between every pair of nearby tokens at each layer and channel.
%, the distribution of the deltas will have a much smaller variance.
This trend is shown in 
Figure~\ref{fig:delta_insight}.
\shan{Yuhan, I simplified the original sentence.
You need to add some methodology information here to explain 
how you get this figure.}
%shows that at a particular layer and channel, the distribution of original KV values has a much lower variance than the distribution of the delta values between two nearby tokens.
% the cumulative density function (CDF) of the original and delta KV features for one channel and one layer.
% As we can see, the delta KV features has smaller variance than the original ones. 

\shan{This paragraph is very poorly written. I don't understand
any one of the sentences here.
If there is a well-known ``theory'', tell people what is that
theory. Or, tell people more convincing/concrete/intuitive argument.
}
\yh{Maybe say that quantizing into the same number of bits, smaller variances will have smaller entropies. }
Since the distribution of delta values has a low variance and a mean around zero, it is well-known that it can be quantized and encoded to achieve a desirable size-loss tradeoff~\cite{doi:10.1080/03610928608829122}\shan{I don't understand the logic here. 1. Why does the `mean around zero' 
matter? Even if the mean is 10000, as long as the variance is small, isn't it the same? 2. How do you define `desirable'?
Depending on your usage scenario, it is possible that no
desirable size-loss tradeoff exists.}.
Specifically, most delta values are close to zero, so our quantization step (explained soon) can quantize them into a few distinct values with minimum information loss\shan{Again, why does
close to zero matter? If all my data is in between 100001 and 100001.01, isn't that good enough?}.
This results in a highly skewed distribution \shan{what does highly ``skewed'' distribution mean?} with low entropy, leading to a small-sized bitstream after the arithmetic coding (explained soon) 

Since the quantized delta tensors and original tensors are close to normal distribution 

has a low variance and they are, it is a well known conclusion that distributions with lower variance yield lower entropy  for normal distributions. 





%, the distribution will have a small bitstream size. 

% \jc{yuhan, i rewrote the paragraph to simplify and smooth the text. please feel free to revert or edit the new text}
% If a distribution has smaller variance,
% it can be more easily compressed and has better size vs error tradeoff 
%  for reduced entropy~\cite{doi:10.1080/03610928608829122}.
% Intuitively, for a distribution with a smaller variance, there will be more repeated symbols in the data distribution after compression, specifically after non-uniform quantization (details in a later section). 
% These repeated symbols can be encoded with fewer bits, thereby reducing the overall size post-compression. Additionally, despite the reduced size, the error introduced by quantization remains minimal. To illustrate this, consider a quantization scheme that divides a distribution into two bins: one for values between 0 and 1, and another for all remaining values, with the quantized value being the bin's mean.
% For instance, a distribution like $[0.1, 0.5, 0.8, 1.5, 3]$ is quantized to $[0.7, 0.7, 0.7, 2.25, 2.25]$ resulting in an entropy value of 0.97. In contrast, a distribution such as $[0, 0.1, 0.2, 0.3, 1.2]$, which is quantized into $[0.15, 0.15, 0.15, 0.15, 1.2]$, this has an entropy of 0.72. 
% Moreover, the quantization error rates for these two distributions are 0.3 and 0.01, respectively.
% Thus, the repeated symbols can be represented with fewer bits, size after compression will be smaller. 
% Moreover, even though having smaller size, the error due to quantization will still be low. 
% As a simple illustrative example, consider the quantization scheme that bucketize a distribution into 2 bins, where values in between 0 and 1 into one bin, and other values into another, with the quantized value as the mean in the bins.
% If one distribution is $[0.1, 0.5, 0.8, 1.5, 3]$, the quantized values are $[0.7, 0.7, 0.7, 2.25, 2.25]$, leading to a entropy value of 0.97. 
% As for another distribution $[0, 0.1, 0.2, 0.3, 1.2]$, which is quantized into $[0.15, 0.15, 0.15, 0.15, 1.2]$, this has an entropy of 0.72. 
% Furthermore,  the error rate for the quantized data for the two is 0.3 and 0.01, respectively. 


% Since distributions with smaller variances have lower entropy\footnote{As the KV features is a normal distribution, many prior works have proved that smaller variance leads to lower entropy~\cite{??, ??, ??}. }, compressing the delta tensors instead of the original ones will be more beneficial. 

To utilize this token-wise locality of feature values, 
we employ the following idea: 

We partition all the tokens of a context into groups of ten contiguous tokens. 
In each group, we compress the KV cache of the first token, called the {\em anchor token}, independently (\ie without comparing it with other tokens), and then compress the delta tensor between each remaining token and the anchor token's decompressed features\footnote{Note that we compute the delta tensor between each remaining token and the \emph{decompressed} anchor token, so that the compression and decompression of remaining tokens in the group share the same reference to decode them. }. 


This process is analogous to video coding, where it also partitions the frames into groups of contiguous frames. 
However, we are different from video coding in that we do not compress the delta between each pair of consecutive tokens, like in video frame encoding, because by comparing all tokens with the same anchor token in one chunk, we can greatly parallelize the compression and decompression of many tokens.
% \yh{The similarity should }
Second, the tokens within a chunk may not change as smoothly as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 
\yc{``change as smoothly as between two consecutive frames'' is vague. What do you mean by ``smooth''? Can we say the distribution of the delta tensor is similar?} \yh{The distribution after delta is similar ==> size after compression will be similar. }

\yc{Should we first talk about quantization then arithmetic coding? Because the workflow is computing delta -- quantization -- arithmetic coding}
\yh{Will do. }

% \begin{figure}
% \centering
% %     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
%      \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{An example of KV values at the same layer and same channel across tokens.
%     We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
%     % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
%     % \jc{drop blue. and extend red to a wider range}
% %    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
% \shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
%     } 
%     \label{fig:delta_vis}
% \end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}


\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
Next, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.
As shown in Figure~\ref{fig:kvcache-illustrated}, the KV cache include $l$ layers of K/V tensors, and 
each layer of the K/V tensor is a two-dimensional
vector of the shape 
%For each layer, the key is a 2-D tensor of shape 
$[N, c]$, where $N$ is the number of input tokens and $c$ is the number of channels in the LLM. 

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads, since we need to store $\NumTokens\times\NumLayers\times\NumChannels$ distributions on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping.
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext}, which is a popular dataset to evaluation LLM's generation quality~\cite{llmint8, smoothquant, scissorhand}, and use the Llama-7B model to produce the KV cache tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
We can see that entropy for grouping the tensors by channel and layer is lower than that of grouping by  token position.
\yc{Figure~\ref{fig:ac_insight} is a bit hard to understand. For example, what's the meaning of each bar? What does 400 mean in Channel400?}
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
% We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

% \begin{insight}
% %{\bf{(Information gain)}}
% In a KV cache, each element is distinguished by its channel, layer, and token index. 
% The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
% \end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV caches produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
% \yh{Earlier and later layers }
So far, the compression (running AC on delta tensors) has been lossless.
To further reduce the bandwidth usage of transferring the KV cache, \name also drops some information from the tokens while minimizing the impact on LLM's performance.
Specifically, \name uses quantization to reduce the precision of the elements in a KV cache so that they can be represented by fewer bits. 

% Recent methods propose to drop some tokens from the context~\cite{liu2023scissorhands,gisting,zhang2023ho}, but they must know the query (the prompt) to obtain the self-attention scores. 
% In contrast, we want to compress the KV feature before the query arrives. 
% \shan{this related work
% has been mentioned before, right? Can we not mention them again and again and again?}


% There are two potential approaches to dropping information. 

% One is to drop some tokens ()\jc{Yuhan, Ari seems to suggest there are many works in this space. can you add more related work and maybe update this statement}, but to determine which tokens are more important than others, they often assume knowledge of the query (the prompt part) of the input, because the important tokens are typically dependent on what the prompt is asking. 
% We do not take this approach because we want to compress KV features offline without seeing the prompt to avoid compression delay in TTFT.

%ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
%There are two potential approaches.
%
%First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
%However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

%\name applies a specially designed quantization scheme that minimizes the impact on LLM's performance.

%This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}, but all elements are uniformly quantized with the same number of bits without leveraging any distributional properties of KV cache.
%in~\cite{flexgen} to trade generation quality for memory footprint of KV features.
%Yet, it uniformly quantizes all elements of KV features with the same number of bits. 
It remains unclear what a better quantization strategy is to compress KV cache while minimizing the impact on LLM's performance.

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
Specifically, later layers are less sensitive to the losses in KV cache than earlier layers. 
%shallower layers are more sensitive to quantization. 
%Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
%We can summarize this insight as follows.

% \begin{insight}
% %{\bf{(Layer-wise sensitivity)}}
% The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
% \end{insight}

%Intuitively, shallower layers (closer to input) in LLMs indicate basic  (\eg basic sentence structure), while deeper layers extract more abstract features~\cite{egeria, ???}. 

Intuitively, KV cache at the later layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV cache of the earlier layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the early-layer cache can propagate and affect the later-layer cache and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}
Driven by this insight, we apply less aggressive quantization (more bits) on the delta tensors of earlier layers. 
Specifically, we split the transformer layers into three layer groups, the first (earliest) 1/3 of layers, the middle 1/3 of layers, the last 1/3 of layers, and apply different amount of quantization bin size on the delta tensors at each layer group, respectively. 
The size of the quantization bin grows larger (\ie larger quantization errors)
from earlier to later layer groups. 
% Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
% Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers,
% and apply $x$-bit, $y$-bit, and $z$-bit quantization on the features at each layer group, respectively.
% % and apply $x$-bit quantization on the first (shallowest) 1/3 of layers, $y$-bit on the second 1/3 of layers, and $z$-bit on the last 1/3 of layers.
% Each combination of $(x,y,z)$, where $x\geq y\geq z$, represents a tradeoff between compression size and loss of the LLM performance and \S\ref{subsec:controller} will explain the exact settings of quantization levels used in \name.

Note that we still use 8-bit quantization, a relatively high precision, on the KV cache of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it makes sense to preserve higher precision just on these anchor tokens.

%We would like to  that though the quantization settings are empirically picked, they work well across a range of LLM models and datasets (\S\ref{subsec:sensitivity}), and future work can refine the quantization scheme.

% not the only way
% AC is recalculated

%With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
%\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
%In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 
%
%To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
%This can be both time and resource-consuming.
%Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
%First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
%Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
%This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).
%
%In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  



% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}

\input{fig-adaptation-case}

\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}

% \yh{Not clear how we stream? 

% Pseudocode 

% drop the equation 
% }



%The transmission of a KV cache can take from hundreds of milliseconds to a few seconds, during which the network bandwidth may fluctuate.
Since the transmission of a KV cache may take up to 100s of milliseconds to a few seconds, the available bandwidth may fluctuate during a transmission. 
%During the transmission of one context, throughput change can happen as it may take hundreds of milliseconds or several seconds to complete.
Thus, streaming the encoded KV bitstreams at a fixed encoding level\jc{is it compression level or encoding level? please be consistent} may violate a given service-level objective (SLO) of fetching the KV cache.\footnote{In practice, SLO is defined on TTFT. We use SLO for fetching KV cache because once the KV cache of the long context is loaded in GPU, the remaining delay to generate the first token is marginal~\cite{??}.}
In Figure~\ref{fig:adaptation-case}, for example, 
% The throughput drops from 2~Gbps to 0.2~Gbps at 1 second, lasting for 2 seconds, then increases to 1~Gbps, during the transmission of one context. 
at the start of the transmission, the available throughput 
%\footnote{In datacenters, the network bandwidth can achieve 10~Gbps to 100~Gbps}
is 2~Gbps, and if the bandwidth remains at 2~Gbps, sending a KV stream of 1~GB can meet the SLO of 4~seconds.
% given an encoded KV cache of 1~GB and a latency SLO of 4 seconds, transmitting the encoded KV cache will be able to meet the SLO. 
However, at $t=2s$, the throughput drops to 0.2~Gbps and only increases to 1~Gbps at $t=4s$, so the actual transmission delay increases from 4 seconds to 7 seconds, which violates the SLO.

\jc{yuhan, i change the def of context chunks to a chunk of text, rather a chunk of kv bitstream, and each context chunk will be encoded independently into kv bitstreams using the kv encoder. i felt it's more natural. do you agree?}

\mypara{Workflow}
To handle changes in available bandwidth, \name splits a context into multiple {\em context chunks} (or {\bf chunks} for short) of consecutive tokens\footnote{A context chunk may contain multiple {\em groups of tokens} used by the KV encoder to calculate delta tensors (\S\ref{subsec:encoding}).} and uses the KV cache encoder to encode each chunk into multiple bitstreams of different encoding (quantization) levels that can be decoded independently (explained shortly).
This can be done offline. 
When fetching a context, \name sends these chunks one by one, and each chunk can choose one of several {\em streaming configuration} (or {\bf configurations} for short): it can be sent at one of the encoding levels or can be sent in the text format to let the LLM recompute K and V tensors. 

\name adapts the configuration of each chunk while streaming the KV cache to keep the transmission delay within an SLO. 
Figure~\ref{fig:adaptation-case} illustrates an example adaptation where 
%As shown in Figure~\ref{fig:adaptation-case}, to start with, \name decides to send the KV cache. 
\name switches to sending text context and recomputing KV cache from the text at $t=2s$ due to the bandwidth drop, and at $t=4s$, since the bandwidth increases back to 1~Gbps, and \name switch to sending KV bitstreams of subsequent chunks at smaller size. 
With adaptation, \name is able to meet the SLO. 


%At a high level, it splits the KV cache for one context into several \emph{context chunks}, and send the context chunk by chunk.
%Based on the throughput, with the objective of meeting the SLO, \name can adapt the configurations independently for each chunk. 
%The configurations include whether to switch between compression levels of \name's encoded KV caches, or fall back to generate the KV cache from text context from scratch.

% This is based on two insights. 
% First, 
% even if the compression level is different for different chunks, the decoded KV caches are tensors of the \emph{same} shape. 
% Thus, they can be concatenated. 
% Second, the nature of how KV cache is constructed enables the KV cache for one specific chunk to be constructed based on the text of this chunk and the KV cache of all the previous chunks~\cite{dai2019transformer, vaswani2023attention}. 

To adapt efficiently, several questions remain.

%Two of the key questions in the adaptation module lie in how to split the whole context into chunks, and how to adapt to bandwidth fluctuations. 
%The context chunks are created by splitting the key tensor into chunks such that each chunk contains the key tensors for multiple contiguous tokens, and similarly for the value tensor. 
%Each of the chunk contains the number of tokens which is just large enough to fit in one congestion window size, for two reasons.
%One, we want to best utilize the bandwidth by filling up one congestion window, while on the other hand, we also want to provide fine-grained enough granularity to perform 
%adaptation to meet SLO. 
%Note that we also  let the number tokens in one context chunk be integer multiples of the number of tokens in one group in the change-based encoding (\S\ref{sec:}).

% The chunks make the decisions of switching between compression levels or generating KV cache from scratch 

First, {\em how to stream multiple chunks at different streaming configurations without affecting compression efficiency?}
%decode each context chunk independently?} Specifically, why encoding each context chunk separately does not affect compression efficiency
To encode the chunks offline, \name first computes the KV cache of the entire context (\ie prefill) and splits the K and V tensors of the KV cache along the token dimension into sub-tensors, each of which contains the layers and channels of the tokens in the same chunk.
It then uses the KV encoder to encode the K or V sub-tensor of a chunk with different encoding (quantization) levels. 
Each chunk is encoded {\em independent} to other chunks {\em without} affect the compression efficiency as long as a chunk is longer than a group of tokens.
This is because encoding the KV tensor of a token only depends on itself and its delta with the anchor token of the group of tokens (\S\ref{subsec:encoding}).
Thus, chunks sent with different encoding levels can be independently decoded and then concatenated to reconstruct the KV cache. 
In the case that a chunk is sent in text format, the LLM will compute its K and V tensors based on the previous chunk's KV tensors that have been received and decoded.\footnote{A similar concept has been used to split LLM input into prefill chunks for more efficient batching~\cite{sarathi}.}

{\em Would streaming chunks at different configurations affect generation quality?}
If one chunk is sent at a lower encoding level than other chunks\jc{do we call aggressive compression a low or high encoding level?} (due to low bandwidth), it will have high compression loss on {\em that} single chunk, but this will not affect the compression loss of other chunks. 
That said, we acknowledge that if the bandwidth is too low to send most chunks in a high encoding level, the quality will still suffer.


 
%In order to adapt the configuration for each chunk, 
%in the offline stage, we encode each chunk of the KV cache into multiple compression levels, specifically by varying the quantization parameters\footnote{\yh{talk about the parameters }}. 
%The reason why we can encode each chunk separately is that the size of encoding each chunk is the same as encoding the whole KV cache.
%Specifically, since encoding each token depends only on the anchor tokens in the same group (see \S\ref{sec:method}), and we only use different quantization levels for different layers, this chunking will not affect the encoding procedure. 
%% The different versions of encoded KV cache lead to a tradeoff in LLM generation quality and size. 
%Each chunk also has the option of falling back to generating KV from scratch (implementation see \S\ref{subsec:impl}).


Second, {\em how long should a context chunk be?}
We believe that the chunk length depends on two considerations. 
\begin{packedenumerate}
% \item Since the next chunk's configuration is decided after the previous chunk is received, the encoded KV bitstream of a chunk should not be smaller than the sender's congestion control window or we would not fully utilize the network bandwidth.
\item The encoded KV bitstream of a chunk size should not be too big because, otherwise, it cannot react to bandwidth changes in a timely manner.
\item The chunk should not be too small either. If we choose to send a chunk in the text form, the LLM cannot be fully utilized to compute the KV tensors.
\end{packedenumerate}
With these considerations in mind, we empirically pick \fillme tokens as the default chunk length in our experiments\footnote{The chunk length is also long enough for the KV bitstream of each chunk to fill the sender's congestion window in our experiment setting.}, though more optimization may find better chunk lengths.

Finally, {\em how does \name decide the streaming configuration of the next chunk?}
\name chooses the configuration for the next chunk based on the measured throughput when sending the last chunk.
Specifically, \name first assumes the same throughput will remain and calculates the expected delay of each streaming configuration if it is applied to all remaining chunks. 
The delay of sending an encoded KV bitstream is calculated by dividing its size by the throughput (more details in \S\ref{sec:appendix}).
% It then picks the configuration that has the least compression loss (\ie text format or lowest encoding level) with an expected delay still within the remaining time before the SLO, and uses the configuration to send the next chunk.
It then picks the configuration that has the least compression loss (\ie text format or lowest encoding level) with an expected delay still within the SLO, and uses the configuration to send the next chunk.
%Specifically, if the delay to generate KV cache from scratch does not meet the SLO, \name will select the compression level that yields the highest generation quality without violating SLO. 
%Otherwise, \name will fall back to generate KV cache from scratch. 
For the first chunk, if some prior knowledge of the network throughput is available, \name will use it to choose the configuration of the first chunk the same way.
Otherwise, \name starts with \fillme (a medium encoding level). 
%The detailed adaptation logic can be found in \S\ref{sec:appendix}. 

%When sending the first chunk, without much information about the network bandwidth, \name starts with \fillme (a medium encoding level). 
%If some prior knowledge of the network throughput is available, it can be used 
%by sending the first chunk of the KV cache at the compression level with a middle-level size and the entire text context. 
%Upon receiving each chunk, \name chooses the configuration for the next chunk based on the empirical throughput of the last chunk. 
%Concretely, if the delay to generate KV cache from scratch does not meet the SLO, \name will select the compression level that yields the highest generation quality without violating SLO. 
%Otherwise, \name will fall back to generate KV cache from scratch. 
%Note that even if \name may choose the version of encoded KV cache yielding the worst generation quality for one context chunk, we empirically find that the final generation quality will not be significantly affected if the number of chunks sent in low quality is not substantial (see \S\ref{sec:??}).




% \begin{equation*}
% \begin{cases} 
% \text{use text to recompute} & \text{if } T_{\text{text}}(L_{\text{rt}}, L_{\text{ct}}) < SLO, \\
% \underset{Q}{\mathrm{argmax}} \text{ s.t. } T_{\text{kv}}(L_{\text{rt}},Q) < SLO & \text{otherwise.}
% \end{cases}
% \label{eq:adapt}
% \end{equation*}

% In the equation, $L_{rt}$ is the number of tokens yet to be received, $L_{ct}$ is the number of tokens that have already been received. The function $T_{kv}(L_{rt}, Q)$ \footnote{$T_{kv}(L_{rt}, Q) = \frac{\alpha \times Q \times C \times L_{rt} \times L}{Throughput} + RTT$, $\alpha$ is a constant of the model} predicts the delay for transmitting a KV cache with $L$ tokens at compression level $Q$, while $T_{text}(L_{rt}, L_{ct})$ \footnote{$T_{text}(L_{rt}, L_{ct}) = \gamma L_{ct} \times L_{rt}^2$, $\gamma$ is a constant of the model} predicts the delay for generating the KV cache from text. 

% Our adaptation logic chooses the compression level that is predicted to deliver highest quality within the SLO.
% Note that we use the throughput detected by the previous chunk to predict future throughput. While this approach may introduce some error to prediction, the performance stays strong (see \S\ref{sec:??}\hc{Yuhan plz fill}) since datacenter network bandwidths are relatively stable.

% \yh{Several comments: 1. need to explain SLO clearly. 2. split into context-chunks, send chunk-by-chunk, each chunk can make  several actions independently based on throughput to adapt to SLO. 3. how to determine chunk size? How to encode it into several chnks? }


% \jc{i commented out the algorithm pseudocode. it's causing a lot of latex errors, and i don't think we really need a pseudocode to explain it. if it can be clearly explained in fewer words, please do that. a pseudocode is usually a sign that the idea is really complicated}
% \begin{algorithm}
% \caption{Get Function Algorithm}\label{alg:sender}
% \begin{algorithmic}[1]
%     \State $remaining\_SLO \gets SLO$
%     \State $all\_KV \gets None$
%     \For{$i \in \{1..N\}$}
%         \State $is\_text, kv\_quality \gets \Call{GetNextQuality}{i, throughput, remaining\_SLO}$
%         \State $all\_KV \gets all\_KV + \Call{GetNextChunk}{is\_text, kv\_quality, i}$
%     \EndFor
%     \State \Return $all\_KV$
% \end{algorithmic}
% \end{algorithm}




% %So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
% Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
% In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
% To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% % , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.





% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

% First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
% %, with larger compressed sizes generally resulting in higher TTFT but better quality.
% %As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
% By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
% The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
% %Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
% Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

% We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
% We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.


% %By default, we \jc{explain the default levels here.}


% %\shan{Please remind readers that the compression is done in
% %the background and hence not part of the TTFT, although
% %decompression is part of TTFT.}
% %The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

% %\jc{need to explain why kv can be compressed offline and refer to the limitation section}

% %beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

% In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
% \begin{align}
% {\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
% \label{eq:prediction1}
% \end{align}
% The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
% %\hc{provided bandwidth in data center?} 
% The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
% The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
% %$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


% In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
% \begin{align}
% {\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
% \label{eq:prediction2}
% \end{align}
% The first term is the round-trip-time (RTT) between the storage server and the GPU server.
% We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
% The second term is the GPU computation to compute the attention from scratch.

% With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
% If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


% The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
% In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% % \todo{Show analytical model to predict ttft here. }


% %When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
% %\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
% %\begin{align}
% %TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
% %\label{eq:prediction}
% %\end{align}



% %Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

% %At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
% %If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
% %It then selects the \kv version that fits within the time budget while maximizing its size. 

% %In addition to different compression levels, we also include the option of raw text of each potential context document. 
% %Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
% %decompression time would outweigh the computation time on
% %short text contexts.
% %
% %\jc{remember to explain why picking the compression level doesn't depend on the prompt}

% %\subsection{Putting all together}
% %\yh{todo}
% %\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, about 1K lines of CUDA kernel code, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
% We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
% Particularly, we use its encoding and decoding functions to perform AC. 
To speed up encoding and decoding, we implemented a GPU-based AC library with CUDA.
\yh{talk to qizheng about implementation of gpu-based encoder}
Specifically, for decoding each CUDA thread is responsible for decoding the KV cache from bitstreams for one single token. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Integration into LLM inference framework} 
\name operates the LLM through two interfaces
\begin{packeditemize}
    \item \texttt{calculate\_kv(prompt) -> KVCache}: given a new prompt, \name invokes LLM through this function to get the corresponding KV cache.
    \item \texttt{generate\_with\_kv(KVCache) -> text}: \name passes the KV cache to LLM and lets it generate the new text while skipping the attention computation.
\end{packeditemize}
We implemented the above two interfaces for HuggingFace models using \texttt{transformers} library~\cite{???} with \fillme lines of Python code.
Both interfaces are implemented based on the \texttt{generate} function provided by the library.
To ensure LLM only calculate the KV cache without generating new text, we pass \texttt{max\_length} \texttt{= 0} and \texttt{return\_dict\_in\_generate} \texttt{=} \texttt{True}. 
The \texttt{generate\_with\_kv} is implemented by simply passing the KV cache through the \texttt{past\_key\_values} argument when calling the \texttt{generate} function.
Similar integration is also applicable to other LLM libraries, such as \fillme, \fillme, and \fillme.

We then integrate \name into LangChain~\cite{langchain}, a popular framework for building LLM applications.
\name is activated in the \texttt{\_generate} function of LangChain's \texttt{BaseLLM} module. 
\yc{Yuhan, please help check the correctness of the following workflow}
If the KV cache of the current prompt already exists inside \name, it will invoke \texttt{generate\_with\_kv} to start generating new texts.
Otherwise, \name will first invoke \texttt{calculate\_kv} to get the KV cache before generating new texts.
%Specifically, \name acts as a plugin module, receiving the input prompt, managing the loading of the KV cache, and calling the LLM to generate the response while bypassing the attention computation.
%Thus, \name requires the underlying LLM to provide two interfaces:
%(1) given a new prompt, LLM calculates the KV cache and return it to \name, 
%and (2) given the KV cache (provided by \name), LLM resumes the inference while skipping the attention computation.
%Many recent LLMs support the two functionalities by default. 
%For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
%\name interacts with LLM inference via two simple interfaces:
%% To apply \name, the model inference pipeline to have incorporate two functionalities: 
%(1) \name extracts the KV features of a given context from an LLM inference, and 
%(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
%Many Pytorch-based LLMs support these APIs. 
%For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.

% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name} To speed up the decoding of KV cache in GPU, we pipeline the transmission of context chunk $i$ with the decoding of context chunk $i-1$(explained in \S\ref{subsec:controller}). 
 
% To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.


==> backups/method-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US



\section{\name Design}

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
    \tightcaption{Overall workflow of \name. } 
    \label{fig:system}
\end{figure}


\subsection{Metrics and objectives}

\mypara{Delay metric}
We focus on {\em time-to-first-token (TTFT)}, defined by the time between knowing the input (the prompt and context) and generating the first token. 
While LLM systems may also reduce the total generation delay (the sum of TTFT and the delay to autoregressively generate response tokens), we choose not to use this metric  because 
(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
(2) we want to focus the delay reduction on processing input faster, not by generating fewer tokens.

Since the context resides in a different machine than the GPUs running the LLM, the TTFT delay consists of 
(1) the {\em communication} delay to fetch the context to GPU memory and 
(2) the {\em computation} delay to process the context and prompt before generating the first token.


\mypara{Quality metric}
We then define {\em generation quality degradation} by how close the generated text under any speedup of input processing is to the text generated when letting the LLM process the context and the prompt from scratch, which is the unoptimized implementation. 
In other words, generation quality degradation measures the impact of speedup on generated text.
If the speedup of input processing does not change the generated output, the quality will be the highest, but sometimes the speedup is achieved by dropping information, yielding a different generation text.

Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
\S\ref{subsec:eval:setup} will describe these metrics in more detail.

\mypara{Objectives}
With these definitions, the objective of this paper can be formulated as follows.
{\em How to minimize the TTFT delay with minimum generation quality degradation?}
Essentially, all methods, including ours, strike some tradeoffs between TTFT delay and generation quality.
Thus, in practice, we will show our improvement by comparing the TTFT delay of two methods under the same generation quality degradation.


\subsection{Overview}

We present \name, a fast context-loading system for LLMs. 
\name has three design objectives:
(1) reduce the network bandwidth usage to load the KV cache of a long context without affecting generation quality; 
(2) no change to the pre-trained LLM or need to train a new model;
(3) the ability to navigate the tradeoffs between TTFT and generation quality.

%In this section, we will describe \name's design in detail. 
To achieve them, \name includes two main components: a context encoder/decoder and a context-loading controller.
Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.
Following the set up of recent works in long-context learning, \name is first provided with the KV features of each context. 
\name then uses the context encoder to compress the KV features of the context into multiple bitstream representations using different compression levels.
When a prompt and its context is received in runtime, the context-loading controller first picks the compression level of the context, fetches it through network, decompresses it and feed it to the LLM. 
%One way to select The compression level is selected 
%determines the compression level of the context such that the resulting TTFT will meet a time budget specified by the application that calls the LLM.


\begin{comment}
before the inference runtime, the context encoding algorithm will compress the key-value cache into bitstreams, with multiple compression configurations.
% \jc{let's dont introduce a separate storage server. it should be just stored where the context is originally stored, right?}
At inference runtime, the context-loading controller will select the right version of compressed key-value cache from the storage server, based on the delay budget specified by the application. 
Then \name will send the compressed key-value cache over the network, decompress them, and feed into LLM inference. 
\end{comment}

% \jc{Yuhan, regarding the terminology, how about we call it "context encoder" and "context-loading controller". the term compressor sounds too much like air compressor :)}


%\subsection{Compressor}
\subsection{KV cache encoding}

% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall that the KV cache of a context consists of two tensors of the same shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
The compression of a KV cache consists of three steps: 
(1) calculate the deltas across consecutive tokens; 
(2) pick the quantization level for each layer; and 
(3) run entropy coding.
Conceptually, these steps may look similar to video coding with each token's KV features being a frame. 
However, the exact design of each step is driven by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens are next to each other, their KV feature values at same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context, and across layers and channels, but in most cases they evolve quite smoothly between tokens of close proximity.
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}




\begin{figure}
\centering
     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
    \tightcaption{Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023}.  \jc{pick fewer channels, so that people can clearly see the correlation across tokens}} 
    \label{fig:delta_vis}
\end{figure}


Why do KV features have token-wise locality? 
The token-wise locality of KV features does not necessarily mean nearby tokens are similar or more correlated (which they are not). 
Rather, it results from the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
A crucial aspect of the self-attention mechanism is that the key and value features for a given token index are calculated based on the key-value features of \textit{all} preceding tokens.
This mechanism inherently leads to numerical similarity in the key and value features of \textit{nearby} token indices.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 


\begin{figure}[t]
\centering
     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
    \tightcaption{Proposed scheme to utilize cross-token locality. } 
    \label{fig:delta}
\end{figure}

To utilize this token-wise locality of feature values, we employ two ideas. 
First, instead of compressing the KV feature values individually, we compress the {\em deltas} between nearby tokens.
Specifically, we assume the features at token $i$, $F_i$, has been compressed with $F_i'$ as its decompressed tensor ($F_i'$ may slightly differ from $F_i$ due to lossy compression).
For the features at token $j$, $F_j$, we calculate the difference $F_j-F_i'$ and then compress this delta tensor (explained shortly).\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, because the compression and decompression will use the same reference to decode $F_j$.}
Given the insight of token-wise locality, these deltas are within a smaller range than the original feature values.




Second, we partition the tokens of a context into multiple chunks, each with 10 tokens, and within each chunk, we compress the first token's KV features independently, without comparing it with other tokens, and compress the delta between each remaining token and the first token's decompressed features. 
To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
The reason for not using this method is two-fold. 
(1) By comparing all tokens with the same reference (the first token of a chunk), we can parallelize the compression of these tokens. 
(2) The tokens within a chunk do not change as smoothly as video frames (as shown in Figure~\ref{??}), so it is not worthy of calculating the delta between consecutive tokens. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 

Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
As we can see, compressing the deltas achieves a better tradeoff. 


\begin{figure}[t]
\centering
     \includegraphics[width=.8\linewidth]{figs/delta_insight.pdf}
    \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. } 
    \label{fig:delta_insight}
\end{figure}



\mypara{Arithmetic coding} 
To further reduce the network bandwidth usage, we apply \textit{arithmetic coding}~\cite{ac} (AC) on the KV cache.
AC is widely used to losslessly compress a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
Given a probability distribution of symbols, AC assigns fewer bits to encode a more frequent symbol and more bits to encode a less frequent symbol. 
Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

Without any insight, the default implementation of AC uses a fixed probability distribution to encode all elements in the KV features.
However, not all elements follow the same probability distribution. 
Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 

One design choice is to use a unique probability distribution for each combination of channel, layer, and token index. 
This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 

Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
However, the information gains from its channel and layer are significantly higher than from its token position.
\end{insight}

Figure~\ref{??} validates this insight by comparing the AC-encoded sizes when the probability distributions are conditioned on different combinations of channel, layer, and token index.
 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}

Thus, in our encoder, we use a  per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

\begin{figure}
\centering
     \includegraphics[width=.9\linewidth]{figs/ac.pdf}
    \tightcaption{How different groupings of segments in key-value features affect the entropy. } 
    \label{fig:ac}
\end{figure}
% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\subsection{Layer-wise quantization}

Quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 
For instance, applying 8-bit quantization on a floating-point tensor linearly rescales the original tensor to fit within the range of $[-2^7, 2^7]$. 
This rescaling is achieved by dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}

To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
Various quantization schemes have been studied in communication reduction literature of NN training. 
Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
%shallower layers are more sensitive to quantization. 
Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

Intuitively, shallower layers (closer to input) in LLMs  extract more basic structural information (\eg basic sentence structure), while deeper layers extract more abstract feature~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may propagate and hinder the model's ability to grasp these deeper structures, thus more impact on results.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 

To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
This can be both time and resource-consuming.
Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).

In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  

% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\subsection{Loading Controller}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.

Specifically, we formulate the goal of the controller as minimizing generation quality degradation, compared to no compression, while meeting the time budget. 

In order to achieve this, \name maintains different versions of compressed \kv.
The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 
As seen in Figure~\ref{fig:??}, beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 
Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
It then selects the \kv version that fits within the time budget while maximizing its size. 

%\subsection{Putting all together}
%\yh{todo}
\jc{no need for a separate putting it together subsec}

\subsection{Implementation}
\begin{itemize}
\item basic library info: how many lines of code (a github link?)? ac? quantization? 
\item integrate with existing apps: how to obtain kv features of a context offline
\item interface with LLM: e.g., how to get kv features, how to feed kv features
\item any optimization to improve compression/decompression speed
\end{itemize}

% \yh{Use a figure to show that it's better to compute the context's self-attention on the fly with the texts, when  the number of input tokens is small. }

% Also, \yh{say a few sentences that different compression configurations form a tradeoff in quality and size. }
% \name maintains a database of key-value caches. 
% For each cached context, \name stores several versions of key-value caches, with different compression configurations.
% \name's controller also profiles the delay and quality tradeoffs for each of the compression configurations.
% The profiling of different compression configurations allows \name to navigate through the quality and size tradeoff. 
% Once the application specifies a delay budget, \name 
% selects the compression configuration that reaches the delay budget with the maximum generation quality, which is typically the most conservative compression configuration below the budget. 

% \name profiles the delay for different compression configurations for each 

% As an illustrative example, we plotted the 

==> backups/method-v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
    \tightcaption{Overall workflow of \name. } 
    \label{fig:system}
\end{figure}

\section{\name Design}
\label{sec:design}

This section presents \name, a fast context-loading system for LLMs. 

\subsection{Design objective}

\mypara{Delay}
To capture both the network and the computation delays of long context, we define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and generating the first token. 
While LLM systems may also reduce the total generation delay (the sum of TTFT and the delay to autoregressively generate response tokens), we choose not to use this metric  because 
(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
(2) we want to focus the delay reduction on processing input faster, not by generating fewer tokens.

Since the context resides in a different machine than the GPUs running the LLM, the TTFT delay consists of 
(1) the {\em communication} delay to fetch the context to GPU memory and 
(2) the {\em computation} delay to process the context and prompt before generating the first token.

\mypara{Quality}
We then define {\em generation quality degradation} by how close the generated text under any speedup of input processing is to the text generated when letting the LLM process the context and the prompt from scratch, which is the unoptimized implementation. 
In other words, generation quality degradation measures the impact of speedup on generated text.
If the speedup of input processing does not change the generated output, the quality will be the highest, but sometimes the speedup is achieved by dropping information, yielding a different generation text.

Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
\S\ref{subsec:eval:setup} will describe these metrics in more detail.


\mypara{Design objective}
With these definitions, the objective of \name is two-fold.
First, \name should achieve lower delay, in TTFT, than baselines at the same generation quality.
Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.


\subsection{Overview}


To achieve them, \name includes two main components: a context encoder/decoder and a context-loading controller.
Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.
Following the set up of recent works in long-context learning, given the context and its KV features, \name uses the context encoder to compress the KV features of the context into multiple bitstream representations using different compression levels.
When a prompt and its context is received in runtime, the context-loading controller first picks the compression level of the context, fetches it through network, decompresses it and feed it to the LLM. 


\subsection{KV cache encoding}

% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall that the KV cache of a context consists of two tensors of the same shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
The compression of a KV cache consists of three steps: 
(1) calculate the deltas across consecutive tokens; 
(2) pick the quantization level for each layer; and 
(3) run entropy coding.
Conceptually, these steps may look similar to video coding with each token's KV features being a frame. 
However, the exact design of each step is driven by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens are next to each other, their KV feature values at same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context, and across layers and channels, but in most cases they evolve quite smoothly between tokens of close proximity.
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}




\begin{figure}
\centering
     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
    \tightcaption{Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023}.  \jc{pick fewer channels, so that people can clearly see the correlation across tokens}} 
    \label{fig:delta_vis}
\end{figure}


Why do KV features have token-wise locality? 
The token-wise locality of KV features does not necessarily mean nearby tokens are similar or more correlated (which they are not). 
Rather, it results from the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
A crucial aspect of the self-attention mechanism is that the key and value features for a given token index are calculated based on the key-value features of \textit{all} preceding tokens.
This mechanism inherently leads to numerical similarity in the key and value features of \textit{nearby} token indices.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 


\begin{figure}[t]
\centering
     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
    \tightcaption{Proposed scheme to utilize cross-token locality. } 
    \label{fig:delta}
\end{figure}

To utilize this token-wise locality of feature values, we employ two ideas. 
First, instead of compressing the KV feature values individually, we compress the {\em deltas} between nearby tokens.
Specifically, we assume the features at token $i$, $F_i$, has been compressed with $F_i'$ as its decompressed tensor ($F_i'$ may slightly differ from $F_i$ due to lossy compression).
For the features at token $j$, $F_j$, we calculate the difference $F_j-F_i'$ and then compress this delta tensor (explained shortly).\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, because the compression and decompression will use the same reference to decode $F_j$.}
Given the insight of token-wise locality, these deltas are within a smaller range than the original feature values.




Second, we partition the tokens of a context into multiple chunks, each with 10 tokens, and within each chunk, we compress the first token's KV features independently, without comparing it with other tokens, and compress the delta between each remaining token and the first token's decompressed features. 
To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
The reason for not using this method is two-fold. 
(1) By comparing all tokens with the same reference (the first token of a chunk), we can parallelize the compression of these tokens. 
(2) The tokens within a chunk do not change as smoothly as video frames (as shown in Figure~\ref{??}), so it is not worthy of calculating the delta between consecutive tokens. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 

Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
As we can see, compressing the deltas achieves a better tradeoff. 


\begin{figure}[t]
\centering
     \includegraphics[width=.8\linewidth]{figs/delta_insight.pdf}
    \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. } 
    \label{fig:delta_insight}
\end{figure}



\mypara{Arithmetic coding} 
To further reduce the network bandwidth usage, we apply \textit{arithmetic coding}~\cite{ac} (AC) on the KV cache.
AC is widely used to losslessly compress a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
Given a probability distribution of symbols, AC assigns fewer bits to encode a more frequent symbol and more bits to encode a less frequent symbol. 
Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

Without any insight, the default implementation of AC uses a fixed probability distribution to encode all elements in the KV features.
However, not all elements follow the same probability distribution. 
Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 

One design choice is to use a unique probability distribution for each combination of channel, layer, and token index. 
This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 

Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
However, the information gains from its channel and layer are significantly higher than from its token position.
\end{insight}

Figure~\ref{??} validates this insight by comparing the AC-encoded sizes when the probability distributions are conditioned on different combinations of channel, layer, and token index.
 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}

Thus, in our encoder, we use a  per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

\begin{figure}
\centering
     \includegraphics[width=.9\linewidth]{figs/ac.pdf}
    \tightcaption{How different groupings of segments in key-value features affect the entropy. } 
    \label{fig:ac}
\end{figure}
% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\subsection{Layer-wise quantization}

Quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 
For instance, applying 8-bit quantization on a floating-point tensor linearly rescales the original tensor to fit within the range of $[-2^7, 2^7]$. 
This rescaling is achieved by dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}

To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
Various quantization schemes have been studied in communication reduction literature of NN training. 
Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
%shallower layers are more sensitive to quantization. 
Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

Intuitively, shallower layers (closer to input) in LLMs  extract more basic structural information (\eg basic sentence structure), while deeper layers extract more abstract feature~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may propagate and hinder the model's ability to grasp these deeper structures, thus more impact on results.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 

To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
This can be both time and resource-consuming.
Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).

In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  

% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\subsection{Loading Controller}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.

Specifically, we formulate the goal of the controller as minimizing generation quality degradation, compared to no compression, while meeting the time budget. 

In order to achieve this, \name maintains different versions of compressed \kv.
The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 
As seen in Figure~\ref{fig:??}, beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 
Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
It then selects the \kv version that fits within the time budget while maximizing its size. 

%\subsection{Putting all together}
%\yh{todo}
\jc{no need for a separate putting it together subsec}

\subsection{Implementation}
\begin{itemize}
\item basic library info: how many lines of code (a github link?)? ac? quantization? 
\item integrate with existing apps: how to obtain kv features of a context offline
\item interface with LLM: e.g., how to get kv features, how to feed kv features
\item any optimization to improve compression/decompression speed
\end{itemize}

% \yh{Use a figure to show that it's better to compute the context's self-attention on the fly with the texts, when  the number of input tokens is small. }

% Also, \yh{say a few sentences that different compression configurations form a tradeoff in quality and size. }
% \name maintains a database of key-value caches. 
% For each cached context, \name stores several versions of key-value caches, with different compression configurations.
% \name's controller also profiles the delay and quality tradeoffs for each of the compression configurations.
% The profiling of different compression configurations allows \name to navigate through the quality and size tradeoff. 
% Once the application specifies a delay budget, \name 
% selects the compression configuration that reaches the delay budget with the maximum generation quality, which is typically the most conservative compression configuration below the budget. 

% \name profiles the delay for different compression configurations for each 

% As an illustrative example, we plotted the 


==> backups/method-v3_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
    \tightcaption{Overall workflow of \name. } 
    \label{fig:system}
\end{figure}

\section{\name Design}
\label{sec:design}

This section presents \name, a fast context-loading system for LLMs. 

\subsection{Design objective}

\mypara{Delay}
To capture both the network and the computation delays of long context, we define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and generating the first token. 
While LLM systems may also reduce the total generation delay (the sum of TTFT and the delay to autoregressively generate response tokens), we choose not to use this metric  because 
(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
(2) we want to focus the delay reduction on processing input faster, not by generating fewer tokens.

Since the context resides in a different machine than the GPUs running the LLM, the TTFT delay consists of 
(1) the {\em communication} delay to fetch the context to GPU memory and 
(2) the {\em computation} delay to process the context and prompt before generating the first token.

\mypara{Quality}
We then define {\em generation quality degradation} by how close the generated text under any speedup of input processing is to the text generated when letting the LLM process the context and the prompt from scratch, which is the unoptimized implementation. 
In other words, generation quality degradation measures the impact of speedup on generated text.
If the speedup of input processing does not change the generated output, the quality will be the highest, but sometimes the speedup is achieved by dropping information, yielding a different generation text.

Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
\S\ref{subsec:eval:setup} will describe these metrics in more detail.


\mypara{Design objective}
With these definitions, the objective of \name is two-fold.
First, \name should achieve lower delay, in TTFT, than baselines at the same generation quality.
Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.


\subsection{Overview}


To achieve them, \name includes two main components: a context encoder/decoder and a context-loading controller.
Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.
Following the set up of recent works in long-context learning, given the context and its KV features, \name uses the context encoder to compress the KV features of the context into multiple bitstream representations using different compression levels.
When a prompt and its context is received in runtime, the context-loading controller first picks the compression level of the context, fetches it through network, decompresses it and feed it to the LLM. 


\subsection{KV cache encoding}

% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall that the KV cache of a context consists of two tensors of the same shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
The compression of a KV cache consists of three steps: 
(1) calculate the deltas across consecutive tokens; 
(2) pick the quantization level for each layer; and 
(3) run entropy coding.
Conceptually, these steps may look similar to video coding with each token's KV features being a frame. 
However, the exact design of each step is driven by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens are next to each other, their KV feature values at same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context, and across layers and channels, but in most cases they evolve quite smoothly between tokens of close proximity.
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}




\begin{figure}
\centering
     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
    \tightcaption{Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023}.  \jc{pick fewer channels, so that people can clearly see the correlation across tokens}} 
    \label{fig:delta_vis}
\end{figure}


Why do KV features have token-wise locality? 
The token-wise locality of KV features does not necessarily mean nearby tokens are similar or more correlated (which they are not). 
Rather, it results from the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
A crucial aspect of the self-attention mechanism is that the key and value features for a given token index are calculated based on the key-value features of \textit{all} preceding tokens.
This mechanism inherently leads to numerical similarity in the key and value features of \textit{nearby} token indices.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 


\begin{figure}[t]
\centering
     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
    \tightcaption{Proposed scheme to utilize cross-token locality. } 
    \label{fig:delta}
\end{figure}

To utilize this token-wise locality of feature values, we employ two ideas. 
First, instead of compressing the KV feature values individually, we compress the {\em deltas} between nearby tokens.
Specifically, we assume the features at token $i$, $F_i$, has been compressed with $F_i'$ as its decompressed tensor ($F_i'$ may slightly differ from $F_i$ due to lossy compression).
For the features at token $j$, $F_j$, we calculate the difference $F_j-F_i'$ and then compress this delta tensor (explained shortly).\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, because the compression and decompression will use the same reference to decode $F_j$.}
Given the insight of token-wise locality, these deltas are within a smaller range than the original feature values.




Second, we partition the tokens of a context into multiple chunks, each with 10 tokens, and within each chunk, we compress the first token's KV features independently, without comparing it with other tokens, and compress the delta between each remaining token and the first token's decompressed features. 
To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
The reason for not using this method is two-fold. 
(1) By comparing all tokens with the same reference (the first token of a chunk), we can parallelize the compression of these tokens. 
(2) The tokens within a chunk do not change as smoothly as video frames (as shown in Figure~\ref{??}), so it is not worthy of calculating the delta between consecutive tokens. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 

Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
As we can see, compressing the deltas achieves a better tradeoff. 


\begin{figure}[t]
\centering
     \includegraphics[width=.8\linewidth]{figs/delta_insight.pdf}
    \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. } 
    \label{fig:delta_insight}
\end{figure}



\mypara{Arithmetic coding} 
To further reduce the network bandwidth usage, we apply \textit{arithmetic coding}~\cite{ac} (AC) on the KV cache.
AC is widely used to losslessly compress a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
Given a probability distribution of symbols, AC assigns fewer bits to encode a more frequent symbol and more bits to encode a less frequent symbol. 
Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

Without any insight, the default implementation of AC uses a fixed probability distribution to encode all elements in the KV features.
However, not all elements follow the same probability distribution. 
Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 

One design choice is to use a unique probability distribution for each combination of channel, layer, and token index. 
This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 

Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
However, the information gains from its channel and layer are significantly higher than from its token position.
\end{insight}

Figure~\ref{??} validates this insight by comparing the AC-encoded sizes when the probability distributions are conditioned on different combinations of channel, layer, and token index.
 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}

Thus, in our encoder, we use a  per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

\begin{figure}
\centering
     \includegraphics[width=.9\linewidth]{figs/ac.pdf}
    \tightcaption{How different groupings of segments in key-value features affect the entropy. } 
    \label{fig:ac}
\end{figure}
% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\subsection{Layer-wise quantization}

Quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 
For instance, applying 8-bit quantization on a floating-point tensor linearly rescales the original tensor to fit within the range of $[-2^7, 2^7]$. 
This rescaling is achieved by dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}

To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
Various quantization schemes have been studied in communication reduction literature of NN training. 
Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
%shallower layers are more sensitive to quantization. 
Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

Intuitively, shallower layers (closer to input) in LLMs  extract more basic structural information (\eg basic sentence structure), while deeper layers extract more abstract feature~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may propagate and hinder the model's ability to grasp these deeper structures, thus more impact on results.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 

To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
This can be both time and resource-consuming.
Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).

In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  

% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\subsection{Loading Controller}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.

Specifically, we formulate the goal of the controller as minimizing generation quality degradation, compared to no compression, while meeting the time budget. 

In order to achieve this, \name maintains different versions of compressed \kv.
The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 
As seen in Figure~\ref{fig:??}, beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 
Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
It then selects the \kv version that fits within the time budget while maximizing its size. 

%\subsection{Putting all together}
%\yh{todo}
\jc{no need for a separate putting it together subsec}

\subsection{Implementation}
\begin{itemize}
\item basic library info: how many lines of code (a github link?)? ac? quantization? 
\item integrate with existing apps: how to obtain kv features of a context offline
\item interface with LLM: e.g., how to get kv features, how to feed kv features
\item any optimization to improve compression/decompression speed
\end{itemize}

% \yh{Use a figure to show that it's better to compute the context's self-attention on the fly with the texts, when  the number of input tokens is small. }

% Also, \yh{say a few sentences that different compression configurations form a tradeoff in quality and size. }
% \name maintains a database of key-value caches. 
% For each cached context, \name stores several versions of key-value caches, with different compression configurations.
% \name's controller also profiles the delay and quality tradeoffs for each of the compression configurations.
% The profiling of different compression configurations allows \name to navigate through the quality and size tradeoff. 
% Once the application specifies a delay budget, \name 
% selects the compression configuration that reaches the delay budget with the maximum generation quality, which is typically the most conservative compression configuration below the budget. 

% \name profiles the delay for different compression configurations for each 

% As an illustrative example, we plotted the 


==> backups/method-v4.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
    \tightcaption{Overall workflow of \name. } 
    \label{fig:system}
\end{figure}

\section{\name Design}
\label{sec:design}

This section presents \name, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
\name minimizes the overall delay for a given context while preserving the task performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

Here, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\em time-to-first-token (TTFT)}, since it measures when the first token is available for the user, thus users' experience can be heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
More importantly, this naturally includes both the {\em network} delay to fetch the context or its KV features into GPU as well as the {\em computation} delay to process the context and the prompt before decoding the first token.

%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on alleviating the impact of long contexts, TTFT excludes two aspects of delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is negligible part of TTFT.}
Second, the context is sometimes selected based on the prompt, but TTFT excludes the context-selection delay, since it has been heavily optimized by recent retrieval-based learning pipelines~\cite{??,??,??} and is relatively marginally compared to TTFT.\jc{Yuhan, any citations for this?}

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


\mypara{Quality}
Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
In other words, generation quality degradation measures the impact of speedup on text generation.
If the speedup does not change the LLM output, the quality will be the highest.
Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
\S\ref{subsec:eval:setup} will describe these metrics in more detail.


\mypara{Design objective}
With these definitions, the objective of \name is two-fold.
\begin{packeditemize}
\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
\end{packeditemize}


\mypara{Overview}
To achieve the design objective, \name includes two main components: 
a {\em context encoder/decoder} and a {\em context-loading controller}.
Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.
Following the set up of recent works in long-context learning, given the context and its KV features, \name uses the context encoder to compress the KV features of the context into multiple bitstream representations using different compression levels.
When a prompt and its context is received in runtime, the context-loading controller first picks the compression level of the context, fetches it through network, decompresses it and feed it to the LLM. \shan{might the controller decide not to use any
compression at all?}


\subsection{Context encoding}
Some prior schemes \cite{xxxx} aim to \emph{shorten} KV features, with the shortened features still in the shape of KV tensors and directly consumed by LLMs with inevitable information losses. In contrast, our context encoder aims to \emph{compress} KV features, with the compressed features
being a bitstream and will be decompressed before consumed by LLMs.
No longer in the shape of KV tensors, this bitstream
can take on a more compact representation of KV features 
with minimum information losses. 
\shan{I have reworded this paragraph. Among the three places that
we discussed this set of related work (introduction, background),
I like our discussion here the most, and I think we should
reword the other places accordingly.}

% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall \shan{really? where was this discussed? if it is in
background section or something, please add a backward reference here.} 
that the KV cache of a context consists of two tensors of the same shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
\name compresses a KV cache in three steps: 
\begin{packedenumerate}
\item calculate the delta tensor between nearby tokens; 
\item pick the quantization level for each layer of the delta tensor and apply quantization on the delta tensor; and 
\item run an arithmetic coder on the quantized delta tensor.
\end{packedenumerate}


Note that these steps of compressing KV features to a bitstream is conceptually similar to video coding (from pixel tensors to .mp4 files) with each token's KV features being a frame. 
However, the exact design of each step is driven by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens are near each other, their KV feature values at same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context, and across layers and channels, but in most cases they evolve quite smoothly between tokens of close proximity.
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}




\begin{figure}
\centering
%     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
     \includegraphics[width=.6\linewidth]{figs/fig2.pdf}
    \tightcaption{Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023}.  \jc{i still don't feel this shows the right motivation. }} 
    \label{fig:delta_vis}
\end{figure}


Why do KV features have such {\em token-wise locality}? 
The token-wise locality of KV features does not necessarily mean nearby tokens are similar or more correlated (which they are not). 
Rather, it stems from the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
%As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
The self-attention mechanism means that the K or V features for a given token index are calculated based on the KV features of previous tokens
This mechanism inherently leads to numerical similarity in the KV features of \textit{nearby} token indices.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 



To utilize this token-wise locality of feature values, we employ two ideas. 

First, instead of compressing the KV feature values individually, we compress the {\em delta} tensor between nearby tokens.
Specifically, we assume the features at token $i$, $F_i$, has already been compressed and its its decompressed tensor is $F_i'$. 
($F_i'$ may slightly differ from $F_i$ due to lossy compression.)
For the features at token $j$, $F_j$, the delta tensor of token $j$ with respect to token $i$ is $F_j-F_i'$, and we then compress this delta tensor (explained shortly).\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, because the compression and decompression will use the same reference to decode $F_j$.}
Given the insight of token-wise locality, these deltas are within a smaller range than the original feature values.



\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}

Second, we partition the tokens of a context into chunks, each with 10 contiguous tokens. 
In each chunk, we compress the KV features of the first token, called {\em anchor tokens}, independently, without comparing it with other tokens, and compress the delta tensor between each remaining token and the first token's decompressed features. 
We do not compress the delta between two consecutive tokens (like like in video frame encoding) for two reasons.
%To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
The reason for not using this method is two-fold. 
First, by comparing all tokens with the same reference (the first token of a chunk), we can parallelize the compression of these tokens. 
Second, the tokens within a chunk do not change as smoothly as video frames (as shown in Figure~\ref{fig:delta}), so it is not worthy of calculating the delta between consecutive tokens. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 



\begin{figure*}[t]
\centering
     \includegraphics[width=.9\linewidth]{figs/ac_insight_placeholder.pdf}
    \tightcaption{} 
    \label{fig:ac_insight}
\end{figure*}



% \begin{figure*}[t]
%     \centering
%          \includegraphics[width=.9\linewidth]{figs/ac_insight.pdf}
%         \tightcaption{\jc{this is nothing like what the placeholder figures look like. it doesn't show the right message. need to change it soon}} 
%         \label{fig:ac_insight}
%     \end{figure*}
    
% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
AC is widely used to losslessly compress a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

To motivate our design, we first consider two extreme design choices:
\begin{packeditemize}
\item First, the default implementation of AC assumes one fixed probability distribution for all elements in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or token necessarily share the same probability distribution. 
\item Alternatively, one can use a different probability distribution for each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions will be much more accurate but also incur a huge storage overheads (in total, $\NumTokens\times\NumLayers\times\NumChannels$ distributions) and they need to be stored on the encoder (context storage servers) and the decoder (GPU servers). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

Ideally, we should group the elements  and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements. 
In other words, the grouping needs to maximize the {\em information gain}.

To examine how grouping should be done in KV features (and delta tensors), we consider three dimensions for grouping: the channel, the layer, and the index of the token in the context, since each KV element is distinguished by these dimensions. 
We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
Figure~\ref{fig:ac_insight} compares the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
We can summarize this insight as follows:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
However, the information gains from its channel and layer are significantly higher than from its token position.
\end{insight}

Inspired by the insight, our context encoder uses a different probability distribution for each channel-layer combinations ($l \times c$ distributions in total). 
We will discuss how the probability distributions are obtained in \S\ref{subsec:impl} and evaluate the size overhead of storing these probability distributions in \S\ref{subsec:eval:storage}.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
The compression so far---applying AC on delta tensors---is lossless. 
To further reduce the bandwidth usage of transferring KV cache, we ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
There are two potential approaches.

First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

The second method, which we adopt, is to quantize the precision of a value so that it can be represented by fewer bits. 
For instance, applying 8-bit quantization on a floating-point tensor $X$ linearly rescales the original tensor to fit within the range of $[-2^7, 2^7]$. 
This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been previously used in \cite{flexgen} to trade generation quality for memory footprint of KV features.
Yet, it uses uniformly quantize all elements of KV features with the same number of bits. 
It remains unclear how KV features should be quantized to strike a balance between size reduction and the impact on LLM generation quality. 

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
%shallower layers are more sensitive to quantization. 
Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

Intuitively, shallower layers (closer to input) in LLMs  extract more basic structural information (\eg basic sentence structure), while deeper layers extract more abstract feature~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may propagate and hinder the model's ability to grasp these deeper structures, thus more impact on results.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 

To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
This can be both time and resource-consuming.
Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).

In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  

% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}

\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
    \tightcaption{} 
    \label{fig:controller}
\end{figure}


\subsection{Context-Loading Controller}

So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
Like any lossy compression, each compressed result represents a single tradeoff point between the compressed size and generation quality. 
In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate, which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.




% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
\name uses a context-loading controller, depicted in Figure~\ref{fig:controller}, to flexibly navigate the tradeoffs between generation quality and delays. 
Specifically, its goal is to minimize
%Specifically, we formulate the goal of the controller as minimizing 
generation quality degradation, compared to no compression, while meeting the TTFT budget. 
\name's controller has two parts.

First, \name compresses the KV cache of each potential context documents at multiple levels.
They cover a range of size-quality tradeoffs, with larger compressed sizes generally resulting in higher TTFT but better quality.
By default, we \jc{explain the default levels here.}
\shan{Please remind readers that the compression is done in
the background and hence not part of the TTFT, although
decompression is part of TTFT.}
%The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

\jc{need to explain why kv can be compressed offline and refer to the limitation section}

%beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

In runtime, the application provides \name with a prompt of length $L_{prompt}$, the selected documents as the context, of length $L_{context}$, and the TTFT budget.
\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ whose estimated TTFT is below the budget.
\begin{align}
TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
\label{eq:prediction}
\end{align}
The first term represents the network delay to transfer the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. \hc{provided bandwidth in data center?} 
The second term represents the computation delay and consists of two parts: 
(1) the decompression and loading of the KV cache into GPU, which is empirically modeled as {\em linear} function of the context length, $L_{context}$, and 
(2) the GPU computation to compute the cross-attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
%$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$
The exact parameters in function $Comp$ depend on the speed of the inference server.
We interpolate these parameters using past queries.

%Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

%At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
%If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
%It then selects the \kv version that fits within the time budget while maximizing its size. 

In addition to different compression levels, we also include the option of raw text of each potential context document. 
Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
decompression time would outweigh the computation time on
short text contexts.

\jc{remember to explain why picking the compression level doesn't depend on the prompt}

%\subsection{Putting all together}
%\yh{todo}
\jc{no need for a separate putting it together subsec}

\subsection{Implementation}
\begin{itemize}
\item basic library info: how many lines of code (a github link?)? ac? quantization? 
\item integrate with existing apps: how to obtain kv features of a context offline
\item interface with LLM: e.g., how to get kv features, how to feed kv features
\item any optimization to improve compression/decompression speed
\end{itemize}

% \yh{Use a figure to show that it's better to compute the context's self-attention on the fly with the texts, when  the number of input tokens is small. }

% Also, \yh{say a few sentences that different compression configurations form a tradeoff in quality and size. }
% \name maintains a database of key-value caches. 
% For each cached context, \name stores several versions of key-value caches, with different compression configurations.
% \name's controller also profiles the delay and quality tradeoffs for each of the compression configurations.
% The profiling of different compression configurations allows \name to navigate through the quality and size tradeoff. 
% Once the application specifies a delay budget, \name 
% selects the compression configuration that reaches the delay budget with the maximum generation quality, which is typically the most conservative compression configuration below the budget. 

% \name profiles the delay for different compression configurations for each 

% As an illustrative example, we plotted the 


==> backups/method-v5.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

This section presents \name, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

\tightsubsection{Context KV encoding}
\label{subsec:encoding}

%Some prior schemes \cite{xxxx} aim to \emph{shorten} KV features, with the shortened features still in the shape of KV tensors and directly consumed by LLMs with inevitable information losses. In contrast, our context encoder aims to \emph{compress} KV features, with the compressed features
%being a bitstream and will be decompressed before consumed by LLMs.
%No longer in the shape of KV tensors, this bitstream
%can take on a more compact representation of KV features 
%with minimum information losses. 
%\shan{I have reworded this paragraph. Among the three places that
%we discussed this set of related work (introduction, background),
%I like our discussion here the most, and I think we should
%reword the other places accordingly.}


% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall from \S\ref{subsec:cache} 
%\shan{really? where was this discussed? if it is in
%background section or something, please add a backward reference here.} 
that the KV cache of a context consists of two tensors of the shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
\name compresses a KV cache in three steps: 
\begin{packedenumerate}
\item calculate the delta tensors between nearby tokens; 
\item pick the quantization level for each layer of the delta tensors and apply quantization; and 
\item run an arithmetic coder on the quantized delta tensors.
\end{packedenumerate}


These steps of compressing KV features to a bitstream are conceptually similar to video coding (from pixel tensors to a .mp4 file), with each token's KV features being a frame. 
However, our designs of these steps in \name are inspired by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens' positions are near each other in the context, their KV feature values at the same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context but in most cases, they are similar among tokens of close proximity.
%, and across layers and channels, 
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}





Why do KV features have such {\em token-wise locality}? 
It does not necessarily mean nearby tokens themselves are similar or more correlated (and they are not). 
Rather, it stems from how the transformer (the self-attention) computes the KV features.
%the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
%As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
%The self-attention mechanism means that 
In essence, the KV features for a given token index are calculated based on the KV features of previous tokens.
This dependency inherently leads to numerical similarity in their KV features across \textit{nearby} tokens in a context.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 



To utilize this token-wise locality of feature values, we employ two ideas: 

\todo{Update our new delta compression here}

First, instead of compressing the KV feature separately for each token, we compress the {\em delta} between nearby tokens.
Specifically, assume that the KV features at a token $i$, $F_i$, have been compressed with its decompressed tensor being $F_i'$. 
($F_i'$ may slightly differ from $F_i$ due to lossy compression.)
For the features at token $j$, $F_j$, the {\em delta tensor} of token $j$ with token $i$ is $F_j-F_i'$, and we compress this delta tensor (explained shortly) instead of $F_j$.\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, so the compression and decompression will use the same reference to decode $F_j$.}



\begin{figure}
\centering
%     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
     \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
    \tightcaption{An example of KV values at the same layer and same channel across tokens.
    We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
    % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
    % \jc{drop blue. and extend red to a wider range}
%    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
\shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
    } 
    \label{fig:delta_vis}
\end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}

Second, we partition the tokens of a context into chunks of ten contiguous tokens. 
In each chunk, we compress the KV features of the first token, called the {\em anchor token}, independently (\ie without comparing it with other tokens), and then compress the delta tensor between each remaining token and the anchor token's decompressed features. 
We do not compress the delta between each pair of consecutive tokens, like in video frame encoding, for two reasons.
%To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
%The reason for not using this method is two-fold. 
First, by comparing all tokens with the same anchor token, we can parallelize the compression and decompression of multiple tokens. 
Second, the tokens within a chunk may not change as smoothly (Figure~\ref{fig:delta}) as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

Due to the token-wise locality, the resulting delta tensors are easier to compress than the KV features themselves.
This corroborates with our component-wise results in \S\ref{subsec:eval:micro}, highlighting delta-based compression's benefits.


%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 



\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
Next, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads ($\NumTokens\times\NumLayers\times\NumChannels$ distributions) on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext} and use the Llama-7B model to produce 3.8K KV feature tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
\end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV features produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
So far, the compression (running AC on delta tensors) has been lossless.
To further reduce the bandwidth usage of transferring the KV cache, \name also drops some information from the tokens while minimizing the impact on LLM's performance.
Recent methods propose to drop some tokens from the context~\cite{liu2023scissorhands,gisting,zhang2023ho}, but they must know the query (the prompt) to obtain the self-attention scores. 
In contrast, we want to compress the KV feature before the query arrives. \shan{this related work
has been mentioned before, right? Can we not mention them again and again and again?}


% There are two potential approaches to dropping information. 

% One is to drop some tokens ()\jc{Yuhan, Ari seems to suggest there are many works in this space. can you add more related work and maybe update this statement}, but to determine which tokens are more important than others, they often assume knowledge of the query (the prompt part) of the input, because the important tokens are typically dependent on what the prompt is asking. 
% We do not take this approach because we want to compress KV features offline without seeing the prompt to avoid compression delay in TTFT.

%ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
%There are two potential approaches.
%
%First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
%However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

%\name applies a specially designed quantization scheme that minimizes the impact on LLM's performance.
Instead of dropping tokens from the context, \name uses quantization to reduce the precision of the elements in a KV cache so that they can be represented by fewer bits. 
For instance, applying 4-bit quantization on a floating-point tensor linearly rescales the original tensor to fit within the integer range of $[-2^3, 2^3]$.
%This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}, but all elements are uniformly quantized with the same number of bits without leveraging any distributional properties of KV features.
%in~\cite{flexgen} to trade generation quality for memory footprint of KV features.
%Yet, it uniformly quantizes all elements of KV features with the same number of bits. 
It remains unclear what a better quantization strategy is to compress KV features while minimizing the impact on LLM's performance.

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
Specifically, our insight can be summarized as follows:
%shallower layers are more sensitive to quantization. 
%Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
%We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

%Intuitively, shallower layers (closer to input) in LLMs indicate basic  (\eg basic sentence structure), while deeper layers extract more abstract features~\cite{egeria, ???}. 

Intuitively, KV features at the deeper layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV features of the shallower layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the shallow-layer features can propagate and affect the deeper-layer features and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers,
and apply $x$-bit, $y$-bit, and $z$-bit quantization on the features at each layer group, respectively.
% and apply $x$-bit quantization on the first (shallowest) 1/3 of layers, $y$-bit on the second 1/3 of layers, and $z$-bit on the last 1/3 of layers.
Each combination of $(x,y,z)$, where $x\geq y\geq z$, represents a tradeoff between compression size and loss of the LLM performance and \S\ref{subsec:controller} will explain the exact settings of quantization levels used in \name.

Note that we still use 8-bit quantization, a relatively high precision, on the KV features of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it makes sense to preserve higher precision just on these anchor tokens.

%We would like to  that though the quantization settings are empirically picked, they work well across a range of LLM models and datasets (\S\ref{subsec:sensitivity}), and future work can refine the quantization scheme.

% not the only way
% AC is recalculated

%With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
%\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
%In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 
%
%To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
%This can be both time and resource-consuming.
%Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
%First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
%Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
%This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).
%
%In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  



% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}
\begin{itemize}
    \item Such a streamer which always transmits KV cache will not always 
    be beneficial given the resource available for the job. Give an example: to transmit a KV cache of size \fillme, would be beneficial when the throughput is \fillme, not beneficial when the throughput is \fillme 
    \item The streamer should adapt to resource changes so that to maximize 
    the beneifit of the streamer. Show what are the configs we can change: 
    whether to transmit KV cache and what quantization level to use 
    \item To make adaptation decisions, one of the most important step is to estimate the delay for transmitting the KV cache or generating KV cche from text context, to do so, we build an analytical model to predict the delay without actual running it
    \begin{itemize}
        \item Predicting \name delay ($T_{\name}$) based on $L_{chunk\_size}$ and quantization level $q$ 
        \item Predicting delay of generating KV from text ($T_{text}$) based on $L_{chunk\_size}, L_{current\_kv}$
    \end{itemize}
    \item Present our adaptation logic (Show detail in a algorithm block): 
    \begin{itemize}
        \item Offline encode the KV cache of each context at multiple compression 
        levels to cover a range of size-performance tradeoffs.
        \item Split each version of the KV cache into multiple token-chunks, 
        each chunk is the KV for a set of tokens.
        \item When a inference request query one context, first start with 
        transmitting the KV cache of the first token-chunk with the least quality, 
        together with the whole text context.
        \item Starting from the second token-chunk, we will decide whether to transmit
        the KV cache of which quantization level, or to generate KV cache from text context.
        This decision is made based on throughput, TTFT SLO, and estimation of $T_{text}$ and $T_{\name}$
\end{itemize}
    \end{itemize}
%So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.



\begin{table*}[t]
\centering
{\footnotesize
\begin{tabular}{c|cc|ccc|c}
\hline
\multirow{2}{*}{Pipeline} & \multicolumn{2}{c|}{Model}                                                                                                                & \multicolumn{3}{c|}{Dataset}                                                                                         & \multirow{2}{*}{Quality metric} \\ \cline{2-6}
                  & Name                                                                                   & Size                                             & Name             & Task                                                                             & Context (\#, length) &                                 \\ \hline\hline
A                 & \begin{tabular}[c]{@{}c@{}}NTK\_scaled\_Llama-13B~\cite{chen2023extending}\\ NTK\_scaled\_Llama-7B~\cite{chen2023extending}\end{tabular} & \begin{tabular}[c]{@{}c@{}}13B\\ 7B\end{tabular} & Wikitext~\cite{wikitext}         & \begin{tabular}[c]{@{}c@{}}Predict probability of \\ the next token\end{tabular} & 73, 1.8-24K         & Perplexity                      \\ \hline
B                 & LongChat-7B-16k~\cite{longchat2023}                                                                        & 7B                                               & LongChat~\cite{longchat2023}         & Long range retrieval                                                             & 200, 9-9.6K         & Accuracy                        \\ \hline
C                 & T5-large~\cite{raffel2023exploring}                                                                               & 770M                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
% D                 & Fastchat-T5-3B~\cite{}                                                                               & 3B                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
\end{tabular}
}
\caption{Summary of evaluation setup.
% \jc{add citations in the table please}
}
\label{tab:eval}
\end{table*}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
%, with larger compressed sizes generally resulting in higher TTFT but better quality.
%As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
%Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.

%By default, we \jc{explain the default levels here.}


%\shan{Please remind readers that the compression is done in
%the background and hence not part of the TTFT, although
%decompression is part of TTFT.}
%The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

%\jc{need to explain why kv can be compressed offline and refer to the limitation section}

%beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
\begin{align}
{\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
\label{eq:prediction1}
\end{align}
The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
%\hc{provided bandwidth in data center?} 
The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
%$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
\begin{align}
{\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
\label{eq:prediction2}
\end{align}
The first term is the round-trip-time (RTT) between the storage server and the GPU server.
We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
The second term is the GPU computation to compute the attention from scratch.

With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% \todo{Show analytical model to predict ttft here. }


%When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
%\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
%\begin{align}
%TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
%\label{eq:prediction}
%\end{align}



%Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

%At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
%If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
%It then selects the \kv version that fits within the time budget while maximizing its size. 

%In addition to different compression levels, we also include the option of raw text of each potential context document. 
%Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
%decompression time would outweigh the computation time on
%short text contexts.
%
%\jc{remember to explain why picking the compression level doesn't depend on the prompt}

%\subsection{Putting all together}
%\yh{todo}
%\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
Particularly, we use its encoding and decoding functions to perform AC. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Interface with LLM} 
\name interacts with LLM inference via two simple interfaces:
% To apply \name, the model inference pipeline to have incorporate two functionalities: 
(1) \name extracts the KV features of a given context from an LLM inference, and 
(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
Many Pytorch-based LLMs support these APIs. 
For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
\todo{Talk about how to match KV cache transparent to users}
% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name}
To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% we use all the 64 CPU cores, each one running a decoding processing with \texttt{torchac}, to load the \kv for different layers. 
% \shan{what does this ``optionally'' mean? are we doing it or not?}
We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.
% To reduce the delay for transferring the decoded \kv from CPU to GPU, we transfer the \kv in a layer-wise fashion. 
% That is, the computation of  layer $i$ in the LLM pipelines with the loading process of \kv for layer $i+1$. 

% \yh{Use a figure to show that it's better to compute the context's self-attention on the fly with the texts, when  the number of input tokens is small. }

% Also, \yh{say a few sentences that different compression configurations form a tradeoff in quality and size. }
% \name maintains a database of key-value caches. 
% For each cached context, \name stores several versions of key-value caches, with different compression configurations.
% \name's controller also profiles the delay and quality tradeoffs for each of the compression configurations.
% The profiling of different compression configurations allows \name to navigate through the quality and size tradeoff. 
% Once the application specifies a delay budget, \name 
% selects the compression configuration that reaches the delay budget with the maximum generation quality, which is typically the most conservative compression configuration below the budget. 

% \name profiles the delay for different compression configurations for each 

% As an illustrative example, we plotted the 


==> backups/method-v5_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

This section presents \name, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

\tightsubsection{Context KV encoding}
\label{subsec:encoding}

%Some prior schemes \cite{xxxx} aim to \emph{shorten} KV features, with the shortened features still in the shape of KV tensors and directly consumed by LLMs with inevitable information losses. In contrast, our context encoder aims to \emph{compress} KV features, with the compressed features
%being a bitstream and will be decompressed before consumed by LLMs.
%No longer in the shape of KV tensors, this bitstream
%can take on a more compact representation of KV features 
%with minimum information losses. 
%\shan{I have reworded this paragraph. Among the three places that
%we discussed this set of related work (introduction, background),
%I like our discussion here the most, and I think we should
%reword the other places accordingly.}


% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall from \S\ref{subsec:cache} 
%\shan{really? where was this discussed? if it is in
%background section or something, please add a backward reference here.} 
that the KV cache of a context consists of two tensors of the shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
\name compresses a KV cache in three steps: 
\begin{packedenumerate}
\item calculate the delta tensors between nearby tokens; 
\item pick the quantization level for each layer of the delta tensors and apply quantization; and 
\item run an arithmetic coder on the quantized delta tensors.
\end{packedenumerate}


These steps of compressing KV features to a bitstream are conceptually similar to video coding (from pixel tensors to a .mp4 file), with each token's KV features being a frame. 
However, our designs of these steps in \name are inspired by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens' positions are near each other in the context, their KV feature values at the same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context but in most cases, they are similar among tokens of close proximity.
%, and across layers and channels, 
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}





Why do KV features have such {\em token-wise locality}? 
It does not necessarily mean nearby tokens themselves are similar or more correlated (and they are not). 
Rather, it stems from how the transformer (the self-attention) computes the KV features.
%the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
%As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
%The self-attention mechanism means that 
In essence, the KV features for a given token index are calculated based on the KV features of previous tokens.
This dependency inherently leads to numerical similarity in their KV features across \textit{nearby} tokens in a context.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 



To utilize this token-wise locality of feature values, we employ two ideas: 

\todo{Update our new delta compression here}

First, instead of compressing the KV feature separately for each token, we compress the {\em delta} between nearby tokens.
Specifically, assume that the KV features at a token $i$, $F_i$, have been compressed with its decompressed tensor being $F_i'$. 
($F_i'$ may slightly differ from $F_i$ due to lossy compression.)
For the features at token $j$, $F_j$, the {\em delta tensor} of token $j$ with token $i$ is $F_j-F_i'$, and we compress this delta tensor (explained shortly) instead of $F_j$.\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, so the compression and decompression will use the same reference to decode $F_j$.}



\begin{figure}
\centering
%     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
     \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
    \tightcaption{An example of KV values at the same layer and same channel across tokens.
    We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
    % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
    % \jc{drop blue. and extend red to a wider range}
%    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
\shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
    } 
    \label{fig:delta_vis}
\end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}

Second, we partition the tokens of a context into chunks of ten contiguous tokens. 
In each chunk, we compress the KV features of the first token, called the {\em anchor token}, independently (\ie without comparing it with other tokens), and then compress the delta tensor between each remaining token and the anchor token's decompressed features. 
We do not compress the delta between each pair of consecutive tokens, like in video frame encoding, for two reasons.
%To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
%The reason for not using this method is two-fold. 
First, by comparing all tokens with the same anchor token, we can parallelize the compression and decompression of multiple tokens. 
Second, the tokens within a chunk may not change as smoothly (Figure~\ref{fig:delta}) as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

Due to the token-wise locality, the resulting delta tensors are easier to compress than the KV features themselves.
This corroborates with our component-wise results in \S\ref{subsec:eval:micro}, highlighting delta-based compression's benefits.


%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 



\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
Next, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads ($\NumTokens\times\NumLayers\times\NumChannels$ distributions) on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext} and use the Llama-7B model to produce 3.8K KV feature tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
\end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV features produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
So far, the compression (running AC on delta tensors) has been lossless.
To further reduce the bandwidth usage of transferring the KV cache, \name also drops some information from the tokens while minimizing the impact on LLM's performance.
Recent methods propose to drop some tokens from the context~\cite{liu2023scissorhands,gisting,zhang2023ho}, but they must know the query (the prompt) to obtain the self-attention scores. 
In contrast, we want to compress the KV feature before the query arrives. \shan{this related work
has been mentioned before, right? Can we not mention them again and again and again?}


% There are two potential approaches to dropping information. 

% One is to drop some tokens ()\jc{Yuhan, Ari seems to suggest there are many works in this space. can you add more related work and maybe update this statement}, but to determine which tokens are more important than others, they often assume knowledge of the query (the prompt part) of the input, because the important tokens are typically dependent on what the prompt is asking. 
% We do not take this approach because we want to compress KV features offline without seeing the prompt to avoid compression delay in TTFT.

%ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
%There are two potential approaches.
%
%First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
%However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

%\name applies a specially designed quantization scheme that minimizes the impact on LLM's performance.
Instead of dropping tokens from the context, \name uses quantization to reduce the precision of the elements in a KV cache so that they can be represented by fewer bits. 
For instance, applying 4-bit quantization on a floating-point tensor linearly rescales the original tensor to fit within the integer range of $[-2^3, 2^3]$.
%This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}, but all elements are uniformly quantized with the same number of bits without leveraging any distributional properties of KV features.
%in~\cite{flexgen} to trade generation quality for memory footprint of KV features.
%Yet, it uniformly quantizes all elements of KV features with the same number of bits. 
It remains unclear what a better quantization strategy is to compress KV features while minimizing the impact on LLM's performance.

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
Specifically, our insight can be summarized as follows:
%shallower layers are more sensitive to quantization. 
%Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
%We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

%Intuitively, shallower layers (closer to input) in LLMs indicate basic  (\eg basic sentence structure), while deeper layers extract more abstract features~\cite{egeria, ???}. 

Intuitively, KV features at the deeper layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV features of the shallower layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the shallow-layer features can propagate and affect the deeper-layer features and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers,
and apply $x$-bit, $y$-bit, and $z$-bit quantization on the features at each layer group, respectively.
% and apply $x$-bit quantization on the first (shallowest) 1/3 of layers, $y$-bit on the second 1/3 of layers, and $z$-bit on the last 1/3 of layers.
Each combination of $(x,y,z)$, where $x\geq y\geq z$, represents a tradeoff between compression size and loss of the LLM performance and \S\ref{subsec:controller} will explain the exact settings of quantization levels used in \name.

Note that we still use 8-bit quantization, a relatively high precision, on the KV features of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it makes sense to preserve higher precision just on these anchor tokens.

%We would like to  that though the quantization settings are empirically picked, they work well across a range of LLM models and datasets (\S\ref{subsec:sensitivity}), and future work can refine the quantization scheme.

% not the only way
% AC is recalculated

%With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
%\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
%In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 
%
%To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
%This can be both time and resource-consuming.
%Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
%First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
%Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
%This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).
%
%In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  



% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}
\begin{itemize}
    \item Such a streamer which always transmits KV cache will not always 
    be beneficial given the resource available for the job. Give an example: to transmit a KV cache of size \fillme, would be beneficial when the throughput is \fillme, not beneficial when the throughput is \fillme 
    \item The streamer should adapt to resource changes so that to maximize 
    the beneifit of the streamer. Show what are the configs we can change: 
    whether to transmit KV cache and what quantization level to use 
    \item To make adaptation decisions, one of the most important step is to estimate the delay for transmitting the KV cache or generating KV cche from text context, to do so, we build an analytical model to predict the delay without actual running it
    \begin{itemize}
        \item Predicting \name delay ($T_{\name}$) based on $L_{chunk\_size}$ and quantization level $q$ 
        \item Predicting delay of generating KV from text ($T_{text}$) based on $L_{chunk\_size}, L_{current\_kv}$
    \end{itemize}
    \item Present our adaptation logic (Show detail in a algorithm block): 
    \begin{itemize}
        \item Offline encode the KV cache of each context at multiple compression 
        levels to cover a range of size-performance tradeoffs.
        \item Split each version of the KV cache into multiple token-chunks, 
        each chunk is the KV for a set of tokens.
        \item When a inference request query one context, first start with 
        transmitting the KV cache of the first token-chunk with the least quality, 
        together with the whole text context.
        \item Starting from the second token-chunk, we will decide whether to transmit
        the KV cache of which quantization level, or to generate KV cache from text context.
        This decision is made based on throughput, TTFT SLO, and estimation of $T_{text}$ and $T_{\name}$
\end{itemize}
    \end{itemize}
%So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.



\begin{table*}[t]
\centering
{\footnotesize
\begin{tabular}{c|cc|ccc|c}
\hline
\multirow{2}{*}{Pipeline} & \multicolumn{2}{c|}{Model}                                                                                                                & \multicolumn{3}{c|}{Dataset}                                                                                         & \multirow{2}{*}{Quality metric} \\ \cline{2-6}
                  & Name                                                                                   & Size                                             & Name             & Task                                                                             & Context (\#, length) &                                 \\ \hline\hline
A                 & \begin{tabular}[c]{@{}c@{}}NTK\_scaled\_Llama-13B~\cite{chen2023extending}\\ NTK\_scaled\_Llama-7B~\cite{chen2023extending}\end{tabular} & \begin{tabular}[c]{@{}c@{}}13B\\ 7B\end{tabular} & Wikitext~\cite{wikitext}         & \begin{tabular}[c]{@{}c@{}}Predict probability of \\ the next token\end{tabular} & 73, 1.8-24K         & Perplexity                      \\ \hline
B                 & LongChat-7B-16k~\cite{longchat2023}                                                                        & 7B                                               & LongChat~\cite{longchat2023}         & Long range retrieval                                                             & 200, 9-9.6K         & Accuracy                        \\ \hline
C                 & T5-large~\cite{raffel2023exploring}                                                                               & 770M                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
% D                 & Fastchat-T5-3B~\cite{}                                                                               & 3B                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
\end{tabular}
}
\caption{Summary of evaluation setup.
% \jc{add citations in the table please}
}
\label{tab:eval}
\end{table*}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
%, with larger compressed sizes generally resulting in higher TTFT but better quality.
%As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
%Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.

%By default, we \jc{explain the default levels here.}


%\shan{Please remind readers that the compression is done in
%the background and hence not part of the TTFT, although
%decompression is part of TTFT.}
%The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

%\jc{need to explain why kv can be compressed offline and refer to the limitation section}

%beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
\begin{align}
{\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
\label{eq:prediction1}
\end{align}
The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
%\hc{provided bandwidth in data center?} 
The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
%$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
\begin{align}
{\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
\label{eq:prediction2}
\end{align}
The first term is the round-trip-time (RTT) between the storage server and the GPU server.
We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
The second term is the GPU computation to compute the attention from scratch.

With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% \todo{Show analytical model to predict ttft here. }


%When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
%\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
%\begin{align}
%TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
%\label{eq:prediction}
%\end{align}



%Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

%At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
%If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
%It then selects the \kv version that fits within the time budget while maximizing its size. 

%In addition to different compression levels, we also include the option of raw text of each potential context document. 
%Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
%decompression time would outweigh the computation time on
%short text contexts.
%
%\jc{remember to explain why picking the compression level doesn't depend on the prompt}

%\subsection{Putting all together}
%\yh{todo}
%\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
Particularly, we use its encoding and decoding functions to perform AC. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Interface with LLM} 
\name interacts with LLM inference via two simple interfaces:
% To apply \name, the model inference pipeline to have incorporate two functionalities: 
(1) \name extracts the KV features of a given context from an LLM inference, and 
(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
Many Pytorch-based LLMs support these APIs. 
For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
\todo{Talk about how to match KV cache transparent to users}
% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name}
To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% we use all the 64 CPU cores, each one running a decoding processing with \texttt{torchac}, to load the \kv for different layers. 
% \shan{what does this ``optionally'' mean? are we doing it or not?}
We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.
% To reduce the delay for transferring the decoded \kv from CPU to GPU, we transfer the \kv in a layer-wise fashion. 
% That is, the computation of  layer $i$ in the LLM pipelines with the loading process of \kv for layer $i+1$. 

% \yh{Use a figure to show that it's better to compute the context's self-attention on the fly with the texts, when  the number of input tokens is small. }

% Also, \yh{say a few sentences that different compression configurations form a tradeoff in quality and size. }
% \name maintains a database of key-value caches. 
% For each cached context, \name stores several versions of key-value caches, with different compression configurations.
% \name's controller also profiles the delay and quality tradeoffs for each of the compression configurations.
% The profiling of different compression configurations allows \name to navigate through the quality and size tradeoff. 
% Once the application specifies a delay budget, \name 
% selects the compression configuration that reaches the delay budget with the maximum generation quality, which is typically the most conservative compression configuration below the budget. 

% \name profiles the delay for different compression configurations for each 

% As an illustrative example, we plotted the 


==> backups/method-v6.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

This section presents \name, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

\tightsubsection{Context KV encoding}
\label{subsec:encoding}

%Some prior schemes \cite{xxxx} aim to \emph{shorten} KV features, with the shortened features still in the shape of KV tensors and directly consumed by LLMs with inevitable information losses. In contrast, our context encoder aims to \emph{compress} KV features, with the compressed features
%being a bitstream and will be decompressed before consumed by LLMs.
%No longer in the shape of KV tensors, this bitstream
%can take on a more compact representation of KV features 
%with minimum information losses. 
%\shan{I have reworded this paragraph. Among the three places that
%we discussed this set of related work (introduction, background),
%I like our discussion here the most, and I think we should
%reword the other places accordingly.}


% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall from \S\ref{subsec:cache} 
%\shan{really? where was this discussed? if it is in
%background section or something, please add a backward reference here.} 
that the KV cache of a context consists of two tensors of the shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
\name compresses a KV cache in three steps: 
\begin{packedenumerate}
\item calculate the delta tensors between nearby tokens; 
\item pick the quantization level for each layer of the delta tensors and apply quantization; and 
\item run an arithmetic coder on the quantized delta tensors.
\end{packedenumerate}


These steps of compressing KV features to a bitstream are conceptually similar to video coding (from pixel tensors to a .mp4 file), with each token's KV features being a frame. 
However, our designs of these steps in \name are inspired by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens' positions are near each other in the context, their KV feature values at the same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context but in most cases, they are similar among tokens of close proximity.
%, and across layers and channels, 
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}





Why do KV features have such {\em token-wise locality}? 
It does not necessarily mean nearby tokens themselves are similar or more correlated (and they are not). 
Rather, it stems from how the transformer (the self-attention) computes the KV features.
%the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
%As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
%The self-attention mechanism means that 
In essence, the KV features for a given token index are calculated based on the KV features of previous tokens.
This dependency inherently leads to numerical similarity in their KV features across \textit{nearby} tokens in a context.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 



To utilize this token-wise locality of feature values, we employ two ideas: 

\todo{Update our new delta compression here}

First, instead of compressing the KV feature separately for each token, we compress the {\em delta} between nearby tokens.
Specifically, assume that the KV features at a token $i$, $F_i$, have been compressed with its decompressed tensor being $F_i'$. 
($F_i'$ may slightly differ from $F_i$ due to lossy compression.)
For the features at token $j$, $F_j$, the {\em delta tensor} of token $j$ with token $i$ is $F_j-F_i'$, and we compress this delta tensor (explained shortly) instead of $F_j$.\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, so the compression and decompression will use the same reference to decode $F_j$.}



\begin{figure}
\centering
%     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
     \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
    \tightcaption{An example of KV values at the same layer and same channel across tokens.
    We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
    % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
    % \jc{drop blue. and extend red to a wider range}
%    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
\shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
    } 
    \label{fig:delta_vis}
\end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}

Second, we partition the tokens of a context into chunks of ten contiguous tokens. 
In each chunk, we compress the KV features of the first token, called the {\em anchor token}, independently (\ie without comparing it with other tokens), and then compress the delta tensor between each remaining token and the anchor token's decompressed features. 
We do not compress the delta between each pair of consecutive tokens, like in video frame encoding, for two reasons.
%To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
%The reason for not using this method is two-fold. 
First, by comparing all tokens with the same anchor token, we can parallelize the compression and decompression of multiple tokens. 
Second, the tokens within a chunk may not change as smoothly (Figure~\ref{fig:delta}) as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

Due to the token-wise locality, the resulting delta tensors are easier to compress than the KV features themselves.
This corroborates with our component-wise results in \S\ref{subsec:eval:micro}, highlighting delta-based compression's benefits.


%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 



\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
Next, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads ($\NumTokens\times\NumLayers\times\NumChannels$ distributions) on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext} and use the Llama-7B model to produce 3.8K KV feature tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
\end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV features produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
So far, the compression (running AC on delta tensors) has been lossless.
To further reduce the bandwidth usage of transferring the KV cache, \name also drops some information from the tokens while minimizing the impact on LLM's performance.
Recent methods propose to drop some tokens from the context~\cite{liu2023scissorhands,gisting,zhang2023ho}, but they must know the query (the prompt) to obtain the self-attention scores. 
In contrast, we want to compress the KV feature before the query arrives. \shan{this related work
has been mentioned before, right? Can we not mention them again and again and again?}


% There are two potential approaches to dropping information. 

% One is to drop some tokens ()\jc{Yuhan, Ari seems to suggest there are many works in this space. can you add more related work and maybe update this statement}, but to determine which tokens are more important than others, they often assume knowledge of the query (the prompt part) of the input, because the important tokens are typically dependent on what the prompt is asking. 
% We do not take this approach because we want to compress KV features offline without seeing the prompt to avoid compression delay in TTFT.

%ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
%There are two potential approaches.
%
%First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
%However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

%\name applies a specially designed quantization scheme that minimizes the impact on LLM's performance.
Instead of dropping tokens from the context, \name uses quantization to reduce the precision of the elements in a KV cache so that they can be represented by fewer bits. 
For instance, applying 4-bit quantization on a floating-point tensor linearly rescales the original tensor to fit within the integer range of $[-2^3, 2^3]$.
%This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}, but all elements are uniformly quantized with the same number of bits without leveraging any distributional properties of KV features.
%in~\cite{flexgen} to trade generation quality for memory footprint of KV features.
%Yet, it uniformly quantizes all elements of KV features with the same number of bits. 
It remains unclear what a better quantization strategy is to compress KV features while minimizing the impact on LLM's performance.

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
Specifically, our insight can be summarized as follows:
%shallower layers are more sensitive to quantization. 
%Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
%We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

%Intuitively, shallower layers (closer to input) in LLMs indicate basic  (\eg basic sentence structure), while deeper layers extract more abstract features~\cite{egeria, ???}. 

Intuitively, KV features at the deeper layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV features of the shallower layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the shallow-layer features can propagate and affect the deeper-layer features and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers,
and apply $x$-bit, $y$-bit, and $z$-bit quantization on the features at each layer group, respectively.
% and apply $x$-bit quantization on the first (shallowest) 1/3 of layers, $y$-bit on the second 1/3 of layers, and $z$-bit on the last 1/3 of layers.
Each combination of $(x,y,z)$, where $x\geq y\geq z$, represents a tradeoff between compression size and loss of the LLM performance and \S\ref{subsec:controller} will explain the exact settings of quantization levels used in \name.

Note that we still use 8-bit quantization, a relatively high precision, on the KV features of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it makes sense to preserve higher precision just on these anchor tokens.

%We would like to  that though the quantization settings are empirically picked, they work well across a range of LLM models and datasets (\S\ref{subsec:sensitivity}), and future work can refine the quantization scheme.

% not the only way
% AC is recalculated

%With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
%\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
%In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 
%
%To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
%This can be both time and resource-consuming.
%Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
%First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
%Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
%This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).
%
%In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  



% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}


\yh{Need a more concrete example, the starting throughput is \fillme, so xxxx. If not adapting, not meeting SLO. If adapting, will meet SLO. 
predicting delay is trivial.
The logic of adaptation is not trivial 

motivation => frameworks => decision of adapt to which one (1. predict delay 2. how to adapt => why the prediction is good)
}

\begin{itemize}
    \item When there are sudden network throughput changes, the initial KV transmission decision made by the streamer may not meet the SLO anymore. Concretely, for example, say we wanna transmit the KV cache of a Llama 13B model with 10K tokens.  (give an example where adapting the quantization level can help meet SLO) Also, note that our adaptation only works when there is a small timeframe of bandwidth change 
    \item To make the choices of quantization levels, we use the following adaptation framework: 
    \begin{itemize}
        \item Offline encodes the KV cache of each context at multiple compression 
        levels to cover a range of size-performance tradeoffs.
        \item Split each version of the KV cache into multiple token-chunks, 
        each chunk is the KV for a set of tokens.
        \item When a inference request query one context, first start with 
        transmitting the KV cache of the first token-chunk with the least quality, 
        together with the whole text context.
        \item Starting from the second token-chunk, we will decide whether to transmit
        the KV cache of which quantization level, or to generate KV cache from text context, based on throughput, TTFT SLO, and estimation of $T_{text}$ and $T_{\name}$
    \end{itemize}
    \item One of the key decisions in this adaptation logic is how to make the quantization level choice. 
    We do this by choosing the quantization level corresponding to the largest TTFT within the SLO.
    % Say the throughput suddenly drops from 1Gbps to 0.5 Gbps.
    % To decide the quality of transmitting the next chunk, we first predict the delay of transmitting the KV at the throughput of 0.5Gbps, and selecting the highest quality below remaining SLO. 
    \item Justify our logic is as good as optimal 
\end{itemize}


When there are sudden throughput changes while transmitting a context via network bandwidth, the initial decision made by the streamer may not meet the latency Service Level Objective (SLO) anymore. 
As a concrete example, say we wanna transmit a piece of context of a Llama 13B model, which has 10K tokens. 
The size of the encoded KV cache is about 1~GB. 
With an 8-second latency SLO and an initial throughput of 1Gbps, the streamer chooses to transmit the encoded KV cache to adhere to the SLO. 
However, if throughput suddenly drops to 0.5Gbps for 2 seconds after 3 seconds into the transmission, then returns to 1Gbps, the total transmission time extends to 9 seconds, exceeding the latency SLO.

Luckily, like any lossy compression, each of the compressed result of the encoder represents one single tradeoff point between the encoded size and the LLM's quality. 
Thus, we can have multiple versions of encoded KV cache, so that whenever throughput changes, we can switch to a smaller or bigger KV cache size to make sure it meets SLO. 
This approach is effective for short-term throughput changes. But if the throughput is low for a long time, using a smaller file might inevitably affect the quality of the LLM.


In the offline stage, we use different compression levels to encode the KV cache of each context. 
By default, we select \fillme quantization settings that cover a range of size-quality tradeoff points. 
Additionally, we divide the KV cache into multiple text chunks because our change-based encoding naturally splits it this way. 
This allows us to adapt more precisely by changing compression levels for different text chunks. 
Each text chunk contains \fillme number of tokens, which is large enough to fit in one congestion window in the datacenter. 
After quantization, the tensors are compressed by AC and stored on the storage server. 
While these quantization settings have shown good performance across various LLM models and datasets (see \S\ref{subsec:eval:sensitivity}), we believe that future work can further refine the quantization scheme to make it more adaptable to LLMs or different context distributions.

During runtime, the streamer begins by sending the first chunk of the KV cache at the compression level yielding the smallest size, along with the entire text context. 
Upon receiving this first chunk, we determine whether to generate the KV cache from the text context or select the compression level for the next chunk.
This decision takes into account factors such as the remaining Service Level Objective (SLO), the remaining tokens to be transmitted, and the current throughput.

One key part in the adaptation framework is how to make the decision of compression level for transmission.
We do this  by selecting the compression level that results in the greatest delay while still meeting the remaining SLO, as in Equation~\ref{eq:adapt}. 
\begin{equation}
\begin{cases} 
\text{"text"} & \text{if } T_{\text{text}}(L_{\text{rt}}, L_{\text{ct}}) < SLO, \\
\underset{Q}{\mathrm{argmax}} \text{ s.t. } T_{\text{kv}}(L_{\text{rt}},Q) < SLO & \text{otherwise,}
\end{cases}
\label{eq:adapt}
\end{equation}

Here, $L_{rt}$ represents the number of tokens yet to be received, and $L_{ct}$ is the number of tokens that have already been received. The function $T_{kv}(L_{rt}, Q)$ predicts the delay for transmitting a KV cache with $L$ tokens at compression level $Q$, while $T_{text}(L_{rt}, L_{ct})$ predicts the delay for generating the KV cache from text.

We assume that all subsequent chunks will maintain the same throughput as the next one. While this approach may not be as optimal as having knowledge of the throughput for all later chunks,
\yh{Talk about why this adaptation logic is close to optimal }

\jc{i commented out the algorithm pseudocode. it's causing a lot of latex errors, and i don't think we really need a pseudocode to explain it. if it can be clearly explained in fewer words, please do that. a pseudocode is usually a sign that the idea is really complicated}
% \begin{algorithm}
% \caption{Get Function Algorithm}\label{alg:sender}
% \begin{algorithmic}[1]
%     \State $remaining\_SLO \gets SLO$
%     \State $all\_KV \gets None$
%     \For{$i \in \{1..N\}$}
%         \State $is\_text, kv\_quality \gets \Call{GetNextQuality}{i, throughput, remaining\_SLO}$
%         \State $all\_KV \gets all\_KV + \Call{GetNextChunk}{is\_text, kv\_quality, i}$
%     \EndFor
%     \State \Return $all\_KV$
% \end{algorithmic}
% \end{algorithm}




% %So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
% Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
% In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
% To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% % , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.



\begin{table*}[t]
\centering
{\footnotesize
\begin{tabular}{c|cc|ccc|c}
\hline
\multirow{2}{*}{Pipeline} & \multicolumn{2}{c|}{Model}                                                                                                                & \multicolumn{3}{c|}{Dataset}                                                                                         & \multirow{2}{*}{Quality metric} \\ \cline{2-6}
                  & Name                                                                                   & Size                                             & Name             & Task                                                                             & Context (\#, length) &                                 \\ \hline\hline
A                 & \begin{tabular}[c]{@{}c@{}}NTK\_scaled\_Llama-13B~\cite{chen2023extending}\\ NTK\_scaled\_Llama-7B~\cite{chen2023extending}\end{tabular} & \begin{tabular}[c]{@{}c@{}}13B\\ 7B\end{tabular} & Wikitext~\cite{wikitext}         & \begin{tabular}[c]{@{}c@{}}Predict probability of \\ the next token\end{tabular} & 73, 1.8-24K         & Perplexity                      \\ \hline
B                 & LongChat-7B-16k~\cite{longchat2023}                                                                        & 7B                                               & LongChat~\cite{longchat2023}         & Long range retrieval                                                             & 200, 9-9.6K         & Accuracy                        \\ \hline
C                 & T5-large~\cite{raffel2023exploring}                                                                               & 770M                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
% D                 & Fastchat-T5-3B~\cite{}                                                                               & 3B                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
\end{tabular}
}
\caption{Summary of evaluation setup.
% \jc{add citations in the table please}
}
\label{tab:eval}
\end{table*}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

% First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
% %, with larger compressed sizes generally resulting in higher TTFT but better quality.
% %As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
% By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
% The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
% %Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
% Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

% We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
% We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.


% %By default, we \jc{explain the default levels here.}


% %\shan{Please remind readers that the compression is done in
% %the background and hence not part of the TTFT, although
% %decompression is part of TTFT.}
% %The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

% %\jc{need to explain why kv can be compressed offline and refer to the limitation section}

% %beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

% In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
% \begin{align}
% {\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
% \label{eq:prediction1}
% \end{align}
% The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
% %\hc{provided bandwidth in data center?} 
% The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
% The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
% %$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


% In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
% \begin{align}
% {\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
% \label{eq:prediction2}
% \end{align}
% The first term is the round-trip-time (RTT) between the storage server and the GPU server.
% We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
% The second term is the GPU computation to compute the attention from scratch.

% With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
% If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


% The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
% In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% % \todo{Show analytical model to predict ttft here. }


% %When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
% %\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
% %\begin{align}
% %TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
% %\label{eq:prediction}
% %\end{align}



% %Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

% %At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
% %If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
% %It then selects the \kv version that fits within the time budget while maximizing its size. 

% %In addition to different compression levels, we also include the option of raw text of each potential context document. 
% %Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
% %decompression time would outweigh the computation time on
% %short text contexts.
% %
% %\jc{remember to explain why picking the compression level doesn't depend on the prompt}

% %\subsection{Putting all together}
% %\yh{todo}
% %\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
Particularly, we use its encoding and decoding functions to perform AC. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Interface with LLM} 
\name interacts with LLM inference via two simple interfaces:
% To apply \name, the model inference pipeline to have incorporate two functionalities: 
(1) \name extracts the KV features of a given context from an LLM inference, and 
(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
Many Pytorch-based LLMs support these APIs. 
For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
\todo{Talk about how to match KV cache transparent to users}
% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name}
To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% we use all the 64 CPU cores, each one running a decoding processing with \texttt{torchac}, to load the \kv for different layers. 
% \shan{what does this ``optionally'' mean? are we doing it or not?}
We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.


==> backups/method-v6_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

This section presents \name, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

\tightsubsection{Context KV encoding}
\label{subsec:encoding}

%Some prior schemes \cite{xxxx} aim to \emph{shorten} KV features, with the shortened features still in the shape of KV tensors and directly consumed by LLMs with inevitable information losses. In contrast, our context encoder aims to \emph{compress} KV features, with the compressed features
%being a bitstream and will be decompressed before consumed by LLMs.
%No longer in the shape of KV tensors, this bitstream
%can take on a more compact representation of KV features 
%with minimum information losses. 
%\shan{I have reworded this paragraph. Among the three places that
%we discussed this set of related work (introduction, background),
%I like our discussion here the most, and I think we should
%reword the other places accordingly.}


% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall from \S\ref{subsec:cache} 
%\shan{really? where was this discussed? if it is in
%background section or something, please add a backward reference here.} 
that the KV cache of a context consists of two tensors of the shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
\name compresses a KV cache in three steps: 
\begin{packedenumerate}
\item calculate the delta tensors between nearby tokens; 
\item pick the quantization level for each layer of the delta tensors and apply quantization; and 
\item run an arithmetic coder on the quantized delta tensors.
\end{packedenumerate}


These steps of compressing KV features to a bitstream are conceptually similar to video coding (from pixel tensors to a .mp4 file), with each token's KV features being a frame. 
However, our designs of these steps in \name are inspired by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens' positions are near each other in the context, their KV feature values at the same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context but in most cases, they are similar among tokens of close proximity.
%, and across layers and channels, 
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}





Why do KV features have such {\em token-wise locality}? 
It does not necessarily mean nearby tokens themselves are similar or more correlated (and they are not). 
Rather, it stems from how the transformer (the self-attention) computes the KV features.
%the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
%As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
%The self-attention mechanism means that 
In essence, the KV features for a given token index are calculated based on the KV features of previous tokens.
This dependency inherently leads to numerical similarity in their KV features across \textit{nearby} tokens in a context.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 



To utilize this token-wise locality of feature values, we employ two ideas: 

\todo{Update our new delta compression here}

First, instead of compressing the KV feature separately for each token, we compress the {\em delta} between nearby tokens.
Specifically, assume that the KV features at a token $i$, $F_i$, have been compressed with its decompressed tensor being $F_i'$. 
($F_i'$ may slightly differ from $F_i$ due to lossy compression.)
For the features at token $j$, $F_j$, the {\em delta tensor} of token $j$ with token $i$ is $F_j-F_i'$, and we compress this delta tensor (explained shortly) instead of $F_j$.\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, so the compression and decompression will use the same reference to decode $F_j$.}



\begin{figure}
\centering
%     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
     \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
    \tightcaption{An example of KV values at the same layer and same channel across tokens.
    We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
    % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
    % \jc{drop blue. and extend red to a wider range}
%    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
\shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
    } 
    \label{fig:delta_vis}
\end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}

Second, we partition the tokens of a context into chunks of ten contiguous tokens. 
In each chunk, we compress the KV features of the first token, called the {\em anchor token}, independently (\ie without comparing it with other tokens), and then compress the delta tensor between each remaining token and the anchor token's decompressed features. 
We do not compress the delta between each pair of consecutive tokens, like in video frame encoding, for two reasons.
%To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
%The reason for not using this method is two-fold. 
First, by comparing all tokens with the same anchor token, we can parallelize the compression and decompression of multiple tokens. 
Second, the tokens within a chunk may not change as smoothly (Figure~\ref{fig:delta}) as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

Due to the token-wise locality, the resulting delta tensors are easier to compress than the KV features themselves.
This corroborates with our component-wise results in \S\ref{subsec:eval:micro}, highlighting delta-based compression's benefits.


%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 



\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
Next, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads ($\NumTokens\times\NumLayers\times\NumChannels$ distributions) on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext} and use the Llama-7B model to produce 3.8K KV feature tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
\end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV features produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
So far, the compression (running AC on delta tensors) has been lossless.
To further reduce the bandwidth usage of transferring the KV cache, \name also drops some information from the tokens while minimizing the impact on LLM's performance.
Recent methods propose to drop some tokens from the context~\cite{liu2023scissorhands,gisting,zhang2023ho}, but they must know the query (the prompt) to obtain the self-attention scores. 
In contrast, we want to compress the KV feature before the query arrives. \shan{this related work
has been mentioned before, right? Can we not mention them again and again and again?}


% There are two potential approaches to dropping information. 

% One is to drop some tokens ()\jc{Yuhan, Ari seems to suggest there are many works in this space. can you add more related work and maybe update this statement}, but to determine which tokens are more important than others, they often assume knowledge of the query (the prompt part) of the input, because the important tokens are typically dependent on what the prompt is asking. 
% We do not take this approach because we want to compress KV features offline without seeing the prompt to avoid compression delay in TTFT.

%ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
%There are two potential approaches.
%
%First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
%However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

%\name applies a specially designed quantization scheme that minimizes the impact on LLM's performance.
Instead of dropping tokens from the context, \name uses quantization to reduce the precision of the elements in a KV cache so that they can be represented by fewer bits. 
For instance, applying 4-bit quantization on a floating-point tensor linearly rescales the original tensor to fit within the integer range of $[-2^3, 2^3]$.
%This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}, but all elements are uniformly quantized with the same number of bits without leveraging any distributional properties of KV features.
%in~\cite{flexgen} to trade generation quality for memory footprint of KV features.
%Yet, it uniformly quantizes all elements of KV features with the same number of bits. 
It remains unclear what a better quantization strategy is to compress KV features while minimizing the impact on LLM's performance.

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
Specifically, our insight can be summarized as follows:
%shallower layers are more sensitive to quantization. 
%Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
%We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

%Intuitively, shallower layers (closer to input) in LLMs indicate basic  (\eg basic sentence structure), while deeper layers extract more abstract features~\cite{egeria, ???}. 

Intuitively, KV features at the deeper layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV features of the shallower layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the shallow-layer features can propagate and affect the deeper-layer features and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers,
and apply $x$-bit, $y$-bit, and $z$-bit quantization on the features at each layer group, respectively.
% and apply $x$-bit quantization on the first (shallowest) 1/3 of layers, $y$-bit on the second 1/3 of layers, and $z$-bit on the last 1/3 of layers.
Each combination of $(x,y,z)$, where $x\geq y\geq z$, represents a tradeoff between compression size and loss of the LLM performance and \S\ref{subsec:controller} will explain the exact settings of quantization levels used in \name.

Note that we still use 8-bit quantization, a relatively high precision, on the KV features of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it makes sense to preserve higher precision just on these anchor tokens.

%We would like to  that though the quantization settings are empirically picked, they work well across a range of LLM models and datasets (\S\ref{subsec:sensitivity}), and future work can refine the quantization scheme.

% not the only way
% AC is recalculated

%With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
%\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
%In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 
%
%To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
%This can be both time and resource-consuming.
%Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
%First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
%Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
%This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).
%
%In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  



% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}


\yh{Need a more concrete example, the starting throughput is \fillme, so xxxx. If not adapting, not meeting SLO. If adapting, will meet SLO. 
predicting delay is trivial.
The logic of adaptation is not trivial 

motivation => frameworks => decision of adapt to which one (1. predict delay 2. how to adapt => why the prediction is good)
}

\begin{itemize}
    \item When there are sudden network throughput changes, the initial KV transmission decision made by the streamer may not meet the SLO anymore. Concretely, for example, say we wanna transmit the KV cache of a Llama 13B model with 10K tokens.  (give an example where adapting the quantization level can help meet SLO) Also, note that our adaptation only works when there is a small timeframe of bandwidth change 
    \item To make the choices of quantization levels, we use the following adaptation framework: 
    \begin{itemize}
        \item Offline encodes the KV cache of each context at multiple compression 
        levels to cover a range of size-performance tradeoffs.
        \item Split each version of the KV cache into multiple token-chunks, 
        each chunk is the KV for a set of tokens.
        \item When a inference request query one context, first start with 
        transmitting the KV cache of the first token-chunk with the least quality, 
        together with the whole text context.
        \item Starting from the second token-chunk, we will decide whether to transmit
        the KV cache of which quantization level, or to generate KV cache from text context, based on throughput, TTFT SLO, and estimation of $T_{text}$ and $T_{\name}$
    \end{itemize}
    \item One of the key decisions in this adaptation logic is how to make the quantization level choice. 
    We do this by choosing the quantization level corresponding to the largest TTFT within the SLO.
    % Say the throughput suddenly drops from 1Gbps to 0.5 Gbps.
    % To decide the quality of transmitting the next chunk, we first predict the delay of transmitting the KV at the throughput of 0.5Gbps, and selecting the highest quality below remaining SLO. 
    \item Justify our logic is as good as optimal 
\end{itemize}


When there are sudden throughput changes while transmitting a context via network bandwidth, the initial decision made by the streamer may not meet the latency Service Level Objective (SLO) anymore. 
As a concrete example, say we wanna transmit a piece of context of a Llama 13B model, which has 10K tokens. 
The size of the encoded KV cache is about 1~GB. 
With an 8-second latency SLO and an initial throughput of 1Gbps, the streamer chooses to transmit the encoded KV cache to adhere to the SLO. 
However, if throughput suddenly drops to 0.5Gbps for 2 seconds after 3 seconds into the transmission, then returns to 1Gbps, the total transmission time extends to 9 seconds, exceeding the latency SLO.

Luckily, like any lossy compression, each of the compressed result of the encoder represents one single tradeoff point between the encoded size and the LLM's quality. 
Thus, we can have multiple versions of encoded KV cache, so that whenever throughput changes, we can switch to a smaller or bigger KV cache size to make sure it meets SLO. 
This approach is effective for short-term throughput changes. But if the throughput is low for a long time, using a smaller file might inevitably affect the quality of the LLM.


In the offline stage, we use different compression levels to encode the KV cache of each context. 
By default, we select \fillme quantization settings that cover a range of size-quality tradeoff points. 
Additionally, we divide the KV cache into multiple text chunks because our change-based encoding naturally splits it this way. 
This allows us to adapt more precisely by changing compression levels for different text chunks. 
Each text chunk contains \fillme number of tokens, which is large enough to fit in one congestion window in the datacenter. 
After quantization, the tensors are compressed by AC and stored on the storage server. 
While these quantization settings have shown good performance across various LLM models and datasets (see \S\ref{subsec:eval:sensitivity}), we believe that future work can further refine the quantization scheme to make it more adaptable to LLMs or different context distributions.

During runtime, the streamer begins by sending the first chunk of the KV cache at the compression level yielding the smallest size, along with the entire text context. 
Upon receiving this first chunk, we determine whether to generate the KV cache from the text context or select the compression level for the next chunk.
This decision takes into account factors such as the remaining Service Level Objective (SLO), the remaining tokens to be transmitted, and the current throughput.

One key part in the adaptation framework is how to make the decision of compression level for transmission.
We do this  by selecting the compression level that results in the greatest delay while still meeting the remaining SLO, as in Equation~\ref{eq:adapt}. 
\begin{equation}
\begin{cases} 
\text{"text"} & \text{if } T_{\text{text}}(L_{\text{rt}}, L_{\text{ct}}) < SLO, \\
\underset{Q}{\mathrm{argmax}} \text{ s.t. } T_{\text{kv}}(L_{\text{rt}},Q) < SLO & \text{otherwise,}
\end{cases}
\label{eq:adapt}
\end{equation}

Here, $L_{rt}$ represents the number of tokens yet to be received, and $L_{ct}$ is the number of tokens that have already been received. The function $T_{kv}(L_{rt}, Q)$ predicts the delay for transmitting a KV cache with $L$ tokens at compression level $Q$, while $T_{text}(L_{rt}, L_{ct})$ predicts the delay for generating the KV cache from text.

We assume that all subsequent chunks will maintain the same throughput as the next one. While this approach may not be as optimal as having knowledge of the throughput for all later chunks,
\yh{Talk about why this adaptation logic is close to optimal }

\jc{i commented out the algorithm pseudocode. it's causing a lot of latex errors, and i don't think we really need a pseudocode to explain it. if it can be clearly explained in fewer words, please do that. a pseudocode is usually a sign that the idea is really complicated}
% \begin{algorithm}
% \caption{Get Function Algorithm}\label{alg:sender}
% \begin{algorithmic}[1]
%     \State $remaining\_SLO \gets SLO$
%     \State $all\_KV \gets None$
%     \For{$i \in \{1..N\}$}
%         \State $is\_text, kv\_quality \gets \Call{GetNextQuality}{i, throughput, remaining\_SLO}$
%         \State $all\_KV \gets all\_KV + \Call{GetNextChunk}{is\_text, kv\_quality, i}$
%     \EndFor
%     \State \Return $all\_KV$
% \end{algorithmic}
% \end{algorithm}




% %So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
% Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
% In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
% To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% % , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.



\begin{table*}[t]
\centering
{\footnotesize
\begin{tabular}{c|cc|ccc|c}
\hline
\multirow{2}{*}{Pipeline} & \multicolumn{2}{c|}{Model}                                                                                                                & \multicolumn{3}{c|}{Dataset}                                                                                         & \multirow{2}{*}{Quality metric} \\ \cline{2-6}
                  & Name                                                                                   & Size                                             & Name             & Task                                                                             & Context (\#, length) &                                 \\ \hline\hline
A                 & \begin{tabular}[c]{@{}c@{}}NTK\_scaled\_Llama-13B~\cite{chen2023extending}\\ NTK\_scaled\_Llama-7B~\cite{chen2023extending}\end{tabular} & \begin{tabular}[c]{@{}c@{}}13B\\ 7B\end{tabular} & Wikitext~\cite{wikitext}         & \begin{tabular}[c]{@{}c@{}}Predict probability of \\ the next token\end{tabular} & 73, 1.8-24K         & Perplexity                      \\ \hline
B                 & LongChat-7B-16k~\cite{longchat2023}                                                                        & 7B                                               & LongChat~\cite{longchat2023}         & Long range retrieval                                                             & 200, 9-9.6K         & Accuracy                        \\ \hline
C                 & T5-large~\cite{raffel2023exploring}                                                                               & 770M                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
% D                 & Fastchat-T5-3B~\cite{}                                                                               & 3B                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
\end{tabular}
}
\caption{Summary of evaluation setup.
% \jc{add citations in the table please}
}
\label{tab:eval}
\end{table*}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

% First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
% %, with larger compressed sizes generally resulting in higher TTFT but better quality.
% %As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
% By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
% The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
% %Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
% Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

% We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
% We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.


% %By default, we \jc{explain the default levels here.}


% %\shan{Please remind readers that the compression is done in
% %the background and hence not part of the TTFT, although
% %decompression is part of TTFT.}
% %The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

% %\jc{need to explain why kv can be compressed offline and refer to the limitation section}

% %beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

% In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
% \begin{align}
% {\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
% \label{eq:prediction1}
% \end{align}
% The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
% %\hc{provided bandwidth in data center?} 
% The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
% The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
% %$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


% In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
% \begin{align}
% {\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
% \label{eq:prediction2}
% \end{align}
% The first term is the round-trip-time (RTT) between the storage server and the GPU server.
% We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
% The second term is the GPU computation to compute the attention from scratch.

% With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
% If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


% The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
% In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% % \todo{Show analytical model to predict ttft here. }


% %When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
% %\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
% %\begin{align}
% %TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
% %\label{eq:prediction}
% %\end{align}



% %Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

% %At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
% %If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
% %It then selects the \kv version that fits within the time budget while maximizing its size. 

% %In addition to different compression levels, we also include the option of raw text of each potential context document. 
% %Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
% %decompression time would outweigh the computation time on
% %short text contexts.
% %
% %\jc{remember to explain why picking the compression level doesn't depend on the prompt}

% %\subsection{Putting all together}
% %\yh{todo}
% %\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
Particularly, we use its encoding and decoding functions to perform AC. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Interface with LLM} 
\name interacts with LLM inference via two simple interfaces:
% To apply \name, the model inference pipeline to have incorporate two functionalities: 
(1) \name extracts the KV features of a given context from an LLM inference, and 
(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
Many Pytorch-based LLMs support these APIs. 
For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
\todo{Talk about how to match KV cache transparent to users}
% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name}
To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% we use all the 64 CPU cores, each one running a decoding processing with \texttt{torchac}, to load the \kv for different layers. 
% \shan{what does this ``optionally'' mean? are we doing it or not?}
We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.


==> backups/method-v8.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

We now present the design of \name, a concrete KV cache streamer for fast context-loading in LLM inference systems.
%, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
%\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

\begin{comment}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\end{comment}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

\tightsubsection{Context KV encoding}
\label{subsec:encoding}

%Some prior schemes \cite{xxxx} aim to \emph{shorten} KV features, with the shortened features still in the shape of KV tensors and directly consumed by LLMs with inevitable information losses. In contrast, our context encoder aims to \emph{compress} KV features, with the compressed features
%being a bitstream and will be decompressed before consumed by LLMs.
%No longer in the shape of KV tensors, this bitstream
%can take on a more compact representation of KV features 
%with minimum information losses. 
%\shan{I have reworded this paragraph. Among the three places that
%we discussed this set of related work (introduction, background),
%I like our discussion here the most, and I think we should
%reword the other places accordingly.}


% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall from \S\ref{subsec:cache} 
%\shan{really? where was this discussed? if it is in
%background section or something, please add a backward reference here.} 
that the KV cache of a context consists of two tensors of the shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ represent the number of tokens, layers, and channels, respectively.
\name compresses a KV cache in three steps: 
\begin{packedenumerate}
\item calculate the delta tensors between nearby tokens; 
\item pick the quantization level for each layer of the delta tensors and apply quantization; and 
\item run an arithmetic coder on the quantized delta tensors.
\end{packedenumerate}


These steps of compressing KV features to a bitstream are conceptually similar to video coding (from pixel tensors to a .mp4 file), with each token's KV features being a frame. 
However, our designs of these steps in \name are inspired by domain-specific insights on KV features produced by LLMs.



%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}
Our first insight is that if two tokens' positions are near each other in the context, their KV feature values at the same channel and same layer are similar.
Figure~\ref{fig:delta_vis} visualizes how the feature value varies across tokens, at a specific layer and channel.
We can see that the values do change across different tokens in a context but in most cases, they are similar among tokens of close proximity.
%, and across layers and channels, 
%The color similarity between two elements directly corresponds to their numerical value similarity. 
%As the figure demonstrates, within a specific feature channel, numerical values for contiguous tokens (e.g., successive rows) display much similarity. 
We can summarize this insight as follows:

%This observation shows our first insight: There is cross-token locality in the key-value features.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV feature values compared to tokens that are further apart.
\end{insight}





Why do KV features have such {\em token-wise locality}? 
It does not necessarily mean nearby tokens themselves are similar or more correlated (and they are not). 
Rather, it stems from how the transformer (the self-attention) computes the KV features.
%the self-attention mechanism of transformer models. 
%This observation is intuitive when we consider the meaning of the key-value features.
%As elaborated in \S\ref{sec:background}, every token within the prompt is associated with a set of key-value features. 
%The self-attention mechanism means that 
In essence, the KV features for a given token index are calculated based on the KV features of previous tokens.
This dependency inherently leads to numerical similarity in their KV features across \textit{nearby} tokens in a context.
% In natural language contexts, adjacent tokens often exhibit similar semantic significance or syntactic connections. \jc{i don't understand, but it sounds intruiging. can you give some concrete examples of such similarity in semantic/syntactic connections?}
% \yh{self-attention mechanically has this property: later tokens dependent on previous tokens}
% The self-attention mechanism inherent to Transformer models seeks to capture such semantic and syntactic relationships, leading neighboring tokens to affect one another's key-value features. 



To utilize this token-wise locality of feature values, we employ two ideas: 

\todo{Update our new delta compression here}

First, instead of compressing the KV feature separately for each token, we compress the {\em delta} between nearby tokens.
Specifically, assume that the KV features at a token $i$, $F_i$, have been compressed with its decompressed tensor being $F_i'$. 
($F_i'$ may slightly differ from $F_i$ due to lossy compression.)
For the features at token $j$, $F_j$, the {\em delta tensor} of token $j$ with token $i$ is $F_j-F_i'$, and we compress this delta tensor (explained shortly) instead of $F_j$.\footnote{We define delta as the difference with the {\em reconstructed} $F_i'$, rather than the original $F_i$, so the compression and decompression will use the same reference to decode $F_j$.}



\begin{figure}
\centering
%     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
     \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
    \tightcaption{An example of KV values at the same layer and same channel across tokens.
    We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
    % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
    % \jc{drop blue. and extend red to a wider range}
%    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
\shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
    } 
    \label{fig:delta_vis}
\end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}

Second, we partition the tokens of a context into chunks of ten contiguous tokens. 
In each chunk, we compress the KV features of the first token, called the {\em anchor token}, independently (\ie without comparing it with other tokens), and then compress the delta tensor between each remaining token and the anchor token's decompressed features. 
We do not compress the delta between each pair of consecutive tokens, like in video frame encoding, for two reasons.
%To explain the reason, let us consider a strawman that compresses the delta between every two consecutive tokens, just like how video is encoded by compressing the difference between consecutive frames. 
%The reason for not using this method is two-fold. 
First, by comparing all tokens with the same anchor token, we can parallelize the compression and decompression of multiple tokens. 
Second, the tokens within a chunk may not change as smoothly (Figure~\ref{fig:delta}) as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 
%While this may minimize the delta (\ie each token is most similar to its immediate last one), but to calculate the delta, one will 

Due to the token-wise locality, the resulting delta tensors are easier to compress than the KV features themselves.
This corroborates with our component-wise results in \S\ref{subsec:eval:micro}, highlighting delta-based compression's benefits.


%For each chunk, we compute the differences (or ``deltas'') between subsequent tokens and the first token.
%Figure~\ref{fig:delta} is an illustration of our proposed approach. 
%Intuitively, the cross-token locality results in deltas with smaller numerical values, thereby making it easier to compress. 



\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
Next, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads ($\NumTokens\times\NumLayers\times\NumChannels$ distributions) on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext} and use the Llama-7B model to produce 3.8K KV feature tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
\end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV features produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
\yh{Make this section fewer variables }
So far, the compression (running AC on delta tensors) has been lossless.
To further reduce the bandwidth usage of transferring the KV cache, \name also drops some information from the tokens while minimizing the impact on LLM's performance.
Recent methods propose to drop some tokens from the context~\cite{liu2023scissorhands,gisting,zhang2023ho}, but they must know the query (the prompt) to obtain the self-attention scores. 
In contrast, we want to compress the KV feature before the query arrives. \shan{this related work
has been mentioned before, right? Can we not mention them again and again and again?}


% There are two potential approaches to dropping information. 

% One is to drop some tokens ()\jc{Yuhan, Ari seems to suggest there are many works in this space. can you add more related work and maybe update this statement}, but to determine which tokens are more important than others, they often assume knowledge of the query (the prompt part) of the input, because the important tokens are typically dependent on what the prompt is asking. 
% We do not take this approach because we want to compress KV features offline without seeing the prompt to avoid compression delay in TTFT.

%ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
%There are two potential approaches.
%
%First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
%However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

%\name applies a specially designed quantization scheme that minimizes the impact on LLM's performance.
Instead of dropping tokens from the context, \name uses quantization to reduce the precision of the elements in a KV cache so that they can be represented by fewer bits. 
For instance, applying 4-bit quantization on a floating-point tensor linearly rescales the original tensor to fit within the integer range of $[-2^3, 2^3]$.
%This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}, but all elements are uniformly quantized with the same number of bits without leveraging any distributional properties of KV features.
%in~\cite{flexgen} to trade generation quality for memory footprint of KV features.
%Yet, it uniformly quantizes all elements of KV features with the same number of bits. 
It remains unclear what a better quantization strategy is to compress KV features while minimizing the impact on LLM's performance.

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
Specifically, our insight can be summarized as follows:
%shallower layers are more sensitive to quantization. 
%Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
%We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

%Intuitively, shallower layers (closer to input) in LLMs indicate basic  (\eg basic sentence structure), while deeper layers extract more abstract features~\cite{egeria, ???}. 

Intuitively, KV features at the deeper layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV features of the shallower layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the shallow-layer features can propagate and affect the deeper-layer features and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}

Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers,
and apply $x$-bit, $y$-bit, and $z$-bit quantization on the features at each layer group, respectively.
% and apply $x$-bit quantization on the first (shallowest) 1/3 of layers, $y$-bit on the second 1/3 of layers, and $z$-bit on the last 1/3 of layers.
Each combination of $(x,y,z)$, where $x\geq y\geq z$, represents a tradeoff between compression size and loss of the LLM performance and \S\ref{subsec:controller} will explain the exact settings of quantization levels used in \name.

Note that we still use 8-bit quantization, a relatively high precision, on the KV features of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it makes sense to preserve higher precision just on these anchor tokens.

%We would like to  that though the quantization settings are empirically picked, they work well across a range of LLM models and datasets (\S\ref{subsec:sensitivity}), and future work can refine the quantization scheme.

% not the only way
% AC is recalculated

%With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
%\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
%In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 
%
%To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
%This can be both time and resource-consuming.
%Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
%First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
%Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
%This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).
%
%In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  



% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}



\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}


\yh{Need a more concrete example, the starting throughput is \fillme, so xxxx. If not adapting, not meeting SLO. If adapting, will meet SLO. 
predicting delay is trivial.
The logic of adaptation is not trivial 

motivation => frameworks => decision of adapt to which one (1. predict delay 2. how to adapt => why the prediction is good)
}

\begin{itemize}
    \item When there are sudden network throughput changes, the initial KV transmission decision made by the streamer may not meet the SLO anymore. Concretely, for example, say we wanna transmit the KV cache of a Llama 13B model with 10K tokens.  (give an example where adapting the quantization level can help meet SLO) Also, note that our adaptation only works when there is a small timeframe of bandwidth change 
    \item To make the choices of quantization levels, we use the following adaptation framework: 
    \begin{itemize}
        \item Offline encodes the KV cache of each context at multiple compression 
        levels to cover a range of size-performance tradeoffs.
        \item Split each version of the KV cache into multiple token-chunks, 
        each chunk is the KV for a set of tokens.
        \item When a inference request query one context, first start with 
        transmitting the KV cache of the first token-chunk with the least quality, 
        together with the whole text context.
        \item Starting from the second token-chunk, we will decide whether to transmit
        the KV cache of which quantization level, or to generate KV cache from text context, based on throughput, TTFT SLO, and estimation of $T_{text}$ and $T_{\name}$
    \end{itemize}
    \item One of the key decisions in this adaptation logic is how to make the quantization level choice. 
    We do this by choosing the quantization level corresponding to the largest TTFT within the SLO.
    % Say the throughput suddenly drops from 1Gbps to 0.5 Gbps.
    % To decide the quality of transmitting the next chunk, we first predict the delay of transmitting the KV at the throughput of 0.5Gbps, and selecting the highest quality below remaining SLO. 
    \item Justify our logic is as good as optimal 
\end{itemize}


When there are sudden throughput changes while transmitting a context via network bandwidth, the initial decision made by the streamer may not meet the latency Service Level Objective (SLO) anymore. 
As a concrete example, say we wanna transmit a piece of context of a Llama 13B model, which has 10K tokens. 
The size of the encoded KV cache is about 1~GB. 
With an 8-second latency SLO and an initial throughput of 1Gbps, the streamer chooses to transmit the encoded KV cache to adhere to the SLO. 
However, if throughput suddenly drops to 0.5Gbps for 2 seconds after 3 seconds into the transmission, then returns to 1Gbps, the total transmission time extends to 9 seconds, exceeding the latency SLO.

Luckily, like any lossy compression, each of the compressed result of the encoder represents one single tradeoff point between the encoded size and the LLM's quality. 
Thus, we can have multiple versions of encoded KV cache, so that whenever throughput changes, we can switch to a smaller or bigger KV cache size to make sure it meets SLO. 
This approach is effective for short-term throughput changes. But if the throughput is low for a long time, using a smaller file might inevitably affect the quality of the LLM.


In the offline stage, we use different compression levels to encode the KV cache of each context. 
By default, we select \fillme quantization settings that cover a range of size-quality tradeoff points. 
Additionally, we divide the KV cache into multiple text chunks because our change-based encoding naturally splits it this way. 
This allows us to adapt more precisely by changing compression levels for different text chunks. 
Each text chunk contains \fillme number of tokens, which is large enough to fit in one congestion window in the datacenter. 
After quantization, the tensors are compressed by AC and stored on the storage server. 
While these quantization settings have shown good performance across various LLM models and datasets (see \S\ref{subsec:eval:sensitivity}), we believe that future work can further refine the quantization scheme to make it more adaptable to LLMs or different context distributions.

During runtime, the streamer begins by sending the first chunk of the KV cache at the compression level yielding the smallest size, along with the entire text context. 
Upon receiving this first chunk, we determine whether to generate the KV cache from the text context or select the compression level for the next chunk.
This decision takes into account factors such as the remaining Service Level Objective (SLO), the remaining tokens to be transmitted, and the current throughput.

One key part in the adaptation framework is how to make the decision of compression level for transmission.
We do this  by selecting the compression level that results in the greatest delay while still meeting the remaining SLO, as in Equation~\ref{eq:adapt}. 
\begin{equation}
\begin{cases} 
\text{"text"} & \text{if } T_{\text{text}}(L_{\text{rt}}, L_{\text{ct}}) < SLO, \\
\underset{Q}{\mathrm{argmax}} \text{ s.t. } T_{\text{kv}}(L_{\text{rt}},Q) < SLO & \text{otherwise,}
\end{cases}
\label{eq:adapt}
\end{equation}

Here, $L_{rt}$ represents the number of tokens yet to be received, and $L_{ct}$ is the number of tokens that have already been received. The function $T_{kv}(L_{rt}, Q)$ predicts the delay for transmitting a KV cache with $L$ tokens at compression level $Q$, while $T_{text}(L_{rt}, L_{ct})$ predicts the delay for generating the KV cache from text.

We assume that all subsequent chunks will maintain the same throughput as the next one. While this approach may not be as optimal as having knowledge of the throughput for all later chunks,
\yh{Talk about why this adaptation logic is close to optimal }

\jc{i commented out the algorithm pseudocode. it's causing a lot of latex errors, and i don't think we really need a pseudocode to explain it. if it can be clearly explained in fewer words, please do that. a pseudocode is usually a sign that the idea is really complicated}
% \begin{algorithm}
% \caption{Get Function Algorithm}\label{alg:sender}
% \begin{algorithmic}[1]
%     \State $remaining\_SLO \gets SLO$
%     \State $all\_KV \gets None$
%     \For{$i \in \{1..N\}$}
%         \State $is\_text, kv\_quality \gets \Call{GetNextQuality}{i, throughput, remaining\_SLO}$
%         \State $all\_KV \gets all\_KV + \Call{GetNextChunk}{is\_text, kv\_quality, i}$
%     \EndFor
%     \State \Return $all\_KV$
% \end{algorithmic}
% \end{algorithm}




% %So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
% Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
% In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
% To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% % , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.



\begin{table*}[t]
\centering
{\footnotesize
\begin{tabular}{c|cc|ccc|c}
\hline
\multirow{2}{*}{Pipeline} & \multicolumn{2}{c|}{Model}                                                                                                                & \multicolumn{3}{c|}{Dataset}                                                                                         & \multirow{2}{*}{Quality metric} \\ \cline{2-6}
                  & Name                                                                                   & Size                                             & Name             & Task                                                                             & Context (\#, length) &                                 \\ \hline\hline
A                 & \begin{tabular}[c]{@{}c@{}}NTK\_scaled\_Llama-13B~\cite{chen2023extending}\\ NTK\_scaled\_Llama-7B~\cite{chen2023extending}\end{tabular} & \begin{tabular}[c]{@{}c@{}}13B\\ 7B\end{tabular} & Wikitext~\cite{wikitext}         & \begin{tabular}[c]{@{}c@{}}Predict probability of \\ the next token\end{tabular} & 73, 1.8-24K         & Perplexity                      \\ \hline
B                 & LongChat-7B-16k~\cite{longchat2023}                                                                        & 7B                                               & LongChat~\cite{longchat2023}         & Long range retrieval                                                             & 200, 9-9.6K         & Accuracy                        \\ \hline
C                 & T5-large~\cite{raffel2023exploring}                                                                               & 770M                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
% D                 & Fastchat-T5-3B~\cite{}                                                                               & 3B                                             & Natural Questions~\cite{47761} & Question Answering                                                               & 7.8K, 8-12K         & F1 score                        \\ \hline
\end{tabular}
}
\caption{Summary of evaluation setup.
% \jc{add citations in the table please}
}
\label{tab:eval}
\end{table*}

% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

% First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
% %, with larger compressed sizes generally resulting in higher TTFT but better quality.
% %As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
% By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
% The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
% %Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
% Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

% We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
% We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.


% %By default, we \jc{explain the default levels here.}


% %\shan{Please remind readers that the compression is done in
% %the background and hence not part of the TTFT, although
% %decompression is part of TTFT.}
% %The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

% %\jc{need to explain why kv can be compressed offline and refer to the limitation section}

% %beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

% In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
% \begin{align}
% {\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
% \label{eq:prediction1}
% \end{align}
% The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
% %\hc{provided bandwidth in data center?} 
% The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
% The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
% %$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


% In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
% \begin{align}
% {\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
% \label{eq:prediction2}
% \end{align}
% The first term is the round-trip-time (RTT) between the storage server and the GPU server.
% We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
% The second term is the GPU computation to compute the attention from scratch.

% With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
% If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


% The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
% In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% % \todo{Show analytical model to predict ttft here. }


% %When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
% %\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
% %\begin{align}
% %TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
% %\label{eq:prediction}
% %\end{align}



% %Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

% %At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
% %If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
% %It then selects the \kv version that fits within the time budget while maximizing its size. 

% %In addition to different compression levels, we also include the option of raw text of each potential context document. 
% %Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
% %decompression time would outweigh the computation time on
% %short text contexts.
% %
% %\jc{remember to explain why picking the compression level doesn't depend on the prompt}

% %\subsection{Putting all together}
% %\yh{todo}
% %\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
Particularly, we use its encoding and decoding functions to perform AC. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Interface with LLM} 
\name interacts with LLM inference via two simple interfaces:
% To apply \name, the model inference pipeline to have incorporate two functionalities: 
(1) \name extracts the KV features of a given context from an LLM inference, and 
(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
Many Pytorch-based LLMs support these APIs. 
For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
\todo{Talk about how to match KV cache transparent to users}
% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name}
To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% we use all the 64 CPU cores, each one running a decoding processing with \texttt{torchac}, to load the \kv for different layers. 
% \shan{what does this ``optionally'' mean? are we doing it or not?}
We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.


==> backups/method-v9.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

We now present the design of \name, a concrete KV cache streamer for fast context-loading in LLM inference systems.
%, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
%\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

\begin{comment}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\end{comment}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

\tightsubsection{Context KV encoding}
\label{subsec:encoding}
\yh{Jumps too much from previous }
\yh{Emphasize the similarity with video coding. 
Before starting change-based encodingxxx, start by saying why blindly applying video techniques is not ok.

move the  insights in one zone.

Mention this is empirical observation. 

What we have is a representative dataset? 
}

%Some prior schemes \cite{xxxx} aim to \emph{shorten} KV features, with the shortened features still in the shape of KV tensors and directly consumed by LLMs with inevitable information losses. In contrast, our context encoder aims to \emph{compress} KV features, with the compressed features
%being a bitstream and will be decompressed before consumed by LLMs.
%No longer in the shape of KV tensors, this bitstream
%can take on a more compact representation of KV features 
%with minimum information losses. 
%\shan{I have reworded this paragraph. Among the three places that
%we discussed this set of related work (introduction, background),
%I like our discussion here the most, and I think we should
%reword the other places accordingly.}


% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall from \S\ref{sec:delay} 
%\shan{really? where was this discussed? if it is in
%background section or something, please add a backward reference here.} 
that a KV cache of a context contains two tensors (K and V) of the same shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ are the number of tokens, layers, and channels, respectively.
\name compresses each tensor in three steps: 
\begin{packedenumerate}
\item calculate the delta tensors between nearby tokens; 
\item apply quantization to each layer of the delta tensors; and 
\item run the arithmetic coder on the quantized delta tensors.
\end{packedenumerate}


These steps of compressing KV features to a bitstream are conceptually similar to video coding (from pixel tensors to a .mp4 file), where each token's KV features can be seen as a frame. 
Yet, the exact design of \name is inspired by domain-specific insights on KV features produced by LLMs.

Next, we will explain each step along with the rationale behind it.


%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}  Our first insight is about the similarity between KV cache across nearby tokens.
%Particularly, we observe that:

%that if two tokens' positions are near to each other in the context, their KV feature values at the same channel and same layer are similar.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV cache values compared to tokens that are further apart.
\end{insight}

This {\em token-wise} locality 
%Why do KV features have such \emph{token-wise} locality? It does
%not necessarily mean nearby tokens themselves are similar
%or more correlated (and they are not). Rather, it 
stems from
the transformer (the self-attention) mechanism that computes the KV
cache. In essence, the KV cache for a given token index
are calculated based on the KV cache of previous tokens\footnote{More strictly, the KV cache are generated in a layer-by-layer manner. The KV of token index $t$ at layer $i$ is computed based on the attention matrix 
 from all the previous tokens' attention matrix at the previous layer~\cite{vaswani2023attention, attention2}.}.

% \jc{i know it's technically correct, but like you said many time, the conventional understanding is that KV is computed layer by layer, not token by token. it seems this claim is essential to the locality observation, can you add some text to explain it and also find any citations to back it up?}
% This dependency inherently leads to numerical similarity in their KV features across \emph{nearby} tokens in a context.


\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.7\linewidth]{figs/delta_insight.pdf}
    \tightcaption{\yh{Replace with real}} 
    \label{fig:delta_insight}
\end{figure}


This token-wise locality suggests an opportunity for better compression without affecting generation quality.
The values in the original KV tensors
% given one channel and layer,\jc{i don't think we really need to stress that it's a given channel or layer, do we?} 
might span a large range with a high variance.
However, if we compute the \emph{delta} between nearby tokens at each layer and channel, the distribution of the deltas will have a much smaller variance.
For instance, Figure~\ref{fig:delta_insight} shows that at a particular layer and channel, the distribution of original KV values has a much lower variance than the distribution of the delta values between two nearby tokens.
% the cumulative density function (CDF) of the original and delta KV features for one channel and one layer.
% As we can see, the delta KV features has smaller variance than the original ones. 

Since the distribution of delta values has a low variance and a mean around zero, it is well-known that it can be quantized and encoded to achieve a desirable size-loss tradeoff~\cite{doi:10.1080/03610928608829122}.
Specifically, most delta values are close to zero, so our quantization step (explained soon) can quantize them into a few distinct values with minimum information loss.
This results in a highly skewed distribution, \ie low entropy, so after arithmetic coding (explained soon), the distribution will have a small bitstream size. 

% \jc{yuhan, i rewrote the paragraph to simplify and smooth the text. please feel free to revert or edit the new text}
% If a distribution has smaller variance,
% it can be more easily compressed and has better size vs error tradeoff 
%  for reduced entropy~\cite{doi:10.1080/03610928608829122}.
% Intuitively, for a distribution with a smaller variance, there will be more repeated symbols in the data distribution after compression, specifically after non-uniform quantization (details in a later section). 
% These repeated symbols can be encoded with fewer bits, thereby reducing the overall size post-compression. Additionally, despite the reduced size, the error introduced by quantization remains minimal. To illustrate this, consider a quantization scheme that divides a distribution into two bins: one for values between 0 and 1, and another for all remaining values, with the quantized value being the bin's mean.
% For instance, a distribution like $[0.1, 0.5, 0.8, 1.5, 3]$ is quantized to $[0.7, 0.7, 0.7, 2.25, 2.25]$ resulting in an entropy value of 0.97. In contrast, a distribution such as $[0, 0.1, 0.2, 0.3, 1.2]$, which is quantized into $[0.15, 0.15, 0.15, 0.15, 1.2]$, this has an entropy of 0.72. 
% Moreover, the quantization error rates for these two distributions are 0.3 and 0.01, respectively.
% Thus, the repeated symbols can be represented with fewer bits, size after compression will be smaller. 
% Moreover, even though having smaller size, the error due to quantization will still be low. 
% As a simple illustrative example, consider the quantization scheme that bucketize a distribution into 2 bins, where values in between 0 and 1 into one bin, and other values into another, with the quantized value as the mean in the bins.
% If one distribution is $[0.1, 0.5, 0.8, 1.5, 3]$, the quantized values are $[0.7, 0.7, 0.7, 2.25, 2.25]$, leading to a entropy value of 0.97. 
% As for another distribution $[0, 0.1, 0.2, 0.3, 1.2]$, which is quantized into $[0.15, 0.15, 0.15, 0.15, 1.2]$, this has an entropy of 0.72. 
% Furthermore,  the error rate for the quantized data for the two is 0.3 and 0.01, respectively. 


% Since distributions with smaller variances have lower entropy\footnote{As the KV features is a normal distribution, many prior works have proved that smaller variance leads to lower entropy~\cite{??, ??, ??}. }, compressing the delta tensors instead of the original ones will be more beneficial. 

To utilize this token-wise locality of feature values, 
we employ the following idea: 

We partition all the tokens of a context into chunks of ten contiguous tokens. 
In each chunk, we compress the KV features of the first token, called the {\em anchor token}, independently (\ie without comparing it with other tokens), and then compress the delta tensor between each remaining token and the anchor token's decompressed features\footnote{Note that we compute the delta tensor between each remaining token and the \emph{decompressed} anchor token, so that the compression and decompression of remaining tokens in the group share the same reference to decode them. }. 


This process is analogous to video coding, where it also partitions the frames into chunks of contiguous frames. 
However, we are different from video coding in that we do not compress the delta between each pair of consecutive tokens, like in video frame encoding, because by comparing all tokens with the same anchor token in one chunk, we can greatly parallelize the compression and decompression of many tokens. 
% Second, the tokens within a chunk may not change as smoothly as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 


% \begin{figure}
% \centering
% %     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
%      \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{An example of KV values at the same layer and same channel across tokens.
%     We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
%     % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
%     % \jc{drop blue. and extend red to a wider range}
% %    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
% \shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
%     } 
%     \label{fig:delta_vis}
% \end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}


\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
Next, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads ($\NumTokens\times\NumLayers\times\NumChannels$ distributions) on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext} and use the Llama-7B model to produce 3.8K KV feature tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
\end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV features produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
\yh{Earlier and later layers }
So far, the compression (running AC on delta tensors) has been lossless.
To further reduce the bandwidth usage of transferring the KV cache, \name also drops some information from the tokens while minimizing the impact on LLM's performance.
Specifically, \name uses quantization to reduce the precision of the elements in a KV cache so that they can be represented by fewer bits. 
% For instance, bucketizing a floating-point tensor into 4 bins make 
% For instance, bucketizing a floating-point tensor linearly rescales the original tensor to fit within the integer range of $[-2^3, 2^3]$.
% Recent methods propose to drop some tokens from the context~\cite{liu2023scissorhands,gisting,zhang2023ho}, but they must know the query (the prompt) to obtain the self-attention scores. 
% In contrast, we want to compress the KV feature before the query arrives. 
% \shan{this related work
% has been mentioned before, right? Can we not mention them again and again and again?}


% There are two potential approaches to dropping information. 

% One is to drop some tokens ()\jc{Yuhan, Ari seems to suggest there are many works in this space. can you add more related work and maybe update this statement}, but to determine which tokens are more important than others, they often assume knowledge of the query (the prompt part) of the input, because the important tokens are typically dependent on what the prompt is asking. 
% We do not take this approach because we want to compress KV features offline without seeing the prompt to avoid compression delay in TTFT.

%ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
%There are two potential approaches.
%
%First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
%However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

%\name applies a specially designed quantization scheme that minimizes the impact on LLM's performance.

%This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}, but all elements are uniformly quantized with the same number of bits without leveraging any distributional properties of KV features.
%in~\cite{flexgen} to trade generation quality for memory footprint of KV features.
%Yet, it uniformly quantizes all elements of KV features with the same number of bits. 
It remains unclear what a better quantization strategy is to compress KV features while minimizing the impact on LLM's performance.

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
Specifically, our insight can be summarized as follows:
%shallower layers are more sensitive to quantization. 
%Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
%We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

%Intuitively, shallower layers (closer to input) in LLMs indicate basic  (\eg basic sentence structure), while deeper layers extract more abstract features~\cite{egeria, ???}. 

Intuitively, KV features at the deeper layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV features of the shallower layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the shallow-layer features can propagate and affect the deeper-layer features and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}
Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers, and apply different amount of quantization bin size on features at each layer group, respectively. 
The size of the quantization bin grows larger (\ie larger quantization errors)
from shallow to deeper layer groups. 
% Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
% Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers,
% and apply $x$-bit, $y$-bit, and $z$-bit quantization on the features at each layer group, respectively.
% % and apply $x$-bit quantization on the first (shallowest) 1/3 of layers, $y$-bit on the second 1/3 of layers, and $z$-bit on the last 1/3 of layers.
% Each combination of $(x,y,z)$, where $x\geq y\geq z$, represents a tradeoff between compression size and loss of the LLM performance and \S\ref{subsec:controller} will explain the exact settings of quantization levels used in \name.

Note that we still use 8-bit quantization, a relatively high precision, on the KV features of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it makes sense to preserve higher precision just on these anchor tokens.

%We would like to  that though the quantization settings are empirically picked, they work well across a range of LLM models and datasets (\S\ref{subsec:sensitivity}), and future work can refine the quantization scheme.

% not the only way
% AC is recalculated

%With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
%\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
%In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 
%
%To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
%This can be both time and resource-consuming.
%Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
%First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
%Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
%This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).
%
%In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  



% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}

\input{F/adaptation-case/fig-adaptation-case}

\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}

\yh{Doing edits now!! }


\yh{Not clear how we stream? 

Pseudocode 

drop the equation 
}

% \yh{Need a more concrete example, the starting throughput is \fillme, so xxxx. If not adapting, not meeting SLO. If adapting, will meet SLO. 
% predicting delay is trivial.
% The logic of adaptation is not trivial 

% motivation => frameworks => decision of adapt to which one (1. predict delay 2. how to adapt => why the prediction is good)
% }

% \begin{itemize}
%     \item When there are sudden network throughput changes, the initial KV transmission decision made by the streamer may not meet the SLO anymore. Concretely, for example, say we wanna transmit the KV cache of a Llama 13B model with 10K tokens.  (give an example where adapting the quantization level can help meet SLO) Also, note that our adaptation only works when there is a small timeframe of bandwidth change 
%     \item To make the choices of quantization levels, we use the following adaptation framework: 
%     \begin{itemize}
%         \item Offline encodes the KV cache of each context at multiple compression 
%         levels to cover a range of size-performance tradeoffs.
%         \item Split each version of the KV cache into multiple token-chunks, 
%         each chunk is the KV for a set of tokens.
%         \item When a inference request query one context, first start with 
%         transmitting the KV cache of the first token-chunk with the least quality, 
%         together with the whole text context.
%         \item Starting from the second token-chunk, we will decide whether to transmit
%         the KV cache of which quantization level, or to generate KV cache from text context, based on throughput, TTFT SLO, and estimation of $T_{text}$ and $T_{\name}$
%     \end{itemize}
%     \item One of the key decisions in this adaptation logic is how to make the quantization level choice. 
%     We do this by choosing the quantization level corresponding to the largest TTFT within the SLO.
%     % Say the throughput suddenly drops from 1Gbps to 0.5 Gbps.
%     % To decide the quality of transmitting the next chunk, we first predict the delay of transmitting the KV at the throughput of 0.5Gbps, and selecting the highest quality below remaining SLO. 
%     \item Justify our logic is as good as optimal 
% \end{itemize}


During the transmission of one context, throughput change can happen as it may take hundreds of milliseconds 
or several seconds to complete, it is possible that there is throughput changes in the middle of transmitting one context. 
For example, Figure~\ref{fig:adaptation-case} shows an example of network bandwidth change (\ie dropping from 2~Gbps to 0.2~Gbps at 1 second, lasting for 2 seconds, then increasing to 1~Gbps) during the transmission of one context. 
At the start of the transmission, given an encoded KV cache of 1~GB and a latency SLO of 4 seconds, transmitting the encoded KV cache will be able to meet the SLO. 
However, due to the change in throughput, the actual transmission grows from 4 seconds to XX, leading to SLO violation. 





% , if sudden throughput changes happen, the original transmission plan may not be able to meet the latency Service Level Objective (SLO) anymore. 
% Here is a concrete example: say we want to transmit an encoded KV context of 1~GB.
% With an 8-second SLO and an initial throughput of 1Gbps, the streamer chooses to directly transmit KV context.
% However, if throughput drops to 0.5~Gbps after 2 seconds and returns to 1~Gbps 3 seconds later, the total transmission time will exceed SLO. 

This motivates the design of an adaptation module in the KV cache streamer.   
Specifically, we split the KV cache for one context into a few context-chunks, and send the context chunk-by-chunk.
Each of the chunks can independently take several actions based on throughput to meet the SLO. 
The actions include switching between multiple versions of \name's encoded KV cache, or generating the KV cache from text context from scratch. 



% Similar to any other lossy compression, each compressed cache of \name encoder represents one tradeoff point between size and quality. 
% Thus, we could save multiple versions of encoded KV cache to prepare for switching between compression levels during throughput fluctuations. 
% This approach is effective for short-term throughput changes. But if the throughput is low for a long time, using a smaller file might inevitably affect the quality of the LLM.

In the offline stage, we first encode the KV cache into separate versions with different quantization levels during the offline stage. 
By default, we select four settings that cover a range of size-quality tradeoff points. 
Then, we divide each KV cache into multiple context chunks. 
During streaming, 



% This allows \name to dynamically adapt to throughput changes in middle of transmission to deliver the best quality under SLO constraint.
Each context chunk contains 
the number of tokens,
% $\frac{max CC window}{ \alpha \times C \times L \times 2}$
 that is just large enough to fit in one congestion window in the datacenter to best utilize bandwidth~\cite{??}\footnote{Essentially it is $\frac{max CC window}{ \alpha \times C \times L \times 2}$, where $C$ is the number of Channels and $L$ is the number of layers in KV cache}. 
 % After quantization, the tensors are compressed by AC and stored on the storage server. 


During streaming, the streamer starts by sending the first chunk of the KV cache at the compression level with smallest size and the entire text context. 
Upon receiving every chunk, we use the following logic to decide whether to generate the KV cache from the text context or select an appropriate compression level for the next chunk:
\begin{equation*}
\begin{cases} 
\text{use text to recompute} & \text{if } T_{\text{text}}(L_{\text{rt}}, L_{\text{ct}}) < SLO, \\
\underset{Q}{\mathrm{argmax}} \text{ s.t. } T_{\text{kv}}(L_{\text{rt}},Q) < SLO & \text{otherwise.}
\end{cases}
\label{eq:adapt}
\end{equation*}

In the equation, $L_{rt}$ is the number of tokens yet to be received, $L_{ct}$ is the number of tokens that have already been received. The function $T_{kv}(L_{rt}, Q)$ \footnote{$T_{kv}(L_{rt}, Q) = \frac{\alpha \times Q \times C \times L_{rt} \times L}{Throughput} + RTT$, $\alpha$ is a constant of the model} predicts the delay for transmitting a KV cache with $L$ tokens at compression level $Q$, while $T_{text}(L_{rt}, L_{ct})$ \footnote{$T_{text}(L_{rt}, L_{ct}) = \gamma L_{ct} \times L_{rt}^2$, $\gamma$ is a constant of the model} predicts the delay for generating the KV cache from text. 

Our adaptation logic chooses the compression level that is predicted to deliver highest quality within the SLO.
Note that we use the throughput detected by the previous chunk to predict future throughput. While this approach may introduce some error to prediction, the performance stays strong (see \S\ref{sec:??}\hc{Yuhan plz fill}) since datacenter network bandwidths are relatively stable.

\yh{Several comments: 1. need to explain SLO clearly. 2. split into context-chunks, send chunk-by-chunk, each chunk can make  several actions independently based on throughput to adapt to SLO. 3. how to determine chunk size? How to encode it into several chnks? }


% \jc{i commented out the algorithm pseudocode. it's causing a lot of latex errors, and i don't think we really need a pseudocode to explain it. if it can be clearly explained in fewer words, please do that. a pseudocode is usually a sign that the idea is really complicated}
% \begin{algorithm}
% \caption{Get Function Algorithm}\label{alg:sender}
% \begin{algorithmic}[1]
%     \State $remaining\_SLO \gets SLO$
%     \State $all\_KV \gets None$
%     \For{$i \in \{1..N\}$}
%         \State $is\_text, kv\_quality \gets \Call{GetNextQuality}{i, throughput, remaining\_SLO}$
%         \State $all\_KV \gets all\_KV + \Call{GetNextChunk}{is\_text, kv\_quality, i}$
%     \EndFor
%     \State \Return $all\_KV$
% \end{algorithmic}
% \end{algorithm}




% %So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
% Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
% In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
% To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% % , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.





% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

% First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
% %, with larger compressed sizes generally resulting in higher TTFT but better quality.
% %As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
% By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
% The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
% %Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
% Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

% We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
% We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.


% %By default, we \jc{explain the default levels here.}


% %\shan{Please remind readers that the compression is done in
% %the background and hence not part of the TTFT, although
% %decompression is part of TTFT.}
% %The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

% %\jc{need to explain why kv can be compressed offline and refer to the limitation section}

% %beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

% In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
% \begin{align}
% {\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
% \label{eq:prediction1}
% \end{align}
% The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
% %\hc{provided bandwidth in data center?} 
% The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
% The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
% %$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


% In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
% \begin{align}
% {\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
% \label{eq:prediction2}
% \end{align}
% The first term is the round-trip-time (RTT) between the storage server and the GPU server.
% We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
% The second term is the GPU computation to compute the attention from scratch.

% With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
% If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


% The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
% In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% % \todo{Show analytical model to predict ttft here. }


% %When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
% %\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
% %\begin{align}
% %TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
% %\label{eq:prediction}
% %\end{align}



% %Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

% %At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
% %If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
% %It then selects the \kv version that fits within the time budget while maximizing its size. 

% %In addition to different compression levels, we also include the option of raw text of each potential context document. 
% %Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
% %decompression time would outweigh the computation time on
% %short text contexts.
% %
% %\jc{remember to explain why picking the compression level doesn't depend on the prompt}

% %\subsection{Putting all together}
% %\yh{todo}
% %\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, about 1K lines of CUDA kernel code, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
% We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
% Particularly, we use its encoding and decoding functions to perform AC. 
We implemented gpu-based AC library with CUDA.
\yh{talk to qizheng about implementation of gpu-based encoder}
Specifically, for decoding each CUDA thread is responsible for decoding the KV cache from bitstreams for one single token. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Integration into LLM inference framework} 
We integrate \name into LangChain~\cite{langchain}, a popular framework for building LLM applications.
Specifically, \name acts as a plugin module, receiving the input prompt, managing the loading of the KV cache, and calling the LLM to generate the response while bypassing the attention computation.
Thus, \name requires the underlying LLM to provide two interfaces:
(1) given a new prompt, LLM calculates the KV cache and return it to \name, 
and (2) given the KV cache (provided by \name), LLM resumes the inference while skipping the attention computation.
Many recent LLMs support the two functionalities by default. 
For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
%\name interacts with LLM inference via two simple interfaces:
%% To apply \name, the model inference pipeline to have incorporate two functionalities: 
%(1) \name extracts the KV features of a given context from an LLM inference, and 
%(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
%Many Pytorch-based LLMs support these APIs. 
%For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.

% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name}
\yh{Update this}
% To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.


==> backups/method-v9_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

We now present the design of \name, a concrete KV cache streamer for fast context-loading in LLM inference systems.
%, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
%\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

\begin{comment}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\end{comment}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

\tightsubsection{Context KV encoding}
\label{subsec:encoding}
\yh{Jumps too much from previous }
\yh{Emphasize the similarity with video coding. 
Before starting change-based encodingxxx, start by saying why blindly applying video techniques is not ok.

move the  insights in one zone.

Mention this is empirical observation. 

What we have is a representative dataset? 
}

%Some prior schemes \cite{xxxx} aim to \emph{shorten} KV features, with the shortened features still in the shape of KV tensors and directly consumed by LLMs with inevitable information losses. In contrast, our context encoder aims to \emph{compress} KV features, with the compressed features
%being a bitstream and will be decompressed before consumed by LLMs.
%No longer in the shape of KV tensors, this bitstream
%can take on a more compact representation of KV features 
%with minimum information losses. 
%\shan{I have reworded this paragraph. Among the three places that
%we discussed this set of related work (introduction, background),
%I like our discussion here the most, and I think we should
%reword the other places accordingly.}


% The overall workflow to compress the key-value caches consists of three key steps: (1) calculating the deltas among tokens; (2) picking the right quantization levels for each layer; (3) performing entropy coding with the right distribution. 
Recall from \S\ref{sec:delay} 
%\shan{really? where was this discussed? if it is in
%background section or something, please add a backward reference here.} 
that a KV cache of a context contains two tensors (K and V) of the same shape: 
$[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ are the number of tokens, layers, and channels, respectively.
\name compresses each tensor in three steps: 
\begin{packedenumerate}
\item calculate the delta tensors between nearby tokens; 
\item apply quantization to each layer of the delta tensors; and 
\item run the arithmetic coder on the quantized delta tensors.
\end{packedenumerate}


These steps of compressing KV features to a bitstream are conceptually similar to video coding (from pixel tensors to a .mp4 file), where each token's KV features can be seen as a frame. 
Yet, the exact design of \name is inspired by domain-specific insights on KV features produced by LLMs.

Next, we will explain each step along with the rationale behind it.


%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}  Our first insight is about the similarity between KV cache across nearby tokens.
%Particularly, we observe that:

%that if two tokens' positions are near to each other in the context, their KV feature values at the same channel and same layer are similar.

\begin{insight}
%{\bf{(Token-wise locality)}} 
At the same layer and channel, tokens in closer proximity have more similar KV cache values compared to tokens that are further apart.
\end{insight}

This {\em token-wise} locality 
%Why do KV features have such \emph{token-wise} locality? It does
%not necessarily mean nearby tokens themselves are similar
%or more correlated (and they are not). Rather, it 
stems from
the transformer (the self-attention) mechanism that computes the KV
cache. In essence, the KV cache for a given token index
are calculated based on the KV cache of previous tokens\footnote{More strictly, the KV cache are generated in a layer-by-layer manner. The KV of token index $t$ at layer $i$ is computed based on the attention matrix 
 from all the previous tokens' attention matrix at the previous layer~\cite{vaswani2023attention, attention2}.}.

% \jc{i know it's technically correct, but like you said many time, the conventional understanding is that KV is computed layer by layer, not token by token. it seems this claim is essential to the locality observation, can you add some text to explain it and also find any citations to back it up?}
% This dependency inherently leads to numerical similarity in their KV features across \emph{nearby} tokens in a context.


\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.7\linewidth]{figs/delta_insight.pdf}
    \tightcaption{\yh{Replace with real}} 
    \label{fig:delta_insight}
\end{figure}


This token-wise locality suggests an opportunity for better compression without affecting generation quality.
The values in the original KV tensors
% given one channel and layer,\jc{i don't think we really need to stress that it's a given channel or layer, do we?} 
might span a large range with a high variance.
However, if we compute the \emph{delta} between nearby tokens at each layer and channel, the distribution of the deltas will have a much smaller variance.
For instance, Figure~\ref{fig:delta_insight} shows that at a particular layer and channel, the distribution of original KV values has a much lower variance than the distribution of the delta values between two nearby tokens.
% the cumulative density function (CDF) of the original and delta KV features for one channel and one layer.
% As we can see, the delta KV features has smaller variance than the original ones. 

Since the distribution of delta values has a low variance and a mean around zero, it is well-known that it can be quantized and encoded to achieve a desirable size-loss tradeoff~\cite{doi:10.1080/03610928608829122}.
Specifically, most delta values are close to zero, so our quantization step (explained soon) can quantize them into a few distinct values with minimum information loss.
This results in a highly skewed distribution, \ie low entropy, so after arithmetic coding (explained soon), the distribution will have a small bitstream size. 

% \jc{yuhan, i rewrote the paragraph to simplify and smooth the text. please feel free to revert or edit the new text}
% If a distribution has smaller variance,
% it can be more easily compressed and has better size vs error tradeoff 
%  for reduced entropy~\cite{doi:10.1080/03610928608829122}.
% Intuitively, for a distribution with a smaller variance, there will be more repeated symbols in the data distribution after compression, specifically after non-uniform quantization (details in a later section). 
% These repeated symbols can be encoded with fewer bits, thereby reducing the overall size post-compression. Additionally, despite the reduced size, the error introduced by quantization remains minimal. To illustrate this, consider a quantization scheme that divides a distribution into two bins: one for values between 0 and 1, and another for all remaining values, with the quantized value being the bin's mean.
% For instance, a distribution like $[0.1, 0.5, 0.8, 1.5, 3]$ is quantized to $[0.7, 0.7, 0.7, 2.25, 2.25]$ resulting in an entropy value of 0.97. In contrast, a distribution such as $[0, 0.1, 0.2, 0.3, 1.2]$, which is quantized into $[0.15, 0.15, 0.15, 0.15, 1.2]$, this has an entropy of 0.72. 
% Moreover, the quantization error rates for these two distributions are 0.3 and 0.01, respectively.
% Thus, the repeated symbols can be represented with fewer bits, size after compression will be smaller. 
% Moreover, even though having smaller size, the error due to quantization will still be low. 
% As a simple illustrative example, consider the quantization scheme that bucketize a distribution into 2 bins, where values in between 0 and 1 into one bin, and other values into another, with the quantized value as the mean in the bins.
% If one distribution is $[0.1, 0.5, 0.8, 1.5, 3]$, the quantized values are $[0.7, 0.7, 0.7, 2.25, 2.25]$, leading to a entropy value of 0.97. 
% As for another distribution $[0, 0.1, 0.2, 0.3, 1.2]$, which is quantized into $[0.15, 0.15, 0.15, 0.15, 1.2]$, this has an entropy of 0.72. 
% Furthermore,  the error rate for the quantized data for the two is 0.3 and 0.01, respectively. 


% Since distributions with smaller variances have lower entropy\footnote{As the KV features is a normal distribution, many prior works have proved that smaller variance leads to lower entropy~\cite{??, ??, ??}. }, compressing the delta tensors instead of the original ones will be more beneficial. 

To utilize this token-wise locality of feature values, 
we employ the following idea: 

We partition all the tokens of a context into chunks of ten contiguous tokens. 
In each chunk, we compress the KV features of the first token, called the {\em anchor token}, independently (\ie without comparing it with other tokens), and then compress the delta tensor between each remaining token and the anchor token's decompressed features\footnote{Note that we compute the delta tensor between each remaining token and the \emph{decompressed} anchor token, so that the compression and decompression of remaining tokens in the group share the same reference to decode them. }. 


This process is analogous to video coding, where it also partitions the frames into chunks of contiguous frames. 
However, we are different from video coding in that we do not compress the delta between each pair of consecutive tokens, like in video frame encoding, because by comparing all tokens with the same anchor token in one chunk, we can greatly parallelize the compression and decompression of many tokens. 
% Second, the tokens within a chunk may not change as smoothly as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 


% \begin{figure}
% \centering
% %     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
%      \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{An example of KV values at the same layer and same channel across tokens.
%     We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
%     % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
%     % \jc{drop blue. and extend red to a wider range}
% %    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
% \shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
%     } 
%     \label{fig:delta_vis}
% \end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}


\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.





\mypara{Arithmetic coding} 
Next, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads ($\NumTokens\times\NumLayers\times\NumChannels$ distributions) on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext} and use the Llama-7B model to produce 3.8K KV feature tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

\begin{insight}
%{\bf{(Information gain)}}
In a KV cache, each element is distinguished by its channel, layer, and token index. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
\end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV features produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}

\mypara{Layer-wise quantization}
\yh{Earlier and later layers }
So far, the compression (running AC on delta tensors) has been lossless.
To further reduce the bandwidth usage of transferring the KV cache, \name also drops some information from the tokens while minimizing the impact on LLM's performance.
Specifically, \name uses quantization to reduce the precision of the elements in a KV cache so that they can be represented by fewer bits. 
% For instance, bucketizing a floating-point tensor into 4 bins make 
% For instance, bucketizing a floating-point tensor linearly rescales the original tensor to fit within the integer range of $[-2^3, 2^3]$.
% Recent methods propose to drop some tokens from the context~\cite{liu2023scissorhands,gisting,zhang2023ho}, but they must know the query (the prompt) to obtain the self-attention scores. 
% In contrast, we want to compress the KV feature before the query arrives. 
% \shan{this related work
% has been mentioned before, right? Can we not mention them again and again and again?}


% There are two potential approaches to dropping information. 

% One is to drop some tokens ()\jc{Yuhan, Ari seems to suggest there are many works in this space. can you add more related work and maybe update this statement}, but to determine which tokens are more important than others, they often assume knowledge of the query (the prompt part) of the input, because the important tokens are typically dependent on what the prompt is asking. 
% We do not take this approach because we want to compress KV features offline without seeing the prompt to avoid compression delay in TTFT.

%ask whether some information can be dropped, \ie lossy compression, but with minimum impact on the generation quality of the LLM. 
%There are two potential approaches.
%
%First, one can drop tokens from the context, but these methods (such as~\cite{liu2023scissorhands}) typically assume that the query (the prompt part) of the input is known in advance, because the important tokens are typically dependent on what the prompt is asking. 
%However, in our case, we want to pre-compress the KV features without seeing the prompt, in order to avoid compression delay.

%\name applies a specially designed quantization scheme that minimizes the impact on LLM's performance.

%This rescaling is achieved by multiplying $\frac{2^7}{max|X|}$ to the original tensor $X$, and then rounding the result to the nearest integer.
% dividing $2^7$ by the absolute maximum value present in the floating-point tensor.\jc{this sentence seems broken. please fix}
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}, but all elements are uniformly quantized with the same number of bits without leveraging any distributional properties of KV features.
%in~\cite{flexgen} to trade generation quality for memory footprint of KV features.
%Yet, it uniformly quantizes all elements of KV features with the same number of bits. 
It remains unclear what a better quantization strategy is to compress KV features while minimizing the impact on LLM's performance.

%quantization is a widely used in lossy compression to strike a balance between size reduction and the impact of loss on NN inference. 
%Quantization reduces the precision of a value so that it can be represented by fewer bits. 
%When applying quantization, we rescale the original floating-point tensor into discrete integer values based on quantization level.
%The quantization level is defined as the size of the integer. 

%To best use quantization, an important decision is whether we should quantize every element with the same number of bits. 
%Various quantization schemes have been studied in communication reduction literature of NN training. 
%Yet, it is still an emerging problem as to how quantization should be done on KV features in LLMs.\jc{it seems weird that no one has done this before. can you double check?}
%FlexGen~\cite{flexgen} recently proposes to reduce the GPU memory footprint of KV features apply uniform quantization all their elements.
%Though uniform quantization reduces the precision equally for all elements, it remains unclear that to preserve the LLM's output, whether all KV elements should be quantized to the same number of bits. 

Our insight is that the impact of quantizing KV elements on LLM's output varies with the layers of the elements.
Specifically, our insight can be summarized as follows:
%shallower layers are more sensitive to quantization. 
%Figure~\ref{??} shows that when the same level of quantization is applied to different layers separately, the impact on LLM's output, measured in perplexity, varies, with quantization having a greater effect when applied to the shallower layers.
%We can summarize this insight as follows.

\begin{insight}
%{\bf{(Layer-wise sensitivity)}}
The output from the LLM is more sensitive to losses in the KV feature values of the shallower layers than to those in the deeper layers.
\end{insight}

%Intuitively, shallower layers (closer to input) in LLMs indicate basic  (\eg basic sentence structure), while deeper layers extract more abstract features~\cite{egeria, ???}. 

Intuitively, KV features at the deeper layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV features of the shallower layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the shallow-layer features can propagate and affect the deeper-layer features and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{comment}
A naive solution of applying  quantization is to use the same quantization levels for \emph{all layers}. 
However, this solution is sub-optimal because different layers have different sensitivity to errors. 
Intuitively, shallower layers (closer to input) in LLMs  extract more low-level linguistic features (\eg basic sentence structure), while deeper layers extract more abstract feature 
~\cite{egeria, ???}. 
Thus, removing too much precision from the earlier layers may hinder the model's ability to grasp these fundamental linguistic features.
Even though deeper layers have little loss in precision, the propagating effects of shallower layers cannot be compromised. 


To illustrate, figure~\ref{fig:} shows the size and quality trade-offs for applying quantization on different layers. 
We can see that deeper layers have a better size and quality trade-offs than shallower layers, confirming our insight. 

\end{comment}

% Quantization, a well-established technique in machine learning, is employed to compress the model quantization ~\cite{llmint8, smoothquant, flexgen} with the objective of minimizing the runtime memory footprint of machine learning models. 
% Building upon prior work in model quantization~\cite{llmint8}, we present a specific method for quantizing the key-value cache denoted as $\Delta$. 
% The quantization procedure is described as follows:

% \begin{align}
%     \Delta_{\text{compressed}} = \lfloor \Delta \times (\frac{B}{max(|\Delta|)}) \rfloor
% \end{align}

% Where $B$ is determined by the quantization level. 
% $B$ represents the maximum absolute value of the integers resulting from the quantization process. 
% To illustrate, when transforming the original tensor from a 32-bit floating-point format into an 8-bit integer format (i.e., int8), the quantization maps the floating-point values into integers within the range [-127, 127]. 
% Consequently, in this scenario, $B$ is 127.

% The subsequent decompression process is the reverse of the quantization, converting the integers back into floating-point values through rescaling:

% \begin{align}
%     \Delta_{\text{decompressed}} = \frac{\Delta_{\text{compressed}} }{B} \times max(|\Delta|)
% \end{align}

% It is worth noting that quantization, unlike other techniques that reduce the dimensionality of key-value cache, maintains the original feature dimensionality but achieves size reduction by utilizing lower precision to represent the feature. 
% The error introduced during this quantization procedure is due to the fact that it approximates the original continuous values with a discrete set of quantized values, leading to information loss and approximation errors.

% It is intuitive to see that the lower the quantization level is (\ie using fewer bits), the more precision it will lose. 
% However, given that the key-value cache we are compressing originate from the forward pass of the Transformer models through all the layers, we find that the key-value features for different layers have different sensitivity of errors.
% Figure~\ref{fig:} shows the generation delay and quality trade-offs for different layers.
% We can see that deeper layers have better delay and quality trade-offs, indicating that using fewer bits to represent deeper layers is sufficient to reach good enough quality. 

% \jc{can we provide some intuitive explanation for why the difference in sensitivity? this is crucial for people to be convinced that this is not some random characteristics of a particular model or context. more generally, please provide such intuition for all other empirical observations in this section}
Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers, and apply different amount of quantization bin size on features at each layer group, respectively. 
The size of the quantization bin grows larger (\ie larger quantization errors)
from shallow to deeper layer groups. 
% Driven by this insight, we apply less aggressive quantization (more bits) on the features of shallower layers of delta tensors. 
% Specifically, we split the transformer layers into three layer groups, the first (shallowest) 1/3 of layers, the middle 1/3 of layers, the deepest 1/3 of layers,
% and apply $x$-bit, $y$-bit, and $z$-bit quantization on the features at each layer group, respectively.
% % and apply $x$-bit quantization on the first (shallowest) 1/3 of layers, $y$-bit on the second 1/3 of layers, and $z$-bit on the last 1/3 of layers.
% Each combination of $(x,y,z)$, where $x\geq y\geq z$, represents a tradeoff between compression size and loss of the LLM performance and \S\ref{subsec:controller} will explain the exact settings of quantization levels used in \name.

Note that we still use 8-bit quantization, a relatively high precision, on the KV features of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it makes sense to preserve higher precision just on these anchor tokens.

%We would like to  that though the quantization settings are empirically picked, they work well across a range of LLM models and datasets (\S\ref{subsec:sensitivity}), and future work can refine the quantization scheme.

% not the only way
% AC is recalculated

%With this insight, we propose using different levels of quantization of key-value features for different layers in a model, namely the \textit{quantization configuration} for such model.
%\jc{Yuhan, we should talk about how to present this. right now, it's a bit too low-level (though important details are still missing), and it doesnt explain the "why" either.}
%In general, we use a more aggressive quantization configuration on deeper layers and a less aggressive one on shallower layers. 
%
%To determine the optimal quantization configuration for a model, before runtime, a \textit{profiler} is run by the context encoder on the validation dataset to profile the impact of different quantization levels on the generation quality. For the purpose of this paper, we use quantization levels ranging from 3-bits to 8-bits (\ie 6 different quantization levels). Naively, we will need to run the number of layers to the power of 6 quantization configurations in total to fully understand the impact of quantization. 
%This can be both time and resource-consuming.
%Hence, to reduce the number of quantization configurations to profile, we apply two techniques.
%First, we evenly divide the layers into certain numbers of groups (a configurable parameter defaults to three groups) and all the layers in the same group will be quantized to the same level.
%Second, based on previous insight, for each group of layers, we define only a subset of possible configurations to profile. 
%This helps us reduce the number of quantization configurations to number of possible configurations in each group to the number of groups  ($2^3$ quantization configurations in our default setting).
%
%In our default setting, the possible configurations for the three layer groups are  \{8-bits, 7-bits\}, \{6-bits, 5-bits\}, \{4-bits, 3-bits\} respectively.  



% To be specific, we first divide all the layers into three groups of layers\footnote{xxx} based on the depth of the layers (\eg the first 1/3 of layers go to the first group etc.). 


% assign a range of different quantization levels we will profile to each group, \{8-bits, 6-bits\}, \{6-bits, 4-bits\}, \{4-bits, 3-bits\}.  

% \jc{can you expand this paragraph with more details? what exactly is the quantization level at each layer? how do you decide it? if it's statically configured, why these configurations don't need to be changed for different contexts or different models?}

\input{F/adaptation-case/fig-adaptation-case}

\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}

\yh{Doing edits now!! }


\yh{Not clear how we stream? 

Pseudocode 

drop the equation 
}

% \yh{Need a more concrete example, the starting throughput is \fillme, so xxxx. If not adapting, not meeting SLO. If adapting, will meet SLO. 
% predicting delay is trivial.
% The logic of adaptation is not trivial 

% motivation => frameworks => decision of adapt to which one (1. predict delay 2. how to adapt => why the prediction is good)
% }

% \begin{itemize}
%     \item When there are sudden network throughput changes, the initial KV transmission decision made by the streamer may not meet the SLO anymore. Concretely, for example, say we wanna transmit the KV cache of a Llama 13B model with 10K tokens.  (give an example where adapting the quantization level can help meet SLO) Also, note that our adaptation only works when there is a small timeframe of bandwidth change 
%     \item To make the choices of quantization levels, we use the following adaptation framework: 
%     \begin{itemize}
%         \item Offline encodes the KV cache of each context at multiple compression 
%         levels to cover a range of size-performance tradeoffs.
%         \item Split each version of the KV cache into multiple token-chunks, 
%         each chunk is the KV for a set of tokens.
%         \item When a inference request query one context, first start with 
%         transmitting the KV cache of the first token-chunk with the least quality, 
%         together with the whole text context.
%         \item Starting from the second token-chunk, we will decide whether to transmit
%         the KV cache of which quantization level, or to generate KV cache from text context, based on throughput, TTFT SLO, and estimation of $T_{text}$ and $T_{\name}$
%     \end{itemize}
%     \item One of the key decisions in this adaptation logic is how to make the quantization level choice. 
%     We do this by choosing the quantization level corresponding to the largest TTFT within the SLO.
%     % Say the throughput suddenly drops from 1Gbps to 0.5 Gbps.
%     % To decide the quality of transmitting the next chunk, we first predict the delay of transmitting the KV at the throughput of 0.5Gbps, and selecting the highest quality below remaining SLO. 
%     \item Justify our logic is as good as optimal 
% \end{itemize}


During the transmission of one context, throughput change can happen as it may take hundreds of milliseconds 
or several seconds to complete, it is possible that there is throughput changes in the middle of transmitting one context. 
For example, Figure~\ref{fig:adaptation-case} shows an example of network bandwidth change (\ie dropping from 2~Gbps to 0.2~Gbps at 1 second, lasting for 2 seconds, then increasing to 1~Gbps) during the transmission of one context. 
At the start of the transmission, given an encoded KV cache of 1~GB and a latency SLO of 4 seconds, transmitting the encoded KV cache will be able to meet the SLO. 
However, due to the change in throughput, the actual transmission grows from 4 seconds to XX, leading to SLO violation. 





% , if sudden throughput changes happen, the original transmission plan may not be able to meet the latency Service Level Objective (SLO) anymore. 
% Here is a concrete example: say we want to transmit an encoded KV context of 1~GB.
% With an 8-second SLO and an initial throughput of 1Gbps, the streamer chooses to directly transmit KV context.
% However, if throughput drops to 0.5~Gbps after 2 seconds and returns to 1~Gbps 3 seconds later, the total transmission time will exceed SLO. 

This motivates the design of an adaptation module in the KV cache streamer.   
Specifically, we split the KV cache for one context into a few context-chunks, and send the context chunk-by-chunk.
Each of the chunks can independently take several actions based on throughput to meet the SLO. 
The actions include switching between multiple versions of \name's encoded KV cache, or generating the KV cache from text context from scratch. 



% Similar to any other lossy compression, each compressed cache of \name encoder represents one tradeoff point between size and quality. 
% Thus, we could save multiple versions of encoded KV cache to prepare for switching between compression levels during throughput fluctuations. 
% This approach is effective for short-term throughput changes. But if the throughput is low for a long time, using a smaller file might inevitably affect the quality of the LLM.

In the offline stage, we first encode the KV cache into separate versions with different quantization levels during the offline stage. 
By default, we select four settings that cover a range of size-quality tradeoff points. 
Then, we divide each KV cache into multiple context chunks. 
During streaming, 



% This allows \name to dynamically adapt to throughput changes in middle of transmission to deliver the best quality under SLO constraint.
Each context chunk contains 
the number of tokens,
% $\frac{max CC window}{ \alpha \times C \times L \times 2}$
 that is just large enough to fit in one congestion window in the datacenter to best utilize bandwidth~\cite{??}\footnote{Essentially it is $\frac{max CC window}{ \alpha \times C \times L \times 2}$, where $C$ is the number of Channels and $L$ is the number of layers in KV cache}. 
 % After quantization, the tensors are compressed by AC and stored on the storage server. 


During streaming, the streamer starts by sending the first chunk of the KV cache at the compression level with smallest size and the entire text context. 
Upon receiving every chunk, we use the following logic to decide whether to generate the KV cache from the text context or select an appropriate compression level for the next chunk:
\begin{equation*}
\begin{cases} 
\text{use text to recompute} & \text{if } T_{\text{text}}(L_{\text{rt}}, L_{\text{ct}}) < SLO, \\
\underset{Q}{\mathrm{argmax}} \text{ s.t. } T_{\text{kv}}(L_{\text{rt}},Q) < SLO & \text{otherwise.}
\end{cases}
\label{eq:adapt}
\end{equation*}

In the equation, $L_{rt}$ is the number of tokens yet to be received, $L_{ct}$ is the number of tokens that have already been received. The function $T_{kv}(L_{rt}, Q)$ \footnote{$T_{kv}(L_{rt}, Q) = \frac{\alpha \times Q \times C \times L_{rt} \times L}{Throughput} + RTT$, $\alpha$ is a constant of the model} predicts the delay for transmitting a KV cache with $L$ tokens at compression level $Q$, while $T_{text}(L_{rt}, L_{ct})$ \footnote{$T_{text}(L_{rt}, L_{ct}) = \gamma L_{ct} \times L_{rt}^2$, $\gamma$ is a constant of the model} predicts the delay for generating the KV cache from text. 

Our adaptation logic chooses the compression level that is predicted to deliver highest quality within the SLO.
Note that we use the throughput detected by the previous chunk to predict future throughput. While this approach may introduce some error to prediction, the performance stays strong (see \S\ref{sec:??}\hc{Yuhan plz fill}) since datacenter network bandwidths are relatively stable.

\yh{Several comments: 1. need to explain SLO clearly. 2. split into context-chunks, send chunk-by-chunk, each chunk can make  several actions independently based on throughput to adapt to SLO. 3. how to determine chunk size? How to encode it into several chnks? }


% \jc{i commented out the algorithm pseudocode. it's causing a lot of latex errors, and i don't think we really need a pseudocode to explain it. if it can be clearly explained in fewer words, please do that. a pseudocode is usually a sign that the idea is really complicated}
% \begin{algorithm}
% \caption{Get Function Algorithm}\label{alg:sender}
% \begin{algorithmic}[1]
%     \State $remaining\_SLO \gets SLO$
%     \State $all\_KV \gets None$
%     \For{$i \in \{1..N\}$}
%         \State $is\_text, kv\_quality \gets \Call{GetNextQuality}{i, throughput, remaining\_SLO}$
%         \State $all\_KV \gets all\_KV + \Call{GetNextChunk}{is\_text, kv\_quality, i}$
%     \EndFor
%     \State \Return $all\_KV$
% \end{algorithmic}
% \end{algorithm}




% %So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
% Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
% In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
% To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% % , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.





% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

% First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
% %, with larger compressed sizes generally resulting in higher TTFT but better quality.
% %As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
% By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
% The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
% %Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
% Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

% We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
% We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.


% %By default, we \jc{explain the default levels here.}


% %\shan{Please remind readers that the compression is done in
% %the background and hence not part of the TTFT, although
% %decompression is part of TTFT.}
% %The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

% %\jc{need to explain why kv can be compressed offline and refer to the limitation section}

% %beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

% In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
% \begin{align}
% {\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
% \label{eq:prediction1}
% \end{align}
% The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
% %\hc{provided bandwidth in data center?} 
% The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
% The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
% %$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


% In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
% \begin{align}
% {\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
% \label{eq:prediction2}
% \end{align}
% The first term is the round-trip-time (RTT) between the storage server and the GPU server.
% We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
% The second term is the GPU computation to compute the attention from scratch.

% With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
% If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


% The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
% In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% % \todo{Show analytical model to predict ttft here. }


% %When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
% %\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
% %\begin{align}
% %TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
% %\label{eq:prediction}
% %\end{align}



% %Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

% %At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
% %If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
% %It then selects the \kv version that fits within the time budget while maximizing its size. 

% %In addition to different compression levels, we also include the option of raw text of each potential context document. 
% %Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
% %decompression time would outweigh the computation time on
% %short text contexts.
% %
% %\jc{remember to explain why picking the compression level doesn't depend on the prompt}

% %\subsection{Putting all together}
% %\yh{todo}
% %\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, about 1K lines of CUDA kernel code, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
% We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
% Particularly, we use its encoding and decoding functions to perform AC. 
We implemented gpu-based AC library with CUDA.
\yh{talk to qizheng about implementation of gpu-based encoder}
Specifically, for decoding each CUDA thread is responsible for decoding the KV cache from bitstreams for one single token. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Integration into LLM inference framework} 
We integrate \name into LangChain~\cite{langchain}, a popular framework for building LLM applications.
Specifically, \name acts as a plugin module, receiving the input prompt, managing the loading of the KV cache, and calling the LLM to generate the response while bypassing the attention computation.
Thus, \name requires the underlying LLM to provide two interfaces:
(1) given a new prompt, LLM calculates the KV cache and return it to \name, 
and (2) given the KV cache (provided by \name), LLM resumes the inference while skipping the attention computation.
Many recent LLMs support the two functionalities by default. 
For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
%\name interacts with LLM inference via two simple interfaces:
%% To apply \name, the model inference pipeline to have incorporate two functionalities: 
%(1) \name extracts the KV features of a given context from an LLM inference, and 
%(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
%Many Pytorch-based LLMs support these APIs. 
%For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.

% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name}
\yh{Update this}
% To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.


==> backups/motivate_v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{} 
    \label{fig:motivate_query_examples}
\end{figure*}

\section{Background}

\jc{Yuhan, please try your best to fill in missing text based on my comment. there are also a few figures i suggested we can add. feel free to ping me if you dont understand them. you should also feel free to reuse the text in your previous draft}

\subsection{Transformer basics}

The {\em Transformer-based} large language models has revolutionized the field of NLP, becoming the de-facto architecture for most state-of-the-art models in NLP tasks.
For this reason, we focus on Transformer-based models in this work.

A Transformer model takes as input a sequence of tokenized words, and generates as output a sequence of tokens. 
Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This process includes two high-level steps.
First, \jc{1-2 sentences here on how it encodes the prompt into kqv vectors}
Then, \jc{1-2 sentences here on the kqv vectors are fed to the decoder to iteratively generate tokens one by one}



\subsection{Augmenting LLM with ``memory'' text}

%\jc{here we should have a figure with three panels: 
%(a) the prompt includes only a short question, 
%(b) the prompt also includes a sequence of prior prompts and responses, and
%(c) the prompt includes multiple long documents and a question whose answer depends on the documents}

While the input prompt is used to be relatively short statement or question (Figure~\ref{fig:motivate_query_examples}(a)), most LLM applications today take long prompts.
Examples of such long prompt can be found in two types of applications. 

\mypara{Conversational applications (Figure~\ref{fig:motivate_query_examples}(b))}
\jc{give a few examples of prompt engineering or in-context learning, such as creating a character or following a sequence of instructions to finish a task, etc}
\jc{then explain how interactions become part of memory}

\mypara{Retrieval-base applications (Figure~\ref{fig:motivate_query_examples}(c))} 
\jc{give a few examples of retrieval-based tasks}
\jc{then explain how documents are selected (by knn for example) and then fed to the LLM}

%We refer to the applications that use prior interactions as memory {\em conversational applications}, and the applications that use auxiliary documents as memory {\em retrieval-based applications}.

It is noteworthy that in both types of applications, the long prompts consists of two parts: a relatively short question, following a potentially long text that is present before the short question.
We refer to this long text as the ``{\em memory}'' part of the prompt, which can be the conversation histories or segments from the supplementary documents.\footnote{The memory part of a prompt is referred to by different names depending on the applications. 
We use the term ``memory'' to refer to this part of the prompt to indicate that it is present before the last question is received.}

%This is because in addition to the question of interest, the prompt also includes a {\em memory} that helps enhance the quality of the generated response.\footnote{The term }

Memory text is playing an increasingly important role in LLM applications. 
It is no secrete that pre-trained LLMs alone do not contain enough information to answer complex questions or questions that require new knowledge that the model has not seen before.
Yet, retraining or even fine-tuning LLMs can be prohibitively expensive for most users. 
%The reason to have "memory" in LLM's input is the increasing realization that 
In the meantime, LLMs are quite powerful at extracting useful information from long input. 
Therefore, in-context learning
\jc{we need some citations for these arguments}


\begin{figure}
\centering
     \includegraphics[width=.9\linewidth]{figs/motivate_formulation.pdf}
    \tightcaption{} 
    \label{fig:motivate_formulation}
\end{figure}

\subsection{Optimization objective}
Given a prompt with memory, we want to minimize the delay to generate the first response token while maintaining the quality of the LLM response.
Note that because the memory size has little impact delay to generate remaining response tokens, we exclude it from our objective.
In retrieval-based applications, given a delay budget, we also try to increase the number of documents, thus improving response quality.
\jc{need a forward pointer to the definition of ``quality''}



\section{Motivation}

\subsection{Characteristics of LLM memory}

The intense efforts from research and industry to improve the quality of LLMs have several implications on the memory for LLMs in both conversational and retrieval-based applications. 

\mypara{Memory can be long}
\jc{use some citations and reasoning that memory is getting longer. in conversational apps, as user interact with LLMs over time, the history gets longer. 
similarly, in retrieval-based apps, people feed more documents (such as search results or a novel).
finally, LLMs are also designed to take longer and longer input}

\mypara{Memory can be dynamic}
\jc{we still need citations to explain why memory is not static. it is customized for each user (for conversational apps). it is also dependent on the query (for retrieval-based apps)}

\mypara{Memory can be distributed}
Memory often must be sent to the GPU running the LLM from a different server. 
\jc{i can think of at least three reasons 
(1) conversational app user goes idle for a long time and then resumes;
(2) retrieved documents are hosted by a different service/company; and 
(3) user moves from one location to another, thus served by different LLM servers.
can we find some citations/evidence for all three?}

Since many commercial LLMs are proprietary, there is little public statistics on how exactly they are used. 
Nonetheless, our hypothesize that these trends have or will materialize in commercial LLMs too.


\subsection{Representation of LLM memory}

These characteristics of LLM memory make it challenging to quickly load the memory such that LLM can generate response.

%\mypara{Design choices}
Memory can be stored in three ways, and they differ in two key aspects: size and compute overhead. 

\mypara{Tokens as memory}
\jc{briefly explain what this is. it represents one extreme of small size but high compute overhead}

\mypara{Self-attention matrix as memory}
\jc{briefly explain what this is. it represents the other extreme of large size but low compute overhead}

\mypara{Key-value features as memory}
\jc{briefly explain what this is. as a compromise, this choice has relatively lower size and low compute}

\jc{we need a figure here to illustrate the tradeoffs between the three choices}


\subsection{Why not loading key-value tensors?}

%\mypara{Growing size of key-value features}
Indeed, loading memory as key-value features is desirable, if the key-value tensors are always in GPU memory or is very small, but the size of key-value features can still be quite large, since it grows with both (1) the memory length, and (2) model dimension.
\jc{here, we need the figure yuhan drew before HotNets that shows the increase of key-value sizes in recent LLMs}

To make it concrete, we show the first-token generation delay if the key-value features are already in GPU RAM. 

\jc{explain the setup: dataset (prompts, etc), and then a few figures to show loading k-v cache vs. recomputing the self-attention
\begin{packeditemize}
\item delay vs. workloads
\item delay vs. history length
\item delay vs. models
\end{packeditemize}
}

Then we consider when key-value features are loaded over a link with bandwidth of \fillme. 
We can see that the benefit are negated.
\jc{refer to the figures}






%While this simple input/output process is stateless, in practice, many LLM applications augment the transformer input with various types of {\em memory}. 




%In practice, however, input prompt may contain a large number of tokens that are previously generated by the model or have been encoded by the model. 


==> backups/motivate_v2_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{} 
    \label{fig:motivate_query_examples}
\end{figure*}

\section{Background}

\jc{Yuhan, please try your best to fill in missing text based on my comment. there are also a few figures i suggested we can add. feel free to ping me if you dont understand them. you should also feel free to reuse the text in your previous draft}

\subsection{Transformer basics}

The {\em Transformer-based} large language models has revolutionized the field of NLP, becoming the de-facto architecture for most state-of-the-art models in NLP tasks.
For this reason, we focus on Transformer-based models in this work.

A Transformer model takes as input a sequence of tokenized words, and generates as output a sequence of tokens. 
Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This process includes two high-level steps.
First, \jc{1-2 sentences here on how it encodes the prompt into kqv vectors}
Then, \jc{1-2 sentences here on the kqv vectors are fed to the decoder to iteratively generate tokens one by one}



\subsection{Augmenting LLM with ``memory'' text}

%\jc{here we should have a figure with three panels: 
%(a) the prompt includes only a short question, 
%(b) the prompt also includes a sequence of prior prompts and responses, and
%(c) the prompt includes multiple long documents and a question whose answer depends on the documents}

While the input prompt is used to be relatively short statement or question (Figure~\ref{fig:motivate_query_examples}(a)), most LLM applications today take long prompts.
Examples of such long prompt can be found in two types of applications. 

\mypara{Conversational applications (Figure~\ref{fig:motivate_query_examples}(b))}
\jc{give a few examples of prompt engineering or in-context learning, such as creating a character or following a sequence of instructions to finish a task, etc}
\jc{then explain how interactions become part of memory}

\mypara{Retrieval-base applications (Figure~\ref{fig:motivate_query_examples}(c))} 
\jc{give a few examples of retrieval-based tasks}
\jc{then explain how documents are selected (by knn for example) and then fed to the LLM}

%We refer to the applications that use prior interactions as memory {\em conversational applications}, and the applications that use auxiliary documents as memory {\em retrieval-based applications}.

It is noteworthy that in both types of applications, the long prompts consists of two parts: a relatively short question, following a potentially long text that is present before the short question.
We refer to this long text as the ``{\em memory}'' part of the prompt, which can be the conversation histories or segments from the supplementary documents.\footnote{The memory part of a prompt is referred to by different names depending on the applications. 
We use the term ``memory'' to refer to this part of the prompt to indicate that it is present before the last question is received.}

%This is because in addition to the question of interest, the prompt also includes a {\em memory} that helps enhance the quality of the generated response.\footnote{The term }

Memory text is playing an increasingly important role in LLM applications. 
It is no secrete that pre-trained LLMs alone do not contain enough information to answer complex questions or questions that require new knowledge that the model has not seen before.
Yet, retraining or even fine-tuning LLMs can be prohibitively expensive for most users. 
%The reason to have "memory" in LLM's input is the increasing realization that 
In the meantime, LLMs are quite powerful at extracting useful information from long input. 
Therefore, in-context learning
\jc{we need some citations for these arguments}


\begin{figure}
\centering
     \includegraphics[width=.9\linewidth]{figs/motivate_formulation.pdf}
    \tightcaption{} 
    \label{fig:motivate_formulation}
\end{figure}

\subsection{Optimization objective}
Given a prompt with memory, we want to minimize the delay to generate the first response token while maintaining the quality of the LLM response.
Note that because the memory size has little impact delay to generate remaining response tokens, we exclude it from our objective.
In retrieval-based applications, given a delay budget, we also try to increase the number of documents, thus improving response quality.
\jc{need a forward pointer to the definition of ``quality''}



\section{Motivation}

\subsection{Characteristics of LLM memory}

The intense efforts from research and industry to improve the quality of LLMs have several implications on the memory for LLMs in both conversational and retrieval-based applications. 

\mypara{Memory can be long}
\jc{use some citations and reasoning that memory is getting longer. in conversational apps, as user interact with LLMs over time, the history gets longer. 
similarly, in retrieval-based apps, people feed more documents (such as search results or a novel).
finally, LLMs are also designed to take longer and longer input}

\mypara{Memory can be dynamic}
\jc{we still need citations to explain why memory is not static. it is customized for each user (for conversational apps). it is also dependent on the query (for retrieval-based apps)}

\mypara{Memory can be distributed}
Memory often must be sent to the GPU running the LLM from a different server. 
\jc{i can think of at least three reasons 
(1) conversational app user goes idle for a long time and then resumes;
(2) retrieved documents are hosted by a different service/company; and 
(3) user moves from one location to another, thus served by different LLM servers.
can we find some citations/evidence for all three?}

Since many commercial LLMs are proprietary, there is little public statistics on how exactly they are used. 
Nonetheless, our hypothesize that these trends have or will materialize in commercial LLMs too.


\subsection{Representation of LLM memory}

These characteristics of LLM memory make it challenging to quickly load the memory such that LLM can generate response.

%\mypara{Design choices}
Memory can be stored in three ways, and they differ in two key aspects: size and compute overhead. 

\mypara{Tokens as memory}
\jc{briefly explain what this is. it represents one extreme of small size but high compute overhead}

\mypara{Self-attention matrix as memory}
\jc{briefly explain what this is. it represents the other extreme of large size but low compute overhead}

\mypara{Key-value features as memory}
\jc{briefly explain what this is. as a compromise, this choice has relatively lower size and low compute}

\jc{we need a figure here to illustrate the tradeoffs between the three choices}


\subsection{Why not loading key-value tensors?}

%\mypara{Growing size of key-value features}
Indeed, loading memory as key-value features is desirable, if the key-value tensors are always in GPU memory or is very small, but the size of key-value features can still be quite large, since it grows with both (1) the memory length, and (2) model dimension.
\jc{here, we need the figure yuhan drew before HotNets that shows the increase of key-value sizes in recent LLMs}

To make it concrete, we show the first-token generation delay if the key-value features are already in GPU RAM. 

\jc{explain the setup: dataset (prompts, etc), and then a few figures to show loading k-v cache vs. recomputing the self-attention
\begin{packeditemize}
\item delay vs. workloads
\item delay vs. history length
\item delay vs. models
\end{packeditemize}
}

Then we consider when key-value features are loaded over a link with bandwidth of \fillme. 
We can see that the benefit are negated.
\jc{refer to the figures}






%While this simple input/output process is stateless, in practice, many LLM applications augment the transformer input with various types of {\em memory}. 




%In practice, however, input prompt may contain a large number of tokens that are previously generated by the model or have been encoded by the model. 


==> backups/motivate_v3.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{} 
    \label{fig:motivate_query_examples}
\end{figure*}

\section{Background and Motivation}

%\jc{please try the best to fill in missing text based on my comment. there are also a few figures i suggested we can add. feel free to ping me if you dont understand them. you should also feel free to reuse the text in your previous draft}

\subsection{Transformer basics}

{\em Transformer} models have revolutionized the field of NLP, becoming the de-facto architecture for most state-of-the-art models in NLP tasks.
For this reason, we focus on transformer-based LLMs in this work.


A transformer model takes as input a prompt which is a sequence of tokenized words\jc{is tokenization part of the transformer framework?}, and generates as output a response, which is another sequence of tokens. 
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This process includes two high-level steps.
First, \jc{1-2 sentences here on how it encodes the prompt into kqv vectors}
Then, \jc{1-2 sentences here on the kqv vectors are fed to the decoder to iteratively generate tokens one by one}



%\subsection{Augmenting LLM with ``memory'' text}
\subsection{Use of ``context'' in LLM applications}

%\jc{here we should have a figure with three panels: 
%(a) the prompt includes only a short question, 
%(b) the prompt also includes a sequence of prior prompts and responses, and
%(c) the prompt includes multiple long documents and a question whose answer depends on the documents}

While an input to the LLM usually contains only the immediate last prompt, which is a relatively short statement or question (Figure~\ref{fig:motivate_query_examples}(a)), in more applications today, the LLM input tends to precede\footnote{The context is put ahead of the immediate prompt in most cases~\cite{??,??,??}, so in this work we assume it is the prefix of the LLM input.} the immediate prompt with more {\em context}\footnote{The memory part of a prompt is referred to by different names depending on the applications. We use the term ``context'' in lack of an umbrella term in the literature.} text to enhance the generation quality.
Since these contexts are often automatically added, users do not notice them or manually type in longer prompt.



The use of contexts can be found in various applications. 
Here we highlight two general types of such applications. 
In \S\ref{sec:eval}, we will evaluate our performance in representative datasets of these applications.

\mypara{Retrieval-based applications (Figure~\ref{fig:motivate_query_examples}(b))} 

\jc{\begin{itemize}
\item start with a general background of knowledge base, query, and retrieval logic. 
\item give a few examples from those retrieval-based learning papers. reading a book or a database of specialized knowledge would be good examples
\end{itemize}}

\mypara{Conversational applications (Figure~\ref{fig:motivate_query_examples}(c))}

\jc{\begin{itemize}
\item start with a general description of user-LLM interactions and why the previous interactions (conversation history) become useful context. 
\item give a few examples for long-context learning and few-shot learning. things to consider: (1) a series of prompts to create a character before interacting with it. (2) giving a bunch of long examples with correct answers to teach LLM some knowledge and then asking the real question, etc
\end{itemize}}

%We refer to the applications that use prior interactions as memory {\em conversational applications}, and the applications that use auxiliary documents as memory {\em retrieval-based applications}.


%\begin{figure}
%\centering
%     \includegraphics[width=.94\linewidth]{figs/motivate_formulation.pdf}
%    \tightcaption{} 
%    \label{fig:motivate_formulation}
%\end{figure}



%the LLM input consists of two parts: a potentially long {\em context} text followed by a relatively short prompt.
%Here, the context might be the conversation histories or segments from the supplementary documents.\footnote{The memory part of a prompt is referred to by different names depending on the applications. We use the term ``context'' in lack of an umbrella term in the literature.}
%to refer to this part of the prompt to indicate that it is present before the last question is received.}

%after a potentially long context text that is present before the short question.
%We refer to this long text as the ``{\em memory}'' part of the prompt, which can be the conversation histories or segments from the supplementary documents.\footnote{The memory part of a prompt is referred to by different names depending on the applications. 
%We use the term ``memory'' to refer to this part of the prompt to indicate that it is present before the last question is received.}

%This is because in addition to the question of interest, the prompt also includes a {\em memory} that helps enhance the quality of the generated response.\footnote{The term }

Context is playing an increasingly important role in LLM applications. 
Since the pre-trained LLMs alone do not always contain enough information to answer complex questions or questions that require new knowledge that the model has not seen before.
Yet, retraining or even fine-tuning LLMs can be prohibitively expensive for most users. 
%The reason to have "memory" in LLM's input is the increasing realization that 
In the meantime, LLMs are quite powerful at learning useful information embedded in text, even if the text is over tens of thousands of tokens~\cite{??}.\footnote{LLM is a fast evolving literature, and latest LLMs can even take a whole book as the context in an input~\cite{??,??}.}
Therefore, feeding the context as part of the LLM input to let LLM learn from the context is a popular choice.
\jc{we need some citations for these arguments}

\begin{figure}[t]
\centering
     \includegraphics[width=.8\linewidth]{figs/motivate_long_input.pdf}
    \tightcaption{} 
    \label{fig:motivate_long_input}
\end{figure}

\begin{figure*}[t]
\centering
     \includegraphics[width=.9\linewidth]{figs/motivate_baselines.pdf}
    \tightcaption{} 
    \label{fig:motivate_baselines}
\end{figure*}



It is also noteworthy that, in both conversational applications and retrieval-based applications, the context part of the input is present {\em before} the prompt is received.
\jc{elaborate a bit in terms of both applications}

\subsection{Characteristics of context in LLM}

%The intense efforts from research and industry to improve the quality of LLMs have several implications on the context in LLMs, in both conversational and retrieval-based applications. 

\mypara{Context can be pre-processed}
\jc{in conversation apps, the conversation histories are known and even processed by LLM before the current prompt. 
in retrieval-based apps, the knowledge base is known in advance and re-used for future queries.}

\mypara{Context needs to be fetched remotely}
The context of an LLM input often needs to be fetched from a different server. 
\jc{i can think of at least three reasons 
(1) retrieved documents are hosted by a different service/company; and 
(2) conversational app user goes idle for a long time and then resumes;
(3) user moves from one location to another, thus served by different LLM servers.
can we find some citations/evidence for all three?}

In this work, we assume that the context resides in a different machine than the GPUs running the LLM.

\mypara{Context can be long}
\jc{use some citations and reasoning that memory is getting longer. in conversational apps, as user interact with LLMs over time, the history gets longer. 
similarly, in retrieval-based apps, people feed more documents (such as search results or a novel).
finally, LLMs are also designed to take longer and longer input. use Figure~\ref{fig:motivate_long_input}.}

%\mypara{Context can be dynamic}
%\jc{we still need citations to explain why context is not static. it is customized for each user (for conversational apps). it is also dependent on the query (for retrieval-based apps)}

Since many commercial LLMs are proprietary, there is little public statistics on how exactly they are used. 
Nonetheless, our hypothesize that these trends have or will materialize in commercial LLMs too.




\subsection{Metrics and objectives}

\mypara{Delay metric}
We define {\em time-to-first-token (TTFT) delay} by the time between receiving the prompt and generating the first token. 
While LLM systems sometime reduce the total generation delay (the sum of TTFT and the delay to autoregressively generate response tokens), we choose not to use this metric  because 
(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
(2) we want to focus the delay reduction on processing input faster, not by generating fewer tokens.

Since the context resides in a different machine than the GPUs running the LLM, the TTFT delay consists of 
(1) the {\em communication} delay to fetch the context to GPU memory and 
(2) the {\em computation} delay to process the context and prompt before generating the first token.


\mypara{Quality metric}
We then define {\em generation quality degradation} by how close the generated text under any speedup of input processing is to the text generated when letting the LLM process the context and the prompt from scratch, which is the unoptimized implementation. 
In other words, generation quality degradation measures the impact of speedup on generated text.
If the speedup of input processing does not change the generated output, the quality will be the highest, but sometimes the speedup is achieved by dropping information, yielding a different generation text.

Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
\S\ref{subsec:eval:setup} will describe these metrics in more detail.

\mypara{Objectives}
With these definitions, the objective of this paper can be formulated as follows.
{\em How to minimize the TTFT delay with minimum generation quality degradation?}
Essentially, all methods, including ours, strike some tradeoffs between TTFT delay and generation quality.
Thus, in practice, we will show our improvement by comparing the TTFT delay of two methods under the same generation quality degradation.

\begin{figure*}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/design_choices.pdf}
    \tightcaption{} 
    \label{fig:design_choices}
\end{figure*}

%Given a prompt with context, we want to minimize the delay to generate the first response token while maintaining the quality of the LLM response.
%(Because the context length has little impact delay to generate remaining response tokens, we exclude it from our objective.)
%In retrieval-based applications, given a delay budget, we also try to increase the number of documents, thus improving response quality.
%\jc{need a forward pointer to the definition of ``quality''}

\jc{Update stopped here}


\section{Design space and tradeoffs}

While focused directly on reducing TTFT with remotely fetched long context, several existing ideas can already affect the delay-quality tradeoff.
At a high level, there are three design choices. \jc{explain each choice. can use Figure~\ref{fig:motivate_baselines}}

%0. Load all context in words
%1. Context word selection
%2. Pre-compute and load key-value features
%3. Smaller model or quantized model
\begin{packeditemize}

\item {\em Choice 1: Reduce context length.}

\item {\em Choice 2: Load compressed key-value features.}

\item {\em Choice 3: Use smaller models.}

\end{packeditemize}

To analyze the tradeoff, let's assume the context has $N$ tokens and the prompt has $k$ tokens ($N>>k$).
All designs strike some tradeoffs between quality and TTFT delay, which can be break down to communication delay to fetch the context and the computation delay to process context and the prompt.
The unoptimized design would load all $N$ context tokens as plain text, yielding a small communication delay but a computation delay of $O(N^2)$.

The three aforementioned design choices make different tradeoffs between quality and TTFT delay, which can be break down to communication delay to fetch the context and the computation delay to process context and the prompt.
Compared to the baseline of loading context as raw text, reducing context length from $N$ to $n$ reduces the computation delay from $O(N+k)$


\jc{use figure~\ref{fig:design_choices} to quantify these points}




\begin{comment}

These characteristics of LLM memory make it challenging to quickly load the memory such that LLM can generate response.

%\mypara{Design choices}
Memory can be stored in three ways, and they differ in two key aspects: size and compute overhead. 

\mypara{Tokens as memory}
\jc{briefly explain what this is. it represents one extreme of small size but high compute overhead}

\mypara{Self-attention matrix as memory}
\jc{briefly explain what this is. it represents the other extreme of large size but low compute overhead}

\mypara{Key-value features as memory}
\jc{briefly explain what this is. as a compromise, this choice has relatively lower size and low compute}

\jc{we need a figure here to illustrate the tradeoffs between the three choices}


%\subsection{Why not loading key-value tensors?}

%\mypara{Growing size of key-value features}
Indeed, loading memory as key-value features is desirable, if the key-value tensors are always in GPU memory or is very small, but the size of key-value features can still be quite large, since it grows with both (1) the memory length, and (2) model dimension.
\jc{here, we need the figure yuhan drew before HotNets that shows the increase of key-value sizes in recent LLMs}

To make it concrete, we show the first-token generation delay if the key-value features are already in GPU RAM. 

\jc{explain the setup: dataset (prompts, etc), and then a few figures to show loading k-v cache vs. recomputing the self-attention
\begin{packeditemize}
\item delay vs. workloads
\item delay vs. history length
\item delay vs. models
\end{packeditemize}
}

Then we consider when key-value features are loaded over a link with bandwidth of \fillme. 
We can see that the benefit are negated.
\jc{refer to the figures}

\end{comment}






%While this simple input/output process is stateless, in practice, many LLM applications augment the transformer input with various types of {\em memory}. 




%In practice, however, input prompt may contain a large number of tokens that are previously generated by the model or have been encoded by the model. 


==> backups/motivate_v3_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{} 
    \label{fig:motivate_query_examples}
\end{figure*}

\section{Background and Motivation}

%\jc{please try the best to fill in missing text based on my comment. there are also a few figures i suggested we can add. feel free to ping me if you dont understand them. you should also feel free to reuse the text in your previous draft}

\subsection{Transformer basics}

{\em Transformer} models have revolutionized the field of NLP, becoming the de-facto architecture for most state-of-the-art models in NLP tasks.
For this reason, we focus on transformer-based LLMs in this work.


A transformer model takes as input a prompt which is a sequence of tokenized words\jc{is tokenization part of the transformer framework?}, and generates as output a response, which is another sequence of tokens. 
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This process includes two high-level steps.
First, \jc{1-2 sentences here on how it encodes the prompt into kqv vectors}
Then, \jc{1-2 sentences here on the kqv vectors are fed to the decoder to iteratively generate tokens one by one}



%\subsection{Augmenting LLM with ``memory'' text}
\subsection{Use of ``context'' in LLM applications}

%\jc{here we should have a figure with three panels: 
%(a) the prompt includes only a short question, 
%(b) the prompt also includes a sequence of prior prompts and responses, and
%(c) the prompt includes multiple long documents and a question whose answer depends on the documents}

While an input to the LLM usually contains only the immediate last prompt, which is a relatively short statement or question (Figure~\ref{fig:motivate_query_examples}(a)), in more applications today, the LLM input tends to precede\footnote{The context is put ahead of the immediate prompt in most cases~\cite{??,??,??}, so in this work we assume it is the prefix of the LLM input.} the immediate prompt with more {\em context}\footnote{The memory part of a prompt is referred to by different names depending on the applications. We use the term ``context'' in lack of an umbrella term in the literature.} text to enhance the generation quality.
Since these contexts are often automatically added, users do not notice them or manually type in longer prompt.



The use of contexts can be found in various applications. 
Here we highlight two general types of such applications. 
In \S\ref{sec:eval}, we will evaluate our performance in representative datasets of these applications.

\mypara{Retrieval-based applications (Figure~\ref{fig:motivate_query_examples}(b))} 

\jc{\begin{itemize}
\item start with a general background of knowledge base, query, and retrieval logic. 
\item give a few examples from those retrieval-based learning papers. reading a book or a database of specialized knowledge would be good examples
\end{itemize}}

\mypara{Conversational applications (Figure~\ref{fig:motivate_query_examples}(c))}

\jc{\begin{itemize}
\item start with a general description of user-LLM interactions and why the previous interactions (conversation history) become useful context. 
\item give a few examples for long-context learning and few-shot learning. things to consider: (1) a series of prompts to create a character before interacting with it. (2) giving a bunch of long examples with correct answers to teach LLM some knowledge and then asking the real question, etc
\end{itemize}}

%We refer to the applications that use prior interactions as memory {\em conversational applications}, and the applications that use auxiliary documents as memory {\em retrieval-based applications}.


%\begin{figure}
%\centering
%     \includegraphics[width=.94\linewidth]{figs/motivate_formulation.pdf}
%    \tightcaption{} 
%    \label{fig:motivate_formulation}
%\end{figure}



%the LLM input consists of two parts: a potentially long {\em context} text followed by a relatively short prompt.
%Here, the context might be the conversation histories or segments from the supplementary documents.\footnote{The memory part of a prompt is referred to by different names depending on the applications. We use the term ``context'' in lack of an umbrella term in the literature.}
%to refer to this part of the prompt to indicate that it is present before the last question is received.}

%after a potentially long context text that is present before the short question.
%We refer to this long text as the ``{\em memory}'' part of the prompt, which can be the conversation histories or segments from the supplementary documents.\footnote{The memory part of a prompt is referred to by different names depending on the applications. 
%We use the term ``memory'' to refer to this part of the prompt to indicate that it is present before the last question is received.}

%This is because in addition to the question of interest, the prompt also includes a {\em memory} that helps enhance the quality of the generated response.\footnote{The term }

Context is playing an increasingly important role in LLM applications. 
Since the pre-trained LLMs alone do not always contain enough information to answer complex questions or questions that require new knowledge that the model has not seen before.
Yet, retraining or even fine-tuning LLMs can be prohibitively expensive for most users. 
%The reason to have "memory" in LLM's input is the increasing realization that 
In the meantime, LLMs are quite powerful at learning useful information embedded in text, even if the text is over tens of thousands of tokens~\cite{??}.\footnote{LLM is a fast evolving literature, and latest LLMs can even take a whole book as the context in an input~\cite{??,??}.}
Therefore, feeding the context as part of the LLM input to let LLM learn from the context is a popular choice.
\jc{we need some citations for these arguments}

\begin{figure}[t]
\centering
     \includegraphics[width=.8\linewidth]{figs/motivate_long_input.pdf}
    \tightcaption{} 
    \label{fig:motivate_long_input}
\end{figure}

\begin{figure*}[t]
\centering
     \includegraphics[width=.9\linewidth]{figs/motivate_baselines.pdf}
    \tightcaption{} 
    \label{fig:motivate_baselines}
\end{figure*}



It is also noteworthy that, in both conversational applications and retrieval-based applications, the context part of the input is present {\em before} the prompt is received.
\jc{elaborate a bit in terms of both applications}

\subsection{Characteristics of context in LLM}

%The intense efforts from research and industry to improve the quality of LLMs have several implications on the context in LLMs, in both conversational and retrieval-based applications. 

\mypara{Context can be pre-processed}
\jc{in conversation apps, the conversation histories are known and even processed by LLM before the current prompt. 
in retrieval-based apps, the knowledge base is known in advance and re-used for future queries.}

\mypara{Context needs to be fetched remotely}
The context of an LLM input often needs to be fetched from a different server. 
\jc{i can think of at least three reasons 
(1) retrieved documents are hosted by a different service/company; and 
(2) conversational app user goes idle for a long time and then resumes;
(3) user moves from one location to another, thus served by different LLM servers.
can we find some citations/evidence for all three?}

In this work, we assume that the context resides in a different machine than the GPUs running the LLM.

\mypara{Context can be long}
\jc{use some citations and reasoning that memory is getting longer. in conversational apps, as user interact with LLMs over time, the history gets longer. 
similarly, in retrieval-based apps, people feed more documents (such as search results or a novel).
finally, LLMs are also designed to take longer and longer input. use Figure~\ref{fig:motivate_long_input}.}

%\mypara{Context can be dynamic}
%\jc{we still need citations to explain why context is not static. it is customized for each user (for conversational apps). it is also dependent on the query (for retrieval-based apps)}

Since many commercial LLMs are proprietary, there is little public statistics on how exactly they are used. 
Nonetheless, our hypothesize that these trends have or will materialize in commercial LLMs too.




\subsection{Metrics and objectives}

\mypara{Delay metric}
We define {\em time-to-first-token (TTFT) delay} by the time between receiving the prompt and generating the first token. 
While LLM systems sometime reduce the total generation delay (the sum of TTFT and the delay to autoregressively generate response tokens), we choose not to use this metric  because 
(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
(2) we want to focus the delay reduction on processing input faster, not by generating fewer tokens.

Since the context resides in a different machine than the GPUs running the LLM, the TTFT delay consists of 
(1) the {\em communication} delay to fetch the context to GPU memory and 
(2) the {\em computation} delay to process the context and prompt before generating the first token.


\mypara{Quality metric}
We then define {\em generation quality degradation} by how close the generated text under any speedup of input processing is to the text generated when letting the LLM process the context and the prompt from scratch, which is the unoptimized implementation. 
In other words, generation quality degradation measures the impact of speedup on generated text.
If the speedup of input processing does not change the generated output, the quality will be the highest, but sometimes the speedup is achieved by dropping information, yielding a different generation text.

Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
\S\ref{subsec:eval:setup} will describe these metrics in more detail.

\mypara{Objectives}
With these definitions, the objective of this paper can be formulated as follows.
{\em How to minimize the TTFT delay with minimum generation quality degradation?}
Essentially, all methods, including ours, strike some tradeoffs between TTFT delay and generation quality.
Thus, in practice, we will show our improvement by comparing the TTFT delay of two methods under the same generation quality degradation.

\begin{figure*}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/design_choices.pdf}
    \tightcaption{} 
    \label{fig:design_choices}
\end{figure*}

%Given a prompt with context, we want to minimize the delay to generate the first response token while maintaining the quality of the LLM response.
%(Because the context length has little impact delay to generate remaining response tokens, we exclude it from our objective.)
%In retrieval-based applications, given a delay budget, we also try to increase the number of documents, thus improving response quality.
%\jc{need a forward pointer to the definition of ``quality''}

\jc{Update stopped here}


\section{Design space and tradeoffs}

While focused directly on reducing TTFT with remotely fetched long context, several existing ideas can already affect the delay-quality tradeoff.
At a high level, there are three design choices. \jc{explain each choice. can use Figure~\ref{fig:motivate_baselines}}

%0. Load all context in words
%1. Context word selection
%2. Pre-compute and load key-value features
%3. Smaller model or quantized model
\begin{packeditemize}

\item {\em Choice 1: Reduce context length.}

\item {\em Choice 2: Load compressed key-value features.}

\item {\em Choice 3: Use smaller models.}

\end{packeditemize}

To analyze the tradeoff, let's assume the context has $N$ tokens and the prompt has $k$ tokens ($N>>k$).
All designs strike some tradeoffs between quality and TTFT delay, which can be break down to communication delay to fetch the context and the computation delay to process context and the prompt.
The unoptimized design would load all $N$ context tokens as plain text, yielding a small communication delay but a computation delay of $O(N^2)$.

The three aforementioned design choices make different tradeoffs between quality and TTFT delay, which can be break down to communication delay to fetch the context and the computation delay to process context and the prompt.
Compared to the baseline of loading context as raw text, reducing context length from $N$ to $n$ reduces the computation delay from $O(N+k)$


\jc{use figure~\ref{fig:design_choices} to quantify these points}




\begin{comment}

These characteristics of LLM memory make it challenging to quickly load the memory such that LLM can generate response.

%\mypara{Design choices}
Memory can be stored in three ways, and they differ in two key aspects: size and compute overhead. 

\mypara{Tokens as memory}
\jc{briefly explain what this is. it represents one extreme of small size but high compute overhead}

\mypara{Self-attention matrix as memory}
\jc{briefly explain what this is. it represents the other extreme of large size but low compute overhead}

\mypara{Key-value features as memory}
\jc{briefly explain what this is. as a compromise, this choice has relatively lower size and low compute}

\jc{we need a figure here to illustrate the tradeoffs between the three choices}


%\subsection{Why not loading key-value tensors?}

%\mypara{Growing size of key-value features}
Indeed, loading memory as key-value features is desirable, if the key-value tensors are always in GPU memory or is very small, but the size of key-value features can still be quite large, since it grows with both (1) the memory length, and (2) model dimension.
\jc{here, we need the figure yuhan drew before HotNets that shows the increase of key-value sizes in recent LLMs}

To make it concrete, we show the first-token generation delay if the key-value features are already in GPU RAM. 

\jc{explain the setup: dataset (prompts, etc), and then a few figures to show loading k-v cache vs. recomputing the self-attention
\begin{packeditemize}
\item delay vs. workloads
\item delay vs. history length
\item delay vs. models
\end{packeditemize}
}

Then we consider when key-value features are loaded over a link with bandwidth of \fillme. 
We can see that the benefit are negated.
\jc{refer to the figures}

\end{comment}






%While this simple input/output process is stateless, in practice, many LLM applications augment the transformer input with various types of {\em memory}. 




%In practice, however, input prompt may contain a large number of tokens that are previously generated by the model or have been encoded by the model. 


==> backups/motivate_v4.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{} 
    \label{fig:motivate_query_examples}
\end{figure*}

\section{Background and Motivation}

\subsection{Transformer basics}
\label{subsec:transformer}

{\em Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks.
Most popular generative NLP services these days are based on transformer models, including GPT, LLaMA, \jc{more names}. 
For this reason, we focus on transformer-based LLMs in this work.

Here, we provide a general introduction of the transformer architecture. 
We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
Readers can refer to \fillme for a more involved introduction.

A transformer model takes as input a sequence of tokenized words\jc{is tokenization part of the transformer framework?}, and generates as output a response, which is another sequence of tokens. \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This generation process includes two high-level steps.
First, \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
Then, \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

The key of the transformer architecture is a neural network (NN) called attention module. 
Each layer of the attention module producing an attention matrix, which describes the connections between each pair of tokens. 
The attention matrix at one layer is obtained by applying a non-linear NN operation on the attention matrix of the last layer.
Intuitively, the attention matrices of deeper layers might embed more complex understanding of tokens under consideration. 

The attention module is a powerful tool to model a sequence of tokens at the expense of computational and storage overheads. 
Given an input of $\NumTokens$ tokens, the computation and space overhead of computing the attention matrices will grow quadratically, $O(\NumTokens^2)$.
Though the overheads could be reduced to $O(\NumTokens\textrm{log}\NumTokens)$ (\eg~\cite{??,??,??,??}), it usually also degrade the quality of generation. 
Note that once the attention matrices of the input are obtained, the time to generate each token is quite marginal and can be reduced to almost constant on GPUs. 

%The intermediate outcome of the first step is called key-value features, or KV features. 

\subsection{Long context in LLM applications}

While an input to the LLM usually contains only the immediate last prompt, which is a relatively short statement or question (Figure~\ref{fig:motivate_query_examples}(a)), in more applications today, the LLM input tends to precede\footnote{The context is put ahead of the immediate prompt in most cases~\cite{??,??,??}, so in this work we assume it is the prefix of the LLM input.} the immediate prompt with more {\em context}\footnote{The memory part of a prompt is referred to by different names depending on the applications. We use the term ``context'' in lack of an umbrella term in the literature.} text to enhance the generation quality.
Since these contexts are often automatically added, users do not notice them or manually type in longer prompt.

\myparaq{Why context}
The use of contexts can be found in various applications.
Here we highlight two general types of such applications. 
In \S\ref{sec:eval}, we will evaluate our performance in representative datasets of these applications.
\begin{packeditemize}

\item{\em Retrieval-based applications (Figure~\ref{fig:motivate_query_examples}(b)):} 

\jc{\begin{itemize}
\item start with a general background of knowledge base, query, and retrieval logic. 
\item give a few examples from those retrieval-based learning papers. reading a book or a database of specialized knowledge would be good examples
\end{itemize}}

\item {\em Conversational applications (Figure~\ref{fig:motivate_query_examples}(c)):}

\jc{\begin{itemize}
\item start with a general description of user-LLM interactions and why the previous interactions (conversation history) become useful context. 
\item give a few examples for long-context learning and few-shot learning. things to consider: (1) a series of prompts to create a character before interacting with it. (2) giving a bunch of long examples with correct answers to teach LLM some knowledge and then asking the real question, etc
\end{itemize}}

\end{packeditemize}

\jc{clarify the terminology of prompt, context, input, query, etc}



%\mypara{Why context is important}
Context is playing an increasingly important role in LLM applications. 
Since the pre-trained LLMs alone do not always contain enough information to answer complex questions or questions that require new knowledge that the model has not seen before.
Yet, retraining or even fine-tuning LLMs can be prohibitively expensive for most users. 
%The reason to have "memory" in LLM's input is the increasing realization that 
In the meantime, LLMs are quite powerful at learning useful information embedded in text, even if the text is over tens of thousands of tokens~\cite{??}.\footnote{LLM is a fast evolving literature, and latest LLMs can even take a whole book as the context in an input~\cite{??,??}.}
Therefore, feeding the context as part of the LLM input to let LLM learn from the context is a popular choice.
\jc{we need some citations for these arguments}


\begin{figure*}[t]
\centering
     \includegraphics[width=.9\linewidth]{figs/motivate_baselines.pdf}
    \tightcaption{} 
    \label{fig:motivate_baselines}
\end{figure*}

\mypara{Context length is increasing}
\jc{use some citations and reasoning that memory is getting longer. in conversational apps, as user interact with LLMs over time, the history gets longer. 
similarly, in retrieval-based apps, people feed more documents (such as search results or a novel).
finally, LLMs are also designed to take longer and longer input. use Figure~\ref{fig:motivate_long_input}.}

\jc{need some empirical evidence here:
\begin{itemize}
\item longer context means more matches
\item models can accept longer input
\end{itemize}}

%\mypara{Context can be dynamic}
%\jc{we still need citations to explain why context is not static. it is customized for each user (for conversational apps). it is also dependent on the query (for retrieval-based apps)}

Since many commercial LLMs are proprietary, there is little public statistics on how exactly they are used. 
Nonetheless, our hypothesize that these trends have or will materialize in commercial LLMs too.

\mypara{Contexts need to be loaded dynamically}
The context of an LLM input often needs to be fetched from a different server. 
\jc{i can think of at least three reasons 
(1) retrieved documents are hosted by a different service/company; and 
(2) conversational app user goes idle for a long time and then resumes;
(3) user moves from one location to another, thus served by different LLM servers.
can we find some citations/evidence for all three?}

In this work, we assume that the context is stored in a different machine than the GPUs running the LLM.



\subsection{Metrics and objectives}

\mypara{Delay metric}
We focus on {\em time-to-first-token (TTFT)}, defined by the time between knowing the input (the prompt and context) and generating the first token. 
While LLM systems may also reduce the total generation delay (the sum of TTFT and the delay to autoregressively generate response tokens), we choose not to use this metric  because 
(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
(2) we want to focus the delay reduction on processing input faster, not by generating fewer tokens.

Since the context resides in a different machine than the GPUs running the LLM, the TTFT delay consists of 
(1) the {\em communication} delay to fetch the context to GPU memory and 
(2) the {\em computation} delay to process the context and prompt before generating the first token.


\mypara{Quality metric}
We then define {\em generation quality degradation} by how close the generated text under any speedup of input processing is to the text generated when letting the LLM process the context and the prompt from scratch, which is the unoptimized implementation. 
In other words, generation quality degradation measures the impact of speedup on generated text.
If the speedup of input processing does not change the generated output, the quality will be the highest, but sometimes the speedup is achieved by dropping information, yielding a different generation text.

Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
\S\ref{subsec:eval:setup} will describe these metrics in more detail.

\mypara{Objectives}
With these definitions, the objective of this paper can be formulated as follows.
{\em How to minimize the TTFT delay with minimum generation quality degradation?}
Essentially, all methods, including ours, strike some tradeoffs between TTFT delay and generation quality.
Thus, in practice, we will show our improvement by comparing the TTFT delay of two methods under the same generation quality degradation.


\subsection{Prior works and their limitations}



As explained in \S\ref{subsec:transformer}, processing a context encompasses the computation of attention modules, whose delay grows superlinearly (quadratic or at least loglinear) with the length of the context. 
Fortunately, the context of a query is often known in advance, so a common optimization to reduce the computing delay is by caching the intermediate outcomes of contexts, namely the , or KV cache.


%\mypara{KV cache}
As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features the key are often cached by LLM applications, referred to as KV cache,  to save computation delay on repeating text. 
\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}


With the KV features of a text, reconstruct the attention matrices of the text is usually an order of magnitude faster than calculating the attention matrices from scratch. 
With the attention matrices of the context, the LLM still needs to process the prompt part of the input, but since the prompt is much shorter than the context, this additional delay is relatively small. 
To put it more concrete, \jc{give an example here of how long it takes to process a context, how much faster with kv cache, and how much more time to start generating the first token}


%\mypara{Prohibitive size}
However, KV features can have a large size. 
For a given text with $\NumTokens$ tokens, the KV features, are two tensors, each of size $\NumTokens\cdot\NumChannels\cdot\NumLayers$, where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
\jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}


Though the large size of KV cache is not a serious issue when the KV cache resides in GPU memory, it will become a communication bottleneck if the KV cache needs to be dynamically loaded from a different machine to GPU memory.
\jc{for a given bandwidth, show the delay to download KV vs. processing the context from scratch, and explain when downloading KV actually doesnt payoff}

%\jc{explain (1) why KV can be computed for conversation history and for knowledge base. cite some papers.
%(2) given cached KV, what would happen before the first token is generated
%(3) if the context is the prefix, then why caching KV doesn't change the output.
%(4) if the context is is not the prefix, why caching KV still helps. again, cite some papers}

Over the last few months, there are some emerging research efforts to reduce the size of KV cache.
For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits and found that \fillme.
Scissorhand~\cite{??}, on the other hand, proposed to prune less important tokens from the long context. 
Both techniques try to drop some part of the KV tensor (bits or tokens), so the size can be reduced, but not by too much, otherwise, useful information can also be dropped, causing high loss in generation quality.
Some more recent proposals~\cite{incontext-autoencoder, gisting} try to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 


Unlike our goal of reducing the loading delay of long context, these existing methods strive to fit more long contexts in GPU memory.
This has two implications.
First, they shrink KV cache or context length but still must keep the shape of KV tensors in GPU memory.
Second, they replace the KV cache with some smaller variant and are agnostic to how fast the KV cache can be fetched. 
Thus, they cannot adapt the compression to available network bandwidth in order to meet a delay budget.

\begin{comment}
While focused directly on reducing TTFT with remotely fetched long context, several existing ideas can already affect the delay-quality tradeoff.
At a high level, there are three design choices. \jc{explain each choice. can use Figure~\ref{fig:motivate_baselines}}

%0. Load all context in words
%1. Context word selection
%2. Pre-compute and load key-value features
%3. Smaller model or quantized model
\begin{packeditemize}

\item {\em Choice 1: Reduce context length.}

\item {\em Choice 2: Load compressed key-value features.}

\item {\em Choice 3: Use smaller models.}

\end{packeditemize}

We assume that the context has $N$ tokens and the prompt has $k$ tokens ($N>>k$).
All designs strike some tradeoffs between quality and TTFT delay, which can be break down to communication delay to fetch the context and the computation delay to process context and the prompt.
The unoptimized design would load all $N$ context tokens as plain text, yielding a small communication delay but a computation delay of $O(N^2)$.

The three aforementioned design choices make different tradeoffs between quality and TTFT delay, which can be break down to communication delay to fetch the context and the computation delay to process context and the prompt.
Compared to the baseline of loading context as raw text, reducing context length from $N$ to $n$ reduces the computation delay from $O(N+k)$

\end{comment}

%\jc{use figure~\ref{fig:design_choices} to quantify these points}



==> backups/motivate_v4_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{} 
    \label{fig:motivate_query_examples}
\end{figure*}

\section{Background and Motivation}

\subsection{Transformer basics}
\label{subsec:transformer}

{\em Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks.
Most popular generative NLP services these days are based on transformer models, including GPT, LLaMA, \jc{more names}. 
For this reason, we focus on transformer-based LLMs in this work.

Here, we provide a general introduction of the transformer architecture. 
We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
Readers can refer to \fillme for a more involved introduction.

A transformer model takes as input a sequence of tokenized words\jc{is tokenization part of the transformer framework?}, and generates as output a response, which is another sequence of tokens. \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This generation process includes two high-level steps.
First, \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
Then, \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

The key of the transformer architecture is a neural network (NN) called attention module. 
Each layer of the attention module producing an attention matrix, which describes the connections between each pair of tokens. 
The attention matrix at one layer is obtained by applying a non-linear NN operation on the attention matrix of the last layer.
Intuitively, the attention matrices of deeper layers might embed more complex understanding of tokens under consideration. 

The attention module is a powerful tool to model a sequence of tokens at the expense of computational and storage overheads. 
Given an input of $\NumTokens$ tokens, the computation and space overhead of computing the attention matrices will grow quadratically, $O(\NumTokens^2)$.
Though the overheads could be reduced to $O(\NumTokens\textrm{log}\NumTokens)$ (\eg~\cite{??,??,??,??}), it usually also degrade the quality of generation. 
Note that once the attention matrices of the input are obtained, the time to generate each token is quite marginal and can be reduced to almost constant on GPUs. 

%The intermediate outcome of the first step is called key-value features, or KV features. 

\subsection{Long context in LLM applications}

While an input to the LLM usually contains only the immediate last prompt, which is a relatively short statement or question (Figure~\ref{fig:motivate_query_examples}(a)), in more applications today, the LLM input tends to precede\footnote{The context is put ahead of the immediate prompt in most cases~\cite{??,??,??}, so in this work we assume it is the prefix of the LLM input.} the immediate prompt with more {\em context}\footnote{The memory part of a prompt is referred to by different names depending on the applications. We use the term ``context'' in lack of an umbrella term in the literature.} text to enhance the generation quality.
Since these contexts are often automatically added, users do not notice them or manually type in longer prompt.

\myparaq{Why context}
The use of contexts can be found in various applications.
Here we highlight two general types of such applications. 
In \S\ref{sec:eval}, we will evaluate our performance in representative datasets of these applications.
\begin{packeditemize}

\item{\em Retrieval-based applications (Figure~\ref{fig:motivate_query_examples}(b)):} 

\jc{\begin{itemize}
\item start with a general background of knowledge base, query, and retrieval logic. 
\item give a few examples from those retrieval-based learning papers. reading a book or a database of specialized knowledge would be good examples
\end{itemize}}

\item {\em Conversational applications (Figure~\ref{fig:motivate_query_examples}(c)):}

\jc{\begin{itemize}
\item start with a general description of user-LLM interactions and why the previous interactions (conversation history) become useful context. 
\item give a few examples for long-context learning and few-shot learning. things to consider: (1) a series of prompts to create a character before interacting with it. (2) giving a bunch of long examples with correct answers to teach LLM some knowledge and then asking the real question, etc
\end{itemize}}

\end{packeditemize}

\jc{clarify the terminology of prompt, context, input, query, etc}



%\mypara{Why context is important}
Context is playing an increasingly important role in LLM applications. 
Since the pre-trained LLMs alone do not always contain enough information to answer complex questions or questions that require new knowledge that the model has not seen before.
Yet, retraining or even fine-tuning LLMs can be prohibitively expensive for most users. 
%The reason to have "memory" in LLM's input is the increasing realization that 
In the meantime, LLMs are quite powerful at learning useful information embedded in text, even if the text is over tens of thousands of tokens~\cite{??}.\footnote{LLM is a fast evolving literature, and latest LLMs can even take a whole book as the context in an input~\cite{??,??}.}
Therefore, feeding the context as part of the LLM input to let LLM learn from the context is a popular choice.
\jc{we need some citations for these arguments}


\begin{figure*}[t]
\centering
     \includegraphics[width=.9\linewidth]{figs/motivate_baselines.pdf}
    \tightcaption{} 
    \label{fig:motivate_baselines}
\end{figure*}

\mypara{Context length is increasing}
\jc{use some citations and reasoning that memory is getting longer. in conversational apps, as user interact with LLMs over time, the history gets longer. 
similarly, in retrieval-based apps, people feed more documents (such as search results or a novel).
finally, LLMs are also designed to take longer and longer input. use Figure~\ref{fig:motivate_long_input}.}

\jc{need some empirical evidence here:
\begin{itemize}
\item longer context means more matches
\item models can accept longer input
\end{itemize}}

%\mypara{Context can be dynamic}
%\jc{we still need citations to explain why context is not static. it is customized for each user (for conversational apps). it is also dependent on the query (for retrieval-based apps)}

Since many commercial LLMs are proprietary, there is little public statistics on how exactly they are used. 
Nonetheless, our hypothesize that these trends have or will materialize in commercial LLMs too.

\mypara{Contexts need to be loaded dynamically}
The context of an LLM input often needs to be fetched from a different server. 
\jc{i can think of at least three reasons 
(1) retrieved documents are hosted by a different service/company; and 
(2) conversational app user goes idle for a long time and then resumes;
(3) user moves from one location to another, thus served by different LLM servers.
can we find some citations/evidence for all three?}

In this work, we assume that the context is stored in a different machine than the GPUs running the LLM.



\subsection{Metrics and objectives}

\mypara{Delay metric}
We focus on {\em time-to-first-token (TTFT)}, defined by the time between knowing the input (the prompt and context) and generating the first token. 
While LLM systems may also reduce the total generation delay (the sum of TTFT and the delay to autoregressively generate response tokens), we choose not to use this metric  because 
(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
(2) we want to focus the delay reduction on processing input faster, not by generating fewer tokens.

Since the context resides in a different machine than the GPUs running the LLM, the TTFT delay consists of 
(1) the {\em communication} delay to fetch the context to GPU memory and 
(2) the {\em computation} delay to process the context and prompt before generating the first token.


\mypara{Quality metric}
We then define {\em generation quality degradation} by how close the generated text under any speedup of input processing is to the text generated when letting the LLM process the context and the prompt from scratch, which is the unoptimized implementation. 
In other words, generation quality degradation measures the impact of speedup on generated text.
If the speedup of input processing does not change the generated output, the quality will be the highest, but sometimes the speedup is achieved by dropping information, yielding a different generation text.

Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
\S\ref{subsec:eval:setup} will describe these metrics in more detail.

\mypara{Objectives}
With these definitions, the objective of this paper can be formulated as follows.
{\em How to minimize the TTFT delay with minimum generation quality degradation?}
Essentially, all methods, including ours, strike some tradeoffs between TTFT delay and generation quality.
Thus, in practice, we will show our improvement by comparing the TTFT delay of two methods under the same generation quality degradation.


\subsection{Prior works and their limitations}



As explained in \S\ref{subsec:transformer}, processing a context encompasses the computation of attention modules, whose delay grows superlinearly (quadratic or at least loglinear) with the length of the context. 
Fortunately, the context of a query is often known in advance, so a common optimization to reduce the computing delay is by caching the intermediate outcomes of contexts, namely the , or KV cache.


%\mypara{KV cache}
As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features the key are often cached by LLM applications, referred to as KV cache,  to save computation delay on repeating text. 
\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}


With the KV features of a text, reconstruct the attention matrices of the text is usually an order of magnitude faster than calculating the attention matrices from scratch. 
With the attention matrices of the context, the LLM still needs to process the prompt part of the input, but since the prompt is much shorter than the context, this additional delay is relatively small. 
To put it more concrete, \jc{give an example here of how long it takes to process a context, how much faster with kv cache, and how much more time to start generating the first token}


%\mypara{Prohibitive size}
However, KV features can have a large size. 
For a given text with $\NumTokens$ tokens, the KV features, are two tensors, each of size $\NumTokens\cdot\NumChannels\cdot\NumLayers$, where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
\jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}


Though the large size of KV cache is not a serious issue when the KV cache resides in GPU memory, it will become a communication bottleneck if the KV cache needs to be dynamically loaded from a different machine to GPU memory.
\jc{for a given bandwidth, show the delay to download KV vs. processing the context from scratch, and explain when downloading KV actually doesnt payoff}

%\jc{explain (1) why KV can be computed for conversation history and for knowledge base. cite some papers.
%(2) given cached KV, what would happen before the first token is generated
%(3) if the context is the prefix, then why caching KV doesn't change the output.
%(4) if the context is is not the prefix, why caching KV still helps. again, cite some papers}

Over the last few months, there are some emerging research efforts to reduce the size of KV cache.
For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits and found that \fillme.
Scissorhand~\cite{??}, on the other hand, proposed to prune less important tokens from the long context. 
Both techniques try to drop some part of the KV tensor (bits or tokens), so the size can be reduced, but not by too much, otherwise, useful information can also be dropped, causing high loss in generation quality.
Some more recent proposals~\cite{incontext-autoencoder, gisting} try to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 


Unlike our goal of reducing the loading delay of long context, these existing methods strive to fit more long contexts in GPU memory.
This has two implications.
First, they shrink KV cache or context length but still must keep the shape of KV tensors in GPU memory.
Second, they replace the KV cache with some smaller variant and are agnostic to how fast the KV cache can be fetched. 
Thus, they cannot adapt the compression to available network bandwidth in order to meet a delay budget.

\begin{comment}
While focused directly on reducing TTFT with remotely fetched long context, several existing ideas can already affect the delay-quality tradeoff.
At a high level, there are three design choices. \jc{explain each choice. can use Figure~\ref{fig:motivate_baselines}}

%0. Load all context in words
%1. Context word selection
%2. Pre-compute and load key-value features
%3. Smaller model or quantized model
\begin{packeditemize}

\item {\em Choice 1: Reduce context length.}

\item {\em Choice 2: Load compressed key-value features.}

\item {\em Choice 3: Use smaller models.}

\end{packeditemize}

We assume that the context has $N$ tokens and the prompt has $k$ tokens ($N>>k$).
All designs strike some tradeoffs between quality and TTFT delay, which can be break down to communication delay to fetch the context and the computation delay to process context and the prompt.
The unoptimized design would load all $N$ context tokens as plain text, yielding a small communication delay but a computation delay of $O(N^2)$.

The three aforementioned design choices make different tradeoffs between quality and TTFT delay, which can be break down to communication delay to fetch the context and the computation delay to process context and the prompt.
Compared to the baseline of loading context as raw text, reducing context length from $N$ to $n$ reduces the computation delay from $O(N+k)$

\end{comment}

%\jc{use figure~\ref{fig:design_choices} to quantify these points}



==> backups/motivate_v5.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

%\newpage


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{} 
    \label{fig:motivate_query_examples}
\end{figure*}

\section{Background and Motivation}

\subsection{Transformer basics}
\label{subsec:transformer}

{\bf Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks~\cite{??,??}.
Today, most popular generative NLP services are based on transformer models, including T5~\cite{??}, LLaMA~\cite{??}, PaLM~\cite{??}, OPT~\cite{??}, and BLOOM~\cite{??}. 
%For these reasons, we focus on transformer-based LLMs in this work.
Here, we provide a general introduction of transformer architecture. 
%We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
%Readers can refer to \fillme for a more involved introduction.

A transformer model takes as input a sequence of tokenized words,
% \jc{is tokenization part of the transformer framework?} \yh{It's something separate to the LLM itself, so ok to say like this}
and generates as output a response, which is another sequence of tokens (usually in the format of integers) \footnote{``Tokens'' in NLP stands for the input unit that is used for DNN inference, which may include punctuations or splitting words into characters. We will use ``tokens'' in the rest of the paper. }. 
% \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This generation process includes two high-level steps.
First, \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
Then, \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

The key of the transformer architecture is a neural network (NN) called attention module. 
Each layer of the attention module produces an attention matrix, which models the connections between each pair of tokens. 
The attention matrix at every layer is obtained by applying a non-linear NN operation on the attention matrix of its previous layer.
Intuitively, the attention matrices of deeper layers might embed more complex understanding of tokens under consideration. 


While attention module is crucial in the transformer architecture, it is also known to be compute-intensive. 
With an input of $\NumTokens$ tokens, the computation overhead of computing the attention matrices will grow quadratically, $O(\NumTokens^2)$.
Though this overhead might be reduced to $O(\NumTokens\textrm{log}\NumTokens)$ (\eg~\cite{??,??,??,??}), it is often at the expense of degraded quality of generation. 
That said, once the attention matrices of the input are obtained, the time to generate (decode) each token is quite marginal and can be reduced to almost constant on GPUs. 

%\begin{itemize}
%\item transformer is the de-factor llm arch, so we focus on it
%\item transformer basics
%    \begin{itemize}
%    \item input vs. output
%    \item processing phase (encoding?)
%    \item generation phase (decoding?)
%    \end{itemize}
%\end{itemize}


\subsection{Long contexts in LLM applications}
\label{subsec:apps}
\shan{This sub-section is tooo long. When we get time, we better
shrink it.}

Traditionally, the input of an LLM, referred to as {\em prompt}, is a relatively short query, as illustrated in Figure~\ref{fig:motivate_query_examples}(a).
Since the prompt contains limited information, the LLM generates the response mostly based on knowledge already embedded in the LLM itself. 

However, as LLMs are increasingly used in real-world applications, it is no longer sufficient to rely only on the knowledge embedded in the LLM.
Consequently, applications often append additional texts to supplement the prompt input to an LLM.
These additional texts are referred to as the {\bf context} part of an LLM input. 
More importantly, LLM applications use {\bf increasingly long} contexts, in order to generate high-quality, coherent responses.\footnote{Since these contexts are often automatically added, users do not notice or need to manually type them.}

To make our discussion more concrete, we highlight two types of applications, retrieval-based apps and chat apps, that often add long context to supplement LLM input.

{\em Retrieval-based apps (Figure~\ref{fig:motivate_query_examples}b)} 
use LLMs to answer queries that require domain-specific knowledge.
Examples of retrieval-based applications include question answering systems~\cite{rubin2023long, retro, fid}, code understanding systems~\cite{rubin2023long, lewis2020retrieval} or fact verification systems~\cite{fid, lewis2020retrieval}.
% \jc{give a few examples from those retrieval-based learning papers.}
To do so, they use a background database which contains a large amount of background documents.
On receiving a question, the app will use some embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid } or BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepends these documents to the prompt, and feeds them as input to the LLM.

For retrieval-based apps, the retrieved background documents are the context of an LLM input.
Intuitively, longer contexts will more likely include the information needed to generate the response. 
Specifically, many previous works~\cite{fid, izacard2020memory, atlas} have shown that the accuracy of the generated answers increases when the number of documents retrieved increases. 
For instance, FiD~\cite{fid} demonstrates that the accuracy score can increase from 40\% to 48\% if increasing number of input tokens from 1K to 10K.
Retro~\cite{retro} shows that the perplexity (lower the better) drops a lot when the number of retrieved tokens increases from 6K to 24K. 
% maybe cite self-retrieval paper here~\cite{self}
Intuitively, longer contexts can provide more information for LLM to  answer users' questions.
For example, the user may ask ``Which of the following countries generated the most total energy from solar sources in 2019?''~\cite{shi2023replug}. 
Without retrieving all the background documents for all countries the user is asking for, it is not possible for the LLM to answer it correctly.

% For instance, FiD~\cite{fid} shows that the accuracy of generated answers for three question answering datasets can grow by 4 to 9 percentage-points (\ie from 43\% to 47\%, 58\% to 65\% or 40\% to 49\%) if the number of retrieved documents increases from 10 to 100. \yh{show evidence that MORE TOKENS lead to more matches.}

%\jc{show some numerical evidence here. maybe a few figure of \% of matches vs. context length. we need to discuss this.} \yh{i added some citations and mentioned the numbers.}

%\jc{\begin{itemize}
%\item start with a general background of knowledge base, query, and retrieval logic. 
%\item give a few examples from those retrieval-based learning papers. reading a book or a database of specialized knowledge would be good examples
%\end{itemize}}

{\em Chat apps (Figure~\ref{fig:motivate_query_examples}c)} 
become popular with the rise of OpenAI's ChatGPT and have many similar offerings from other corporations~\cite{??}, \eg Google BARD, Facebook Blender, Microsoft DialoGPT.
% \jc{some names of chat apps}
%The conversational history between a user and the LLM can be seen as the ``memory''.
In order to produce high-quality and coherent responses, a user's conversation history with the LLM, or at least part of it, is often included in the input to the LLM as the context of each user query. 
For instance, some open-source applications use ChatGPT API to create Non-player characters in video games~\cite{KelSolaar2023} and their users will supply a series of prompts to create a character to the LLM, and then interact with the character by asking questions.
%Other applications~\cite{??} use ChatGPT to summarize technical papers or long documents. \jc{why is this using conversation history?}
Furthermore, in few-shot learning scenarios, users may provide several long examples and their the desired responses to the LLM, before they actually ask the real questions\jc{need citations here}. 

% \jc{ give a few examples. things to consider: 
% (1) a series of prompts to create a character before asking new questions. 
% (2) few-shot learning: giving a bunch of long examples with correct answers to teach LLM some knowledge and then asking the real question, etc}

As users have more interactions with these chat applications, they accumulate an increasing amount of conversational histories, \ie contexts, that only grow over time.
For example, usage report~\cite{usagereport} for ChatGPT shows that more than 35\% of the users use ChatGPT for more than 5 rounds of conversations, making the context potentially very long.
\jc{Yuhan, 5 rounds dont sound very long?}
%\jc{some evidence that shows the growing length of conversational histories. maybe chatgpt user behavior report?} 

%\jc{\begin{itemize}
%\item start with a general description of user-LLM interactions and why the previous interactions (conversation history) become useful context. 
%\item give a few examples for long-context learning and few-shot learning. things to consider: (1) a series of prompts to create a character before interacting with it. (2) giving a bunch of long examples with correct answers to teach LLM some knowledge and then asking the real question, etc
%\end{itemize}}

%\end{packeditemize}

%why context is useful
Long contexts play an increasingly important role in LLM applications for three reasons.
% - llm's superb ability to learn from text
First, modern LLMs have a superb ability to reason about new texts and potentially learn knowledge from them. 
There has been a fast-growing literature on in-context learning, which improves how context can be optimized (sometimes called prompting) in order to induce better response from LLMs.
Second, to take in long contexts, the latest LLMs are trained with the capability to take longer input sequences. 
For instance, Vicuna models~\cite{zheng2023judging}, GPT-4-32K~\cite{openai2023gpt4} and MPT models~\cite{MosaicML2023Introducing} can take up to 32K tokens as input. 
Latest models like LongNet~\cite{ding2023longnet} can even take up to 1 billion tokens as input.
% \jc{some numbers here}
% - fine-tuning is often not feasible
Finally, while LLMs are sometimes fine-tuned for specific domains, it is not always feasible.
For instance, it is unrealistic to fine-tune an LLM for each user in chat apps.
In retrieval-based apps, the background database may be managed separately from the LLM provider.
Due to their huge number of parameters, fine-tuning LLMs is also slow and can be very tricky to do it right (\eg catastrophic forgetting, loss of reasoning ability, etc\jc{find some citations}).


% \jc{mention the bloomberg example somewhere}

\jc{To Ganesh's concern: there is still little justification in the text why the "retrieved part" from the background documents or the conversation history is still quite long (Ks or 10s K). 
i remembered you had a figure showing \% of matches vs. context length, and there are several other pointers like that. again, the point is not to show longer contexts lead to higher accuracy, but contexts have to be as long as Ks or 10sK or even 100s of Ks.}



%\begin{itemize}
%    \item traditionally, prompt doesn't have context
%    \item apps with contexts
%    \begin{itemize}
%        \item retrieval apps. examples
%        \item chat apps. examples
%    \end{itemize}
%    \item why is context useful
%    \begin{itemize}
%        \item llm doesnt have all knowledge, and can't keep states
%        \item new knowledge embed in context
%    \end{itemize}
%    \item why not fine-tuning? => fine-tuning cost is high. can't fine tune (chat history and background database is managed separately
%    \item why is context getting longer?
%    \begin{itemize}
%        \item more knowledge can be embedded
%        \item evidence: \# of matches vs. context length
%        \item evidence: chat apps have longer conversational histories
%        \item research: recent llms are capable of processing extremely long context
%        \item research: long-context learning, few-shot, retrieval-based, => llms can process extremely long context
%    \end{itemize}
%\end{itemize}



\subsection{\hspace{-0.2cm}Saving computation by caching KV features}

%There has been a growing literature to tackle the {\em computational} overhead of long contexts.
%\shan{I think the remainder of this paragraph should be moved to 
%Section\ref{subsec:transformer}. It is really part of transformer
%background.}
%In transformer models, the attention module is a powerful tool to model a sequence of tokens, but it also incur a prohibitive computational overheads, particularly on long inputs, as illustrated in Figure~\ref{fig:motivate_baselines}(a). 

Recall that the computation overhead of attention module on the context grows superlinearly (quadratically) with the context length (\S\ref{subsec:transformer}), so longer contexts dramatically increases the computation delay. 
A growing literature has been tackling the {\em computational} overhead of long contexts.

A common optimization to reduce the computing delay, illustrated in Figure~\ref{fig:motivate_baselines}(a), is to cache the intermediate outcomes of contexts, namely the key and value (KV) features,.
%As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features can be cached by LLM applications.
Thus, when the context is used again as part of another LLM input, one can save the computation delay of processing the context by using its KV features to reconstruct the self-attention matrices of the context (illustrated in Figure~\ref{fig:motivate_baselines}(b)). 
The cached KV features of a context are called the {\bf KV cache}.

Specifically, KV cache can be used in both chat apps and retrieval-based apps. 
In chat apps, the context is the past prompts and responses, and their KV features can be cached when they are first processed (for prompts) and generated (for responses)~\cite{??,??}.
In retrieval-based apps, applications often preprocess each background document by the LLM to compute the self-attention matrices and save the KV features~\cite{??,??}.
%\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}
Of course, not all applications can be optimized by KV cache.
Search-based apps (Google or Bing), for instance, use real-time searched web pages as the context, and the KV features of these dynamic contexts have to be obtained on the fly.

\yh{Should we add the discussion of discussion of KV feature shrinking related work here?}

\begin{comment}
    


Some emerging research shrinking the tensor size of KV cache, in order to further speed up the computation or fit more contexts in GPU memory.
For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits, and Scissorhand~\cite{??} proposed to prune less important tokens from the long context. 
Some more recent proposals~\cite{incontext-autoencoder, gisting} modify the pre-trained LLMs or train a new autoencoder to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
%However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 

\end{comment}

Essentially, LLM systems for long contexts assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delay and keeping the KV cache of more contexts in memory.
%Therefore, their goal has been to maintain the tensor shape of KV features in GPU memory and fit as many contexts' KV cache as possible.

%drop some part of the KV tensor (bits or tokens), so the size can be reduced but they maintain the tensor shape of KV features.
%, but not by too much, otherwise, useful information can also be dropped, causing high loss in generation quality.



%\begin{itemize}
%    \item processing text is too slow => KV cache is a common fix
%    \item what's KV cache => why KV cache can save delay
%    \item how KV cache is used in chat apps and retrieval apps (not apps can cache kv)
%    \item emerging research on reducing kv memory footprint
%    \item assumption: kv is already in GPU
%\end{itemize}


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{Contrasting \name with two prior approaches in their network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}


\section{Hidden network delay of loading contexts}


% \shan{I suggest making this sub-section a separate section and
% name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% section is REALLY tooo long. 2. this sub-section is actually not
% a background. instead, it is an important observation made by us
% that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% make it a separate section. If it is in background, it sounds
% more like previous work's observation.}
In practice, however, the KV cache is {\em not} always in the memory of the GPUs that run the LLM inference. 
Instead, the context of an LLM input often needs to be fetched {\bf remotely} from a different server. 


In retrieval-based apps, the background documents are often hosted on a different server than the one serving LLMs to users~\cite{li2022decoupled, retro}. 
This is because the the background documents can be huge in size (even if raw texts for the documents are stored), and the storage server on which LLM inference runs may not have enough space to store them.
For example, in a recent work~\cite{li2022decoupled}, there can be up to 364 Million documents~\cite{C4} in the background database, and storing these texts can take a space up to around 750 GB. 
Another recent work~\cite{retro} of up to 2 trillion tokens, and those tokens can take up to 1 TB of storage.
The background database may even be managed by a different service than the LLMs.
% \jc{please add some evidence and citations here}
% \yh{todo: add more citations for retrieval-based apps}

Similarly, in chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions.
\jc{please add some evidence and citations here}
Moreover, over time, a user may issue her prompts to the LLM from different locations.
These prompts can be processed by different machines, and the contexts must be remotely fetched.



%In this work, we assume that the context is stored in a different machine than the GPUs running the LLM
\begin{figure}
\centering
     \includegraphics[width=.7\linewidth]{figs/size_models.pdf}
    \tightcaption{How size of KV features grow with input length for different models. The size of KV features is reported without compression. \yh{Should we add the size after naive AC? }} 
    \label{fig:size_models}
\end{figure}

As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the overall delay.
However, the size of a context's KV cache can be much bigger than the context itself, making network bandwidth a potential bottleneck.
%Though the size of KV cache is not a serious issue when the KV cache resides in GPU memory, it will become a communication bottleneck if the KV cache needs to be dynamically loaded from a different machine to GPU memory.
%This is because KV features can have a large size. 
For a given text with $\NumTokens$ tokens, the KV features, are two tensors, each of size $\NumTokens\cdot\NumChannels\cdot\NumLayers$, where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
For example, for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be as large as 1.3 GB.
On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
Similarly for other LLMs, the size of KV features can be large, and grows linearly with the input token lengths, as shown in Figure~\ref{fig:size_models}.
% \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}

Given a network bandwidth, 1Gbps for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
However, processing the context from scratch only takes around 5 seconds on a A40 GPU.
The large size of KV features makes fetching them remotely doesn't payoff the benefit of eliminating self-attention computation. 

% In order to benefit the most from loading the KV features, we target at reducing the bandwidth needed to transmit the KV features.\shan{What ``we target'' should be the content of
% Section \ref{subsec:designgoal}. Here, we should talk about the
% takeway message of all this analysis.
% }
% % \jc{for a given bandwidth, show the delay to download KV vs. processing the context from scratch, and explain when downloading KV actually doesnt payoff}

% Unlike our goal of reducing the loading delay of long context, these existing methods strive to fit more long contexts in GPU memory.
% This has two implications.
% First, they shrink KV cache or context length but still must keep the shape of KV tensors in GPU memory.
% Second, they replace the KV cache with some smaller variant and are agnostic to how fast the KV cache can be fetched. 
% Thus, they cannot adapt the compression to available network bandwidth in order to meet a delay budget.
% \shan{This paragraph doesn't fit here. It seems better be 
% combined with the first paragraph in this sub-section.}





%\begin{itemize}
%    \item why long context cant always be kept on gpu memory
%    \begin{itemize}
%        \item chat app: user move in time and space
%        \item retrieval: database in a separate place
%    \end{itemize}
%    \item delay must include the loading delay
%    \item why existing work for kv not enough? 
%    \begin{itemize}
%        \item must be in tensor shape
%        \item not considering kv loading delay => sometimes loading text is better
%        \item can't control the loading delay
%    \end{itemize}
%\end{itemize}

\jc{need a diagram to show where our solution is in the stack}






==> backups/motivate_v5_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

%\newpage


\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{} 
    \label{fig:motivate_query_examples}
\end{figure*}

\section{Background and Motivation}

\subsection{Transformer basics}
\label{subsec:transformer}

{\bf Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks~\cite{??,??}.
Today, most popular generative NLP services are based on transformer models, including T5~\cite{??}, LLaMA~\cite{??}, PaLM~\cite{??}, OPT~\cite{??}, and BLOOM~\cite{??}. 
%For these reasons, we focus on transformer-based LLMs in this work.
Here, we provide a general introduction of transformer architecture. 
%We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
%Readers can refer to \fillme for a more involved introduction.

A transformer model takes as input a sequence of tokenized words,
% \jc{is tokenization part of the transformer framework?} \yh{It's something separate to the LLM itself, so ok to say like this}
and generates as output a response, which is another sequence of tokens (usually in the format of integers) \footnote{``Tokens'' in NLP stands for the input unit that is used for DNN inference, which may include punctuations or splitting words into characters. We will use ``tokens'' in the rest of the paper. }. 
% \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This generation process includes two high-level steps.
First, \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
Then, \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

The key of the transformer architecture is a neural network (NN) called attention module. 
Each layer of the attention module produces an attention matrix, which models the connections between each pair of tokens. 
The attention matrix at every layer is obtained by applying a non-linear NN operation on the attention matrix of its previous layer.
Intuitively, the attention matrices of deeper layers might embed more complex understanding of tokens under consideration. 


While attention module is crucial in the transformer architecture, it is also known to be compute-intensive. 
With an input of $\NumTokens$ tokens, the computation overhead of computing the attention matrices will grow quadratically, $O(\NumTokens^2)$.
Though this overhead might be reduced to $O(\NumTokens\textrm{log}\NumTokens)$ (\eg~\cite{??,??,??,??}), it is often at the expense of degraded quality of generation. 
That said, once the attention matrices of the input are obtained, the time to generate (decode) each token is quite marginal and can be reduced to almost constant on GPUs. 

%\begin{itemize}
%\item transformer is the de-factor llm arch, so we focus on it
%\item transformer basics
%    \begin{itemize}
%    \item input vs. output
%    \item processing phase (encoding?)
%    \item generation phase (decoding?)
%    \end{itemize}
%\end{itemize}


\subsection{Long contexts in LLM applications}
\label{subsec:apps}
\shan{This sub-section is tooo long. When we get time, we better
shrink it.}

Traditionally, the input of an LLM, referred to as {\em prompt}, is a relatively short query, as illustrated in Figure~\ref{fig:motivate_query_examples}(a).
Since the prompt contains limited information, the LLM generates the response mostly based on knowledge already embedded in the LLM itself. 

However, as LLMs are increasingly used in real-world applications, it is no longer sufficient to rely only on the knowledge embedded in the LLM.
Consequently, applications often append additional texts to supplement the prompt input to an LLM.
These additional texts are referred to as the {\bf context} part of an LLM input. 
More importantly, LLM applications use {\bf increasingly long} contexts, in order to generate high-quality, coherent responses.\footnote{Since these contexts are often automatically added, users do not notice or need to manually type them.}

To make our discussion more concrete, we highlight two types of applications, retrieval-based apps and chat apps, that often add long context to supplement LLM input.

{\em Retrieval-based apps (Figure~\ref{fig:motivate_query_examples}b)} 
use LLMs to answer queries that require domain-specific knowledge.
Examples of retrieval-based applications include question answering systems~\cite{rubin2023long, retro, fid}, code understanding systems~\cite{rubin2023long, lewis2020retrieval} or fact verification systems~\cite{fid, lewis2020retrieval}.
% \jc{give a few examples from those retrieval-based learning papers.}
To do so, they use a background database which contains a large amount of background documents.
On receiving a question, the app will use some embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid } or BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepends these documents to the prompt, and feeds them as input to the LLM.

For retrieval-based apps, the retrieved background documents are the context of an LLM input.
Intuitively, longer contexts will more likely include the information needed to generate the response. 
Specifically, many previous works~\cite{fid, izacard2020memory, atlas} have shown that the accuracy of the generated answers increases when the number of documents retrieved increases. 
For instance, FiD~\cite{fid} demonstrates that the accuracy score can increase from 40\% to 48\% if increasing number of input tokens from 1K to 10K.
Retro~\cite{retro} shows that the perplexity (lower the better) drops a lot when the number of retrieved tokens increases from 6K to 24K. 
% maybe cite self-retrieval paper here~\cite{self}
Intuitively, longer contexts can provide more information for LLM to  answer users' questions.
For example, the user may ask ``Which of the following countries generated the most total energy from solar sources in 2019?''~\cite{shi2023replug}. 
Without retrieving all the background documents for all countries the user is asking for, it is not possible for the LLM to answer it correctly.

% For instance, FiD~\cite{fid} shows that the accuracy of generated answers for three question answering datasets can grow by 4 to 9 percentage-points (\ie from 43\% to 47\%, 58\% to 65\% or 40\% to 49\%) if the number of retrieved documents increases from 10 to 100. \yh{show evidence that MORE TOKENS lead to more matches.}

%\jc{show some numerical evidence here. maybe a few figure of \% of matches vs. context length. we need to discuss this.} \yh{i added some citations and mentioned the numbers.}

%\jc{\begin{itemize}
%\item start with a general background of knowledge base, query, and retrieval logic. 
%\item give a few examples from those retrieval-based learning papers. reading a book or a database of specialized knowledge would be good examples
%\end{itemize}}

{\em Chat apps (Figure~\ref{fig:motivate_query_examples}c)} 
become popular with the rise of OpenAI's ChatGPT and have many similar offerings from other corporations~\cite{??}, \eg Google BARD, Facebook Blender, Microsoft DialoGPT.
% \jc{some names of chat apps}
%The conversational history between a user and the LLM can be seen as the ``memory''.
In order to produce high-quality and coherent responses, a user's conversation history with the LLM, or at least part of it, is often included in the input to the LLM as the context of each user query. 
For instance, some open-source applications use ChatGPT API to create Non-player characters in video games~\cite{KelSolaar2023} and their users will supply a series of prompts to create a character to the LLM, and then interact with the character by asking questions.
%Other applications~\cite{??} use ChatGPT to summarize technical papers or long documents. \jc{why is this using conversation history?}
Furthermore, in few-shot learning scenarios, users may provide several long examples and their the desired responses to the LLM, before they actually ask the real questions\jc{need citations here}. 

% \jc{ give a few examples. things to consider: 
% (1) a series of prompts to create a character before asking new questions. 
% (2) few-shot learning: giving a bunch of long examples with correct answers to teach LLM some knowledge and then asking the real question, etc}

As users have more interactions with these chat applications, they accumulate an increasing amount of conversational histories, \ie contexts, that only grow over time.
For example, usage report~\cite{usagereport} for ChatGPT shows that more than 35\% of the users use ChatGPT for more than 5 rounds of conversations, making the context potentially very long.
\jc{Yuhan, 5 rounds dont sound very long?}
%\jc{some evidence that shows the growing length of conversational histories. maybe chatgpt user behavior report?} 

%\jc{\begin{itemize}
%\item start with a general description of user-LLM interactions and why the previous interactions (conversation history) become useful context. 
%\item give a few examples for long-context learning and few-shot learning. things to consider: (1) a series of prompts to create a character before interacting with it. (2) giving a bunch of long examples with correct answers to teach LLM some knowledge and then asking the real question, etc
%\end{itemize}}

%\end{packeditemize}

%why context is useful
Long contexts play an increasingly important role in LLM applications for three reasons.
% - llm's superb ability to learn from text
First, modern LLMs have a superb ability to reason about new texts and potentially learn knowledge from them. 
There has been a fast-growing literature on in-context learning, which improves how context can be optimized (sometimes called prompting) in order to induce better response from LLMs.
Second, to take in long contexts, the latest LLMs are trained with the capability to take longer input sequences. 
For instance, Vicuna models~\cite{zheng2023judging}, GPT-4-32K~\cite{openai2023gpt4} and MPT models~\cite{MosaicML2023Introducing} can take up to 32K tokens as input. 
Latest models like LongNet~\cite{ding2023longnet} can even take up to 1 billion tokens as input.
% \jc{some numbers here}
% - fine-tuning is often not feasible
Finally, while LLMs are sometimes fine-tuned for specific domains, it is not always feasible.
For instance, it is unrealistic to fine-tune an LLM for each user in chat apps.
In retrieval-based apps, the background database may be managed separately from the LLM provider.
Due to their huge number of parameters, fine-tuning LLMs is also slow and can be very tricky to do it right (\eg catastrophic forgetting, loss of reasoning ability, etc\jc{find some citations}).


% \jc{mention the bloomberg example somewhere}

\jc{To Ganesh's concern: there is still little justification in the text why the "retrieved part" from the background documents or the conversation history is still quite long (Ks or 10s K). 
i remembered you had a figure showing \% of matches vs. context length, and there are several other pointers like that. again, the point is not to show longer contexts lead to higher accuracy, but contexts have to be as long as Ks or 10sK or even 100s of Ks.}



%\begin{itemize}
%    \item traditionally, prompt doesn't have context
%    \item apps with contexts
%    \begin{itemize}
%        \item retrieval apps. examples
%        \item chat apps. examples
%    \end{itemize}
%    \item why is context useful
%    \begin{itemize}
%        \item llm doesnt have all knowledge, and can't keep states
%        \item new knowledge embed in context
%    \end{itemize}
%    \item why not fine-tuning? => fine-tuning cost is high. can't fine tune (chat history and background database is managed separately
%    \item why is context getting longer?
%    \begin{itemize}
%        \item more knowledge can be embedded
%        \item evidence: \# of matches vs. context length
%        \item evidence: chat apps have longer conversational histories
%        \item research: recent llms are capable of processing extremely long context
%        \item research: long-context learning, few-shot, retrieval-based, => llms can process extremely long context
%    \end{itemize}
%\end{itemize}



\subsection{\hspace{-0.2cm}Saving computation by caching KV features}

%There has been a growing literature to tackle the {\em computational} overhead of long contexts.
%\shan{I think the remainder of this paragraph should be moved to 
%Section\ref{subsec:transformer}. It is really part of transformer
%background.}
%In transformer models, the attention module is a powerful tool to model a sequence of tokens, but it also incur a prohibitive computational overheads, particularly on long inputs, as illustrated in Figure~\ref{fig:motivate_baselines}(a). 

Recall that the computation overhead of attention module on the context grows superlinearly (quadratically) with the context length (\S\ref{subsec:transformer}), so longer contexts dramatically increases the computation delay. 
A growing literature has been tackling the {\em computational} overhead of long contexts.

A common optimization to reduce the computing delay, illustrated in Figure~\ref{fig:motivate_baselines}(a), is to cache the intermediate outcomes of contexts, namely the key and value (KV) features,.
%As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features can be cached by LLM applications.
Thus, when the context is used again as part of another LLM input, one can save the computation delay of processing the context by using its KV features to reconstruct the self-attention matrices of the context (illustrated in Figure~\ref{fig:motivate_baselines}(b)). 
The cached KV features of a context are called the {\bf KV cache}.

Specifically, KV cache can be used in both chat apps and retrieval-based apps. 
In chat apps, the context is the past prompts and responses, and their KV features can be cached when they are first processed (for prompts) and generated (for responses)~\cite{??,??}.
In retrieval-based apps, applications often preprocess each background document by the LLM to compute the self-attention matrices and save the KV features~\cite{??,??}.
%\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}
Of course, not all applications can be optimized by KV cache.
Search-based apps (Google or Bing), for instance, use real-time searched web pages as the context, and the KV features of these dynamic contexts have to be obtained on the fly.

\yh{Should we add the discussion of discussion of KV feature shrinking related work here?}

\begin{comment}
    


Some emerging research shrinking the tensor size of KV cache, in order to further speed up the computation or fit more contexts in GPU memory.
For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits, and Scissorhand~\cite{??} proposed to prune less important tokens from the long context. 
Some more recent proposals~\cite{incontext-autoencoder, gisting} modify the pre-trained LLMs or train a new autoencoder to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
%However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 

\end{comment}

Essentially, LLM systems for long contexts assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delay and keeping the KV cache of more contexts in memory.
%Therefore, their goal has been to maintain the tensor shape of KV features in GPU memory and fit as many contexts' KV cache as possible.

%drop some part of the KV tensor (bits or tokens), so the size can be reduced but they maintain the tensor shape of KV features.
%, but not by too much, otherwise, useful information can also be dropped, causing high loss in generation quality.



%\begin{itemize}
%    \item processing text is too slow => KV cache is a common fix
%    \item what's KV cache => why KV cache can save delay
%    \item how KV cache is used in chat apps and retrieval apps (not apps can cache kv)
%    \item emerging research on reducing kv memory footprint
%    \item assumption: kv is already in GPU
%\end{itemize}


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{Contrasting \name with two prior approaches in their network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}


\section{Hidden network delay of loading contexts}


% \shan{I suggest making this sub-section a separate section and
% name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% section is REALLY tooo long. 2. this sub-section is actually not
% a background. instead, it is an important observation made by us
% that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% make it a separate section. If it is in background, it sounds
% more like previous work's observation.}
In practice, however, the KV cache is {\em not} always in the memory of the GPUs that run the LLM inference. 
Instead, the context of an LLM input often needs to be fetched {\bf remotely} from a different server. 


In retrieval-based apps, the background documents are often hosted on a different server than the one serving LLMs to users~\cite{li2022decoupled, retro}. 
This is because the the background documents can be huge in size (even if raw texts for the documents are stored), and the storage server on which LLM inference runs may not have enough space to store them.
For example, in a recent work~\cite{li2022decoupled}, there can be up to 364 Million documents~\cite{C4} in the background database, and storing these texts can take a space up to around 750 GB. 
Another recent work~\cite{retro} of up to 2 trillion tokens, and those tokens can take up to 1 TB of storage.
The background database may even be managed by a different service than the LLMs.
% \jc{please add some evidence and citations here}
% \yh{todo: add more citations for retrieval-based apps}

Similarly, in chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions.
\jc{please add some evidence and citations here}
Moreover, over time, a user may issue her prompts to the LLM from different locations.
These prompts can be processed by different machines, and the contexts must be remotely fetched.



%In this work, we assume that the context is stored in a different machine than the GPUs running the LLM
\begin{figure}
\centering
     \includegraphics[width=.7\linewidth]{figs/size_models.pdf}
    \tightcaption{How size of KV features grow with input length for different models. The size of KV features is reported without compression. \yh{Should we add the size after naive AC? }} 
    \label{fig:size_models}
\end{figure}

As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the overall delay.
However, the size of a context's KV cache can be much bigger than the context itself, making network bandwidth a potential bottleneck.
%Though the size of KV cache is not a serious issue when the KV cache resides in GPU memory, it will become a communication bottleneck if the KV cache needs to be dynamically loaded from a different machine to GPU memory.
%This is because KV features can have a large size. 
For a given text with $\NumTokens$ tokens, the KV features, are two tensors, each of size $\NumTokens\cdot\NumChannels\cdot\NumLayers$, where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
For example, for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be as large as 1.3 GB.
On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
Similarly for other LLMs, the size of KV features can be large, and grows linearly with the input token lengths, as shown in Figure~\ref{fig:size_models}.
% \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}

Given a network bandwidth, 1Gbps for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
However, processing the context from scratch only takes around 5 seconds on a A40 GPU.
The large size of KV features makes fetching them remotely doesn't payoff the benefit of eliminating self-attention computation. 

% In order to benefit the most from loading the KV features, we target at reducing the bandwidth needed to transmit the KV features.\shan{What ``we target'' should be the content of
% Section \ref{subsec:designgoal}. Here, we should talk about the
% takeway message of all this analysis.
% }
% % \jc{for a given bandwidth, show the delay to download KV vs. processing the context from scratch, and explain when downloading KV actually doesnt payoff}

% Unlike our goal of reducing the loading delay of long context, these existing methods strive to fit more long contexts in GPU memory.
% This has two implications.
% First, they shrink KV cache or context length but still must keep the shape of KV tensors in GPU memory.
% Second, they replace the KV cache with some smaller variant and are agnostic to how fast the KV cache can be fetched. 
% Thus, they cannot adapt the compression to available network bandwidth in order to meet a delay budget.
% \shan{This paragraph doesn't fit here. It seems better be 
% combined with the first paragraph in this sub-section.}





%\begin{itemize}
%    \item why long context cant always be kept on gpu memory
%    \begin{itemize}
%        \item chat app: user move in time and space
%        \item retrieval: database in a separate place
%    \end{itemize}
%    \item delay must include the loading delay
%    \item why existing work for kv not enough? 
%    \begin{itemize}
%        \item must be in tensor shape
%        \item not considering kv loading delay => sometimes loading text is better
%        \item can't control the loading delay
%    \end{itemize}
%\end{itemize}

\jc{need a diagram to show where our solution is in the stack}






==> backups/motivate_v6.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\tightsection{Background and Motivation}

\vspace{0.2cm}

\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
    \label{fig:motivate_query_examples}
\end{figure*}

\tightsubsection{Transformer basics}
\label{subsec:transformer}

{\bf Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks~\cite{vaswani2023attention, openai2023gpt4, palm, brown2020language, kasneci2023chatgpt, retro, zhai2022scaling}.
Today, most generative NLP services are based on transformer models, including T5~\cite{raffel2023exploring}, Llama~\cite{touvron2023llama}, PaLM~\cite{palm}, OPT~\cite{zhang2022opt}, and BLOOM. 
%For these reasons, we focus on transformer-based LLMs in this work.
%Here, we provide a general introduction to transformer architecture. 
%We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
%Readers can refer to \fillme for a more involved introduction.

A transformer model takes as input a sequence of tokenized words and generates an output response, which is another sequence of tokens (usually in the format of integers) \footnote{``Tokens'' in NLP stands for the input unit that is used for DNN inference, which includes punctuations or splitting words into characters. Tokenizing input is typically fast. We will use ``tokens'' in the rest of the paper. }. 
% \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This generation process includes two high-level steps.
First, the attention module processes the input tokens to obtain encoded features.
% \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
Then, the encoded features of the input are utilized to generate new tokens in an autoregressive manner. 
Specifically, the input tokens and previously generated tokens are fed into the transformer model to generate the next token.  
% \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

The key of the transformer architecture is 
%a neural network (NN) called 
the attention module. 
Each layer of the attention module produces an attention matrix, which models the connections between each pair of tokens. 
The attention matrix at every layer is obtained by applying a non-linear neural network operation on the attention matrix of its previous layer.
Intuitively, the attention matrices of deeper layers might embed a more complex understanding of the tokens under consideration. 


While the attention module is crucial, it is known to be compute-intensive. 
Given an input of $\NumTokens$ tokens, the computation overhead of computing the attention matrices grows quadratically, $O(\NumTokens^2)$.
Though the complexity could be reduced to $O(\NumTokens\textrm{log}\NumTokens)$ (\eg~\cite{luo2021stable, kitaev2020reformer}), such reduction often degrades the
generation quality. 
Once the attention matrices are obtained, the time to generate (decode) each token is quite marginal and can be reduced to almost constant on GPUs.


\tightsubsection{Long contexts in LLM applications}
\label{subsec:apps}

Traditionally, the input of an LLM is a relatively short {\em prompt}, as illustrated in Figure~\ref{fig:motivate_query_examples}(a).
Since the prompt contains limited information, the LLM generates the response based solely on the knowledge already embedded in the LLM itself. 

However, as LLMs are used in more real-world applications, it is no longer sufficient to rely on the knowledge embedded in the LLM.
Instead, LLM applications often append additional texts, referred to as the 
{\bf context}, to supplement the prompt input to an LLM\footnote{Since these contexts are often automatically added, users do not notice or need to manually type them.}.
To make our discussion more concrete, we highlight two types of applications, retrieval-based apps and chat apps.%, which often add long context to supplement their LLM input.


{\em Retrieval-based apps (Figure~\ref{fig:motivate_query_examples}b)} 
use LLMs to answer queries that require domain-specific knowledge.
Examples include question-answering systems~\cite{rubin2023long, retro, fid}, code understanding systems~\cite{rubin2023long, lewis2020retrieval} or fact verification systems~\cite{fid, lewis2020retrieval}.
% \jc{give a few examples from those retrieval-based learning papers.}
They use a background database that contains a large number of background documents.
On retrieving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM. 
\edit{Note that the search procedure is done by a \textit{seperate} DNN or a vector similarity search algorithm, which is not part of the LLM.}

% \jc{yuhan, i temporarily changed all the appearances of the term "retriever" to "application", simply because it's not defined yet and i don't know what it is. if you think it's not appropriate, please define it and change the term back to retriever}
% \edit{

% % For example, given the question ``When did the first mammal appear on Earth''~\cite{metablog2023}, the application selects documents on ``Mammals'', ``History of Earth'', or ``Evolution of Mammals''. 
% % % Then, the apps concatenate the tokens from the retrieved documents and feed the concatenated contexts into the LLM. 

% \jc{this paragraph is simultaneously doing too much and too little :) 
% on one hand, it talks too much detail about the search algorithms (which can be moved to related work).
% on the other hand, it doesn't make clear that the search delay is separate from what we optimize --- the loading and processing delays of long context.}
% }

% On receiving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM.


{\em Chat apps (Figure~\ref{fig:motivate_query_examples}c)} 
become popular with the rise of OpenAI's ChatGPT and have many similar products~\cite{google_bard, microsoft_bing}. %, \eg Google BARD, Facebook Blender, Microsoft DialoGPT.
% \jc{some names of chat apps}
%The conversational history between a user and the LLM can be seen as the ``memory''.
To produce high-quality and coherent responses, a user's conversation history with the LLM, or at least part of it, is often included in the input to the LLM as the context. 
% For instance, some open-source applications use ChatGPT API to create characters in video games~\cite{KelSolaar2023} and their users 
For instance, some applications supply a series of prompts to the LLM (ChatGPT) to create a character in a video game and then interact with the character by asking questions~\cite{KelSolaar2023}.
%Other applications~\cite{??} use ChatGPT to summarize technical papers or long documents. \jc{why is this using conversation history?}
Chat app users themselves are also intentionally using long prompts to offer more background
information (i.e., context) to the LLM. For example,
in few-shot learning, users provide several long examples and their desired responses to the LLM before  ask the real questions~\cite{brown2020language, few_shot_se}.
% \jc{need citations here}. 

Importantly, LLM applications use {\bf increasingly long} contexts to raise the probability of including the right information needed to generate high-quality, coherent responses.
% Intuitively, longer contexts will more likely include the information needed to generate the response. 
For example, the user may ask ``Which of the following countries generated the most total energy from solar sources in 2019?''~\cite{shi2023replug}. 
It is hard for the LLM to answer the question correctly without retrieving enough background documents for the relevant countries the user is asking for.
Though it is a hypothetical example, many studies have shown that the accuracy of the generated answers increases with more retrieved documents~\cite{fid, izacard2020memory, atlas}. 
For instance, FiD~\cite{fid} found that the accuracy score increased from 40\% to 48\% when increasing the number of context tokens from 1K to 10K.
Retro~\cite{retro} shows that the perplexity (a proxy score of generation quality) improves significantly when increasing the number of context tokens from 6K to 24K. 
% maybe cite self-retrieval paper here~\cite{self}
%Intuitively, longer contexts can provide more information for LLM to  answer users' questions.

To take in such long contexts, the LLM industry has been training LLMs with the capability to accept ever longer input sequences. 
For instance, Vicuna models~\cite{zheng2023judging}, GPT-4-32K~\cite{openai2023gpt4}, and MPT models~\cite{MosaicML2023Introducing} can take up to 32K tokens as input. 
Latest models like LongNet~\cite{ding2023longnet} can even take up to 1 billion tokens as input.

In essence, long contexts play an increasingly important role in LLM applications for two reasons.
% - llm's superb ability to learn from text
First, modern LLMs have a superb ability to reason about new texts and potentially learn new knowledge from them. 
To exploit this ability, many works on in-context learning aim at optimizing what should the LLM input encompass to induce better responses from LLMs.
% \jc{some numbers here}
% - fine-tuning is often not feasible
Second, while LLMs are sometimes fine-tuned in specific domains, it is not always feasible.
For instance, it is unrealistic to fine-tune an LLM for each user in chat apps.
The background database may be managed separately from the LLM provider in retrieval-based apps.
Due to their huge number of parameters, fine-tuning LLMs is also slow and can be very tricky to do right (\eg catastrophic forgetting, loss of reasoning ability, etc~\cite{lin2023speciality, ding2023selfagreement}
% \jc{find some citations}
).




\tightsubsection{\hspace{-0.2cm}Saving computation by KV cache}
\label{subsec:cache}

Recall that the computation overhead of the transformer (attention module) on a context grows superlinearly (quadratically) with longer contexts (\S\ref{subsec:transformer}), so longer contexts will dramatically increase the computation delay (Figure~\ref{fig:motivate_baselines}a). 

Many recent works have tackled the long contexts' {\em computation} overheads.
A common optimization, illustrated in Figure~\ref{fig:motivate_baselines}b, is to cache the intermediate outcomes of contexts, namely the key and value (KV) features, in GPU memory.
For a given text with $\NumTokens$ tokens, the KV features are two tensors, each with the shape $[\NumTokens, \NumChannels, \NumLayers]$, 
%, each of size $\NumTokens\times\NumChannels\times\NumLayers$, 
where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
For instance, with the LLaMa-7B model, there are 4096 channels and 32 layers.
%As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features can be cached by LLM applications.

When the context is used again as part of another LLM input, one can save the computation delay of processing the context by using its KV features to reconstruct the self-attention matrices of the context. 
To put it more concretely, the computation delay can be reduced by about 15-30$\times$ for the Llama-7B model on contexts with more than 5K tokens, assuming the KV features are already in GPU. 
% \jc{Yuhan, can you add a sentence here to highlight that compute delay can be reduced 10-20 times with a kv cache?}


Caching KV features of a context, called a {\bf KV cache},\footnote{We use a context's KV features and its KV cache interchangeably.} can be used in both chat apps and retrieval-based apps. 
In chat apps, the context is the past prompts and responses, whose KV features can be cached when the past prompts were first processed and responses were first generated~\cite{dai*2019transformerxl}. 
% , and their KV features can be cached when they are first processed (for prompts) and generated (for responses)~\cite{??,??}.
Retrieval-based apps often preprocess each background document by the LLM to compute the self-attention matrices and cache their KV features~\cite{borzunov2023distributed, mohtashami2023landmark, miao2023specinfer, dejong2023fido}.

%\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}
%the KV features of these highly dynamic contexts have to be obtained on the fly.

%\yh{Should we add the discussion of discussion of KV feature shrinking related work here?}


%\begin{comment}
%
%Some emerging research shrinking the tensor size of KV cache, in order to further speed up the computation or fit more contexts in GPU memory.
%For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits, and Scissorhand~\cite{??} proposed to prune less important tokens from the long context. 
%Some more recent proposals~\cite{incontext-autoencoder, gisting} modify the pre-trained LLMs or train a new autoencoder to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
%%However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 
%
%\end{comment}

%Essentially, LLM systems for long contexts assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delay and keeping the KV cache of more contexts in memory.


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}

\tightsection{Hidden network delays of loading contexts}


% \shan{I suggest making this sub-section a separate section and
% name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% section is REALLY tooo long. 2. this sub-section is actually not
% a background. instead, it is an important observation made by us
% that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% make it a separate section. If it is in background, it sounds
% more like previous work's observation.}
Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
\yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}
In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
\yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% \yh{Per request Bandwidth needs to be within a reasonable range  }
% \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% }
% \todo{}

% \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% \todo{More evidences on why context is not in GPU}
In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
\yhedit{A common practice for developers using existing LLM frameworks like Langchain or LlamaIndex is building the vector databases which store the context documents locally on their own machines, while hosting the LLMs in the cloud~\cite{nimje_2023, blog3, autogpt, ZillizTech2023, blog4}.}

One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% and the storage server on which LLM inference runs may not have enough space to store them.
For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
%and storing these texts can take a space up to around 750 GB. 
In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% \jc{please add some evidence and citations here}
% \yh{todo: add more citations for retrieval-based apps}

In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% \jc{please add some evidence and citations here}
Moreover, a user may issue her prompts to the LLM from different locations at different points.
As these prompts can be processed by different machines, the contexts must be remotely fetched.



%In this work, we assume that the context is stored in a different machine than the GPUs running the LLM
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}

As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context.
However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.
%Though the size of KV cache is not a serious issue when the KV cache resides in GPU memory, it will become a communication bottleneck if the KV cache needs to be dynamically loaded from a different machine to GPU memory.
%This is because KV features can have a large size. 
%For a given text with $\NumTokens$ tokens, the KV features are two tensors, each of size $\NumTokens\cdot\NumChannels\cdot\NumLayers$, where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
%(with 32 layers and 4096 channels) can be 1.3~GB. 
%for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
%On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
This network bottleneck does not only affect one model.
As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/motivate_v6_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\tightsection{Background and Motivation}

\vspace{0.2cm}

\begin{figure*}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
    \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
    \label{fig:motivate_query_examples}
\end{figure*}

\tightsubsection{Transformer basics}
\label{subsec:transformer}

{\bf Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks~\cite{vaswani2023attention, openai2023gpt4, palm, brown2020language, kasneci2023chatgpt, retro, zhai2022scaling}.
Today, most generative NLP services are based on transformer models, including T5~\cite{raffel2023exploring}, Llama~\cite{touvron2023llama}, PaLM~\cite{palm}, OPT~\cite{zhang2022opt}, and BLOOM. 
%For these reasons, we focus on transformer-based LLMs in this work.
%Here, we provide a general introduction to transformer architecture. 
%We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
%Readers can refer to \fillme for a more involved introduction.

A transformer model takes as input a sequence of tokenized words and generates an output response, which is another sequence of tokens (usually in the format of integers) \footnote{``Tokens'' in NLP stands for the input unit that is used for DNN inference, which includes punctuations or splitting words into characters. Tokenizing input is typically fast. We will use ``tokens'' in the rest of the paper. }. 
% \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
This generation process includes two high-level steps.
First, the attention module processes the input tokens to obtain encoded features.
% \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
Then, the encoded features of the input are utilized to generate new tokens in an autoregressive manner. 
Specifically, the input tokens and previously generated tokens are fed into the transformer model to generate the next token.  
% \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

The key of the transformer architecture is 
%a neural network (NN) called 
the attention module. 
Each layer of the attention module produces an attention matrix, which models the connections between each pair of tokens. 
The attention matrix at every layer is obtained by applying a non-linear neural network operation on the attention matrix of its previous layer.
Intuitively, the attention matrices of deeper layers might embed a more complex understanding of the tokens under consideration. 


While the attention module is crucial, it is known to be compute-intensive. 
Given an input of $\NumTokens$ tokens, the computation overhead of computing the attention matrices grows quadratically, $O(\NumTokens^2)$.
Though the complexity could be reduced to $O(\NumTokens\textrm{log}\NumTokens)$ (\eg~\cite{luo2021stable, kitaev2020reformer}), such reduction often degrades the
generation quality. 
Once the attention matrices are obtained, the time to generate (decode) each token is quite marginal and can be reduced to almost constant on GPUs.


\tightsubsection{Long contexts in LLM applications}
\label{subsec:apps}

Traditionally, the input of an LLM is a relatively short {\em prompt}, as illustrated in Figure~\ref{fig:motivate_query_examples}(a).
Since the prompt contains limited information, the LLM generates the response based solely on the knowledge already embedded in the LLM itself. 

However, as LLMs are used in more real-world applications, it is no longer sufficient to rely on the knowledge embedded in the LLM.
Instead, LLM applications often append additional texts, referred to as the 
{\bf context}, to supplement the prompt input to an LLM\footnote{Since these contexts are often automatically added, users do not notice or need to manually type them.}.
To make our discussion more concrete, we highlight two types of applications, retrieval-based apps and chat apps.%, which often add long context to supplement their LLM input.


{\em Retrieval-based apps (Figure~\ref{fig:motivate_query_examples}b)} 
use LLMs to answer queries that require domain-specific knowledge.
Examples include question-answering systems~\cite{rubin2023long, retro, fid}, code understanding systems~\cite{rubin2023long, lewis2020retrieval} or fact verification systems~\cite{fid, lewis2020retrieval}.
% \jc{give a few examples from those retrieval-based learning papers.}
They use a background database that contains a large number of background documents.
On retrieving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM. 
\edit{Note that the search procedure is done by a \textit{seperate} DNN or a vector similarity search algorithm, which is not part of the LLM.}

% \jc{yuhan, i temporarily changed all the appearances of the term "retriever" to "application", simply because it's not defined yet and i don't know what it is. if you think it's not appropriate, please define it and change the term back to retriever}
% \edit{

% % For example, given the question ``When did the first mammal appear on Earth''~\cite{metablog2023}, the application selects documents on ``Mammals'', ``History of Earth'', or ``Evolution of Mammals''. 
% % % Then, the apps concatenate the tokens from the retrieved documents and feed the concatenated contexts into the LLM. 

% \jc{this paragraph is simultaneously doing too much and too little :) 
% on one hand, it talks too much detail about the search algorithms (which can be moved to related work).
% on the other hand, it doesn't make clear that the search delay is separate from what we optimize --- the loading and processing delays of long context.}
% }

% On receiving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM.


{\em Chat apps (Figure~\ref{fig:motivate_query_examples}c)} 
become popular with the rise of OpenAI's ChatGPT and have many similar products~\cite{google_bard, microsoft_bing}. %, \eg Google BARD, Facebook Blender, Microsoft DialoGPT.
% \jc{some names of chat apps}
%The conversational history between a user and the LLM can be seen as the ``memory''.
To produce high-quality and coherent responses, a user's conversation history with the LLM, or at least part of it, is often included in the input to the LLM as the context. 
% For instance, some open-source applications use ChatGPT API to create characters in video games~\cite{KelSolaar2023} and their users 
For instance, some applications supply a series of prompts to the LLM (ChatGPT) to create a character in a video game and then interact with the character by asking questions~\cite{KelSolaar2023}.
%Other applications~\cite{??} use ChatGPT to summarize technical papers or long documents. \jc{why is this using conversation history?}
Chat app users themselves are also intentionally using long prompts to offer more background
information (i.e., context) to the LLM. For example,
in few-shot learning, users provide several long examples and their desired responses to the LLM before  ask the real questions~\cite{brown2020language, few_shot_se}.
% \jc{need citations here}. 

Importantly, LLM applications use {\bf increasingly long} contexts to raise the probability of including the right information needed to generate high-quality, coherent responses.
% Intuitively, longer contexts will more likely include the information needed to generate the response. 
For example, the user may ask ``Which of the following countries generated the most total energy from solar sources in 2019?''~\cite{shi2023replug}. 
It is hard for the LLM to answer the question correctly without retrieving enough background documents for the relevant countries the user is asking for.
Though it is a hypothetical example, many studies have shown that the accuracy of the generated answers increases with more retrieved documents~\cite{fid, izacard2020memory, atlas}. 
For instance, FiD~\cite{fid} found that the accuracy score increased from 40\% to 48\% when increasing the number of context tokens from 1K to 10K.
Retro~\cite{retro} shows that the perplexity (a proxy score of generation quality) improves significantly when increasing the number of context tokens from 6K to 24K. 
% maybe cite self-retrieval paper here~\cite{self}
%Intuitively, longer contexts can provide more information for LLM to  answer users' questions.

To take in such long contexts, the LLM industry has been training LLMs with the capability to accept ever longer input sequences. 
For instance, Vicuna models~\cite{zheng2023judging}, GPT-4-32K~\cite{openai2023gpt4}, and MPT models~\cite{MosaicML2023Introducing} can take up to 32K tokens as input. 
Latest models like LongNet~\cite{ding2023longnet} can even take up to 1 billion tokens as input.

In essence, long contexts play an increasingly important role in LLM applications for two reasons.
% - llm's superb ability to learn from text
First, modern LLMs have a superb ability to reason about new texts and potentially learn new knowledge from them. 
To exploit this ability, many works on in-context learning aim at optimizing what should the LLM input encompass to induce better responses from LLMs.
% \jc{some numbers here}
% - fine-tuning is often not feasible
Second, while LLMs are sometimes fine-tuned in specific domains, it is not always feasible.
For instance, it is unrealistic to fine-tune an LLM for each user in chat apps.
The background database may be managed separately from the LLM provider in retrieval-based apps.
Due to their huge number of parameters, fine-tuning LLMs is also slow and can be very tricky to do right (\eg catastrophic forgetting, loss of reasoning ability, etc~\cite{lin2023speciality, ding2023selfagreement}
% \jc{find some citations}
).




\tightsubsection{\hspace{-0.2cm}Saving computation by KV cache}
\label{subsec:cache}

Recall that the computation overhead of the transformer (attention module) on a context grows superlinearly (quadratically) with longer contexts (\S\ref{subsec:transformer}), so longer contexts will dramatically increase the computation delay (Figure~\ref{fig:motivate_baselines}a). 

Many recent works have tackled the long contexts' {\em computation} overheads.
A common optimization, illustrated in Figure~\ref{fig:motivate_baselines}b, is to cache the intermediate outcomes of contexts, namely the key and value (KV) features, in GPU memory.
For a given text with $\NumTokens$ tokens, the KV features are two tensors, each with the shape $[\NumTokens, \NumChannels, \NumLayers]$, 
%, each of size $\NumTokens\times\NumChannels\times\NumLayers$, 
where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
For instance, with the LLaMa-7B model, there are 4096 channels and 32 layers.
%As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features can be cached by LLM applications.

When the context is used again as part of another LLM input, one can save the computation delay of processing the context by using its KV features to reconstruct the self-attention matrices of the context. 
To put it more concretely, the computation delay can be reduced by about 15-30$\times$ for the Llama-7B model on contexts with more than 5K tokens, assuming the KV features are already in GPU. 
% \jc{Yuhan, can you add a sentence here to highlight that compute delay can be reduced 10-20 times with a kv cache?}


Caching KV features of a context, called a {\bf KV cache},\footnote{We use a context's KV features and its KV cache interchangeably.} can be used in both chat apps and retrieval-based apps. 
In chat apps, the context is the past prompts and responses, whose KV features can be cached when the past prompts were first processed and responses were first generated~\cite{dai*2019transformerxl}. 
% , and their KV features can be cached when they are first processed (for prompts) and generated (for responses)~\cite{??,??}.
Retrieval-based apps often preprocess each background document by the LLM to compute the self-attention matrices and cache their KV features~\cite{borzunov2023distributed, mohtashami2023landmark, miao2023specinfer, dejong2023fido}.

%\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}
%the KV features of these highly dynamic contexts have to be obtained on the fly.

%\yh{Should we add the discussion of discussion of KV feature shrinking related work here?}


%\begin{comment}
%
%Some emerging research shrinking the tensor size of KV cache, in order to further speed up the computation or fit more contexts in GPU memory.
%For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits, and Scissorhand~\cite{??} proposed to prune less important tokens from the long context. 
%Some more recent proposals~\cite{incontext-autoencoder, gisting} modify the pre-trained LLMs or train a new autoencoder to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
%%However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 
%
%\end{comment}

%Essentially, LLM systems for long contexts assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delay and keeping the KV cache of more contexts in memory.


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}

\tightsection{Hidden network delays of loading contexts}


% \shan{I suggest making this sub-section a separate section and
% name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% section is REALLY tooo long. 2. this sub-section is actually not
% a background. instead, it is an important observation made by us
% that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% make it a separate section. If it is in background, it sounds
% more like previous work's observation.}
Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
\yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}
In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
\yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% \yh{Per request Bandwidth needs to be within a reasonable range  }
% \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% }
% \todo{}

% \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% \todo{More evidences on why context is not in GPU}
In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
\yhedit{A common practice for developers using existing LLM frameworks like Langchain or LlamaIndex is building the vector databases which store the context documents locally on their own machines, while hosting the LLMs in the cloud~\cite{nimje_2023, blog3, autogpt, ZillizTech2023, blog4}.}

One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% and the storage server on which LLM inference runs may not have enough space to store them.
For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
%and storing these texts can take a space up to around 750 GB. 
In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% \jc{please add some evidence and citations here}
% \yh{todo: add more citations for retrieval-based apps}

In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% \jc{please add some evidence and citations here}
Moreover, a user may issue her prompts to the LLM from different locations at different points.
As these prompts can be processed by different machines, the contexts must be remotely fetched.



%In this work, we assume that the context is stored in a different machine than the GPUs running the LLM
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}

As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context.
However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.
%Though the size of KV cache is not a serious issue when the KV cache resides in GPU memory, it will become a communication bottleneck if the KV cache needs to be dynamically loaded from a different machine to GPU memory.
%This is because KV features can have a large size. 
%For a given text with $\NumTokens$ tokens, the KV features are two tensors, each of size $\NumTokens\cdot\NumChannels\cdot\NumLayers$, where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
%(with 32 layers and 4096 channels) can be 1.3~GB. 
%for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
%On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
This network bottleneck does not only affect one model.
As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/motivate_v7.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\tightsection{Background and Motivation}

\vspace{0.2cm}

To help understand KV cache streaming and its challenges, we start with a primer on transformers and KV cache. 

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/kvcache-illustrated.pdf}
    \tightcaption{An illustration of the KV cache.} 
    \label{fig:kvcache-illustrated}
\end{figure}

% \begin{figure*}
% \centering
%      \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
%     \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
%     \label{fig:motivate_query_examples}
% \end{figure*}

\tightsubsection{Transformer basics}
\label{subsec:transformer}


% {\bf Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks~\cite{vaswani2023attention, openai2023gpt4, palm, brown2020language, kasneci2023chatgpt, retro, zhai2022scaling}.
Transformers~\cite{??,??,??} have become the de facto model for most generative services, including natural language generation, code generation (\eg~\cite{??}), and more~\cite{??}. 
% Today, most generative natural language processing (NLP) services are based on transformer models, such as GPT~\cite{??}, Bard~\cite{??}, Llama~\cite{touvron2023llama}, T5~\cite{raffel2023exploring}, PaLM~\cite{palm}, OPT~\cite{zhang2022opt}, and BLOOM. 
%For these reasons, we focus on transformer-based LLMs in this work.
%Here, we provide a general introduction to transformer architecture. 
%We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
%Readers can refer to \fillme for a more involved introduction.
At a high level, most transformers take a sequence of tokenized words as input and generate a sequence of tokens as the output response.\footnote{A ``token'' is the input unit used by transformer inference. It can be a punctuation, a word, or a part of a word. 
The delay of tokenizing an input prompt is typically negligible compared to the generation process, so we assume that tokens are the input to the transformer.}
% splitting words into characters. Tokenizing input is typically fast. We will use ``tokens'' in the rest of the paper. }. 
% \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
The generation process has two phases.
In the prefill phase, the attention module processes the input tokens to obtain encoded features called KV cache (explained shortly).
% \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
In the generation phase, the KV cache of the input is used to generate new tokens in an autoregressive manner. 
% Specifically, the input tokens and previously generated tokens are fed into the transformer model to generate the next token.  
% \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

% The key in the prefill phase is
% %a neural network (NN) called 
% the attention module. 
The attention module contains multiple layers, each producing one layer in the key (K) vector and value (V) vector in the KV cache (Figure~\ref{fig:kvcache-illustrated}).
The KV vectors at each layer can produce an attention matrix, which models the connections between each token pair. 
The attention matrix at every layer is effectively a result of applying non-linear neural network operations on the attention matrix of its previous layer.
Intuitively, the attention matrix of a deeper layer captures a more complex understanding of the tokens under consideration. 


The prefill phase is known to be compute-intensive. 
% For an input of $\NumTokens$ tokens, 
The computation overhead of the attention module %computing the attention matrices 
grows quadratically with the number of input tokens.
Though the complexity could be reduced to log-linear 
% $O(\NumTokens\textrm{log}\NumTokens)$ 
(\eg~\cite{luo2021stable, kitaev2020reformer}), such reduction often degrades the generation quality and the overhead is still superlinear.
After the prefill phase, 
% Once the attention matrices are obtained, 
the delay to generate tokens is proportional to the number of generated tokens.
Thus, the prefill phase determines when the user sees the first token, and if the answer is relatively shorter than the input context and prompt (\eg question-answering), the prefill phase can dominate the overall delay.
% is almost constant on GPU and 
% is quite marginal and can be reduced to almost constant on GPUs.


\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples_short.pdf}
    \tightcaption{LLMs increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
    \label{fig:motivate_query_examples}
\end{figure}


\tightsubsection{Long contexts in LLM applications}
\label{subsec:apps}

The input {\em prompt} to language models was traditionally short, but then the LLM generates the response based solely on the knowledge already embedded in the LLM itself, causing low quality and ``hallucination'' if the response requires new knowledge. 
% Since the prompt contains limited information, the LLM generates the response based solely on the knowledge already embedded in the LLM itself. 
As LLMs are used in more real-world applications, it is no longer sufficient to rely on the knowledge embedded in the LLM.
Instead, LLM applications often append additional texts, referred to as the 
{\bf context}, to supplement the prompt input to an LLM.
% \footnote{Since these contexts are often automatically added, users do not notice or need to manually type them.}.
To make our discussion more concrete, we highlight two types of applications, retrieval-based apps and chat apps, where long contexts are often used to supplement their LLM input.%, which often add long context to supplement their LLM input.


{\em Retrieval-based apps (Figure~\ref{fig:motivate_query_examples}b)} 
use LLMs to answer queries that require domain-specific knowledge.
Examples include question-answering (QA)~\cite{rubin2023long, retro, fid}, understanding a specific code repository~\cite{rubin2023long, lewis2020retrieval} or verifying fact based on latest documents~\cite{fid, lewis2020retrieval}. \jc{yuhan, the citation seems a bit outdated. can you replace the old ones with newer pointers? also mostly citations are papers. maybe a good idea to cite some real products or open-source apps}
% \jc{give a few examples from those retrieval-based learning papers.}
They use a background database that contains a large number of background documents.
On retrieving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM. 
\edit{Note that the search procedure is done by a \textit{seperate} DNN or a vector similarity search algorithm, which is not part of the LLM.}

% \jc{yuhan, i temporarily changed all the appearances of the term "retriever" to "application", simply because it's not defined yet and i don't know what it is. if you think it's not appropriate, please define it and change the term back to retriever}
% \edit{

% % For example, given the question ``When did the first mammal appear on Earth''~\cite{metablog2023}, the application selects documents on ``Mammals'', ``History of Earth'', or ``Evolution of Mammals''. 
% % % Then, the apps concatenate the tokens from the retrieved documents and feed the concatenated contexts into the LLM. 

% \jc{this paragraph is simultaneously doing too much and too little :) 
% on one hand, it talks too much detail about the search algorithms (which can be moved to related work).
% on the other hand, it doesn't make clear that the search delay is separate from what we optimize --- the loading and processing delays of long context.}
% }

% On receiving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM.


{\em Chat apps (Figure~\ref{fig:motivate_query_examples}c)} 
have become popular with the rise of OpenAI's ChatGPT and several other similar services~\cite{google_bard, microsoft_bing}. %, \eg Google BARD, Facebook Blender, Microsoft DialoGPT.
% \jc{some names of chat apps}
%The conversational history between a user and the LLM can be seen as the ``memory''.
To obtain high quality responses, Chat app users often intentionally use long prompts to offer more background
information (i.e., context) to the LLM. For example,
in few-shot learning, users provide several long examples and their desired responses to the LLM before ask the real questions~\cite{brown2020language, few_shot_se}.
% \jc{need citations here}. 
Furthermore, to produce coherent responses over time, all or part of a user's conversation history with the LLM is often included by the chat app in the input to the LLM as the context. 
% For instance, some open-source applications use ChatGPT API to create characters in video games~\cite{KelSolaar2023} and their users 
For instance, some applications supply a series of prompts to the LLM (ChatGPT) to create a character in a video game and then interact with the character by asking questions~\cite{KelSolaar2023}.
\shan{I slightly re-organized this paragraph.}
%Other applications~\cite{??} use ChatGPT to summarize technical papers or long documents. \jc{why is this using conversation history?}

Importantly, LLM applications use {\bf increasingly long} contexts to raise the probability of including the right information needed to generate high-quality, coherent responses.
% Intuitively, longer contexts will more likely include the information needed to generate the response. 
For example, the user may ask ``Which of the following countries generated the most total energy from solar sources in 2019?''~\cite{shi2023replug}. 
It is hard for the LLM to answer the question correctly without retrieving enough background documents for the relevant countries the user is asking for.
Though it is a hypothetical example, many studies have shown that the accuracy of the generated answers increases with more retrieved documents~\cite{fid, izacard2020memory, atlas}.
\shan{The last three sentences, ``For example ... It is hard ... Though it is ...'', do not seem to belong here. They seem to belong to the ``retrieval-based apps'' paragraph?}
For instance, FiD~\cite{fid} found that the accuracy score increased from 40\% to 48\% when increasing the number of context tokens from 1K to 10K.
Retro~\cite{retro} shows that the perplexity (a proxy score of generation quality) improves significantly when increasing the number of context tokens from 6K to 24K. 
% maybe cite self-retrieval paper here~\cite{self}
%Intuitively, longer contexts can provide more information for LLM to  answer users' questions.

\yhedit{Although the benefits of incorporating long contexts is substantial, the key bottleneck in incorporating longer context is the high-end computation resource required to train those LLMs with longer context~\cite{??}. 
To tackle this,}\shan{??This newly added sentence doesn't seem to be relevant to this project. Does it?}
% To take in such long contexts,
the LLM industry has been training LLMs with the capability to accept even longer input sequences with more advanced GPUs. 
For instance, Vicuna models~\cite{zheng2023judging}, GPT-4-32K~\cite{openai2023gpt4}, and MPT models~\cite{MosaicML2023Introducing} can take up to 32K tokens as input. 
Latest models like LongNet~\cite{ding2023longnet} can even take up to 1 billion tokens as input.
\yhedit{Another line of work, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and so on~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing, ??},  enables longer input sequences by activating an extra decision logic in the self-attention module.
This module allows it not to connect each pair of tokens, but only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and with this enabled, longer sequences can be taken by the LLMs.
We refer to these works as ``text-shortening'' techniques. 
}


In essence, long contexts play an increasingly important role in LLM applications for two reasons.
% - llm's superb ability to learn from text
First, modern LLMs have a superb ability to reason about new texts and potentially learn new knowledge from them. 
To exploit this ability, many works on in-context learning aim at optimizing what should the LLM input encompass to induce better responses from LLMs.
% \jc{some numbers here}
% - fine-tuning is often not feasible
Second, while LLMs are sometimes fine-tuned in specific domains, it is not always feasible.
For instance, it is unrealistic to fine-tune an LLM for each user in chat apps.
The background database may be managed separately from the LLM provider in retrieval-based apps.\shan{This sentence does not belong here.}
Due to their huge number of parameters, fine-tuning LLMs is also slow and can be very tricky to do right (\eg catastrophic forgetting, loss of reasoning ability, etc~\cite{lin2023speciality, ding2023selfagreement}
% \jc{find some citations}
).




\tightsubsection{\hspace{-0.2cm}Saving computation by KV cache}
\label{subsec:cache}

Recall that the computation overhead of the transformer (attention module) on a context grows superlinearly (quadratically) with longer contexts (\S\ref{subsec:transformer}), so longer contexts will dramatically increase the computation delay (Figure~\ref{fig:motivate_baselines}a). 

Many recent works have tackled the long contexts' {\em computation} overheads.
A common optimization, illustrated in Figure~\ref{fig:motivate_baselines}b, is to cache the intermediate outcomes of contexts, namely the key and value (KV) features, in GPU memory.
For a given text with $\NumTokens$ tokens, the KV features are two tensors, each with the shape $[\NumTokens, \NumChannels, \NumLayers]$, 
%, each of size $\NumTokens\times\NumChannels\times\NumLayers$, 
where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
For instance, with the LLaMa-7B model, there are 4096 channels and 32 layers.
%As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features can be cached by LLM applications.

When the context is used again as part of another LLM input, one can save the computation delay of processing the context by using its KV features to reconstruct the self-attention matrices of the context. 
To put it more concretely, the computation delay can be reduced by about 15-30$\times$ for the Llama-7B model on contexts with more than 5K tokens, assuming the KV features are already in GPU. 
% \jc{Yuhan, can you add a sentence here to highlight that compute delay can be reduced 10-20 times with a kv cache?}


Caching KV features of a context, called a {\bf KV cache},\footnote{We use a context's KV features and its KV cache interchangeably.} can be used in both chat apps and retrieval-based apps. 
In chat apps, the context is the past prompts and responses, whose KV features can be cached when the past prompts were first processed and responses were first generated~\cite{dai*2019transformerxl}. 
% , and their KV features can be cached when they are first processed (for prompts) and generated (for responses)~\cite{??,??}.
% Retrieval-based apps often preprocess each background document by the LLM to compute the self-attention matrices and cache their KV features~\cite{borzunov2023distributed, mohtashami2023landmark, miao2023specinfer, dejong2023fido}.
\yhedit{In retrieval apps, the context is the background documents that are used to support answering users' questions. 
%The KV cache for the background documents used in previous queries can be cached.
%This can help avoid the computation of self-attention matrices for future queries.
As a concrete example, LangChain~\cite{??}, which is a popular LLM inference framework, builds a retrieval-based app that allows users to ask any questions on how to write specific functionalities with it.
For example, users can ask a question ``how to use Langchain to build a vector database to search for relevant documents to answer a question?'', and corresponding pages in LangChain's documentation will be retrieved to answer it. 
% \shan{This sentence is very confusing. Is ``langchain'' an example of ``libraries''? If so, langchain builds retrieval-based apps that allow 
% users to ask questions on how to write specific functionalities with langchain??}. 
% In this case, when users submit questions, corresponding pages of the documentation\shan{what documentation?} will be retrieved to answer them. 
Thus, most of, if not all, pages in LangChain's documentation can be cached to avoid recomputation of the self-attention matrices.\yh{Ask ganesh about more examples. } 
\yh{Add enterprise apps examples?}


}


% ``The Code Library Help'' ChatGPT plugin, when users ask questions about specific libraries (\eg TensorFlow, PyTorch), the plugin will query the documentation or codebase of the libraries to answer the questions. 
% In this app, the KV cache for codebase or documentations of very popular  libraries, such as TensorFlow, PyTorch, or OpenAI, can be cached to avoid recomputing their self-attention matrices.\yh{Justify why not fine-tune the LLM? } 



% \begin{figure}
% \centering
%      \includegraphics[width=.99\linewidth]{figs/h2o_motivation.pdf}
%     \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
%     \label{fig:h2o_motivation}
% \end{figure}

% In the above scenarios, the KV cache of the context is already generated before, and needs to be loaded back into GPU memory, as shown in figure~\ref{fig:h2o_motivation}a.
% No prior work shares the same goal as ours. 
% One line of prior works~\cite{zhang2023h2o, scissorhand} reduces the GPU memory consumption of using KV cache for faster generation. 
% However, as illustrated in figure~\ref{fig:h2o_motivation}b, they assume the KV cache is freshly generated from the raw text input. 
% Then the newly generated KV cache is used by the process of generating more tokens in order to avoid the recomputation of self-attention matrices for all the previously generated tokens. 
% They try to reduce the memory usage of the KV cache so that it can fit into limited GPU memory for generating later tokens, by selecting important tokens to keep. 






%\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}
%the KV features of these highly dynamic contexts have to be obtained on the fly.

%\yh{Should we add the discussion of discussion of KV feature shrinking related work here?}


%\begin{comment}
%
%Some emerging research shrinking the tensor size of KV cache, in order to further speed up the computation or fit more contexts in GPU memory.
%For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits, and Scissorhand~\cite{??} proposed to prune less important tokens from the long context. 
%Some more recent proposals~\cite{incontext-autoencoder, gisting} modify the pre-trained LLMs or train a new autoencoder to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
%%However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 
%
%\end{comment}

%Essentially, LLM systems for long contexts assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delay and keeping the KV cache of more contexts in memory.


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}


% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

\tightsection{Hidden network delays of loading contexts}


% \shan{I suggest making this sub-section a separate section and
% name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% section is REALLY tooo long. 2. this sub-section is actually not
% a background. instead, it is an important observation made by us
% that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% make it a separate section. If it is in background, it sounds
% more like previous work's observation.}
Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
\yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance.
In this case, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
This is because the size of the KV cache is much bigger than the text context itself.
To be more concrete, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
}
\shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.}
\jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% \yh{Per request Bandwidth needs to be within a reasonable range  }
% \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% }
% \todo{}


In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.

In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
Moreover, a user may issue her prompts to the LLM from different locations at different points.
As these prompts can be processed by different machines, the contexts must be remotely fetched.




\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}

As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large, as discussed before.
Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
%(with 32 layers and 4096 channels) can be 1.3~GB. 
%for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
%On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
This network bottleneck does not only affect one model.
As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/motivate_v7_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\tightsection{Background and Motivation}

\vspace{0.2cm}

To help understand KV cache streaming and its challenges, we start with a primer on transformers and KV cache. 

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/kvcache-illustrated.pdf}
    \tightcaption{An illustration of the KV cache.} 
    \label{fig:kvcache-illustrated}
\end{figure}

% \begin{figure*}
% \centering
%      \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
%     \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
%     \label{fig:motivate_query_examples}
% \end{figure*}

\tightsubsection{Transformer basics}
\label{subsec:transformer}


% {\bf Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks~\cite{vaswani2023attention, openai2023gpt4, palm, brown2020language, kasneci2023chatgpt, retro, zhai2022scaling}.
Transformers~\cite{??,??,??} have become the de facto model for most generative services, including natural language generation, code generation (\eg~\cite{??}), and more~\cite{??}. 
% Today, most generative natural language processing (NLP) services are based on transformer models, such as GPT~\cite{??}, Bard~\cite{??}, Llama~\cite{touvron2023llama}, T5~\cite{raffel2023exploring}, PaLM~\cite{palm}, OPT~\cite{zhang2022opt}, and BLOOM. 
%For these reasons, we focus on transformer-based LLMs in this work.
%Here, we provide a general introduction to transformer architecture. 
%We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
%Readers can refer to \fillme for a more involved introduction.
At a high level, most transformers take a sequence of tokenized words as input and generate a sequence of tokens as the output response.\footnote{A ``token'' is the input unit used by transformer inference. It can be a punctuation, a word, or a part of a word. 
The delay of tokenizing an input prompt is typically negligible compared to the generation process, so we assume that tokens are the input to the transformer.}
% splitting words into characters. Tokenizing input is typically fast. We will use ``tokens'' in the rest of the paper. }. 
% \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
The generation process has two phases.
In the prefill phase, the attention module processes the input tokens to obtain encoded features called KV cache (explained shortly).
% \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
In the generation phase, the KV cache of the input is used to generate new tokens in an autoregressive manner. 
% Specifically, the input tokens and previously generated tokens are fed into the transformer model to generate the next token.  
% \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

% The key in the prefill phase is
% %a neural network (NN) called 
% the attention module. 
The attention module contains multiple layers, each producing one layer in the key (K) vector and value (V) vector in the KV cache (Figure~\ref{fig:kvcache-illustrated}).
The KV vectors at each layer can produce an attention matrix, which models the connections between each token pair. 
The attention matrix at every layer is effectively a result of applying non-linear neural network operations on the attention matrix of its previous layer.
Intuitively, the attention matrix of a deeper layer captures a more complex understanding of the tokens under consideration. 


The prefill phase is known to be compute-intensive. 
% For an input of $\NumTokens$ tokens, 
The computation overhead of the attention module %computing the attention matrices 
grows quadratically with the number of input tokens.
Though the complexity could be reduced to log-linear 
% $O(\NumTokens\textrm{log}\NumTokens)$ 
(\eg~\cite{luo2021stable, kitaev2020reformer}), such reduction often degrades the generation quality and the overhead is still superlinear.
After the prefill phase, 
% Once the attention matrices are obtained, 
the delay to generate tokens is proportional to the number of generated tokens.
Thus, the prefill phase determines when the user sees the first token, and if the answer is relatively shorter than the input context and prompt (\eg question-answering), the prefill phase can dominate the overall delay.
% is almost constant on GPU and 
% is quite marginal and can be reduced to almost constant on GPUs.


\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples_short.pdf}
    \tightcaption{LLMs increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
    \label{fig:motivate_query_examples}
\end{figure}


\tightsubsection{Long contexts in LLM applications}
\label{subsec:apps}

The input {\em prompt} to language models was traditionally short, but then the LLM generates the response based solely on the knowledge already embedded in the LLM itself, causing low quality and ``hallucination'' if the response requires new knowledge. 
% Since the prompt contains limited information, the LLM generates the response based solely on the knowledge already embedded in the LLM itself. 
As LLMs are used in more real-world applications, it is no longer sufficient to rely on the knowledge embedded in the LLM.
Instead, LLM applications often append additional texts, referred to as the 
{\bf context}, to supplement the prompt input to an LLM.
% \footnote{Since these contexts are often automatically added, users do not notice or need to manually type them.}.
To make our discussion more concrete, we highlight two types of applications, retrieval-based apps and chat apps, where long contexts are often used to supplement their LLM input.%, which often add long context to supplement their LLM input.


{\em Retrieval-based apps (Figure~\ref{fig:motivate_query_examples}b)} 
use LLMs to answer queries that require domain-specific knowledge.
Examples include question-answering (QA)~\cite{rubin2023long, retro, fid}, understanding a specific code repository~\cite{rubin2023long, lewis2020retrieval} or verifying fact based on latest documents~\cite{fid, lewis2020retrieval}. \jc{yuhan, the citation seems a bit outdated. can you replace the old ones with newer pointers? also mostly citations are papers. maybe a good idea to cite some real products or open-source apps}
% \jc{give a few examples from those retrieval-based learning papers.}
They use a background database that contains a large number of background documents.
On retrieving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM. 
\edit{Note that the search procedure is done by a \textit{seperate} DNN or a vector similarity search algorithm, which is not part of the LLM.}

% \jc{yuhan, i temporarily changed all the appearances of the term "retriever" to "application", simply because it's not defined yet and i don't know what it is. if you think it's not appropriate, please define it and change the term back to retriever}
% \edit{

% % For example, given the question ``When did the first mammal appear on Earth''~\cite{metablog2023}, the application selects documents on ``Mammals'', ``History of Earth'', or ``Evolution of Mammals''. 
% % % Then, the apps concatenate the tokens from the retrieved documents and feed the concatenated contexts into the LLM. 

% \jc{this paragraph is simultaneously doing too much and too little :) 
% on one hand, it talks too much detail about the search algorithms (which can be moved to related work).
% on the other hand, it doesn't make clear that the search delay is separate from what we optimize --- the loading and processing delays of long context.}
% }

% On receiving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM.


{\em Chat apps (Figure~\ref{fig:motivate_query_examples}c)} 
have become popular with the rise of OpenAI's ChatGPT and several other similar services~\cite{google_bard, microsoft_bing}. %, \eg Google BARD, Facebook Blender, Microsoft DialoGPT.
% \jc{some names of chat apps}
%The conversational history between a user and the LLM can be seen as the ``memory''.
To obtain high quality responses, Chat app users often intentionally use long prompts to offer more background
information (i.e., context) to the LLM. For example,
in few-shot learning, users provide several long examples and their desired responses to the LLM before ask the real questions~\cite{brown2020language, few_shot_se}.
% \jc{need citations here}. 
Furthermore, to produce coherent responses over time, all or part of a user's conversation history with the LLM is often included by the chat app in the input to the LLM as the context. 
% For instance, some open-source applications use ChatGPT API to create characters in video games~\cite{KelSolaar2023} and their users 
For instance, some applications supply a series of prompts to the LLM (ChatGPT) to create a character in a video game and then interact with the character by asking questions~\cite{KelSolaar2023}.
\shan{I slightly re-organized this paragraph.}
%Other applications~\cite{??} use ChatGPT to summarize technical papers or long documents. \jc{why is this using conversation history?}

Importantly, LLM applications use {\bf increasingly long} contexts to raise the probability of including the right information needed to generate high-quality, coherent responses.
% Intuitively, longer contexts will more likely include the information needed to generate the response. 
For example, the user may ask ``Which of the following countries generated the most total energy from solar sources in 2019?''~\cite{shi2023replug}. 
It is hard for the LLM to answer the question correctly without retrieving enough background documents for the relevant countries the user is asking for.
Though it is a hypothetical example, many studies have shown that the accuracy of the generated answers increases with more retrieved documents~\cite{fid, izacard2020memory, atlas}.
\shan{The last three sentences, ``For example ... It is hard ... Though it is ...'', do not seem to belong here. They seem to belong to the ``retrieval-based apps'' paragraph?}
For instance, FiD~\cite{fid} found that the accuracy score increased from 40\% to 48\% when increasing the number of context tokens from 1K to 10K.
Retro~\cite{retro} shows that the perplexity (a proxy score of generation quality) improves significantly when increasing the number of context tokens from 6K to 24K. 
% maybe cite self-retrieval paper here~\cite{self}
%Intuitively, longer contexts can provide more information for LLM to  answer users' questions.

\yhedit{Although the benefits of incorporating long contexts is substantial, the key bottleneck in incorporating longer context is the high-end computation resource required to train those LLMs with longer context~\cite{??}. 
To tackle this,}\shan{??This newly added sentence doesn't seem to be relevant to this project. Does it?}
% To take in such long contexts,
the LLM industry has been training LLMs with the capability to accept even longer input sequences with more advanced GPUs. 
For instance, Vicuna models~\cite{zheng2023judging}, GPT-4-32K~\cite{openai2023gpt4}, and MPT models~\cite{MosaicML2023Introducing} can take up to 32K tokens as input. 
Latest models like LongNet~\cite{ding2023longnet} can even take up to 1 billion tokens as input.
\yhedit{Another line of work, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and so on~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing, ??},  enables longer input sequences by activating an extra decision logic in the self-attention module.
This module allows it not to connect each pair of tokens, but only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and with this enabled, longer sequences can be taken by the LLMs.
We refer to these works as ``text-shortening'' techniques. 
}


In essence, long contexts play an increasingly important role in LLM applications for two reasons.
% - llm's superb ability to learn from text
First, modern LLMs have a superb ability to reason about new texts and potentially learn new knowledge from them. 
To exploit this ability, many works on in-context learning aim at optimizing what should the LLM input encompass to induce better responses from LLMs.
% \jc{some numbers here}
% - fine-tuning is often not feasible
Second, while LLMs are sometimes fine-tuned in specific domains, it is not always feasible.
For instance, it is unrealistic to fine-tune an LLM for each user in chat apps.
The background database may be managed separately from the LLM provider in retrieval-based apps.\shan{This sentence does not belong here.}
Due to their huge number of parameters, fine-tuning LLMs is also slow and can be very tricky to do right (\eg catastrophic forgetting, loss of reasoning ability, etc~\cite{lin2023speciality, ding2023selfagreement}
% \jc{find some citations}
).




\tightsubsection{\hspace{-0.2cm}Saving computation by KV cache}
\label{subsec:cache}

Recall that the computation overhead of the transformer (attention module) on a context grows superlinearly (quadratically) with longer contexts (\S\ref{subsec:transformer}), so longer contexts will dramatically increase the computation delay (Figure~\ref{fig:motivate_baselines}a). 

Many recent works have tackled the long contexts' {\em computation} overheads.
A common optimization, illustrated in Figure~\ref{fig:motivate_baselines}b, is to cache the intermediate outcomes of contexts, namely the key and value (KV) features, in GPU memory.
For a given text with $\NumTokens$ tokens, the KV features are two tensors, each with the shape $[\NumTokens, \NumChannels, \NumLayers]$, 
%, each of size $\NumTokens\times\NumChannels\times\NumLayers$, 
where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
For instance, with the LLaMa-7B model, there are 4096 channels and 32 layers.
%As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features can be cached by LLM applications.

When the context is used again as part of another LLM input, one can save the computation delay of processing the context by using its KV features to reconstruct the self-attention matrices of the context. 
To put it more concretely, the computation delay can be reduced by about 15-30$\times$ for the Llama-7B model on contexts with more than 5K tokens, assuming the KV features are already in GPU. 
% \jc{Yuhan, can you add a sentence here to highlight that compute delay can be reduced 10-20 times with a kv cache?}


Caching KV features of a context, called a {\bf KV cache},\footnote{We use a context's KV features and its KV cache interchangeably.} can be used in both chat apps and retrieval-based apps. 
In chat apps, the context is the past prompts and responses, whose KV features can be cached when the past prompts were first processed and responses were first generated~\cite{dai*2019transformerxl}. 
% , and their KV features can be cached when they are first processed (for prompts) and generated (for responses)~\cite{??,??}.
% Retrieval-based apps often preprocess each background document by the LLM to compute the self-attention matrices and cache their KV features~\cite{borzunov2023distributed, mohtashami2023landmark, miao2023specinfer, dejong2023fido}.
\yhedit{In retrieval apps, the context is the background documents that are used to support answering users' questions. 
%The KV cache for the background documents used in previous queries can be cached.
%This can help avoid the computation of self-attention matrices for future queries.
As a concrete example, LangChain~\cite{??}, which is a popular LLM inference framework, builds a retrieval-based app that allows users to ask any questions on how to write specific functionalities with it.
For example, users can ask a question ``how to use Langchain to build a vector database to search for relevant documents to answer a question?'', and corresponding pages in LangChain's documentation will be retrieved to answer it. 
% \shan{This sentence is very confusing. Is ``langchain'' an example of ``libraries''? If so, langchain builds retrieval-based apps that allow 
% users to ask questions on how to write specific functionalities with langchain??}. 
% In this case, when users submit questions, corresponding pages of the documentation\shan{what documentation?} will be retrieved to answer them. 
Thus, most of, if not all, pages in LangChain's documentation can be cached to avoid recomputation of the self-attention matrices.\yh{Ask ganesh about more examples. } 
\yh{Add enterprise apps examples?}


}


% ``The Code Library Help'' ChatGPT plugin, when users ask questions about specific libraries (\eg TensorFlow, PyTorch), the plugin will query the documentation or codebase of the libraries to answer the questions. 
% In this app, the KV cache for codebase or documentations of very popular  libraries, such as TensorFlow, PyTorch, or OpenAI, can be cached to avoid recomputing their self-attention matrices.\yh{Justify why not fine-tune the LLM? } 



% \begin{figure}
% \centering
%      \includegraphics[width=.99\linewidth]{figs/h2o_motivation.pdf}
%     \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
%     \label{fig:h2o_motivation}
% \end{figure}

% In the above scenarios, the KV cache of the context is already generated before, and needs to be loaded back into GPU memory, as shown in figure~\ref{fig:h2o_motivation}a.
% No prior work shares the same goal as ours. 
% One line of prior works~\cite{zhang2023h2o, scissorhand} reduces the GPU memory consumption of using KV cache for faster generation. 
% However, as illustrated in figure~\ref{fig:h2o_motivation}b, they assume the KV cache is freshly generated from the raw text input. 
% Then the newly generated KV cache is used by the process of generating more tokens in order to avoid the recomputation of self-attention matrices for all the previously generated tokens. 
% They try to reduce the memory usage of the KV cache so that it can fit into limited GPU memory for generating later tokens, by selecting important tokens to keep. 






%\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}
%the KV features of these highly dynamic contexts have to be obtained on the fly.

%\yh{Should we add the discussion of discussion of KV feature shrinking related work here?}


%\begin{comment}
%
%Some emerging research shrinking the tensor size of KV cache, in order to further speed up the computation or fit more contexts in GPU memory.
%For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits, and Scissorhand~\cite{??} proposed to prune less important tokens from the long context. 
%Some more recent proposals~\cite{incontext-autoencoder, gisting} modify the pre-trained LLMs or train a new autoencoder to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
%%However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 
%
%\end{comment}

%Essentially, LLM systems for long contexts assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delay and keeping the KV cache of more contexts in memory.


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}


% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

\tightsection{Hidden network delays of loading contexts}


% \shan{I suggest making this sub-section a separate section and
% name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% section is REALLY tooo long. 2. this sub-section is actually not
% a background. instead, it is an important observation made by us
% that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% make it a separate section. If it is in background, it sounds
% more like previous work's observation.}
Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
\yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance.
In this case, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
This is because the size of the KV cache is much bigger than the text context itself.
To be more concrete, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
}
\shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.}
\jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% \yh{Per request Bandwidth needs to be within a reasonable range  }
% \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% }
% \todo{}


In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.

In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
Moreover, a user may issue her prompts to the LLM from different locations at different points.
As these prompts can be processed by different machines, the contexts must be remotely fetched.




\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}

As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large, as discussed before.
Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
%(with 32 layers and 4096 channels) can be 1.3~GB. 
%for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
%On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
This network bottleneck does not only affect one model.
As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/motivate_v8.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\tightsection{Background and Motivation}

\vspace{0.2cm}

To help understand KV cache streaming and its challenges, we start with a primer on transformers and KV cache. 

\yh{New outline below: }
\begin{itemize}
    \item Section 2.1: transformer basics (Expand the last paragraph of the current 2.1 to say that reusing the KV cache for the context can eliminate time to process the context)
    \item section 2.2: Long contexts in LLM apps 
    \begin{itemize}
        \item LLMs need long context to incorporate new information that's not learned during training so as to reduce hallucination 
        \item Retrieval-based apps answer queries requiring domain-specific knowledge. Relevant context will be retrieved on receiving a query 
        \item For retrieval-based apps, the context can be long since longer context can increase the probability of including right information to answer the question. 
        \item List an example app that is likely to reuse the context used in one query before. (\eg LangChain's ``Chat with our docs'')
        \item Chat-based apps allow users to continuously interact with LLMs (\eg asking questions, solving tasks)
        \item For chat-based apps, it may take the users several rounds to make their requirements more clear and the answer more desirable, leading to long context. 
        \item List an example app that is likely to reuse the chat history. (\eg when user resumed one conversation after some period of time)
        \item Although having many benefits, taking in long contexts makes the prefill delay long since the  delay of the self-attention module grows super-linear to the length of the input. 
      \yh{In some cases, context is long and is reused, do not overclaim}
        
    \end{itemize}
    \item Section 3 KV Cache Streaming
        \begin{itemize}
        \item Section 3.1: Hidden network delay of loading the context 
        \begin{itemize}
            \item One natural way to reuse the context is to store the KV cache and directly load them when needed, like figure 4b. Cite some apps doing so if found? 
            \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            \item This can be slow because the size of the KV cache is large. And will negate the benefit of reusing KV cache.
            \item We want to make the loading of KV cache for reusing as fast as possible. 
            \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
        \item Section 3.2: 
        \begin{itemize}
            \item To make the loading of KV cache as fast as possible, one way to do it is to encode the KV cache to make its size as small as possible, like figure 4c. 
            \item A common way of encoding data transmitted over the network is to encode it into bitstreams. Explain in our case, it would be encoding the original KV cache tensor into bitstreams on the storage server, decoding it back to tensor of original shape on the inference server 
            \item Ideally, the encoder can make the loading delay of KV cache very small  to maximize the benefit of reusing KV cache 
            \item KV cache streaming can also be applied to other scenarios, such as reducing the delay of migrating KV cache in distributed inference setting 
        \end{itemize}
            % \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            % \item This will negate the benefit of reusing KV cache. 
            % \item We want to make the loading of KV cache for reusing as fast as possible. 
            % \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
\end{itemize}

\jc{the outline looks great. thanks! several comments
\begin{itemize}
    \item Right now, 2.2 only says why context can be long, which is not enough. It should explain why contexts can sometimes be long {\bf and} will be reused over time and by different requests. Both are necessary requirements.
    \item Let's drop 2.3, and add a short paragraph (or maybe just expand on an existing one) on the background of kv cache.
    \item I actually think section 3 should go straight to the problem of kv cache streaming. So it will have two subsections. 
    \begin{itemize}
        \item 3.1 (hidden delay of loading context) starts by saying a natural approach to long and reused contexts is by storing the KV cache and loading them when reused. If there's existing system that does this, we can cite them here. The remaining of 3.1 can follow your outline.
        \item 3.2 introduces the goal of kv cache streaming and why it can improve (using fig 4) reusing KV cache of long context. We can also bring up other uses of KV cache streaming (distributed kv cache).  
    \end{itemize}
\end{itemize}
}

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/kvcache-illustrated.pdf}
    \tightcaption{An illustration of the KV cache.} 
    \label{fig:kvcache-illustrated}
\end{figure}

% \begin{figure*}
% \centering
%      \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
%     \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
%     \label{fig:motivate_query_examples}
% \end{figure*}

\tightsubsection{Transformer basics}
\label{subsec:transformer}


% {\bf Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks~\cite{vaswani2023attention, openai2023gpt4, palm, brown2020language, kasneci2023chatgpt, retro, zhai2022scaling}.
Transformers~\cite{??,??,??} have become the de facto model for most generative services, including natural language generation, code generation (\eg~\cite{??}), and more~\cite{??}. 
% Today, most generative natural language processing (NLP) services are based on transformer models, such as GPT~\cite{??}, Bard~\cite{??}, Llama~\cite{touvron2023llama}, T5~\cite{raffel2023exploring}, PaLM~\cite{palm}, OPT~\cite{zhang2022opt}, and BLOOM. 
%For these reasons, we focus on transformer-based LLMs in this work.
%Here, we provide a general introduction to transformer architecture. 
%We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
%Readers can refer to \fillme for a more involved introduction.
At a high level, most transformers take a sequence of tokenized words as input and generate a sequence of tokens as the output response.\footnote{A ``token'' is the input unit used by transformer inference. It can be a punctuation, a word, or a part of a word. 
The delay of tokenizing an input prompt is typically negligible compared to the generation process, so we assume that tokens are the input to the transformer.}
% splitting words into characters. Tokenizing input is typically fast. We will use ``tokens'' in the rest of the paper. }. 
% \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
The generation process has two phases.
In the prefill phase, the attention module processes the input tokens to obtain encoded features called KV cache (explained shortly).
% \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
In the generation phase, the KV cache of the input is used to generate new tokens in an autoregressive manner. 
% Specifically, the input tokens and previously generated tokens are fed into the transformer model to generate the next token.  
% \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

% The key in the prefill phase is
% %a neural network (NN) called 
% the attention module. 
The attention module contains multiple layers, each producing one layer in the key (K) vector and value (V) vector in the KV cache (Figure~\ref{fig:kvcache-illustrated}).
The KV vectors at each layer can produce an attention matrix, which models the connections between each token pair. 
The attention matrix at every layer is effectively a result of applying non-linear neural network operations on the attention matrix of its previous layer.
Intuitively, the attention matrix of a deeper layer captures a more complex understanding of the tokens under consideration. 


The prefill phase is known to be compute-intensive. 
% For an input of $\NumTokens$ tokens, 
The computation overhead of the attention module %computing the attention matrices 
grows quadratically with the number of input tokens.
Though the complexity could be reduced to log-linear 
% $O(\NumTokens\textrm{log}\NumTokens)$ 
(\eg~\cite{luo2021stable, kitaev2020reformer}), such reduction often degrades the generation quality, and the overhead is still superlinear.
After the prefill phase, 
% Once the attention matrices are obtained, 
the delay to generate tokens is proportional to the number of generated tokens.
Thus, the prefill phase determines when the user sees the first token, and if the answer is relatively shorter than the input context and prompt (\eg question-answering), the prefill phase can dominate the overall delay.
% is almost constant on GPU and 
% is quite marginal and can be reduced to almost constant on GPUs.



\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples_short.pdf}
    \tightcaption{LLMs increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
    \label{fig:motivate_query_examples}
\end{figure}


\tightsubsection{Long contexts in LLM applications}
\label{subsec:apps}

The input {\em prompt} to language models was traditionally short, so the inference is solely based on the knowledge embedded in the model itself, causing low quality or hallucination when the response requires new knowledge. 
% Since the prompt contains limited information, the LLM generates the response based solely on the knowledge already embedded in the LLM itself. 
As LLMs are used in more complex tasks, relying on the knowledge embedded in the LLM is no longer sufficient.
Instead, LLM applications often append additional texts, referred to as the 
{\bf context}, to supplement the prompt input to an LLM.
% \footnote{Since these contexts are often automatically added, users do not notice or need to manually type them.}.
To make our discussion more concrete, we highlight two types of applications, retrieval-based apps and chat apps, where long contexts are often used to supplement their LLM input.%, which often add long context to supplement their LLM input.


{\em Retrieval-based apps (Figure~\ref{fig:motivate_query_examples}b)} 
use LLMs to answer queries that require domain-specific knowledge.
Examples include question-answering (QA)~\cite{rubin2023long, retro, fid}, understanding a specific code repository~\cite{rubin2023long, lewis2020retrieval} or verifying fact based on latest documents~\cite{fid, lewis2020retrieval}. \jc{yuhan, the citation seems a bit outdated. can you replace the old ones with newer pointers? also mostly citations are papers. maybe a good idea to cite some real products or open-source apps}
% \jc{give a few examples from those retrieval-based learning papers.}
They use a background database that contains a large number of background documents, containing a large number of tokens.
On retrieving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM. 
\edit{Note that the search procedure is done by a \textit{seperate} DNN or a vector similarity search algorithm, which is not part of the LLM.}


% \jc{yuhan, i temporarily changed all the appearances of the term "retriever" to "application", simply because it's not defined yet and i don't know what it is. if you think it's not appropriate, please define it and change the term back to retriever}
% \edit{

% % For example, given the question ``When did the first mammal appear on Earth''~\cite{metablog2023}, the application selects documents on ``Mammals'', ``History of Earth'', or ``Evolution of Mammals''. 
% % % Then, the apps concatenate the tokens from the retrieved documents and feed the concatenated contexts into the LLM. 

% \jc{this paragraph is simultaneously doing too much and too little :) 
% on one hand, it talks too much detail about the search algorithms (which can be moved to related work).
% on the other hand, it doesn't make clear that the search delay is separate from what we optimize --- the loading and processing delays of long context.}
% }

% On receiving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM.


{\em Chat apps (Figure~\ref{fig:motivate_query_examples}c)} 
have become popular with the rise of OpenAI's ChatGPT and several other similar services~\cite{google_bard, microsoft_bing}. %, \eg Google BARD, Facebook Blender, Microsoft DialoGPT.
% \jc{some names of chat apps}
%The conversational history between a user and the LLM can be seen as the ``memory''.
To obtain high quality responses, Chat app users often intentionally use long prompts to offer more background
information (i.e., context) to the LLM. For example,
in few-shot learning, users provide several long examples and their desired responses to the LLM before ask the real questions~\cite{brown2020language, few_shot_se}.
% \jc{need citations here}. 
Furthermore, to produce coherent responses over time, all or part of a user's conversation history with the LLM is often included by the chat app in the input to the LLM as the context. 
% For instance, some open-source applications use ChatGPT API to create characters in video games~\cite{KelSolaar2023} and their users 
For instance, some applications supply a series of prompts to the LLM (ChatGPT) to create a character in a video game and then interact with the character by asking questions~\cite{KelSolaar2023}.
\shan{I slightly re-organized this paragraph.}
%Other applications~\cite{??} use ChatGPT to summarize technical papers or long documents. \jc{why is this using conversation history?}

Importantly, LLM applications use {\bf increasingly long} contexts to raise the probability of including the right information needed to generate high-quality, coherent responses.
% Intuitively, longer contexts will more likely include the information needed to generate the response. 
For example, the user may ask ``Which of the following countries generated the most total energy from solar sources in 2019?''~\cite{shi2023replug}. 
It is hard for the LLM to answer the question correctly without retrieving enough background documents for the relevant countries the user is asking for.
Though it is a hypothetical example, many studies have shown that the accuracy of the generated answers increases with more retrieved documents~\cite{fid, izacard2020memory, atlas}.
\shan{The last three sentences, ``For example ... It is hard ... Though it is ...'', do not seem to belong here. They seem to belong to the ``retrieval-based apps'' paragraph?}
For instance, FiD~\cite{fid} found that the accuracy score increased from 40\% to 48\% when increasing the number of context tokens from 1K to 10K.
Retro~\cite{retro} shows that the perplexity (a proxy score of generation quality) improves significantly when increasing the number of context tokens from 6K to 24K. 
% maybe cite self-retrieval paper here~\cite{self}
%Intuitively, longer contexts can provide more information for LLM to  answer users' questions.

% \yhedit{Although the benefits of incorporating long contexts is substantial, the key bottleneck in incorporating longer context is the high-end computation resource required to train those LLMs with longer context~\cite{??}. 
% To tackle this,}
% \shan{??This newly added sentence doesn't seem to be relevant to this project. Does it?}
To take in such long contexts,
the LLM industry has been training LLMs with the capability to accept even longer input sequences with more advanced GPUs. 
For instance, Vicuna models~\cite{zheng2023judging}, GPT-4-32K~\cite{openai2023gpt4}, and MPT models~\cite{MosaicML2023Introducing} can take up to 32K tokens as input. 
Latest models like LongNet~\cite{ding2023longnet} can even take up to 1 billion tokens as input.
\yhedit{Another line of work, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and so on~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing, ??},  enables longer input sequences by activating an extra decision logic in the self-attention module.
This module allows it not to connect each pair of tokens, but only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and with this enabled, longer sequences can be taken by the LLMs.
We refer to these works as ``text-shortening'' techniques. 
}


In essence, long contexts play an increasingly important role in LLM applications for two reasons.
% - llm's superb ability to learn from text
First, modern LLMs have a superb ability to reason about new texts and potentially learn new knowledge from them. 
To exploit this ability, many works on in-context learning aim at optimizing what should the LLM input encompass to induce better responses from LLMs.
% \jc{some numbers here}
% - fine-tuning is often not feasible
Second, while LLMs are sometimes fine-tuned in specific domains, it is not always feasible.
For instance, it is unrealistic to fine-tune an LLM for each user in chat apps.
The background database may be managed separately from the LLM provider in retrieval-based apps.\shan{This sentence does not belong here.}
Due to their huge number of parameters, fine-tuning LLMs is also slow and can be very tricky to do right (\eg catastrophic forgetting, loss of reasoning ability, etc~\cite{lin2023speciality, ding2023selfagreement}
% \jc{find some citations}
).




\tightsubsection{\hspace{-0.2cm}Saving computation by KV cache}
\label{subsec:cache}

Recall that the computation overhead of the transformer (attention module) on a context grows superlinearly (quadratically) with longer contexts (\S\ref{subsec:transformer}), so longer contexts will dramatically increase the computation delay (Figure~\ref{fig:motivate_baselines}a). 

Many recent works have tackled the long contexts' {\em computation} overheads.
A common optimization, illustrated in Figure~\ref{fig:motivate_baselines}b, is to cache the intermediate outcomes of contexts, namely the key and value (KV) features, in GPU memory.
For a given text with $\NumTokens$ tokens, the KV features are two tensors, each with the shape $[\NumTokens, \NumChannels, \NumLayers]$, 
%, each of size $\NumTokens\times\NumChannels\times\NumLayers$, 
where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
For instance, with the LLaMa-7B model, there are 4096 channels and 32 layers.
%As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features can be cached by LLM applications.

When the context is used again as part of another LLM input, one can save the computation delay of processing the context by using its KV features to reconstruct the self-attention matrices of the context. 
To put it more concretely, the computation delay can be reduced by about 15-30$\times$ for the Llama-7B model on contexts with more than 5K tokens, assuming the KV features are already in GPU. 
% \jc{Yuhan, can you add a sentence here to highlight that compute delay can be reduced 10-20 times with a kv cache?}


Caching KV features of a context, called a {\bf KV cache},\footnote{We use a context's KV features and its KV cache interchangeably.} can be used in both chat apps and retrieval-based apps. 
In chat apps, the context is the past prompts and responses, whose KV features can be cached when the past prompts were first processed and responses were first generated~\cite{dai*2019transformerxl}. 
% , and their KV features can be cached when they are first processed (for prompts) and generated (for responses)~\cite{??,??}.
% Retrieval-based apps often preprocess each background document by the LLM to compute the self-attention matrices and cache their KV features~\cite{borzunov2023distributed, mohtashami2023landmark, miao2023specinfer, dejong2023fido}.
\yhedit{In retrieval apps, the context is the background documents that are used to support answering users' questions. 
%The KV cache for the background documents used in previous queries can be cached.
%This can help avoid the computation of self-attention matrices for future queries.
As a concrete example, LangChain~\cite{??}, which is a popular LLM inference framework, builds a retrieval-based app that allows users to ask any questions on how to write specific functionalities with it.
For example, users can ask a question ``how to use Langchain to build a vector database to search for relevant documents to answer a question?'', and corresponding pages in LangChain's documentation will be retrieved to answer it. 
% \shan{This sentence is very confusing. Is ``langchain'' an example of ``libraries''? If so, langchain builds retrieval-based apps that allow 
% users to ask questions on how to write specific functionalities with langchain??}. 
% In this case, when users submit questions, corresponding pages of the documentation\shan{what documentation?} will be retrieved to answer them. 
Thus, most of, if not all, pages in LangChain's documentation can be cached to avoid recomputation of the self-attention matrices.\yh{Ask ganesh about more examples. } 
\yh{Add enterprise apps examples?}


}


% ``The Code Library Help'' ChatGPT plugin, when users ask questions about specific libraries (\eg TensorFlow, PyTorch), the plugin will query the documentation or codebase of the libraries to answer the questions. 
% In this app, the KV cache for codebase or documentations of very popular  libraries, such as TensorFlow, PyTorch, or OpenAI, can be cached to avoid recomputing their self-attention matrices.\yh{Justify why not fine-tune the LLM? } 



% \begin{figure}
% \centering
%      \includegraphics[width=.99\linewidth]{figs/h2o_motivation.pdf}
%     \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
%     \label{fig:h2o_motivation}
% \end{figure}

% In the above scenarios, the KV cache of the context is already generated before, and needs to be loaded back into GPU memory, as shown in figure~\ref{fig:h2o_motivation}a.
% No prior work shares the same goal as ours. 
% One line of prior works~\cite{zhang2023h2o, scissorhand} reduces the GPU memory consumption of using KV cache for faster generation. 
% However, as illustrated in figure~\ref{fig:h2o_motivation}b, they assume the KV cache is freshly generated from the raw text input. 
% Then the newly generated KV cache is used by the process of generating more tokens in order to avoid the recomputation of self-attention matrices for all the previously generated tokens. 
% They try to reduce the memory usage of the KV cache so that it can fit into limited GPU memory for generating later tokens, by selecting important tokens to keep. 






%\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}
%the KV features of these highly dynamic contexts have to be obtained on the fly.

%\yh{Should we add the discussion of discussion of KV feature shrinking related work here?}


%\begin{comment}
%
%Some emerging research shrinking the tensor size of KV cache, in order to further speed up the computation or fit more contexts in GPU memory.
%For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits, and Scissorhand~\cite{??} proposed to prune less important tokens from the long context. 
%Some more recent proposals~\cite{incontext-autoencoder, gisting} modify the pre-trained LLMs or train a new autoencoder to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
%%However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 
%
%\end{comment}

%Essentially, LLM systems for long contexts assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delay and keeping the KV cache of more contexts in memory.


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}


% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

\tightsection{Hidden network delays of loading contexts}


% \shan{I suggest making this sub-section a separate section and
% name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% section is REALLY tooo long. 2. this sub-section is actually not
% a background. instead, it is an important observation made by us
% that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% make it a separate section. If it is in background, it sounds
% more like previous work's observation.}
Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
\yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance. \yh{Find another example maybe in chat apps? } 
% In chat apps, a user may resume his/her conversation with LLM a few days after the last interaction on the same topic. 
% So, the KV cache of his/her conversation history needs to be swapped out of GPU memory to save space for other active conversations~\cite{orca,shepherd,clockwork}. 
% The KV cache that is swapped out is likely to be used by a resumed conversation at a different inference server. 
% \yh{Add another example? }
In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
Specifically, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
}
\shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.} 
% \jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% \yh{Per request Bandwidth needs to be within a reasonable range  }
% \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% }
% \todo{}

% \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% \todo{More evidences on why context is not in GPU}


% In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
% One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% % and the storage server on which LLM inference runs may not have enough space to store them.
% For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
% %and storing these texts can take a space up to around 750 GB. 
% In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% % \jc{please add some evidence and citations here}
% % \yh{todo: add more citations for retrieval-based apps}

% In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
% In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% % \jc{please add some evidence and citations here}
% Moreover, a user may issue her prompts to the LLM from different locations at different points.
% As these prompts can be processed by different machines, the contexts must be remotely fetched.




%In this work, we assume that the context is stored in a different machine than the GPUs running the LLM
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}

% As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large.
% Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
% More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
%(with 32 layers and 4096 channels) can be 1.3~GB. 
%for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
%On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
This network bottleneck does not only affect one model.
As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/motivate_v8_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\tightsection{Background and Motivation}

\vspace{0.2cm}

To help understand KV cache streaming and its challenges, we start with a primer on transformers and KV cache. 

\yh{New outline below: }
\begin{itemize}
    \item Section 2.1: transformer basics (Expand the last paragraph of the current 2.1 to say that reusing the KV cache for the context can eliminate time to process the context)
    \item section 2.2: Long contexts in LLM apps 
    \begin{itemize}
        \item LLMs need long context to incorporate new information that's not learned during training so as to reduce hallucination 
        \item Retrieval-based apps answer queries requiring domain-specific knowledge. Relevant context will be retrieved on receiving a query 
        \item For retrieval-based apps, the context can be long since longer context can increase the probability of including right information to answer the question. 
        \item List an example app that is likely to reuse the context used in one query before. (\eg LangChain's ``Chat with our docs'')
        \item Chat-based apps allow users to continuously interact with LLMs (\eg asking questions, solving tasks)
        \item For chat-based apps, it may take the users several rounds to make their requirements more clear and the answer more desirable, leading to long context. 
        \item List an example app that is likely to reuse the chat history. (\eg when user resumed one conversation after some period of time)
        \item Although having many benefits, taking in long contexts makes the prefill delay long since the  delay of the self-attention module grows super-linear to the length of the input. 
      \yh{In some cases, context is long and is reused, do not overclaim}
        
    \end{itemize}
    \item Section 3 KV Cache Streaming
        \begin{itemize}
        \item Section 3.1: Hidden network delay of loading the context 
        \begin{itemize}
            \item One natural way to reuse the context is to store the KV cache and directly load them when needed, like figure 4b. Cite some apps doing so if found? 
            \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            \item This can be slow because the size of the KV cache is large. And will negate the benefit of reusing KV cache.
            \item We want to make the loading of KV cache for reusing as fast as possible. 
            \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
        \item Section 3.2: 
        \begin{itemize}
            \item To make the loading of KV cache as fast as possible, one way to do it is to encode the KV cache to make its size as small as possible, like figure 4c. 
            \item A common way of encoding data transmitted over the network is to encode it into bitstreams. Explain in our case, it would be encoding the original KV cache tensor into bitstreams on the storage server, decoding it back to tensor of original shape on the inference server 
            \item Ideally, the encoder can make the loading delay of KV cache very small  to maximize the benefit of reusing KV cache 
            \item KV cache streaming can also be applied to other scenarios, such as reducing the delay of migrating KV cache in distributed inference setting 
        \end{itemize}
            % \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            % \item This will negate the benefit of reusing KV cache. 
            % \item We want to make the loading of KV cache for reusing as fast as possible. 
            % \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
\end{itemize}

\jc{the outline looks great. thanks! several comments
\begin{itemize}
    \item Right now, 2.2 only says why context can be long, which is not enough. It should explain why contexts can sometimes be long {\bf and} will be reused over time and by different requests. Both are necessary requirements.
    \item Let's drop 2.3, and add a short paragraph (or maybe just expand on an existing one) on the background of kv cache.
    \item I actually think section 3 should go straight to the problem of kv cache streaming. So it will have two subsections. 
    \begin{itemize}
        \item 3.1 (hidden delay of loading context) starts by saying a natural approach to long and reused contexts is by storing the KV cache and loading them when reused. If there's existing system that does this, we can cite them here. The remaining of 3.1 can follow your outline.
        \item 3.2 introduces the goal of kv cache streaming and why it can improve (using fig 4) reusing KV cache of long context. We can also bring up other uses of KV cache streaming (distributed kv cache).  
    \end{itemize}
\end{itemize}
}

\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/kvcache-illustrated.pdf}
    \tightcaption{An illustration of the KV cache.} 
    \label{fig:kvcache-illustrated}
\end{figure}

% \begin{figure*}
% \centering
%      \includegraphics[width=.99\linewidth]{figs/motivate_query_examples.pdf}
%     \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
%     \label{fig:motivate_query_examples}
% \end{figure*}

\tightsubsection{Transformer basics}
\label{subsec:transformer}


% {\bf Transformer} models have revolutionized the field of natural language processing (NLP), becoming the de-facto architecture for most NLP tasks~\cite{vaswani2023attention, openai2023gpt4, palm, brown2020language, kasneci2023chatgpt, retro, zhai2022scaling}.
Transformers~\cite{??,??,??} have become the de facto model for most generative services, including natural language generation, code generation (\eg~\cite{??}), and more~\cite{??}. 
% Today, most generative natural language processing (NLP) services are based on transformer models, such as GPT~\cite{??}, Bard~\cite{??}, Llama~\cite{touvron2023llama}, T5~\cite{raffel2023exploring}, PaLM~\cite{palm}, OPT~\cite{zhang2022opt}, and BLOOM. 
%For these reasons, we focus on transformer-based LLMs in this work.
%Here, we provide a general introduction to transformer architecture. 
%We intent to keep the descriptions at a high level, so they can be applied to a variety of transformer models and cover enough background for system operators to understand the the performance implication of transformer. 
%Readers can refer to \fillme for a more involved introduction.
At a high level, most transformers take a sequence of tokenized words as input and generate a sequence of tokens as the output response.\footnote{A ``token'' is the input unit used by transformer inference. It can be a punctuation, a word, or a part of a word. 
The delay of tokenizing an input prompt is typically negligible compared to the generation process, so we assume that tokens are the input to the transformer.}
% splitting words into characters. Tokenizing input is typically fast. We will use ``tokens'' in the rest of the paper. }. 
% \jc{we probably need a footnote here to clarify the difference between tokens and words and say we either use them interchangeably or stick to one of them.}
%Following the convention, we call the input the {\em prompt} and the output the {\em response}. 
The generation process has two phases.
In the prefill phase, the attention module processes the input tokens to obtain encoded features called KV cache (explained shortly).
% \jc{1-2 sentences here on how it encodes the input tokens with self-attention}
In the generation phase, the KV cache of the input is used to generate new tokens in an autoregressive manner. 
% Specifically, the input tokens and previously generated tokens are fed into the transformer model to generate the next token.  
% \jc{1-2 sentences here on how each new token is generated in an autoregressive way}

% The key in the prefill phase is
% %a neural network (NN) called 
% the attention module. 
The attention module contains multiple layers, each producing one layer in the key (K) vector and value (V) vector in the KV cache (Figure~\ref{fig:kvcache-illustrated}).
The KV vectors at each layer can produce an attention matrix, which models the connections between each token pair. 
The attention matrix at every layer is effectively a result of applying non-linear neural network operations on the attention matrix of its previous layer.
Intuitively, the attention matrix of a deeper layer captures a more complex understanding of the tokens under consideration. 


The prefill phase is known to be compute-intensive. 
% For an input of $\NumTokens$ tokens, 
The computation overhead of the attention module %computing the attention matrices 
grows quadratically with the number of input tokens.
Though the complexity could be reduced to log-linear 
% $O(\NumTokens\textrm{log}\NumTokens)$ 
(\eg~\cite{luo2021stable, kitaev2020reformer}), such reduction often degrades the generation quality, and the overhead is still superlinear.
After the prefill phase, 
% Once the attention matrices are obtained, 
the delay to generate tokens is proportional to the number of generated tokens.
Thus, the prefill phase determines when the user sees the first token, and if the answer is relatively shorter than the input context and prompt (\eg question-answering), the prefill phase can dominate the overall delay.
% is almost constant on GPU and 
% is quite marginal and can be reduced to almost constant on GPUs.



\begin{figure}
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_query_examples_short.pdf}
    \tightcaption{LLMs increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
    \label{fig:motivate_query_examples}
\end{figure}


\tightsubsection{Long contexts in LLM applications}
\label{subsec:apps}

The input {\em prompt} to language models was traditionally short, so the inference is solely based on the knowledge embedded in the model itself, causing low quality or hallucination when the response requires new knowledge. 
% Since the prompt contains limited information, the LLM generates the response based solely on the knowledge already embedded in the LLM itself. 
As LLMs are used in more complex tasks, relying on the knowledge embedded in the LLM is no longer sufficient.
Instead, LLM applications often append additional texts, referred to as the 
{\bf context}, to supplement the prompt input to an LLM.
% \footnote{Since these contexts are often automatically added, users do not notice or need to manually type them.}.
To make our discussion more concrete, we highlight two types of applications, retrieval-based apps and chat apps, where long contexts are often used to supplement their LLM input.%, which often add long context to supplement their LLM input.


{\em Retrieval-based apps (Figure~\ref{fig:motivate_query_examples}b)} 
use LLMs to answer queries that require domain-specific knowledge.
Examples include question-answering (QA)~\cite{rubin2023long, retro, fid}, understanding a specific code repository~\cite{rubin2023long, lewis2020retrieval} or verifying fact based on latest documents~\cite{fid, lewis2020retrieval}. \jc{yuhan, the citation seems a bit outdated. can you replace the old ones with newer pointers? also mostly citations are papers. maybe a good idea to cite some real products or open-source apps}
% \jc{give a few examples from those retrieval-based learning papers.}
They use a background database that contains a large number of background documents, containing a large number of tokens.
On retrieving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM. 
\edit{Note that the search procedure is done by a \textit{seperate} DNN or a vector similarity search algorithm, which is not part of the LLM.}


% \jc{yuhan, i temporarily changed all the appearances of the term "retriever" to "application", simply because it's not defined yet and i don't know what it is. if you think it's not appropriate, please define it and change the term back to retriever}
% \edit{

% % For example, given the question ``When did the first mammal appear on Earth''~\cite{metablog2023}, the application selects documents on ``Mammals'', ``History of Earth'', or ``Evolution of Mammals''. 
% % % Then, the apps concatenate the tokens from the retrieved documents and feed the concatenated contexts into the LLM. 

% \jc{this paragraph is simultaneously doing too much and too little :) 
% on one hand, it talks too much detail about the search algorithms (which can be moved to related work).
% on the other hand, it doesn't make clear that the search delay is separate from what we optimize --- the loading and processing delays of long context.}
% }

% On receiving a question, they use embedding-based search algorithms (\eg~DPR\cite{izacard2020memory,fid}, BM25~\cite{fid, ram2023incontext}) to quickly identify a subset of background documents from the database, prepend these documents to the prompt, and feed them together as input to the LLM.


{\em Chat apps (Figure~\ref{fig:motivate_query_examples}c)} 
have become popular with the rise of OpenAI's ChatGPT and several other similar services~\cite{google_bard, microsoft_bing}. %, \eg Google BARD, Facebook Blender, Microsoft DialoGPT.
% \jc{some names of chat apps}
%The conversational history between a user and the LLM can be seen as the ``memory''.
To obtain high quality responses, Chat app users often intentionally use long prompts to offer more background
information (i.e., context) to the LLM. For example,
in few-shot learning, users provide several long examples and their desired responses to the LLM before ask the real questions~\cite{brown2020language, few_shot_se}.
% \jc{need citations here}. 
Furthermore, to produce coherent responses over time, all or part of a user's conversation history with the LLM is often included by the chat app in the input to the LLM as the context. 
% For instance, some open-source applications use ChatGPT API to create characters in video games~\cite{KelSolaar2023} and their users 
For instance, some applications supply a series of prompts to the LLM (ChatGPT) to create a character in a video game and then interact with the character by asking questions~\cite{KelSolaar2023}.
\shan{I slightly re-organized this paragraph.}
%Other applications~\cite{??} use ChatGPT to summarize technical papers or long documents. \jc{why is this using conversation history?}

Importantly, LLM applications use {\bf increasingly long} contexts to raise the probability of including the right information needed to generate high-quality, coherent responses.
% Intuitively, longer contexts will more likely include the information needed to generate the response. 
For example, the user may ask ``Which of the following countries generated the most total energy from solar sources in 2019?''~\cite{shi2023replug}. 
It is hard for the LLM to answer the question correctly without retrieving enough background documents for the relevant countries the user is asking for.
Though it is a hypothetical example, many studies have shown that the accuracy of the generated answers increases with more retrieved documents~\cite{fid, izacard2020memory, atlas}.
\shan{The last three sentences, ``For example ... It is hard ... Though it is ...'', do not seem to belong here. They seem to belong to the ``retrieval-based apps'' paragraph?}
For instance, FiD~\cite{fid} found that the accuracy score increased from 40\% to 48\% when increasing the number of context tokens from 1K to 10K.
Retro~\cite{retro} shows that the perplexity (a proxy score of generation quality) improves significantly when increasing the number of context tokens from 6K to 24K. 
% maybe cite self-retrieval paper here~\cite{self}
%Intuitively, longer contexts can provide more information for LLM to  answer users' questions.

% \yhedit{Although the benefits of incorporating long contexts is substantial, the key bottleneck in incorporating longer context is the high-end computation resource required to train those LLMs with longer context~\cite{??}. 
% To tackle this,}
% \shan{??This newly added sentence doesn't seem to be relevant to this project. Does it?}
To take in such long contexts,
the LLM industry has been training LLMs with the capability to accept even longer input sequences with more advanced GPUs. 
For instance, Vicuna models~\cite{zheng2023judging}, GPT-4-32K~\cite{openai2023gpt4}, and MPT models~\cite{MosaicML2023Introducing} can take up to 32K tokens as input. 
Latest models like LongNet~\cite{ding2023longnet} can even take up to 1 billion tokens as input.
\yhedit{Another line of work, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and so on~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing, ??},  enables longer input sequences by activating an extra decision logic in the self-attention module.
This module allows it not to connect each pair of tokens, but only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and with this enabled, longer sequences can be taken by the LLMs.
We refer to these works as ``text-shortening'' techniques. 
}


In essence, long contexts play an increasingly important role in LLM applications for two reasons.
% - llm's superb ability to learn from text
First, modern LLMs have a superb ability to reason about new texts and potentially learn new knowledge from them. 
To exploit this ability, many works on in-context learning aim at optimizing what should the LLM input encompass to induce better responses from LLMs.
% \jc{some numbers here}
% - fine-tuning is often not feasible
Second, while LLMs are sometimes fine-tuned in specific domains, it is not always feasible.
For instance, it is unrealistic to fine-tune an LLM for each user in chat apps.
The background database may be managed separately from the LLM provider in retrieval-based apps.\shan{This sentence does not belong here.}
Due to their huge number of parameters, fine-tuning LLMs is also slow and can be very tricky to do right (\eg catastrophic forgetting, loss of reasoning ability, etc~\cite{lin2023speciality, ding2023selfagreement}
% \jc{find some citations}
).




\tightsubsection{\hspace{-0.2cm}Saving computation by KV cache}
\label{subsec:cache}

Recall that the computation overhead of the transformer (attention module) on a context grows superlinearly (quadratically) with longer contexts (\S\ref{subsec:transformer}), so longer contexts will dramatically increase the computation delay (Figure~\ref{fig:motivate_baselines}a). 

Many recent works have tackled the long contexts' {\em computation} overheads.
A common optimization, illustrated in Figure~\ref{fig:motivate_baselines}b, is to cache the intermediate outcomes of contexts, namely the key and value (KV) features, in GPU memory.
For a given text with $\NumTokens$ tokens, the KV features are two tensors, each with the shape $[\NumTokens, \NumChannels, \NumLayers]$, 
%, each of size $\NumTokens\times\NumChannels\times\NumLayers$, 
where $\NumChannels$ is the number of channels and $\NumLayers$ is the number of layers. 
For instance, with the LLaMa-7B model, there are 4096 channels and 32 layers.
%As the intermediate result of LLM's self-attention computation on a given text, the key and value (KV) features can be cached by LLM applications.

When the context is used again as part of another LLM input, one can save the computation delay of processing the context by using its KV features to reconstruct the self-attention matrices of the context. 
To put it more concretely, the computation delay can be reduced by about 15-30$\times$ for the Llama-7B model on contexts with more than 5K tokens, assuming the KV features are already in GPU. 
% \jc{Yuhan, can you add a sentence here to highlight that compute delay can be reduced 10-20 times with a kv cache?}


Caching KV features of a context, called a {\bf KV cache},\footnote{We use a context's KV features and its KV cache interchangeably.} can be used in both chat apps and retrieval-based apps. 
In chat apps, the context is the past prompts and responses, whose KV features can be cached when the past prompts were first processed and responses were first generated~\cite{dai*2019transformerxl}. 
% , and their KV features can be cached when they are first processed (for prompts) and generated (for responses)~\cite{??,??}.
% Retrieval-based apps often preprocess each background document by the LLM to compute the self-attention matrices and cache their KV features~\cite{borzunov2023distributed, mohtashami2023landmark, miao2023specinfer, dejong2023fido}.
\yhedit{In retrieval apps, the context is the background documents that are used to support answering users' questions. 
%The KV cache for the background documents used in previous queries can be cached.
%This can help avoid the computation of self-attention matrices for future queries.
As a concrete example, LangChain~\cite{??}, which is a popular LLM inference framework, builds a retrieval-based app that allows users to ask any questions on how to write specific functionalities with it.
For example, users can ask a question ``how to use Langchain to build a vector database to search for relevant documents to answer a question?'', and corresponding pages in LangChain's documentation will be retrieved to answer it. 
% \shan{This sentence is very confusing. Is ``langchain'' an example of ``libraries''? If so, langchain builds retrieval-based apps that allow 
% users to ask questions on how to write specific functionalities with langchain??}. 
% In this case, when users submit questions, corresponding pages of the documentation\shan{what documentation?} will be retrieved to answer them. 
Thus, most of, if not all, pages in LangChain's documentation can be cached to avoid recomputation of the self-attention matrices.\yh{Ask ganesh about more examples. } 
\yh{Add enterprise apps examples?}


}


% ``The Code Library Help'' ChatGPT plugin, when users ask questions about specific libraries (\eg TensorFlow, PyTorch), the plugin will query the documentation or codebase of the libraries to answer the questions. 
% In this app, the KV cache for codebase or documentations of very popular  libraries, such as TensorFlow, PyTorch, or OpenAI, can be cached to avoid recomputing their self-attention matrices.\yh{Justify why not fine-tune the LLM? } 



% \begin{figure}
% \centering
%      \includegraphics[width=.99\linewidth]{figs/h2o_motivation.pdf}
%     \tightcaption{LLMs used to take short inputs but increasingly take longer inputs augmented with long contexts, \eg background texts and conversation histories.} 
%     \label{fig:h2o_motivation}
% \end{figure}

% In the above scenarios, the KV cache of the context is already generated before, and needs to be loaded back into GPU memory, as shown in figure~\ref{fig:h2o_motivation}a.
% No prior work shares the same goal as ours. 
% One line of prior works~\cite{zhang2023h2o, scissorhand} reduces the GPU memory consumption of using KV cache for faster generation. 
% However, as illustrated in figure~\ref{fig:h2o_motivation}b, they assume the KV cache is freshly generated from the raw text input. 
% Then the newly generated KV cache is used by the process of generating more tokens in order to avoid the recomputation of self-attention matrices for all the previously generated tokens. 
% They try to reduce the memory usage of the KV cache so that it can fit into limited GPU memory for generating later tokens, by selecting important tokens to keep. 






%\jc{explain why KV can be computed for conversation history and for knowledge base. cite some papers.}
%the KV features of these highly dynamic contexts have to be obtained on the fly.

%\yh{Should we add the discussion of discussion of KV feature shrinking related work here?}


%\begin{comment}
%
%Some emerging research shrinking the tensor size of KV cache, in order to further speed up the computation or fit more contexts in GPU memory.
%For instance, FlexGen~\cite{??} proposed to quantize the KV features from \fillme bits to \fillme bits, and Scissorhand~\cite{??} proposed to prune less important tokens from the long context. 
%Some more recent proposals~\cite{incontext-autoencoder, gisting} modify the pre-trained LLMs or train a new autoencoder to rewrite the context with fewer tokens, in the hope that the new tokens contain the same amount of information. 
%%However, they must either modify the pre-trained LLM or train a new special model for context rewriting. 
%
%\end{comment}

%Essentially, LLM systems for long contexts assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delay and keeping the KV cache of more contexts in memory.


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}


% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

\tightsection{Hidden network delays of loading contexts}


% \shan{I suggest making this sub-section a separate section and
% name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% section is REALLY tooo long. 2. this sub-section is actually not
% a background. instead, it is an important observation made by us
% that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% make it a separate section. If it is in background, it sounds
% more like previous work's observation.}
Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
\yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance. \yh{Find another example maybe in chat apps? } 
% In chat apps, a user may resume his/her conversation with LLM a few days after the last interaction on the same topic. 
% So, the KV cache of his/her conversation history needs to be swapped out of GPU memory to save space for other active conversations~\cite{orca,shepherd,clockwork}. 
% The KV cache that is swapped out is likely to be used by a resumed conversation at a different inference server. 
% \yh{Add another example? }
In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
Specifically, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
}
\shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.} 
% \jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% \yh{Per request Bandwidth needs to be within a reasonable range  }
% \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% }
% \todo{}

% \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% \todo{More evidences on why context is not in GPU}


% In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
% One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% % and the storage server on which LLM inference runs may not have enough space to store them.
% For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
% %and storing these texts can take a space up to around 750 GB. 
% In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% % \jc{please add some evidence and citations here}
% % \yh{todo: add more citations for retrieval-based apps}

% In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
% In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% % \jc{please add some evidence and citations here}
% Moreover, a user may issue her prompts to the LLM from different locations at different points.
% As these prompts can be processed by different machines, the contexts must be remotely fetched.




%In this work, we assume that the context is stored in a different machine than the GPUs running the LLM
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}

% As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large.
% Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
% More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
%(with 32 layers and 4096 channels) can be 1.3~GB. 
%for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
%On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
This network bottleneck does not only affect one model.
As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/outline-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Background and Motivation}

\subsection{Transformer basics}

\begin{itemize}
\item transformer is the de-factor llm arch, so we focus on it
\item transformer basics
    \begin{itemize}
    \item input vs. output
    \item processing phase (encoding?)
    \item generation phase (decoding?)
    \end{itemize}
\end{itemize}


\subsection{Context in LLM applications}

\begin{itemize}
\item context in apps
    \begin{itemize}
    \item traditionally, prompt doesn't have context
    \item retrieval apps. examples
    \item chat apps. examples
    \end{itemize}
\item why is context useful
    \begin{itemize}
    \item llm doesnt have all knowledge, and can't keep states
    \item new knowledge embed in context
    \item long context learning
    \item few-shot learning
    \item retrieval-based learning
    \end{itemize}
\item why is context getting longer?
    \begin{itemize}
    \item more knowledge can be embedded
    \item evidence: \# of matches vs. context length
    \item evidence: chat apps have longer conversational histories
    \item recent llms are capable of processing extremely long context
    \end{itemize}
\item why is context dynamically loaded?
    \begin{itemize}
    \item chat app: user move in time and space
    \item retrieval: database in a separate place
    \end{itemize}
\end{itemize}


\subsection{Limitations of prior approaches}
\begin{itemize}
\item why not feeding context directly? 
    \begin{itemize}
    \item quadratic processing time
    \item mention feeding token embeddings
    \end{itemize}
\item kv cache: 
    \begin{itemize}
    \item what is kv? => benefit
    \item why caching kv doesn't change llm results? prefix vs otherwise
    \item chat app: user move in time and space
    \item retrieval: database in a separate place
    \end{itemize}
\item but kv cache has a large size
    \begin{itemize}
    \item concrete numbers: size of kv cache per token vs token size
    \end{itemize}
\item emerging research: kv quantization, token selection, gisting.
    \begin{itemize}
    \item kv quantization (flexgen) 
    \item token selection (scissorhand) 
    \item why not? quality drop. both flexgen and scissorhand drop part of tensor
    \item gisting + autoencoder: smarter way of rewriting context
    \item why not? require change of the model or rewriting prompt or prompt-specific tuning
    \item doesn't have control over ttft
    \item no coding
%    \item they reduce the gpu memory footprint, but there can be much redundancy. use the video coding analogy
%    \item they do not optimize the loading part
%    \item most require change of the model or rewriting prompt or prompt-specific tuning
    \end{itemize}
%\item most work to deal with long context still yield large kv cache size
%    \begin{itemize}
%    \item many efforts try to reduce memory usage for long context
%    \end{itemize}
\end{itemize}

\subsection{Metrics and objectives}
\begin{itemize}
\item delay metric
\item quality metric
\item objective
\end{itemize}



\section{Design}

\subsection{Overview}
\begin{itemize}
\item compression: compress kv cache to short bitstream
\item kv loader: speedup the decompression, loading to GPU, and attention computation
\item controller: for a given delay budget, pick text vs kv \& pick the right compression level
\end{itemize}

\subsection{Compression}
\begin{itemize}
\item workflow: calculate delta among tokens + pick quantization + entropy coding
\item cross-token locality
    \begin{itemize}
    \item explain what cross-token locality means
    \item examples (figure)
    \item intuitive explanation of why such locality exists
    \item how we use the insight
    \end{itemize}
\item choose quantization level
    \begin{itemize}
    \item explain what quantization is
    \item insight: examples of different layers have different sensitivity
    \item how to use the insight
    \end{itemize}
\item arithmetic coding
    \begin{itemize}
    \item explain what ac is
    \item insight: different layers and channels have different distributions
    \item how to use the insight
    \end{itemize}
\item highlight key difference with other kv or context compressors
    \begin{itemize}
    \item optimize the bitstream size. why is it better?
    \item no change of model or prompt
    \item can be combined with other compressors
    \end{itemize}
\end{itemize}



% \subsection{KV Loader}
% \begin{itemize}
% \item reiterate the goal
% \item naive solution: 
%     \begin{itemize}
%     \item load the whole kv cache and then compute
%     \item compute includes decompression, loading and inference.  
%     \end{itemize}
% \item idea: pipelining loading and compute
%     \begin{itemize}
%     \item use an example to explain it
%     \item do everything in gpu?
%     \end{itemize}
% \end{itemize}

\subsection{Controller}
\begin{itemize}
\item reiterate goal: given a delay budget, pick what config?
\item explain (with numbers) why loading short context is faster
\item show the tradeoff curves of different compression configs
\item how are the configs picked?
\end{itemize}



==> backups/outline-v2_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\section{Background and Motivation}

\subsection{Transformer basics}

\begin{itemize}
\item transformer is the de-factor llm arch, so we focus on it
\item transformer basics
    \begin{itemize}
    \item input vs. output
    \item processing phase (encoding?)
    \item generation phase (decoding?)
    \end{itemize}
\end{itemize}


\subsection{Context in LLM applications}

\begin{itemize}
\item context in apps
    \begin{itemize}
    \item traditionally, prompt doesn't have context
    \item retrieval apps. examples
    \item chat apps. examples
    \end{itemize}
\item why is context useful
    \begin{itemize}
    \item llm doesnt have all knowledge, and can't keep states
    \item new knowledge embed in context
    \item long context learning
    \item few-shot learning
    \item retrieval-based learning
    \end{itemize}
\item why is context getting longer?
    \begin{itemize}
    \item more knowledge can be embedded
    \item evidence: \# of matches vs. context length
    \item evidence: chat apps have longer conversational histories
    \item recent llms are capable of processing extremely long context
    \end{itemize}
\item why is context dynamically loaded?
    \begin{itemize}
    \item chat app: user move in time and space
    \item retrieval: database in a separate place
    \end{itemize}
\end{itemize}


\subsection{Limitations of prior approaches}
\begin{itemize}
\item why not feeding context directly? 
    \begin{itemize}
    \item quadratic processing time
    \item mention feeding token embeddings
    \end{itemize}
\item kv cache: 
    \begin{itemize}
    \item what is kv? => benefit
    \item why caching kv doesn't change llm results? prefix vs otherwise
    \item chat app: user move in time and space
    \item retrieval: database in a separate place
    \end{itemize}
\item but kv cache has a large size
    \begin{itemize}
    \item concrete numbers: size of kv cache per token vs token size
    \end{itemize}
\item emerging research: kv quantization, token selection, gisting.
    \begin{itemize}
    \item kv quantization (flexgen) 
    \item token selection (scissorhand) 
    \item why not? quality drop. both flexgen and scissorhand drop part of tensor
    \item gisting + autoencoder: smarter way of rewriting context
    \item why not? require change of the model or rewriting prompt or prompt-specific tuning
    \item doesn't have control over ttft
    \item no coding
%    \item they reduce the gpu memory footprint, but there can be much redundancy. use the video coding analogy
%    \item they do not optimize the loading part
%    \item most require change of the model or rewriting prompt or prompt-specific tuning
    \end{itemize}
%\item most work to deal with long context still yield large kv cache size
%    \begin{itemize}
%    \item many efforts try to reduce memory usage for long context
%    \end{itemize}
\end{itemize}

\subsection{Metrics and objectives}
\begin{itemize}
\item delay metric
\item quality metric
\item objective
\end{itemize}



\section{Design}

\subsection{Overview}
\begin{itemize}
\item compression: compress kv cache to short bitstream
\item kv loader: speedup the decompression, loading to GPU, and attention computation
\item controller: for a given delay budget, pick text vs kv \& pick the right compression level
\end{itemize}

\subsection{Compression}
\begin{itemize}
\item workflow: calculate delta among tokens + pick quantization + entropy coding
\item cross-token locality
    \begin{itemize}
    \item explain what cross-token locality means
    \item examples (figure)
    \item intuitive explanation of why such locality exists
    \item how we use the insight
    \end{itemize}
\item choose quantization level
    \begin{itemize}
    \item explain what quantization is
    \item insight: examples of different layers have different sensitivity
    \item how to use the insight
    \end{itemize}
\item arithmetic coding
    \begin{itemize}
    \item explain what ac is
    \item insight: different layers and channels have different distributions
    \item how to use the insight
    \end{itemize}
\item highlight key difference with other kv or context compressors
    \begin{itemize}
    \item optimize the bitstream size. why is it better?
    \item no change of model or prompt
    \item can be combined with other compressors
    \end{itemize}
\end{itemize}



% \subsection{KV Loader}
% \begin{itemize}
% \item reiterate the goal
% \item naive solution: 
%     \begin{itemize}
%     \item load the whole kv cache and then compute
%     \item compute includes decompression, loading and inference.  
%     \end{itemize}
% \item idea: pipelining loading and compute
%     \begin{itemize}
%     \item use an example to explain it
%     \item do everything in gpu?
%     \end{itemize}
% \end{itemize}

\subsection{Controller}
\begin{itemize}
\item reiterate goal: given a delay budget, pick what config?
\item explain (with numbers) why loading short context is faster
\item show the tradeoff curves of different compression configs
\item how are the configs picked?
\end{itemize}



==> backups/outline.tex <==


\section{Introduction}
\begin{outline}
\1 generative ai has seen an inflection point in popularity
  \2 bunch of citations
\1 not just more users, but a richer set of ways to interact with LLMs
  \2 traditional: a few interactions in a short time span
  \2 today: many interactions over several days or months and augmented with external knowledge
  \2 this means a lot of ``history'' tokens need to be processed before generating anything
\1 delay grows quickly with length of relevant information
  \2 briefly explain it using the transformer arch 
\1 existing work: caching key values
  \2 explain why key-value embedding could be cached without affecting correctness
\1 however, current work works poorly when the kv cache is not readily in gpu memory
  \2 reasons why they may not in gpu memory: (1) dormant sessions, and (2) large augmented database \yh{check gpu preemption papers on llm}
\1 our contributions:
  \2 a systematic measurement study to motivate the need for a compression scheme for kv cache
  \2 propose a kv compression system to reduce the communication and loading delay (driven by novel measurement insights)
\end{outline}


\section{Background}
\begin{outline}
\1 transformer arch
  \2 encoder arch
  \2 decoder arch
  \2 key, value embedding
\1 why caching k-v embeddings?
  \2 reduce delay to generate each token
  \2 delay reduction in conversational apps
  \2 delay reduction in retrieval-based apps   
  \yh{Need to discuss why cache kv embeds not attn matrices? }

\end{outline}

\section{Motivation}
\begin{outline}
\1 kv cache need to dynamically loaded
  \2 indeed, the kv cache can be in memory when it always fits, but
  \2 reason 1: when there are many concurrent sessions and one session is dormant for a long time, the history must be removed from gpu memory
  \2 reason 2: when the retrieval database is large, it must be put at a separate location.
\1 loading the raw embeddings can be slow
  \2 explain the system workflow we have in mind
\1 first, we show how much delay reduction can be realized, IF the kv is in gpu memory
  \2 dataset (prompts, etc)
  \2 delay reduction vs. workloads
  \2 delay reduction vs. history length
  \2 delay reduction vs. models
\1 what if kv is NOT in gpu memory?
  \2 revisit the benefits, most of which will be negated
\end{outline}


\section{Compression system}
\begin{outline}
\1 problem formulation: achieve high accuracy/perplexity while storing \& transferring less data
\1 design space
  \2 framework: (kv) => pick quantization => pick ac granularity => (q) => pick embeddings to transfer => decompress
  \2 three design decisions: 
    (1) how to pick quantization, 
    (2) how to pick AC granularity, and 
    (3) which token's key values to transfer
\1 pick quantization
  \2 insight a: diff layers have diff impact
  \2 insight b: diff layers have diff skewness
  \2 different quantization for diff layer
\1 pick ac granularity
  \2 insight c: nearby layers share the sim distrib
  \2 insight d: nearby tokens share the sim distrib
  \2 use same z for a group of layer-token combos
\1 pick embedding
  \2 insight e: not all tokens are relevant to the query
  \2 use cross-product to identify only relevant embeddings to transfer
\1 how to adapt to delay budget
  \2 so far, we have a curve between perplexity and size
  \2 given a delay budget, pick the best parameter
\end{outline}


\section{Evaluation}
\begin{outline}
\1 setup:
  \2 metrics: perplexity, storage size, transfer size
  \2 datasets
  \2 baselines: no caching, no compression, gzip, torch obj, quantization
\1 end-to-end: perplexity \& accuracy vs. storage size \& transfer size
\1 compute overhead and delay
\1 improvement breakdown
\end{outline}

\section{Related work}
\begin{outline}
\1 key-value caching papers: most relevant to us, but assume the key values are stored locally on gpu
\1 memory efficient LLM: reduce memory footprint, but the reduced size is still too large to load through the network/cpu bus
\1 retrieval-augmented LLM: this doesn't solve our problem, but it motivates the benefits for kv caching.
                 \1 tensor compression: including ae. our work borrows techniques from this line of work but customize it with domain-specific insights
\end{outline}

\newpage



==> backups/outline_2.tex <==


\section{Introduction}
\begin{outline}
\1 generative ai has seen an inflection point in popularity
  \2 bunch of citations
\1 not just more users, but a richer set of ways to interact with LLMs
  \2 traditional: a few interactions in a short time span
  \2 today: many interactions over several days or months and augmented with external knowledge
  \2 this means a lot of ``history'' tokens need to be processed before generating anything
\1 delay grows quickly with length of relevant information
  \2 briefly explain it using the transformer arch 
\1 existing work: caching key values
  \2 explain why key-value embedding could be cached without affecting correctness
\1 however, current work works poorly when the kv cache is not readily in gpu memory
  \2 reasons why they may not in gpu memory: (1) dormant sessions, and (2) large augmented database \yh{check gpu preemption papers on llm}
\1 our contributions:
  \2 a systematic measurement study to motivate the need for a compression scheme for kv cache
  \2 propose a kv compression system to reduce the communication and loading delay (driven by novel measurement insights)
\end{outline}


\section{Background}
\begin{outline}
\1 transformer arch
  \2 encoder arch
  \2 decoder arch
  \2 key, value embedding
\1 why caching k-v embeddings?
  \2 reduce delay to generate each token
  \2 delay reduction in conversational apps
  \2 delay reduction in retrieval-based apps   
  \yh{Need to discuss why cache kv embeds not attn matrices? }

\end{outline}

\section{Motivation}
\begin{outline}
\1 kv cache need to dynamically loaded
  \2 indeed, the kv cache can be in memory when it always fits, but
  \2 reason 1: when there are many concurrent sessions and one session is dormant for a long time, the history must be removed from gpu memory
  \2 reason 2: when the retrieval database is large, it must be put at a separate location.
\1 loading the raw embeddings can be slow
  \2 explain the system workflow we have in mind
\1 first, we show how much delay reduction can be realized, IF the kv is in gpu memory
  \2 dataset (prompts, etc)
  \2 delay reduction vs. workloads
  \2 delay reduction vs. history length
  \2 delay reduction vs. models
\1 what if kv is NOT in gpu memory?
  \2 revisit the benefits, most of which will be negated
\end{outline}


\section{Compression system}
\begin{outline}
\1 problem formulation: achieve high accuracy/perplexity while storing \& transferring less data
\1 design space
  \2 framework: (kv) => pick quantization => pick ac granularity => (q) => pick embeddings to transfer => decompress
  \2 three design decisions: 
    (1) how to pick quantization, 
    (2) how to pick AC granularity, and 
    (3) which token's key values to transfer
\1 pick quantization
  \2 insight a: diff layers have diff impact
  \2 insight b: diff layers have diff skewness
  \2 different quantization for diff layer
\1 pick ac granularity
  \2 insight c: nearby layers share the sim distrib
  \2 insight d: nearby tokens share the sim distrib
  \2 use same z for a group of layer-token combos
\1 pick embedding
  \2 insight e: not all tokens are relevant to the query
  \2 use cross-product to identify only relevant embeddings to transfer
\1 how to adapt to delay budget
  \2 so far, we have a curve between perplexity and size
  \2 given a delay budget, pick the best parameter
\end{outline}


\section{Evaluation}
\begin{outline}
\1 setup:
  \2 metrics: perplexity, storage size, transfer size
  \2 datasets
  \2 baselines: no caching, no compression, gzip, torch obj, quantization
\1 end-to-end: perplexity \& accuracy vs. storage size \& transfer size
\1 compute overhead and delay
\1 improvement breakdown
\end{outline}

\section{Related work}
\begin{outline}
\1 key-value caching papers: most relevant to us, but assume the key values are stored locally on gpu
\1 memory efficient LLM: reduce memory footprint, but the reduced size is still too large to load through the network/cpu bus
\1 retrieval-augmented LLM: this doesn't solve our problem, but it motivates the benefits for kv caching.
                 \1 tensor compression: including ae. our work borrows techniques from this line of work but customize it with domain-specific insights
\end{outline}

\newpage



==> backups/problem-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US






%\tightsection{KV Cache Streaming}

\tightsection{Hidden network delay of loading the KV cache}
\label{sec:delay}

\begin{comment}
\begin{itemize}
    \item Section 3 KV Cache Streaming
        \begin{itemize}
        \item Section 3.1: Hidden network delay of loading the context 
        \begin{itemize}
            \item One natural way to reuse the context is to store the KV cache and directly load them when needed, like Figure 4b. cite chunkattention etc. 
            \item these prior works assume the KV cache is in the GPU memory of the inference server. However  the KV cache may not necessarily lie on the same server as the inference server. Reason: the background database for retrieval apps is too large to be replicated on each inference server. For chat apps, users may resume the conversation after a long period of time, thus the KV cache will need to be swapped out. List a concrete example
            % \item For example, when users build LLM apps, they usually upload context (in text format) to the storage server, while querying LLMs hosted in a compute server. In these cases, KV cache is on a remote server than the inference one. 
            \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (Cite interdc throughput)
            \item This can be slow because the size of the KV cache is large. And will negate the benefit of reusing KV cache.
            \item We want to make the loading of KV cache for reusing as fast as possible. 
        \end{itemize}
        \item Section 3.2: 
        \begin{itemize}
            \item To make the loading of KV cache as fast as possible, one way to do it is to encode the KV cache to make its size as small as possible, like figure 4c. 
            \item A common way of encoding data transmitted over the network is to encode it into bitstreams. Explain in our case, it would be encoding the original KV cache tensor into bitstreams on the storage server, decoding it back to tensor of original shape on the inference server 
            \item Ideally, the encoder can make the loading delay of KV cache very small  to maximize the benefit of reusing KV cache 
            \item KV cache streaming can also be applied to other scenarios, such as reducing the delay of migrating KV cache in distributed inference setting 
             \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
            % \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            % \item This will negate the benefit of reusing KV cache. 
            % \item We want to make the loading of KV cache for reusing as fast as possible. 
            % \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
\end{itemize}

\end{comment}

A natural idea to skip the heavy compute of prefill is to {\em reuse the KV cache} of the context if it has been used before.
% Long contexts increase the input length and cause high prefill delay, but since the contexts are often reused, one can naturally reduce the prefill delay is by {\em reusing the KV cache} of the context. 
Indeed, recent studies (\eg~\cite{vllm, chunkattention, promptcache}) have suggested that by saving the KV cache of a context and reusing it when the same context is used again, one could eliminate the prefill delay and significantly reduce TTFT. 

\begin{comment}

one can first run the prefill phase of LLM inference on the context, save the K and V tensors in the resulting KV cache, and reuse them in the future if the same context is used again. %, thus eliminating the future prefill delay. % which grows superlinearly with the context length.
As suggested in recent studies (\eg~\cite{vllm, chunkattention, promptcache}), this method can eliminate the future prefill delay, {\em if} the KV cache is {\em already} in the GPU memory when the same context is used again.
\end{comment}

% \jc{somewhere in this section, we need to define TTFT. we don't need much text about it as before, since TTFT is widely used by industry already}

%In this way, the superlinear procedure of prefilling the context can be bypassed. 
%Indeed, several recent studies~\cite{vllm, chunkattention, promptcache} reuse KV cache that is already in GPU memory to speed-up the processing (prefill) of contexts shared across LLM inference requests. 
%These prior works assume the KV cache is stored in the GPU memory.

In practice, however, the reused KV cache of long contexts may have to be fetched from another machine(s), but this {\em network delay} in fetching the KV cache has been largely overlooked since existing LLM systems assume that the KV cache is always in GPU memory or the KV cache is small enough to be retrieved quickly via a fast GPU interconnection.
% However, the prior systems assume that either the KV cache is always in GPU memory or the KV cache is small enough to be quickly fetched via a dedicated fast interconnection.
% Unfortunately, {\em the network delay} in fetching the KV cache of long contexts can be substantial in practice.
% may {\em not} always be available in the GPU when reused.
This is because the KV cache of a context can be 3-4 orders of magnitude bigger than the context in text format, so the GPU memory may not be big enough to hold the KV caches of all contexts that might be reused.
% \jc{yuhan, please write something like this: GPU memory is typically below \fillme GB, and even if all of it is used for KV cache produced by \fillme model, we will be able to put in the KV cache of \fillme tokens, which roughly translate to \fillme pages of documents, and for KV cache produced by a \fillme (a bigger model), only the KV cache of \fillme tokens can fit in.}

Popular GPUs used for serving LLMs such as the NVidia A40 or RTX A6000 have a maximum GPU memory of 46-48 GB. A common LLM model such as LLama-33B with 8-bit quantized weights requires around 33 GB of GPU memory~\cite{anyscale_blog}. 
If we devote the entire remaining 13 GB to store the KV cache, we can store a maximum token length of around 8000 tokens. 
Standard tokenizers have a ratio of one word equalling 1.33 tokens~\cite{token_blog}, this translates to 6000 words or 6 pages of text of roughly 1000 words per page. 
Thus in general, storing the KV cache on the GPU is challenging, especially when the model size increases, we can store the KV cache of a fewer number of tokens.

Even for chat-based apps where the KV cache of one conversation can fit in the GPU memory, the KV cache may have to be offloaded before the next user query comes. 
For instance, when a user asks the LLM to generate a long story, then the KV cache of the long story (part of context) will be available in GPU memory right after the generation. 
%becomes the context of subsequent conversations.
%, and the KV cache of this context is available in GPU memory. 
However, if the next query about the story does not come until several hours or days later, the GPU may choose to offload the KV cache of this conversation, so even if the next query is routed to the {\em same} GPU, the KV cache will not be available locally and has to be loaded from another machine.

% \jc{yuhan, i deleted your old examples, such as 2T tokens, 364 million docs, etc. in generally, these examples are easy to attack and people's first reaction is we are exaggerating since not all of them are needed at once. in generally, try to avoid examples that people can easily attack.
% same logic goes to the example of azure openai storage service being separate. people can easily attack and say the kv cache doesn't have to be colocated with the text.}


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}

%in the GPU memory of the GPUs that run the LLM inference. 

\begin{comment}
In retrieval-based applications, the size of KV cache of the related background documents is too big to be replicated locally on \emph{each} GPU server that potentially runs LLM inference jobs. 
For example, one recent work uses a background database containing up to 2 trillion tokens in total, which requires 1 TB of storage to save the documents in text format. 
Similarly, another recent work uses a  database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
Thus, the developers of the LLM applications may upload their data to the cloud storage servers, and query LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may build their database and store it on Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance.
Although storing the KV cache in the storage services is not widely applied in existing LLM applications, we envision this will be a popular practice in the near future. \yh{Missing some evidence here. Maybe say that many popular LLM inference frameworks support KV cache as input? }

For chat-based applications, users may resume their conversation with the LLMs after several days. 
Accordingly, those chat histories need to be swapped out from the GPU memory to save space for other active sessions.
Whenever the chat session is resumed, the cached chat histories are highly likely to be loaded from another GPU server. 
Also, given that the number of active users for chat apps is huge (\eg 180 million active users till now for ChatGPT~\cite{vermeer_2023}), it is difficult to store all of the users' chat histories on every GPU server in the inference 
serving system.  
% \yh{Missing why KV cache is on a remote server}
\end{comment}

In these cases, the stored KV cache of the context must be fetched from another machine(s) before being reused, and this network transmission incurs a delay that could \emph{negate} the benefit in saving computation delays from reusing KV cache.
For instance, the KV cache produced by the 65-billion Llama model \ga{Stick to one version of the LLama model for the description.}
%\jc{pick a big one.}
of 5K  tokens is two tensors each of the size $5$K (tokens)$\times$8192 (channels)$\times$80 (layers), leading to a total size of 13~GB.
%\jc{4.1GB was a bit small}
With a throughput of 16~Gbps, typical to the full capacity of a inter-datacenter link~\cite{skyplane}, it will take 6.5 seconds to transmit the KV cache. \ga{inter-DC is a bit confusing.} \ga{It would help to give a breakdown of the times, for me to put the 6.5s in context.}
% To put it in perspective, this delay is similar to the prefill delay from scratch, thus almost negating the benefit of reusing KV cache.
As illustrated in Figure~\ref{fig:motivate_baselines}, transmitting the large KV cache (Figure~\ref{fig:motivate_baselines}(b)) can be almost as large as the delay of prefilling from scratch (Figure~\ref{fig:motivate_baselines}(a)),  thus almost negating the benefit of reusing KV cache.
% \jc{try to connect this discussion with fig~\ref{fig:motivate_baselines}}
Even with 100~Gbps throughput, which is typical for RDMA
% \jc{think about specialized infra like RDMA, memcachd, etc}
, transmitting the KV cache can take up to 1000ms.
If we can reduce it down by 3$\times$, it still makes a perceivable difference~\cite{llmperf}.

In summary, we want to reduce the overall delay for loading and processing a given context.
Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the
generation of the first token. We refer to it as the
\emph{time-to-first-token} (TTFT), since it measures when the first
token is available for the user. 
As shown by previous studies,
users’ experience can be heavily affected by the TTFT since it
demonstrates the responsiveness of the application.
Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
% TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. 

%via a limited bandwidth link.  



\begin{comment}
In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane, ??}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
This is because the size of KV cache is large, far larger than the context in raw text context form.
Specifically, 
for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV cache produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$5120 (channels)$\times$40 (layers), and the size of KV cache serialized by \texttt{torch.save} is 4.1~GB~\footnote{Assumed saving with 16-bit floating point numbers, which is a standard practice~\cite{??}. }.
Given a throughput of 2~Gbps, transmitting the KV cache over the bandwidth can take 16 seconds. 

In short, fetching large KV cache remotely \emph{negates} the benefit of reusing KV cache in saving computation delays. 
This network bottleneck does not only affect one model. 
As shown in Figure~\ref{fig:size_models}, the size of KV cache of popular LLMs all grows with the input token lengths. 
Thus, we want to make the loading of KV cache for reusing as fast as possible, in order to fully maximize the benefit of reusing KV cache in saving prefill delays. 

\end{comment}

\tightsection{\hspace{-0.0cm}\name: KV Cache Streaming}

%\begin{itemize}
%\item what's a kv cache streamer: encode, stream, and decode
%\item how it may help? send a kv cache much faster => faster ttft than prior work. other uses (downplay)
%\item how does it differs from other kv cache compression papers. complementary (top-off) and more compression. deals with bw changes
%\item \name is a concrete design
%\end{itemize}

The need to reduce KV cache transmission delay motivates a new module in LLM systems, which we call a {\em KV cache streamer}.
Put simply, the KV cache streamer serves three roles: 
\begin{packeditemize}
\item {\em (1) encoding} a given KV cache into more compact bitstream representations, called {\em KV bitstreams}, 
\item {\em (2) streaming} the encoded KV bitstreams through a network connection of varying throughput, and 
\item {\em (3) decoding} the received KV bitstreams to get the KV cache.
\end{packeditemize}
Though KV cache has been widely used, there has been little effort on how to encode KV cache to bitstreams efficiently, or on how to stream KV cache under dynamic network bandwidth to reduce TTFT. \ga{Put in a line on how sub-optimal the existing KV cache systems are.}
% \jc{remember to introduce TTFT in the last section}

This paper presents {\bf \name}, a concrete design of the KV cache streamer, which makes two technical contributions.
First, \name uses a custom KV cache codec (encoder and decoder) which minimize size of KV bitreams by embracing several distributional properties of the given KV cache tensors (\S\ref{??}).
Second, when streaming the KV bitstreams under dynamic bandwidth, \name dynamically switches between different compression levels or computing the KV cache on demand. %, in order to complete the transmission of KV cache under a given deadline with high quality.
In addition, the KV coding/decoding in \name incurs a negligible compute overhead and is pipelined with network transmission to minimize the impact on end-to-end delay. 

If successful, the benefit of \name as a KV cache streamer is two-fold.
First, it greatly reduces the bandwidth demand to transmit the KV cache, thus directly reducing TTFT. 
Second, it can dynamically choose the appropriate compression level (or KV compute on-demand) to ensure that TTFT is within a given deadline while maintaining a high response quality.\footnote{The KV cache streamer could also be used to share KV cache more efficiently across different machines in emerging model-parallelism systems for serving LLMs~\cite{lin2024infinitellm, agrawal2023sarathi,??}. 
%These distributed inference systems may migrate KV cache across GPUs, which can also be optimized by such a streaming system. 
}
%by dynamically choosing the compression level streaming KV cache in order to contain TTFT within a deadline, while maintaining a high response quality.

A KV cache streamer (\name) has a key distinction with the emergent techniques for compressing KV cache.
Through dropping less important tokens from context, these techniques (\eg~\cite{scissorhand,zhang2023h2o,beltagy2020longformer}) 
%and others~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing}.
\jc{yuhan, i dropped the other citations. but maybe we need to add the autoencoder paper?}
enable longer contexts or reduce GPU memory footprint. 
Thus, they optimize how to best use GPU memory to store KV cache, rather than how to transmit KV cache over the network, like \name. \ga{The difference is unclear. Lossy vs. lossless? Memory vs. network? Be clear.}
\name is complementary to these techniques and can be used to transmit any KV cache produced by these methods (see \S\ref{??} for a case study of \name with H2O~\cite{zhang2023h2o}).

%, because it can be used to stream any KV cache, including the KV cache after these methods drop the unimportant tokens.
%Moreover, it does not tackle the problem of bandwidth adaptation. 
%This line of work adds a separate module in the self-attention module, which  allows it not to connect each pair of tokens, but to select only a subset of them to approximate the effect of connecting each pair. 
%This will make the self-attention operation less compute and memory-intensive, and thus longer sequences can be taken by the LLMs.

\begin{comment}
How to reuse KV cache while minimizing the network delay?
This paper explores a {\em KV cache streaming} module and a concrete design named \name. 
The KV cache streaming module has three logical steps 

%\tightsubsection{KV cache streaming }

One way of making KV cache loading fast is to encode the KV cache and stream it via the network.   
A common way of encoding data transmitted over the network is to encode it into bitstreams. 
In the scenario of KV cache streaming, the streamer encodes the KV cache into bitstreams on the storage server, and decodes it back to the original KV cache for LLM inference, as shown in Figure~\ref{fig:motivate_baselines}c.
Ideally, with such a streamer, the transmission delay, together with the decoding delay, will be much smaller than the delay of computing the KV cache of the context from raw text context, in order to  maximize the benefit of reusing KV cache in terms of computation. 
Furthermore, the streamer should also be able to adapt to dynamic resource allocation and make optimal decisions to stream KV cache differently under resource change. 


Potentially, KV cache streaming can also be applied in other scenarios, such as in distributed inference systems~\cite{lin2024infinitellm, agrawal2023sarathi, ??}. 
These distributed inference systems may migrate KV cache across GPUs, which can also be optimized by such a streaming system. 

This goal is fundamentally different from the prior works that try to enable longer context by text shortening, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and many others~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing}. 
This line of work adds a separate module in the self-attention module, which  allows it not to connect each pair of tokens, but to select only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and thus longer sequences can be taken by the LLMs.

\end{comment}


% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

% \tightsection{Hidden network delays of loading contexts}


% % \shan{I suggest making this sub-section a separate section and
% % name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% % section is REALLY tooo long. 2. this sub-section is actually not
% % a background. instead, it is an important observation made by us
% % that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% % make it a separate section. If it is in background, it sounds
% % more like previous work's observation.}
% Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% % \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% % need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
% In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
% Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
% \yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
% To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance. \yh{Find another example maybe in chat apps? } 
% % In chat apps, a user may resume his/her conversation with LLM a few days after the last interaction on the same topic. 
% % So, the KV cache of his/her conversation history needs to be swapped out of GPU memory to save space for other active conversations~\cite{orca,shepherd,clockwork}. 
% % The KV cache that is swapped out is likely to be used by a resumed conversation at a different inference server. 
% % \yh{Add another example? }
% In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
% With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
% Specifically, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
% Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
% }
% \shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.} 
% % \jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% % \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% % \yh{Per request Bandwidth needs to be within a reasonable range  }
% % \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% % In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% % In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% % Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% % \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% % }
% % \todo{}

% % \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% % \todo{More evidences on why context is not in GPU}


% % In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
% % One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% % % and the storage server on which LLM inference runs may not have enough space to store them.
% % For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
% % %and storing these texts can take a space up to around 750 GB. 
% % In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% % Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% % % \jc{please add some evidence and citations here}
% % % \yh{todo: add more citations for retrieval-based apps}

% % In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
% % In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% % % \jc{please add some evidence and citations here}
% % Moreover, a user may issue her prompts to the LLM from different locations at different points.
% % As these prompts can be processed by different machines, the contexts must be remotely fetched.




% %In this work, we assume that the context is stored in a different machine than the GPUs running the LLM



\begin{comment}
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}
\end{comment}


% % As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large.
% % Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
% % More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% % However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% % To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% % In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
% %(with 32 layers and 4096 channels) can be 1.3~GB. 
% %for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
% %On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% % \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% % Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% % By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

% In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
% This network bottleneck does not only affect one model.
% As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/problem-v2_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US






%\tightsection{KV Cache Streaming}

\tightsection{Hidden network delay of loading the KV cache}
\label{sec:delay}

\begin{comment}
\begin{itemize}
    \item Section 3 KV Cache Streaming
        \begin{itemize}
        \item Section 3.1: Hidden network delay of loading the context 
        \begin{itemize}
            \item One natural way to reuse the context is to store the KV cache and directly load them when needed, like Figure 4b. cite chunkattention etc. 
            \item these prior works assume the KV cache is in the GPU memory of the inference server. However  the KV cache may not necessarily lie on the same server as the inference server. Reason: the background database for retrieval apps is too large to be replicated on each inference server. For chat apps, users may resume the conversation after a long period of time, thus the KV cache will need to be swapped out. List a concrete example
            % \item For example, when users build LLM apps, they usually upload context (in text format) to the storage server, while querying LLMs hosted in a compute server. In these cases, KV cache is on a remote server than the inference one. 
            \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (Cite interdc throughput)
            \item This can be slow because the size of the KV cache is large. And will negate the benefit of reusing KV cache.
            \item We want to make the loading of KV cache for reusing as fast as possible. 
        \end{itemize}
        \item Section 3.2: 
        \begin{itemize}
            \item To make the loading of KV cache as fast as possible, one way to do it is to encode the KV cache to make its size as small as possible, like figure 4c. 
            \item A common way of encoding data transmitted over the network is to encode it into bitstreams. Explain in our case, it would be encoding the original KV cache tensor into bitstreams on the storage server, decoding it back to tensor of original shape on the inference server 
            \item Ideally, the encoder can make the loading delay of KV cache very small  to maximize the benefit of reusing KV cache 
            \item KV cache streaming can also be applied to other scenarios, such as reducing the delay of migrating KV cache in distributed inference setting 
             \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
            % \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            % \item This will negate the benefit of reusing KV cache. 
            % \item We want to make the loading of KV cache for reusing as fast as possible. 
            % \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
\end{itemize}

\end{comment}

A natural idea to skip the heavy compute of prefill is to {\em reuse the KV cache} of the context if it has been used before.
% Long contexts increase the input length and cause high prefill delay, but since the contexts are often reused, one can naturally reduce the prefill delay is by {\em reusing the KV cache} of the context. 
Indeed, recent studies (\eg~\cite{vllm, chunkattention, promptcache}) have suggested that by saving the KV cache of a context and reusing it when the same context is used again, one could eliminate the prefill delay and significantly reduce TTFT. 

\begin{comment}

one can first run the prefill phase of LLM inference on the context, save the K and V tensors in the resulting KV cache, and reuse them in the future if the same context is used again. %, thus eliminating the future prefill delay. % which grows superlinearly with the context length.
As suggested in recent studies (\eg~\cite{vllm, chunkattention, promptcache}), this method can eliminate the future prefill delay, {\em if} the KV cache is {\em already} in the GPU memory when the same context is used again.
\end{comment}

% \jc{somewhere in this section, we need to define TTFT. we don't need much text about it as before, since TTFT is widely used by industry already}

%In this way, the superlinear procedure of prefilling the context can be bypassed. 
%Indeed, several recent studies~\cite{vllm, chunkattention, promptcache} reuse KV cache that is already in GPU memory to speed-up the processing (prefill) of contexts shared across LLM inference requests. 
%These prior works assume the KV cache is stored in the GPU memory.

In practice, however, the reused KV cache of long contexts may have to be fetched from another machine(s), but this {\em network delay} in fetching the KV cache has been largely overlooked since existing LLM systems assume that the KV cache is always in GPU memory or the KV cache is small enough to be retrieved quickly via a fast GPU interconnection.
% However, the prior systems assume that either the KV cache is always in GPU memory or the KV cache is small enough to be quickly fetched via a dedicated fast interconnection.
% Unfortunately, {\em the network delay} in fetching the KV cache of long contexts can be substantial in practice.
% may {\em not} always be available in the GPU when reused.
This is because the KV cache of a context can be 3-4 orders of magnitude bigger than the context in text format, so the GPU memory may not be big enough to hold the KV caches of all contexts that might be reused.
% \jc{yuhan, please write something like this: GPU memory is typically below \fillme GB, and even if all of it is used for KV cache produced by \fillme model, we will be able to put in the KV cache of \fillme tokens, which roughly translate to \fillme pages of documents, and for KV cache produced by a \fillme (a bigger model), only the KV cache of \fillme tokens can fit in.}

Popular GPUs used for serving LLMs such as the NVidia A40 or RTX A6000 have a maximum GPU memory of 46-48 GB. A common LLM model such as LLama-33B with 8-bit quantized weights requires around 33 GB of GPU memory~\cite{anyscale_blog}. 
If we devote the entire remaining 13 GB to store the KV cache, we can store a maximum token length of around 8000 tokens. 
Standard tokenizers have a ratio of one word equalling 1.33 tokens~\cite{token_blog}, this translates to 6000 words or 6 pages of text of roughly 1000 words per page. 
Thus in general, storing the KV cache on the GPU is challenging, especially when the model size increases, we can store the KV cache of a fewer number of tokens.

Even for chat-based apps where the KV cache of one conversation can fit in the GPU memory, the KV cache may have to be offloaded before the next user query comes. 
For instance, when a user asks the LLM to generate a long story, then the KV cache of the long story (part of context) will be available in GPU memory right after the generation. 
%becomes the context of subsequent conversations.
%, and the KV cache of this context is available in GPU memory. 
However, if the next query about the story does not come until several hours or days later, the GPU may choose to offload the KV cache of this conversation, so even if the next query is routed to the {\em same} GPU, the KV cache will not be available locally and has to be loaded from another machine.

% \jc{yuhan, i deleted your old examples, such as 2T tokens, 364 million docs, etc. in generally, these examples are easy to attack and people's first reaction is we are exaggerating since not all of them are needed at once. in generally, try to avoid examples that people can easily attack.
% same logic goes to the example of azure openai storage service being separate. people can easily attack and say the kv cache doesn't have to be colocated with the text.}


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}

%in the GPU memory of the GPUs that run the LLM inference. 

\begin{comment}
In retrieval-based applications, the size of KV cache of the related background documents is too big to be replicated locally on \emph{each} GPU server that potentially runs LLM inference jobs. 
For example, one recent work uses a background database containing up to 2 trillion tokens in total, which requires 1 TB of storage to save the documents in text format. 
Similarly, another recent work uses a  database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
Thus, the developers of the LLM applications may upload their data to the cloud storage servers, and query LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may build their database and store it on Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance.
Although storing the KV cache in the storage services is not widely applied in existing LLM applications, we envision this will be a popular practice in the near future. \yh{Missing some evidence here. Maybe say that many popular LLM inference frameworks support KV cache as input? }

For chat-based applications, users may resume their conversation with the LLMs after several days. 
Accordingly, those chat histories need to be swapped out from the GPU memory to save space for other active sessions.
Whenever the chat session is resumed, the cached chat histories are highly likely to be loaded from another GPU server. 
Also, given that the number of active users for chat apps is huge (\eg 180 million active users till now for ChatGPT~\cite{vermeer_2023}), it is difficult to store all of the users' chat histories on every GPU server in the inference 
serving system.  
% \yh{Missing why KV cache is on a remote server}
\end{comment}

In these cases, the stored KV cache of the context must be fetched from another machine(s) before being reused, and this network transmission incurs a delay that could \emph{negate} the benefit in saving computation delays from reusing KV cache.
For instance, the KV cache produced by the 65-billion Llama model \ga{Stick to one version of the LLama model for the description.}
%\jc{pick a big one.}
of 5K  tokens is two tensors each of the size $5$K (tokens)$\times$8192 (channels)$\times$80 (layers), leading to a total size of 13~GB.
%\jc{4.1GB was a bit small}
With a throughput of 16~Gbps, typical to the full capacity of a inter-datacenter link~\cite{skyplane}, it will take 6.5 seconds to transmit the KV cache. \ga{inter-DC is a bit confusing.} \ga{It would help to give a breakdown of the times, for me to put the 6.5s in context.}
% To put it in perspective, this delay is similar to the prefill delay from scratch, thus almost negating the benefit of reusing KV cache.
As illustrated in Figure~\ref{fig:motivate_baselines}, transmitting the large KV cache (Figure~\ref{fig:motivate_baselines}(b)) can be almost as large as the delay of prefilling from scratch (Figure~\ref{fig:motivate_baselines}(a)),  thus almost negating the benefit of reusing KV cache.
% \jc{try to connect this discussion with fig~\ref{fig:motivate_baselines}}
Even with 100~Gbps throughput, which is typical for RDMA
% \jc{think about specialized infra like RDMA, memcachd, etc}
, transmitting the KV cache can take up to 1000ms.
If we can reduce it down by 3$\times$, it still makes a perceivable difference~\cite{llmperf}.

In summary, we want to reduce the overall delay for loading and processing a given context.
Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the
generation of the first token. We refer to it as the
\emph{time-to-first-token} (TTFT), since it measures when the first
token is available for the user. 
As shown by previous studies,
users’ experience can be heavily affected by the TTFT since it
demonstrates the responsiveness of the application.
Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
% TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. 

%via a limited bandwidth link.  



\begin{comment}
In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane, ??}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
This is because the size of KV cache is large, far larger than the context in raw text context form.
Specifically, 
for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV cache produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$5120 (channels)$\times$40 (layers), and the size of KV cache serialized by \texttt{torch.save} is 4.1~GB~\footnote{Assumed saving with 16-bit floating point numbers, which is a standard practice~\cite{??}. }.
Given a throughput of 2~Gbps, transmitting the KV cache over the bandwidth can take 16 seconds. 

In short, fetching large KV cache remotely \emph{negates} the benefit of reusing KV cache in saving computation delays. 
This network bottleneck does not only affect one model. 
As shown in Figure~\ref{fig:size_models}, the size of KV cache of popular LLMs all grows with the input token lengths. 
Thus, we want to make the loading of KV cache for reusing as fast as possible, in order to fully maximize the benefit of reusing KV cache in saving prefill delays. 

\end{comment}

\tightsection{\hspace{-0.0cm}\name: KV Cache Streaming}

%\begin{itemize}
%\item what's a kv cache streamer: encode, stream, and decode
%\item how it may help? send a kv cache much faster => faster ttft than prior work. other uses (downplay)
%\item how does it differs from other kv cache compression papers. complementary (top-off) and more compression. deals with bw changes
%\item \name is a concrete design
%\end{itemize}

The need to reduce KV cache transmission delay motivates a new module in LLM systems, which we call a {\em KV cache streamer}.
Put simply, the KV cache streamer serves three roles: 
\begin{packeditemize}
\item {\em (1) encoding} a given KV cache into more compact bitstream representations, called {\em KV bitstreams}, 
\item {\em (2) streaming} the encoded KV bitstreams through a network connection of varying throughput, and 
\item {\em (3) decoding} the received KV bitstreams to get the KV cache.
\end{packeditemize}
Though KV cache has been widely used, there has been little effort on how to encode KV cache to bitstreams efficiently, or on how to stream KV cache under dynamic network bandwidth to reduce TTFT. \ga{Put in a line on how sub-optimal the existing KV cache systems are.}
% \jc{remember to introduce TTFT in the last section}

This paper presents {\bf \name}, a concrete design of the KV cache streamer, which makes two technical contributions.
First, \name uses a custom KV cache codec (encoder and decoder) which minimize size of KV bitreams by embracing several distributional properties of the given KV cache tensors (\S\ref{??}).
Second, when streaming the KV bitstreams under dynamic bandwidth, \name dynamically switches between different compression levels or computing the KV cache on demand. %, in order to complete the transmission of KV cache under a given deadline with high quality.
In addition, the KV coding/decoding in \name incurs a negligible compute overhead and is pipelined with network transmission to minimize the impact on end-to-end delay. 

If successful, the benefit of \name as a KV cache streamer is two-fold.
First, it greatly reduces the bandwidth demand to transmit the KV cache, thus directly reducing TTFT. 
Second, it can dynamically choose the appropriate compression level (or KV compute on-demand) to ensure that TTFT is within a given deadline while maintaining a high response quality.\footnote{The KV cache streamer could also be used to share KV cache more efficiently across different machines in emerging model-parallelism systems for serving LLMs~\cite{lin2024infinitellm, agrawal2023sarathi,??}. 
%These distributed inference systems may migrate KV cache across GPUs, which can also be optimized by such a streaming system. 
}
%by dynamically choosing the compression level streaming KV cache in order to contain TTFT within a deadline, while maintaining a high response quality.

A KV cache streamer (\name) has a key distinction with the emergent techniques for compressing KV cache.
Through dropping less important tokens from context, these techniques (\eg~\cite{scissorhand,zhang2023h2o,beltagy2020longformer}) 
%and others~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing}.
\jc{yuhan, i dropped the other citations. but maybe we need to add the autoencoder paper?}
enable longer contexts or reduce GPU memory footprint. 
Thus, they optimize how to best use GPU memory to store KV cache, rather than how to transmit KV cache over the network, like \name. \ga{The difference is unclear. Lossy vs. lossless? Memory vs. network? Be clear.}
\name is complementary to these techniques and can be used to transmit any KV cache produced by these methods (see \S\ref{??} for a case study of \name with H2O~\cite{zhang2023h2o}).

%, because it can be used to stream any KV cache, including the KV cache after these methods drop the unimportant tokens.
%Moreover, it does not tackle the problem of bandwidth adaptation. 
%This line of work adds a separate module in the self-attention module, which  allows it not to connect each pair of tokens, but to select only a subset of them to approximate the effect of connecting each pair. 
%This will make the self-attention operation less compute and memory-intensive, and thus longer sequences can be taken by the LLMs.

\begin{comment}
How to reuse KV cache while minimizing the network delay?
This paper explores a {\em KV cache streaming} module and a concrete design named \name. 
The KV cache streaming module has three logical steps 

%\tightsubsection{KV cache streaming }

One way of making KV cache loading fast is to encode the KV cache and stream it via the network.   
A common way of encoding data transmitted over the network is to encode it into bitstreams. 
In the scenario of KV cache streaming, the streamer encodes the KV cache into bitstreams on the storage server, and decodes it back to the original KV cache for LLM inference, as shown in Figure~\ref{fig:motivate_baselines}c.
Ideally, with such a streamer, the transmission delay, together with the decoding delay, will be much smaller than the delay of computing the KV cache of the context from raw text context, in order to  maximize the benefit of reusing KV cache in terms of computation. 
Furthermore, the streamer should also be able to adapt to dynamic resource allocation and make optimal decisions to stream KV cache differently under resource change. 


Potentially, KV cache streaming can also be applied in other scenarios, such as in distributed inference systems~\cite{lin2024infinitellm, agrawal2023sarathi, ??}. 
These distributed inference systems may migrate KV cache across GPUs, which can also be optimized by such a streaming system. 

This goal is fundamentally different from the prior works that try to enable longer context by text shortening, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and many others~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing}. 
This line of work adds a separate module in the self-attention module, which  allows it not to connect each pair of tokens, but to select only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and thus longer sequences can be taken by the LLMs.

\end{comment}


% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

% \tightsection{Hidden network delays of loading contexts}


% % \shan{I suggest making this sub-section a separate section and
% % name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% % section is REALLY tooo long. 2. this sub-section is actually not
% % a background. instead, it is an important observation made by us
% % that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% % make it a separate section. If it is in background, it sounds
% % more like previous work's observation.}
% Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% % \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% % need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
% In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
% Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
% \yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
% To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance. \yh{Find another example maybe in chat apps? } 
% % In chat apps, a user may resume his/her conversation with LLM a few days after the last interaction on the same topic. 
% % So, the KV cache of his/her conversation history needs to be swapped out of GPU memory to save space for other active conversations~\cite{orca,shepherd,clockwork}. 
% % The KV cache that is swapped out is likely to be used by a resumed conversation at a different inference server. 
% % \yh{Add another example? }
% In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
% With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
% Specifically, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
% Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
% }
% \shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.} 
% % \jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% % \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% % \yh{Per request Bandwidth needs to be within a reasonable range  }
% % \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% % In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% % In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% % Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% % \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% % }
% % \todo{}

% % \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% % \todo{More evidences on why context is not in GPU}


% % In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
% % One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% % % and the storage server on which LLM inference runs may not have enough space to store them.
% % For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
% % %and storing these texts can take a space up to around 750 GB. 
% % In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% % Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% % % \jc{please add some evidence and citations here}
% % % \yh{todo: add more citations for retrieval-based apps}

% % In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
% % In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% % % \jc{please add some evidence and citations here}
% % Moreover, a user may issue her prompts to the LLM from different locations at different points.
% % As these prompts can be processed by different machines, the contexts must be remotely fetched.




% %In this work, we assume that the context is stored in a different machine than the GPUs running the LLM



\begin{comment}
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}
\end{comment}


% % As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large.
% % Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
% % More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% % However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% % To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% % In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
% %(with 32 layers and 4096 channels) can be 1.3~GB. 
% %for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
% %On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% % \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% % Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% % By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

% In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
% This network bottleneck does not only affect one model.
% As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/problem.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US






%\tightsection{KV Cache Streaming}

\tightsection{Hidden network delay of loading the KV cache}

\begin{comment}
\begin{itemize}
    \item Section 3 KV Cache Streaming
        \begin{itemize}
        \item Section 3.1: Hidden network delay of loading the context 
        \begin{itemize}
            \item One natural way to reuse the context is to store the KV cache and directly load them when needed, like Figure 4b. cite chunkattention etc. 
            \item these prior works assume the KV cache is in the GPU memory of the inference server. However  the KV cache may not necessarily lie on the same server as the inference server. Reason: the background database for retrieval apps is too large to be replicated on each inference server. For chat apps, users may resume the conversation after a long period of time, thus the KV cache will need to be swapped out. List a concrete example
            % \item For example, when users build LLM apps, they usually upload context (in text format) to the storage server, while querying LLMs hosted in a compute server. In these cases, KV cache is on a remote server than the inference one. 
            \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (Cite interdc throughput)
            \item This can be slow because the size of the KV cache is large. And will negate the benefit of reusing KV cache.
            \item We want to make the loading of KV cache for reusing as fast as possible. 
        \end{itemize}
        \item Section 3.2: 
        \begin{itemize}
            \item To make the loading of KV cache as fast as possible, one way to do it is to encode the KV cache to make its size as small as possible, like figure 4c. 
            \item A common way of encoding data transmitted over the network is to encode it into bitstreams. Explain in our case, it would be encoding the original KV cache tensor into bitstreams on the storage server, decoding it back to tensor of original shape on the inference server 
            \item Ideally, the encoder can make the loading delay of KV cache very small  to maximize the benefit of reusing KV cache 
            \item KV cache streaming can also be applied to other scenarios, such as reducing the delay of migrating KV cache in distributed inference setting 
             \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
            % \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            % \item This will negate the benefit of reusing KV cache. 
            % \item We want to make the loading of KV cache for reusing as fast as possible. 
            % \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
\end{itemize}

\end{comment}


Long contexts increase the input length and cause high prefill delay, but since the contexts are often reused, one can naturally reduce the prefill delay is by {\em reusing the KV cache} of the context. 
Specifically, one can first run the prefill phase of LLM inference on the context, save the K and V tensors in the resulting KV cache, and reuse them in the future if the same context is used again. %, thus eliminating the future prefill delay. % which grows superlinearly with the context length.
As suggested in recent studies~\cite{vllm, chunkattention, promptcache}, this method can eliminate the future prefill delay, {\em if} the KV cache is {\em already} in the GPU memory when the same context is used again.
%In this way, the superlinear procedure of prefilling the context can be bypassed. 
%Indeed, several recent studies~\cite{vllm, chunkattention, promptcache} reuse KV cache that is already in GPU memory to speed-up the processing (prefill) of contexts shared across LLM inference requests. 
%These prior works assume the KV cache is stored in the GPU memory.

Unfortunately, the KV cache of a context may {\em not} always be available in the GPU when it is reused.
This is because the KV cache of a context can be 3-4 orders of magnitude greater in size than the context in text format, so the GPU memory may not be big enough to hold all potentially needed KV cache.
\jc{yuhan, please write something like this: GPU memory is typically below \fillme GB, and even if all of it is used for KV cache produced by \fillme model, we will be able to put in the KV cache of \fillme tokens, which roughly translate to \fillme pages of documents, and for KV cache produced by a \fillme (a bigger model), only the KV cache of \fillme tokens can fit in.}

Even for chat-based apps where the KV cache of one conversation can fit in the GPU memory, the KV cache may have to be offloaded before the next user query comes. 
For instance, when a user asks the LLM to generate a long story, then the KV cache of the long story (part of context) will be available in GPU memory right after the generation. 
%becomes the context of subsequent conversations.
%, and the KV cache of this context is available in GPU memory. 
However, if the next query about the story does not come until several hours or days later, the GPU may choose to offload the KV cache of this conversation, so even if the next query is routed to the {\em same} GPU, the KV cache will not be available locally and has to be loaded from another machine.

\jc{yuhan, i deleted your old examples, such as 2T tokens, 364 million docs, etc. in generally, these examples are easy to attack and people's first reaction is we are exaggerating since not all of them are needed at once. in generally, try to avoid examples that people can easily attack.
same logic goes to the example of azure openai storage service being separate. people can easily attack and say the kv cache doesn't have to be colocated with the text.}


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}

%in the GPU memory of the GPUs that run the LLM inference. 

\begin{comment}
In retrieval-based applications, the size of KV cache of the related background documents is too big to be replicated locally on \emph{each} GPU server that potentially runs LLM inference jobs. 
For example, one recent work uses a background database containing up to 2 trillion tokens in total, which requires 1 TB of storage to save the documents in text format. 
Similarly, another recent work uses a  database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
Thus, the developers of the LLM applications may upload their data to the cloud storage servers, and query LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may build their database and store it on Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance.
Although storing the KV cache in the storage services is not widely applied in existing LLM applications, we envision this will be a popular practice in the near future. \yh{Missing some evidence here. Maybe say that many popular LLM inference frameworks support KV cache as input? }

For chat-based applications, users may resume their conversation with the LLMs after several days. 
Accordingly, those chat histories need to be swapped out from the GPU memory to save space for other active sessions.
Whenever the chat session is resumed, the cached chat histories are highly likely to be loaded from another GPU server. 
Also, given that the number of active users for chat apps is huge (\eg 180 million active users till now for ChatGPT~\cite{vermeer_2023}), it is difficult to store all of the users' chat histories on every GPU server in the inference 
serving system.  
% \yh{Missing why KV cache is on a remote server}
\end{comment}

In these cases, the stored KV cache of the context must be fetched from another machine(s) before being reused, and this network transmission incurs a delay that could \emph{negate} the benefit in saving computation delays from reusing KV cache.
For instance, the KV cache produced by the \fillme model\jc{pick a big one.} of \fillme tokens is two tensors each of the size $5$K (tokens)$\times$5120 (channels)$\times$40 (layers), leading to a total size of \fillme~GB\jc{4.1GB was a bit small}
With a throughput of \fillme~Gbps, typical to the full capacity of \fillme, it will take \fillme seconds to transmit the KV cache. 
To put it in perspective, this delay is similar to the prefill delay from scratch, thus almost negating the benefit of reusing KV cache.
\jc{try to connect this discussion with fig~\ref{fig:motivate_baselines}}
Even with a throughput of \fillme~Gbps, which is typical to \fillme\jc{think about specialized infra like RDMA, memcachd, etc}, transmitting the KV cache can take \fillme milliseconds\jc{try to get to about 800ms}.
If we can reduce it down by \fillme, it can still make a perceivable difference to users~\cite{??,??}.

%via a limited bandwidth link.  



\begin{comment}
In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane, ??}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
This is because the size of KV cache is large, far larger than the context in raw text context form.
Specifically, 
for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV cache produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$5120 (channels)$\times$40 (layers), and the size of KV cache serialized by \texttt{torch.save} is 4.1~GB~\footnote{Assumed saving with 16-bit floating point numbers, which is a standard practice~\cite{??}. }.
Given a throughput of 2~Gbps, transmitting the KV cache over the bandwidth can take 16 seconds. 

In short, fetching large KV cache remotely \emph{negates} the benefit of reusing KV cache in saving computation delays. 
This network bottleneck does not only affect one model. 
As shown in Figure~\ref{fig:size_models}, the size of KV cache of popular LLMs all grows with the input token lengths. 
Thus, we want to make the loading of KV cache for reusing as fast as possible, in order to fully maximize the benefit of reusing KV cache in saving prefill delays. 

\end{comment}

\tightsubsection{KV cache streaming }

One way of making KV cache loading fast is to encode the KV cache and stream it via the network.   
A common way of encoding data transmitted over the network is to encode it into bitstreams. 
In the scenario of KV cache streaming, the streamer encodes the KV cache into bitstreams on the storage server, and decodes it back to the original KV cache for LLM inference, as shown in Figure~\ref{fig:motivate_baselines}c.
Ideally, with such a streamer, the transmission delay, together with the decoding delay, will be much smaller than the delay of computing the KV cache of the context from raw text context, in order to  maximize the benefit of reusing KV cache in terms of computation. 
Furthermore, the streamer should also be able to adapt to dynamic resource allocation and make optimal decisions to stream KV cache differently under resource change. 


Potentially, KV cache streaming can also be applied in other scenarios, such as in distributed inference systems~\cite{lin2024infinitellm, agrawal2023sarathi, ??}. 
These distributed inference systems may migrate KV cache across GPUs, which can also be optimized by such a streaming system. 

This goal is fundamentally different from the prior works that try to enable longer context by text shortening, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and many others~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing}. 
This line of work adds a separate module in the self-attention module, which  allows it not to connect each pair of tokens, but to select only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and thus longer sequences can be taken by the LLMs.




% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

% \tightsection{Hidden network delays of loading contexts}


% % \shan{I suggest making this sub-section a separate section and
% % name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% % section is REALLY tooo long. 2. this sub-section is actually not
% % a background. instead, it is an important observation made by us
% % that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% % make it a separate section. If it is in background, it sounds
% % more like previous work's observation.}
% Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% % \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% % need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
% In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
% Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
% \yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
% To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance. \yh{Find another example maybe in chat apps? } 
% % In chat apps, a user may resume his/her conversation with LLM a few days after the last interaction on the same topic. 
% % So, the KV cache of his/her conversation history needs to be swapped out of GPU memory to save space for other active conversations~\cite{orca,shepherd,clockwork}. 
% % The KV cache that is swapped out is likely to be used by a resumed conversation at a different inference server. 
% % \yh{Add another example? }
% In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
% With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
% Specifically, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
% Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
% }
% \shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.} 
% % \jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% % \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% % \yh{Per request Bandwidth needs to be within a reasonable range  }
% % \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% % In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% % In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% % Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% % \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% % }
% % \todo{}

% % \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% % \todo{More evidences on why context is not in GPU}


% % In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
% % One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% % % and the storage server on which LLM inference runs may not have enough space to store them.
% % For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
% % %and storing these texts can take a space up to around 750 GB. 
% % In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% % Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% % % \jc{please add some evidence and citations here}
% % % \yh{todo: add more citations for retrieval-based apps}

% % In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
% % In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% % % \jc{please add some evidence and citations here}
% % Moreover, a user may issue her prompts to the LLM from different locations at different points.
% % As these prompts can be processed by different machines, the contexts must be remotely fetched.




% %In this work, we assume that the context is stored in a different machine than the GPUs running the LLM
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}

% % As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large.
% % Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
% % More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% % However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% % To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% % In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
% %(with 32 layers and 4096 channels) can be 1.3~GB. 
% %for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
% %On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% % \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% % Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% % By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

% In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
% This network bottleneck does not only affect one model.
% As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/problem_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US






%\tightsection{KV Cache Streaming}

\tightsection{Hidden network delay of loading the KV cache}

\begin{comment}
\begin{itemize}
    \item Section 3 KV Cache Streaming
        \begin{itemize}
        \item Section 3.1: Hidden network delay of loading the context 
        \begin{itemize}
            \item One natural way to reuse the context is to store the KV cache and directly load them when needed, like Figure 4b. cite chunkattention etc. 
            \item these prior works assume the KV cache is in the GPU memory of the inference server. However  the KV cache may not necessarily lie on the same server as the inference server. Reason: the background database for retrieval apps is too large to be replicated on each inference server. For chat apps, users may resume the conversation after a long period of time, thus the KV cache will need to be swapped out. List a concrete example
            % \item For example, when users build LLM apps, they usually upload context (in text format) to the storage server, while querying LLMs hosted in a compute server. In these cases, KV cache is on a remote server than the inference one. 
            \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (Cite interdc throughput)
            \item This can be slow because the size of the KV cache is large. And will negate the benefit of reusing KV cache.
            \item We want to make the loading of KV cache for reusing as fast as possible. 
        \end{itemize}
        \item Section 3.2: 
        \begin{itemize}
            \item To make the loading of KV cache as fast as possible, one way to do it is to encode the KV cache to make its size as small as possible, like figure 4c. 
            \item A common way of encoding data transmitted over the network is to encode it into bitstreams. Explain in our case, it would be encoding the original KV cache tensor into bitstreams on the storage server, decoding it back to tensor of original shape on the inference server 
            \item Ideally, the encoder can make the loading delay of KV cache very small  to maximize the benefit of reusing KV cache 
            \item KV cache streaming can also be applied to other scenarios, such as reducing the delay of migrating KV cache in distributed inference setting 
             \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
            % \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            % \item This will negate the benefit of reusing KV cache. 
            % \item We want to make the loading of KV cache for reusing as fast as possible. 
            % \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
\end{itemize}

\end{comment}


Long contexts increase the input length and cause high prefill delay, but since the contexts are often reused, one can naturally reduce the prefill delay is by {\em reusing the KV cache} of the context. 
Specifically, one can first run the prefill phase of LLM inference on the context, save the K and V tensors in the resulting KV cache, and reuse them in the future if the same context is used again. %, thus eliminating the future prefill delay. % which grows superlinearly with the context length.
As suggested in recent studies~\cite{vllm, chunkattention, promptcache}, this method can eliminate the future prefill delay, {\em if} the KV cache is {\em already} in the GPU memory when the same context is used again.
%In this way, the superlinear procedure of prefilling the context can be bypassed. 
%Indeed, several recent studies~\cite{vllm, chunkattention, promptcache} reuse KV cache that is already in GPU memory to speed-up the processing (prefill) of contexts shared across LLM inference requests. 
%These prior works assume the KV cache is stored in the GPU memory.

Unfortunately, the KV cache of a context may {\em not} always be available in the GPU when it is reused.
This is because the KV cache of a context can be 3-4 orders of magnitude greater in size than the context in text format, so the GPU memory may not be big enough to hold all potentially needed KV cache.
\jc{yuhan, please write something like this: GPU memory is typically below \fillme GB, and even if all of it is used for KV cache produced by \fillme model, we will be able to put in the KV cache of \fillme tokens, which roughly translate to \fillme pages of documents, and for KV cache produced by a \fillme (a bigger model), only the KV cache of \fillme tokens can fit in.}

Even for chat-based apps where the KV cache of one conversation can fit in the GPU memory, the KV cache may have to be offloaded before the next user query comes. 
For instance, when a user asks the LLM to generate a long story, then the KV cache of the long story (part of context) will be available in GPU memory right after the generation. 
%becomes the context of subsequent conversations.
%, and the KV cache of this context is available in GPU memory. 
However, if the next query about the story does not come until several hours or days later, the GPU may choose to offload the KV cache of this conversation, so even if the next query is routed to the {\em same} GPU, the KV cache will not be available locally and has to be loaded from another machine.

\jc{yuhan, i deleted your old examples, such as 2T tokens, 364 million docs, etc. in generally, these examples are easy to attack and people's first reaction is we are exaggerating since not all of them are needed at once. in generally, try to avoid examples that people can easily attack.
same logic goes to the example of azure openai storage service being separate. people can easily attack and say the kv cache doesn't have to be colocated with the text.}


\begin{figure}[t]
\centering
     \includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).} 
    \label{fig:motivate_baselines}
\end{figure}

%in the GPU memory of the GPUs that run the LLM inference. 

\begin{comment}
In retrieval-based applications, the size of KV cache of the related background documents is too big to be replicated locally on \emph{each} GPU server that potentially runs LLM inference jobs. 
For example, one recent work uses a background database containing up to 2 trillion tokens in total, which requires 1 TB of storage to save the documents in text format. 
Similarly, another recent work uses a  database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
Thus, the developers of the LLM applications may upload their data to the cloud storage servers, and query LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may build their database and store it on Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance.
Although storing the KV cache in the storage services is not widely applied in existing LLM applications, we envision this will be a popular practice in the near future. \yh{Missing some evidence here. Maybe say that many popular LLM inference frameworks support KV cache as input? }

For chat-based applications, users may resume their conversation with the LLMs after several days. 
Accordingly, those chat histories need to be swapped out from the GPU memory to save space for other active sessions.
Whenever the chat session is resumed, the cached chat histories are highly likely to be loaded from another GPU server. 
Also, given that the number of active users for chat apps is huge (\eg 180 million active users till now for ChatGPT~\cite{vermeer_2023}), it is difficult to store all of the users' chat histories on every GPU server in the inference 
serving system.  
% \yh{Missing why KV cache is on a remote server}
\end{comment}

In these cases, the stored KV cache of the context must be fetched from another machine(s) before being reused, and this network transmission incurs a delay that could \emph{negate} the benefit in saving computation delays from reusing KV cache.
For instance, the KV cache produced by the \fillme model\jc{pick a big one.} of \fillme tokens is two tensors each of the size $5$K (tokens)$\times$5120 (channels)$\times$40 (layers), leading to a total size of \fillme~GB\jc{4.1GB was a bit small}
With a throughput of \fillme~Gbps, typical to the full capacity of \fillme, it will take \fillme seconds to transmit the KV cache. 
To put it in perspective, this delay is similar to the prefill delay from scratch, thus almost negating the benefit of reusing KV cache.
\jc{try to connect this discussion with fig~\ref{fig:motivate_baselines}}
Even with a throughput of \fillme~Gbps, which is typical to \fillme\jc{think about specialized infra like RDMA, memcachd, etc}, transmitting the KV cache can take \fillme milliseconds\jc{try to get to about 800ms}.
If we can reduce it down by \fillme, it can still make a perceivable difference to users~\cite{??,??}.

%via a limited bandwidth link.  



\begin{comment}
In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane, ??}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
This is because the size of KV cache is large, far larger than the context in raw text context form.
Specifically, 
for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV cache produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$5120 (channels)$\times$40 (layers), and the size of KV cache serialized by \texttt{torch.save} is 4.1~GB~\footnote{Assumed saving with 16-bit floating point numbers, which is a standard practice~\cite{??}. }.
Given a throughput of 2~Gbps, transmitting the KV cache over the bandwidth can take 16 seconds. 

In short, fetching large KV cache remotely \emph{negates} the benefit of reusing KV cache in saving computation delays. 
This network bottleneck does not only affect one model. 
As shown in Figure~\ref{fig:size_models}, the size of KV cache of popular LLMs all grows with the input token lengths. 
Thus, we want to make the loading of KV cache for reusing as fast as possible, in order to fully maximize the benefit of reusing KV cache in saving prefill delays. 

\end{comment}

\tightsubsection{KV cache streaming }

One way of making KV cache loading fast is to encode the KV cache and stream it via the network.   
A common way of encoding data transmitted over the network is to encode it into bitstreams. 
In the scenario of KV cache streaming, the streamer encodes the KV cache into bitstreams on the storage server, and decodes it back to the original KV cache for LLM inference, as shown in Figure~\ref{fig:motivate_baselines}c.
Ideally, with such a streamer, the transmission delay, together with the decoding delay, will be much smaller than the delay of computing the KV cache of the context from raw text context, in order to  maximize the benefit of reusing KV cache in terms of computation. 
Furthermore, the streamer should also be able to adapt to dynamic resource allocation and make optimal decisions to stream KV cache differently under resource change. 


Potentially, KV cache streaming can also be applied in other scenarios, such as in distributed inference systems~\cite{lin2024infinitellm, agrawal2023sarathi, ??}. 
These distributed inference systems may migrate KV cache across GPUs, which can also be optimized by such a streaming system. 

This goal is fundamentally different from the prior works that try to enable longer context by text shortening, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and many others~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing}. 
This line of work adds a separate module in the self-attention module, which  allows it not to connect each pair of tokens, but to select only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and thus longer sequences can be taken by the LLMs.




% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

% \tightsection{Hidden network delays of loading contexts}


% % \shan{I suggest making this sub-section a separate section and
% % name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% % section is REALLY tooo long. 2. this sub-section is actually not
% % a background. instead, it is an important observation made by us
% % that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% % make it a separate section. If it is in background, it sounds
% % more like previous work's observation.}
% Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% % \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% % need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
% In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
% Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
% \yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
% To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance. \yh{Find another example maybe in chat apps? } 
% % In chat apps, a user may resume his/her conversation with LLM a few days after the last interaction on the same topic. 
% % So, the KV cache of his/her conversation history needs to be swapped out of GPU memory to save space for other active conversations~\cite{orca,shepherd,clockwork}. 
% % The KV cache that is swapped out is likely to be used by a resumed conversation at a different inference server. 
% % \yh{Add another example? }
% In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
% With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
% Specifically, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
% Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
% }
% \shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.} 
% % \jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% % \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% % \yh{Per request Bandwidth needs to be within a reasonable range  }
% % \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% % In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% % In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% % Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% % \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% % }
% % \todo{}

% % \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% % \todo{More evidences on why context is not in GPU}


% % In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
% % One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% % % and the storage server on which LLM inference runs may not have enough space to store them.
% % For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
% % %and storing these texts can take a space up to around 750 GB. 
% % In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% % Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% % % \jc{please add some evidence and citations here}
% % % \yh{todo: add more citations for retrieval-based apps}

% % In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
% % In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% % % \jc{please add some evidence and citations here}
% % Moreover, a user may issue her prompts to the LLM from different locations at different points.
% % As these prompts can be processed by different machines, the contexts must be remotely fetched.




% %In this work, we assume that the context is stored in a different machine than the GPUs running the LLM
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}

% % As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large.
% % Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
% % More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% % However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% % To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% % In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
% %(with 32 layers and 4096 channels) can be 1.3~GB. 
% %for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
% %On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% % \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% % Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% % By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

% In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
% This network bottleneck does not only affect one model.
% As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.




==> backups/related-works-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\section{Related work}
\label{sec:related}

\mypara{Faster LLM serving}
Recent efforts in LLM systems research aim at either at speeding up LLM training~\cite{deepspeed, shoeybi2019megatron} or making the LLM serving systems faster. Different ways include parallelizing the generation of multiple tokens with smaller approximating models~\cite{Leviathan2022FastIF, miao2023specinfer}, accelerating the inference of Mix-of-Expert LLMs on edge devices~\cite{yi2023edgemoe}, quantizing LLM model weights~\cite{aminabadi2022deepspeed}, reducing memory I/O of GPU on-chip SRAM~\cite{dao2022flashattention}, and reducing self-attention computation complexity by k-means~\cite{roy2021efficient}. 
New LLM service scheduling strategies are proposed in ~\cite{wu2023fast,orca} along with more efficient GPU memory utilization in~\cite{vllm}.

A common approach for faster inference without modifying the LLMs is by {\em caching the KV} of previously used inputs for {\em one} LLM query~\cite{wu2023fast,flexgen,li2022decoupled, dai*2019transformerxl, ott2019fairseq, zhang2023ho, scissorhand, pope2022efficiently, miao2023specinfer, wolf-etal-2020-transformers}. 
However \name benefits by storing multiple KV caches (which might be commonly used) on a separate server and transmits them in a bandwidth-efficient way over the network for {\em reuse across  multiple} LLM queries.

% The landscape of LLM systems research is fast evolving.
% Besides speeding up LLM training (\eg~\cite{deepspeed, shoeybi2019megatron}), many recent efforts, including ours, focus on the LLM serving systems. 
% Some try to parallelize the generation of multiple tokens with smaller approximating models~\cite{Leviathan2022FastIF, miao2023specinfer} and accelerate the inference of Mix-of-Expert LLMs on edge devices~\cite{yi2023edgemoe}. 
% Others quantize LLM model weights (\eg~\cite{aminabadi2022deepspeed}), reduce memory I/O of GPU on-chip SRAM~\cite{dao2022flashattention}, and reduce self-attention computation complexity by k-means~\cite{roy2021efficient}. 
% New scheduling strategies are also proposed for LLM services~\cite{wu2023fast,orca} along with more efficient GPU memory utilization~\cite{vllm}.
% Nonetheless, a common approach to speeding up without modifying the LLMs is by {\em caching KV} cache of repeatedly used input sequences, such as contexts~\cite{wu2023fast,flexgen,li2022decoupled, dai*2019transformerxl, ott2019fairseq, zhang2023ho, scissorhand, pope2022efficiently, miao2023specinfer, wolf-etal-2020-transformers}. 
% However, caching KV cache results in a dramatically increased amount of cached data, which requires a bandwidth-efficient KV/context-loading system like \name.



% many works. change models, etc. kv cache is common, but more data need to be loaded
% kv cache
% smaller models
% sim: also use kv
% diff: doesn't optimize loading


\mypara{Longer LLM inputs (contexts)}
While benefits of long contexts are still under scrutiny~\cite{liu2023lost,sun2021longrange, roy2021efficient}, many recent efforts aim at enabling LLMs to process very long contexts~\cite{xu2024retrieval}.
% , under the premise that longer contexts improve generation quality (\eg~\cite{wu2022memorizing,dai*2019transformerxl}).
The main challenge is fitting the corresponding larger attention matrices of longer contexts into limited GPU memory. 
Processing longer input sequences is enabled by
offloading less used parts of the attention matrices~\cite{flexgen},
using external knowledge via KNN~\cite{wu2022memorizing}, approximating via 
retraining self-attention to only attend to top-k keys~\cite{bertsch2023unlimiformer,ainslie2020etc}, 
mapping long inputs into smaller latent spaces~\cite{pmlr-v162-hawthorne22a} and using local windowed~\cite{beltagy2020longformer}, dilated~\cite{ding2023longnet} or sparse~\cite{zaheer2021big} attention to scale to input lengths of $\sim$1 billion tokens.
These longer inputs (contexts) inflate the KV cache, and \name complements these efforts by enabling fast remote loading of the KV cache.

% While benefits of longer contexts are still under scrutiny~\cite{liu2023lost,sun2021longrange, roy2021efficient}, many recent efforts aim at enabling LLMs to accept even {\em longer} contexts~\cite{xu2024retrieval}.
% % , under the premise that longer contexts improve generation quality (\eg~\cite{wu2022memorizing,dai*2019transformerxl}).
% The main challenge is to hold the attention matrices of more tokens without needing a bigger GPU memory. 
% They enable longer input sequences by
% dynamically offloading less used parts of the attention matrices~\cite{flexgen},
% using external knowledge via KNN~\cite{wu2022memorizing}, 
% retraining the self-attention module to only attend to top-k keys to approximate the full attention~\cite{bertsch2023unlimiformer,ainslie2020etc}, 
% mapping long inputs into smaller latent space~\cite{pmlr-v162-hawthorne22a}, 
% using local windowed self-attention~\cite{beltagy2020longformer}, 
% or 
% using dilated attention~\cite{ding2023longnet} or sparse attention~\cite{zaheer2021big} to scale the input length to even 1 billion tokens.
% However, the longer inputs (contexts) also inflate the KV cache, and this work complements these efforts by focusing on fast remote loading of KV cache.


% moreover, contexts are longer. stretching the limit of gpu mem. causing even bigger kv features.
% increase context length
% memory compression
% sim: inspire longer context
% diff: doesn't optimize loading

\mypara{Context shortening/pruning}
A lot of emerging literature on shortening and pruning long contexts relates well to \name. These efforts aim to select the most important text segments and prune the rest to reduce context length. Methods for this can be based on the similarity between the user query and the potentially relevant documents ~\cite{retro}. Dropping tokens that are less attended to by the current prompt is done in ~\cite{scissorhand, zhang2023ho}. This can be done by identifying a smaller subset of {\em heavy hitter} tokens which contribute most to the overall attention scores~\cite{ge2023model}. Using  query-aware compression with document reordering to reduce loss-in-the-middle, is another recent method proposed to shorten context lengths~\cite{jiang2023longllmlingua}. Approximating attention scores using a subset of query and key vector components allows for only fetching the most relevant tokens and reduces memory traffic~\cite{ribar2023sparq}. 

One limitation of all these methods are that they need to know the query else they risk dropping/missing potentially important tokens. Choosing the right compression ratio is also hard, many models already show quality degradation at 2$x$ compressed length~\cite{ribar2023sparq} Finally, some works retrain LLM models to directly take in contexts that are rewritten by gisting~\cite{gisting} or auto-encoding~\cite{autoencoder-incontext}.

\name differs from the above by compressing the KV cache into bitstreams, rather than shortening the context in its original form (i.e., text or tensor) and fetching the compressed KV cache efficiently. \name's KV compression does not need to know the query/prompt and it doesn't risk quality loss from dropping potentially important tokens. It allows for better compression rates by leveraging unique distributional properties of KV cache and achieves better delay-quality trade-offs than existing context compressors (\S\ref{subsec:eval:micro}). Finally \name does not need to re-train the LLM.

% \sid{Don't emphasise the following para.}
%  Different from them, 
% %Second, \name minimizes the sum of network delay to transfer the KV cache and the computation delay, rather than only the computation delay.
% %Moreover, unlike~\cite{scissorhand,borgeaud2022improving}, \name's KV compression does not need to know the query (prompt), and 
% \name does not need to train a new LLM model and also achieves better compression rate with
% less information loss by leveraging unique distributional properties of KV cache.
% %to rewrite contexts, like in~\cite{gisting,in-context-autoencoder}.
% Finally, we show \name achieves better delay-quality tradeoffs than existing context compressors (\S\ref{subsec:eval:micro}).
% and can potentially be combined with them to further improve the delay-quality tradeoffs.

% More relevant to our work is the emerging literature on shortening and pruning long contexts. 
% These efforts select the most important text segments and prune out the others to reduce context length, based on the similarity between the user query and the potentially relevant documents (\eg~\cite{retro}), 
% drop tokens that are less attended to by the current prompt~\cite{scissorhand, zhang2023ho, ge2023model} or use query-aware compression with document reordering to reduce loss-in-the-middle~\cite{jiang2023longllmlingua}.

% Different from them, \name compresses the KV cache into bitstreams, rather than shortening the context in its original form (i.e., text or tensor). 
% Unlike~\cite{scissorhand, retro, zhang2023ho,jiang2023longllmlingua}, \name's KV compression does not need to know the query/prompt. 

% \sid{Don't emphasise the following para.}
% Recently, some work retrains LLM models to directly take in contexts that are
% rewritten by gisting~\cite{gisting} or auto-encoding
% ~\cite{autoencoder-incontext}. Different from them, 
% %Second, \name minimizes the sum of network delay to transfer the KV cache and the computation delay, rather than only the computation delay.
% %Moreover, unlike~\cite{scissorhand,borgeaud2022improving}, \name's KV compression does not need to know the query (prompt), and 
% \name does not need to train a new LLM model and also achieves better compression rate with
% less information loss by leveraging unique distributional properties of KV cache.
% %to rewrite contexts, like in~\cite{gisting,in-context-autoencoder}.
% Finally, we show \name achieves better delay-quality tradeoffs than existing context compressors (\S\ref{subsec:eval:micro}).
% and can potentially be combined with them to further improve the delay-quality tradeoffs.

% one common approach is to shorten context, but dropping tokens or rewriting or better doc selection.
% diff: we compress KV cache

\mypara{Tensor compression}
\name's KV encoder can be seen as a special tensor compression technique tailored for LLM's KV caches.
General tensor compression has been intensively studied, \eg relaxing rank and ordering constraint~\cite{zhao2016tensor} or decomposing large tensors into products of smaller ones~\cite{tensor_decomp}.
In DNN training, tensor compression has been used to compress gradient updates of DNN weights (\eg~\cite{espresso,MLSYS2022_773862fc,agarwal2020accordion}).
However KV caches and gradients have very different properties.
These training systems often leverage the sparsity of gradient updates which occurs due to methods like~\cite{chen2023sparse, zehui2019dropattention, child2019generating}. However the KV cache is not known to be sparse in general.
% to strike a balance between compression efficiency and loss of accuracy.
% \yh{Gradient compression: Three major schemes:
% (1) quantization based SignSGD; (2) low-rank decomposition based PowerSGD (3) Sparsification based Top-K. 
% The assumptions under those schemes are that the gradient to be updated is sparse. Which is not the case in \kv. 
% Also, 
% Note that in popular distributed training 
% \cite{agarwal2020accordion}  }

% \jc{the title may be a bit misleading. should we call it ``Retrieval-augmented generation''?}

\mypara{Retrieval-augmented generation}
A wide range of works ~\cite{retro, atlas, fid,rubin2023long,lewis2020retrieval,Yang_2019, karpukhin2020dense, wang2023zemi, ram2023incontext} focus on optimizing retrieval-augmented generation (RAG). Retrieval-augmented generation includes retrieving relevant documents to the user's question, by comparing the question with documents in the database via vector based~\cite{chen2017reading, Yang_2019, nie2019revealing} or DNN-based~\cite{lewis2020retrieval, karpukhin2020dense,xiong-etal-2021-progressively, reranking} similarity search algorithms. The retrieved documents are fed as the context to the LLMs to generate the answers to the question.

We envision RAG as a fitting use case for \name, as many LLM inference platforms support feeding in the KV cache as retrieved context instead of text documents~\cite{hf2020, Chase_LangChain_2022}. Relevant KV cache can be retrieved using similarity based searching as mentioned above.
Optimal methods on which KV cache to reuse in RAG (to generate the best output) is still an open area, though some works have attempted to define a systematic way to choose them~\cite{gim2023prompt}.

% \edit{\mypara{Retrieval-augmented generation} A wide range of works
% %~\cite{retro, atlas, fid,rubin2023long,lewis2020retrieval,Yang_2019, karpukhin2020dense,xiong-etal-2021-progressively, reranking, shi2023replug,li2022decoupled, wang2023zemi}
% ~\cite{retro, atlas, fid,rubin2023long,lewis2020retrieval,Yang_2019, karpukhin2020dense, wang2023zemi, ram2023incontext}
% focus on optimizing retrieval-augmented generation. 
% The workflow of retrieval-augmented generation includes retrieving relevant documents to the user's question, and feeding the retrieved documents as the context to the LLMs to generate the answers to the question.
% Upon receiving a question submitted by the user, the application decides the relevant documents by comparing the question with documents in the database via similarity search algorithms, such as dense or sparse vector methods~\cite{chen2017reading, Yang_2019, nie2019revealing} and DNN-based schemes~\cite{lewis2020retrieval, karpukhin2020dense,xiong-etal-2021-progressively, reranking}.
% For example, FiD~\cite{fid} represents the prompt text and the documents' text in the form of ``bag of words'' and ranks the relevance of the documents with the term frequency-inverse document frequence (TF-IDF).
% As another example, Atlas~\cite{atlas} pre-trains a BERT-based retriever, which  encodes the prompt text and documents' text into vectors, and searches for top-k documents whose embeddings are most relevant to the prompt. 
% The application then concatenates the retrieved documents with the user query as the context to the LLMs.
% \sid{GPT cache caches direct results, Cachegen is more generic. Title: Other uses of cache in LLM}
% The LLM then process the concatenated contexts with \textit{cross-attention} module~\cite{lewis2021retrievalaugmented,shi2023replug,li2022decoupled, wang2023zemi, retro, chen2021open, atlas, ye2023tram}.
% This module allows the questions to attend to all the retrieved documents without allowing the retrieved documents to attend to each other.

% It is important to note that the delay to search for relevant documents is marginal compared to the LLM inference delay~\cite{li2022decoupled, zhang2023hybrid}.
% To put this into perspective, recent studies~\cite{zhang2023hybrid, li2022decoupled} have shown that the retrieval step typically constitutes only 1-3\% of the delay in generating the LLM's first token, not to mention the loading delay of  the KV cache. 
% Thus, in our work, we exclude the retrieval delay from the TTFT.

\mypara{Alternative caching in LLM systems}
Recent developments in LLMs have led to applications that cache the query's generated answers to reduce repetitive query costs~\cite{ZillizTech2023, Martinez2023}. While caching answers of queries is useful for reuse, \name provides a generic and flexible way to incorporate context reuse and can generate more specific answers by optimally reusing shared contexts.


% Another line of research 
% % explores 
% % vector databases, designed to store high-dimensional vectors efficiently and enable vector-based queries~\cite{milvus, Elastic2023, li2019design, analyticdb}. 
% % Recent developments in LLMs have led to 
% develops applications that cache query results from LLMs to reduce repetitive query costs~\cite{ZillizTech2023, Martinez2023}.
% These applications convert user queries previously submitted by a user into \textit{semantic embeddings}, which are DNN features\footnote{The semantic embeddings are either extracted via open-source LLMs or OpenAI embedding API. } that represent the semantic meaning. 
% The applications then store them 
% % store previously submitted query semantic embeddings\jc{this seems an important term. what IS the semantic embedding of a query? and is there an embedding of each document or segment in the background database? how are these embeddings typically generated?} 
% in vector databases~\cite{milvus, FacebookEngineering2017, malkov2018efficient, Pgvector2023}, which are designed to store high-dimensional vectors and enable vector-based queries. 
% When queries with similar semantic embeddings come, cached answers are retrieved to reduce latency.
% These works are complementary to us, as they focus on enabling the efficient storage and retrieval of the cached vectors, usually the semantic embeddings of the queries, not the KV cache, while \name focuses on reducing the bandwidth usage needed to transfer the KV cache.
% % For example, \cite{milvus, Elastic2023, li2019design, analyticdb} build  vector data management systems
% % for large-scale distributed AI applications, which is able to quickly query or update the database with dynamic data. 
% % \jc{again, it's important to clarify that the search delay in these retrieval applications is being optimized by these applications and thus are not considered in TTFT. To strengthen this argument, can we cite some concrete numbers and say the search delay is much shorter than the TTFT, especially when the context is long?}

% }

% diff: we use KV feature





==> backups/related-works-v2_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US

\section{Related work}
\label{sec:related}

\mypara{Faster LLM serving}
Recent efforts in LLM systems research aim at either at speeding up LLM training~\cite{deepspeed, shoeybi2019megatron} or making the LLM serving systems faster. Different ways include parallelizing the generation of multiple tokens with smaller approximating models~\cite{Leviathan2022FastIF, miao2023specinfer}, accelerating the inference of Mix-of-Expert LLMs on edge devices~\cite{yi2023edgemoe}, quantizing LLM model weights~\cite{aminabadi2022deepspeed}, reducing memory I/O of GPU on-chip SRAM~\cite{dao2022flashattention}, and reducing self-attention computation complexity by k-means~\cite{roy2021efficient}. 
New LLM service scheduling strategies are proposed in ~\cite{wu2023fast,orca} along with more efficient GPU memory utilization in~\cite{vllm}.

A common approach for faster inference without modifying the LLMs is by {\em caching the KV} of previously used inputs for {\em one} LLM query~\cite{wu2023fast,flexgen,li2022decoupled, dai*2019transformerxl, ott2019fairseq, zhang2023ho, scissorhand, pope2022efficiently, miao2023specinfer, wolf-etal-2020-transformers}. 
However \name benefits by storing multiple KV caches (which might be commonly used) on a separate server and transmits them in a bandwidth-efficient way over the network for {\em reuse across  multiple} LLM queries.

% The landscape of LLM systems research is fast evolving.
% Besides speeding up LLM training (\eg~\cite{deepspeed, shoeybi2019megatron}), many recent efforts, including ours, focus on the LLM serving systems. 
% Some try to parallelize the generation of multiple tokens with smaller approximating models~\cite{Leviathan2022FastIF, miao2023specinfer} and accelerate the inference of Mix-of-Expert LLMs on edge devices~\cite{yi2023edgemoe}. 
% Others quantize LLM model weights (\eg~\cite{aminabadi2022deepspeed}), reduce memory I/O of GPU on-chip SRAM~\cite{dao2022flashattention}, and reduce self-attention computation complexity by k-means~\cite{roy2021efficient}. 
% New scheduling strategies are also proposed for LLM services~\cite{wu2023fast,orca} along with more efficient GPU memory utilization~\cite{vllm}.
% Nonetheless, a common approach to speeding up without modifying the LLMs is by {\em caching KV} cache of repeatedly used input sequences, such as contexts~\cite{wu2023fast,flexgen,li2022decoupled, dai*2019transformerxl, ott2019fairseq, zhang2023ho, scissorhand, pope2022efficiently, miao2023specinfer, wolf-etal-2020-transformers}. 
% However, caching KV cache results in a dramatically increased amount of cached data, which requires a bandwidth-efficient KV/context-loading system like \name.



% many works. change models, etc. kv cache is common, but more data need to be loaded
% kv cache
% smaller models
% sim: also use kv
% diff: doesn't optimize loading


\mypara{Longer LLM inputs (contexts)}
While benefits of long contexts are still under scrutiny~\cite{liu2023lost,sun2021longrange, roy2021efficient}, many recent efforts aim at enabling LLMs to process very long contexts~\cite{xu2024retrieval}.
% , under the premise that longer contexts improve generation quality (\eg~\cite{wu2022memorizing,dai*2019transformerxl}).
The main challenge is fitting the corresponding larger attention matrices of longer contexts into limited GPU memory. 
Processing longer input sequences is enabled by
offloading less used parts of the attention matrices~\cite{flexgen},
using external knowledge via KNN~\cite{wu2022memorizing}, approximating via 
retraining self-attention to only attend to top-k keys~\cite{bertsch2023unlimiformer,ainslie2020etc}, 
mapping long inputs into smaller latent spaces~\cite{pmlr-v162-hawthorne22a} and using local windowed~\cite{beltagy2020longformer}, dilated~\cite{ding2023longnet} or sparse~\cite{zaheer2021big} attention to scale to input lengths of $\sim$1 billion tokens.
These longer inputs (contexts) inflate the KV cache, and \name complements these efforts by enabling fast remote loading of the KV cache.

% While benefits of longer contexts are still under scrutiny~\cite{liu2023lost,sun2021longrange, roy2021efficient}, many recent efforts aim at enabling LLMs to accept even {\em longer} contexts~\cite{xu2024retrieval}.
% % , under the premise that longer contexts improve generation quality (\eg~\cite{wu2022memorizing,dai*2019transformerxl}).
% The main challenge is to hold the attention matrices of more tokens without needing a bigger GPU memory. 
% They enable longer input sequences by
% dynamically offloading less used parts of the attention matrices~\cite{flexgen},
% using external knowledge via KNN~\cite{wu2022memorizing}, 
% retraining the self-attention module to only attend to top-k keys to approximate the full attention~\cite{bertsch2023unlimiformer,ainslie2020etc}, 
% mapping long inputs into smaller latent space~\cite{pmlr-v162-hawthorne22a}, 
% using local windowed self-attention~\cite{beltagy2020longformer}, 
% or 
% using dilated attention~\cite{ding2023longnet} or sparse attention~\cite{zaheer2021big} to scale the input length to even 1 billion tokens.
% However, the longer inputs (contexts) also inflate the KV cache, and this work complements these efforts by focusing on fast remote loading of KV cache.


% moreover, contexts are longer. stretching the limit of gpu mem. causing even bigger kv features.
% increase context length
% memory compression
% sim: inspire longer context
% diff: doesn't optimize loading

\mypara{Context shortening/pruning}
A lot of emerging literature on shortening and pruning long contexts relates well to \name. These efforts aim to select the most important text segments and prune the rest to reduce context length. Methods for this can be based on the similarity between the user query and the potentially relevant documents ~\cite{retro}. Dropping tokens that are less attended to by the current prompt is done in ~\cite{scissorhand, zhang2023ho}. This can be done by identifying a smaller subset of {\em heavy hitter} tokens which contribute most to the overall attention scores~\cite{ge2023model}. Using  query-aware compression with document reordering to reduce loss-in-the-middle, is another recent method proposed to shorten context lengths~\cite{jiang2023longllmlingua}. Approximating attention scores using a subset of query and key vector components allows for only fetching the most relevant tokens and reduces memory traffic~\cite{ribar2023sparq}. 

One limitation of all these methods are that they need to know the query else they risk dropping/missing potentially important tokens. Choosing the right compression ratio is also hard, many models already show quality degradation at 2$x$ compressed length~\cite{ribar2023sparq} Finally, some works retrain LLM models to directly take in contexts that are rewritten by gisting~\cite{gisting} or auto-encoding~\cite{autoencoder-incontext}.

\name differs from the above by compressing the KV cache into bitstreams, rather than shortening the context in its original form (i.e., text or tensor) and fetching the compressed KV cache efficiently. \name's KV compression does not need to know the query/prompt and it doesn't risk quality loss from dropping potentially important tokens. It allows for better compression rates by leveraging unique distributional properties of KV cache and achieves better delay-quality trade-offs than existing context compressors (\S\ref{subsec:eval:micro}). Finally \name does not need to re-train the LLM.

% \sid{Don't emphasise the following para.}
%  Different from them, 
% %Second, \name minimizes the sum of network delay to transfer the KV cache and the computation delay, rather than only the computation delay.
% %Moreover, unlike~\cite{scissorhand,borgeaud2022improving}, \name's KV compression does not need to know the query (prompt), and 
% \name does not need to train a new LLM model and also achieves better compression rate with
% less information loss by leveraging unique distributional properties of KV cache.
% %to rewrite contexts, like in~\cite{gisting,in-context-autoencoder}.
% Finally, we show \name achieves better delay-quality tradeoffs than existing context compressors (\S\ref{subsec:eval:micro}).
% and can potentially be combined with them to further improve the delay-quality tradeoffs.

% More relevant to our work is the emerging literature on shortening and pruning long contexts. 
% These efforts select the most important text segments and prune out the others to reduce context length, based on the similarity between the user query and the potentially relevant documents (\eg~\cite{retro}), 
% drop tokens that are less attended to by the current prompt~\cite{scissorhand, zhang2023ho, ge2023model} or use query-aware compression with document reordering to reduce loss-in-the-middle~\cite{jiang2023longllmlingua}.

% Different from them, \name compresses the KV cache into bitstreams, rather than shortening the context in its original form (i.e., text or tensor). 
% Unlike~\cite{scissorhand, retro, zhang2023ho,jiang2023longllmlingua}, \name's KV compression does not need to know the query/prompt. 

% \sid{Don't emphasise the following para.}
% Recently, some work retrains LLM models to directly take in contexts that are
% rewritten by gisting~\cite{gisting} or auto-encoding
% ~\cite{autoencoder-incontext}. Different from them, 
% %Second, \name minimizes the sum of network delay to transfer the KV cache and the computation delay, rather than only the computation delay.
% %Moreover, unlike~\cite{scissorhand,borgeaud2022improving}, \name's KV compression does not need to know the query (prompt), and 
% \name does not need to train a new LLM model and also achieves better compression rate with
% less information loss by leveraging unique distributional properties of KV cache.
% %to rewrite contexts, like in~\cite{gisting,in-context-autoencoder}.
% Finally, we show \name achieves better delay-quality tradeoffs than existing context compressors (\S\ref{subsec:eval:micro}).
% and can potentially be combined with them to further improve the delay-quality tradeoffs.

% one common approach is to shorten context, but dropping tokens or rewriting or better doc selection.
% diff: we compress KV cache

\mypara{Tensor compression}
\name's KV encoder can be seen as a special tensor compression technique tailored for LLM's KV caches.
General tensor compression has been intensively studied, \eg relaxing rank and ordering constraint~\cite{zhao2016tensor} or decomposing large tensors into products of smaller ones~\cite{tensor_decomp}.
In DNN training, tensor compression has been used to compress gradient updates of DNN weights (\eg~\cite{espresso,MLSYS2022_773862fc,agarwal2020accordion}).
However KV caches and gradients have very different properties.
These training systems often leverage the sparsity of gradient updates which occurs due to methods like~\cite{chen2023sparse, zehui2019dropattention, child2019generating}. However the KV cache is not known to be sparse in general.
% to strike a balance between compression efficiency and loss of accuracy.
% \yh{Gradient compression: Three major schemes:
% (1) quantization based SignSGD; (2) low-rank decomposition based PowerSGD (3) Sparsification based Top-K. 
% The assumptions under those schemes are that the gradient to be updated is sparse. Which is not the case in \kv. 
% Also, 
% Note that in popular distributed training 
% \cite{agarwal2020accordion}  }

% \jc{the title may be a bit misleading. should we call it ``Retrieval-augmented generation''?}

\mypara{Retrieval-augmented generation}
A wide range of works ~\cite{retro, atlas, fid,rubin2023long,lewis2020retrieval,Yang_2019, karpukhin2020dense, wang2023zemi, ram2023incontext} focus on optimizing retrieval-augmented generation (RAG). Retrieval-augmented generation includes retrieving relevant documents to the user's question, by comparing the question with documents in the database via vector based~\cite{chen2017reading, Yang_2019, nie2019revealing} or DNN-based~\cite{lewis2020retrieval, karpukhin2020dense,xiong-etal-2021-progressively, reranking} similarity search algorithms. The retrieved documents are fed as the context to the LLMs to generate the answers to the question.

We envision RAG as a fitting use case for \name, as many LLM inference platforms support feeding in the KV cache as retrieved context instead of text documents~\cite{hf2020, Chase_LangChain_2022}. Relevant KV cache can be retrieved using similarity based searching as mentioned above.
Optimal methods on which KV cache to reuse in RAG (to generate the best output) is still an open area, though some works have attempted to define a systematic way to choose them~\cite{gim2023prompt}.

% \edit{\mypara{Retrieval-augmented generation} A wide range of works
% %~\cite{retro, atlas, fid,rubin2023long,lewis2020retrieval,Yang_2019, karpukhin2020dense,xiong-etal-2021-progressively, reranking, shi2023replug,li2022decoupled, wang2023zemi}
% ~\cite{retro, atlas, fid,rubin2023long,lewis2020retrieval,Yang_2019, karpukhin2020dense, wang2023zemi, ram2023incontext}
% focus on optimizing retrieval-augmented generation. 
% The workflow of retrieval-augmented generation includes retrieving relevant documents to the user's question, and feeding the retrieved documents as the context to the LLMs to generate the answers to the question.
% Upon receiving a question submitted by the user, the application decides the relevant documents by comparing the question with documents in the database via similarity search algorithms, such as dense or sparse vector methods~\cite{chen2017reading, Yang_2019, nie2019revealing} and DNN-based schemes~\cite{lewis2020retrieval, karpukhin2020dense,xiong-etal-2021-progressively, reranking}.
% For example, FiD~\cite{fid} represents the prompt text and the documents' text in the form of ``bag of words'' and ranks the relevance of the documents with the term frequency-inverse document frequence (TF-IDF).
% As another example, Atlas~\cite{atlas} pre-trains a BERT-based retriever, which  encodes the prompt text and documents' text into vectors, and searches for top-k documents whose embeddings are most relevant to the prompt. 
% The application then concatenates the retrieved documents with the user query as the context to the LLMs.
% \sid{GPT cache caches direct results, Cachegen is more generic. Title: Other uses of cache in LLM}
% The LLM then process the concatenated contexts with \textit{cross-attention} module~\cite{lewis2021retrievalaugmented,shi2023replug,li2022decoupled, wang2023zemi, retro, chen2021open, atlas, ye2023tram}.
% This module allows the questions to attend to all the retrieved documents without allowing the retrieved documents to attend to each other.

% It is important to note that the delay to search for relevant documents is marginal compared to the LLM inference delay~\cite{li2022decoupled, zhang2023hybrid}.
% To put this into perspective, recent studies~\cite{zhang2023hybrid, li2022decoupled} have shown that the retrieval step typically constitutes only 1-3\% of the delay in generating the LLM's first token, not to mention the loading delay of  the KV cache. 
% Thus, in our work, we exclude the retrieval delay from the TTFT.

\mypara{Alternative caching in LLM systems}
Recent developments in LLMs have led to applications that cache the query's generated answers to reduce repetitive query costs~\cite{ZillizTech2023, Martinez2023}. While caching answers of queries is useful for reuse, \name provides a generic and flexible way to incorporate context reuse and can generate more specific answers by optimally reusing shared contexts.


% Another line of research 
% % explores 
% % vector databases, designed to store high-dimensional vectors efficiently and enable vector-based queries~\cite{milvus, Elastic2023, li2019design, analyticdb}. 
% % Recent developments in LLMs have led to 
% develops applications that cache query results from LLMs to reduce repetitive query costs~\cite{ZillizTech2023, Martinez2023}.
% These applications convert user queries previously submitted by a user into \textit{semantic embeddings}, which are DNN features\footnote{The semantic embeddings are either extracted via open-source LLMs or OpenAI embedding API. } that represent the semantic meaning. 
% The applications then store them 
% % store previously submitted query semantic embeddings\jc{this seems an important term. what IS the semantic embedding of a query? and is there an embedding of each document or segment in the background database? how are these embeddings typically generated?} 
% in vector databases~\cite{milvus, FacebookEngineering2017, malkov2018efficient, Pgvector2023}, which are designed to store high-dimensional vectors and enable vector-based queries. 
% When queries with similar semantic embeddings come, cached answers are retrieved to reduce latency.
% These works are complementary to us, as they focus on enabling the efficient storage and retrieval of the cached vectors, usually the semantic embeddings of the queries, not the KV cache, while \name focuses on reducing the bandwidth usage needed to transfer the KV cache.
% % For example, \cite{milvus, Elastic2023, li2019design, analyticdb} build  vector data management systems
% % for large-scale distributed AI applications, which is able to quickly query or update the database with dynamic data. 
% % \jc{again, it's important to clarify that the search delay in these retrieval applications is being optimized by these applications and thus are not considered in TTFT. To strengthen this argument, can we cite some concrete numbers and say the search delay is much shorter than the TTFT, especially when the context is long?}

% }

% diff: we use KV feature





==> backups/related_works-v1.tex <==
% \begin{itemize}
%     \item Related works on profiling Transformer-based generative models
%     \begin{itemize}
%         \item Papers: ~\cite{kim2023stack, FasterTransformer, pope2022efficiently, dao2022flashattention, narayanan2023cheaply}
%         \item Limitations: they did not show how inference delay changes with different impact factors or did not perform evaluation on different generative tasks other than text generation

%     \end{itemize}
% \end{itemize}

% % definition of delay budget: 
% % 1. w/ caching 
% % 2. User tolerable delay budget constant
\section{Related works}

\mypara{LLMs inference/training speedup} Many works have been focusing on speeding up LLM inference. 
\begin{itemize}
    \item \cite{Leviathan2022FastIF, miao2023specinfer}: Generating several tokens concurrently with approximating models. This can paralleize the generation of multiple tokens 
    \item \cite{deepspeed, shoeybi2019megatron}: provides the distributed training frameworks for scaling up LLM training. 
    \item \cite{aminabadi2022deepspeed}: improves LLM inference throughput by weight quantization and \kv offloading. 
    \item \cite{flexgen}: applies offloading to enable LLM inference on a single GPU.
    \item \cite{yi2023edgemoe}: reduces memory usage of mixture-of-expert(MoE) LLMs, and accelerates the inference of MoE LLMs on edge devices. 
\end{itemize}

\mypara{Compressing LLMs} 
\begin{itemize}
\item augmenting the memory for better generation quality:
\begin{itemize}
    \item \cite{wu2022memorizing}: Augments LLM's memory with external knowledge via KNN. Shows longer contexts improve generation quality 
    \item \cite{dai*2019transformerxl}: Enlarges LLM's memory and shows that it improves perplexity
    \item \cite{bertsch2023unlimiformer}: Only attend to top-k keys to enlarge LLM memory to approximate the full attention, and improves quality 
    \item \cite{pmlr-v162-hawthorne22a}: maps the total input into smaller latent to attend to, so as to enable the capture of long context.
    \item \cite{ding2023longnet}: uses dilated attention to enable the scaling of input length to 1 billion tokens. 
\end{itemize}
\item reduces compute complexity of self-attention: 
\begin{itemize}
    \item \cite{dao2022flashattention}: speedup self-attention computation delay by reducing the number of memory reads or writes between GPU high bandwidth memory (HBM) and GPU on-chip SRAM.
    \item \cite{roy2021efficient}: use k-means to reducing the complexity of self-attention
    \item \cite{beltagy2020longformer}: enables long sequence input by using a local windowed self-attention to reduce computation complexity 
    \item \cite{ainslie2020etc}: Redesign the self-attention module and retrain it so as it only attends to part of the tokens. 
    \item \cite{zaheer2021big}: Uses sparse attention to reduce the complexity of self attention, also needs retraining. 
\end{itemize}
\end{itemize}

% \mypara{Enlarging LLMs token limit}

\mypara{Retrieval-based generation }
\begin{itemize} 
    \item \cite{borgeaud2022improving}: enhances LLMs from a large database based on similarity between user query and documents in the database. 
    \item \cite{li2022decoupled}: Proposes decoupling the encoding of context documents and cross-attention between the query and context. 
    \item \cite{}
\end{itemize}

\mypara{Generic tensor compression}
\begin{itemize}
    \item \cite{bernstein2018signsgd}: 
    % \item \cite{yin2021tt}: 
    \item \cite{zhao2016tensor}: Generalizes Tensor train model by relaxing rank, ordering constraint and making model symmetric to attain better accuracy.
    \item \cite{tensor_decomp}: proposes methods to decompose a bigger tensor into products of small tensors. 
    \item \cite{espresso}: efficiently selects gradient compression strategy and communication strategy in distributed training. 
    \item \cite{MLSYS2022_773862fc}: studies when different gradient compression methods, such as sparsification, low-rank, will achieve faster training time. 
    \item \cite{agarwal2020accordion}: studies the accuracy and delay trade-offs of different compression ratios of different gradient compression techniques, and  develops a adaptive gradient compression configuration selection method. 
\end{itemize}
Summary: these techniques do not assume any model or task specific knowledge. Applies the same kinds of compression techniques for all types of models. \hc{However the accuracy after naively applying them are very low. We leave the work to adopt these methods to save size while preserving accuracy to future work.}

==> backups/related_works-v1_2.tex <==
% \begin{itemize}
%     \item Related works on profiling Transformer-based generative models
%     \begin{itemize}
%         \item Papers: ~\cite{kim2023stack, FasterTransformer, pope2022efficiently, dao2022flashattention, narayanan2023cheaply}
%         \item Limitations: they did not show how inference delay changes with different impact factors or did not perform evaluation on different generative tasks other than text generation

%     \end{itemize}
% \end{itemize}

% % definition of delay budget: 
% % 1. w/ caching 
% % 2. User tolerable delay budget constant
\section{Related works}

\mypara{LLMs inference/training speedup} Many works have been focusing on speeding up LLM inference. 
\begin{itemize}
    \item \cite{Leviathan2022FastIF, miao2023specinfer}: Generating several tokens concurrently with approximating models. This can paralleize the generation of multiple tokens 
    \item \cite{deepspeed, shoeybi2019megatron}: provides the distributed training frameworks for scaling up LLM training. 
    \item \cite{aminabadi2022deepspeed}: improves LLM inference throughput by weight quantization and \kv offloading. 
    \item \cite{flexgen}: applies offloading to enable LLM inference on a single GPU.
    \item \cite{yi2023edgemoe}: reduces memory usage of mixture-of-expert(MoE) LLMs, and accelerates the inference of MoE LLMs on edge devices. 
\end{itemize}

\mypara{Compressing LLMs} 
\begin{itemize}
\item augmenting the memory for better generation quality:
\begin{itemize}
    \item \cite{wu2022memorizing}: Augments LLM's memory with external knowledge via KNN. Shows longer contexts improve generation quality 
    \item \cite{dai*2019transformerxl}: Enlarges LLM's memory and shows that it improves perplexity
    \item \cite{bertsch2023unlimiformer}: Only attend to top-k keys to enlarge LLM memory to approximate the full attention, and improves quality 
    \item \cite{pmlr-v162-hawthorne22a}: maps the total input into smaller latent to attend to, so as to enable the capture of long context.
    \item \cite{ding2023longnet}: uses dilated attention to enable the scaling of input length to 1 billion tokens. 
\end{itemize}
\item reduces compute complexity of self-attention: 
\begin{itemize}
    \item \cite{dao2022flashattention}: speedup self-attention computation delay by reducing the number of memory reads or writes between GPU high bandwidth memory (HBM) and GPU on-chip SRAM.
    \item \cite{roy2021efficient}: use k-means to reducing the complexity of self-attention
    \item \cite{beltagy2020longformer}: enables long sequence input by using a local windowed self-attention to reduce computation complexity 
    \item \cite{ainslie2020etc}: Redesign the self-attention module and retrain it so as it only attends to part of the tokens. 
    \item \cite{zaheer2021big}: Uses sparse attention to reduce the complexity of self attention, also needs retraining. 
\end{itemize}
\end{itemize}

% \mypara{Enlarging LLMs token limit}

\mypara{Retrieval-based generation }
\begin{itemize} 
    \item \cite{borgeaud2022improving}: enhances LLMs from a large database based on similarity between user query and documents in the database. 
    \item \cite{li2022decoupled}: Proposes decoupling the encoding of context documents and cross-attention between the query and context. 
    \item \cite{}
\end{itemize}

\mypara{Generic tensor compression}
\begin{itemize}
    \item \cite{bernstein2018signsgd}: 
    % \item \cite{yin2021tt}: 
    \item \cite{zhao2016tensor}: Generalizes Tensor train model by relaxing rank, ordering constraint and making model symmetric to attain better accuracy.
    \item \cite{tensor_decomp}: proposes methods to decompose a bigger tensor into products of small tensors. 
    \item \cite{espresso}: efficiently selects gradient compression strategy and communication strategy in distributed training. 
    \item \cite{MLSYS2022_773862fc}: studies when different gradient compression methods, such as sparsification, low-rank, will achieve faster training time. 
    \item \cite{agarwal2020accordion}: studies the accuracy and delay trade-offs of different compression ratios of different gradient compression techniques, and  develops a adaptive gradient compression configuration selection method. 
\end{itemize}
Summary: these techniques do not assume any model or task specific knowledge. Applies the same kinds of compression techniques for all types of models. \hc{However the accuracy after naively applying them are very low. We leave the work to adopt these methods to save size while preserving accuracy to future work.}

==> backups/sec-abstract.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


\begin{abstract}


As large language models (LLMs) take on complex tasks, their inputs are supplemented with {\em longer contexts} that incorporate domain knowledge or user-specific information.
Yet using long contexts poses a challenge for responsive LLM systems, as nothing can be generated
until the whole context is processed by the LLM. 
While the context-processing delay can be reduced by reusing the KV cache of a context across different inputs, fetching the KV cache, which contains large tensors, over the network can cause high extra network delays.


\name is a fast context-loading module for LLM systems.
First, \name uses a custom tensor encoder, which leverages KV cache's distributional properties
%, such as locality across tokens, 
to {\em encode}  a KV cache into more compact bitstream representations with negligible encoding/decoding overhead.
This reduces the bandwidth demand to fetch the KV cache.
Second, to maintain low context-loading delay and high generation quality, \name{ }{\em adapts} the streaming strategies to cope with changes in available bandwidth.
When available bandwidth drops, \name may raise the compression level for a part of the context or choose to recompute its KV cache on the fly. 
We test \name on three popular LLMs of various sizes and four datasets (662 contexts in total).
Our code is publicly available at: \href{https://github.com/UChi-JCL/CacheGen}{\textbf{https://github.com/UChi-JCL/CacheGen}}. 

\end{abstract}


%This paper presents \name to minimize the total delay in fetching \emph{and} processing contexts for LLMs.
%\name uses two ideas.
%First, it greatly reduces the bandwidth needed for transmitting KV cache by a novel encoder that compresses KV cache into more compact bitstream representations.
%% \name reduces the bandwidth needed for transmitting long contexts' KV cache through a novel encoder that compresses KV cache into more compact bitstream representations.
%Our encoder of KV cache combines adaptive quantization with a tailored arithmetic coder, taking advantage of the distributional properties of KV cache, such as locality across tokens.
%Second, to cope with the temporal variance of network throughput, \name splits contexts into {\em token chunks} and stores the KV cache of each chunk at multiple compression levels with various quality-size tradeoffs. 
%\name then uses a custom adaptation logic to determine, for each token chunk, in which compression level it should be fetched or whether the throughput is too low and it is faster to compute the KV cache on the fly.
%We test \name on three models of various sizes and three datasets of different context lengths.
%Compared to recent methods that handle long contexts, \name reduces bandwidth usage by 3.7-4.3$\times$ and the {\em total} delay in fetching and processing contexts by 2.7-3$\times$ while maintaining almost the same LLM response quality on various tasks as loading the text contexts.


% and uses an adaptation logic to dynamically determine, for each KV chunk, which the compression level should it be 
% Furthermore, \name minimizes the {\em total} delay in fetching and processing a context by using
% % rather than separately, 
% % while maintaining a high LLM performance on various tasks.
% % a high generation quality.
% %of the network delay and computation delay 
% a controller that determines when to load the context as compressed KV features or raw text and picks the appropriate compression level if loaded as KV features.
%based on the context length.
% \shan{What does this last sentence mean? Does ``performance'' here mean accuracy or throughput/latency or something else?}
% similar quality of generated response.
% Compared to the state-of-the-art methods for handling long context (\eg quantization and token selection), \name reduces 
% \shan{is it similar as text-context baseline or similar as quantization-based prior work?}
% while achieving the same generation quality in perplexity or accuracy.

==> backups/sec-eval-0304.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US
\input{fig-e2e-longchat}
\input{fig-e2e-70b}

\tightsection{Evaluation}

Our evaluation answers the following key questions:

%\begin{itemize}
    %\item 
    1) Given a context, how much can \name's KV encoder reduce the bandwidth needed to transfer its KV cache? 
    %\item % Given a network bandwidth, 
    2) How much can \name reduce TTFT (including both network and compute delays)? 
    %\item 
    3) How sensitive is \name's performance gain to the workload, including different context lengths, network bandwidths, and the number of concurrent requests?
    % and the ratio of available GPU cycles? 
    %\item 
    4) How much is \name's decoding overhead in terms of compute and delay? 
    % \item Does \name have a better tradeoff between LLM performance and TTFT than baselines that reduce TTFT by pruning the contexts or using smaller models?
    
    % \jc{the items blow dont seem high priority?}
    % \item How much runtime memory usage does \name reduce? 
    % \item What's the overhead of \name?
    % \item How much does each of the components of \name contribute to the total improvement? 
%    \item How generalizable is \name's compressor? 
%\end{itemize}




% \begin{figure*}[t]
% \centering
%     \includegraphics[width=.92\textwidth]{figs/sensitivity_all.pdf}
%     \vspace{-0.2cm}
%     \tightcaption{Sensitivity of \name's gains over the baseline across different token lengths, network bandwidths, and models.}
%     \label{fig:sensitivity}
% \end{figure*}
\tightsubsection{Setup}
\label{subsec:evalsetup}


\mypara{Models} We evaluate \name on four models of different sizes, specifically the fine-tuned versions of Llama-7B, Llama-13B, Llama-33B, Llama-70B. 
All models are fine-tuned such that they can take long contexts (up to 32K). 
We did not test \name on other LLMs (\eg OPT, BLOOM) because there are no public fine-tuned versions for long contexts to our best knowledge. 

\mypara{Datasets}
We evaluate \name on 662 contexts from four different datasets with different tasks (Table~\ref{tab:datasets}): 
% \ga{Call out the number of queries, size of dataset etc. to impress upon the large scale of evaluation. }
\begin{packeditemize}
    \item {\em LongChat:} The task is recently released~\cite{longchat2023} to test LLMs on queries like ``What was the first topic we discussed?'' by using all the previous conversations as the context.  
    Most contexts are around 9-9.6K tokens. 
    \item {\em TriviaQA:} The task tests the reading comprehension ability of the LLMs~\cite{bai2023longbench}, by giving the LLMs a single document (context), and letting it answer questions based on it. The dataset is part of the LongBench benchmark~\cite{bai2023longbench} suite. 
    \item {\em NarrativeQA:} The task is used to let LLMs answer questions based on stories or scripts, provided as a single document (context).
    The dataset is also part of LongBench.
    \item {\em Wikitext:} The task is to predict the probability of the next token in a sequence based on the context consisting of relevant documents that belong to a specific Wiki page~\cite{wikitext}.
\end{packeditemize}

\input{tab-1}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}



%\begin{table}[]
%\begin{tabular}{cccc}
%\hline
%  & Dataset          & Model(s)                                                                               & Quality metric \\ \hline\hline
%A & LongChat         & longchat-7B-16k                                                                        & Accuracy       \\ \hline
%B & NaturalQuestions & T5-large                                                                               & F1 score       \\ \hline
%C & Wikitext         & \begin{tabular}[c]{@{}c@{}}LLaMA-13B\\ LLaMA-7B\end{tabular} & Perplexity     \\ \hline
%\end{tabular}
%\caption{}
%\label{tab:my-table}
%\end{table}

% \mypara{Generation quality metric}
\mypara{Quality metrics}
We measure generation quality using the standard metric of each dataset.
\begin{packeditemize}

% \item {\em Perplexity} is used to evaluate the model's performance on the Wikitext dataset. 
% The perplexity is defined as the exponentiated average negative log-likelihood of the next token~\cite{ppl1, ppl2}.
% A low perplexity means the model likely generates the right next token.
% While perplexity does not equate to text-generation quality, it is widely used as a decent proxy~\cite{adiwardana2020humanlike}.
% This metric has been commonly used by prior works to test the impact of pruning or quantizing LLMs on generation performance~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% % widely used in previous works in evaluating whether shrinking the model size or quantizing models degrade the generation quality~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% % \jc{this metric may not sound intuitive to system reviewers. add some citations and explain why we should care about it?}

\item {\em Accuracy} is used to evaluate the model's output on the LongChat dataset. 
The task predicts the first topic in the conversational history between the user and the LLM. 
The accuracy is defined as the percentage of generated answers that exactly includes the ground-truth topic. % It is defined as the percentage of the generated answer that matches the ground-truth first topic of the conversation.
% \jc{Yuhan, please add some details and explain why it is a good metric}

\item {\em F1 score} is used to evaluate the model's response in the TriviaQA and NarrativeQA datasets.
It measures the probability that the generated answer matches the ground-truth answer of the question-answering task.
\item {\em Perplexity} is used to evaluate the model's performance on the Wikitext dataset. 
The perplexity is defined as the exponentiated average negative log-likelihood of the next token~\cite{ppl1, ppl2}.
A low perplexity means that the model likely generates the next token correctly.
While perplexity does not equate to text-generation quality, it is widely used as a proxy~\cite{adiwardana2020humanlike} 
% This metric has been commonly used by prior works 
to test the impact of pruning or quantizing LLMs on generation performance~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
\end{packeditemize}

\input{fig-h2o}


\mypara{Baselines} 
We compare \name with baselines that do not change the contexts or model (more baselines in \S\ref{subsec:eval:micro}). 
\begin{itemize}
% \item \code{torch.save}: 
% \item {\em ``Original KV''} uses \texttt{torch.save} to serialize the KV features in GPU memory to a file.
% This serves as a reference for the most straightforward implementation. 
% \item {\em ``Default quantization \& AC''} combines the uniform quantization of KV features~\cite{flexgen} with the default arithmetic coding (AC) that uses a global probability distribution for all elements.
% Like \name, this baseline also uses quantization and AC but with a simpler design on each component. 
\item {\em ``Default quantization''} uses the uniform quantization of KV cache, specifically the same quantization level for every layer in the LLM (which was used in~\cite{flexgen}). 
\item {\em ``Text context''} fetches the text of the context and feeds it to LLM to generate the KV cache for it. 
It represents the design of minimizing data transmission but at the expense of high computation overhead. %, especially under long contexts.
\item {\em ``Context compression''} either drops tokens in the text context (LLMlingua~\cite{jiang2023longllmlingua}) or in the KV cache (H2O~\cite{zhang2023h2o}). 

    % \item \recomp: This scheme sends the texts of the context and compute the \kv based on the texts before generating the first token. 
    % % \item Model quantization baseline: This scheme quantizes the model weights into less number of bits in order to reduce the memory usage at inference time~\cite{??, ??, ??}. For this scheme, we report the quality metrics after applying the model quantization. 
    % % For the size metrics, we report the size of the key-value caches saved by \code{torch.save}.
    % % \item Original models with shorter contexts: This scheme rewrites the contexts with gisting~\cite{??}, and generates the first token with the compressed contexts. \yh{Say a few sentences about the pretrained gisting models only allow us to test on specific models and datasets}
    % \item \kv quantization + \code{torch.save}: This scheme quantizes the key-value cache, and saves the compressed \kv via \code{torch.save}. 
    % \item \kv quantization + naive AC: This scheme quantizes the key-value cache, and saves the compressed \kv via naive AC (\ie no optimization on the grouping of \kv to improve compression ratio). 
    % % \item Smaller model architectures: This scheme approximates the line of work that uses smaller model architectures to reduce the memory footprint of LLMs~\cite{??, ??}. We compare \name's \kv with smaller models' \kv in terms of our metrics. 
    % \item \name (Ours): The orignal models with compressed \kv with \name's compressor and controller. 
\end{itemize}




\mypara{Hardware settings} We use an NVIDIA A40 GPU server with four GPUs to benchmark our results. 
The server is equipped with 384GB of memory and two Intel(R) Xeon(R) Gold 6130 CPUs with Hyper-threading and Turbo Boost enabled by default.
% The server is equipped with 64 Intel(R) Xeon(R) Gold 6130 CPU cores. 
% \yh{describe our CPU and GPU machines }




% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock2.pdf}
%     \tightcaption{Results on Size of KV cache } 
%     \label{fig:mock2}
% \end{figure*}



% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock1.pdf}
%     \tightcaption{Results on TTFT } 
%     \label{fig:mock1}
% \end{figure*}
% \input{fig-e2e-70b}
%


\extightsubsection{Overall improvement}
\label{subsec:overall_eval}

\mypara{TTFT reduction} 
Figure~\ref{fig:e2e-longchat}a and left part of Figure~\ref{fig:e2e-70b} demonstrate \name's ability to reduce TTFT, across four models and four datasets. Under bandwidth of 3~Gbps, 
\name reduces TTFT by 2.7-3.2$\times$ compared with the strongest baseline. (We test \name under varying of bandwidth in \S\ref{subsec:eval:sensitivity}.)
% \shan{This sentence sounds really odd. Can we delete it?}



It is important to note that even when the compression is lossless, specifically applying our AC on the KV cache after 8-bit quantization, \name can still reduce the TTFT by 1.67-1.81$\times$. 
\name's reduction in TTFT is a result of a shorter transmission delay to send the smaller KV caches.


% It is important to note that even under our 8-bit quantization pipeline with largest bitstream size, \name's encoded KV still reduces TTFT by \fillme $\times$ with no performance degradation. This shows that \name' is able to improve user experience with little cost.



\mypara{Reduction on KV cache size}
Figure~\ref{fig:e2e-longchat}b and Figure~\ref{fig:e2e-70b}b show that, across three datasets and four models, 
\name's KV encoder reduces the KV cache size by $3.7-4.3\times$ compared to the best baseline when achieving similar performance for downstream tasks after decoding. 
Thus, it achieves better quality-size trade-offs across different settings.
The degradation caused by lossy compression is marginal---the degradation is no more than 2\% in accuracy, less than 0.1\% in F1 score, and less than 0.1 in perplexity~\cite{huggingface_ppl}.
% in accuracy in Figure~\ref{fig:e2e-longchat} is less than 0.02, and the F1 Score decrease is below 0.1\%, it increases the perplexity by less than 0.1. 
Some example text outputs for different baselines are available in \S\ref{sec:appendix}. 


\input{fig-sens-bw}


% The next section will show more sensitivity tests. 


% This consistent improvement across these models and pipelines also indicate that \name is generally applicable to different model architectures and sizes. 

% Compared to the \recomp baseline, \name is able to reduce the TTFT because it 
% avoids the computation of the self-attention operation on the long context.

% \yh{Comments a bit on why \name can achieve smaller sizes compared to baselines}



\mypara{Gains over context compression}\name can compress any KV cache and is thus compatible with the recent context-compression techniques. 
To demonstrate this, we test \name's encoder on the KV cache produced by H2O~\cite{zhang2023h2o} and LLMlingua~\cite{jiang2023longllmlingua} for Llama-7B on 
the LongChat dataset. 
Figure~\ref{fig:h2o}a and Figure~\ref{fig:h2o}b shows that \name consistently improved TTFT over the quantization baseline by a factor of $2.8-3.7 \times$ without losing accuracy.
This suggests that after condensing contexts by H2O or LLMlingua, the resulting KV caches may still have the statistical observations behind \name's KV encoder.
Thus, the techniques used in \name's encoder remain beneficial when we encode the KV cache after applying these techniques.
Finally, we also compared LLMlingua directly with \name. 
As shown in Figure~\ref{fig:h2o}c, \name still outperforms LLMlingua by about 48\% in accuracy when reaching a similar delay. 







% We evaluate the ability 
% Figure~\ref{fig:adapt} shows how \name's controller adapts to changes of workloads when transmitting KV cache. 

% In figure~\ref{fig:adapt} illustrates a timeline of transmitting the KV cache for one piece of context. 
% To start with, \name's controller decides to transmit the compressed KV cache for the first \fillme layers. 
% At 2 seconds,
% the throughput suddenly drops from \fillme to \fillme. 
% After the throughput change is being reflected to the transmission server, \name's controller decides to transmit the text context and do the computation to generate the KV for subsequent \fillme layers.
% After 4 seconds, the throughput increases again from \fillme to \fillme, and \name's controller decides to switch back to transmit the KV cache for later layers. 
% Nevertheless, for the baseline that applies default quantization on the KV cache, it always sends the quantized version of KV cache without any adaptation, which leads to \fillme from 2 seconds to 4 seconds. 

% In figure~\ref{fig:adapt2}, we show how \name's controller adapts to different workloads change across time when transmitting different contexts. 
% We can see that due to the adaptation made by \name's controller, everytime when the workloads change in the middle of transmitting the context, the adaptation \name made further improves the gain of \name over the baseline. 



% \begin{figure}[t]
% \centering
%     \includegraphics[width=.5\textwidth]{figs/adaptation2.pdf}
%     \vspace{-0.2cm}
%     \tightcaption{\todo{Mock fig for now. replace with real!}}
%     \label{fig:adapt2}
% \end{figure}

% \vspace{-0.3cm}


\tightsubsection{Sensitivity analysis}
\label{subsec:eval:sensitivity}

\mypara{Available bandwidth} The left and right figures in Figure~\ref{fig:sensitivity-bw} compares the TTFT of \name with baselines under a wide range of bandwidth from 0.1--10 Gbps and 10--100 Gbps, while we fix the context length at 9.6K tokens. 
We can see that \name consistently outperforms baselines under almost all bandwidth situations. 
Arguably, the absolute reduction in TTFT becomes smaller under high bandwidth (over 20Gbps).
% However, the reduction of TTFT from \fillme~ms to \fillme~ms still makes a perceivable difference to human users who expect smooth interaction~\cite{??}.

\input{fig-sens-gpu-context-len}
\mypara{Number of concurrent requests}
Figure~\ref{fig:sensitivity-gpu}a shows the TTFT under different numbers of concurrent requests.
When the number of concurrent requests increases (\ie fewer available GPU cycles for one individual query), \name significantly reduces TTFT than the baselines.
This is because the amount of computation required for prefilling on a long input (9.6K in this case) is huge, as discussed in \S\ref{subsec:context}. 
\S\ref{app:space} shows \name's improvement over a complete space of workloads of different bandwidth and GPU resources. 


% \yh{Say more sentences that when we have improvement }



% To study how different network bandwidths or input token lengths affect the performance of \name, we conduct a sensitivity analysis to study the impact of these two factors on the gains of \name compared to the baselines.


% \input{fig-sens-context-len}
\mypara{Context lengths}
Figure~\ref{fig:sensitivity-gpu}b compares \name's TTFT with the baselines under different input lengths from 0.1K to 15K tokens under a fixed network bandwidth of 3~Gbps.
% The result follows our expectations in \S\ref{sec:design}.
When the context is long, the gain of \name mainly comes from reducing the KV cache sizes.
And when the context is short (below 1K), \name will automatically revert to loading the text context as that yields a lower TTFT.


% \input{fig-compress-ratio}




% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.9\columnwidth]{figs/concurrent.pdf}
%     \tightcaption{TTFT of \name and the baselines when there are multiple concurrent requests. }
%     \label{fig:concurrent}
% \end{figure}



% \mypara{Impact of number of concurrent requests} Figure~\ref{fig:concurrent} shows how the TTFT varies when there are $X$ concurrent requests sharing one link and one GPU. 
% As we can see in the breakdown of \name, although the transmission delay grows linearly when there are multiple requests sharing one link, the decompression time grows only marginally since the decompression for one request does not saturate the GPU computation. 
% The computation delay of processing the prompt also grows marginally as batching $X$ jobs has little increase in delay. 

\subsection{KV streamer adaptation}
\input{fig-adaptation-res}
The adaptation logic described in \S\ref{subsec:controller} allows \name to adapt to bandwidth changes and achieve good quality while meeting the SLO on TTFT. 
In Figure~\ref{fig:adaptation_res}, we generate bandwidth traces where each context chunk's bandwidth is sampled from a random distribution of 0.1 -- 10~Gbps.
Each point is averaged across 20 bandwidth traces on the LongChat dataset.
We can see that \name significantly outperforms the quantization baseline and \name without adaptation. 
Specifically, given an SLO on the TTFT of 2.5s, \name reaches the same quality as the quantization baseline with an 80\% lower SLO violation rate. 
Under an SLO of 4.5s, 
% \name reaches the same quality as the quantization baseline, while reducing the SLO violation rate by 100\%. 
The reason why \name has a lower SLO violation rate is that
when the bandwidth drops, \name can dynamically reduce the quantization level or fall back to the configuration of computing text from scratch, while the quantization baseline and \name without adaptation cannot. 

% \hc{Yuhan fill in setting and reason for having better performance}



% \fillme \jc{Yuhan :)}

\tightsubsection{Overheads and microbenchmarks} 
\label{subsec:eval:micro}
\input{fig-overhead}
\mypara{Decoding overhead}
While having a better size-quality and TTFT-quality trade-off, \name requires an extra decoding step compared to the quantization baseline.
\name minimizes the decoding overhead by pipelining the decoding of context chunks with the transmission of the context chunks, so as shown in Figure~\ref{fig:overhead}a, the decoding has minimal impact on the end-to-end delay.
% overhead can be hidden, thus is minimal to the end-to-end delay as shown in Figure~\ref{fig:overhead}a. 
% Figure~\ref{fig:resource}a breaks down the TTFTs of \name and the baselines on a context of 9.5K tokens into data transfer, decompression (or \texttt{torch.load}), CPU-GPU data movement, and computation by LLM in GPU. 
It is also important to note that although \name's decoding is performed on GPU (see \S\ref{subsec:impl}), the amount of computation needed by \name's decoding module is negligible compared to the baseline that generates KV cache from text context. 

% Although \name has slightly more delays in encoding and decoding, these delay are much less than the reduction of transmission time. 



\mypara{Offline encoding and storage overheads}
% \input{F/offline/fig-offline}
\label{subsec:eval:storage}
Unlike prior methods that compress each context only once, \name compresses it into
multiple versions (\S\ref{subsec:controller}). 
\name compresses each context almost as fast as the baselines because the encoding delay is very small (200 ms), as shown in Figure~\ref{fig:overhead}c.
Figure \ref{fig:overhead}d evaluates the overhead in storage.
We can see that despite needing to encode and store multiple bitstream representations, the total
storage cost for \name is on par with the quantization baseline. 
% More discussion around storage cost is in \S\ref{sec:cost}.
  


\input{fig-insight}
\input{fig-user-study}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.5\columnwidth]{figs/intrusive2.pdf}
%     \tightcaption{}
%     \label{fig:intrusive2}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.6\columnwidth]{figs/gisting.pdf}
%     \tightcaption{}
%     \label{fig:intrusive3}
% \end{figure}



%\mypara{How does \name compare with context reduction baselines? }
% The evaluation till now assumes the context is already been preprocessed and ready to use. 
% However, there are other works~\cite{??, ??} trying to shrink the length of the context so as to reduce the memory footprint of LLMs. 
%  \yh{say that previous evals assumes the context is given. Now we wanna compare with techniques that reduce context length via prompt rewriting or token selection. }

% \begin{figure}
% \centering
% \includegraphics[width=0.33\textwidth]{figs/scissorhands.pdf}
% \caption{Comparison of \name and \scis*. }
% \label{fig:scissorhands}
% \end{figure}


% \scis removes tokens from the LLM input with low self-attention scores. 
% This method has to execute the  \emph{self-attention} operation in order to determine the tokens to be removed. 
% Thus, \scis would not be able to reduce the TTFT. 
% However, we evaluate the idealized version of \scis to see how much it can reduce the size of \kv. 
% By an idealized version, we simply run the self-attention operation and obtain the scores, and remove those tokens whose attention scores are small.  
% Figure~\ref{fig:scissorhands} shows the quality and size trade-off for \name and \scis. 
% \name even achieves better trade-offs than the idealized \scis. 

% Similarly, we apply another context reduction 
% \yh{todo: add gisting's results}



%\mypara{How does \name compare with smaller model architectures? } 
% To alleviate the high computation delay or the memory footprint of LLMs,
% applications may choose to use smaller model architectures~\cite{??, ??}.
% In order to show if using a smaller model can achieve better trade-offs than \name, we evaluate 
% \name's \kv with smaller models' \kv.
% As shown in Figure~\ref{fig:smaller}, the trade-off curve of the smaller model (Llama-3B) is obtained by varying the quantization levels. 
% We can see that \name achieves better trade-offs than smaller models.

% \begin{figure}
% \centering
%         \includegraphics[width=0.4\textwidth]{figs/quantize_model.pdf} 
%         \tightcaption{}
%         \label{fig:quant}
%     \end{figure}



% \todo{Add a section which shows \name is applicable on quantized models, like figure~\ref{fig:quant}. }

% \todo{Add a section to show \name is similarly effective in compressing the size of kv cache for larger models (Llama 65B model)~\ref{fig:larger}}

\mypara{Ablation Study}
% As shown in Section \ref{sec:??}, \name's context encoder incorporates three key insights. 
To study the impact of individual components in \name's KV encoder,  Figure~\ref{fig:insights} progressively adds each idea into the baseline of uniform quantization and default AC, starting with the use of our AC that uses probability distribution for each channel-layer combination, then change-based encoding, and finally layer-wise quantization.
This result underscores the substantial contribution from each idea to the overall reduction of KV cache size. %, with the combined effect being particularly impactful.



\mypara{Quality of Experience}
We performed an IRB-approved user study to validate the effectiveness of \name. We selected three conversation history from the LongChat dataset used in previous evaluations. For each user, we first present the conversation history with ChatGPT. Then we show the same response but produced by different pipelines by adding different TTFT and let users rate the quality of response. With 270 ratings collected from Amazon MTurk~\cite{mturk}, we show that \name consistently outperforms other pipelines in QoE with shorter TTFT in Figure~\ref{fig:user-study}.

Evaluation results of \name with more baselines is available \S\ref{appendix:intrusive}, including using a smaller-sized model to speed up TTFT and Gisting, another context-shrinking technique.


% Each curve represents a trade-off obtained by adding our AC, delta compression, and layer-wise quantization atop the quantization baseline employing naive AC.

% Our AC technique alone achieves a remarkable reduction in size, approximately two times more efficient than naive AC. 
% The other two insights further enhance the size reduction. Specifically, they reduce the size in comparison to the baseline quantization and our AC by approximately \fillme and \fillme, respectively.



% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.7\columnwidth]{figs/prediction_error.pdf}
%     \tightcaption{The prediction errors of \name's controller. Measured with Llama-7B on the Wikitext dataset.}
%     \label{fig:cdf_error}
% \end{figure}

% \mypara{Controller prediction error}
% Finally, we zoom in on \name's controller and test whether the controller can predict the TTFT of a compression level with low errors based on history measurements.
% Figure~\ref{fig:cdf_error} shows the distribution of \name's prediction error, defined by the difference between the predicted TTFT and the real TTFT, on the contexts in the Wikitext dataset.
% Since the TTFT does not depend on the content of the context, the prediction error mostly reflects the statistical noise of loading and processing contexts of the same length.
% Empirically, as prediction errors are dominantly smaller than the actual TTFT, \name can almost always pick the right compression level to meet a given TTFT target. 




%\mypara{What's the storage overhead of \name? } 
% \jc{need to add the storage overhead here}






% \mypara{Does the position of the context affect the gains of \name? } In some scenarios, the context is 
% not always at the beginning of the input~\cite{??, ??}.
% For example, some applications may define some templates for the user to fill in, 
% and the context may lie in any position of the input.
% In order to understand how the position of the context affects the gains of \name,
%  we conduct an experiment to evaluate \name on the wikitext dataset with the context being at the end of the input.
% Similar to the case where the context appears in front of the query, 
% we can see that our gain, compared to the \recomp baseline and the quantization baseline, 
% \name still achieves similar reduction in TTFT, as shown in Figure~\ref{fig:}.




%\mypara{How does each insight in \name's encoder contribute to the overall reduction in size? } 
% As shown in \S\ref{sec:??}, we use three insights in \name's context encoder. 
% In order to understand how much does each component in the context-encoder contribute to the overall reduction in size of \kv. 
% In Figure~\ref{fig:insights}, we incrementally add \name's three insights step-by-step. 
% From right to left, the trade-off curves are obtained by adding our AC, compressing deltas and layer-wise quantization, on top of the quantization baseline with naive AC respectively. 
% As we can see, our AC can reduce the size by about 2$times$ compared to naive AC.
% The other two insights reduces the size from baseline quantization and our AC by \fillme and \fillme respectively. 


% \begin{figure}[t]
% \centering
%      \includegraphics[width=.8\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. \jc{some cosmetic changes:
%     (1) change x-axis title to real size (in bits). 
%     (2) change y-axis title to "generation quality (perplexity)", 
%     (3) add a "better" arrow pointing to the bottom left corner, 
%     (4) legend: Original KV feature compression vs. Delta-based compression, 
%     (5) cut the x-axis to remove the blank on the left side}
%     \yh{remove this}} 
%     \label{fig:delta_insight}
% \end{figure}

%Next, we zoom-in on individual components and evaluate the effect of their design choices.

% \mypara{Delta-based compression}
% To validate the advantage of delta-based compression, we pick the contexts in the \fillme dataset and contrast the performance of compressing their original KV features and the delta tensors explained above.
% %compress them with different quantization levels .
% In Figure~\ref{fig:delta_insight}, we vary the quantization levels (explained shortly) and show the spectrum of the tradeoffs between the compressed sizes and the generation quality (measured in perplexity) of the \fillme model on the decompressed context. 
% We can see that compared to compressing the original KV features, \name's delta-based compression has a much more favorable tradeoff.
% \jc{we should say something about other models? otherwise, people may feel it applies only to this model.}

% \begin{figure}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/ac.pdf}
%     \tightcaption{How different groupings of segments in key-value features affect the entropy. \yh{remove this}} 
%     \label{fig:ac}
% \end{figure}

% \mypara{Different grouping in AC}
% To illustrate the effectiveness of grouping feature values by their channels and layers, Figure~\ref{fig:ac} uses the same dataset and model from Figure~\ref{fig:delta_insight} and comparing the AC-encoded sizes when the probability distributions are conditioned on different combinations of channel, layer, and token index.

% \mypara{Benefit of \name's controller}
% \yh{discuss this}


==> backups/sec-eval-0304_2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US
\input{fig-e2e-longchat}
\input{fig-e2e-70b}

\tightsection{Evaluation}

Our evaluation answers the following key questions:

%\begin{itemize}
    %\item 
    1) Given a context, how much can \name's KV encoder reduce the bandwidth needed to transfer its KV cache? 
    %\item % Given a network bandwidth, 
    2) How much can \name reduce TTFT (including both network and compute delays)? 
    %\item 
    3) How sensitive is \name's performance gain to the workload, including different context lengths, network bandwidths, and the number of concurrent requests?
    % and the ratio of available GPU cycles? 
    %\item 
    4) How much is \name's decoding overhead in terms of compute and delay? 
    % \item Does \name have a better tradeoff between LLM performance and TTFT than baselines that reduce TTFT by pruning the contexts or using smaller models?
    
    % \jc{the items blow dont seem high priority?}
    % \item How much runtime memory usage does \name reduce? 
    % \item What's the overhead of \name?
    % \item How much does each of the components of \name contribute to the total improvement? 
%    \item How generalizable is \name's compressor? 
%\end{itemize}




% \begin{figure*}[t]
% \centering
%     \includegraphics[width=.92\textwidth]{figs/sensitivity_all.pdf}
%     \vspace{-0.2cm}
%     \tightcaption{Sensitivity of \name's gains over the baseline across different token lengths, network bandwidths, and models.}
%     \label{fig:sensitivity}
% \end{figure*}
\tightsubsection{Setup}
\label{subsec:evalsetup}


\mypara{Models} We evaluate \name on four models of different sizes, specifically the fine-tuned versions of Llama-7B, Llama-13B, Llama-33B, Llama-70B. 
All models are fine-tuned such that they can take long contexts (up to 32K). 
We did not test \name on other LLMs (\eg OPT, BLOOM) because there are no public fine-tuned versions for long contexts to our best knowledge. 

\mypara{Datasets}
We evaluate \name on 662 contexts from four different datasets with different tasks (Table~\ref{tab:datasets}): 
% \ga{Call out the number of queries, size of dataset etc. to impress upon the large scale of evaluation. }
\begin{packeditemize}
    \item {\em LongChat:} The task is recently released~\cite{longchat2023} to test LLMs on queries like ``What was the first topic we discussed?'' by using all the previous conversations as the context.  
    Most contexts are around 9-9.6K tokens. 
    \item {\em TriviaQA:} The task tests the reading comprehension ability of the LLMs~\cite{bai2023longbench}, by giving the LLMs a single document (context), and letting it answer questions based on it. The dataset is part of the LongBench benchmark~\cite{bai2023longbench} suite. 
    \item {\em NarrativeQA:} The task is used to let LLMs answer questions based on stories or scripts, provided as a single document (context).
    The dataset is also part of LongBench.
    \item {\em Wikitext:} The task is to predict the probability of the next token in a sequence based on the context consisting of relevant documents that belong to a specific Wiki page~\cite{wikitext}.
\end{packeditemize}

\input{tab-1}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}



%\begin{table}[]
%\begin{tabular}{cccc}
%\hline
%  & Dataset          & Model(s)                                                                               & Quality metric \\ \hline\hline
%A & LongChat         & longchat-7B-16k                                                                        & Accuracy       \\ \hline
%B & NaturalQuestions & T5-large                                                                               & F1 score       \\ \hline
%C & Wikitext         & \begin{tabular}[c]{@{}c@{}}LLaMA-13B\\ LLaMA-7B\end{tabular} & Perplexity     \\ \hline
%\end{tabular}
%\caption{}
%\label{tab:my-table}
%\end{table}

% \mypara{Generation quality metric}
\mypara{Quality metrics}
We measure generation quality using the standard metric of each dataset.
\begin{packeditemize}

% \item {\em Perplexity} is used to evaluate the model's performance on the Wikitext dataset. 
% The perplexity is defined as the exponentiated average negative log-likelihood of the next token~\cite{ppl1, ppl2}.
% A low perplexity means the model likely generates the right next token.
% While perplexity does not equate to text-generation quality, it is widely used as a decent proxy~\cite{adiwardana2020humanlike}.
% This metric has been commonly used by prior works to test the impact of pruning or quantizing LLMs on generation performance~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% % widely used in previous works in evaluating whether shrinking the model size or quantizing models degrade the generation quality~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
% % \jc{this metric may not sound intuitive to system reviewers. add some citations and explain why we should care about it?}

\item {\em Accuracy} is used to evaluate the model's output on the LongChat dataset. 
The task predicts the first topic in the conversational history between the user and the LLM. 
The accuracy is defined as the percentage of generated answers that exactly includes the ground-truth topic. % It is defined as the percentage of the generated answer that matches the ground-truth first topic of the conversation.
% \jc{Yuhan, please add some details and explain why it is a good metric}

\item {\em F1 score} is used to evaluate the model's response in the TriviaQA and NarrativeQA datasets.
It measures the probability that the generated answer matches the ground-truth answer of the question-answering task.
\item {\em Perplexity} is used to evaluate the model's performance on the Wikitext dataset. 
The perplexity is defined as the exponentiated average negative log-likelihood of the next token~\cite{ppl1, ppl2}.
A low perplexity means that the model likely generates the next token correctly.
While perplexity does not equate to text-generation quality, it is widely used as a proxy~\cite{adiwardana2020humanlike} 
% This metric has been commonly used by prior works 
to test the impact of pruning or quantizing LLMs on generation performance~\cite{llmint8,smoothquant,liu2023scissorhands, roy2021efficient}.
\end{packeditemize}

\input{fig-h2o}


\mypara{Baselines} 
We compare \name with baselines that do not change the contexts or model (more baselines in \S\ref{subsec:eval:micro}). 
\begin{itemize}
% \item \code{torch.save}: 
% \item {\em ``Original KV''} uses \texttt{torch.save} to serialize the KV features in GPU memory to a file.
% This serves as a reference for the most straightforward implementation. 
% \item {\em ``Default quantization \& AC''} combines the uniform quantization of KV features~\cite{flexgen} with the default arithmetic coding (AC) that uses a global probability distribution for all elements.
% Like \name, this baseline also uses quantization and AC but with a simpler design on each component. 
\item {\em ``Default quantization''} uses the uniform quantization of KV cache, specifically the same quantization level for every layer in the LLM (which was used in~\cite{flexgen}). 
\item {\em ``Text context''} fetches the text of the context and feeds it to LLM to generate the KV cache for it. 
It represents the design of minimizing data transmission but at the expense of high computation overhead. %, especially under long contexts.
\item {\em ``Context compression''} either drops tokens in the text context (LLMlingua~\cite{jiang2023longllmlingua}) or in the KV cache (H2O~\cite{zhang2023h2o}). 

    % \item \recomp: This scheme sends the texts of the context and compute the \kv based on the texts before generating the first token. 
    % % \item Model quantization baseline: This scheme quantizes the model weights into less number of bits in order to reduce the memory usage at inference time~\cite{??, ??, ??}. For this scheme, we report the quality metrics after applying the model quantization. 
    % % For the size metrics, we report the size of the key-value caches saved by \code{torch.save}.
    % % \item Original models with shorter contexts: This scheme rewrites the contexts with gisting~\cite{??}, and generates the first token with the compressed contexts. \yh{Say a few sentences about the pretrained gisting models only allow us to test on specific models and datasets}
    % \item \kv quantization + \code{torch.save}: This scheme quantizes the key-value cache, and saves the compressed \kv via \code{torch.save}. 
    % \item \kv quantization + naive AC: This scheme quantizes the key-value cache, and saves the compressed \kv via naive AC (\ie no optimization on the grouping of \kv to improve compression ratio). 
    % % \item Smaller model architectures: This scheme approximates the line of work that uses smaller model architectures to reduce the memory footprint of LLMs~\cite{??, ??}. We compare \name's \kv with smaller models' \kv in terms of our metrics. 
    % \item \name (Ours): The orignal models with compressed \kv with \name's compressor and controller. 
\end{itemize}




\mypara{Hardware settings} We use an NVIDIA A40 GPU server with four GPUs to benchmark our results. 
The server is equipped with 384GB of memory and two Intel(R) Xeon(R) Gold 6130 CPUs with Hyper-threading and Turbo Boost enabled by default.
% The server is equipped with 64 Intel(R) Xeon(R) Gold 6130 CPU cores. 
% \yh{describe our CPU and GPU machines }




% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock2.pdf}
%     \tightcaption{Results on Size of KV cache } 
%     \label{fig:mock2}
% \end{figure*}



% \begin{figure*}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/mock1.pdf}
%     \tightcaption{Results on TTFT } 
%     \label{fig:mock1}
% \end{figure*}
% \input{fig-e2e-70b}
%


\extightsubsection{Overall improvement}
\label{subsec:overall_eval}

\mypara{TTFT reduction} 
Figure~\ref{fig:e2e-longchat}a and left part of Figure~\ref{fig:e2e-70b} demonstrate \name's ability to reduce TTFT, across four models and four datasets. Under bandwidth of 3~Gbps, 
\name reduces TTFT by 2.7-3.2$\times$ compared with the strongest baseline. (We test \name under varying of bandwidth in \S\ref{subsec:eval:sensitivity}.)
% \shan{This sentence sounds really odd. Can we delete it?}



It is important to note that even when the compression is lossless, specifically applying our AC on the KV cache after 8-bit quantization, \name can still reduce the TTFT by 1.67-1.81$\times$. 
\name's reduction in TTFT is a result of a shorter transmission delay to send the smaller KV caches.


% It is important to note that even under our 8-bit quantization pipeline with largest bitstream size, \name's encoded KV still reduces TTFT by \fillme $\times$ with no performance degradation. This shows that \name' is able to improve user experience with little cost.



\mypara{Reduction on KV cache size}
Figure~\ref{fig:e2e-longchat}b and Figure~\ref{fig:e2e-70b}b show that, across three datasets and four models, 
\name's KV encoder reduces the KV cache size by $3.7-4.3\times$ compared to the best baseline when achieving similar performance for downstream tasks after decoding. 
Thus, it achieves better quality-size trade-offs across different settings.
The degradation caused by lossy compression is marginal---the degradation is no more than 2\% in accuracy, less than 0.1\% in F1 score, and less than 0.1 in perplexity~\cite{huggingface_ppl}.
% in accuracy in Figure~\ref{fig:e2e-longchat} is less than 0.02, and the F1 Score decrease is below 0.1\%, it increases the perplexity by less than 0.1. 
Some example text outputs for different baselines are available in \S\ref{sec:appendix}. 


\input{fig-sens-bw}


% The next section will show more sensitivity tests. 


% This consistent improvement across these models and pipelines also indicate that \name is generally applicable to different model architectures and sizes. 

% Compared to the \recomp baseline, \name is able to reduce the TTFT because it 
% avoids the computation of the self-attention operation on the long context.

% \yh{Comments a bit on why \name can achieve smaller sizes compared to baselines}



\mypara{Gains over context compression}\name can compress any KV cache and is thus compatible with the recent context-compression techniques. 
To demonstrate this, we test \name's encoder on the KV cache produced by H2O~\cite{zhang2023h2o} and LLMlingua~\cite{jiang2023longllmlingua} for Llama-7B on 
the LongChat dataset. 
Figure~\ref{fig:h2o}a and Figure~\ref{fig:h2o}b shows that \name consistently improved TTFT over the quantization baseline by a factor of $2.8-3.7 \times$ without losing accuracy.
This suggests that after condensing contexts by H2O or LLMlingua, the resulting KV caches may still have the statistical observations behind \name's KV encoder.
Thus, the techniques used in \name's encoder remain beneficial when we encode the KV cache after applying these techniques.
Finally, we also compared LLMlingua directly with \name. 
As shown in Figure~\ref{fig:h2o}c, \name still outperforms LLMlingua by about 48\% in accuracy when reaching a similar delay. 







% We evaluate the ability 
% Figure~\ref{fig:adapt} shows how \name's controller adapts to changes of workloads when transmitting KV cache. 

% In figure~\ref{fig:adapt} illustrates a timeline of transmitting the KV cache for one piece of context. 
% To start with, \name's controller decides to transmit the compressed KV cache for the first \fillme layers. 
% At 2 seconds,
% the throughput suddenly drops from \fillme to \fillme. 
% After the throughput change is being reflected to the transmission server, \name's controller decides to transmit the text context and do the computation to generate the KV for subsequent \fillme layers.
% After 4 seconds, the throughput increases again from \fillme to \fillme, and \name's controller decides to switch back to transmit the KV cache for later layers. 
% Nevertheless, for the baseline that applies default quantization on the KV cache, it always sends the quantized version of KV cache without any adaptation, which leads to \fillme from 2 seconds to 4 seconds. 

% In figure~\ref{fig:adapt2}, we show how \name's controller adapts to different workloads change across time when transmitting different contexts. 
% We can see that due to the adaptation made by \name's controller, everytime when the workloads change in the middle of transmitting the context, the adaptation \name made further improves the gain of \name over the baseline. 



% \begin{figure}[t]
% \centering
%     \includegraphics[width=.5\textwidth]{figs/adaptation2.pdf}
%     \vspace{-0.2cm}
%     \tightcaption{\todo{Mock fig for now. replace with real!}}
%     \label{fig:adapt2}
% \end{figure}

% \vspace{-0.3cm}


\tightsubsection{Sensitivity analysis}
\label{subsec:eval:sensitivity}

\mypara{Available bandwidth} The left and right figures in Figure~\ref{fig:sensitivity-bw} compares the TTFT of \name with baselines under a wide range of bandwidth from 0.1--10 Gbps and 10--100 Gbps, while we fix the context length at 9.6K tokens. 
We can see that \name consistently outperforms baselines under almost all bandwidth situations. 
Arguably, the absolute reduction in TTFT becomes smaller under high bandwidth (over 20Gbps).
% However, the reduction of TTFT from \fillme~ms to \fillme~ms still makes a perceivable difference to human users who expect smooth interaction~\cite{??}.

\input{fig-sens-gpu-context-len}
\mypara{Number of concurrent requests}
Figure~\ref{fig:sensitivity-gpu}a shows the TTFT under different numbers of concurrent requests.
When the number of concurrent requests increases (\ie fewer available GPU cycles for one individual query), \name significantly reduces TTFT than the baselines.
This is because the amount of computation required for prefilling on a long input (9.6K in this case) is huge, as discussed in \S\ref{subsec:context}. 
\S\ref{app:space} shows \name's improvement over a complete space of workloads of different bandwidth and GPU resources. 


% \yh{Say more sentences that when we have improvement }



% To study how different network bandwidths or input token lengths affect the performance of \name, we conduct a sensitivity analysis to study the impact of these two factors on the gains of \name compared to the baselines.


% \input{fig-sens-context-len}
\mypara{Context lengths}
Figure~\ref{fig:sensitivity-gpu}b compares \name's TTFT with the baselines under different input lengths from 0.1K to 15K tokens under a fixed network bandwidth of 3~Gbps.
% The result follows our expectations in \S\ref{sec:design}.
When the context is long, the gain of \name mainly comes from reducing the KV cache sizes.
And when the context is short (below 1K), \name will automatically revert to loading the text context as that yields a lower TTFT.


% \input{fig-compress-ratio}




% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.9\columnwidth]{figs/concurrent.pdf}
%     \tightcaption{TTFT of \name and the baselines when there are multiple concurrent requests. }
%     \label{fig:concurrent}
% \end{figure}



% \mypara{Impact of number of concurrent requests} Figure~\ref{fig:concurrent} shows how the TTFT varies when there are $X$ concurrent requests sharing one link and one GPU. 
% As we can see in the breakdown of \name, although the transmission delay grows linearly when there are multiple requests sharing one link, the decompression time grows only marginally since the decompression for one request does not saturate the GPU computation. 
% The computation delay of processing the prompt also grows marginally as batching $X$ jobs has little increase in delay. 

\subsection{KV streamer adaptation}
\input{fig-adaptation-res}
The adaptation logic described in \S\ref{subsec:controller} allows \name to adapt to bandwidth changes and achieve good quality while meeting the SLO on TTFT. 
In Figure~\ref{fig:adaptation_res}, we generate bandwidth traces where each context chunk's bandwidth is sampled from a random distribution of 0.1 -- 10~Gbps.
Each point is averaged across 20 bandwidth traces on the LongChat dataset.
We can see that \name significantly outperforms the quantization baseline and \name without adaptation. 
Specifically, given an SLO on the TTFT of 2.5s, \name reaches the same quality as the quantization baseline with an 80\% lower SLO violation rate. 
Under an SLO of 4.5s, 
% \name reaches the same quality as the quantization baseline, while reducing the SLO violation rate by 100\%. 
The reason why \name has a lower SLO violation rate is that
when the bandwidth drops, \name can dynamically reduce the quantization level or fall back to the configuration of computing text from scratch, while the quantization baseline and \name without adaptation cannot. 

% \hc{Yuhan fill in setting and reason for having better performance}



% \fillme \jc{Yuhan :)}

\tightsubsection{Overheads and microbenchmarks} 
\label{subsec:eval:micro}
\input{fig-overhead}
\mypara{Decoding overhead}
While having a better size-quality and TTFT-quality trade-off, \name requires an extra decoding step compared to the quantization baseline.
\name minimizes the decoding overhead by pipelining the decoding of context chunks with the transmission of the context chunks, so as shown in Figure~\ref{fig:overhead}a, the decoding has minimal impact on the end-to-end delay.
% overhead can be hidden, thus is minimal to the end-to-end delay as shown in Figure~\ref{fig:overhead}a. 
% Figure~\ref{fig:resource}a breaks down the TTFTs of \name and the baselines on a context of 9.5K tokens into data transfer, decompression (or \texttt{torch.load}), CPU-GPU data movement, and computation by LLM in GPU. 
It is also important to note that although \name's decoding is performed on GPU (see \S\ref{subsec:impl}), the amount of computation needed by \name's decoding module is negligible compared to the baseline that generates KV cache from text context. 

% Although \name has slightly more delays in encoding and decoding, these delay are much less than the reduction of transmission time. 



\mypara{Offline encoding and storage overheads}
% \input{F/offline/fig-offline}
\label{subsec:eval:storage}
Unlike prior methods that compress each context only once, \name compresses it into
multiple versions (\S\ref{subsec:controller}). 
\name compresses each context almost as fast as the baselines because the encoding delay is very small (200 ms), as shown in Figure~\ref{fig:overhead}c.
Figure \ref{fig:overhead}d evaluates the overhead in storage.
We can see that despite needing to encode and store multiple bitstream representations, the total
storage cost for \name is on par with the quantization baseline. 
% More discussion around storage cost is in \S\ref{sec:cost}.
  


\input{fig-insight}
\input{fig-user-study}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.5\columnwidth]{figs/intrusive2.pdf}
%     \tightcaption{}
%     \label{fig:intrusive2}
% \end{figure}

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.6\columnwidth]{figs/gisting.pdf}
%     \tightcaption{}
%     \label{fig:intrusive3}
% \end{figure}



%\mypara{How does \name compare with context reduction baselines? }
% The evaluation till now assumes the context is already been preprocessed and ready to use. 
% However, there are other works~\cite{??, ??} trying to shrink the length of the context so as to reduce the memory footprint of LLMs. 
%  \yh{say that previous evals assumes the context is given. Now we wanna compare with techniques that reduce context length via prompt rewriting or token selection. }

% \begin{figure}
% \centering
% \includegraphics[width=0.33\textwidth]{figs/scissorhands.pdf}
% \caption{Comparison of \name and \scis*. }
% \label{fig:scissorhands}
% \end{figure}


% \scis removes tokens from the LLM input with low self-attention scores. 
% This method has to execute the  \emph{self-attention} operation in order to determine the tokens to be removed. 
% Thus, \scis would not be able to reduce the TTFT. 
% However, we evaluate the idealized version of \scis to see how much it can reduce the size of \kv. 
% By an idealized version, we simply run the self-attention operation and obtain the scores, and remove those tokens whose attention scores are small.  
% Figure~\ref{fig:scissorhands} shows the quality and size trade-off for \name and \scis. 
% \name even achieves better trade-offs than the idealized \scis. 

% Similarly, we apply another context reduction 
% \yh{todo: add gisting's results}



%\mypara{How does \name compare with smaller model architectures? } 
% To alleviate the high computation delay or the memory footprint of LLMs,
% applications may choose to use smaller model architectures~\cite{??, ??}.
% In order to show if using a smaller model can achieve better trade-offs than \name, we evaluate 
% \name's \kv with smaller models' \kv.
% As shown in Figure~\ref{fig:smaller}, the trade-off curve of the smaller model (Llama-3B) is obtained by varying the quantization levels. 
% We can see that \name achieves better trade-offs than smaller models.

% \begin{figure}
% \centering
%         \includegraphics[width=0.4\textwidth]{figs/quantize_model.pdf} 
%         \tightcaption{}
%         \label{fig:quant}
%     \end{figure}



% \todo{Add a section which shows \name is applicable on quantized models, like figure~\ref{fig:quant}. }

% \todo{Add a section to show \name is similarly effective in compressing the size of kv cache for larger models (Llama 65B model)~\ref{fig:larger}}

\mypara{Ablation Study}
% As shown in Section \ref{sec:??}, \name's context encoder incorporates three key insights. 
To study the impact of individual components in \name's KV encoder,  Figure~\ref{fig:insights} progressively adds each idea into the baseline of uniform quantization and default AC, starting with the use of our AC that uses probability distribution for each channel-layer combination, then change-based encoding, and finally layer-wise quantization.
This result underscores the substantial contribution from each idea to the overall reduction of KV cache size. %, with the combined effect being particularly impactful.



\mypara{Quality of Experience}
We performed an IRB-approved user study to validate the effectiveness of \name. We selected three conversation history from the LongChat dataset used in previous evaluations. For each user, we first present the conversation history with ChatGPT. Then we show the same response but produced by different pipelines by adding different TTFT and let users rate the quality of response. With 270 ratings collected from Amazon MTurk~\cite{mturk}, we show that \name consistently outperforms other pipelines in QoE with shorter TTFT in Figure~\ref{fig:user-study}.

Evaluation results of \name with more baselines is available \S\ref{appendix:intrusive}, including using a smaller-sized model to speed up TTFT and Gisting, another context-shrinking technique.


% Each curve represents a trade-off obtained by adding our AC, delta compression, and layer-wise quantization atop the quantization baseline employing naive AC.

% Our AC technique alone achieves a remarkable reduction in size, approximately two times more efficient than naive AC. 
% The other two insights further enhance the size reduction. Specifically, they reduce the size in comparison to the baseline quantization and our AC by approximately \fillme and \fillme, respectively.



% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.7\columnwidth]{figs/prediction_error.pdf}
%     \tightcaption{The prediction errors of \name's controller. Measured with Llama-7B on the Wikitext dataset.}
%     \label{fig:cdf_error}
% \end{figure}

% \mypara{Controller prediction error}
% Finally, we zoom in on \name's controller and test whether the controller can predict the TTFT of a compression level with low errors based on history measurements.
% Figure~\ref{fig:cdf_error} shows the distribution of \name's prediction error, defined by the difference between the predicted TTFT and the real TTFT, on the contexts in the Wikitext dataset.
% Since the TTFT does not depend on the content of the context, the prediction error mostly reflects the statistical noise of loading and processing contexts of the same length.
% Empirically, as prediction errors are dominantly smaller than the actual TTFT, \name can almost always pick the right compression level to meet a given TTFT target. 




%\mypara{What's the storage overhead of \name? } 
% \jc{need to add the storage overhead here}






% \mypara{Does the position of the context affect the gains of \name? } In some scenarios, the context is 
% not always at the beginning of the input~\cite{??, ??}.
% For example, some applications may define some templates for the user to fill in, 
% and the context may lie in any position of the input.
% In order to understand how the position of the context affects the gains of \name,
%  we conduct an experiment to evaluate \name on the wikitext dataset with the context being at the end of the input.
% Similar to the case where the context appears in front of the query, 
% we can see that our gain, compared to the \recomp baseline and the quantization baseline, 
% \name still achieves similar reduction in TTFT, as shown in Figure~\ref{fig:}.




%\mypara{How does each insight in \name's encoder contribute to the overall reduction in size? } 
% As shown in \S\ref{sec:??}, we use three insights in \name's context encoder. 
% In order to understand how much does each component in the context-encoder contribute to the overall reduction in size of \kv. 
% In Figure~\ref{fig:insights}, we incrementally add \name's three insights step-by-step. 
% From right to left, the trade-off curves are obtained by adding our AC, compressing deltas and layer-wise quantization, on top of the quantization baseline with naive AC respectively. 
% As we can see, our AC can reduce the size by about 2$times$ compared to naive AC.
% The other two insights reduces the size from baseline quantization and our AC by \fillme and \fillme respectively. 


% \begin{figure}[t]
% \centering
%      \includegraphics[width=.8\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{The quality v.s. key-value feature size for compressing the raw features or compressing the deltas. The x-axis is the entropy (\ie estimated size of the compressed tensor), and the y-axis is the perplexity, the lower the better. \jc{some cosmetic changes:
%     (1) change x-axis title to real size (in bits). 
%     (2) change y-axis title to "generation quality (perplexity)", 
%     (3) add a "better" arrow pointing to the bottom left corner, 
%     (4) legend: Original KV feature compression vs. Delta-based compression, 
%     (5) cut the x-axis to remove the blank on the left side}
%     \yh{remove this}} 
%     \label{fig:delta_insight}
% \end{figure}

%Next, we zoom-in on individual components and evaluate the effect of their design choices.

% \mypara{Delta-based compression}
% To validate the advantage of delta-based compression, we pick the contexts in the \fillme dataset and contrast the performance of compressing their original KV features and the delta tensors explained above.
% %compress them with different quantization levels .
% In Figure~\ref{fig:delta_insight}, we vary the quantization levels (explained shortly) and show the spectrum of the tradeoffs between the compressed sizes and the generation quality (measured in perplexity) of the \fillme model on the decompressed context. 
% We can see that compared to compressing the original KV features, \name's delta-based compression has a much more favorable tradeoff.
% \jc{we should say something about other models? otherwise, people may feel it applies only to this model.}

% \begin{figure}
% \centering
%      \includegraphics[width=.9\linewidth]{figs/ac.pdf}
%     \tightcaption{How different groupings of segments in key-value features affect the entropy. \yh{remove this}} 
%     \label{fig:ac}
% \end{figure}

% \mypara{Different grouping in AC}
% To illustrate the effectiveness of grouping feature values by their channels and layers, Figure~\ref{fig:ac} uses the same dataset and model from Figure~\ref{fig:delta_insight} and comparing the AC-encoded sizes when the probability distributions are conditioned on different combinations of channel, layer, and token index.

% \mypara{Benefit of \name's controller}
% \yh{discuss this}


==> fig-adaptation.tex <==




\begin{figure}[t]
\centering


    \begin{tabular}{@{}c@{}}
        \includegraphics[width=0.4\textwidth]{figs/adaptation_res.png} 
        \vspace{-0.5cm}
        \\[\abovecaptionskip]
    \end{tabular}

    \tightcaption{ 
    }
    \label{fig:adaptation_res}
\end{figure}


\begin{figure}[t]
\centering


    \begin{tabular}{@{}c@{}}
        \includegraphics[width=0.4\textwidth]{figs/adaptation.png} 
        \vspace{-0.5cm}
        \\[\abovecaptionskip]
    \end{tabular}

    \tightcaption{ 
    }
    \label{fig:adaptation}
\end{figure}


==> fig-compress-ratio.tex <==

% \begin{figure}[]
% \   \centering
%     \includegraphics{F/compress-ratio/fig-compress-ratio.pdf}
%     \vminten
%     \tightcaption{\yh{Mock figure, junchen, I'm not sure if i have time to do this :( let me try tomorrow }The distribution of compressed ratio of \name compared with the default quantization baseline at the same quality, plotted with different contexts in the Wikitext dataset.}
%     \label{fig:compress-ratio}
% \end{figure}


==> fig-e2e-70b.tex <==

% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.95\linewidth]{F/e2e-70b/fig-e2e-70b.pdf}
%     %\vmintwenty
%     \vspace{-12pt}
%     \tightcaption{\name's improvement over baselines with Llama 70B on three more datasets (NarrativeQA, TriviaQA and Wikitext). The results of Llama 70B on Longchat is in Figure~\ref{fig:e2e-longchat}.} 
%     \vspace{-8pt}
%     \label{fig:e2e-70b}
% \end{figure}



% \begin{figure}[t]
% \centering
%     \includegraphics[width=0.95\linewidth]{F/e2e-70b/fig-e2e-70b-h2o.pdf}
%     %\vmintwenty
%     \vspace{-12pt}
%     \tightcaption{\name's improvement over H2O and LLMLingua with Llama 70B on three more datasets (NarrativeQA, TriviaQA and Wikitext). The results of Llama 70B on Longchat is in Figure~\ref{fig:e2e-longchat}.} 
%     \vspace{-8pt}
%     \label{fig:e2e-70b-h2o}
% \end{figure}


==> fig-e2e.tex <==

\begin{figure*}[t]
\centering

    \begin{tabular}{@{}c@{}}
        \includegraphics[width=0.8\textwidth]{figs/end-to-end.pdf}
        \vspace{-0.4cm}
        \\[\abovecaptionskip]
        KV cache size and TTFT reduction by dataset.
    \end{tabular}



    % \begin{tabular}{@{}c@{}}
    %     \includegraphics[width=0.92\textwidth]{figs/ttft_e2e.pdf} 
    %     \vspace{-0.5cm}
    %     \\[\abovecaptionskip]
    %     (b) TTFT reduction vs. LLM performance by dataset.
    % \end{tabular}


     % \begin{subfigure}{1\textwidth}
     %     \centering
     %     \includegraphics[width=0.99\textwidth]{figs/overall_bot.pdf}
     %     \caption{TTFT reduction}
     %     % \label{fig:three sin x}
     % \end{subfigure}
    
    \tightcaption{End-to-end test result (KV cache size and TTFT reduction) of LongChat 7B, LongChat 13B, Yi 34B, and Llama 70B on LongChat dataset. 
    % Overall results on three different pipelines shown in Table~\ref{tab:eval}.
    \yh{Put last two in another group }
    \yh{1. llm lingua 2. no context compress}
    }
    \label{fig:overall}
\end{figure*}


==> fig-example.tex <==

\begin{figure}[t]
\centering
    \includegraphics[width=.55\textwidth]{figs/improv.pdf}
    \vspace{-0.2cm}
    \tightcaption{\name's gains over the best baseline across different workloads (\ie Bandwidth throughput, GPU utilization).
    \yh{Putting this for now, let's polish later}
    }
    \yh{Better visualization. linear scale. Only need the number for a long input? rent a cloud instance for longer input? }

    \label{fig:resource}
\end{figure}



==> fig-sens-context-len.tex <==

\begin{figure}[t]
    \centering
    \includegraphics{F/sens/fig-sens-context-len.pdf}
    \vspace{-0.2cm}
    \tightcaption{\name's gain varying context lengths on Llama-13B.
    }
    \label{fig:sensitivity-context-len}
\end{figure}


==> fig-sens.tex <==

\begin{figure}[t]
    \centering
    \includegraphics{F/sens/fig-sens.pdf}
    \vspace{-0.2cm}
    \tightcaption{\name's gain varying bandwidth, available GPU cycles , and context lengths on Llama 13B. \jc{please add subfig index}\jc{can we pick a different setting for (b)? quantization and cachegen seems too similar} \jc{add an arrow between the blue and red and label it something like ``3x''.}
    \yh{split three single column figures, first figure one with 1-10Gbps, another one with 10-100Gbps, middle figure call it number of concurrent requests}
    }
    \label{fig:sensitivity}
\end{figure}


==> sec-method-v2.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}



\tightsection{\name Design}
\label{sec:design}

We now describe the design of \name, starting with the insights on KV cache (\S\ref{subsec:insight}) that inspires KV cache encoder (\S\ref{subsec:encoder}), followed by how \name adapts to bandwidth (\S\ref{subsec:controller}).

\tightsubsection{Empirical insights of KV cache}
\label{subsec:insight}

We highlight three observations on the characteristics of KV cache values. 
Though it is intrinsically hard to prove they apply to any LLM on any context, 
%we show empirical evidence over a large representative workload that they are prevalent among the KV cache produced by the models and contexts in our datasets. 
here, we use a representative workload to empirically demonstrate the prevalence of these observations.
The workload includes two LLMs of different capacities (Llama-7B and Llama-13B) and LongChat dataset~\cite{longchat2023} (which contains 100 long contexts between 9.2K and 9.6K tokens, randomly sampled from the whole set of 200 contexts), one of the largest datasets of long contexts. 
Details of this workload can be found in \S\ref{subsec:evalsetup}.
%To efficiently reduce the size of a KV cache, we first highlight three empirical observations on the characteristics of KV cache values.

%Moreover, they also corroborate with common intuitions in the literature. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/fig-cdf-measurement-7b.pdf}
    \vspace{-22pt}
    \tightcaption{Contrasting the distribution of the original values and the delta values. We model two Llama models with various long contexts (\S\ref{subsec:insight}). We show absolute values for clarity.} 
    \label{fig:locality}
\end{figure}

%\vspace{0.15cm}
%\myparashort{{\em Token-wise locality.}}
\subsubsection{{\bf \em Token-wise locality}}\label{subsubsec:locality}
The first observation is about how the K and V tensor values change {\em across tokens} in a context. Specifically, we observe that

\begin{insight}
    Within the same layer and channel, tokens in closer proximity have more similar K/V tensor values compared to tokens that are further apart.
\end{insight}

For each model, we contrast the distribution of K (or V) tensors' original values and the distribution of the {\em deltas}---the differences between of K (or V) tensors' values at the same layer and channel between every pair of consecutive tokens in the contexts.
Figure~\ref{fig:locality} shows the distribution of absolute values in the original tensor and the deltas of one layer across all the contexts\footnote{We randomly sampled a single layer from the K tensor because the values in the different layers have different ranges.}.
%Since the values of different channels have different ranges, we normalize the values of each channel to between -1 and 1 before calculating the deltas and putting them in the same CDF.
In both models across the contexts, we can see that the deltas are much more concentrated around zero than the original values. 
Consequently, the variance of the deltas is 2.4-2.9$\times$ lower than that of the original values.
The token-wise locality of K and V tensors inspires \name to encode deltas rather than original values. 
%, which as elaborated soon, is critical to the delta-based encoding in \name.

This token-wise locality can be intuitively explained by the transformer's self-attention mechanism, which computes the KV tensors. 
Though KV cache is computed in a layer-by-layer manner, this is mathematically equivalent to calculating the KV tensors of one token based on the KV tensors of the previous token.
This means KV tensors at one token are intrinsically correlated with those of the previous token.


\begin{figure}[t]
\centering
    \includegraphics[width=.99\linewidth]{figs/fig-accuracy-measurement.pdf}
    \vspace{-12pt}
    \tightcaption{Applying data loss to different layers of a KV cache has different impact on accuracy. (Same workload as Figure~\ref{fig:locality}).} 
    \label{fig:layer-sensitivity}
\end{figure}

%\vspace{0.15cm}
%\myparashort{{\em Layer-wise sensitivity to loss.}}
\subsubsection{{\bf \em Layer-wise sensitivity to loss}}\label{subsubsec:sensitivity}
The second observation concerns how sensitive different values in the K and V tensors are to data loss. Our observation is the following.

\begin{insight}
    The output quality of LLM is more sensitive to losses in the KV cache values of the shallower layers than to those in the deeper layers.
\end{insight}

The heterogeneous loss sensitivity on different layers suggests that our KV cache encoder should compress different layers differently.
Figure~\ref{fig:layer-sensitivity} shows how much accuracy is affected by applying data losses to the values of a specific layer group in the K and V tensors.
Here, we apply rounding as the data loss, and we compute the average resulting response accuracy (defined in \S\ref{subsec:evalsetup}) across 100 contexts in the dataset.
We can see that the average response accuracy drops significantly when the loss is applied to the early layers of a model while applying the same loss on the deeper layers has much less impact on the average response accuracy. This result holds consistently across different models we tested.

Intuitively, the deeper layers of a KV cache extract higher-level structures and knowledge than the shallower layers of a KV, which embed more primitive information~\cite{egeria, shao2024oneshot}.
As a result, the loss of information by removing precision on the early-layer cache might propagate and affect the later-layer cache and thus hinder the model's ability to grasp the higher-level structures necessary to produce quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 

\begin{figure}[t]
\centering
    \includegraphics[width=.99\linewidth]{figs/fig-entropy-measurement.pdf}
    \vspace{-12pt}
    \tightcaption{Entropy (bits per element) when using different grouping strategies.
    (Same workload as Figure~\ref{fig:locality}.)
    Grouping values by token position (red) reduces entropy much less than grouping by channel (yellow) or by layer (green).} 
    \label{fig:entropy}
\end{figure}


%\vspace{0.15cm}
%\myparashort{{\em Distribution along layers, channels, and tokens.}}
\subsubsection{{\bf \em Distribution along layers, channels, and tokens}}\label{subsubsec:entropy}
Finally, regarding the distributions of values along the three dimensions of KV cache---layers, channels, and token positions---we make the following observation.

\begin{insight}
Each value in a KV cache is indexed 
by its channel, layer, and token position. 
The information gain of grouping values by their channel and layer is significantly higher than the information gain of grouping values by their token position.
\end{insight}

% Intuitively, this can be loosely interpreted as: the KV values that belong to the same channel (or layer) but different token positions are more similar to each other than the KV values that belong to the same token position but different channels (or layer).
Intuitively, this can be loosely interpreted as: different KV values in the same channel (or layer) are more similar to each other than different KV values belonging to the same token position.
\yhedit{The intuition behind this insight is that different channels or layers capture diverse types of features in the input. 
Some channels may capture subject-object relationships, while others might focus on adjectives~\cite{lin2021survey}. 
Prior works have shown that different layers have shown that later layers capture more abstract semantic information compared to earlier ones~\cite{lin2021survey, devlin2018bert}.
On the other hand, given a layer and a channel, the KV values for different tokens are similar to each other due to the self-attention mechanism. 
Specifically, the KV for one token is derived from the KVs of all preceding tokens~\cite{attention2}. Consequently, each token only differs from its predecessor to a small extent.
}
%In other words, grouping values by channels and by layers can significantly reduce the entropy of elements in a group, which can then be separately compressed at a much smaller size. 
%\shan{This insight is not very easy to understand. Informally, are you trying to say that the KV values that belong to the same channel (layer) but different tokens are more similar to each other than the KV values that belong to the same token but different channel (layer)?}\jc{i like that. it's very close to what it is, though not quite, so i rewrite it as a loose interpretation.}
To show the insight empirically, we first group the values in the KV caches produced by the two models and 100 contexts based on their layers, channels, or token positions, and compute the entropy of each group. 
Figure~\ref{fig:entropy} shows the average entropy (bits per element) when different grouping strategy is applied, including no grouping, grouping by tokens positions, grouping by channels, and grouping by layers. 
%the channel-based groups, layer-based groups, or token-position-based groups. 
%The information gain along the channels, layers, or token positions is represented by the gap between 0the average entropy and the entropy of all values in these tensors (``global''). 


\subsection{KV cache encoding}
\label{subsec:encoder}

The aforementioned insights inspire the design of \name's KV cache encoder.
The encoding consists of three high-level steps (elaborated shortly):
%\begin{packedenumerate}
%\item 

First, it calculates the {\em delta tensors} (defined later) between the K and V tensors of nearby tokens. 
This is inspired by the token-wise locality observation (\S\ref{subsubsec:locality}) which suggests deltas between tokens might be easier to compress than the original values in the KV tensors.

%\item 
Second, it applies different levels of quantization to different layers of the delta tensors.
% \shan{??
% this sentence means we compress one layer in multiple different ways. This is not what you
% mean, right?}. 
The use of different quantizations at different layers is inspired by the observation of heterogeneous loss sensitivity (\S\ref{subsubsec:sensitivity}).

%\item 
Third, it runs a lossless arithmetic coder to encode the quantized delta tensors into bitstreams.
Specifically, inspired by the observation in \S\ref{subsubsec:entropy}, the arithmetic coder compresses the values in each layer and channel separately (\S\ref{subsubsec:entropy}).
%\end{packedenumerate}

These steps may seem similar to video coding, which encodes pixels into bitstreams.
Video coding also computes the delta between nearby frames, quantizes them, and encodes the delta by arithmetic coding~\cite{cabac}.
%Here, the delta between two nearby frames (\textit{e.g.}, motion vectors and residuals) are quantized and then encoded with arithmetic coding~\cite{cabac}.
%In KV cache compression, each token's KV cache is similar to a frame in video coding.
%can be seen as a frame. 
% where each token's KV cache can be seen as a frame. 
Yet, blindly applying existing video codecs could not work well since they were only optimized for pixel values in natural video content. 
Instead, the exact design of \name is inspired by domain-specific insights on LLM-generated KV cache (\S\ref{subsec:insight}).

Next, we explain the details of each step. 

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.93\linewidth]{figs/delta_fig_v2-arial.pdf}
    \tightcaption{Within a token group, \name computes the delta tensors between the KV tensors of the first anchor token and those of each remaining token.}
    \label{fig:delta}
\end{figure}

\mypara{Change-based encoding} 
To leverage the token-wise locality, we first split the context into {\em groups of tokens} each containing ten contiguous tokens. 
As shown in Figure~\ref{fig:delta}, in each group, we independently (\ie without referencing other tokens) compress the KV tensor of the first token, called the {\em anchor token}, and then compress and record the {\em delta tensors} with respect to the anchor token for every other token.% in the group.

This process is analogous to video coding, where the frames are separated into groups of {\em pictures}, within which it runs similar delta-based encoding. 
The difference, however, 
% \shan{To be honest, I feel the difference is not fundamental. Why don't
% we just acknowledge that we took inspiration from video compression? I don't think that hurts our 
% paper's value.} 
is that instead of compressing the delta between each pair of consecutive tokens, we reference the same anchor token for every token in the chunk. This allows us to do compression and decompression in parallel and saves time.
\begin{comment}
% \yh{The similarity should }
Moreover, the distributions of deltas between two consecutive tokens have similar
\shan{this sounds like a 
strong cliam. do you have experimental evidence?} distributions to that of the deltas between remaining tokens and the anchor tokens, 
thus the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 
\end{comment}
%\sid{Do "delta" and "delta tensors" mean the same thing? If so, we should have one term for consistency}

\mypara{Layer-wise quantization}
After partitioning the tokens into groups, \name uses quantization to reduce the precision of elements (floating points) in a KV cache so that they can be represented by fewer bits.
Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}. However, in previous work, elements are uniformly quantized with the same number of bits without leveraging any unique properties of KV cache.
Driven by the insight of heterogeneous loss sensitivity (\S\ref{subsubsec:sensitivity}), we apply more conservative quantization (i.e., using more bits) on the delta tensors of earlier layers. 
Specifically, we split the transformer layers into three layer groups, the first (earliest) 1/3 of layers, the middle 1/3 of layers, and the last 1/3 of layers, and apply different amounts of quantization bin size on the delta tensors at each layer group respectively. 
The size of the quantization bin grows larger (\ie larger quantization errors)
from earlier to later layer groups. 
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights. 

Note that we still use 8-bit quantization, a relatively high precision, on the KV cache of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it is important to preserve higher precision just for these anchor tokens.


\mypara{Arithmetic coding}
After quantizing the KV cache into discrete symbols, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context into bitstreams.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.

Driven by the observation of the KV value distributions along layers, channels, and token positions (\S\ref{subsubsec:entropy}), we group KV values by channel and layer to obtain probability distributions.
Specifically, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV caches produced by the same LLM.
\name uses modified AC library~\cite{mentzer2019practical} with CUDA to speed up encoding and decoding (\S\ref{subsec:impl}).
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution. 





\tightsubsection{KV cache streaming adaptation}
\input{fig-adaptation-case}

\label{subsec:controller}

% \yh{Not clear how we stream? 

% Pseudocode 

% drop the equation 
% }



%The transmission of a KV cache can take from hundreds of milliseconds to a few seconds, during which the network bandwidth may fluctuate.
Since the transmission of a KV cache may take up to hundreds of milliseconds to a few seconds, the available bandwidth may fluctuate during a transmission. 
%During the transmission of one context, throughput change can happen as it may take hundreds of milliseconds or several seconds to complete.
Thus, streaming the encoded KV bitstreams at a fixed encoding level may violate a given service-level objective (SLO)~\cite{10.5555/3006357} of fetching the KV cache.\footnote{In practice, SLO is defined on TTFT. Once the KV cache of the long context is loaded in GPU, the remaining delay of one forward pass is marginal~\cite{vllm}.}
In Figure~\ref{fig:adaptation-case}, for example, 
% The throughput drops from 2~Gbps to 0.2~Gbps at 1 second, lasting for 2 seconds, then increases to 1~Gbps, during the transmission of one context. 
at the start of the transmission, the available throughput 
%\footnote{In datacenters, the network bandwidth can achieve 10~Gbps to 100~Gbps}
is 2~Gbps, and if the bandwidth remains at 2~Gbps, sending a KV stream of 1~GB can meet the SLO of 4~seconds.
% given an encoded KV cache of 1~GB and a latency SLO of 4 seconds, transmitting the encoded KV cache will be able to meet the SLO. 
However, at $t=2s$, the throughput drops to 0.2~Gbps and only increases to 1~Gbps at $t=4s$, so the actual transmission delay increases from 4 seconds to 7 seconds, which violates the SLO.

\mypara{Workflow}
To handle variations in bandwidth, \name splits a context into multiple {\em context chunks} (or {\bf chunks} for short) of consecutive tokens and uses the KV cache encoder to encode each chunk into multiple bitstreams of different encoding (quantization) levels that can be decoded independently (explained shortly).
This can be done offline. 
When fetching a context, \name sends these chunks one by one, and each chunk can choose one of several {\em streaming configuration} (or {\bf configurations} for short): it can be sent at one of the encoding levels or can be sent in the text format to let the LLM recompute K and V tensors. 

\name adapts the configuration of each chunk while streaming the KV cache to keep the transmission delay within an SLO. 
Figure~\ref{fig:adaptation-case} illustrates an example adaptation where 
%As shown in Figure~\ref{fig:adaptation-case}, to start with, \name decides to send the KV cache. 
\name switches to sending text context and recomputing KV cache from the text at $t=2s$ due to the bandwidth drop, and at $t=4s$, since the bandwidth increases back to 1~Gbps, and \name switch to sending KV bitstreams of subsequent chunks at smaller size. 
With our adaptation logic (specific algorithm in \S\ref{Adaptation Logic}), \name can meet the SLO. 


%At a high level, it splits the KV cache for one context into several \emph{context chunks}, and send the context chunk by chunk.
%Based on the throughput, with the objective of meeting the SLO, \name can adapt the configurations independently for each chunk. 
%The configurations include whether to switch between compression levels of \name's encoded KV caches, or fall back to generate the KV cache from text context from scratch.

% This is based on two insights. 
% First, 
% even if the compression level is different for different chunks, the decoded KV caches are tensors of the \emph{same} shape. 
% Thus, they can be concatenated. 
% Second, the nature of how KV cache is constructed enables the KV cache for one specific chunk to be constructed based on the text of this chunk and the KV cache of all the previous chunks~\cite{dai2019transformer, vaswani2023attention}. 

However, to adapt efficiently, several questions remain.

%Two of the key questions in the adaptation module lie in how to split the whole context into chunks, and how to adapt to bandwidth fluctuations. 
%The context chunks are created by splitting the key tensor into chunks such that each chunk contains the key tensors for multiple contiguous tokens, and similarly for the value tensor. 
%Each of the chunk contains the number of tokens which is just large enough to fit in one congestion window size, for two reasons.
%One, we want to best utilize the bandwidth by filling up one congestion window, while on the other hand, we also want to provide fine-grained enough granularity to perform 
%adaptation to meet SLO. 
%Note that we also  let the number tokens in one context chunk be integer multiples of the number of tokens in one group in the change-based encoding (\S\ref{sec:}).

% The chunks make the decisions of switching between compression levels or generating KV cache from scratch 

First, {\em how to stream multiple chunks at different streaming configurations without affecting compression efficiency?}
%decode each context chunk independently?} Specifically, why encoding each context chunk separately does not affect compression efficiency
To encode the chunks offline, \name first computes the KV cache of the entire context (\ie prefill) and splits the K and V tensors of the KV cache along the token dimension into sub-tensors, each of which contains the layers and channels of the tokens in the same chunk.
It then uses the KV encoder to encode the K or V sub-tensor of a chunk with different encoding (quantization) levels. 
Each chunk is encoded {\em independent} to other chunks {\em without} affect the compression efficiency as long as a chunk is longer than a group of tokens.
This is because encoding the KV tensor of a token only depends on itself and its delta with the anchor token of the group of tokens (\S\ref{subsec:encoder}).
Thus, chunks sent with different encoding levels can be independently decoded and then concatenated to reconstruct the KV cache. 
In the case that a chunk is sent in text format, the LLM will compute its K and V tensors based on the previous chunk's KV tensors that have been received and decoded.\footnote{A similar concept has been used to split LLM input into prefill chunks for more efficient batching~\cite{agrawal2023sarathi}.}

{\em Would streaming chunks at different configurations affect generation quality?}
If one chunk is sent at a smaller-sized encoding level than other chunks (due to low bandwidth), it will have high compression loss on {\em that} single chunk, but this will not affect the compression loss of other chunks. 
That said, we acknowledge that if the bandwidth is too low to send most chunks in a high encoding level, the quality will still suffer.


 
%In order to adapt the configuration for each chunk, 
%in the offline stage, we encode each chunk of the KV cache into multiple compression levels, specifically by varying the quantization parameters\footnote{\yh{talk about the parameters }}. 
%The reason why we can encode each chunk separately is that the size of encoding each chunk is the same as encoding the whole KV cache.
%Specifically, since encoding each token depends only on the anchor tokens in the same group (see \S\ref{sec:method}), and we only use different quantization levels for different layers, this chunking will not affect the encoding procedure. 
%% The different versions of encoded KV cache lead to a tradeoff in LLM generation quality and size. 
%Each chunk also has the option of falling back to generating KV from scratch (implementation see \S\ref{subsec:impl}).


Second, {\em how long should a context chunk be?}
We believe that the chunk length depends on two considerations. 
\begin{packedenumerate}
% \item Since the next chunk's configuration is decided after the previous chunk is received, the encoded KV bitstream of a chunk should not be smaller than the sender's congestion control window or we would not fully utilize the network bandwidth.
\item The encoded KV bitstream of a chunk size should not be too big because, otherwise, it cannot react to bandwidth changes in a timely manner.
\item The chunk should not be too small either since then we can not fully utilize the batching ability of GPU to compute KV tensors if text format is chosen.
\end{packedenumerate}
With these considerations in mind, we empirically pick 1.5K tokens as the default chunk length in our experiments\footnote{The chunk length is also long enough for the KV bitstream of each chunk to fill the sender's congestion window in our experiment setting.}, though more optimization may find better chunk lengths.

Finally, {\em how does \name decide the streaming configuration of the next chunk?}
\name chooses the configuration for the next chunk based on the measured throughput when sending the previous chunk.
Specifically, \name first assumes the same throughput will remain and calculates the expected delay of each streaming configuration if it is applied to all remaining chunks. 
The delay of sending an encoded KV bitstream is calculated by dividing its size by the throughput (more details in \S\ref{sec:appendix}).
% It then picks the configuration that has the least compression loss (\ie text format or lowest encoding level) with an expected delay still within the remaining time before the SLO, and uses the configuration to send the next chunk.
It then picks the configuration that has the least compression loss (\ie text format or lowest encoding level) with an expected delay still within the SLO, and uses the configuration to send the next chunk.
%Specifically, if the delay to generate KV cache from scratch does not meet the SLO, \name will select the compression level that yields the highest generation quality without violating SLO. 
%Otherwise, \name will fall back to generate KV cache from scratch. 
For the first chunk, if some prior knowledge of the network throughput is available, \name will use it to choose the configuration of the first chunk the same way.
Otherwise, \name starts with a default medium encoding level (140~MB per chunk for Llama 7B, detailed setting in \S\ref{medium_encoding}). 
%The detailed adaptation logic can be found in \S\ref{sec:appendix}. 

%When sending the first chunk, without much information about the network bandwidth, \name starts with \fillme (a medium encoding level). 
%If some prior knowledge of the network throughput is available, it can be used 
%by sending the first chunk of the KV cache at the compression level with a middle-level size and the entire text context. 
%Upon receiving each chunk, \name chooses the configuration for the next chunk based on the empirical throughput of the last chunk. 
%Concretely, if the delay to generate KV cache from scratch does not meet the SLO, \name will select the compression level that yields the highest generation quality without violating SLO. 
%Otherwise, \name will fall back to generate KV cache from scratch. 
%Note that even if \name may choose the version of encoded KV cache yielding the worst generation quality for one context chunk, we empirically find that the final generation quality will not be significantly affected if the number of chunks sent in low quality is not substantial (see \S\ref{sec:??}).




% \begin{equation*}
% \begin{cases} 
% \text{use text to recompute} & \text{if } T_{\text{text}}(L_{\text{rt}}, L_{\text{ct}}) < SLO, \\
% \underset{Q}{\mathrm{argmax}} \text{ s.t. } T_{\text{kv}}(L_{\text{rt}},Q) < SLO & \text{otherwise.}
% \end{cases}
% \label{eq:adapt}
% \end{equation*}

% In the equation, $L_{rt}$ is the number of tokens yet to be received, $L_{ct}$ is the number of tokens that have already been received. The function $T_{kv}(L_{rt}, Q)$ \footnote{$T_{kv}(L_{rt}, Q) = \frac{\alpha \times Q \times C \times L_{rt} \times L}{Throughput} + RTT$, $\alpha$ is a constant of the model} predicts the delay for transmitting a KV cache with $L$ tokens at compression level $Q$, while $T_{text}(L_{rt}, L_{ct})$ \footnote{$T_{text}(L_{rt}, L_{ct}) = \gamma L_{ct} \times L_{rt}^2$, $\gamma$ is a constant of the model} predicts the delay for generating the KV cache from text. 

% Our adaptation logic chooses the compression level that is predicted to deliver highest quality within the SLO.
% Note that we use the throughput detected by the previous chunk to predict future throughput. While this approach may introduce some error to prediction, the performance stays strong (see \S\ref{sec:??}\hc{Yuhan plz fill}) since datacenter network bandwidths are relatively stable.

% \yh{Several comments: 1. need to explain SLO clearly. 2. split into context-chunks, send chunk-by-chunk, each chunk can make  several actions independently based on throughput to adapt to SLO. 3. how to determine chunk size? How to encode it into several chnks? }


% \jc{i commented out the algorithm pseudocode. it's causing a lot of latex errors, and i don't think we really need a pseudocode to explain it. if it can be clearly explained in fewer words, please do that. a pseudocode is usually a sign that the idea is really complicated}
% \begin{algorithm}
% \caption{Get Function Algorithm}\label{alg:sender}
% \begin{algorithmic}[1]
%     \State $remaining\_SLO \gets SLO$
%     \State $all\_KV \gets None$
%     \For{$i \in \{1..N\}$}
%         \State $is\_text, kv\_quality \gets \Call{GetNextQuality}{i, throughput, remaining\_SLO}$
%         \State $all\_KV \gets all\_KV + \Call{GetNextChunk}{is\_text, kv\_quality, i}$
%     \EndFor
%     \State \Return $all\_KV$
% \end{algorithmic}
% \end{algorithm}




% %So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
% Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
% In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
% To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% % , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.





% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

% First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
% %, with larger compressed sizes generally resulting in higher TTFT but better quality.
% %As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
% By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
% The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
% %Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
% Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

% We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
% We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.


% %By default, we \jc{explain the default levels here.}


% %\shan{Please remind readers that the compression is done in
% %the background and hence not part of the TTFT, although
% %decompression is part of TTFT.}
% %The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

% %\jc{need to explain why kv can be compressed offline and refer to the limitation section}

% %beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

% In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
% \begin{align}
% {\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
% \label{eq:prediction1}
% \end{align}
% The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
% %\hc{provided bandwidth in data center?} 
% The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
% The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
% %$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


% In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
% \begin{align}
% {\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
% \label{eq:prediction2}
% \end{align}
% The first term is the round-trip-time (RTT) between the storage server and the GPU server.
% We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
% The second term is the GPU computation to compute the attention from scratch.

% With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
% If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


% The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
% In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% % \todo{Show analytical model to predict ttft here. }


% %When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
% %\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
% %\begin{align}
% %TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
% %\label{eq:prediction}
% %\end{align}



% %Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

% %At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
% %If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
% %It then selects the \kv version that fits within the time budget while maximizing its size. 

% %In addition to different compression levels, we also include the option of raw text of each potential context document. 
% %Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
% %decompression time would outweigh the computation time on
% %short text contexts.
% %
% %\jc{remember to explain why picking the compression level doesn't depend on the prompt}

% %\subsection{Putting all together}
% %\yh{todo}
% %\jc{no need for a separate putting it together subsec}



\tightsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, about 1K lines of CUDA kernel code, based on PyTorch v2.0 and CUDA 12.0.
% \footnote{Code and video demo at: {\bf \url{https://github.com/CacheGenAuthors/CacheGen}}}
% The implementation for each component in our prototype will be discussed shortly. 

\begin{comment}
\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
% We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
% Particularly, we use its encoding and decoding functions to perform AC. 
We implemented a GPU-based AC library~\cite{??} with CUDA to speed up encoding and decoding.
\yh{talk to qizheng about implementation of gpu-based encoder}
Specifically, each CUDA thread is responsible for decoding the KV cache from bitstreams for one token. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}
\end{comment}

\mypara{Integration into LLM inference framework} 
\name operates the LLM through two interfaces: 
\begin{packeditemize}
    \item \texttt{calculate\_kv(context) -> KVCache}: given a piece of context, \name invokes LLM through this function to get the corresponding KV cache.
    \item \texttt{generate\_with\_kv(KVCache) -> text}: \name passes a KV cache to the LLM and lets it generate the tokens while skipping the attention computation (prefill) of the context.
\end{packeditemize}
We implement these two interfaces in HuggingFace models using the \texttt{transformers} library~\cite{huggingface_transformer} with about 500 lines of Python code.
Both interfaces are implemented based on the \texttt{generate} function provided by the library.
For \texttt{calculate\_kv}, we let LLM only calculate the KV cache without generating new text, by passing the options of \texttt{max\_length} \texttt{= 0} and \texttt{return\_dict\_in\_generate} \texttt{=} \texttt{True} when getting the KV cache. 
The \texttt{generate\_with\_kv} is implemented by simply passing the KV cache through the \texttt{past\_key\_values} argument when calling the \texttt{generate} function.
Similar integrations are also applicable to other LLM libraries, such as FastChat~\cite{zheng2023judging}, llama.cpp~\cite{llamacpp}, and GGML~\cite{ggml}.

We have also integrated \name in LangChain~\cite{langchain}, a popular LLM application framework.
\name is activated in the \texttt{\_generate} function of  LangChain's  \texttt{BaseLLM} module. 
% \yc{Yuhan, please help check the correctness of the following workflow}
\name first checks whether the KV cache of the current context already exists (explained shortly).
If so, \name will invoke \texttt{generate\_with\_kv} to start generating new texts.
Otherwise, \name will invoke \texttt{calculate\_kv} to create the KV cache first before generating new texts.
%Specifically, \name acts as a plugin module, receiving the input prompt, managing the loading of the KV cache, and calling the LLM to generate the response while bypassing the attention computation.
%Thus, \name requires the underlying LLM to provide two interfaces:
%(1) given a new prompt, LLM calculates the KV cache and return it to \name, 
%and (2) given the KV cache (provided by \name), LLM resumes the inference while skipping the attention computation.
%Many recent LLMs support the two functionalities by default. 
%For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
%\name interacts with LLM inference via two simple interfaces:
%% To apply \name, the model inference pipeline to have incorporate two functionalities: 
%(1) \name extracts the KV features of a given context from an LLM inference, and 
%(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
%Many Pytorch-based LLMs support these APIs. 
%For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.

% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.


\mypara{KV cache management in \name} To manage the KV cache, \name implements two modules:
\begin{packeditemize}
    \item \texttt{store\_kv(LLM) --> \{chunk\_id: encoded\_KV\}}: calls
    \\ \noindent 
    \texttt{caculate\_kv}, splitting the returned KV cache into context chunks, and encodes each chunk. 
    Then, it stores a dictionary on the storage server, where it maps the \texttt{chunk\_id} to the encoded bitstreams for the K and V tensors for the corresponding chunk.
    \item \texttt{get\_kv(chunk\_id) --> encoded\_KV} fetches the encoded KV tensors corresponding to \texttt{chunk\_id} on the storage server and transmits it to the inference server. 
\end{packeditemize}
Whenever a new piece of context comes in, \name first calls \texttt{store\_kv}, which first generates the KV cache, and then stores the encoded bitstreams on the storage server. 
At run time, \name calls \texttt{get\_kv} to fetch the corresponding chunk of KV cache and feed into \texttt{generate\_with\_kv}. 

% \yh{Say how we match context with KV. }

\mypara{Speed optimization for \name} 
To speed up the decoding of KV cache in GPU, we pipeline the transmission of context chunk $i$ with the decoding of context chunk $i-1$. %(explained in \S\ref{subsec:controller}). 
We implemented a GPU-based AC library~\cite{mentzer2019practical} with CUDA to speed up encoding and decoding.
Specifically, each CUDA thread is responsible for decoding the KV cache from bitstreams for one token. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
 
% To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.



==> sec-method.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US


%\begin{figure}
%\centering
%     \includegraphics[width=.99\linewidth]{figs/cachegen.pdf}
%    \tightcaption{Overall workflow of \name. \jc{for junchen: merge it with fig 10}} 
%    \label{fig:system}
%\end{figure}




\section{\name Design}
\label{sec:design}

We now present the design of \name, a concrete KV cache streamer for fast context-loading in LLM inference systems.
%, a fast context-loading module for LLM inference systems. 
%\subsection{Design objective and overview}
%\label{subsec:designgoal}
%\name minimizes the overall delay for loading and processing a given context while preserving the performance of the LLM.
%a balance between the generation quality and the context-loading \shan{again, are
%you sure we want to use loading to refer to network+computation?
%if so, give a clear definition earlier.} delay, which includes both the computation delay and the network delay.
%We first formally define the delay and quality metrics, before stating the design objective.
%\mypara{Delay}

\begin{comment}

Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the generation (decoding) of the first token.
We refer to it as the {\bf time-to-first-token (TTFT)}, since it measures when the first token is available for the user. 
As shown by previous studies, users' experience can be heavily affected by the TTFT since it demonstrates the responsiveness of the application~\cite{latency_experience1, latency_experience2, latency_experience3}

Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
%A few remarks about TTFT should be mentioned.
%We define this delay as the {\em time-to-first-token (TTFT)}, as it measures when the first token is available for the user. 
%As a result, users' experience is heavily affected by the TTFT~\cite{??}\jc{Yuhan, any citations for this?}
To focus on the impact of long contexts, TTFT excludes two delays.
First, TTFT excludes the time to decode generated tokens one by one, which grows with the response length, so we exclude it to better focus on speeding up the loading and processing of contexts in the input.\footnote{TTFT does include the decoding of the first token, though it is a negligible part of TTFT.}\shan{I suggest that we completely remove this ``First ...''. Your definition earlier already made it very clear that you only includes the time of generating the first token. What you put here is actually really confusing and requires a footnote to go back to what you already clearly defined earlier. So, I really don't see the point here. Let's just mention the second point below and simplify this pargraph.}
\edit{Second, TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. }
% Second, TTFT excludes the delay to select relevant the context based on the prompt because this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}.

%We formally define {\em time-to-first-token (TTFT)}, as the time between knowing the input (the prompt and context) and the generation of the first token. 
%Since the context may reside in a different machine than the GPUs running the LLM, the TTFT delay consists of 
%\begin{packeditemize}
%\item {\em network} delay to fetch the context to GPU memory, and 
%\item {\em computation} delay to process the context and prompt before generating the first token.
%\end{packeditemize}
%%To capture both the network and the computation delays of long context, 
%An alternative delay metric is the total generation delay (the sum of TTFT and the time to autoregressively generate all response tokens), we choose not to use this metric  because 
%(1) the time to generate each token of the response is largely constant for the methods considered in this work, and 
%(2) the total delay may also be affected by the response length, but we want to focus reducing the delay directly affected by long contexts.
%\shan{I think another point is that users' experience
%is heavily affected by the TTFT. I am not sure if we can find
%citations to support this though.}
%reduction on processing input faster.


%\mypara{Quality}
%Since the speedup of TTFT may be achieved by dropping information during input processing, the output of LLM may be affected.
%We define {\em generation quality degradation} by how close the  text generated under any speedup of input processing is to the text generated when letting the LLM processes the input without any speed optimization. 
%In other words, generation quality degradation measures the impact of speedup on text generation.
%If the speedup does not change the LLM output, the quality will be the highest.
%Specifically, generation quality degradation can be measured in terms of perplexity scores, classification accuracy, and quality assessment by a more powerful model. 
%\S\ref{subsec:eval:setup} will describe these metrics in more detail.
%
%
%\mypara{Design objective}
%With these definitions, the objective of \name is two-fold.
%\begin{packeditemize}
%\item First, \name should achieve lower delay, in terms of TTFT, than baselines at the same generation quality.
%\item Second, \name should be able navigate the tradeoffs between TTFT and generation quality, and minimize quality degradation under a given budget of TTFT.
%\end{packeditemize}


\tightsubsection{Overview}

To balance the overall delay and LLM's performance on a given context, \name employs a {\em KV encoder/decoder} and a {\em loading controller}, depicted in Figure~\ref{fig:system}.
%Before we explain each component in details, Figure~\ref{fig:system} depicts the high-level workflow between the two components and the LLM.



Given the cached KV features of a context, \name's KV encoder first compresses the KV features into bitstream representations.
While some recent schemes~\cite{gisting,autoencoder-incontext} have proposed to \emph{shorten} the context or its KV features, they do so by dropping tokens, with inevitable information loss. 
% They drop tokens after the context has been loaded the GPU memory.
Moreover, with the shortened KV features still in the shape of large tensors in GPU memory and directly consumed by LLMs, they still require a high bandwidth to be loaded in the first place. \shan{Exact same content is already mentioned multiple times earlier ... Different readers have different preferences. For me, I feel really frustrated when the paper keeps repeating the same thing and yet doesn't tell me what the design actually is as late as page 6 :'-).}
% with inevitable information losses due to the shortening of KV features. 
In contrast, our encoder aims to \emph{compress} KV features, with the compressed features being a bitstream and will be decompressed before being consumed by LLMs.
No longer in the shape of KV tensors, this bitstream can take on a more compact representation with minimum information losses. 

To flexibly navigate the tradeoffs between TTFT and generation performance, \name compresses the KV cache of a context in multiple bitstream representations with different compression levels {\em in advance} before user query arrives.
With a new prompt and selected context, \name's loading controller picks the compression level of the context based on the TTFT budget, fetches it through the network, decompresses it, and feeds it to the LLM. 
Notably, depending on the context's length, the controller may choose to load the original text of the context when the estimated time of loading and decompressing the KV features is longer than the time of loading and processing the text directly.
This often happens when the context is relatively short or the available bandwidth to fetch the context is relatively low, as will be shown in \S\ref{subsec:eval:sensitivity}.
%\shan{might the controller decide not to use any compression at all?}

\end{comment}

\begin{figure}[t]
\centering
%     \includegraphics[width=.99\linewidth]{figs/controller.pdf}
     \includegraphics[width=.99\linewidth]{figs/controller-v3.pdf}
    \tightcaption{Overview of \name's main components.} 
    \label{fig:system}
\end{figure}

%multiple bitstream representations using different compression levels

% \tightsubsection{Context KV encoding}
\tightsubsection{KV cache encoding}
\label{subsec:encoding}
% \yh{Jumps too much from previous }
% \yh{Emphasize the similarity with video coding. 
% Before starting change-based encodingxxx, start by saying why blindly applying video techniques is not ok.

% move the  insights in one zone.

% Mention this is empirical observation. 

% What we have is a representative dataset? 
% }

% \shan{Again, where is this discussed? I guess it should be in Section 2.1, but currently Figure 1
% is not well explained in that sub-section.}
% Recall from \S\ref{sec:delay} 
% that a KV cache of a context contains two tensors (K and V) of the same shape: 
% $[\NumTokens, \NumLayers, \NumChannels]$, where $\NumTokens, \NumLayers, \NumChannels$ are the number of tokens, layers, and channels, respectively.

At high level, for any given context, \name compresses the K and V tensor of its KV cache in three steps: 
\begin{packedenumerate}
\item calculate the {\em delta tensors} (defined later) between the KV cache of nearby tokens; 
\item apply selected levels of quantization to each layer of the delta tensors;
\item run the arithmetic coder on the quantized delta tensors.
\end{packedenumerate}
% \yc{Is delta tensor defined anywhere? It's not clear what's a delta tensor.}


These steps of compressing KV cache to a bitstream are analogical to video coding, which transforms from pixels to an encoded bitstream.
Video coding also computes the delta between two nearby frames, quantizes them, and encodes the result with arithmetic coding~\cite{cabac}.
%Here, the delta between two nearby frames (\textit{e.g.}, motion vectors and residuals) are quantized and then encoded with arithmetic coding~\cite{cabac}.
%In KV cache compression, each token's KV cache is similar to a frame in video coding.
%can be seen as a frame. 
% where each token's KV cache can be seen as a frame. 
Yet, blindly apply existing video codecs could not work well since they were only optimized for pixel values in natural video content. 
Instead, the exact design of \name is inspired by domain-specific insights on LLM-generated KV cache.

% Specifically, \name leverages the following empirical observations on KV cache.
% the insights we empirically find in the KV cache include: 
% \begin{packedenumerate}
%     \item \emph{At the same layer and channel, tokens in closer proximity have more similar KV cache values compared to tokens that are further apart.}
%     \item \emph{In a KV cache, each element is distinguished by its channel, layer, and token. 
% The information gain of grouping by channel and layer is significantly higher than that of grouping by tokens.}
% \item \emph{The output from the LLM is more sensitive to losses in the KV cache values of the shallower layers than to those in the deeper layers.}
% \end{packedenumerate}

Next, we will explain each part of \name's KV cache encoder and its rationale. %and insight along with the rationale behind it.


%\mypara{Cross-token locality} 
%Given one feature channel, the key-value features between nearby tokens have similar numerical values. 
%We refer to this as cross-token locality. 

\mypara{Change-based encoding}  Our first insight is about the similarity between KV cache values of nearby tokens.
This {\em token-wise} locality 
%Why do KV features have such \emph{token-wise} locality? It does
%not necessarily mean nearby tokens themselves are similar
%or more correlated (and they are not). Rather, it 
stems from
the transformer (the self-attention) mechanism that computes the KV
cache. In essence, the KV cache of a given token
% \shan{token or token index? Are they the same thing? If they
% are the same, please use one consistently.}
are calculated based on the KV cache of previous tokens\footnote{More strictly, the KV cache are generated in a layer-by-layer manner. The KV of token $t$ at layer $i$ is computed based on the attention matrix 
 from all the previous tokens' attention matrix at the previous layer~\cite{vaswani2023attention, attention2}.}.
We summarize our insights here:

\begin{insight}
    Within the same layer and channel, tokens in closer proximity have more similar K/V tensor values compared to tokens that are further apart.
\end{insight}
 
%Particularly, we observe that:

%that if two tokens' positions are near to each other in the context, their KV feature values at the same channel and same layer are similar.

% \begin{insight}
% %{\bf{(Token-wise locality)}} 
% At the same layer and channel, tokens in closer proximity have more similar KV cache values compared to tokens that are further apart.
% \end{insight}



% \jc{i know it's technically correct, but like you said many time, the conventional understanding is that KV is computed layer by layer, not token by token. it seems this claim is essential to the locality observation, can you add some text to explain it and also find any citations to back it up?}
% This dependency inherently leads to numerical similarity in their KV features across \emph{nearby} tokens in a context.


\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.7\linewidth]{figs/delta_insight.pdf}
    \tightcaption{\hc{specify the setting. Channel/layer... basically how you got the figure like Shan sai}\yh{Replace with real}} 
    \label{fig:delta_insight}
\end{figure}


This token-wise locality suggests an opportunity for achieving better size-quality tradeoff:
% \yc{Yuhan, I feel like ``without affecting generation quality'' is a bit vague here. I can understand why we can have more efficient compression by reading the text below, but it's not clear why it does not affect the generation quality.} 
within the same layer and channel, the values in the original KV cache
% \shan{terminology: what is
% the difference between KV cache and KV tensors?} 
% given one channel and layer,\jc{i don't think we really need to stress that it's a given channel or layer, do we?} 
tend to span a wider range with a higher variance than 
%However, if we compute 
the \emph{delta} between every pair of nearby tokens, which is defined by \hc{Yuhan please define}.
%, the distribution of the deltas will have a much smaller variance.
We illustrate this difference in 
Figure~\ref{fig:delta_insight} by juxtaposing the distributions of the delta and the original tensors.
Similar results hold for other channels and layers. 
\shan{How you get this figure}\hc{Maybe just do it in caption.}
% Yuhan, I simplified the original sentence.
% You need to add some methodology information here to explain 
% how you get this figure.}
%shows that at a particular layer and channel, the distribution of original KV values has a much lower variance than the distribution of the delta values between two nearby tokens.
% the cumulative density function (CDF) of the original and delta KV features for one channel and one layer.
% As we can see, the delta KV features has smaller variance than the original ones. 
% Since the distributions of delta tensors and original tensors have low variance, they also have low entropy~\cite{doi:10.1080/03610928608829122, entropyvariance1999} under the same quantization level. 

Since at the same quantization level, a normal distribution with lower variance has lower entropy~\cite{doi:10.1080/03610928608829122, entropyvariance1999}, we employ the following method to utilize this token-wise locality of feature values:

For every ten contiguous tokens in the context, we put them into a token group.
In each group, we independently (\ie without referencing other tokens) compress the KV cache of the first token, called the {\em anchor token}, and then compress and record the delta tensors with respect to the anchor token for every other token in the group.

This process is analogous to video coding, where the frames are separated into groups of contiguous ones and then compressed. 
However, the difference here 
% \shan{To be honest, I feel the difference is not fundamental. Why don't
% we just acknowledge that we took inspiration from video compression? I don't think that hurts our 
% paper's value.} 
is that instead of compressing the delta between each pair of consecutive tokens, we reference the same anchor token for every token in the chunk. This allows us to do compression and decompression in parallel and saves time.
% \yh{The similarity should }
Moreover, the distributions of deltas between two consecutive tokens have similar
\shan{this sounds like a 
strong cliam. do you have experimental evidence?} distributions to that of the deltas between remaining tokens and the anchor tokens, 
thus the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. \sid{Do "delta" and "delta tensors" mean the same thing? If so, we should have one term for consistency}


% Second, the tokens within a chunk may not change as smoothly as between two consecutive video frames, so the benefit of compressing the difference with the immediate last tokens vs. with the anchor token is marginal. 
% \yc{``change as smoothly as between two consecutive frames'' is vague. What do you mean by ``smooth''? Can we say the distribution of the delta tensor is similar?} \yh{The distribution after delta is similar ==> size after compression will be similar. }

% \yc{Should we first talk about quantization then arithmetic coding? Because the workflow is computing delta -- quantization -- arithmetic coding}
% \yh{Will do. }

% \begin{figure}
% \centering
% %     \includegraphics[width=.6\linewidth]{figs/2800_12.pdf}
%      \includegraphics[width=.67\linewidth]{figs/delta_insight.pdf}
%     \tightcaption{An example of KV values at the same layer and same channel across tokens.
%     We use LongChat-7b model and one example context in the LongChat dataset (Table~\ref{tab:eval}).
%     % Visualization of the numerical values of the key features for one example layer. Plotted with LongChat-7b model on the LongChat dataset~\cite{longchat2023} \yh{Keep font size consistent. }.  
%     % \jc{drop blue. and extend red to a wider range}
% %    \jc{i still don't feel this shows the right motivation. also, consider splitting it to two subfigures}
% \shan{I don't see why this figure tells me insight 1. I think I prefer the CDF figures you showed in our recent meeting; those figures clearly showed that the delta and the original values have different distributions, with the former more clustered towards 0/very-small values.}\jc{i completely agree with shan on this. this figure was put there last-minute. let's find a better visualization this time.}
%     } 
%     \label{fig:delta_vis}
% \end{figure}

\begin{figure}[t]
\centering
%     \includegraphics[width=.9\linewidth]{figs/delta_fig.pdf}
     \includegraphics[width=.99\linewidth]{figs/delta_fig_v2.pdf}
    \tightcaption{Within a chunk of tokens, \name computes the delta tensors between the KV features of the first token and that of each remaining token.} 
    \label{fig:delta}
\end{figure}


\begin{figure}[t]
\centering
     \includegraphics[width=.95\columnwidth]{figs/ac_insight.pdf}
    \tightcaption{Entropy of all elements vs. entropy of the elements at specific channels, layers, or token positions. \yh{Explain what's the labels. } } 
    \label{fig:ac_insight}
\end{figure}


% \begin{figure*}[t]
%     \centering
%         \subfloat[][Perplexity and size of KV cache tradeoff (NTK\_scaled\_LLaMA-7B model on wikitext dataset)]
%         {
%             \includegraphics[width=0.24\textwidth]{figs/ppl_size.pdf} 
%             \label{fig:multi_choice}
%         }

%     \tightcaption{}
%     \label{}
% \end{figure*}
%Figure~\ref{fig:delta_insight} shows the delay-quality tradeoffs of compressing the KV features individually vs. compressing the deltas with different levels of quantization (explained shortly). 
%It confirms that compressing the deltas achieves a better tradeoff.


\mypara{Layer-wise quantization}
\label{subsec:layerwise_quant}
% \yh{Earlier and later layers }
% So far, the compression (running AC on delta tensors) has been lossless.
After partitioning the tokens into groups,
\name uses quantization to reduce the precision of elements (floating points) in a KV cache so that they can be represented by fewer bits. 

Quantization has been used recently to reduce attention matrices to pack longer contexts in GPU memory~\cite{flexgen}. However, elements are uniformly quantized with the same number of bits without leveraging any unique properties of KV cache.
It remains unclear how to design a better quantization strategy to reduce size while minimizing the negative impact on LLM's performance.

Our insight is that the impact of quantizing KV elements on LLM's output varies is related to the layer position of the elements:

\begin{insight}
    The output quality of LLM is more sensitive to losses in the KV cache values of the earlier layers than to those in the later layers.
\end{insight}


Intuitively, KV cache at the later layers of an LLM extract higher-level structures and knowledge by applying NN operations on the KV cache of the earlier layers, which embed more primitive information~\cite{egeria}.
As a result, the loss of information by removing precision on the early-layer cache can propagate and affect the later-layer cache and thus hinder the model's ability to grasp the higher-level structures necessary to produce high-quality responses. %, thus more impact on results.
%Even though deeper layers have little loss in precision, the propagating effects of shallower layers will be relatively more pronounced. 



Driven by this insight, we apply less aggressive quantization (more bits) on the delta tensors of earlier layers. 
Specifically, we split the transformer layers into three layer groups, the first (earliest) 1/3 of layers, the middle 1/3 of layers, the last 1/3 of layers, and apply different amount of quantization bin size on the delta tensors at each layer group respectively. 
The size of the quantization bin grows larger (\ie larger quantization errors)
from earlier to later layer groups. 


Note that we still use 8-bit quantization, a relatively high precision, on the KV cache of the anchor token (the first token of a token chunk). 
This is because these anchor tokens account for a small fraction of all tokens, but their precision affects the distribution of all delta tensors of the remaining tokens in a chunk.
Thus, it is important to preserve higher precision just for these anchor tokens.



\mypara{Arithmetic coding} After quantizing the KV cache into discrete symbols, \name uses \textit{arithmetic coding}~\cite{ac} (AC) to losslessly compress the delta tensors and anchor tensors of a context to bitstreams.
%To further reduce the network bandwidth usage, \name applies \textit{arithmetic coding}~\cite{ac} (AC) on the delta tensors.
%AC enjoys a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.
Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols.
% while enjoying a closer-to-optimal coding efficiency among entropy coding schemes~\cite{??}.


%losslessly compresses a sequence of symbols into a more compact bitstream and enjoys closer-to-optimal coding efficiency than other entropy coding schemes~\cite{??}.
%Like other entropy coding schemes, AC assigns fewer bits to encode more frequent symbols and more bits to encode less frequent symbols. 
%Thus, for AC to be more efficient, we need an {\em accurate, low-entropy} probability distribution to describe each element.
%The key step of AC is to estimate of the probability distribution of the symbols, and the probability distribution is used by AC to encode the KV features.
As shown in Figure~\ref{fig:kvcache-illustrated}, the KV cache include $l$ layers of K/V tensors, and 
each layer of the K/V tensor is a two-dimensional
vector of the shape 
%For each layer, the key is a 2-D tensor of shape 
$[N, c]$, where $N$ is the number of input tokens and $c$ is the number of channels in the LLM. 

For it to be efficient, AC needs {\em accurate, low-entropy} probability distributions of the elements in the KV cache.
To motivate our design, we first consider two strawmen:
\begin{packeditemize}
\item {\em Global symbol distribution:} 
By default, AC uses a global probability distribution for {\em all} elements of a tensor. %in the KV features of anchor tokens and one probability distribution for the delta tensors.
However, elements of different layers, channels, or tokens do not necessarily share the same probability distribution. 
\item {\em Fine-grained symbol distributions:} 
Alternatively, a {\em separate} probability distribution can be used for elements at each combination of channel, layer, and token position.\footnote{This is called {\em contextual arithmetic coding} in coding literature and is used in modern video codecs.}
% , but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.} 
These probability distributions are more accurate but also incur prohibitive storage overheads, since we need to store $\NumTokens\times\NumLayers\times\NumChannels$ distributions on both the context storage servers (KV encoder) and the GPU servers (KV decoder). 
%This results in a prohibitive number of distributions, \eg the KV features of \fillme model on a 1K-token context have \fillme layers, \fillme channels, and 1K token indices, so \fillme distributions are needed in total. 
%This can cause a huge storage overhead as the distribution must be stored on the encoder (context storage servers) and the decoder (GPU servers). 
\end{packeditemize}

To strike a better balance between AC's compression efficiency and the storage overhead of the symbol probability distributions, we should group the elements in the tensors into as few groups as possible while minimizing the entropy of the distribution at each group. 
% and use one probability distribution for each group, such that the entropy of each group is significantly smaller than that of all elements with as few groups as possible. 
In other words, we should maximize the {\em information gain} of such grouping.
% between with and without the grouping.
%To examine how grouping should be done in KV features (and delta tensors), 
We consider three dimensions for grouping elements in KV features: the channel, the layer, and the position of the token in the context.
% , as each KV element is distinguished by these dimensions. 
%We pick the contexts from the same dataset dataset as Figure~\ref{fig:delta_insight} and use the same model to produce KV features (only the anchor tokens).
To examine the impact of each grouping, we pick the contexts in the Wikitext dataset~\cite{wikitext}, which is a popular dataset to evaluation LLM's generation quality~\cite{llmint8, smoothquant, scissorhand}, and use the Llama-7B model to produce the KV cache tensors.
Figure~\ref{fig:ac_insight} compares the entropy across all elements vs. the entropy at individual groups of certain layers, channels, or token indices, and their difference indicates the information of a grouping.
% We can see that entropy for grouping the tensors by channel and layer is lower than that of grouping by  token position.
We summarize the observations in the following insight: 

\begin{insight}
    In the KV cache for one context, each element is distinguished by its channel, layer, and token. 
The information gain of grouping by channel and layer is significantly higher than that of grouping by tokens.
\end{insight}
\hc{information gain is not clear to me. Is there a simpler substitute?}
\yc{Figure~\ref{fig:ac_insight} is a bit hard to understand. For example, what's the meaning of each bar? What does 400 mean in Channel400?}
%the probability distributions of all elements and when they are grouped by their layers, channels, or token indices. 
%We can see that on this dataset and this model, the probability distributions of feature values depend more on their channels and layers, than on their token index. 
% We can summarize the observation in the following insight:


%Figure~\ref{??} shows that the distribution of elements across all layers is widely scattered (\ie a high entropy). %vs. the distributions of elements at two particular layers. 
%In contrast, by conditioning the distribution at a specific layer, the distributions have much lower entropy and each element requires fewer bits to be encoded.
%Thus, we should use a different probability distribution to encode each element depending on the {\em position} of the element in the KV feature\footnote{This is often called {\em contextual arithmetic coding} and is used in modern video codecs, but we refrain from using it, otherwise the meaning of ``context'' will be ambiguous.}, which is distinguished by its channel, layer, and token index. 


%Instead of conditioning probability distributions on all three dimensions, our insight is that using a distribution for each layer-channel combination effectively reduces the entropy, but using a distribution for each token index does not.
%Formally, this insight can be summarized as follows:

% \begin{insight}
% %{\bf{(Information gain)}}
% In a KV cache, each element is distinguished by its channel, layer, and token index. 
% The information gain of grouping by channel and layer is significantly higher than that of grouping by token position.
% \end{insight}

Inspired by the insight, our KV encoder offline profiles a separate probability distribution for each channel-layer combination of delta tensors and another for anchor tensors produced by an LLM, and uses the same distributions for all KV caches produced by the same LLM.
In \S\ref{subsec:eval:micro}, we empirically show that our method reduces the bitstream size by up to 53\% compared to the strawman of using one global symbol distribution.
Compared to the strawman of finest-grained symbol distributions, our method stores $\NumTokens$ times fewer distributions ($\NumLayers\times\NumChannels$),  where $\NumTokens$ can be several thousand.
% \S\ref{subsec:impl} will explain how the probability distributions are obtained and 
\S\ref{subsec:eval:storage} will quantify the size overhead of storing these probability distributions.




% \jc{Yuhan, your text seems to say you still use per layer-channel-position in some cases. this can be very confusing to readers. unless there's a strong reason to do it (which should be clearly explained), we should not do?}


%per-layer, per-channel, and per-token-position grouping only for high quantization levels (\ie 8-bits and 7-bits), and use a per-layer and per-channel grouping for lower quantization levels. 



 

%The best trade-off is achieved by the finest-granularity grouping. 
%The next best grouping strategy combines each layer and feature channel into one group. 
%However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
%This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.





%This inspires the use of {\em contextual} arithmetic coding, which uses a different probability distribution based on the context\footnote{The term ``context'' refers to  We realize the use of term ``context'' is ambiguous} in which a symbol appears.
%Specifically, in KV features, each element 


\begin{comment}
When using AC, we need to compute the probability distribution for all the symbols (\eg the quantized integer values) over tensors in a dataset, and then input the distribution to compress the tensors. 
However, this can be sub-optimal as the probabilities for all the symbols in the whole tensor can be scattered, leading to small compression ratio. 
This is because a key property of AC is it will use \textit{less bits} to represent more frequent occurring symbols, and \textit{more bits} to represent less frequent occurring ones.
Scattered probability distributions results in inefficient compression, leading to larger sizes.

To address this, our encoder divides the entire tensor into distinct \textit{groups}, ensuring that elements within each group show highly similar distributions.


A naive solution is to group the tensor into the finest granularity. 
That is, each channel in one layer at the one token position forms a group.
However, since we need to store a unique probability distribution for each group, the number of probability distributions that need to be stored can explode. 

Fortunately, we find that given one feature channel and one layer, different token positions share very similar data distributions. 
We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.
The best trade-off is achieved by the finest-granularity grouping. 
The next best grouping strategy combines each layer and feature channel into one group. 
However, for higher quantization levels, the entropy difference between this grouping and the finest-grained one becomes more significant. 
This occurs because even minor distinctions between groupings are amplified when quantized into more discretized values.

\end{comment}


% The input to AC encoding are (1) symbol probabilities: a model that estimates the probabilities of different symbols or symbol sequences occurring in the input data \cite{rissanen1979arithmetic}, which we denote as $Z$; (2) The actual data to be encoded: Denoted as $I$, this represents the actual data that needs to be compressed.

% AC transforms the input data $I$ into a single real number within a specific range, typically [0, 1) \cite{rissanen1976generalized}. 
% This transformation is achieved through a series of interval divisions based on the probabilities specified by the symbol probabilities $Z$.

% An important property of AC is it will achieve good reduction rate when the distribution of  $Z$ is skewed.
% That is, a subset of symbols appear frequently, thus can be represented with a smaller number of bits. 
% To make AC most effective, we aim to group data into segments to reflect as much skewness as possible. 
% Ideally, these segments should have similar data distributions within them. 
% If the data is more evenly spread within the segments, it would result in a less skewed $Z$ and may not achieve the much compression benefits. 


% There are three primary factors that influence the grouping of key-value features: (1) layer, (2) feature channel, and (3) token position.

% Our key insight for optimizing AC is that different layers and feature channels in key-value features have distinct data distributions. 
% We validate this insight by studying trade-offs between entropy (compression size) and quality for various data groupings in Figure~\ref{fig:ac}.


% As shown in the figure, the finest-grained grouping (per-layer, per-feature-channel, and per-token-position $Z$) achieves the best quality-entropy balance. 
% This aligns with our intuition that smaller entropy results from similar data distributions.
% However, this grouping requires the highest additional storage for $Z$. 

% The next best grouping is using per-layer and per-feature-channel $Z$, indicating that for a given feature channel and layer, the key-value features for different tokens share similarities. 
% However, for higher quantization levels, the difference in entropy between this grouping and the finest-grained grouping becomes more significant. 
% The reason is even if the difference between the groupings is small, quantizing into more discretized values will enlarge the difference. 

% The second-best grouping (per-feature-channel and per-layer $Z$) is used for small quantization levels (e.g., 4-bit or 6-bit). 
% For larger quantization levels (e.g., 8-bit), we still use the finest-grained grouping to maximize compression ratio.



% \jc{too much background of quantization. there's nothing new about the way we use quantization, so just explain how we quantize a tensor with a given bit level, and then move quickly to the question "whether the KV feature of different layers should be quantized with the same level? and why not?"}
%\mypara{Picking level of quantization}




\input{fig-adaptation-case}

\tightsubsection{KV cache streaming adaptation}
\label{subsec:controller}

% \yh{Not clear how we stream? 

% Pseudocode 

% drop the equation 
% }



%The transmission of a KV cache can take from hundreds of milliseconds to a few seconds, during which the network bandwidth may fluctuate.
Since the transmission of a KV cache may take up to 100s of milliseconds to a few seconds, the available bandwidth may fluctuate during a transmission. 
%During the transmission of one context, throughput change can happen as it may take hundreds of milliseconds or several seconds to complete.
Thus, streaming the encoded KV bitstreams at a fixed encoding level\jc{is it compression level or encoding level? please be consistent} may violate a given service-level objective (SLO) of fetching the KV cache.\footnote{In practice, SLO is defined on TTFT. We use SLO for fetching KV cache because once the KV cache of the long context is loaded in GPU, the remaining delay to generate the first token is marginal~\cite{??}.}
In Figure~\ref{fig:adaptation-case}, for example, 
% The throughput drops from 2~Gbps to 0.2~Gbps at 1 second, lasting for 2 seconds, then increases to 1~Gbps, during the transmission of one context. 
at the start of the transmission, the available throughput 
%\footnote{In datacenters, the network bandwidth can achieve 10~Gbps to 100~Gbps}
is 2~Gbps, and if the bandwidth remains at 2~Gbps, sending a KV stream of 1~GB can meet the SLO of 4~seconds.
% given an encoded KV cache of 1~GB and a latency SLO of 4 seconds, transmitting the encoded KV cache will be able to meet the SLO. 
However, at $t=2s$, the throughput drops to 0.2~Gbps and only increases to 1~Gbps at $t=4s$, so the actual transmission delay increases from 4 seconds to 7 seconds, which violates the SLO.

\jc{yuhan, i change the def of context chunks to a chunk of text, rather a chunk of kv bitstream, and each context chunk will be encoded independently into kv bitstreams using the kv encoder. i felt it's more natural. do you agree?}

\mypara{Workflow}
To handle changes in available bandwidth, \name splits a context into multiple {\em context chunks} (or {\bf chunks} for short) of consecutive tokens\footnote{A context chunk may contain multiple {\em groups of tokens} used by the KV encoder to calculate delta tensors (\S\ref{subsec:encoding}).} and uses the KV cache encoder to encode each chunk into multiple bitstreams of different encoding (quantization) levels that can be decoded independently (explained shortly).
This can be done offline. 
When fetching a context, \name sends these chunks one by one, and each chunk can choose one of several {\em streaming configuration} (or {\bf configurations} for short): it can be sent at one of the encoding levels or can be sent in the text format to let the LLM recompute K and V tensors. 

\name adapts the configuration of each chunk while streaming the KV cache to keep the transmission delay within an SLO. 
Figure~\ref{fig:adaptation-case} illustrates an example adaptation where 
%As shown in Figure~\ref{fig:adaptation-case}, to start with, \name decides to send the KV cache. 
\name switches to sending text context and recomputing KV cache from the text at $t=2s$ due to the bandwidth drop, and at $t=4s$, since the bandwidth increases back to 1~Gbps, and \name switch to sending KV bitstreams of subsequent chunks at smaller size. 
With adaptation, \name is able to meet the SLO. 


%At a high level, it splits the KV cache for one context into several \emph{context chunks}, and send the context chunk by chunk.
%Based on the throughput, with the objective of meeting the SLO, \name can adapt the configurations independently for each chunk. 
%The configurations include whether to switch between compression levels of \name's encoded KV caches, or fall back to generate the KV cache from text context from scratch.

% This is based on two insights. 
% First, 
% even if the compression level is different for different chunks, the decoded KV caches are tensors of the \emph{same} shape. 
% Thus, they can be concatenated. 
% Second, the nature of how KV cache is constructed enables the KV cache for one specific chunk to be constructed based on the text of this chunk and the KV cache of all the previous chunks~\cite{dai2019transformer, vaswani2023attention}. 

To adapt efficiently, several questions remain.

%Two of the key questions in the adaptation module lie in how to split the whole context into chunks, and how to adapt to bandwidth fluctuations. 
%The context chunks are created by splitting the key tensor into chunks such that each chunk contains the key tensors for multiple contiguous tokens, and similarly for the value tensor. 
%Each of the chunk contains the number of tokens which is just large enough to fit in one congestion window size, for two reasons.
%One, we want to best utilize the bandwidth by filling up one congestion window, while on the other hand, we also want to provide fine-grained enough granularity to perform 
%adaptation to meet SLO. 
%Note that we also  let the number tokens in one context chunk be integer multiples of the number of tokens in one group in the change-based encoding (\S\ref{sec:}).

% The chunks make the decisions of switching between compression levels or generating KV cache from scratch 

First, {\em how to stream multiple chunks at different streaming configurations without affecting compression efficiency?}
%decode each context chunk independently?} Specifically, why encoding each context chunk separately does not affect compression efficiency
To encode the chunks offline, \name first computes the KV cache of the entire context (\ie prefill) and splits the K and V tensors of the KV cache along the token dimension into sub-tensors, each of which contains the layers and channels of the tokens in the same chunk.
It then uses the KV encoder to encode the K or V sub-tensor of a chunk with different encoding (quantization) levels. 
Each chunk is encoded {\em independent} to other chunks {\em without} affect the compression efficiency as long as a chunk is longer than a group of tokens.
This is because encoding the KV tensor of a token only depends on itself and its delta with the anchor token of the group of tokens (\S\ref{subsec:encoding}).
Thus, chunks sent with different encoding levels can be independently decoded and then concatenated to reconstruct the KV cache. 
In the case that a chunk is sent in text format, the LLM will compute its K and V tensors based on the previous chunk's KV tensors that have been received and decoded.\footnote{A similar concept has been used to split LLM input into prefill chunks for more efficient batching~\cite{sarathi}.}

{\em Would streaming chunks at different configurations affect generation quality?}
If one chunk is sent at a lower encoding level than other chunks\jc{do we call aggressive compression a low or high encoding level?} (due to low bandwidth), it will have high compression loss on {\em that} single chunk, but this will not affect the compression loss of other chunks. 
That said, we acknowledge that if the bandwidth is too low to send most chunks in a high encoding level, the quality will still suffer.


 
%In order to adapt the configuration for each chunk, 
%in the offline stage, we encode each chunk of the KV cache into multiple compression levels, specifically by varying the quantization parameters\footnote{\yh{talk about the parameters }}. 
%The reason why we can encode each chunk separately is that the size of encoding each chunk is the same as encoding the whole KV cache.
%Specifically, since encoding each token depends only on the anchor tokens in the same group (see \S\ref{sec:method}), and we only use different quantization levels for different layers, this chunking will not affect the encoding procedure. 
%% The different versions of encoded KV cache lead to a tradeoff in LLM generation quality and size. 
%Each chunk also has the option of falling back to generating KV from scratch (implementation see \S\ref{subsec:impl}).


Second, {\em how long should a context chunk be?}
We believe that the chunk length depends on two considerations. 
\begin{packedenumerate}
% \item Since the next chunk's configuration is decided after the previous chunk is received, the encoded KV bitstream of a chunk should not be smaller than the sender's congestion control window or we would not fully utilize the network bandwidth.
\item The encoded KV bitstream of a chunk size should not be too big because, otherwise, it cannot react to bandwidth changes in a timely manner.
\item The chunk should not be too small either. If we choose to send a chunk in the text form, the LLM cannot be fully utilized to compute the KV tensors.
\end{packedenumerate}
With these considerations in mind, we empirically pick \fillme tokens as the default chunk length in our experiments\footnote{The chunk length is also long enough for the KV bitstream of each chunk to fill the sender's congestion window in our experiment setting.}, though more optimization may find better chunk lengths.

Finally, {\em how does \name decide the streaming configuration of the next chunk?}
\name chooses the configuration for the next chunk based on the measured throughput when sending the last chunk.
Specifically, \name first assumes the same throughput will remain and calculates the expected delay of each streaming configuration if it is applied to all remaining chunks. 
The delay of sending an encoded KV bitstream is calculated by dividing its size by the throughput (more details in \S\ref{sec:appendix}).
% It then picks the configuration that has the least compression loss (\ie text format or lowest encoding level) with an expected delay still within the remaining time before the SLO, and uses the configuration to send the next chunk.
It then picks the configuration that has the least compression loss (\ie text format or lowest encoding level) with an expected delay still within the SLO, and uses the configuration to send the next chunk.
%Specifically, if the delay to generate KV cache from scratch does not meet the SLO, \name will select the compression level that yields the highest generation quality without violating SLO. 
%Otherwise, \name will fall back to generate KV cache from scratch. 
For the first chunk, if some prior knowledge of the network throughput is available, \name will use it to choose the configuration of the first chunk the same way.
Otherwise, \name starts with \fillme (a medium encoding level). 
%The detailed adaptation logic can be found in \S\ref{sec:appendix}. 

%When sending the first chunk, without much information about the network bandwidth, \name starts with \fillme (a medium encoding level). 
%If some prior knowledge of the network throughput is available, it can be used 
%by sending the first chunk of the KV cache at the compression level with a middle-level size and the entire text context. 
%Upon receiving each chunk, \name chooses the configuration for the next chunk based on the empirical throughput of the last chunk. 
%Concretely, if the delay to generate KV cache from scratch does not meet the SLO, \name will select the compression level that yields the highest generation quality without violating SLO. 
%Otherwise, \name will fall back to generate KV cache from scratch. 
%Note that even if \name may choose the version of encoded KV cache yielding the worst generation quality for one context chunk, we empirically find that the final generation quality will not be significantly affected if the number of chunks sent in low quality is not substantial (see \S\ref{sec:??}).




% \begin{equation*}
% \begin{cases} 
% \text{use text to recompute} & \text{if } T_{\text{text}}(L_{\text{rt}}, L_{\text{ct}}) < SLO, \\
% \underset{Q}{\mathrm{argmax}} \text{ s.t. } T_{\text{kv}}(L_{\text{rt}},Q) < SLO & \text{otherwise.}
% \end{cases}
% \label{eq:adapt}
% \end{equation*}

% In the equation, $L_{rt}$ is the number of tokens yet to be received, $L_{ct}$ is the number of tokens that have already been received. The function $T_{kv}(L_{rt}, Q)$ \footnote{$T_{kv}(L_{rt}, Q) = \frac{\alpha \times Q \times C \times L_{rt} \times L}{Throughput} + RTT$, $\alpha$ is a constant of the model} predicts the delay for transmitting a KV cache with $L$ tokens at compression level $Q$, while $T_{text}(L_{rt}, L_{ct})$ \footnote{$T_{text}(L_{rt}, L_{ct}) = \gamma L_{ct} \times L_{rt}^2$, $\gamma$ is a constant of the model} predicts the delay for generating the KV cache from text. 

% Our adaptation logic chooses the compression level that is predicted to deliver highest quality within the SLO.
% Note that we use the throughput detected by the previous chunk to predict future throughput. While this approach may introduce some error to prediction, the performance stays strong (see \S\ref{sec:??}\hc{Yuhan plz fill}) since datacenter network bandwidths are relatively stable.

% \yh{Several comments: 1. need to explain SLO clearly. 2. split into context-chunks, send chunk-by-chunk, each chunk can make  several actions independently based on throughput to adapt to SLO. 3. how to determine chunk size? How to encode it into several chnks? }


% \jc{i commented out the algorithm pseudocode. it's causing a lot of latex errors, and i don't think we really need a pseudocode to explain it. if it can be clearly explained in fewer words, please do that. a pseudocode is usually a sign that the idea is really complicated}
% \begin{algorithm}
% \caption{Get Function Algorithm}\label{alg:sender}
% \begin{algorithmic}[1]
%     \State $remaining\_SLO \gets SLO$
%     \State $all\_KV \gets None$
%     \For{$i \in \{1..N\}$}
%         \State $is\_text, kv\_quality \gets \Call{GetNextQuality}{i, throughput, remaining\_SLO}$
%         \State $all\_KV \gets all\_KV + \Call{GetNextChunk}{is\_text, kv\_quality, i}$
%     \EndFor
%     \State \Return $all\_KV$
% \end{algorithmic}
% \end{algorithm}




% %So far, we have discussed how the context encoder compresses KV features to reduce the bandwidth needed to transmit the cached KV on-demand. 
% Like any lossy compression, each compressed result of the KV encoder represents a single tradeoff point between the compressed size and the LLM's performance. 
% In practice, however, the best tradeoff depends on the maximum TTFT the application can tolerate.
% To flexibly navigate the size-performance tradeoffs, \name uses a context-loading controller. %, depicted in Figure~\ref{fig:controller}.
% % , which we refer to as the {\em TTFT budget}---a higher TTFT budget means the compression can be less aggressive, \ie less loss on the decompressed KV features, allowing better generation quality.





% The main purpose of \name's controller is to pick the right quantization configuration in order to meet a specific delay budget. 

%As discussed in \S\ref{sec: ??}, \name allows applications to specify a time budget for loading the context. 
%\name will automatically select the quantization levels and loading strategies (\ie either loading the \kv or the text) in order to meet the budget.
%
 
% Specifically, its goal is to minimize
% %Specifically, we formulate the goal of the controller as minimizing 
% degradation of LLM's performance, compared to no compression, while meeting the TTFT budget. 
% \name's controller has two parts.

% First, \name offline compresses the KV cache of each context document at multiple compression levels to cover a range of size-performance tradeoffs.
% %, with larger compressed sizes generally resulting in higher TTFT but better quality.
% %As elaborated in \S\ref{subsec:controller}, having multiple compressed versions is important to fit different TTFT time budget. 
% By default, we pick three quantization settings of $(x,y,z)$: $(8,6,4)$, $(6,4,3)$, and $(5,4,3)$, where $x$, $y$ and $z$ are the number of quantized bits of delta tensor elements at the shallowest 1/3, the middle 1/3, and the deepest 1/3 of transformer layers (defined in \S\ref{subsec:encoding}).
% The quantized tensors are then compressed by AC and stored on the storage server, together with the probability distributions.
% %Note that the probability distributions used by AC are calculated after the quantization and stored on the storage server as well.
% Though these quantization settings empirically work well across a range of LLM models and datasets (\S\ref{subsec:eval:sensitivity}), we believe future work can further refine the quantization scheme to make it more adaptive to LLMs or context distributions.

% We should stress that the compression of each KV cache is {\em offline}, so its delay is not part of the TTFT of loading and processing a context, though decompression of KV features {\em is} still part of TTFT.
% We will evaluate both compression and decompression delays in \S\ref{subsec:eval:micro}.


% %By default, we \jc{explain the default levels here.}


% %\shan{Please remind readers that the compression is done in
% %the background and hence not part of the TTFT, although
% %decompression is part of TTFT.}
% %The different versions of \kv will form a trade-off in size and generation quality, where larger sizes yield better quality. 

% %\jc{need to explain why kv can be compressed offline and refer to the limitation section}

% %beyond a certain length of context tokens, transmitting  \kv becomes faster than calculating them on-the-fly from the text. 

% In runtime, the application provides \name with a prompt (with length $L_{prompt}$) and the selected documents as the context (with length $L_{context}$), the controller then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction1},
% \begin{align}
% {\scalebox{0.94}{$T_{KV}(\Level)=\frac{S_\Level}{B}+C_{decompress}(L_{context})+C_{process}(L_{prompt})$}}
% \label{eq:prediction1}
% \end{align}
% The first term represents the network delay in transferring the compressed KV features: $S_\Level$ is the size of the compressed bitrate of the context at level $\Level$ and $B$ is the estimated bandwidth. 
% %\hc{provided bandwidth in data center?} 
% The second term estimates the decompression of KV features, which is modeled by a {\em linear} function of $L_{context}$.
% The third term is the computation delay of calculating the attention between context and the prompt, which is empirically modeled as a {\em quadratic} function of the prompt length, $L_{prompt}$.
% %$Comp(L_{context},L_{prompt})$ is the estimated computation time, which to decompress and load the KV cache, which is a linear function of $L_{context}$


% In addition, the controller also estimates the TTFT if the context is loaded as raw text as follows:
% \begin{align}
% {\scalebox{0.94}{$T_{text}=RTT+C_{process}(L_{context}+L_{prompt})$}}
% \label{eq:prediction2}
% \end{align}
% The first term is the round-trip-time (RTT) between the storage server and the GPU server.
% We use it to estimate the network delay because the context test is usually small enough to fit in one congestion window size. 
% The second term is the GPU computation to compute the attention from scratch.

% With these delay estimates, the controller can then decide whether it is faster to load the text context or some compressed KV features (and which compression level).
% If the application also specifies a TTFT budget, then the controller can pick the minimum compression level $\Level$ that fits the budget.


% The exact parameters in function $C_{process}$ and $C_{decompress}$ depend on the speed of the inference server, and in our experiments, we record the past compute delays from the same server and interpolate these parameters.
% In this work, we assume the estimated bandwidth $B$ and the estimate of $RTT$ are known beforehand. In practice, they can be obtained by probing or controlled bandwidth in data center~\cite{eyeq, 10.1145/2486001.2486027, 10.1145/2018436.2018465}. And this is beyond the focus of this paper.

% % \todo{Show analytical model to predict ttft here. }


% %When the application provides \name with a prompt (with length $L_{prompt}$), the selected documents as the context (with length $L_{context}$), and the TTFT budget, $T^*$.
% %\name then estimates the TTFT of each compression level $\Level$ using Equation~\ref{eq:prediction}, and picks the minimum compression level $\Level$ that fits the budget ($TTFT_{estimate}<T^*$).
% %\begin{align}
% %TTFT_{estimate}=\frac{S_\Level}{B}+Comp(L_{context},L_{prompt})
% %\label{eq:prediction}
% %\end{align}



% %Thus, \name profiles how the TTFT changes with context token length and records cut-off lengths under various network bandwidths.

% %At runtime, once the applications specify the loading time budget, the controller determines whether to load the text or \kv depending on the estimated network bandwidth and the length of the context.
% %If it decides to load the \kv, then the controller estimates the loading delay with the network bandwidth and the size for each version of \kv.
% %It then selects the \kv version that fits within the time budget while maximizing its size. 

% %In addition to different compression levels, we also include the option of raw text of each potential context document. 
% %Loading the text, as opposed to KV features, makes sense particularly on relatively short contexts, because the
% %decompression time would outweigh the computation time on
% %short text contexts.
% %
% %\jc{remember to explain why picking the compression level doesn't depend on the prompt}

% %\subsection{Putting all together}
% %\yh{todo}
% %\jc{no need for a separate putting it together subsec}



\tightsubsection{Implementation}
\label{subsec:impl}
% \begin{itemize}
% \item basic library info: how many lines of code (a github link?)? ac? quantization? 
% \item integrate with existing apps: how to obtain kv features of a context offline
% \item interface with LLM: e.g., how to get kv features, how to feed kv features
% \item any optimization to improve compression/decompression speed
% \end{itemize}
We implement \name with about 2K lines of code in Python, about 1K lines of CUDA kernel code, based on PyTorch v2.0 and CUDA 12.0. 
% The implementation for each component in our prototype will be discussed shortly. 

\mypara{Quantization, arithmetic coding (AC)}
Following previous work~\cite{llmint8}, we use the \texttt{vectorwise} quantization method, which has been usually used for quantizing model weights.
% and adapt from their open-source codebase to perform quantization.
% The quantization function takes in the tensors to be quantized and the number of discretized symbols after quantization and returns the quantized tensors. % in 8-bit integers. 
% We use this function to quantize delta tensors and the KV of anchor tokens based on our algorithm. 
% \mypara{Arithmetic coding (AC)} 
% We use \texttt{torchac}~\cite{mentzer2019practical}, a CPU-based AC library designed for Pytorch tensors.
% Particularly, we use its encoding and decoding functions to perform AC. 
To speed up encoding and decoding, we implemented a GPU-based AC library with CUDA.
\yh{talk to qizheng about implementation of gpu-based encoder}
Specifically, for decoding each CUDA thread is responsible for decoding the KV cache from bitstreams for one single token. 
The probability distributions are obtained by
counting the frequencies of quantized symbols in the KV feature for the corresponding context.
% \fillme\jc{Yuhan, a sentence here}

\mypara{Integration into LLM inference framework} 
\name operates the LLM through two interfaces
\begin{packeditemize}
    \item \texttt{calculate\_kv(prompt) -> KVCache}: given a new prompt, \name invokes LLM through this function to get the corresponding KV cache.
    \item \texttt{generate\_with\_kv(KVCache) -> text}: \name passes the KV cache to LLM and lets it generate the new text while skipping the attention computation.
\end{packeditemize}
We implemented the above two interfaces for HuggingFace models using \texttt{transformers} library~\cite{???} with \fillme lines of Python code.
Both interfaces are implemented based on the \texttt{generate} function provided by the library.
To ensure LLM only calculate the KV cache without generating new text, we pass \texttt{max\_length} \texttt{= 0} and \texttt{return\_dict\_in\_generate} \texttt{=} \texttt{True}. 
The \texttt{generate\_with\_kv} is implemented by simply passing the KV cache through the \texttt{past\_key\_values} argument when calling the \texttt{generate} function.
Similar integration is also applicable to other LLM libraries, such as FastChat~\cite{zheng2023judging}, llama.cpp~\cite{llamacpp}, and GGML~\cite{ggml}.

We then integrate \name into LangChain~\cite{langchain}, a popular framework for building LLM applications.
\name is activated in the \texttt{\_generate} function of LangChain's \texttt{BaseLLM} module. 
\yc{Yuhan, please help check the correctness of the following workflow}
If the KV cache of the current prompt already exists inside \name, it will invoke \texttt{generate\_with\_kv} to start generating new texts.
Otherwise, \name will first invoke \texttt{calculate\_kv} to get the KV cache before generating new texts.
%Specifically, \name acts as a plugin module, receiving the input prompt, managing the loading of the KV cache, and calling the LLM to generate the response while bypassing the attention computation.
%Thus, \name requires the underlying LLM to provide two interfaces:
%(1) given a new prompt, LLM calculates the KV cache and return it to \name, 
%and (2) given the KV cache (provided by \name), LLM resumes the inference while skipping the attention computation.
%Many recent LLMs support the two functionalities by default. 
%For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.
%\name interacts with LLM inference via two simple interfaces:
%% To apply \name, the model inference pipeline to have incorporate two functionalities: 
%(1) \name extracts the KV features of a given context from an LLM inference, and 
%(2) \name feeds the KV features (which can be the decompressed ones) to resume the LLM inference while skipping the attention computation on the context. 
%Many Pytorch-based LLMs support these APIs. 
%For instance, Huggingface provides these APIs as part of each LLM model's \texttt{forward} method~\cite{wolf-etal-2020-transformers}.

% \jc{Yuhan, is this true?}
% it should  be able to output the \kv for the context being processed, and (2) it should be able to take in the \kv, skips the attention computation to process the \kv for the context, and then generate the first token. 
% The Huggingface's Transformers~\cite{wolf-etal-2020-transformers}, which we build our prototype on top of, does support the above  functionalities for the mainstream models in the model hub. 
% The limitation of using the Transformers library to build our prototype upon is discussed in \S\ref{sec:limitation}.

\mypara{Speed optimization for \name} To speed up the decoding of KV cache in GPU, we pipeline the transmission of context chunk $i$ with the decoding of context chunk $i-1$(explained in \S\ref{subsec:controller}). 
 
% To speed up the decompression of KV features, we parallelize the decompression of delta tensors (explained in \S\ref{subsec:encoding}), running multiple instances of \texttt{torchac} simultaneously.
% We further speed up the loading of decompressed KV features from CPU to GPU by pipelining the loading of layer $i$ with the DNN inference computation of layer $i+1$.


==> sec-problem.tex <==
%!TEX root = main.tex
%!TEX spellcheck = en_US






%\tightsection{KV Cache Streaming}
\vspace{-4pt}
\tightsection{Hidden network bottleneck}
%\tightsection{Hidden network delay of loading the KV cache}
\label{sec:delay}

\begin{comment}
\begin{itemize}
    \item Section 3 KV Cache Streaming
        \begin{itemize}
        \item Section 3.1: Hidden network delay of loading the context 
        \begin{itemize}
            \item One natural way to reuse the context is to store the KV cache and directly load them when needed, like Figure 4b. cite chunkattention etc. 
            \item these prior works assume the KV cache is in the GPU memory of the inference server. However  the KV cache may not necessarily lie on the same server as the inference server. Reason: the background database for retrieval apps is too large to be replicated on each inference server. For chat apps, users may resume the conversation after a long period of time, thus the KV cache will need to be swapped out. List a concrete example
            % \item For example, when users build LLM apps, they usually upload context (in text format) to the storage server, while querying LLMs hosted in a compute server. In these cases, KV cache is on a remote server than the inference one. 
            \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (Cite interdc throughput)
            \item This can be slow because the size of the KV cache is large. And will negate the benefit of reusing KV cache.
            \item We want to make the loading of KV cache for reusing as fast as possible. 
        \end{itemize}
        \item Section 3.2: 
        \begin{itemize}
            \item To make the loading of KV cache as fast as possible, one way to do it is to encode the KV cache to make its size as small as possible, like figure 4c. 
            \item A common way of encoding data transmitted over the network is to encode it into bitstreams. Explain in our case, it would be encoding the original KV cache tensor into bitstreams on the storage server, decoding it back to tensor of original shape on the inference server 
            \item Ideally, the encoder can make the loading delay of KV cache very small  to maximize the benefit of reusing KV cache 
            \item KV cache streaming can also be applied to other scenarios, such as reducing the delay of migrating KV cache in distributed inference setting 
             \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
            % \item Reusing KV cache has some hidden network delays because the KV cache is often stored on a remote server. (List some example scenarios and inter-DC throughput)
            % \item This will negate the benefit of reusing KV cache. 
            % \item We want to make the loading of KV cache for reusing as fast as possible. 
            % \item This is fundamentally different from those prior works that try to enable longer context by text shortening, since the size of KV cache can still be large after text-shortening. 
        \end{itemize}
\end{itemize}

\end{comment}

Although promising in drastically reducing TTFT, recent studies of reusing the KV cache \cite{vllm, chunkattention, promptcache} all rely on the assumption that
%A natural solution to reduce TTFT is to {\em store and reuse the KV cache} of repeated context and hence skip much expensive computation in the prefill phase. Indeed, recent studies (\eg~\cite{vllm, chunkattention, promptcache}) have suggested that by keeping the KV cache of a context and reusing it when the same context is used again, one {\em could} potentially eliminate the prefill delay and significantly reduce TTFT if 
the KV cache to be re-used is locally available in GPU memory. 

\begin{comment}

one can first run the prefill phase of LLM inference on the context, save the K and V tensors in the resulting KV cache, and reuse them in the future if the same context is used again. %, thus eliminating the future prefill delay. % which grows superlinearly with the context length.
As suggested in recent studies (\eg~\cite{vllm, chunkattention, promptcache}), this method can eliminate the future prefill delay, {\em if} the KV cache is {\em already} in the GPU memory when the same context is used again.
\end{comment}

% \jc{somewhere in this section, we need to define TTFT. we don't need much text about it as before, since TTFT is widely used by industry already}

%In this way, the superlinear procedure of prefilling the context can be bypassed. 
%Indeed, several recent studies~\cite{vllm, chunkattention, promptcache} reuse KV cache that is already in GPU memory to speed-up the processing (prefill) of contexts shared across LLM inference requests. 
%These prior works assume the KV cache is stored in the GPU memory.

In practice, however, the reused KV cache of a long context may need to be fetched from another machine(s).
This is because GPU memory is likely not enough to store the KV cache of all repeated contexts. 
For instance, for the Llama-33B model, the KV cache of a 16K-token\footnote{About 12,000 English words or merely one SIGCOMM paper!} context, a common
context length in practice~\cite{bai2023longbench},
is 25~GB, on par with the size of the LLM itself. 
Storing the KV cache on the GPU for a long time will be even more challenging when the model size increases.
%, we can store the KV cache of a fewer number of tokens.
%Thus, GPU memory is unlikely to be enough to store the KV cache of all contexts that might be reused. 
Even in chat-based apps that route all requests of a user to the same GPU, the KV cache of the conservation history may not always be in the GPU memory, especially if the next query from the user comes after several hours, during which the KV cache may have been offloaded to make space for fresh chat sessions.


%Therefore, the KV cache of the reused context must sometimes be fetched from another machine(s), but
However, the network delay for fetching the KV cache can be substantial, yet it has not received enough attention. 
%been largely overlooked.
Existing LLM systems assume that the KV cache is always in GPU memory or that the KV cache is small enough to be retrieved quickly via a high-speed interconnection.
%Yet, the actual network delay to fetch KV cache could \emph{negate} the benefit in saving computation delays from reusing KV cache.
Taking the KV cache size of 25~GB from the previous example, to send it over a 20Gbps link takes 10 seconds whereas running the prefill phase on the text context by the same Llama-34B model takes about the same time. 
Even with a 100Gbps link, sending the KV cache will take 2 seconds, which damages user experience for its long TTFT~\cite{latency_experience1, latency_experience3}.

%\yh{Find a citation that shows TTFT should be below xx> }
In short, we need a solution to reuse KV cache while reducing the network delay to fetch the KV cache.


\begin{comment}

% However, the prior systems assume that either the KV cache is always in GPU memory or the KV cache is small enough to be quickly fetched via a dedicated fast interconnection.
% Unfortunately, {\em the network delay} in fetching the KV cache of long contexts can be substantial in practice.
% may {\em not} always be available in the GPU when reused.
This is because the KV cache of a context can be 3-4 orders of magnitude bigger than the context in text format, so the GPU memory may not be big enough to hold the KV caches of all contexts that might be reused.
% \jc{yuhan, please write something like this: GPU memory is typically below \fillme GB, and even if all of it is used for KV cache produced by \fillme model, we will be able to put in the KV cache of \fillme tokens, which roughly translate to \fillme pages of documents, and for KV cache produced by a \fillme (a bigger model), only the KV cache of \fillme tokens can fit in.}

Popular GPUs used for serving LLMs such as the NVidia A40 or RTX A6000 have a maximum GPU memory of 46-48 GB. A common LLM model such as LLama-33B with 8-bit quantized weights requires around 33 GB of GPU memory~\cite{anyscale_blog}. 
If we devote the entire remaining 13 GB to store the KV cache, we can store a maximum token length of around 8000 tokens. 
Standard tokenizers have a ratio of one word equalling 1.33 tokens~\cite{token_blog}, this translates to 6000 words or 6 pages of text of roughly 1000 words per page. 
Thus in general, storing the KV cache on the GPU is challenging, especially when the model size increases, we can store the KV cache of a fewer number of tokens.

Even for chat-based apps where the KV cache of one conversation can fit in the GPU memory, the KV cache may have to be offloaded before the next user query comes. 
For instance, when a user asks the LLM to generate a long story, then the KV cache of the long story (part of context) will be available in GPU memory right after the generation. 
%becomes the context of subsequent conversations.
%, and the KV cache of this context is available in GPU memory. 
However, if the next query about the story does not come until several hours or days later, the GPU may choose to offload the KV cache of this conversation, so even if the next query is routed to the {\em same} GPU, the KV cache will not be available locally and has to be loaded from another machine.



\end{comment}

% \jc{yuhan, i deleted your old examples, such as 2T tokens, 364 million docs, etc. in generally, these examples are easy to attack and people's first reaction is we are exaggerating since not all of them are needed at once. in generally, try to avoid examples that people can easily attack.
% same logic goes to the example of azure openai storage service being separate. people can easily attack and say the kv cache doesn't have to be colocated with the text.}


\begin{figure}[t]
\centering
     %\includegraphics[width=.99\linewidth]{figs/motivate_baselines_v3.pdf}
     %\includegraphics[width=1.03\linewidth]{figs/motivate_baselines_v3-arial.pdf}
     \includegraphics[width=1.02\linewidth]{figs/motivate_baselines_v3-arial2.pdf}
    \tightcaption{How different ways of loading context affect the network delay (to transfer context or KV cache) and the computation delay (to run the attention module on the context).  } 
     \vspace{-6pt}
    \label{fig:motivate_baselines}
\end{figure}

%in the GPU memory of the GPUs that run the LLM inference. 

\begin{comment}
In retrieval-based applications, the size of KV cache of the related background documents is too big to be replicated locally on \emph{each} GPU server that potentially runs LLM inference jobs. 
For example, one recent work uses a background database containing up to 2 trillion tokens in total, which requires 1 TB of storage to save the documents in text format. 
Similarly, another recent work uses a  database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
Thus, the developers of the LLM applications may upload their data to the cloud storage servers, and query LLMs hosted in the GPUs servers managed by the same cloud service. 
To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may build their database and store it on Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance.
Although storing the KV cache in the storage services is not widely applied in existing LLM applications, we envision this will be a popular practice in the near future. \yh{Missing some evidence here. Maybe say that many popular LLM inference frameworks support KV cache as input? }

For chat-based applications, users may resume their conversation with the LLMs after several days. 
Accordingly, those chat histories need to be swapped out from the GPU memory to save space for other active sessions.
Whenever the chat session is resumed, the cached chat histories are highly likely to be loaded from another GPU server. 
Also, given that the number of active users for chat apps is huge (\eg 180 million active users till now for ChatGPT~\cite{vermeer_2023}), it is difficult to store all of the users' chat histories on every GPU server in the inference 
serving system.  
% \yh{Missing why KV cache is on a remote server}




In these cases, the stored KV cache of the context must be fetched from another machine(s) before being reused, and this network transmission incurs a delay that could \emph{negate} the benefit in saving computation delays from reusing KV cache.
However, this {\em network delay} in fetching the KV cache has been largely overlooked since existing LLM systems assume that the KV cache is always in GPU memory or the KV cache is small enough to be retrieved quickly via a fast GPU interconnection.
For instance, the KV cache produced by the 65-billion Llama model \ga{Stick to one version of the LLama model for the description.}
%\jc{pick a big one.}
of 5K  tokens is two tensors each of the size $5$K (tokens)$\times$8192 (channels)$\times$80 (layers), leading to a total size of 13~GB.
%\jc{4.1GB was a bit small}
With a throughput of 16~Gbps, typical to the full capacity of a inter-datacenter link~\cite{skyplane}, it will take 6.5 seconds to transmit the KV cache. \ga{inter-DC is a bit confusing.} \ga{It would help to give a breakdown of the times, for me to put the 6.5s in context.}
% To put it in perspective, this delay is similar to the prefill delay from scratch, thus almost negating the benefit of reusing KV cache.
As illustrated in Figure~\ref{fig:motivate_baselines}, transmitting the large KV cache (Figure~\ref{fig:motivate_baselines}(b)) can be almost as large as the delay of prefilling from scratch (Figure~\ref{fig:motivate_baselines}(a)),  thus almost negating the benefit of reusing KV cache.
% \jc{try to connect this discussion with fig~\ref{fig:motivate_baselines}}
Even with 100~Gbps throughput, which is typical for RDMA
% \jc{think about specialized infra like RDMA, memcachd, etc}
, transmitting the KV cache can take up to 1000ms.
If we can reduce it down by 3$\times$, it still makes a perceivable difference~\cite{llmperf}.

In summary, we want to reduce the overall delay for loading and processing a given context.
Specifically, we define the overall delay as the time between obtaining the input (the prompt and context) and the
generation of the first token. We refer to it as the
\emph{time-to-first-token} (TTFT), since it measures when the first
token is available for the user. 
As shown by previous studies,
users’ experience can be heavily affected by the TTFT since it
demonstrates the responsiveness of the application.
Importantly, TTFT includes both the {\em network} delay to remotely fetch the context or its KV features and the {\em computation} delay to process the context/KV features and the prompt before decoding the first token.
% TTFT excludes the delay of selecting relevant documents based on prompt because of two reasons: (1) this procedure is handled by another separate DNN or algorithm than the LLM itself, which is not the focus of this paper; (2) this delay has been optimized by recent retrieval-based pipelines~\cite{johnson2017billionscale,atlas, fid, chen2021open} and it is relatively marginally compared to TTFT~\cite{zhang2023hybrid, li2022decoupled}. 

%via a limited bandwidth link.  

\end{comment}



\begin{comment}
In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane, ??}. 
With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
This is because the size of KV cache is large, far larger than the context in raw text context form.
Specifically, 
for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
In contrast, its KV cache produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$5120 (channels)$\times$40 (layers), and the size of KV cache serialized by \texttt{torch.save} is 4.1~GB~\footnote{Assumed saving with 16-bit floating point numbers, which is a standard practice~\cite{??}. }.
Given a throughput of 2~Gbps, transmitting the KV cache over the bandwidth can take 16 seconds. 

In short, fetching large KV cache remotely \emph{negates} the benefit of reusing KV cache in saving computation delays. 
This network bottleneck does not only affect one model. 
As shown in Figure~\ref{fig:size_models}, the size of KV cache of popular LLMs all grows with the input token lengths. 
Thus, we want to make the loading of KV cache for reusing as fast as possible, in order to fully maximize the benefit of reusing KV cache in saving prefill delays. 

\end{comment}

\tightsection{\hspace{-0.0cm}\name: KV Cache Streaming}
\label{sec:streamer}

%\begin{itemize}
%\item what's a kv cache streamer: encode, stream, and decode
%\item how it may help? send a kv cache much faster => faster ttft than prior work. other uses (downplay)
%\item how does it differs from other kv cache compression papers. complementary (top-off) and more compression. deals with bw changes
%\item \name is a concrete design
%\end{itemize}

The need to reduce KV cache transmission delay motivates a new module in LLM systems, which we call a {\em KV cache streamer}.
The KV cache streamer serves three roles: 
\begin{packeditemize}
\item {\em (1) Encoding} a given KV cache into more compact bitstream representations --- {\em KV bitstreams}. This can be done offline. 
\item {\em (2) Streaming} the encoded KV bitstream through a network connection of varying throughput.
\item {\em (3) Decoding} the received KV bitstream into the KV cache.
\end{packeditemize}

At first glance, our KV cache streamer may look similar to recent techniques (\eg~\cite{jiang2023longllmlingua,zhang2023h2o,scissorhand}) that compress long contexts by dropping less important tokens. Yet, they differ in crucial ways:

Those recent techniques aim at reducing the {\em run-time} size of the KV cache to accommodate the
GPU memory-size constraint or LLM input-window constraint, and yet we aim at reducing the {\em transmission-time} size of the KV cache to reduce network delay. 
As a result, previous techniques have to
maintain the KV caches'
shapes of large floating-point tensors so that the shrunk KV caches can be directly consumed by the LLM at the run-time;
meanwhile, they can use information during the generation phase to know which tokens in the context are more 
important to the particular query under processing. 
In contrast, 
%.\footnote{In addition, many techniques select less important tokens for {\em particular query} and do so during the generation process when it is clear which tokens of the context are more important to the query. As a result, they will be less effective or hurt quality when compressing contexts in a way that work for future queries.}
 %; since the compressed KV caches are {\em not} directly consumed by the LLM, 
 we need {\em not}
to maintain the original tensor shapes, and can encode them into more compact bitstreams and adapt their representation to network bandwidth. 
Meanwhile, we have to decide which compression scheme to use before a particular query is processed and hence cannot use information
from the generation phase.
%Moreover, the KV cache streamer can adapt the encoding levels of the bitstreams based on bandwidth to further reduce the TTFT, as we will show in \S\ref{subsec:??}.
%\shan{What does this last sentence mean??} \yh{Rewrote the last sentence. }
%Though KV cache has been widely used, there has been little effort on how to encode KV cache to bitstreams efficiently, or on how to stream KV cache under dynamic network bandwidth to reduce TTFT. 
%The most relevant techniques are those that compresses a long context by dropping less important context tokens (\eg~\cite{llmlingua,h2o}), yet they still keep the large tensor shapes and inevitably degrades the generation quality. 
%\ga{Put in a line on how sub-optimal the existing KV cache systems are.}\ga{The difference is unclear. Lossy vs. lossless? Memory vs. network? Be clear.}\jc{updated the previous paragraph. can you take a look?}
% \jc{remember to introduce TTFT in the last section}

This paper presents {\bf \name}, a concrete design of the KV cache streamer.
First, \name uses a custom KV cache codec (encoder and decoder) to minimize the size of KV bitreams, by embracing several distributional properties of KV cache tensors (\S\ref{subsec:insight}).
This greatly reduces the bandwidth demand to transmit the KV cache, thus directly reducing TTFT. 
Second, when streaming the KV bitstreams under dynamic bandwidth, \name dynamically switches between different encoding levels or computing the KV cache on demand, %, in order to complete the transmission of KV cache under a given deadline with high quality.
in order to keep the TTFT within a given deadline while maintaining a high response quality.
The KV encoding/decoding incurs a negligible compute overhead and is pipelined with network transmission to minimize the impact on end-to-end delay. 

\begin{comment}
If successful, the benefit of \name as a KV cache streamer is two-fold.
First, it greatly reduces the bandwidth demand to transmit the KV cache, thus directly reducing TTFT. 
Second, it can dynamically choose the appropriate compression level (or KV compute on-demand) to ensure that TTFT is within a given deadline while maintaining a high response quality.\footnote{The KV cache streamer could also be used to share KV cache more efficiently across different machines in emerging model-parallelism systems for serving LLMs~\cite{lin2024infinitellm, agrawal2023sarathi,??}. 
%These distributed inference systems may migrate KV cache across GPUs, which can also be optimized by such a streaming system. 
}
%by dynamically choosing the compression level streaming KV cache in order to contain TTFT within a deadline, while maintaining a high response quality.

A KV cache streamer (\name) has a key distinction with the emergent techniques for compressing KV cache.
Through dropping less important tokens from context, these techniques (\eg~\cite{scissorhand,zhang2023h2o,beltagy2020longformer}) 
%and others~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing}.
\jc{yuhan, i dropped the other citations. but maybe we need to add the autoencoder paper?}
enable longer contexts or reduce GPU memory footprint. 
Thus, they optimize how to best use GPU memory to store KV cache, rather than how to transmit KV cache over the network, like \name. \ga{The difference is unclear. Lossy vs. lossless? Memory vs. network? Be clear.}
\name is complementary to these techniques and can be used to transmit any KV cache produced by these methods (see \S\ref{??} for a case study of \name with H2O~\cite{zhang2023h2o}).

\end{comment}

%, because it can be used to stream any KV cache, including the KV cache after these methods drop the unimportant tokens.
%Moreover, it does not tackle the problem of bandwidth adaptation. 
%This line of work adds a separate module in the self-attention module, which  allows it not to connect each pair of tokens, but to select only a subset of them to approximate the effect of connecting each pair. 
%This will make the self-attention operation less compute and memory-intensive, and thus longer sequences can be taken by the LLMs.

\begin{comment}
How to reuse KV cache while minimizing the network delay?
This paper explores a {\em KV cache streaming} module and a concrete design named \name. 
The KV cache streaming module has three logical steps 

%\tightsubsection{KV cache streaming }

One way of making KV cache loading fast is to encode the KV cache and stream it via the network.   
A common way of encoding data transmitted over the network is to encode it into bitstreams. 
In the scenario of KV cache streaming, the streamer encodes the KV cache into bitstreams on the storage server, and decodes it back to the original KV cache for LLM inference, as shown in Figure~\ref{fig:motivate_baselines}c.
Ideally, with such a streamer, the transmission delay, together with the decoding delay, will be much smaller than the delay of computing the KV cache of the context from raw text context, in order to  maximize the benefit of reusing KV cache in terms of computation. 
Furthermore, the streamer should also be able to adapt to dynamic resource allocation and make optimal decisions to stream KV cache differently under resource change. 


Potentially, KV cache streaming can also be applied in other scenarios, such as in distributed inference systems~\cite{lin2024infinitellm, agrawal2023sarathi, ??}. 
These distributed inference systems may migrate KV cache across GPUs, which can also be optimized by such a streaming system. 

This goal is fundamentally different from the prior works that try to enable longer context by text shortening, such as Scissorhands~\cite{scissorhand}, H2O~\cite{zhang2023h2o}, Longformer~\cite{beltagy2020longformer} and many others~\cite{zaheer2021big,roy2020efficient,sukhbaatar2021memories,qiu2020blockwise, wu2022memorizing}. 
This line of work adds a separate module in the self-attention module, which  allows it not to connect each pair of tokens, but to select only a subset of them to approximate the effect of connecting each pair. 
This will make the self-attention operation less compute and memory-intensive, and thus longer sequences can be taken by the LLMs.

\end{comment}


% \yhedit{
% \tightsubsection{Prior works in reducing memory usage of KV cache }
% While we Prior proposals~\cite{scissorhand, zhang2023h2o} have been developed to reduce the runtime GPU memory 
% }

% \tightsection{Hidden network delays of loading contexts}


% % \shan{I suggest making this sub-section a separate section and
% % name it something like ``Understanding the hidden network overhead''. There are several reasons: 1. the current background
% % section is REALLY tooo long. 2. this sub-section is actually not
% % a background. instead, it is an important observation made by us
% % that is backed up by our back-of-envelope calculation and motivates our whole design. I think it is worthwhile to
% % make it a separate section. If it is in background, it sounds
% % more like previous work's observation.}
% Current LLM systems assume that the KV cache is already in the GPU memory (or on the same machine), so they focus on reducing computation delays.
% % \yhedit{It is true that loading KV cache is never the bottleneck if it stores in the local storage accompanied by the GPUs.}\shan{I don't think we 
% % need this sentence. A phrase like ``loading KV cache is never the bottleneck'' sounds very dangerous.}
% In practice, however, the KV cache is {\em not} always in the memory of the GPUs \yhedit{or the local storage on the GPUs} that run the LLM inference. 
% Rather, the context of an LLM input often needs to be fetched {\bf remotely} from another machine(s) \edit{via a limited bandwidth link}. 
% \yhedit{For example, the developers of the LLM applications may upload their data to the cloud storage servers and using LLMs hosted in the GPUs servers managed by the same cloud service. 
% To be more concrete, when developers build LLM applications with Azure OpenAI. Developers may upload their data, such as the KV cache of the context to Azure storage~\cite{blog1, blog2}, while submitting LLM inference queries to the LLMs hosted in an Azure compute instance. \yh{Find another example maybe in chat apps? } 
% % In chat apps, a user may resume his/her conversation with LLM a few days after the last interaction on the same topic. 
% % So, the KV cache of his/her conversation history needs to be swapped out of GPU memory to save space for other active conversations~\cite{orca,shepherd,clockwork}. 
% % The KV cache that is swapped out is likely to be used by a resumed conversation at a different inference server. 
% % \yh{Add another example? }
% In these cases, the KV cache will be transmitted at an inter-datacenter bandwidth, which can typically reach a throughput of 2-10 Gbps~\cite{skyplane}. 
% With this throughput, transmitting the KV cache can become the bottleneck of the end-to-end delay.  
% Specifically, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% In contrast, its KV features produced by the Llama-13B model are two tensors, each with a size of $5$K (tokens)$\times$512 (channels)$\times$40 (layers), and the size of KV features serialized by \texttt{torch.save} is 4.1~GB.
% Given a throughput of 2Gbps, transmitting the KV features over the bandwidth can take 16 seconds. 
% }
% \shan{I appreciate the concrete example and the calculation. But the position of this example and calculation is not good. Particularly, what is the relationship between this example and the next two paragraphs? Is this LLM application a retrieval-based app, or a chat app, or either? Does this discussion of ``upload theor data to the cloud storage'' apply to either or both of the retrieval-based app and chat app? I also feel there are now too much repetition and just too much content on motivation now. Can we merge section 2.2 with this section? I feel we are just repeatedly talk about two types of apps, data used as context, large context, blah blah. five pages of extended motivation and background are tooo long.} 
% % \jc{thanks for adding the new paragraph. right after spelling out the throughput numbers, it would be an opportune time to estimate the transfer delay of KV cache (estimate the KV cache size and then estimate the delay, and then say the delay is actually quite substantial}
% % \yh{Add new motivation to show that KV needs to be fetched from a remote server. }
% % \yh{Per request Bandwidth needs to be within a reasonable range  }
% % \yhedit{To be more concrete, when developers build LLM applications with Azure OpenAI, they may upload their data, such as the KV cache, of the context to the Azure storage~\cite{blog1, blog2}. 
% % In this case, the storage servers may or may not reside in the same data center as the GPU servers which serve the LLM models. 
% % In this case, the context will need to be fetched over a inter-datacenter or a intra-datacenter link, which typically has a throughput of about 5Gbps or 10Gbps~\cite{skyplane}. 
% % Furthermore, when there are many requests sharing the same link, the throughput of each request will be even lower. 
% % \yh{Make it more general, and what's the fundamental reason that makes the context on a different machine than the inference server. and then use some examples like langchain etc. }


% % % In other cases, developers may build their LLM applications with  ~\cite{nimje_2023}
% % }
% % \todo{}

% % \todo{If KV stores at local storage or stored at the same rack, then KV loading is never the bottleneck. However, there are several scenarios where: 1. users upload kv to openai storage, so not in the same DC as LLM. 2. users use langchain to write the code, so data is local on users' side; 3. many users sharing the bandwidth link.  }
% % \todo{More evidences on why context is not in GPU}


% % In retrieval-based apps, the background documents can be hosted on different servers than the LLMs~\cite{li2022decoupled, retro}. 
% % One reason is that background documents can be too big (even in raw texts) to be stored locally on the GPU servers running the LLM.
% % % and the storage server on which LLM inference runs may not have enough space to store them.
% % For example, a recent work~\cite{li2022decoupled} uses a background database that contains 364 Million documents~\cite{2019t5}, requiring 750~GB to store their texts.
% % %and storing these texts can take a space up to around 750 GB. 
% % In another recent work~\cite{retro}, the documents contain up to 2 trillion tokens and require 1~TB of storage.
% % Moreover, the background database may be managed by a different service than the LLM service for proprietary considerations~\cite{li2022decoupled, morgan_stanley_private_cloud}.
% % % \jc{please add some evidence and citations here}
% % % \yh{todo: add more citations for retrieval-based apps}

% % In chat apps, a user may resume her conversation with the LLM a few days after the last interaction. 
% % In these cases, the KV cache of her conversation history may need to be swapped out of GPU memory to save space for other active conversation sessions~\cite{orca,shepherd,clockwork}.
% % % \jc{please add some evidence and citations here}
% % Moreover, a user may issue her prompts to the LLM from different locations at different points.
% % As these prompts can be processed by different machines, the contexts must be remotely fetched.




% %In this work, we assume that the context is stored in a different machine than the GPUs running the LLM



\begin{comment}
\begin{figure}
\centering
     \includegraphics[width=1.\linewidth]{figs/size_models.pdf}
    \tightcaption{The size of the KV features produced by different LLMs grow with input length. 
    We measure the serialized file size returned by torch.save.
%    The size of KV features is reported without compression. 
    % \jc{can you draw BOTH y-axis and x-axis in LOG scale? so the lines are still linear but closer to each other? right now, people may be focusing on the DIFFERENCE between models, rather than their trend :) }
    } 
    \label{fig:size_models}
\end{figure}
\end{comment}


% % As KV features need to be fetched on-demand to the GPUs running the LLM, the latency to transmit them must be added to the end-to-end delay of loading and processing a context, \yhedit{which can be significant when the context is large.
% % Even after applying the text-shortening techniques as mentioned in section~\ref{subsec:cache}, the size of the KV cache can still be a bottleneck in loading. 
% % More concretely, given the original contexts with 5-40K tokens, as in popular datasets~\cite{bai2023longbench, longchat2023}, the KV cache can still be as large as 0.8-6.5 GB for a 13-billion Llama model. }
% % However, the size of a context's KV cache can be orders of magnitudes bigger than the context itself, making network bandwidth a potential bottleneck.

% % To put it in perspective, for a context of 5K tokens, storing each token in int-8 representation needs 5KB. 
% % In contrast, its KV features produced by the Llama-7B model are two tensors, each with a size of $5$K (tokens)$\times$4096 (channels)$\times$32 (layers), and the size of KV features serialized by \texttt{torch.save} is 1.3~GB.
% %(with 32 layers and 4096 channels) can be 1.3~GB. 
% %for a 5K-tokens-long context, the KV features of a LLaMA-7B model with 32 layers and 4096 channels can be 1.3~GB.
% %On the other hand, storing the tokenized text (\ie 5K integers) of the context itself only takes around 5KB.
% % \jc{(1) explain how large it could be in bytes, (2) show a figure of the size vs. \# of tokens on a few example models, (3) how much bigger is it than the text itself?}
% % Given a network bandwidth of 1Gbps, for example, the transmission delay of KV feature over the network bandwidth takes more than 10 seconds. 
% % By contrast, processing the text context by the transformer takes only 5 seconds on an A40 GPU.

% In short, the need to fetch large KV features remotely {\em negates} the benefit of KV cache in saving the computation delays. 
% This network bottleneck does not only affect one model.
% As shown in Figure~\ref{fig:size_models}, the size of KV features of popular LLMs all grows with the input token lengths.



